The supernova cosmology cookbook: Bayesian numerical recipes

Theoretical and observational cosmology have enjoyed a number of significant successes over the last two decades. Cosmic microwave background measurements from the Wilkinson Microwave Anisotropy Probe and Planck, together with large-scale structure and supernova (SN) searches, have put very tight constraints on cosmological parameters. Type Ia supernovae (SNIa) played a central role in the discovery of the accelerated expansion of the Universe, recognised by the Nobel Prize in Physics in 2011. The last decade has seen an enormous increase in the amount of high quality SN observations, with SN catalogues now containing hundreds of objects. This number is expected to increase to thousands in the next few years, as data from next-generation missions, such as the Dark Energy Survey and Large Synoptic Survey Telescope become available. In order to exploit the vast amount of forthcoming high quality data, it is extremely important to develop robust and efficient statistical analysis methods to answer cosmological questions, most notably determining the nature of dark energy. To address these problems my work is based on nested-sampling approaches to parameter estimation and model selection and neural networks for machine-learning. Using advanced Bayesian techniques, I constrain the properties of dark-matter haloes along the SN lines-of-sight via their weak gravitational lensing effects, develop methods for classifying SNe photometrically from their lightcurves, and present results on more general issues associated with constraining cosmological parameters and testing the consistency of different SN compilations.

==> Bibliography/OrderReferences/all-new-new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Introduction}
\label{intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





Since its introduction in 1916~\cite{Einstein:1916vd}, Einstein's theory of General Relativity (GR) has successfully explained the majority of gravity-related phenomena. It reproduces Newtonian dynamics in the weak-gravity limit, makes observable predictions, such as the bending of light by massive objects, and until today it withstands solar system tests to a very high precision. At the same time, containing the scalar curvature of a metric tensor, the Einstein-Hilbert action for GR offers an intuitive geometrical interpretation of the theory and Einstein's field equations can be regarded as capturing the interplay between matter and space-time geometry. 

On scales larger than the solar system, however, astrophysical observations have posed questions that to a large extend remain unanswered in the context of GR. These enigmas include the cosmological constant problem, which we will explain in more detail below, as well as the nature of dark matter. 
While there exists a large variety of promising candidates for dark matter particles in various extensions of the Standard Model of Particle Physics, so far there is no convincing explanation for the smallness of the observed cosmological constant. Unless they eventually both turn out to be resolved on the particle physics side, the severeness of the phenomenological problems challenges GR as the ultimate and complete theory of gravity. Therefore, it is reasonable to investigate the possibility of modifying Einstein's beautiful theory with the goal to provide explanations for the perplexing astrophysical observations. 

Of course, such a modification of the theory of gravity is already heavily constrained from the observational side since it must not alter the well-tested predictions of GR at solar-system scales.  
From a more theoretical perpective, looking for alternatives beyond GR is also motivated by String Theory, the most promising candidate for a quantum theory of gravity. GR itself cannot be promoted into a renormalizable quantum theory; it can at most be an effective theory that requires an ultraviolet (UV) completion. 
String Theory in the UV predicts an effective action at low energies that includes the Einstein-Hilbert term of GR plus higher-curvature corrections, as well as couplings to many fields of different spin. Computing this effective action explicitly in string perturbation theory is tedious but, alternatively, one can choose to search for consistent effective theories in a bottom-up approach. 
Following this strategy reveals that modifying GR is surprisingly difficult; almost any alteration of the Einstein-Hilbert action leads to inconsistencies in the theory. Moreover, the nonlinearities of GR often complicate consistency analyses of suggested modified theories and it happens rather rarely that a modification is proven to be consistent. Finding an alternative theory of gravity without inconsistencies is therefore always an important achievement and it is worth investigating the new theory in detail.

As a field theory, GR describes nonlinear self-interactions of a massless spin-2 excitation. A logical first guess for a modification of this setup would be the addition of a mass term for the spin-2 field. The resulting theory should describe nonlinear interactions of a massive spin-2 field and is commonly referred to as \textit{Massive Gravity}. However, the problem with a massive graviton is that a generic mass term introduces ghosts into the physical spectrum. Ghosts correspond to fields with negative kinetic energy that lead to instabilities at the classical and nonunitarity at the quantum level. In a consistent theory, it is necessary to avoid the presence of ghost-fields which puts severe constraints on the mass term and interaction potential of the spin-2 field.

To summarize, the search for a consistent theory of an interacting massive spin-2 field is motivated by the following question:
\begin{itemize}
\item[] Can a massive graviton explain unresolved puzzles in cosmology? 
\end{itemize}
But due to the difficulty of consistently modifying GR, before we can address this question, we need to answer an even more fundamental one:
\begin{itemize}
\item[] How can we describe massive spin-2 particles in field theory?
\end{itemize}
Even without a cosmological constant or Dark Matter problem, this task is interesting from a purely theoretical point of view: It is well-known how to describe massless and massive particles with spin $<2$ in field theory, and there is no obvious reason why there should not exist a corresponding model for spin 2.

Discussing consistency proofs and special features of recently discovered nonlinear theories for massive spin-2 fields, this thesis is mostly devoted to the latter of the two problems, although basic applications to cosmology are also provided. Before diving into this engrossing new subject we present the history of Massive Gravity, explain the cosmological constant problem and provide the basics of theories with spin-2 fields in the remainder of the introduction.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Historical development}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Finding a consistent theory that describes a massive spin-2 field is an old problem. In the year 1939, Fierz and Pauli wrote down the unique ghost-free mass term for a linearized spin-2 fluctuation~\cite{Fierz:1939ix}. An a priori arbitrary coefficient in the mass term needs to be tuned to a specific value in order to remove inconsistencies. 
About 30 years later, in two independent articles, van Dam and Veltman as well as Zakharov discovered that in the zero-mass limit the Fierz-Pauli theory coupled to sources does not converge to the massless theory~\cite{vanDam:1970vg, Zakharov:1970cc}. Namely, the helicity-zero mode of the massive spin-2 field does not decouple in this limit but gives an additional contribution to the vacuum amplitude of two interacting sources. Therefore, this \textit{vDVZ discontinuity} implies that even a very small graviton mass has significant impact on gravitational interactions between sources. In particular, in the zero-mass limit, GR augmented by the Fierz-Pauli term predicts different gravitational constants for conformal and non-conformal matter. Such a difference would be observable in measurements of the gravitational constant for light bending, whose value in the Fierz-Pauli theory with infinitely small mass differs by 25$\%$ from the one predicted by GR. Observations clearly rule out this possibility and a massive graviton would have been discarded decades ago had Vainshtein not found his famous loophole which suggested that a nonlinear completion of the Fierz-Pauli theory could avoid the vDVZ discontinuity~\cite{Vainshtein:1972sx}. Vainshtein showed that around massive sources the linear approximation loses its validity below a certain distance scale. This \textit{Vainshtein radius} becomes infinitely large in the limit of zero Fierz-Pauli mass and in this case there is no regime where the linear theory is valid. Clearly, such a \textit{Vainshtein mechanism} requires a nonlinear extension of the Fierz-Pauli mass term which, not unexpectedly, generically reintroduces inconsistencies. In fact, already in 1972, Boulware and Deser claimed that any nonlinear completion of Fierz-Pauli theory would exhibit a ghost instability~\cite{Boulware:1972zf, Boulware:1973my}. Their results were trusted and for almost 40 years there was little progress in the field of Massive Gravity. Moreover, in 2005, an analysis by Creminelli et.~al.~that was based on earlier work by Arkani-Hamed et.~al.~\cite{ArkaniHamed:2002sp} seemingly confirmed the unavoidable presence of the Boulware-Deser ghost in any nonlinear extension of the Fierz-Pauli theory.

The peripeteia came in 2010, when de Rham, Gabadadze and Tolley (dRGT) revisited the analysis of Creminelli et.~al.~and discovered a minor sign mistake which unfortunately had a large impact on the paper's final conclusion \cite{deRham:2010ik, deRham:2010kj}. After correcting the sign, they found that it is possible to construct a theory of nonlinear Massive Gravity which is ghost-free in a certain decoupling limit. This alone did not guarantee the consistency of the full theory away from the decoupling limit but, in the following year, their reformulation of the dRGT theory~\cite{Hassan:2011vm} enabled Hassan and Rosen to prove the absence of the Boulware-Deser ghost in a Hamiltonian constraint analysis~\cite{Hassan:2011hr, Hassan:2011ea}. Furthermore, they generalized the dRGT setup, which describes a nonlinearly interacting massive spin-2 field in flat space, to a ghost-free bimetric theory containing nonlinear interactions of a massless and massive spin-2 field in a dynamical background~\cite{Hassan:2011zd}. These works established the first consistent nonlinear theory for massive spin-2 fields. 

%The discovery of a consistent nonlinear theory for massive spin-2 fields opened up a new research area. Of particular interest were classical solutions within the dRGT and the Hassan-Rosen model~\cite{} as well as perturbations around them~\cite{}.

Inconsistent models with bimetric interactions had been considered earlier in the literature, for the first time by Rosen in 1940~\cite{Rosen:1940zz,Rosen:1975kk} and later by Aragone and Deser~\cite{Aragone:1971kh} as well as Isham, Salaam and Strathdee~\cite{Isham:1971gm}. The consistent bimetric model had actually already appeared in \cite{Chamseddine:1978yu} where, however, the ghost issue was not addressed.
Besides these, alternative theories with massive gravitons have also been under investigation. These include the DGP model~\cite{Dvali:2000rv,Dvali:2000hr}, Kaluza-Klein scenarios~\cite{Kaluza:1921tu, Klein:1926tv}, New Massive Gravity~\cite{Bergshoeff:2009hq}, Topological Massive Gravity~\cite{Deser:1981wh,Deser:1982vy} and Lorentz violating models~\cite{ArkaniHamed:2003uy}.











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The cosmological constant problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Einstein's equations, the equations of motion for the metric tensor $\gmn$ that follow from the Einstein-Hilbert action of General Relativity, are of the form
\beqn\label{ee}
R_{\mu\nu}-\frac{1}{2}R\,\gmn=\frac{1}{M_{\mathrm{Pl}}^{2}}T_{\mu\nu}-\Lambda\gmn\,.
\eeqn 
The left-hand side contains the Ricci curvature tensor and scalar of $\gmn$ and hence describes the dynamics of space-time geometry. The right-hand side consists of matter sources with stress energy tensor $T_{\mu\nu}$ to which we have added a cosmological constant term. 

In the absence of local sources, there is still a contribution from the matter sector to Einstein's equations because quantum field theory predicts a vacuum expectation value $\braket{T_{\mu\nu}}$ for the source. In particular, the component $\braket{T_{00}}$ is the vacuum energy density that includes contributions from normal ordering of operators in the Hamiltonian and from expectation values of scalar potentials after symmetry breaking. The size of these contributions depends on the specific model, its symmetry breaking mechanisms and UV cutoff, but generically it certainly satisfies $\braket{T_{00}}>(1\,\text{TeV})^4$. In the worst case, it is as large as the Planck density, $\braket{T_{00}}\sim (10^{18}\text{GeV})^4$. As we will review in chapter~\ref{ch:cosmo}, such a huge value for the vacuum energy density would make the expansion of the universe accelerate at an immense rate. Although in the late 1990's observational data revealed that the cosmological expansion is indeed accelerating~\cite{Riess:1998cb, Perlmutter:1998np}, the vacuum energy density driving this acceleration must be as tiny as $10^{-47}(\text{GeV})^4$. The theoretical prediction and the observed value therefore differ by 60 to 120 orders of magnitude. 

In principle, there is a way to cure the discrepancy by hand: One could simply adjust the free parameter $\Lambda$ in (\ref{ee}) such that it cancels the large number in $\braket{T_{00}}$ up to 60-120 decimal places. Obviously this method of dealing with the difference in observed and measured vacuum energies requires an enormous amount of fine-tuning. Although there is no mathematical inconsistency in this procedure, the inexplicable almost exact cancellation is a thorn in the flesh of most theoretical physicists. 
The \textit{cosmological constant problem} has become one of the greatest challenges of modern theoretical physics and there is a countless number of proposals for solutions in the literature. For a recent review we refer the reader to~\cite{Martin:2012bt}.  


A priori, there is good reason to believe that a theory of Massive Gravity could be a step towards explaining the smallness of the observed vacuum energy. 
The main idea is that a small graviton mass is protected against quantum corrections, which relies on the appearance of a gauge symmetry (namely diffeomorphism invariance) in the zero-mass limit. Contrarily, when the cosmological constant is taken to zero, no such symmetry emerges and hence the value for the vacuum energy is unprotected. A tiny graviton mass is therefore considered less unnatural than a cosmological constant of the same scale. The smallness of the mass parameter would still have to be explained, but once it is small at the classical level, quantum corrections will be of the same order of magnitude and not drive it to the cut-off scale. 
If now, in a Massive Gravity theory, a large vacuum energy $\braket{T_{00}}$ generated on the matter side is somehow ``screened" by a mass term with a small graviton mass in the modified Einstein equations, the effect of the vacuum energy on the acceleration of the cosmological expansion could be small. Despite these promising ideas, it seems that a straightforward screening mechnanism does not exist in the dRGT and Hassan-Rosen models to be considered in this thesis. However, this question is not yet finally settled and, moreover, there appear to exist other interesting possibilities to address the cosmological constant problem. 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Massless and massive field theories}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The modern description of particle physics is based on the extremely successful framework of quantum field theory (QFT). Quantum states that correspond to physical particles are created and annihilated by local operators, or quantum fields, that transform in irreducible unitary representations of the Poincar\'e group which, in turn, characterizes the isometries of the underlying Minkowski space time. According to Wigner's classification~\cite{Wigner:1939cj}, the irreducible unitary representations with non-negative energy can be labelled by two Casimir invariants related to mass and spin (or helicity) of the corresponding particle. 
%It is furthermore important to distinguish between the massless and massive case which correspond to different little groups that leave the particle's four-momentum invariant.  

The construction of a QFT with a Hilbert space of particle states is usually achieved in two steps:  
One begins by writing down a Lagrangian of a consistent classical field theory for which the Hamiltonian is bounded from below. Then one quantizes the theory either in the path integral formalism or by imposing canonical (anti)commutation relations for the fields. The process of quantization can in principle reintroduce inconsistencies that render the theory nonunitary but, if one is lucky, it is possible to avoid these. Then, in the absence of gauge anomalies, there may exist a consistent quantum version of the classical theory. The crucial point is that for the existence of a unitary description of particles in a QFT framework, it is absolutely necessary to start from a classically consistent field theory. 

Apart from the problem of nonunitarity in its quantum version, a classical field theory with a Hamiltonian that is not bounded from below is not even meaningful on its own. The instability allows the field to transfer an infinite amount of energy to other fields it interacts with and hence the theory cannot make any useful predictions. Thus, a Hamiltonian that is bounded from below is required from any feasible field theory (classical or quantum). In particular, one must demand the absence of fields that have wrong signs in front of their mass terms (\textit{tachyons}) or kinetic terms (\textit{ghosts}).  

Consistent classical theories for both massless and massive fields with spin 0, 1/2 and 1 are well-known\footnote{Note also that a consistent classical theory for a massive/massless gravitino with spin 3/2 exists in the form of broken/unbroken supergravity.} and their quantum versions play an important role in theoretical particle physics. In fact, the Standard Model of Particle Physics is a consistent quantum theory of fields with spin~1/2 (fermions), spin~1 (gauge bosons) and spin~0 (Higgs boson). Table~\ref{fttable} displays the structure of Lagrangians for fields of different spin.

\begin{table}[htdp]
\caption{Lagrangians for fields of different spin. The massless theories correspond to setting $m=0$.}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline && \\
spin 0& scalar field $\phi$ & $\mathcal{L}_\phi=-\partial_\mu\phi\partial^\mu\phi-m^2\phi^2$
 \\ &&\\
\hline && \\
spin $\tfrac{1}{2}$&  spinor field $\psi^\alpha$ & $\mathcal{L}_\psi=-\bar{\psi}\gamma^\mu\partial_\mu\psi-m\bar{\psi}\psi$ \\ &&\\
\hline &&\\
spin 1& vector field $A_\mu$& $\mathcal{L}_A=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-\frac{m^2}{2}A^\mu A_\mu$ \\ &&\\
\hline 
\end{tabular}
\end{center}
\label{fttable}
\end{table}%

Compared to its lower-spin companions, spin-2 fields turn out to be much more difficult to handle. The consistent classical theory for a massless spin-2 particle with nonlinear self-interactions is General Relativity. However, when trying to quantize the theory one faces another problem because the Lagrangian for GR is nonrenormalizable. This means that predictions for scattering cross sections contain infinities that cannot be absorbed into perturbatively renormalized coupling constants. Due to this obstruction, GR makes sense only as an effective field theory valid at low energies which is believed to have a consistent, renormalizable completion in the ultraviolet regime. For massive spin-2 fields the situation is even worse: Adding a mass term to the Einstein-Hilbert action of GR generically introduces ghost instabilities that render the theory inconsistent already at the classical level. 

In the following we discuss classical field theories of massless and massive spin-1 and spin-2 particles in more detail. In particular we review the degree-of-freedom counting in these theories using gauge invariances and constraints in the equations of motion. 

















%%%%%%%%%%%%%%%%%%%%%
\subsection{Spin-1}
%%%%%%%%%%%%%%%%%%%%%

Before coming to the more relevant example of linear spin-2 theories, it is instructive to begin by considering spin-1 fields that share several features with their spin-2 analogues. Unlike in the theories for spin-0 and spin-1/2 fields, gauge invariance is needed in the massless case to obtain the correct number of propagating degrees of freedom.
We first discuss the massless vector field that appears in classical electrodynamics and then present the Proca theory for massive spin-1 fields.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Massless theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The theory for a massless spin-1 field $A_\mu(x)$ in flat space is given by Maxwell's Lagrangian,
\beqn
\mathcal{L}_\mathrm{Maxwell}=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-J^\mu A_\mu\,,\qquad F_{\mu\nu}\equiv \partial_\mu A_\nu-\partial_\nu A_\mu\,,
\eeqn
where $J^\mu$ is an external source and indices are contracted with the Minkowski metric $\emn$. 
The equations of motion obtained from varying with respect to $A_\nu$ are
\beqn
\partial^\mu F_{\mu\nu}=J_\nu\,.
\eeqn
Due the identity $\partial^\nu\partial^\mu F_{\mu\nu}=0$, the divergence of the equations implies that the source must be conserved, $\partial^\mu J_\mu=0$.
With the help of this conservation law\footnote{In general, the source is not necessarily conserved off-shell since its conservation is an on-shell constraint. For a Lagrangian with off-shell gauge-invariance we need to require off-shell conservation of $J_\mu$ or, equivalently, off-shell gauge-invariance of the source term $J^\mu A_\mu$.} it can be shown that both the above Lagrangian and the equations are invariant under a U(1) gauge transformation,
\beqn\label{gtso}
A_\mu(x)\longrightarrow A_\mu(x)+\partial_\mu\phi(x)\,,
\eeqn
where $\phi(x)$ is a scalar gauge parameter. The symmetry transformation may be used to choose the Lorenz gauge which is defined through the condition $\partial^\mu A_\mu=0$.
In this gauge the equations of motion reduce to 
\beqn
\Box A_\mu=J_\mu\,,
\eeqn
which is simply a sourced Klein-Gordon equation for a massless field.
However, the gauge is not yet fixed completely because we can still perform gauge transformations~(\ref{gtso}) with $\Box\phi=0$ that do not take us out of the Lorenz gauge. The gauge condition $\partial^\mu A_\mu=0$ together with this residual gauge transformation remove two degrees of freedom from $A_\mu$. In~$d$ dimensions the theory for a massless spin-1 particle therefore propagates $d-2$ degrees of freedom.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Massive theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, let us turn to the massive spin-1 particle. It is described by the Proca Lagrangian,
\beqn
\mathcal{L}_\mathrm{Proca}=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-\frac{m^2}{2}A^\mu A_\mu-J^\mu A_\mu\,.
\eeqn
Clearly, this is the same as Maxwell's Lagrangian with an additional mass term quadratic in the field.
The equations of motion in the Proca theory read 
\beqn
\partial^\mu F_{\mu\nu}-m^2A_\nu=J_\nu\,.
\eeqn
The mass term breaks the above U(1) symmetry and the Lagrangian is no longer gauge invariant. Hence, this time there is no symmetry that can be used to remove redundant components of the field.
On the other hand, taking the divergence of the equations of motion we now obtain a constraint equation that contains the field,
\beqn\label{constAmu}
\partial^\mu A_\mu=-\frac{1}{m^2}\partial^\mu J_\mu\,.
\eeqn
The source is no longer necessarily conserved but, if we anyway assume $\partial^\mu J_\mu=0$, then the constraint corresponds precisely to the above Lorenz gauge condition. Plugging it back into the equations of motion we obtain (for a conserved source)
\beqn
(\Box-m^2)A_\mu=J_\mu\,.
\eeqn
Thus the massive spin-1 field again satisfies a sourced Klein-Gordon equation. Since one degree of freedom is removed by the constraint, the theory has $d-1$ propagating degrees of freedom.

 








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Spin-2}\label{sec:FP}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Now we are ready to perform the degree-of-freedom counting in the linear spin-2 theory. Once more, we begin with the massless case before turning to the massive Fierz-Pauli theory. Eventually, we draw the connection between the linear massless theory and nonlinear General Relativity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear massless theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The Lagrangian for a massless spin-2 field in flat space to quadratic order in the field reads
\beqn\label{masslesslin}
\mathcal{L}_\mathrm{lin}=h^{\mu\nu}\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}-\kappa h^{\mu\nu} T_{\mu\nu}\,,
\eeqn
where $T^{\mu\nu}$ is an external source and the structure of the kinetic terms is captured by the two-derivative operator,
\begin{align}\label{kinstruc1}
	\mathcal{E}_{\mu\nu}^{\phantom\mu\phantom\nu\rho\sigma} = \tfrac{1}{2}\Big(
	\eta_\mu^{\phantom\mu\rho}\eta_\nu^{\phantom\nu\sigma}\Box
	&-\eta_\nu^{\phantom\nu\sigma}\partial_\mu\partial^\rho
	-\eta_\mu^{\phantom\mu\sigma}\partial_\nu\partial^\rho\nn\\
	&+\eta_{\mu\nu} \partial^\sigma\partial^\rho
	+\eta^{\rho\sigma}\partial_\mu\partial_\nu
	-\eta^{\rho\sigma}\eta_{\mu\nu}\Box\Big)
	\,. 
\end{align}
The corresponding equations of motion are 
\beqn
\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}=\frac{\kappa}{2} T_{\mu\nu}\,.
\eeqn
The linear Bianchi identity, $\partial^\mu \mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}=0$, implies conservation of the source, $\partial^\mu T_{\mu\nu}=0$. Using this it can easily be verified that the Lagrangian and equations for the massless spin-2 particle are invariant under the following gauge transformations,
\beqn\label{lindiff}
\hmn(x)\longrightarrow \hmn(x) + \partial_\mu\xi_\nu(x)+\partial_\nu\xi_\mu(x)\,,
\eeqn
with vector gauge parameter $\xi_\mu(x)$. As in the spin-1 case, we can use this symmetry to pick a convenient gauge. The Lorenz gauge condition for the spin-2 field is $\partial^\mu\hmn-\frac{1}{2}\partial_\nu h=0$, and, in this gauge, the equations of motion can be written as
\beqn
\Box\hmn=\kappa T_{\mu\nu}-\frac{\kappa}{d-2}T\,.
\eeqn
Again, there exist residual gauge transformations, namely those with $\Box\xi_\mu=0$, that leave the Lorenz gauge intact and correspond to further redundant degrees of freedom.
In total, gauge invariance therefore removes $2d$ of the $d(d+1)/2$ components in $\hmn$, and the only propagating modes are the $d(d-3)/2$ degrees of freedom of a massless spin-2 particle.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear massive theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As has been known since the work of Fierz and Pauli from 1939~\cite{Fierz:1939ix}, the quadratic Lagrangian for a massive spin-2 particle in flat space has the form
\beqn\label{FPlag}
\mathcal{L}_\mathrm{FP}=h^{\mu\nu}\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}-\frac{m_\mathrm{FP}^2}{2}(h^{\mu\nu}\hmn-h^2)-\kappa h^{\mu\nu} T_{\mu\nu}\,,
\eeqn
where the kinetic operator is the same as in the massless case, given by (\ref{kinstruc1}).
The equations of motion obtained from the Lagrangian for the massive particle are
\beqn
\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}-\frac{m_\mathrm{FP}^2}{2}(\hmn-\emn h)=\frac{\kappa}{2} T_{\mu\nu}\,.
\eeqn
The mass term breaks the gauge invariance of the massless theory but, as a consequence of the linearized Bianchi identity, the divergence and trace of these equations give rise to $d+1$ constraints,
\beqn\label{twoconstr}
\partial^\mu \hmn-\partial_\nu h&=&-\frac{\kappa}{m_\mathrm{FP}^2}\partial_\mu T^{\mu\nu}\,,\nn\\
h&=&\frac{1}{d-1}\frac{\kappa}{m_\mathrm{FP}^2}T+\frac{d-2}{d-1}\frac{\kappa}{m_\mathrm{FP}^4}\partial^\nu\partial^\mu T_{\mu\nu}\,.
\eeqn
The source is not necessarily conserved but we shall anyway assume $\partial_\mu T^{\mu\nu}=0$.
Then, unlike in the spin-1 example, the constraint equation obtained from taking the divergence of the equations of motion does not resemble the Lorenz gauge condition but differs by a factor of $1/2$ in front of the trace. For vanishing sources, the constraints imply that the massive spin-2 field is transverse and traceless. 

Using (\ref{twoconstr}) in the equations of motion, we arrive at
\beqn
(\Box-m_\mathrm{FP}^2)\hmn=\kappa\left(T_{\mu\nu}-\frac{1}{d-1}\left[\eta_{\mu\nu}-\frac{1}{m_\mathrm{FP}^2}\partial_\mu\partial_\nu T\right]\right) \,.
\eeqn
Therefore the massive spin-2 field also satisfies a sourced Klein-Gordon equation.
The constraints (\ref{twoconstr}) remove $d+1$ of the $d(d+1)/2$ components in $\hmn$, leaving us with the $d(d-1)/2-1$ propagating degrees of freedom of a massive spin-2 particle. 

An important observation is that modifying the structure of the mass term, i.e.~changing the numerical factor in front of $h^2$ in (\ref{FPlag}), introduces an additional degree of freedom into the theory. This happens because the trace constraint in (\ref{twoconstr}) is lost and $h$ satisfies a dynamical equation of motion instead. It can also be shown that the propagator corresponding to the extra degree of freedom comes with a residue of the wrong sign and therefore gives rise to a ghost instability. This unwanted dynamical field is referred to as the \textit{Boulware-Deser-ghost}. It is this ghost mode that complicates the construction of a nonlinear interaction potential for a spin-2 field because, even when banned from the linear theory, the ghost notoriously reappears through the higher-order interactions.

On the other hand, tuning the linear mass potential to the Fierz-Pauli structure comes with its own problems that threaten the phenomenological viability of the theory as a modification of general relativity. Namely, as already mentioned, it was shown by van Dam, Veltman and Zakharov (vDVZ) \cite{vanDam:1970vg, Zakharov:1970cc} that the $m_\mathrm{FP}\rightarrow 0$ limit of linear massive gravity is discontinuous. More precisely, the helicity-zero mode does not decouple from the sources in this limit and gives an extra contribution to the gravitational force for matter sources whose stress-energy tensors has nonvanishing trace. This leads to a substantial difference between the interactions of massive objects and massless particles, such as photons. This difference can be tested, for instance, by observing light bending by heavy objects. Such tests clearly rule out the existence of a vDVZ discontinuity.

Fortunately, it has been demonstrated by Vainshtein in that nonlinear self-interaction for the spin-2 field may be able to cure this problem~\cite{Vainshtein:1972sx}: The nonlinear theory becomes strongly coupled and the linear approximation breaks down at disctance scales smaller than the \textit{Vainshtein radius}. This radius is large for small $m_\mathrm{FP}$ and goes to infinity in the zero-mass limit. If it is large enough then, although beyond it the linear theory is valid, the vDVZ discontinuity cannot be observed.  
The existence of such a \textit{Vainshtein mechanism} requires a nonlinear completion of the Fierz-Pauli mass term which is one of the main motivations for the construction of a nonlinear theory of Massive Gravity.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Nonlinear massless theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To conclude the introduction, we outline the relation between the linear theory for massless spin-2 fields discussed above and Einstein's General Relativity.
The graviton in GR is a massless spin-2 particle and should hence be described by the Lagrangian~(\ref{masslesslin}). However, the equivalence principle tells us that the field should couple to all kinds of energy in the same manner, including its own stress-energy tensor. Implementing this requirement in~(\ref{masslesslin}) iteratively introduces nonlinearities and eventually leads to the Einstein-Hilbert action for GR.
In turn, the quadratic Lagrangian for a massless spin-2 particle follows from linearizing the Einstein-Hilbert action,
\beqn\label{EHGR}
S_{\mathrm{GR}}=M_{\mathrm{Pl}}^{d-2}\int \mathrm{d}^dx\,\sqrt{-g}~R ~+ \int \mathrm{d}^dx\,\sqrt{-g}~\mathcal{L}_\mathrm{m} \,,
\eeqn
in the perturbation $\hmn=\kappa^{-1}(\gmn-\emn)$ with $\kappa=M^{(2-d)/2}_{\mathrm{Pl}}$. The source is related to the matter Lagrangian~$\mathcal{L}_\mathrm{m}$ through the definition of the stress-energy tensor,
\beqn
T_{\mu\nu}\equiv-\frac{1}{\sqrt{-g}}\frac{\partial(\sqrt{-g}\,\mathcal{L}_\mathrm{m})}{\partial g^{\mu\nu}}\,.
\eeqn
The Einstein-Hilbert action is the gauge invariant nonlinear extension\footnote{One can also include self-interactions into the theory for the massless spin-1 field considered above. In order for the field to remain massless, these interactions must respect gauge invariance and this requirement leads to the structure of Yang-Mills theories~\cite{Henneaux:1997bm}. In the quantum theory, giving mass to non-Abelian spin-1 fields in a unitary and renormalizable way requires a Higgs mechanism, see e.g.~\cite{Ruegg:2003ps}.} of~(\ref{masslesslin}). It can be defined uniquely, as the field theory that describes nonlinear self-interactions of a massless spin-2 particle \cite{Hinterbichler:2011tt}. The gauge transformations~(\ref{lindiff}) are linearized general coordinate transformations (GCTs), under which the metric at the nonlinear level transforms as
\beqn
\gmn\longrightarrow\gmn+\nabla_\mu\xi_\nu+\nabla_\nu\xi_\mu\,.
\eeqn
The presence of a gauge symmetry at the nonlinear level ensures that the full theory propagates the same number of degrees of freedom as its linear version.

Naturally, the existence of a nonlinear closed form for the kinetic terms of a spin-2 particle motivates the search for a nonlinear completion of the Fierz-Pauli mass term. As we saw above, consistency of linearized Massive Gravity requires tuning of a coefficient in the mass potential. One can therefore expect that a consistent (i.e.~ghost-free) nonlinear potential cannot contain arbitrary interaction terms, but that the coefficients of certain terms will be related to each other by demanding the absence of the extra degree of freedom. We shall see in the next chapter that this is precisely what happens. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\chapter{Consistent Nonlinear Massive Gravity}
\label{ch:MG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

In this chapter we introduce the recently discovered consistent theory of nonlinear Massive Gravity. Its nonlinear interaction potential is the unique ghost-free completion of the Fierz-Pauli mass term and contains $(d-2)$ independent parameters in $d$ dimensions. Proving the consistency of the theory in two different formulations was the purpose of {\protect{\hyperref[papI]{Paper~I}}} and~{\protect{\hyperref[papIII]{III}}}.

We begin the discussion by pointing out some general features of nonlinear spin-2 interactions, emphasizing the necessity of a second rank-2 tensor in the theory.
Afterwards, we use insights from the Hamiltonian formulation of General Relativity to construct the ghost-free nonlinear mass potential. 
The resulting Massive Gravity action is the model constructed by de Rham, Gabadadze and Tolley (dRGT) in \cite{deRham:2010ik, deRham:2010kj}, generalized to arbitrary backgrounds. 
The interaction term manifestly breaks diffeomorphism invariance which can be restored using St\"uckelberg fields. The consistency proof in the gauge invariant formulation of nonlinear Massive Gravity is subject of the second half of this chapter.



  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\section{Construction of the ghost-free nonlinear theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 This section is devoted to the construction of the dRGT model for nonlinear Massive Gravity~\cite{deRham:2010ik, deRham:2010kj} as well as its generalization to arbitrary backgrounds by Hassan and Rosen~\cite{Hassan:2011vm}.
  The constructive consistency proof presented here is neither part of any of the papers accompanying the thesis nor has it appeared anywhere else in the literature. Nevertheless, it constitutes the most efficient and straightforward way to arrive at the consistent theory. 
Before we come to the proof, it is worthwile to make a few remarks on general properties of spin-2 interaction potentials.
 
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{General remarks on nonlinear interactions}\label{sec:nonlin}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the introduction we considered massless and massive theories for a linear fluctuation $\hmn$ in a fixed Minkowski background $\emn$. In the nonlinear massless theory given by the Einstein-Hilbert action of GR, it was possible to combine the background and the fluctuation into a single field $\gmn$. We would now like to do something similar in the massive case.

What we call a mass term for a rank-2 tensor $\gmn$ must be a scalar density, i.e.~it has to be a nontrivial scalar function $V(g)$ multiplied by the scalar density $\sqrt{-g}$. Obviously, the scalar function $V(g)$ cannot have any loose covariant indices. Moreover, it should not contain any derivatives. But then, the only object at hand to contract the indices of the metric tensor $\gmn$ is the metric itself which, since $g^{\mu\nu}\gmn=d$, leads to a trivial cosmological constant contribution in the action. We conclude that there is no possibility to construct a covariant nonlinear interaction term for a spin-2 field using only one tensor field.\footnote{Note the difference to e.g.~the vector example, where the metric $\gmn$ can be used to contract the indices in nonlinear interaction terms for $A_\mu$ in a nontrivial way. Furthermore, in the massless spin-2 theory this problem did not occur because in the kinetic terms the indices of the metric could be contracted with derivative operators.} 
Hence, we are forced to introduce a second rank-2 tensor, which we shall call $\fmn$ and which can be used to build nonlinear contractions with $\gmn$. The interaction potential will then be given by $\sqrt{-g}$ multiplying a scalar function of $g^{\rho\mu}\fmn$. 
  

In summary, we expect the nonlinear massive gravity action to be of the form,
\beqn\label{mggenact}
S_\mathrm{MG}=\int \mathrm{d}^dx~\sqrt{-g}~\left[M_{\mathrm{Pl}}^{d-2}R(g) - m^d\, V(g^{-1}f)\right]\,,
\eeqn
where $m$ is an arbitrary energy scale that sets the mass of the spin-2 field. In this setup, the second ``metric" $\fmn$ is a fixed background field that needs to be put into the theory by hand. From the viewpoint of field theory this seems unfamiliar because $\fmn$ is not determined by an equation of motion. But, in fact, there is no need to worry about this, since we will resolve this slightly confusing point in the next chapter, when we introduce the fully dynamical bimetric theory that treats $\gmn$ and $\fmn$ on the same footing. For now, let us accept the possibility to work with a fixed reference metric $\fmn$ and investigate the consistency of this class of theories. 

Obviously, a necessary requirement on the interaction potential in (\ref{mggenact}) is that it reduces to the Fierz-Pauli mass term when linearized around flat space (i.e.~with flat reference metric $\fmn$ and flat background for $\gmn$), otherwise it will certainly propagate the Boulware-Deser ghost. As it will turn out in a nonlinear constraint analysis, a generic interaction potential, even if it incorporates the Fierz-Pauli structure around flat space, will reintroduce this extra degree of freedom at the nonlinear level. This is anticipated from a simple degree-of-freedom counting:
The introduction of the interaction potential breaks the diffeomorphism invariance of general relativity. Therefore the $d$ gauge symmetries are lost and the theory generically will propagate $d$ additional degrees of freedom. Since $d(d-3)/2+d=d(d-1)/2$, this does not give the correct number for a massive spin-2 particle, but there is an extra degree of freedom in the theory. This is the nonlinear Boulware-Deser ghost and an extra constraint is needed to remove it from the spectrum of propagating modes. Tuning the linear mass term to the Fierz-Pauli combination ensured the presence of this constraint in the linear theory.
In section~\ref{sec:conspot} we will demonstrate that, in order to obtain an additional constraint and thereby ensure the absence of the ghost, it is necessary to impose strong restrictions on the structure of nonlinear interactions. In fact, demanding the presence of a constraint will fix all but $(d-2)$ coefficients of all possible interaction terms.
 
 
In the construction of the consistent theory, we will follow the approach of Boulware and Deser who studied Massive Gravity in the Hamiltonian formulation~\cite{Boulware:1972zf, Boulware:1973my}. They claimed that, even though it is possible to remove the ghost from the spectrum of propagating modes at the linear level, it will return for any nonlinear interaction terms that are added to the Lagrangian (\ref{FPlag}). In order to show that this result is in fact incorrect, we first need to familiarize us with variables suitable for the Hamiltonian formulation of GR.
   
  
   


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
\subsection{ADM variables for General Relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  




The Hamiltonian formulation of GR traces back to work by Arnowitt, Deser, and Misner (ADM) from 1962~\cite{Arnowitt:1962hi}. The authors decomposed the metric $\gmn$ into a scalar $N$, a symmetric $(d-1)\times (d-1)$ matrix $\gamma_{ij}$, and a vector $N_i$ with $(d-1)$ components as follows: 
\beqn\label{admmetr}
\gmn=\begin{pmatrix}
-N^2+N_i \gamma^{ij}N_j& N_j\\
N_i & \gamma_{ij}
\end{pmatrix}\,,
\eeqn
where $\gamma^{ij}$ denotes the inverse of $\gamma_{ij}$. This parametrization essentially splits the metric into its time ($0\mu$) and spatial ($ij$) components; in $d=4$ it is therefore also referred to as \textit{(3+1)-decomposition}. From (\ref{admmetr}) we can also compute the inverse of the metric,
\beqn\label{invadm}
g^{\mu\nu}=\frac{1}{N^2}\begin{pmatrix}
-1& N^j\\
N^i & N^2\gamma^{ij}-N^iN^j
\end{pmatrix}\,.
\eeqn
It turns out that, in any theory with kinetic structure given by the Einstein-Hilbert term, the $0\mu$-components are nondynamical gauge degrees of freedom because the Ricci scalar of $\gmn$ contains no derivatives of those components. Hence, all of the propagating modes are contained in the spatial metric $\gamma_{ij}$ which has $d(d-1)/2$ independent components. As we will see now, the gauge invariance of GR will reduce the number of propagating degrees of freedom to $d(d-3)/2$, along with the same number of corresponding canonical momenta.


In terms of the ADM variables the Einstein-Hilbert action (\ref{EHGR}) becomes (up to total derivatives that can be discarded) \cite{Arnowitt:1962hi}
\beqn\label{gradm}
S_{\mathrm{GR}}%=M_\mathrm{P}^{d-2}\int \mathrm{d}^4x~\sqrt{-g}~R
=M_\mathrm{P}^{d-2}\int \mathrm{d}^dx~\left(\pi^{ij}\partial_t \gamma_{ij}-NR^0-N_iR^i\right)\,,
\eeqn
where, in terms of the curvature scalar $R_{(d-1)}$ of the metric $\gamma_{ij}$,
\beqn
R^0&=& -\sqrt{\gamma}~ \left[R_{(d-1)} +\gamma^{-1}\left(\frac{1}{2}({\pi^i}_i)^2-\pi^{ij}\pi_{ij}\right)\right] \,,\nonumber\\
R^i&=& -2\partial_j\pi^{ij}.
\eeqn
The conjugate momenta $\pi^{ij}$ of the $d(d-1)/2$ metric components $\gamma_{ij}$ are computed from the GR Lagrangian in the standard way which leads to expressions in terms of derivatives of the $d$-dimensional metric.

As pointed out before, the action (\ref{gradm}) does not contain dynamical terms for the scalar $N$ nor for the vector $N^i$. On top of that, these variables appear only linearly.
Therefore they act as Lagrange multipliers, and their equations of motion do not contain $N$ and $N^i$ themselves. This means that these equations
constitute $d$ primary constraints~$R^\mu=(R^0, R^i)$ on the remaining $d(d-1)$ variables $\gamma_{ij}$ and $\pi^{ij}$. 

According to the theory of constrained Hamiltonian systems,\footnote{For review of this subject see~\cite{Date:2010xr}.} the presence of a gauge symmetry can now be seen in the Poisson algebra of the constraints, $\{R^\mu, R^\nu\}$. Here, the Poisson bracket for functions $A,B$ is defined as
\beqn\label{defpoisb}
\{A(x), B(y)\}\equiv\int \mathrm{d}^3z~\left(  \frac{\delta A(x)}{\delta g_{ij}(z)}\frac{\delta B(y)}{\delta \pi^{ij}(z)} -\frac{\delta A(y)}{\delta \pi^{ij}(z)}\frac{\delta B(x)}{\delta g_{ij}(z)}\right)\,.
\eeqn
The result for the constraint algebra of GR reads~(see e.g.~\cite{Khoury:2011ay})
\beqn
\{R^0(x), R^0(y)\}&=& R^i(y)\frac{\partial}{\partial y^i}\delta^3(x-y)-R^i(x)\frac{\partial}{\partial x^i}\delta^3(x-y)\, , \nonumber\\
\{R_i(x), R_j(y)\}&=& R_i(y)\frac{\partial}{\partial y^j}\delta^3(x-y)-R_j(x)\frac{\partial}{\partial x^i}\delta^3(x-y)\,,\nonumber\\
\{R^0(x), R_i(y)\}&=& -R^0(y)\frac{\partial}{\partial x^i}\delta^3(x-y)\,.
\eeqn
Since these brackets are proportional to the constraints themselves, they vanish on the constraint surface, as they should in the presence of a gauge symmetry. This implies that all $d$ primary constraints will serve to put conditions on the remaining variables $\gamma_{ij}$ and $\pi^{ij}$, while the Lagrange multipliers $N$ and $N^i$ remain undetermined. There will be no secondary constraints because the primary constraints are automatically preserved in time.

After imposing the $d$ conditions on $\gamma_{ij}$ and $\pi^{ij}$, we can still use gauge transformations to remove $d$ more degrees of freedom. In total we therefore end up with $d(d-3)$ variables, corresponding to the helicity states of the massless graviton and their canonical momenta. This shows that, even nonlinearly, GR propagates the correct number of degrees of freedom for describing a massless spin-2 particle.

Note that throughout the above discussion we never actually wrote down the Hamiltonian, but remained in the Lagrangian formulation. In order to investigate the positivity of the energy, this is naturally insufficient, but since here we were only interested in counting degrees of freedom there was no need to work with the Hamiltonian, which can trivially be obtained from (\ref{gradm}). 


        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%         
\subsection{ADM variables for Massive Gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

In a general nonlinearly interacting theory of the form (\ref{mggenact}), the lapse and shift functions $N$ and $N^i$ will still appear without derivatives. However, the interaction potential will in general no longer be linear in these functions. Therefore, their equations of motion, instead of imposing constraints on the remaining variables, will now determine $N$ and $N^i$ themselves. The $d$ gauge constraints are lost and, as already explained in section \ref{sec:nonlin}, the number of propagating modes will now be $d(d-1)/2$, plus the corresponding canonical momenta. These are two phase-space degrees of freedom too many for the theory of a massive spin-2 particle. Moreover, the Hamiltonian of a generic theory will not be positive definite~\cite{Boulware:1972zf, Boulware:1973my}, signaling that the extra propagating mode is a ghost.  
The necessary requirement on a consistent interaction potential is therefore the presence of an additional constraint that removes the nonlinear Boulware-Deser ghost.

In order to investigate the posibility for a potential in~(\ref{mggenact}) that gives rise to a constraint, we first decompose the second rank-2 tensor $f_{\mu\nu}$ into its own ADM variables,
\beqn\label{admf}
f_{\mu\nu}=\begin{pmatrix}
-L^2+L_l \tilde{f}^{lk}L_k& L_j\\
L_i & \tilde{f}_{ij}
\end{pmatrix}\,.
\eeqn
Here, $\tilde{f}^{ij}$ denote the inverse of the $(d-1)\times (d-1)$ matrix $\tilde{f}_{ij}$, $L_i$ is the shift, and $L$ is the lapse of~$f_{\mu\nu}$. 
We furthermore express the measure factor $\sqrt{-g}$ in terms of the lapse $N$ and the determinant $\gamma$ of $\gamma_{ij}$,
\beqn\label{measur}
\sqrt{-g}=N \sqrt{\gamma}\,.
\eeqn
With these expressions at hand, we can write a generic interaction potential in terms of ADM variables,
\beqn
\sqrt{-g}~V(g^{-1}f)=N \sqrt{\gamma}~V(\gamma_{ij}, N, N^i; \tilde{f}_{ij}, L, L^i)\,.
\eeqn
In order to provide a constraint, the right-hand side of this equation needs to be linear in the lapse $N$. In fact, the necessary condition on the potential is slightly weaker than that because the constraint may be obtained after combining several of the equations for $N$ and $N^i$. If there exists a combination of these equations that is independent of $N^i$ and $N$, then this equation will constrain the remaining variables. At the level of the action, this means that we should allow for a field-dependent redefinition of the shift, $N^i\rightarrow n^i$, that renders the Lagrangian linear in the lapse $N$. Certainly, such a redefinition must be linear in $N$ itself since $N^i$ appears linearly in the kinetic term. Furthermore, since the redefined shift $n^i$ is expected to appear in the constraint, it must be fully determined by its own equation of motion which therefore must not depend on $N$.  To summarize, we make two requirements on the potential in terms of the redefined shift $n^i$:
\begin{itemize}
\item[(i)] linearity of the Lagrangian in $N$,
\item[(ii)]  absence of $N$ in the $n^i$ equations of motion.
\end{itemize} 
Next, we observe that the interaction potential already has a factor of $N$ in front coming from the measure factor (\ref{measur}). Hence, in order to satisfy requirement (i), the potential $V(g^{-1}f)$ written in ADM variables must be of the form
\beqn
V(g^{-1}f)=\frac{1}{N}V_1+V_2
\eeqn
where $V_1$ and $V_2$ are functions of $(\gamma_{ij}, n^i; \tilde{f}_{ij}, L, L^i)$, i.e.~independent of~$N$. Recalling the ADM decomposition (\ref{admmetr}) of $\gmn$, it is clear that the only object that has the chance of giving something linear in $1/N$ is the square root of the inverse metric~(\ref{invadm}). We are thus lead to consider a potential~$V$ that is a function of the matrix $S\equiv\sqrt{g^{-1}f}$, defined via $S^2=g^{-1}f$. This square-root matrix has a very nontrivial ADM decomposition and is certainly highly nonlinear in $1/N$. However, we will now make use of the allowed redefinition of the shift $N^i$ in order to write $S$ in the form
\beqn\label{sadm}
S=\frac{1}{N}\mA+\mB\,,
\eeqn
where $\mA$ and $\mB$ are matrix-valued functions of $(\gamma_{ij}, n^i; \tilde{f}_{ij}, L, L^i)$. The redefinition that leads to (\ref{sadm}) as well as the explicit expressions for $\mA$ and $\mB$ can be obtained straightforwardly by the following method: Square the right-hand side of the ansatz (\ref{sadm}) and equate it with the ADM expression for $g^{-1}f$ obtained from (\ref{admmetr}) and (\ref{admf}). Then compare the expressions on both sides order by order in $1/N$ to read off the shift redefinition as well as the matrices $\mA$ and $\mB$.
This derivation is discussed in more detail in {\protect{\hyperref[papI]{Paper~I}}}; here we simply state the result. The redefinition that renders the square-root matrix $S$ linear in $1/N$ takes the rather simple form
\beqn\label{shiftred}
N^i=Ln^i+L^i+N{D^i}_kn^k\,.
\eeqn
The $(d-1)\times(d-1)$ matrix $D$ on the right-hand side is a function of the variables $(\gamma_{ij}, n^i; \tilde{f}_{ij})$. Explicitly, it is given by
\beqn
D=\sqrt{\gamma^{-1}\tilde{f}Q}\,Q^{-1}\,,
\eeqn
where we have defined another matrix $Q$ through
\beqn
{Q^i}_j=x{\delta^i}_j+n^in^k\tilde{f}_{kj}\,,\qquad x=1-n^i\tilde{f}_{ij}n^j\,.
\eeqn
The matrices $\mA$ and $\mB$ then turn out to be
\beqn
\mA=\frac{1}{L\sqrt{x}}
\begin{pmatrix}
a_0&a_j\\
-a_0c^i&-c^ia_j
\end{pmatrix}\,,~~\quad~~
\mB=\sqrt{x}
\begin{pmatrix}
0&0\\
{D^i}_jL^j&{D^i}_j
\end{pmatrix}\,,
\eeqn
in which
\beqn\label{defa}
a_0=L+n^kL_k\,,\qquad a_i=n^kf_{ki}\,,\qquad
c^i=Ln^i+L^i\,.
\eeqn
The form of the redefinition is not entirely unique. In {\protect{\hyperref[papI]{Paper~I}}} we mainly work with a set of variables that slightly differs from the one presented here. This difference does not affect any of the conclusions drawn in the following, but the choice of variables we made here is more suitable for application to bimetric theory in the next chapter.  

Although the above expressions seem rather complicated, what is essential for the construction of the ghost-free potential is the structure of the matrices $\mA$ and $\mB$. Most importantly, $\mA$ has rank one, i.e.~it can be written as the outer product of two vectors,
\beqn\label{vwa}
\mA=v w^\mathrm{T}\,,~~\quad~~\text{where}~~v=\begin{pmatrix}1\\-c^i \end{pmatrix}\,~~\text{and}~~~w=\frac{1}{\sqrt{x}}\begin{pmatrix}a_0\\a^i\end{pmatrix}\,.
\eeqn
Having obtained the suitable ADM expression (\ref{sadm}) for the square-root matrix $S=\sqrt{g^{-1}f}$, we are ready to construct the interactions which give rise to an additional constraint that removes the Boulware-Deser ghost.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%         
\subsection{Construction of the interaction potential}\label{sec:conspot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As explained above, the mass potential has to be a function of the square-root matrix $S=\sqrt{g^{-1}f}=\frac{1}{N}\mA+\mB$, multiplied by $\sqrt{-g}=N\sqrt{\gamma}$\,. We assume this function to be expandable as a Taylor series in $S$. Generically, this will give an expression that is nonlinear in the lapse $N$. 
The only way to ensure linearity in $N$ is to demand the absence of higher powers of~$\frac{1}{N}\mA$ in the expansion. Obviously, the simplest possible term is $\sqrt{-g}~\tr~(\frac{1}{N}\mA+\mB)$. At first sight it seems that all higher powers of $\frac{1}{N}\mA+\mB$ will involve higher powers of~$1/N$. However, due to the special structure of the matrix $\mA$ there is a caveat here:
Since $\mA$ has rank one, it is a projection operator on a one-dimensional subspace. Because of that, there is a unique way of building polynomials of $\frac{1}{N}\mA+\mB$ that are linear in $\frac{1}{N}\mA$. Namely, an antisymmetric product of $\mA$'s will automatically contain only one power of~$\mA$. Let us see how this works in detail. In $d$ dimensions we consider
\beqn\label{potantisym}
V(S)=\sum_{k=0}^d ~b_n~\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d}~{S^{\nu_1}}_{\mu_1}\hdots{S^{\nu_n}}_{\mu_n}\,,
\eeqn
with arbitrary coefficients $b_n$.
Since the simultaneous exchange of $\mu_i$, $\mu_j$ and $\nu_i$, $\nu_j$ only changes the sign of both $\epsilon$-tensors, it leaves the whole term invariant.
Therefore, at $n$th order, the product of $S$'s under the sum can be written in the form,
\beqn
\sum_{l=0}^n {n \choose l}\left(\frac{1}{N}\right)^l   {\mA^{\nu_1}}_{\mu_1}\hdots {\mA^{\nu_l}}_{\mu_l}{\mB^{\nu_{l+1}}}_{\mu_{l+1}}\hdots {\mB^{\nu_n}}_{\mu_n}\,.      
\eeqn
We insert this expression into (\ref{potantisym}) and obtain
\beqn
V(S)=\sum_{n=0}^d b_n\sum_{l=0}^n {n \choose l}\left(\frac{1}{N}\right)^l V_n(\mA,\mB)\,,
\eeqn
with
\beqn
V_n(\mA,\mB)&=&\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d} \nn\\
&~&\hspace{50pt}\cdot~{\mA ^{\nu_1}}_{\mu_1}\hdots {\mA ^{\nu_l}}_{\mu_l}{\mB^{\nu_{l+1}}}_{\mu_{l+1}}\hdots {\mB^{\nu_n}}_{\mu_n}  \nonumber\\
&=&\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d}\nn\\
&~&\hspace{50pt} \cdot~{v ^{\nu_1}}w_{\mu_1}\hdots {v ^{\nu_l}}w_{\mu_l}{\mB^{\nu_{l+1}}}_{\mu_{l+1}}\hdots {\mB^{\nu_n}}_{\mu_n}\,.
\eeqn
Here we have used (\ref{vwa}).
Since all indices of the symmetric product of $v^{\nu_i}$ are contracted with the totally antisymmetric indices of $\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d} $, we find that in $V_n(\mA,\mB)$ only terms with at most one $\mA$ contribute. This is precisely the property that we were looking for.  
We conclude that the most general form of the potential that is linear in $N$ after the redefinition (\ref{shiftred}) is
\beqn
\sqrt{-g}\,\sum_{n=0}^d ~b_n~\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d}~{S^{\nu_1}}_{\mu_1}\hdots{S^{\nu_n}}_{\mu_n}\,,
\eeqn
with $S=\sqrt{g^{-1}f}$. A more convenient way of writing this is by introducing the elementary symmetric polynomials of the matrix $S$ that can be defined through a recursion formula,
\beqn
e_n(S)=\frac{(-1)^{n+1}}{n}\sum_{k=0}^{n-1}(-1)^{k}\tr (S^{n-k})e_k(S)\,,\quad \text{with}~~e_0(S)=1\,.
\eeqn
Properties of the elementary symmetric polynomials are summarized in appendix~\ref{app:el}.
In terms of these the potential takes the simple form,
\beqn\label{potsympol}
\sqrt{-g}~V(S)=\sqrt{-g}\,\sum_{n=0}^d ~\beta_ne_n(S)\,,
\eeqn
where we have introduced the rescaled coefficients $\beta_n=\frac{n!(d-n)!}{2}b_n$. Since the elementary symmetric polynomials also appear in the expansion of the determinant, the above potential can be regarded as a \textit{deformed determinant}. Note in particular that there is only a finite number of terms giving a potential which is linear in $N$. Due to the antisymmetric structure of the interactions, the possible terms are limited by the dimension of space time. Moreover, out of the $d$ parameters $\beta_n$, only $(d-2)$ are truely measuring interaction strengths: Since $e_0(S)=1$, the $\beta_0$-term is simply a cosmological constant. Also, the last term in the sum that is proportional to $\beta_d$ is just a cosmological constant term for $\fmn$ because $e_d(S)=\det S$. It is therefore independent of $\gmn$ and does not contribute to the equation of motion. Nonetheless, we choose to include it in the action because it will become relevant when we give dynamics to $\fmn$ in the next chapter.

As we have argued, (\ref{potsympol}) is the most general potential that satisfies the above criterion (i). We now explain why requirement (ii) follows automatically. Namely, we can write the equations of motion for $n^i$ obtained from the nonlinear massive gravity action $S_\mathrm{MG}$ as
\beqn
\frac{\delta S_\mathrm{MG}}{\delta n^i}=\frac{\delta N^j}{\delta n^i}\frac{\delta S_\mathrm{MG}}{\delta N^j}=0\,.
\eeqn
Observe that these equations can depend on $N$ at most linearly because the action is linear in $N$. But since the redefinition (\ref{shiftred}) is already linear in $N$, so is $\frac{\delta N^j}{\delta n^i}$ and consequently $\frac{\delta S_\mathrm{MG}}{\delta N^j}$ is independent of $N$. Furthermore, $\frac{\delta N^j}{\delta n^i}$ is nonzero since it is the Jacobian of the redefinition. The $n^i$ equations of motion are therefore equivalent to $\frac{\delta S_\mathrm{MG}}{\delta N^j}=0$ which is independent of~$N$. Hence, by constructing a potential that meets requirement (i), we automatically satisfy criterion (ii). This has also been shown explicitly in {\protect{\hyperref[papI]{Paper~I}}}. 
 

To summarize, we have derived the nonlinear massive gravity action equipped with an additional constraint that removes the Boulware-Deser ghost,
\beqn\label{HRMG}
S_\mathrm{MG}=\int \mathrm{d}^dx\,\sqrt{-g}\,\left[M_{\mathrm{Pl}}^{d-2}R(g) -2 m^d\sum_{n=0}^d ~\beta_ne_n\left(S\right)\right]\,,
\eeqn
with $S=\sqrt{g^{-1}f}$. Once the structure of the theory was known, it was also possible to derive the constraint in a purely covariant formulation for some simplifying parameter choices~\cite{Deffayet:2012nr}. 
In the literature, the above action has been widely referred to as the dRGT model. However, it should be stressed that the theory derived by de Rham, Gabadadze and Tolley in \cite{deRham:2010ik, deRham:2010kj} was defined with flat reference metric $\fmn=\emn$ only. The dRGT construction uses St\"uckelberg fields (see section~\ref{sec:stuck}) and is valid only in a certain decoupling limit that strongly relies on the flat reference metric. In contrast, the construction we have presented here is valid for all reference metrics and demonstrates the consistency of the fully nonlinear theory away from any limiting approximation.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The secondary constraint}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The above requirements on the consistent interaction potential were necessary but not sufficient: A secondary constraint is crucial for the absence of the Boulware-Deser ghost because two constraints are needed to remove both the ghost mode and its canonical momentum from the set of dynamical variables.

It was motivated in Paper I that there is in fact a secondary constraint arising from demanding the primary constraint to be constant in time.  In order to compute the time evolution of the constraint one uses the Poisson bracket (\ref{defpoisb}) and the Hamiltonian, which for the above Massive Gravity action is of the form
 \beqn\label{hamsecc}
H=\int \mathrm{d}^{d-1} y~(\mathcal{H}_0-N\mathcal{C})\,.
\eeqn
Here $\mathcal{H}_0$ is independent of $N$ and $\mathcal{C}$ is the Hamiltonian constraint obtained from varying the action with respect to $N$. The time evolution of $\mathcal{C}$ then reads
\beqn\label{seccons}
\frac{\mathrm{d}\mathcal{C}(x)}{\mathrm{d}t}=\{\mathcal{C}(x),H\}=0\,.
\eeqn  
As in the case of the primary constraint, this equation should be independent of $N$, because otherwise it would determine $N$ instead of constraining $\gamma_{ij}$ and $\pi^{ij}$. Inserting~(\ref{seccons}) into~(\ref{hamsecc}) gives
\beqn
\int \mathrm{d}^{d-1} x~\Big(\{\mathcal{C}(x),\mathcal{H}_0(y)\}-N\{\mathcal{C}(x),\mathcal{C}(y)\}\Big)=0\,.
\eeqn  
Since $\mathcal{C}$ and $\mathcal{H}_0$ are independent of $N$, we therefore need the Poisson bracket among the constraints $\{\mathcal{C}(x),\mathcal{C}(y)\}$ to vanish because the secondary constraint cannot depend on $N$. Before this was actually demonstrated to be the case, there had been objections against the theory claiming that $\{\mathcal{C}(x),\mathcal{C}(y)\}$ could be nonzero \cite{Kluson:2011qe}. The issue was resolved when the secondary constraint was eventually shown to exist in a detailed calculation in~\cite{Hassan:2011ea}. With this, the consistency of the nonlinear Massive Gravity action (\ref{HRMG}) was fully proven.




 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%        
\section{Consistency in the St\"uckelberg formulation}\label{sec:stuck}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As stated earlier, the invariance under general coordinate transformations of General Relativity is broken by the mass term for the graviton. This is because the metric $\gmn$ itself transforms as a covariant rank-two tensor under GCTs while the fixed background metric $\fmn$ does not. Therefore objects like $g^{\mu\nu}\fmn$ are not diffeomorphism invariant. However, there exist a method to restore the gauge symmetry in the action: By introducing new gauge degrees of freedom, so-called St\"uckelberg fields, that transform in a certain way under the gauge group, one can rewrite the theory in a manifestly gauge invariant way. In turn, fixing the so-called physical gauge will give back the original action.

While the proof of absence of the Boulware-Deser ghost given in {\protect{\hyperref[papI]{Paper~I}}} was formulated in the gauge-fixed version of massive gravity, i.e.~without introducing the St\"uckelberg fields, it is expected that restoring the gauge invariance does not alter the dynamics of the theory. In fact, since gauge symmetry is merely a redundancy in the description of the underlying physics, the two formulations are completely equivalent. In particular, absence of ghost in the gauge fixed version of Massive Gravity implies that the St\"uckelberg formulation cannot exhibit the instability either.

Nevertheless, before the constraint needed to remove the ghost was computed explicitly in the St\"uckelberg formulation, there had been some confusion regarding this issue. Namely, in \cite{Chamseddine:2011mu, Kluson:2011rt, Kluson:2012gz}, it was claimed that the Boulware-Deser ghost seems to reappear in the gauge invariant theory. If this was true, it would have suggested a flaw in the consistency proof of gauge fixed Massive Gravity. Fortunately, we were eventually able to prove the absence of ghost in the St\"uckelberg formulation in {\protect{\hyperref[papIII]{Paper~III}}}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The St\"uckelberg trick}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
One possibility to reintroduce diffeomorphism invariance in Massive Gravity is to perform a gauge transformation on the dynamical metric~$\gmn$ and treat the gauge parameters as new fields in the action. Under a GCT, $x^\alpha\rightarrow x'^\alpha(x)$, the metric transforms as
\beqn
\gmn(x)\rightarrow\frac{\partial x'^\alpha}{\partial x^\mu}\frac{\partial x'^\beta}{\partial x^\nu}g_{\alpha\beta}(\phi)\,.
\eeqn
After performing this GCT, one interprets the $x'^\alpha$ as dynamical fields. Another equivalent way, that will be more convenient for our purposes, is to mimic this kind of transformation on the reference metric $\fmn$, which, of course, actually does not transform under GCTs.  But since a simultaneous coordinate transformation of $\gmn$ and $\fmn$ would be a symmetry of the Massive Gravity action, instead of transforming $\gmn$ we can choose to perform the transformation on $\fmn$. 
That is to say, we replace $\fmn$ by its covariantized form
\beqn\label{etcov}
\fmn\rightarrow\frac{\partial \varphi^\alpha}{\partial x^\mu}\frac{\partial \varphi^\beta}{\partial x^\nu}\bar{f}_{\alpha\beta}\,.
\eeqn
Here, $\bar{f}_{\alpha\beta}$ is a new fixed background metric that does not transform under the gauge group. The ``coordinates'' $\varphi^\alpha$ are promoted to dynamical fields that transform as scalars under GCTs. Introducing these St\"uckelberg fields ensures that objects such as
\beqn
 \Tr\, (g^{-1}f) =g^{\mu\nu}\frac{\partial \varphi^\alpha}{\partial x^\mu}\frac{\partial \varphi^\beta}{\partial x^\nu}\bar{f}_{\alpha\beta}
 \eeqn
are diffeomorphism invariant. In addition to the equations of motion for the metric $\gmn$, we now also consider the $\varphi^\alpha$ equations and, as we will see below, this system of equations is equivalent to the original $\gmn$ equation without St\"uckelberg fields.
 
Let us expand the St\"uckelberg fields around the identity transformation, which corresponds to considering infinitesimal GCTs,
\beqn
\varphi^\alpha=x^\alpha-\pi^\alpha\,.
\eeqn 
Furthermore, we decompose the perturbations into a transverse and a longitudinal mode,
\beqn\label{decpi}
\pi^\alpha=\hat{\pi}^\alpha+\partial^\alpha\pi\,.
\eeqn
The power of the St\"uckelberg formalism lies in the conjecture that the ghost instability of nonlinear Massive Gravity can be traced back to higher derivative interactions of the $\pi$ fields in flat space, where $\bar{f}_{\alpha\beta}=\eta_{\alpha\beta}$ \cite{ArkaniHamed:2002sp}. This assumption relies on an analogy to the Goldstone equivalence theorem for spin-1 fields \cite{Lee:1977yc, Chanowitz:1985hj}. In that case, the longitudinal modes of the gauge fields have been shown to carry all information needed for computing scattering processes at high energies. Although the theorem has not been proven for the spin-2 case, it is reasonable to start with the assumption of its validity in order to investigate the stability of Massive Gravity in a certain high energy limit. This limit (also referred to as \textit{decoupling limit}) essentially corresponds to setting the metric perturbation to zero and also ignoring all terms involving the transverse components of the St\"uckelberg fields. Then the conjecture of \cite{ArkaniHamed:2002sp} suggests to construct the interaction potential in such a way that there appear no higher-order interactions of the longitudinal modes. Since each of these modes always comes with two derivatives, their interactions generically give rise to higher derivative terms. These can be shown to lead to ghosts and must therefore be avoided in a consistent theory.
The conclusion of an exhaustive analysis in \cite{Creminelli:2005qk} was that avoiding the higher derivative terms was impossible, and once more it seemed that there exists no consistent nonlinear theory for Massive Gravity. However, it turned out that the authors of~\cite{Creminelli:2005qk} had made sign mistake, and after correcting that flaw, de Rham, Gabadadze and Tolley were indeed able to construct a theory without higher-derivative interactions of the $\pi$ fields. The trick they employed was to tune the coefficients of the interaction terms in such a way that the higher derivative terms combined into total derivatives that could be dropped from the action. 
This lead to the nonlinear Massive Gravity action (\ref{HRMG}) with flat $\fmn$ (and limited parameter space since one of the $\beta_n$ was fixed to ensure a flat background solution for $\gmn$). The complete expression for its decoupling limit, including the transverse vector modes in~(\ref{decpi}), was worked out in~\cite{Ondo:2013wka}.
 
Being free of ghost instabilities in the decoupling limit, the dRGT model is definitely a promising candidate for a consistent theory of nonlinear Massive Gravity in flat space. However, consistency of the theory in all its interactions, that is, away from the decoupling limit, is difficult to prove in the St\"uckelberg formulation, in particular for general $\beta_n$ parameters. The main complication arises due to the square-root matrices appearing in the potential. However, as we explain in the following, it is easy to see that the ghost proof of the gauge fixed theory carries over to the gauge invariant mass potential.
Thereafter, in order to support our arguments even further, we demonstrate the consistency of Massive Gravity in the St\"uckelberg formulation explicitly by identifying the constraint that removes the ghost.  



        
                

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{General arguments for consistency}\label{secgenargst}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
The fact that the dynamics remain unaltered in the gauge invariant theory can be demonstrated by considering the equations of motions for the St\"uckelberg fields. After making the replacement (\ref{etcov}) for $f_{\mu\nu}$, the mass potential $V(g,f)$  becomes a function of the scalar fields and their equations of motions read
\beqn\label{varphieoms}
\frac{\delta}{\delta\varphi^A} V(g,\varphi^B)=0\,.
\eeqn
However, this equation will not give rise to any new dynamics because it is, in fact, already implied by the Bianchi constraint of the gauge fixed theory,
\beqn
&~&\nabla^\mu V_{\mu\nu}(g,\varphi^B)=0\,,\nn\\
&~& \text{where}~~~V_{\mu\nu}(g,\varphi^B)\equiv\frac{1}{\sqrt{-g}}\frac{\delta}{\delta g^{\mu\nu}}\left(\sqrt{-g}~ V(g,\varphi^B)\right)\,.
\eeqn
This constraint follows from the divergence of the $\gmn$ equations after using the Bianchi identity $\nabla^\mu G_{\mu\nu}=0$.
In order to see the equivalence, consider a gauge transformation $\delta x^\mu=\xi^\mu$ of the action involving St\"uckelberg fields,
\begin{align}
&\delta S=\int\mathrm{d}^dx\sqrt{-g}\left[\left(\mpl^{d-2} G_{\mu\nu}
-2m^dV_{\mu\nu}\right)\delta g^{\mu\nu}
-2m^d\frac{\delta V}{\delta\varphi^A}\delta\varphi^A\right]\,.
\end{align}
Here $G_{\mu\nu}$ is the Einstein tensor and the variations under the gauge transformation read $\delta g^{\mu\nu}=-2\nabla^{(\mu} \xi^{\nu)}$ and $\delta\varphi^A=-\xi^\mu\partial_\mu\varphi^A$. As the action is invariant under GCTs, integrating by parts and using the Bianchi identity shows that
\beqn\label{coordconst}
\nabla^\mu V_{\mu\nu} = \frac{\delta V}{\delta\varphi^A}\partial_\nu\varphi^A\,,
\eeqn
identically.
Since the St\"uckelberg fields were introduced to mimic nonsingular coordinate transformations, the matrix $\partial_\nu\varphi^A$ is invertible and hence the Bianchi constraint $\nabla^\mu V_{\mu\nu}=0$ is equivalent to the $\varphi^A$ equations of motion~(\ref{varphieoms}). As expected, the redundant gauge degrees of freedom $\varphi^A$ therefore do not introduce new dynamics into the theory.

From these general arguments we thus expect the consistency proof of Paper~I to be valid for both the gauge fixed and the gauge invariant version of Massive Gravity.
Nonetheless there had been some work arguing against the consistency of the action involving St\"uckelberg fields: In \cite{Chamseddine:2011mu} it was claimed that the ghost generically reappears in the St\"uckelberg sector and the author of \cite{Kluson:2011rt, Kluson:2012gz} could not find a constraint to remove the ghost. Although this constraint was shown to be present in a two-dimensional toy model and to fourth order in perturbation theory in four dimensions \cite{deRham:2011rn}, the issue remained unresolved until we performed the full Hamiltonian analysis in Paper~II. The following section summarizes our findings.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%       
\subsection{Hamiltonian analysis}\label{hamstuck}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

For the sake of simplicity, in {\protect{\hyperref[papIII]{Paper~III}}} we restrict the constraint analysis of Massive Gravity with St\"uckelberg fields to an interaction potential with only $\beta_1\neq 0$. The analysis for general $\beta_n$ is much more involved and has not been carried out yet. Also, here we focus on $d=4$ although the results straightforwardly generalize to arbitrary number of space-time dimensions. 

The reason why the so-called \textit{minimal model} with only $\beta_1\neq 0$ is simpler, is that, as has been noticed in \cite{Golovnev:2011aa, Buchbinder:2012wb}, in this case the action involving St\"uckelberg fields is equivalent to
\beqn\label{phistuckact}
S_\Phi=M_\mathrm{g}^2\int \md^4 x\sqrt{-g}\left(R-m^4\left[{\Phi^A}_A+{(\Phi^{-1})^A}_B {{\bf A}^B}_A\right]\right)\,,
\eeqn
where ${{\bf A}^B}_A\equiv g^{\mu\nu}\partial_\mu\varphi^B\partial_\nu\varphi^C\bar{f}_{CA}$ and ${\Phi^A}_B$ is an auxiliary field that has been introduced in order to remove the square root. Integrating out ${\Phi^A}_B$ gives back the original action involving $\sqrt{g^{-1}f}$ with $\beta_1=1$. This formulation of the minimal model greatly simplifies the ADM analysis. 
In the following, we raise and lower indices on the St\"uckelberg fields as well as on the auxiliary field with the background metric $\bar{f}_{AB}$.

Using the ADM variables (\ref{admmetr}) for the metric $\gmn$ and computing the canonical momenta $p_A$ conjugate to the St\"uckelberg fields $\varphi^A$, we obtain the Hamiltonian corresponding to (\ref{phistuckact}),
\beqn
\mathcal{H}=-NR_0-N^iR_i+N\mathcal{H}_T^\mathrm{sc}+N^i\mathcal{H}^\mathrm{sc}_i\,,
\eeqn
in which the first two pieces are the familiar ones coming from the Einstein-Hilbert term and where
\beqn
\mathcal{H}_T^\mathrm{sc}&=&\sqrt{\gamma}M_\mathrm{P}^2m^2\big({\Phi^A}_A+{(\Phi^{-1})^A}_B{V^B}_A\big)+\frac{1}{4m^2M_\mathrm{P}^2\sqrt{\gamma}}\Phi^{AB}p_Ap_B\,, \nonumber\\
\mathcal{H}^\mathrm{sc}_i&=& p_A\partial_i\varphi^A\,.
\eeqn
Here we have also defined 
\beqn\label{defvab}
{V^B}_A\equiv \gamma^{ij}\partial_i\varphi^B\partial_j\varphi^C\bar{f}_{CA}\,.
\eeqn
Note that in this formulation involving the auxiliary field ${\Phi^A}_B$ the Hamiltonian is manifestly linear in $N$ and $N^i$. There is no need for a field redefinition in order to demonstrate the linearity in the lapse. The linearity in $N^i$ is of course due to the fact that we have reintroduced the gauge invariance and now, as in General Relativity, expect to encounter four first class constraints. They can be thought of as removing the St\"uckelberg fields from the set of dynamical variables. Gauge fixing then serves to also remove their canonical momenta. However, the Hamiltonian constraint that is needed to remove the Boulware-Deser ghost mode within the metric $\gamma_{ij}$ is not among the gauge constraints but has to arise separately. Hence, as in the gauge fixed case, a generic theory would be inconsistent and an extra constraint is present only for special choices of the potential. 

The important observation that was missed in \cite{Kluson:2011rt, Kluson:2012gz} is now that, besides the constraints imposed by the equations of motion for $N$ and $N^i$, the 10 equations of motion for the symmetric field $\Phi^{AB}$ actually only determine 9 independent combinations of the $\Phi^{AB}$. One equation is independent of $\Phi^{AB}$ and therefore constrains the remaining variables. The reason for this is the singularity of the matrix ${V^B}_A$ defined in (\ref{defvab}). The equations of motion obtained from varying (\ref{phistuckact}) with respect to $\Phi^{AB}$ read
\beqn\label{capphieom}
%\Psi_{AB}\equiv
\sqrt{\gamma}\,M_\mathrm{P}^2m^2\Big(\bar{f}_{AB}-
(\Phi^{-1})_{AC}V^{CD}(\Phi^{-1})_{DB}\Big)&~&
\nn\\ 
+~\frac{1}{4m^2M_\mathrm{P}^2\sqrt{\gamma}}\,p_A\,p_B&=&0\,.
\eeqn
Being composed of two $3\times 4$ matrices and a $3\times 3$ matrix, ${V^B}_A$ can at most have rank three. The same is true for the combination of matrices $(\Phi^{-1})_{AC}V^{CD}(\Phi^{-1})_{DB}$ that appears in (\ref{capphieom}). A generic $4\times 4$ symmetric matrix of rank-three has only nine independent components and therefore the ten equations of motion for $\Phi^{AB}$ determine only nine independent combinations of $\Phi^{AB}$. The tenth equation serves to constrain the remaining variables.

Moreover, it is straightforward to extract the constraint from~(\ref{capphieom}) by taking the determinant of the equation. Since the determinant of a matrix that does not have full rank is zero, we obtain the following constraint equation,
\beqn\label{cconstrainteq}
\mathcal{C}\equiv\det{\bar{f}}\left(\bar{f}_{AB}\frac{p^Ap^B}{\gamma}+4(m^2M_\mathrm{P}^2)^2\right)\approx 0\,.
\eeqn
This extra constraint is not first class, it does not arise from the presence of a gauge symmetry. Just as in the gauge fixed version of the theory, it is therefore necessary to show the existence of a secondary constraint generated by the time evolution of (\ref{cconstrainteq}). This second constraint is needed to remove the canonical momentum of the ghost. From the general arguments given in section \ref{secgenargst} we know that the secondary constraint has to be there, and it can be found explicitly in a straightforward way. The time evolution of the primary constraint (\ref{cconstrainteq}) is given by the Poisson bracket $\{\mathcal{C}(x),H_\mathrm{tot}\}$, in which the total Hamiltonian reads
\beqn\label{htot2}
H_\mathrm{tot}=\int \mathrm{d}^3 x \left[N(\mathcal{H}_T^\mathrm{sc}-R_0+{\Gamma^A}_{B}{\Psi^B}_A)+N^i(\mathcal{H}^\mathrm{sc}_i-R_i)\right]\,.
\eeqn
In this we have included 10 Lagrange multipliers ${\Gamma^A}_{B}$ that enforce the ${\Phi^A}_B$ equations of motion. In fact, we really need to include only the constraint (\ref{cconstrainteq}), i.e.~add a term $\lambda \mathcal{C}$ with one Lagrange multiplier $\lambda$. The two approaches are equivalent and their connection is discussed in {\protect{\hyperref[papIII]{Paper~III}}}. Here we only give the arguments for the absence of the ghost and its momentum. 

The crucial point that still needs to be proven is that the secondary constraint $\mathcal{C}_2=\{\mathcal{C},H_\mathrm{tot}\}\approx 0$ must be independent of $N$ and $N^i$, or otherwise it would determine the classical value for these fields instead of constraining the canonical momentum of the ghost mode. Fortunately, it is quite straightforward to show that the pieces in $\mathcal{C}_2$ that involve $N^i$ cancel out on-shell. Moreover, all remaining terms in $\mathcal{C}_2$ are proportional to $N$ which can therefore be divided out. Hence the secondary constraint is indeed independent of the lapse and shift. Furthermore, all dependence on the Lagrange multipliers ${\Gamma^A}_{B}$ drops out upon use of the ${\Phi^A}_B$ equations of motion. Plugging in the solutions\footnote{In fact, we never derive these solutions explicitly. All that is needed for the proof are some general relations from linear algebra.} to the ${\Phi^A}_B$ equations therefore leaves us with a constraint on the remaining variables that will remove the ghost momentum,
\beqn
\mathcal{C}_2\approx-2\alpha\gamma^{-{1/2}}\bar{f}{(\Phi^{-1})^B}_{D}\partial_j\varphi^D\gamma^{jk}\nabla^{(f)}_kp_B-\alpha^2  \gamma^{-1/2}\bar{f} \pi\,.
\eeqn
Here, we have defined $\nabla^{(f)}_kp_B=\partial_kp_B-\Gamma^D_{AB}p_D\partial_k\varphi^A$, with $\Gamma^D_{AB}$ being the Levi-Civita connection of the metric~$\bar{f}_{AB}$.

Of course, this proof is valid only for the special parameter choice $\beta_1\neq 0$ and all other~$\beta_n$ equal to zero. But from the general arguments given in section \ref{secgenargst} it should be clear that, although it may be harder to find, a constraint is also present in the St\"uckelberg formulation of the full theory. This proves that nonlinear Massive Gravity is ghost-free both in its gauge-fixed and gauge invariant version.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Consistent Bimetric Theory}
\label{ch:HR}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the previous chapter we dealt with the nonlinear theory for a massive spin-2 field~$\gmn$, embedded in some arbitrary but fixed reference frame, set by a second rank-two tensor $f_{\mu\nu}$. The important question that we are about to address now is whether this reference metric can be given dynamics on its own without reintroducing instabilities. From a field-theoretical point of view this would result in a much more natural setup: All fields in the action would be determined dynamically without the need of fixing any of their values by hand. A priori, since the constraint analysis of {\protect{\hyperref[papI]{Paper~I}}} assumed a fixed reference frame, it is not clear whether the Massive Gravity action with dynamical $\fmn$ will still avoid the Boulware-Deser ghost instability. Certainly, the consistency of the theory with two dynamical metrics will depend on the kinetic structure assumed for the second rank-2 tensor. 

The ADM variables introduced above for the constraint analysis of nonlinear Massive Gravity enabled Hassan and Rosen to demonstrate the possibility of promoting $\fmn$ to a dynamical field by simply adding its own Einstein-Hilbert term to the Massive Gravity action~\cite{Hassan:2011zd}. The resulting theory contains two interacting spin-2 fields, one massive and one massless one, as expected from general arguments \cite{Boulanger:2000rq}. Such theories had been under consideration for a long time (see e.g.~\cite{Rosen:1940zz}, \cite{Isham:1971gm}, \cite{Damour:2002wu}), but never with the correct consistent interaction potential (except for very few accidental exceptions~\cite{Chamseddine:1978yu, Nibbelink:2006sz}). It required the discovery of ghost-free Massive Gravity to find the unique consistent bimetric theory. 


%In recent years, bimetric theories were mainly considered in relation to the dark matter problem \cite{Banados:2008fi, Milgrom:2009gv} and in the context of spontaneous Lorentz symmetry breaking \cite{Berezhiani:2007zf, Blas:2009my}. 
%Furthermore, the consistency of effective Lagrangians for interacting spin-2 fields, that could arise in brane models or string theory, has been investigated in~\cite{PhysRevD.40.1095, Buchbinder:1999be, Buchbinder:1999ar, Damour:2002ws}.









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Hassan-Rosen action}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   

The Hassan-Rosen action for bimetric gravity consists of two Einstein-Hilbert terms for $\gmn$ and $\fmn$ as well as non-derivative interactions between the two tensor fields. The interaction potential is given by (\ref{potsympol}), i.e.~it has exactly the same form as in nonlinear Massive Gravity.
Hence the bimetric action reads
\begin{align}\label{HR}
S_\mathrm{HR}~=~m_g^{d-2}\int \mathrm{d}^dx\,\sqrt{-g}&\,R(g)~+~m_f^{d-2}\int \mathrm{d}^dx\,\sqrt{-f}\,R(f) \nn\\
&-~2 m^d\sum_{n=0}^d ~\beta_ne_n(S)\,.
\end{align}  
Here we used again the definition of the matrix square root, $S=\sqrt{g^{-1}f}$. Moreover, $m_g$,$m_f$ denote the Planck masses for $\gmn$ and $\fmn$, respectively.

Na\"ively, there seems to be a straightforward argument why this action cannot be consistent: Suppose we go backwards and freeze one of the two metrics to rearrive at a theory for one spin-two field $\gmn$ in a fixed background. For example, we could set $f_{\mu\nu}=\emn$ which gives back the dRGT action that is known to be consistent. Contrarily, freezing $\gmn$ leads to an action for $f_{\mu\nu}$ whose interaction potential does not seem to resemble the form that is known to be the only consistent one. One could be lead to conclude that bimetric theory therefore has to be inconsistent. However, it turns out that the elementary symmetric polynomials possess a rather unexpected property,
\beqn\label{symprop}
e_n(S)=e_{d-n}(S^{-1})\cdot\det S\qquad \text{for}\quad n=0,\hdots, d\,.
\eeqn
Owing to these identities, Hassan-Rosen bimetric gravity is invariant under the following discrete symmetry,
\beqn\label{symbg}
\gmn \longleftrightarrow \fmn\,,\quad m_g \longleftrightarrow m_f\,,\quad \beta_n\longrightarrow\beta_{d-n}\,. 
\eeqn
This interchange symmetry guarantees that freezing $\gmn$ also gives back the consistent Massive Gravity theory for $f_{\mu\nu}$. Of course, this observation does not automatically prove that the theory with both $\gmn$ and $f_{\mu\nu}$ taken to be dynamical is consistent. It merely shows that one necessary condition on a consistent bimetric theory is indeed satisfied. The actual consistency can only be proven in an ADM analysis, which has been performed in \cite{Hassan:2011zd}. Since now both metrics are dynamical, there are two potential Boulware-Deser ghosts within the theory, the usual one coming from $g_{\mu\nu}$ and another one coming from $f_{\mu\nu}$. One therefore has to show that the action is linear in both of the lapses~$N$ and~$L$. Furthermore, in contrast to the action for massive gravity, the bimetric action (\ref{HR}) has a gauge symmetry: It is invariant under diffeomorphisms, under which~$\gmn$ and~$\fmn$ transform simultaneously. 
It is therefore expected that the bimetric action, if consistent, should describe the $(d(d-2)-1)$ degrees of freedom of a massive and a massless spin-2 field.

Indeed, in \cite{Hassan:2011zd} it has been shown that the action (\ref{HR}) becomes linear in both of the lapses $N$ and $L$. It further turns out that the action becomes also linear in $L^i$. As in general relativity, the shift vectors of $\fmn$ now give rise to three further constraints. In addition to this, the presence of a secondary constraint for the Hamiltonian constraint has been demonstrated in \cite{Hassan:2011ea}. Both of the Boulware-Deser ghosts are therefore absent and the number of degrees of freedom is $(d(d-2)-1)$, the correct number for a massive and a massless spin-2 field. In section~\ref{sec:massspec}, we will see that at the linear level these mass eigenstates are neither the fluctuations of $\gmn$ nor those of $\fmn$ but a superposition of the two. Before we turn to the mass spectrum, however, we need to address the question of how the metrics should couple to matter.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsubsection{Including matter sources}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

So far, the bimetric action in the form (\ref{HR}) does not take into account couplings of $\gmn$ and $\fmn$ to other fields. For phenomenological purposes the nature of the matter couplings is of great importance. The only presently known couplings that can be added to (\ref{HR}) without reintroducing the ghost instabilities are the standard minimal couplings familiar from general relativity,
\beqn\label{matcoup}
S_\mathrm{m}=\int\dd^dx~\sqrt{-g}\,\mathcal{L}^g_m+\int\dd^dx~\sqrt{-f}\,\mathcal{L}^f_m\,.
\eeqn
Here, $\mathcal{L}^g_m$ and $\mathcal{L}^f_m$ are Lagrangians involving matter fields as well as the respective metrics.
The variations of $S_\mathrm{m}$ define the two stress-energy tensors,
\beqn\label{strente}
T^{g}_{\mu\nu}\equiv-\frac{1}{\sqrt{-g}}\frac{\delta S_\mathrm{m}}{\delta g^{\mu\nu}}\,,\qquad 
T^{f}_{\mu\nu}\equiv-\frac{1}{\sqrt{-f}}\frac{\delta S_\mathrm{m}}{\delta f^{\mu\nu}}\,.
\eeqn
We shall not discuss the phenomenological implications of a second metric coupled to matter. In {\protect{\hyperref[papII]{Paper II}}}, where we derive homogeneous and isotropic solutions to the bimetric equations of motion, we set the matter coupling of $\fmn$ to zero. This is always a consistent choice and results in a theory for a spin-2 field that only couples to matter indirectly through gravity. For recent work dealing with both of the couplings, see~\cite{Akrami:2013ffa}.

   
    
    
    
    
 
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\section{Equations of motion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
    
We now turn to the equations of motions for $\gmn$ and $\fmn$, obtained from the Hassan-Rosen action (\ref{HR}) including the matter couplings (\ref{matcoup}). When computing these, the only complication arises from variation of the square-root matrix $S=\sqrt{g^{-1}f}$. However, since this matrix only appears under the trace, one can make use of $\delta (S^2)=(\delta S)S+S(\delta S)$ to obtain $\delta(\Tr\,S)=\Tr(\delta S)=\tfrac{1}{2}\Tr(S^{-1}\delta (S^2))$, and similarly for higher powers of $S$ under the trace~\cite{Hassan:2011vm}. Then it is easy to derive the equations of motion, wich in terms of the Einstein tensor $\mathcal{G}_{\mu\nu}(g)\equiv R_{\mu\nu}(g)-\frac{1}{2}\gmn R(g)$ read
\beqn
\mathcal{G}_{\mu\nu}(g) + \frac{m^d}{m_g^{d-2}}V^g_{\mu\nu}(g,f)&=&\frac{1}{m_g^{d-2}}T^g_{\mu\nu}\,,\label{geq} \\
\mathcal{G}_{\mu\nu}(f)+\frac{m^d}{m_f^{d-2}}V^f_{\mu\nu}(g,f)&=&\frac{1}{m_f^{d-2}}T^f_{\mu\nu}\,.\label{feq}
\eeqn
The contributions coming from the bimetric interaction potential are of the following form,
\beqn\label{poteom}
V^g_{\mu\nu}(g,f)&\equiv& \sum_{n=0}^{d-1}(-1)^n\beta_n \,g_{\mu\lambda}{\big(Y^{(n)}\big)^\lambda}_{\nu}(S)\,,\nn\\
V^f_{\mu\nu}(g,f)&\equiv&\sum_{n=0}^{d-1}(-1)^n\beta_{d-n} \,f_{\mu\lambda}{\big(Y^{(n)}\big)^\lambda}_{\nu}(S^{-1})\,,
\eeqn
in which the matrix functions ${(Y^{(n)})^\lambda}_{\nu}$ are defined in terms of the elementary symmetric polynomials through
\beqn\label{defY}
{\big(Y^{(n)}\big)^\lambda}_{\nu}(S)=\sum_{k=0}^n(-1)^ke_k(S){(S^{n-k})^\lambda}_{\nu}\,.
\eeqn
An immediate consequence of the interchange symmetry (\ref{symbg}) in the bimetric action, which of course carries over to the equations of motion, is the identity $V^f_{\mu\nu}(g,f; \beta_{d-n})=V^g_{\mu\nu}(f,g, ; \beta_{n})$.

Note that in nonlinear Massive Gravity with fixed reference metric $\fmn$, there is only one equation of motion for $\gmn$, given by (\ref{geq}).
In contrast, bimetric gravity has two sets of equations of motion and is therefore much more constrained. Moreover, the $\beta_4$-term enters the $\fmn$ equation and is thus no longer nondynamical but rather appears as a cosmological constant term in the equation for $\fmn$. We will have to say more about the important differences between the two theories in section~(\ref{sec:MGlim}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bianchi constraints}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $\nabla$ and $\tilde{\nabla}$ denote the covariant derivatives compatible with the metrics $\gmn$ and $\fmn$, respectively. In General Relativity without interaction term, covariant conservation of the stress-energy tensor, $\nabla^\mu T^{g}_{\mu\nu}=0$, is a consequence of the equations of motion because the Einstein tensor satisfies the Bianchi identity $\nabla^\mu \mathcal{G}_{\mu\nu}=0$. In other words, a massless spin-2 field can only couple to conserved matter sources. In bimetric gravity the condition is weaker: Invariance of the interaction potential under simultaneous diffeomorphisms of $\gmn$ and $\fmn$ implies 
\beqn\label{bicog}
\sqrt{-g}\,\nabla^\mu V^g_{\mu\nu}+\sqrt{-f}\,\tilde{\nabla}^\mu V^f_{\mu\nu}=0\,.
\eeqn
The constraint on the sources enforced by the equations of motion then reads
\beqn
\sqrt{-g}\,\nabla^\mu T^{g}_{\mu\nu}+\sqrt{-f}\,\tilde{\nabla}^\mu T^{f}_{\mu\nu}=0,
\eeqn
meaning that in bimetric gravity the two source contributions are not forced to be separately conserved by the equations. 
Nevertheless, we shall always assume their separate conservation, that is $\nabla^\mu T^{g}_{\mu\nu}=\tilde{\nabla}^\mu T^{f}_{\mu\nu}=0$. This is equivalent to imposing the separate invariance of the two matter Lagrangians $\mathcal{L}^g_\mathrm{m}$ and $\mathcal{L}^f_\mathrm{m}$ under diffeomorphisms, which appears to be a natural requirement.
In this case, the equations of motion for $\gmn$ then give rise to $d$ Bianchi constraints,
\beqn\label{Bianchi}
\nabla^\mu \sum_{n=0}^{d-1}(-1)^n\beta_n \,g_{\mu\lambda}{(Y^{(n)})^\lambda}_{\nu}(S)&=&0\,.
\eeqn 
Accordingly, there is a set of similar constraints arising from the $\fmn$ equation which, as a consequence of the identity (\ref{bicog}), is equivalent to (\ref{Bianchi}). In summary, under the assumption of separate covariant conservation of the stress-energy tensors, the equations of motion contain $d$ constraints~(\ref{Bianchi}) following from diffeomorphism invariance.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Massive Gravity limit}\label{sec:MGlim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

An intriguing question is whether there exist a limit in the Hassan-Rosen theory in which one of the metrics decouples and the remaining metric describes a massive excitation. It turns out that this is indeed possible, but as always the exact limit needs to be treated with care. Massive Gravity limits of bimetric gravity have been studied in~\cite{Baccetti:2012bk}, where it was shown that only one of two possible limiting procedures leads to a nontrivial theory.

Consider again the nonlinear equations of motion (\ref{geq}) and (\ref{feq}) for $\gmn$ and $\fmn$, respectively. In these we now take the following limit,
\beqn\label{mglimit}
\frac{m_f}{M}\rightarrow \infty\,,\qquad \beta_d\rightarrow \infty\,,\qquad \text{such~that}\quad \frac{\beta_dM}{m_f}=\text{const.}
\eeqn
Here, $M$ denotes any other mass scale in the theory, such as $m_g$, $m$ and the energy scale of the sources. Provided that the $\beta_n$ parameters are independent of $m_f/M$, then the equations of motion in this limit reduce to
\begin{align}
\mathcal{G}_{\mu\nu}(g)
+\tfrac{m^d}{m_g^{d-2}}\sum_{n=0}^{d-1}(-1)^n\beta_n \,g_{\mu\lambda}{(Y^{(n)})^\lambda}_{\nu}(S)=\tfrac{1}{m_g^{d-2}}T^{g}_{\mu\nu}\,, \label{gdrgt} \\
\mathcal{G}_{\mu\nu}(f)
+\Lambda\fmn=0 \,,\label{fdrgt}
\end{align}
where $\Lambda\equiv{\beta_d\,m^d}/{m_f^{d-2}}$. The equation for $\gmn$ is unaltered, while the equation for $\fmn$ decouples and simply becomes an ordinary Einstein equation with cosmological constant $\Lambda$. Hence, the solution for $\fmn$ will be an Einstein metric which can be plugged into the $\gmn$ equation. The resulting equation for $\gmn$ is exactly the same as in the nonlinear Massive Gravity where the auxiliary metric $\fmn$ is fixed to be an Einstein metric. Note, however, that it is not possible to derive the equations (\ref{gdrgt}) and (\ref{gdrgt}) from an action principle. 
One may therefore think that a more natural limit would be given by $m_f/M\rightarrow 0$ which could directly be taken in the bimetric action. However, it is quite easy to see that in this limit the equations of motion admit only GR solutions for $\gmn$~\cite{Baccetti:2012bk}.

Another important observation is that, as long as the above limit~(\ref{mglimit}) is not taken exactly, the bimetric equations of motion always force both metrics to be Einstein solutions if one of them is. This follows, for example, from the perturbative solutions that we obtain in chapter~\ref{ch:HD} and can also be shown explicitly for certain parameter choices. Therefore the Massive Gravity limit is a singular point in parameter space, where an important relation among the two metrics is lost.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
\section{Mass spectrum}\label{sec:massspec}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

From the nonlinear ADM analysis of \cite{Hassan:2011zd} it is known that ghost-free bimetric theory propgates $(d(d-2)-1)$ degrees of freedom. At the linear level around a certain class of backgrounds, these can be attributed to a massless and massive fluctuation. Around general backgrounds or at the nonlinear level, however, such a split is usually not well-defined. In {\protect{\hyperref[papV]{Paper V}}} we identify the backgrounds suitable for discussing the theory's mass spectrum in four dimensions. Then we perturb around these backgrounds and show how to diagonalize the fluctuations into modes with definite mass. {\protect{\hyperref[papVII]{Paper VII}}} generalizes these findings to an arbitrary number of space-time dimensions. Both papers also discuss possible nonlinear extensions of mass eigenstates, a topic which we leave for the next section.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Proportional backgrounds}\label{secpropbg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

A simple, yet very important class of solutions to the bimetric equations of motion is obtained by making an ansatz that conformally relates the two metrics, $\bfmn=c(x)^2\bgmn$, where $c(x)$ is a space-time dependent function. Having plugged this ansatz into the equations of motion, we first note that the Bianchi constraint~(\ref{Bianchi}) immediately enforces $\partial_\mu c(x)=0$ and hence $c(x)=$\,const. This restricts our ansatz to proportional metrics,
\beqn
\bfmn=c^2\bgmn\qquad \text{with}\quad c=\mathrm{const.}
\eeqn
Using this in (\ref{geq}) and (\ref{feq}) we find that the equations of motion simply reduce to two copies of Einstein's equations,
\begin{align}\label{bgeq}
\mathcal{G}_{\mu\nu}(\bar{g})
+\Lambda_g\bgmn=\frac{1}{m_g^{d-2}}\bar{T}^{g}_{\mu\nu}\,, \quad
\mathcal{G}_{\mu\nu}(\bar{g})
+\Lambda_f\bgmn=\frac{1}{m_f^{d-2}}\bar{T}^{f}_{\mu\nu} \,.
\end{align}
In this we have defined the cosmological constant contributions arising from the interaction potential,
\beqn\label{lambdas}
\Lambda_g&\equiv&\frac{m^d}{m_g^{d-2}}\sum_{n=0}^{d-1}{d-1\choose n}c^n\beta_n\,,\nn\\
\Lambda_f&\equiv&\frac{m^d}{(m_f c)^{d-2}}\sum_{n=1}^{d}{d-1\choose n-1}c^n\beta_n\,,
\eeqn
Proportional backgrounds thus simply correspond to solutions to Einstein's equations in General Relativity.
After all constant contributions in the stress-energy tensors have been shifted into $\Lambda_g$ and $\Lambda_f$, respectively,\footnote{This can always be achieved by redefining $\beta_0$ and $\beta_d$.} the difference of the above background equations implies that
\beqn\label{propbackeq}
\Lambda_g=\Lambda_f\,,\qquad
\bar{T}^{f}_{\mu\nu}=\alpha^{d-2}\bar{T}^{g}_{\mu\nu}\,,~~~~~\text{where}~~\alpha\equiv \frac{m_f}{m_g}\,.
\eeqn
From (\ref{lambdas}) it is clear that the first equation relating the cosmological constants is a polynomial in $c$ with coefficients depending on the $\beta_n$ parameters. In general, this equation serves to determine the proportionality constant $c$ of our ansatz in terms of the parameters of the theory and thereby specifies the solution completely. An important exception to this generic situation is the partially massless case, to be introduced in chapter~\ref{ch:PM}.  

The second equation in (\ref{propbackeq}) that relates the sources for the two metrics is very constraining. From a phenomenological point of view, there is no reason to believe that the matter sources satisfy such a strong constraint. Proportional background solutions, however, only exist in this case. Since any deviation from the proportional backgrounds constitutes a deviation from GR solutions, the difference in the source terms may be regarded as a measure for the difference of bimetric solutions from those of GR. 
 
The proportional background solutions are of particular interest because they allow for a definite mass spectrum of fluctuations around them. In general, the linear perturbation equations have a rather complicated structure because in order to derive them one needs to vary the square-root matrix $S=\sqrt{g^{-1}f}$. This is always possible but, for backgrounds giving rise to matrices $\bar{g}^{-1}\bar{f}$ that do not commute with the fluctuations, the resulting expressions are lengthy and not illuminating. In particular, the equations will not contain a mass term with Fierz-Pauli structure which makes it difficult to identify the massive field. In contrast, for the proportional backgrounds we have $\bar{g}^{-1}\bar{f}=c^2\mathbb{1}$ which does commute with any other matrix and hence drastically simplifies the perturbation equations which now will exhibit the Fierz-Pauli structure. Moreover, in the absence of sources, these backgrounds correspond to maximally symmetric ones for which the concept of mass as a label of representations of the underlying isometry group is well-defined. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsection{Linear perturbations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

We shall now consider small perturbations around the proportional backgrounds for both of the metrics as well as the sources,
\beqn
\gmn&=&\bgmn+\dg_{\mu\nu}\,,\qquad \fmn~=~c^2\bgmn+\df_{\mu\nu}\,,\nn\\
T^{g}_{\mu\nu}&=&\bar{T}^{g}_{\mu\nu}+\delta T^{g}_{\mu\nu}\,,\qquad T^{f}_{\mu\nu}~=~\alpha^{d-2}\bar{T}^{g}_{\mu\nu}+\delta T^{f}_{\mu\nu}\,.
\eeqn
In the following we set the background values of the sources to zero, $\bar{T}^{g}_{\mu\nu}=0$. In {\protect{\hyperref[papV]{Paper V}}} we keep them in the equations, which modifies the structure of the kinetic operator (\ref{kinopds}) below. As a consequence, the coupling of the fluctuations to the cosmological constant term assumes a less familiar form, which is our main motivation to present the equations without background sources here. Note however that their inclusion does not alter any of the results.


As stated earlier, around the proportional backgrounds the linearized equations of motion can be diagonalized into an equation for a massless and a massive perturbation. To this end, consider the following redefinitions of fluctuations,
\beqn\label{dGanddM}
\delta G_{\mu\nu} &\equiv&\left[1+(\alpha c )^{d-2}\right]^{\frac{4-d}{d-2}}\big(\dg_{\mu\nu}+c^{d-4}\alpha^{d-2}\df_{\mu\nu}\big)\,,\nn\\
\delta M_{\mu\nu} &\equiv& \frac{1}{2c}\big(\df_{\mu\nu}-c^2 \dg_{\mu\nu}\big)\,,
\eeqn
in which the overall normalizations have been chosen conveniently. Now, taking the appropriate linear combinations of the original fluctuation equations for $\delta\gmn$ and $\delta\fmn$ decouples the massless from the massive mode. The resulting equations read
\begin{align}
{\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}\delta G_{\rho\sigma}&-\tfrac{2}{d-2}\bar{\Lambda}_g\left(\delta G_{\mu\nu}-\tfrac{1}{2}\bar{G}_{\mu\nu}\delta G\right) \nn\\
& \hspace{75pt}=\left(\tfrac{1}{m_g}\right)^{\frac{d-2}{2}}\left(\delta T^g_{\mu\nu}+c^{d-2}\delta T^f_{\mu\nu}\right)\,, \label{dGeq}\\
{\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}\delta M_{\rho\sigma}&-\tfrac{2}{d-2}\bar{\Lambda}_g\left(\delta M_{\mu\nu}-\tfrac{1}{2}\bar{G}_{\mu\nu}\delta M\right)
+\tfrac{\bar{m}^2_\mathrm{FP}}{2}\Big(\delta M_{\mu\nu}-\bgmn\delta M\Big)\nn\\
& \hspace{75pt}=\left(\tfrac{c}{m_f}\right)^{\frac{d-2}{2}}\left(\delta T^f_{\mu\nu}-\alpha^{d-2}\delta T^g_{\mu\nu}\right)\,.\label{dMeq}
\end{align}
Here, the traces of the fluctuations are taken with respect to a redefined background metric, 
\beqn
\bar{G}_{\mu\nu}\equiv \big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}\bgmn\,,
\eeqn
that is $\delta G=\bar{G}^{\mu\nu}\delta G_{\mu\nu}$ and $\delta M=\bar{G}^{\mu\nu}\delta M_{\mu\nu}$. Also, we have redefined the cosmological constant with respect to this background,
\beqn
\bar{\Lambda}_g\equiv \big(1+(\alpha c)^2\big)^{-\frac{2}{d-2}} \Lambda_g  \,, \qquad R_{\mu\nu}(\bar{G})=\frac{2\bar{\Lambda}_g}{d-2}\bar{G}_{\mu\nu}\,.
\eeqn
Furthermore, the kinetic operator ${\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}$ with respect to the $\bar{G}_{\mu\nu}$ background is defined as
\begin{align}\label{kinopds}
\bar{\mathcal{E}}^{\rho\sigma}_{\mu\nu}\delta G_{\rho\sigma} 
=-\tfrac{1}{2}\Big[\delta^\rho_\mu\delta^\sigma_\nu\bar{\nabla}^2
&+\bar G^{\rho\sigma}\bar{\nabla}_\mu\bar{\nabla}_\nu 
-\delta^\rho_\mu\bar{\nabla}^\sigma\bar{\nabla}_\nu
-\delta^\rho_\nu\bar{\nabla}^\sigma\bar{\nabla}_\mu \nn\\
&-\bar{G}_{\mu\nu}\bar G^{\rho\sigma}\bar{\nabla}^2 
+\bar{G}_{\mu\nu}\bar{\nabla}^\rho\bar{\nabla}^\sigma\Big]\delta G_{\rho\sigma}\,,
\end{align}
in which $\bar{\nabla}$ is the covariant derivative compatible with $\bar{G}_{\mu\nu}$. Finally, the Fierz-Pauli mass is given in terms of the parameters of the theory through
\beqn\label{FPmass}
\bar{m}^2_\mathrm{FP}=\frac{m^d}{m_g^{d-2}} \big(1+(\alpha c)^2\big)^{-\frac{2}{d-2}}\left(1+(\alpha c)^{2-d}\right)\sum_{n=1}^{d-1}{d-2\choose n-1}c^n\beta_n\,.
\eeqn
Recall that in the above expressions $c$ is to be regarded as a function of the Planck masses and the $\beta_n$ parameters, determined by the background equation $\Lambda_g=\Lambda_f$. At this stage, the main reason for choosing the new background $\bar{G}_{\mu\nu}$ is to render the equations as simple as possible. However, as our notation already indicates, $\bar{G}_{\mu\nu}$ will also turn out to be the background of the nonlinear massless field that we identify below. Alternatively, we could have written the equations with respect to the original background $\bgmn$, in terms of $\Lambda_g$ and a properly rescaled Fierz-Pauli mass, $m^2_\mathrm{FP}\equiv \big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}\bar{m}^2_\mathrm{FP}$. In addition, there would be a factor of $\big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}$ in front of the source terms, modifying the effective Planck masses of the theory. In {\protect{\hyperref[papV]{Paper V}}} (and also in {\protect{\hyperref[papVI]{Paper VI}}}) we use $\bgmn$ as the background metric, whereas in {\protect{\hyperref[papVII]{Paper VII}}} we express the equations in terms of $\bar{G}_{\mu\nu}$. 

As promised, (\ref{dGeq}) and (\ref{dMeq}), respectively,  describe a massless and a massive spin-2 fluctuation in (Anti-) de Sitter background. At the linear level around proportional backgrounds, one can therefore assign $d(d-3)/2$ degrees of freedom to a massless fluctuation $\delta G_{\mu\nu}$ and the remaining $(d(d-1)/2-1)$ ones to a massive fluctuation $\delta M_{\mu\nu}$.

Observe that in the limit of small $\alpha$ (which is the limit opposite to the massive gravity limit discussed in section~\ref{sec:MGlim}), we have that $\delta G_{\mu\nu}\sim\delta \gmn$ and hence the fluctuation for the metric $\gmn$ becomes mostly massless. This is important because, at least to our present knowledge, only the couplings of the original metrics to matter are ghost-free, whereas on the other hand the gravitational metric needs to be mostly massless for phenomenological reasons. Fortunately, the limit in which the perturbation of $\gmn$ is dominated by the massless mode corresponds to a large Planck mass $m_g$, which is required for having a weak gravitational force anyway. We will come back to this point when discussing the nonlinear extension of the massless field below.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
\section{Nonlinear extensions of mass eigenstates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

In the previous section, we saw that the fluctuations of $\gmn$ and $\fmn$ around proportional backgrounds are not mass eigenstates, whereas certain linear combinations of them do satisfy the equations for massless and massive spin-2 fields. We now turn to the derivation of nonlinear fields  $G_{\mu\nu}$ and $M^G_{\mu\nu}$ that, when linearized around the proportional background solutions, give rise to these massless and massive perturbations. Having obtained expressions for these we are also able to address the question whether it is possible to couple the massless field to matter without reintroducing the Boulware-Deser ghost.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
\subsection{Identifying the nonlinear fields}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

In the following we will see that, as may have been anticipated, there are infinitely many possibilities to define nonlinear fields with massless or massive fluctuations around the proportional backgrounds. In {\protect{\hyperref[papVI]{Paper VI}}} and {\protect{\hyperref[papVII]{Paper VII}}}, we therefore invoke additional criteria of simplicity and invertibility which allow us to single out unique nonlinear extensions of the linear mass eigenstates.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsubsection{The massless field}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

General covariance implies that the most general ansatz for the nonlinear field $G_{\mu\nu}$ with massless fluctuation around proportional backgrounds is of the form
\beqn\label{ansatzG}
G_{\mu\nu}=g_{\mu\rho}{\Phi^\rho}_\nu(S)\,.
\eeqn
Here, ${\Phi^\rho}_\nu(S)$ is an arbitrary matrix-valued function of the square-root matrix $S=\sqrt{g^{-1}f}$. The transposed matrix $S^\mathrm{T}$ does not appear in the ansatz due to the symmetry property $gS=S^\mathrm{T}g$. Now, on the proportional backgrounds, any function of $S$ is proportional to the unit matrix and hence $\Phi(\bar{S})\equiv\phi( c)\mathbb{1}$, where $\phi( c)$ is just a scalar function of $c$. With (\ref{ansatzG}) the fluctuation of $G_{\mu\nu}$ can thus be written as
\beqn
\delta G_{\mu\nu}=\phi( c)\delta g_{\mu\nu}+\bar{g}_{\mu\rho}\left.\frac{\delta {\Phi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}\delta {S^\alpha}_\beta\,.
\eeqn
Using the variation of the square root around proportional backgrounds,
\beqn\label{sfluc}
\delta {S^\alpha}_\beta=\frac{1}{2c}\bar{g}^{\alpha\lambda}(\delta f_{\lambda\beta}-c^2\delta g_{\lambda\beta})\,,
\eeqn
we can compare this expression to the definition of the massless fluctuation in~(\ref{dGanddM}). This gives
\beqn
\phi(s)&=&\big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}\,,\nn\\
 \left.\frac{\delta {\Phi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}&=& 2\left[1+(\alpha c )^{d-2}\right]^{\frac{4-d}{d-2}}c^{d-3}\alpha^{d-2}\delta^\rho_\alpha\delta^\nu_\beta\,.
\eeqn
These constraints on the matrix function ${\Phi^\rho}_\nu(S)$ have an infinite number of solutions given through power series of the matrix $S$ with mildly constrained coefficients. We present their general form in the case of four space-time dimensions in {\protect{\hyperref[papV]{Paper V}}}. From all of these possible definitions for the nonlinear massless field we choose the one that gives the simplest invertible relation to the original variables $\gmn$ and $\fmn$. This particular choice corresponds to
\beqn\label{defG}
G_{\mu\nu} = \left[1+(\alpha c )^{d-2}\right]^{\frac{4-d}{d-2}}\big(g_{\mu\nu}+c^{d-4}\alpha^{d-2}f_{\mu\nu}\big)\,.
\eeqn
Remarkably, it turns out to be simply a linear combination of the original metrics.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsubsection{The massive field}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to identify a nonlinear extension of the massive fluctuation, we make an ansatz similar to the one for the massless field above,
\beqn\label{ansatzM}
M_{\mu\nu}=g_{\mu\rho}{\Psi^\rho}_\nu(S)\,,
\eeqn
where ${\Psi^\rho}_\nu(S)$ is an arbitrary matrix-valued function of the square-root matrix ${S^\mu}_\nu$. Again, on the background we have $\Psi(\bar{S})=\psi( c)\mathbb{1}$ with $\psi( c)$ being a scalar function. The variation of the ansatz therefore reads
\beqn
\delta M_{\mu\nu}=\psi( c)\delta g_{\mu\nu}+\bar{g}_{\mu\rho}\left.\frac{\delta {\Psi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}\delta {S^\alpha}_\beta\,.
\eeqn
Comparing this to the definition of the massive fluctuation in (\ref{dGanddM}), we see that
\beqn\label{constdm}
\psi( c)=0\,,\qquad \left.\frac{\delta {\Psi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}=\delta^\rho_\alpha\delta^\beta_\nu\,. 
\eeqn
As in the massless case, there are infinitely many solutions to these constraints whose general form is provided in {\protect{\hyperref[papV]{Paper V}}} for $d=4$.
In order to single out a nonlinear extension of the massive fluctuation, we first observe that the interaction potential in the action is a polynomial in the square-root matrix ${S^\mu}_\nu$. Moreover, as can be seen by comparing~(\ref{dGanddM}) and~(\ref{sfluc}), the variation of this matrix gives the massive fluctuation up to normalization. However, ${S^\mu}_\nu$ is a (1,1)-tensor which furthermore satisfies the symmetry property $G_{\rho\mu}{S^\mu}_\nu=G_{\nu\mu}{S^\mu}_\rho$ and can therefore not be regarded as independent of the massless field. We would like the massive field to be a (0,2)-tensor that is independent of $G_{\mu\nu}$. On the other hand, lowering an index ${S^\mu}_\nu$ with $G_{\mu\nu}$ modifies the expression of its variation in terms of $\delta\gmn$ and $\delta\fmn$. According to (\ref{constdm}), in oder to obtain the massive fluctuation in~(\ref{dGanddM}) we must subtract the field's background value. 
Hence, our choice for the nonlinear massive fields is given by
\beqn
M^G_{\mu\nu} \equiv \left[1+(\alpha c )^{d-2}\right]^{-\frac{2}{d-2}}\left(G_{\mu\rho} {S^\rho}_\sigma-cG_{\mu\nu}\right)\,.
\eeqn
The reader is reminded once again that in this definition (and in the one for the massless field above), $c$ is a function of the $\beta_n$ parameters obtained by setting $\Lambda_g=\Lambda_f$.

In the next section it will be shown that the massless field $G_{\mu\nu}$, as defined in~(\ref{defG}), cannot consistently couple to matter sources. It is therefore not a suitable candidate for the gravitational metric and rewriting the bimetric theory in terms of $G_{\mu\nu}$ and $M^G_{\mu\nu}$ is probably not useful for phenomenological purposes. On the other hand, $\gmn$ can couple to matter without introducing inconsistencies and a formulation of the theory in terms of $\gmn$ and a corresponding massive field $M_{\mu\nu}$ may be of use for applications. A definition for this new field $M_{\mu\nu}$ which can be considered as independent of $\gmn$ while being compatible with (\ref{constdm}) is
\beqn\label{defMg}
M_{\mu\nu} \equiv g_{\mu\rho} {S^\rho}_\sigma-cg_{\mu\nu}\,.
\eeqn
A particular feature, shared by all possible definitions of the nonlinear massive fields, is that their background value vanishes on the proportional backgrounds. Because these backgrounds precisely corresponds to GR solutions, a nonzero background value for the nonlinear massive field is a measure for deviations of bimetric theory from General Relativity.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Inconsistency of coupling the massless field to matter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   

Astrophysical observations show that the mass of the graviton cannot be larger than the Hubble scale $\sim 10^{-33}$eV. A massless gravitational metric would therefore be favoured from a phenomenological point of view. Having obtained an expression for a nonlinear massless spin-2 field in the bimetric setup, we are therefore interested in the question whether this field could consistently be coupled to matter alone and hence represent the gravitational metric.
This motivates an ADM analysis of interactions between the massless field $G_{\mu\nu}$ and matter sources. To this end, consider the addition of a standard minimal matter coupling of the form
\beqn\label{mmcoup}
S^G_\mathrm{m}=\int \dd^d x~\sqrt{-G}\,\mathcal{L}^G_\mathrm{m}
\eeqn 
to the bimetric action. Since the Hamiltonian analysis of the latter has been performed in the original formulation of the theory, the simplest route to follow is to use the definition (\ref{defG}) of the massless field to obtain its ADM variables as functions of the ADM variables of $\gmn$ and $\fmn$. In fact, since constant factors are not of interest in the ADM analysis, we can simply rescale the metrics such that we have $G_{\mu\nu}=\gmn'+\fmn'$, where $\gmn'$ and $\fmn'$ possess ADM decompositions as in (\ref{admmetr}) and (\ref{admf}), respectively.
That is to say, we define 
\beqn
G_{\mu\nu}=\begin{pmatrix}
-K^2+K_m\Gamma^{mn}K_n&K_j\\ K_i & \Gamma_{ij}
\end{pmatrix}\,,
\eeqn
whose components obey
\beqn\label{ADMG}
K_i&=&N_i+L_i\,,\qquad \Gamma_{ij}~=~\gamma_{ij}+\tilde{f}_{ij}\,,\nn\\
K^2&=&N^2+L^2+\Gamma^{ij}K_iK_j-\gamma_{ij}N^iN^j-\tilde{f}_{ij}L^iL^j\,.
\eeqn
In these, the shift $N_i$ of $\gmn$ should be understood as a function of the other ADM variables and the redefined shift vectors $n_i$, according to~(\ref{shiftred}).  
After this redefinition the bimetric action is linear in the lapses $N$ and $L$ of $\gmn$ and $\fmn$ as well as the shift $L_i$ of $\fmn$. In order not to reintroduce the Boulware-Deser ghosts and maintain diffeomorphism invariance, the coupling (\ref{mmcoup}) must also be linear in these variables. 
On the other hand, since we take the couplings (\ref{mmcoup}) to resemble those of the metric in General Relativity, we know that due to general covariance of GR they have to be linear in the lapse $K$ and shift $K_i$ of $G_{\mu\nu}$.\footnote{For instance, this can explicitly be verified for the standard coupling of a massless scalar field, $\mathcal{L}^G_\mathrm{m}=G^{\mu\nu}\partial_\mu\phi\partial_\nu\phi$.} But from~(\ref{ADMG}) it is clear that the lapse $K$ is a nonlinear function of $N$, $L$ and $L^i$. In order to demonstrate the consistency bimetric action without matter coupling, so far we have only redefined $N_i$. We therefore still have the freedom to perform a redefinition of $L_i$ which possibly could render the expression for $K$ linear in $N$, $L$ and $L^i$. However, as we will now argue, such a redefintion does not exist. To see this, rewrite the above expression for~$K^2$ as
\beqn\label{defk2} 
K^2=N^2+L^2+(N^i-L^i) (\gamma_{ij}-\gamma_{ik} \Gamma^{kl} \gamma_{lj}) (N^j-L^j)  \,.
\eeqn
The redefinition of $L^i$ would have to turn the right-hand side of this equation into a perfect square of a function linear in $N$, $L$ and $L^i$. 
But due to the form of the redefinition~(\ref{shiftred}) required by the bimetric interaction potential, we have that 
\beqn 
N^i-L^i=Ln^i-N{D^i}_kn^k\,,
\eeqn
implying that the above expression for $K^2$ does not depend on $L^i$. Consequently, redefining $L^i$ cannot change the fact that $K$ is nonlinear in $N$ and $L$ and hence a coupling term of the form (\ref{mmcoup}) cannot be consistent.


Of course, we have not shown that a massless field in bimetric theory can never couple to matter in a ghost-free manner.
The above proof only applies to standard matter couplings and to the massless field singled out in the previous section. It is possible that other types of couplings or more complicated choices for the field remedy the above conclusion and there exist a way to obtain a massless gravitational metric.\footnote{Another option is to tune the $\beta_n$ parameters such that the Fierz-Pauli mass (\ref{FPmass}) vanishes. In this case, both $\gmn$ and $\fmn$ have massless fluctuations and the graviton could be massless while still interacting nontrivially with another spin-2 field at the nonlinear level.}  




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Massive spin-2 interactions with gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

Owing to the absence of ghost-free matter couplings for the nonlinear massless field, we choose to consider the standard consistent interactions of the metric $\gmn$ with matter sources. In this case, $\gmn$ is the gravitational metric with geometric interpretation. Its fluctuations, however, are neither massless nor massive; they are superpositions of mass eigenstates. Nonetheless, it is still possible to consider a nonlinear version of the massive spin-2 perturbation in this gravitational background. The appropriate nonlinear field which is independent of $\gmn$ is the one given in~(\ref{defMg}). 

In {\protect{\hyperref[papV]{Paper V}}} we rewrite the Hassan-Rosen bimetric action in terms of the variables $\gmn$ and $M_{\mu\nu}$. In the interaction potential, implementing the field redefinition is straightforward,
\beqn
\sum_{n=0}^d\beta_ne_n(S)=\sum_{n=0}^d\beta_ne_n(c\mathbb{1}+g^{-1}M)=\sum_{n=0}^d\alpha_n^ce_n(g^{-1}M)\,.
\eeqn
Here the new parameters $\alpha_n^c$ depend on the original $\beta_n$-parameters in the following way,
\beqn
\alpha^c_n\equiv\sum_{k=n}^d {d-n \choose k-n} c^k\beta_k\,.
\eeqn
The potential is therefore simply a polynomial in $M_{\mu\nu}$. In the kinetic term for $\fmn$ we invoke the curvature relations~(\ref{curvrel}) to rewrite it in terms of $\gmn$-covariant derivatives acting on $M_{\mu\nu}$. For notational simplicity, we present the result in terms of the matrix $S=c\mathbb{1}+g^{-1}M$,
\beqn
\sqrt{-f}\,R(f)=\sqrt{-g}\,(\det S)\left[\phi^{\mu\nu}R_{\mu\nu}(g)+\Pi_{\rho\omega}^{\sigma\pi\alpha\beta}\nabla_\alpha{S^\rho}_\sigma\nabla_\beta{S^\omega}_\pi\right]\,.
\eeqn
Here we have used the abbreviation,
\beqn
\phi^{\mu\nu}\equiv{(S^{-2})^\mu}_\rho g^{\rho\nu}\,,
\eeqn
as well as defined a nonlinear polarization tensor,
\begin{align}
\Pi_{\rho\omega}^{\sigma\pi\alpha\beta}
\equiv\big(2&\phi^{\alpha\mu}\phi^{\kappa\delta}\phi^{\beta\nu}
-2\phi^{\alpha\mu}\phi^{\beta\kappa}\phi^{\delta\nu}
\nn\\
&-\phi^{\alpha\beta}\phi^{\kappa\delta}\phi^{\mu\nu}
+\phi^{\alpha\beta}\phi^{\kappa\mu}\phi^{\delta\nu}\big)
\delta^\sigma_{(\kappa}\delta^\gamma_{\delta)}\,  
\delta^\pi_{(\mu} \delta^\lambda_{\nu)}\, S_{\gamma\rho}\,
S_{\lambda\omega}. 
\end{align}
Collecting all the terms we arrive at the nonlinear action for a massive spin-2 field $M_{\mu\nu}$ in a gravitational background $\gmn$,
\begin{align}\label{sp2gr}
&S_{M,g}~=~m_g^{d-2}\int\dd^d x~\sqrt{-g}\,R(g) +\int\dd^d x~\sqrt{-g}\,\mathcal{L}^g_\mathrm{m}\nn\\
&~+~m_f^{d-2}\int\dd^d x~\sqrt{-g}\,(\det S)\left[\phi^{\mu\nu}R_{\mu\nu}(g)+\Pi_{\rho\omega}^{\sigma\pi\alpha\beta}\nabla_\alpha{S^\rho}_\sigma\nabla_\beta{S^\omega}_\pi\right] \nn\\
&~-~2m^d\int\dd^dx~\sqrt{-g}\,\sum_{n=0}^d\alpha_n^ce_n(g^{-1}M)\,.
\end{align}
While in the bimetric formulation of the theory in terms of $\gmn$ and $\fmn$ the kinetic terms are diagonal, the massive spin-2 field shows highly nontrivial kinetic mixing with the gravitational metric. Moreover, as already stated above, $\gmn$ does not give rise to a massless fluctuation around maximally symmetric backgrounds, which could endanger the compatibility of the theory with observations. However, we also already observed that gravity becomes essentially massless in the limit where its interactions are weak, $m_g/m_f\rightarrow \infty$. Hence, although the presence of a massive spin-2 field always implies that the graviton is a superposition of mass eigenstates, the effects of this mixing are expected to be small due to the weakly interacting nature of gravity.

Of course, it is also possible to formulate the theory in terms of the nonlinear fields $G_{\mu\nu}$ and $M^G_{\mu\nu}$. The structure of the resulting action is even more involved than in~(\ref{sp2gr}) and we refrain from presenting it here. Its expression in four space-time dimensions can be found in {\protect{\hyperref[papV]{Paper V}}}.

From the consistent matter couplings in the original bimetric formulation one can furthermore derive ghost-free interactions between the massive spin-2 field $M_{\mu\nu}$ and arbitrary types of matter fields. For interactions with bosonic matter this is straightforwardly realized by making the replacement $\fmn=g_{\mu\alpha}{S^\alpha}_\beta{S^\beta}_\nu$ in the standard matter couplings $\int\dd^dx\, \sqrt{-f}\,\mathcal{L}^f_\mathrm{m}$ for $\fmn$. In {\protect{\hyperref[papV]{Paper V}}} we give an explicit example of coupling $M_{\mu\nu}$ to a massive spin-1 field and also work out the slightly more complicated couplings of the massive spin-2 field to fermions. The latter requires working in the vielbein formulation and making appropriate replacements in the $\gamma^\mu$ matrices as well as the spin connections.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Generalization to Multimetric Theory} 
\label{ch:MV}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Ghost-free bimetric theory describes the interaction of two spin-2 fields, one with massless and one with massive fluctuations around proportional backgrounds. In this section we discuss a generalization of the Hassan-Rosen action to an interacting theory for an arbitrary number of spin-2 fields as introduced in~\cite{Hinterbichler:2012cn}. In general, such a theory will contain one massless spin-2 mode along with many massive ones and, again, one has to ensure the absence of the corresponding Boulware-Deser ghosts. A formulation of the theory in terms of vielbeins turns out to be very convenient for the ghost proof, but reexpressing the consistent multivielbein action in terms of metrics is not entirely trivial.
In {\protect{\hyperref[papIV]{Paper IV}}} we develop a method to rewrite the multivielbein theory of~\cite{Hinterbichler:2012cn} in terms of the corresponding metrics as well as St\"uckelberg fields that take care of local Lorentz invariances. 
We begin the discussion with a demonstration of consistent and inconsistent multimetric couplings before going over to the multivielbein formulation. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multiple bimetric couplings}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

When constructing a theory for more than two spin-2 fields, of course, the main requirement on its structure remains the absence of the Boulware-Deser ghosts. The interaction potential for $\mathcal{N}$ fields therefore has to be chosen such that the action in Hamiltonian formulation gives rise to $(d+\mathcal{N}-1)$ constraints. Out of these,  $d$ should be first class constraints, generating the group of general coordinate transformations, while the remaining $(\mathcal{N}-1)$ are expected to be second class and serve to remove all Boulware-Deser ghosts from the spectrum. 


An obvious way to satisfy these requirements is to simply add up several copies of the Hassan-Rosen action for fields $\fmn$ and $\gmn^{(i)}$ with $i=1,\hdots, \mathcal{N}-1$, to obtain a theory in which one of the metrics coupled to all the others,
\beqn\label{centercoup}
S_\mathrm{center}(f,\{g^{(i)}\})=\sum_{i=1}^{\mathcal{N}-1}S_{\mathrm{HR}}(g^{(i)},f)\,.
\eeqn
This will be consistent because in every interaction potential one can redefine the ADM variables for $\gmn^{(i)}$ to make it linear in the lapse and shift of~$\fmn$ as well as the lapse of $\gmn^{(i)}$, such that one obtains the desired $(d+\mathcal{N}-1)$ constraints. 

The left panel of Figure~4.1 shows how such a coupling can be visualized in a graph~\cite{Hinterbichler:2012cn}. Each solid dot represents a different spin-2 field and the lines stand for standard Hassan-Rosen bimetric couplings between them. Fields corresponding to dots that are not connected by a line do not directly interact. Due to the corresponding picture with one metric in the center, we shall refer to interactions of the form~(\ref{centercoup}) as ``center couplings".

Another option to obtain consistent multiple bimetric interactions is to build a ``chain" of $\mathcal{N}$ coupled spin-2 fields $\gmn^{(k)}$ where $k=1,\hdots,\mathcal{N}$. That is to say, we take an action is of the form,
\beqn
S_\mathrm{chain}(\{g^{(k)}\})=\sum_{k=1}^{\mathcal{N}-1}S_{\mathrm{HR}}(g^{(k)},g^{(k+1)})\,,
\eeqn
for which the corresponding graph is depicted in the right panel of Figure~4.1.
This construction works because in the first term one can redefine the ADM variables for $g^{(1)}$ such that it becomes linear in the lapse and shift of $g^{(2)}$ as well as the lapse of $g^{(1)}$. In the second term one performs a similiar redefinition for the shift of $g^{(2)}$ which, since the redefinition is linear in the lapses, does not destroy the linearity in the lapse of $g^{(2)}$ in the first term. Note however that the second term will no longer be linear in the shift of $g^{(2)}$. Continuing with this procedure in all the terms results in an action that is linear in the lapse and shift of $g^{(\mathcal{N})}$ and in all the other lapses. 



    \begin{figure}[h]
    \begin{center}
    \includegraphics[width=210pt]{Pictures/vbvertex.pdf}
    \caption{The center couplings \textit{(left)} and the chain couplings \textit{(right)}.}
    \end{center}\label{figcentchaint}
    \end{figure}
    
  

In fact, it is also possible to combine the two above constructions in the following manner: First introduce a chain coupling for fields $f^{(k)}$, $k=1,\hdots,\mathcal{K}$, and then to each $f^{(k)}$ attach $I_k$ fields $g_{(k)}^{(i_k)}$, $i_k=1,\hdots\mathcal{I}_k$, in a center coupling. This gives 
\beqn\label{gencv}
S_\mathrm{c-v}~=~S_\mathrm{chain}(\{f^{(k)}\})+\sum_{k=1}^\mathcal{K}S_\mathrm{center}(f^{(k)},\{g_{(k)}^{(i_k)}\})\,.
\eeqn
In this theory the total number of fields is $\mathcal{N}=\mathcal{K}+\sum_{k=1}^\mathcal{K}\mathcal{I}_k$. An example for a graph is shown in the left panel of Figure~4.2.
  \begin{figure}[h]
    \begin{center}$
    \begin{array}{cc}
    \includegraphics[width=140pt]{Pictures/vbchainvertex.pdf}~~~~~ & ~~~~~
    \includegraphics[width=45pt]{Pictures/vbloop.pdf}
    \end{array}$
    \caption{The combined chain and center couplings \textit{(left)} and a forbidden loop coupling \textit{(right)}.}
    \end{center}
    \end{figure}
Note that the action~$S_\mathrm{c-v}$ still consists purely of multiple copies of the Hassan-Rosen bimetric action; we have not introduced any type of new interaction term. 
Of course, in the above construction, it is also possible to add further center couplings to each of the $g_{(k)}^{(i_k)}$.
However, it is important to realize that not all possible bimetric couplings are allowed. In particular, one may not couple the metrics in a ``loop", which means adding terms such as $S_{\mathrm{HR}}(f^{(k)},f^{(k+2)})$ or $S_{\mathrm{HR}}(f^{(k+1)},g_{(k)}^{(i_k)})$ to (\ref{gencv}). To see why this fails, consider a simple loop coupling among three metrics,
\beqn\label{loopact}
S_\mathrm{loop}(g,f,h)=S_{\mathrm{HR}}(g,f)+ S_{\mathrm{HR}}(f,h)+S_{\mathrm{HR}}(h,g)\,,
\eeqn
whose graph is depicted in the right panel of Figure~4.2.
Now imagine that in the first term one redefines the shift of $g$ to render it linear in the lapse and shift of $f$ and the lapse of $g$. Then, in the second term redefine the shift of $f$ such that the first two terms afterwards are linear in the lapse and shift of $h$ and the lapses of $g$ and $f$. In the third term, one would now have to redefine the shift of $h$, but from the particular form~(\ref{shiftred}) of the redefinition it is clear that afterwards, the action will again contain the original shift variable for $g$ which cannot be expressed in terms of the redefined variables only. Therefore there is at least no obvious consistent redefinition of ADM variables that renders (\ref{loopact}) linear in all the lapses and we conclude that the loop couplings most likely give rise to Boulware-Deser ghosts. This is in agreement with results of a similar analysis performed in~\cite{Nomura:2012xr}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multivielbein couplings}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

So far we have used the earlier results of the bimetric ADM analysis in order to couple several spin-2 fields to each other using only bimetric interactions. Now we would like to address the question whether there exist more general couplings than the bimetric vertex. We introduce graphs for two examples of such $n$-point vertices in Figure~4.3. 
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=150pt]{Pictures/vbmulti1.pdf}
       \caption{A three- and a four-point vertex.}
    \end{center}
    \end{figure}
A priori, such couplings could be very different from the bimetric ones and the ADM analysis has to be redone from the start.

The problem is simplified when working with vielbeins ${E^a}_\mu(I)$, labeled by an index $I=1,\hdots,\mathcal{N}$, instead of the corresponding metrics $g_{\mu\nu}(I)$. The metrics expressed in terms of the vielbeins read
\beqn\label{defvielbein}
g_{\mu\nu}(I)={E^a}_\mu(I)\eta_{ab}{E^b}_\nu(I)\,.
\eeqn 
The vielbeins have a coordinate index $\mu$ as well as a Lorentz index $a$ and the definition of the metric is invariant under local Lorentz transformations.
Their kinetic terms are simply taken to be the Einstein-Hilbert terms $S_\mathrm{EH}(I)$ for the metrics expressed in terms of~${E^a}_\mu(I)$ through~(\ref{defvielbein}).
In~\cite{Hinterbichler:2012cn} it is shown that then the interactions of vielbeins that lead to ghost-free theories are of the form
\begin{align}\label{vielbeinpot}
S_\mathrm{int}&=\frac{m^2}{4}\sum_{\{I\}}\int\dd^dx~T^{I_1\hdots I_d}U_{I_1\hdots I_d}\,,\nn\\
\text{with}~~~~U_{I_1\hdots I_d}&=\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{a_1\hdots a_d}{E^{a_1}}_{\mu_1}(I_1)\hdots{E^{a_d}}_{\mu_d}(I_d)\,,
\end{align}
where $T^{I_1\hdots I_d}$ are coupling constants, and $\tilde{\epsilon}^{\mu_1\hdots\mu_d}$ and $\tilde{\epsilon}_{a_1\hdots a_d}$ are the totally antisymmetric tensor densities with respect to GCT and Lorentz transformations, respectively. The total multivielbein action is then given by
\beqn\label{multac}
S_\mathrm{multi}=\sum_{I=1}^\mathcal{N}S_\mathrm{EH}(I)+S_\mathrm{int}\,.
\eeqn
Note that the antisymmetric structure of (\ref{vielbeinpot}) ensures that there cannot be more than $d$ vielbeins interacting in one vertex. The ghost-free theory therefore gives rise to diagrams of the type displayed in Figure~3.3 with at most $d$ lines ending in one vertex. 
%We will summarize the consistency proof of~\cite{Hinterbichler:2012cn} in section~\ref{secvbghost}. 

A few remarks on degree-of-freedom counting in the vielbein theory are in order. A general vielbein has no symmetry properties and therefore consists of $d^2$ independent components, whereas the corresponding metric is symmetric and thus only $d(d+1)/2$ of its components are independent. This discrepancy can of course be explained by the presence of additional gauge symmetries in the vielbein theory which serve to remove the redundant degrees of freedom. These $d(d-1)/2$ gauge transformations are the local Lorentz transformations ${\Lambda^b}_a(I)$ that act on the upper index of the vielbein ${E^a}_\mu(I)$. A general theory for $\mathcal{N}$ vielbeins ${E^a}_\mu(I)$ will therefore be invariant under $\mathcal{N}$ distinct local Lorentz transformations. Note however that in (\ref{vielbeinpot}), $\mathcal{N}-1$ of the local Lorentz gauges have already been fixed in order to identify the different Lorentz frames for each vielbein with each other and contract all their indices with a common antisymmetric tensor. Only one overall Lorentz invariance is left over. As discussed in~\cite{Hinterbichler:2012cn} and reviewed in {\protect{\hyperref[papIV]{Paper IV}}}, for each vielbein there exist $d(d-1)/2$ combinations of its equations of motion following from (\ref{multac}) that do not contain any derivatives. These read
\beqn\label{constvierb}
\frac{\delta S_\mathrm{int}}{\delta {E^a}_\mu(I)}{E^c}_\mu(I)\eta_{cb}-\frac{\delta S_\mathrm{int}}{\delta {E^b}_\mu(I)}{E^c}_\mu(I)\eta_{ca}=0\,,
\eeqn
and give the correct number of constraints to reduce the number of independent components of each vielbein to $d(d+1)/2$, as expected in a gauge-fixed theory. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Hamiltonian analysis of the vielbein theory}
\label{secvbghost}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Before we come to its metric formulation, we review the ADM analysis of the multivielbein theory as presented in~\cite{Hinterbichler:2012cn}, which proves the absence of the Boulware-Deser ghosts. 
The Hamiltonian analysis is carried out for the vielbein action with interaction potential in its gauge fixed form~(\ref{vielbeinpot}). It makes use of the fact that the vielbein ${E^a}_\mu$ can be decomposed as 
\beqn\label{decvbla}
{E^a}_\mu(I)={\hat{\Lambda}^a}_{~b}(I){\hat{E}^b}_{~\mu}(I)\,,
\eeqn
where ${\hat{\Lambda}^a}_{~b}(I)$ is a Lorentz transformation and ${\hat{E}^b}_{~\mu}(I)$ is a constrained vielbein for which the following ADM parameterization may be chosen,
\beqn\label{ADMvb}
{\hat{E}^b}_{~\mu}(I)=\begin{pmatrix}
N(I)&0\\ {\hat{e}^s}_{~j}(I)N^j(I)&{\hat{e}^s}_{~i}(I)
\end{pmatrix}\,.
\eeqn
At this point it becomes evident why the vielbein formulation significantly simplifies the Hamiltonian analysis: In contrast to the ADM parameterization of the metric, c.f.~(\ref{admmetr}), the expression for the vielbein is itself already linear in lapse and shift. 
When $d$ vielbeins are contracted with the totally antisymmetric $\tilde{\epsilon}$-tensors in~(\ref{vielbeinpot}), the resulting expression will be linear in all ${E^a}_0(I)$, which implies linearity in $N(I)$ and $N^j(I)$. This certainly is a great advantage over the metric formulation because, due to the absence of square root matrices, no redefinition of ADM variables is needed. However, the simplification does not come without a price, because one still has to deal with the Lorentz matrices ${\hat{\Lambda}^a}_{~b}(I)$ and the extra gauge invariances, as we will explain now. 

The parameterization (\ref{ADMvb}) does not fix the gauge completely but is invariant under the residual gauge group of spatial rotations. To the action one should therefore add a term $\lambda^{ab}(I)\mathcal{P}_{ab}(I)$ for each vielbein, where $\lambda^{ab}(I)$ is a Lagrange multiplier and $\mathcal{P}_{ab}(I)$ are the $\mathcal{N}$ first class constraints that generate the residual gauge group of spatial rotations. The explicit expressions for the matrices $\mathcal{P}_{ab}(I)$ are not important to us but we emphasize that they are functions of the spatial vielbeins and there canonical momenta alone.
It also follows that each ${\hat{\Lambda}^a}_{~b}(I)$ can be parameterized by $d-1$ boosts~$p^a(I)$ which, when the decomposition (\ref{decvbla}) is plugged into the interaction potential~(\ref{vielbeinpot}), enter as St\"uckelberg fields. 

Thus, the potential in ADM variables is of the form
\beqn
S_\mathrm{int}=\int\dd^dx~\sum_{I=1}^{\mathcal{N}}\Big(N(I)\mathcal{C}(I)+N^j(I)\mathcal{C}_j(I)\Big)\,,
\eeqn
where the lapse and shift constraints $\mathcal{C}(I)$ and $\mathcal{C}_j(I)$ are functions of the spatial vielbeins ${\hat{e}^s}_{~i}(I)$ and the boosts $p^a(I)$.  When expressed in terms of vielbeins, the ADM form of the Lorentz invariant kinetic terms is similar to~(\ref{gradm}) in the metric theory, and the full action is linear in all~$N(I)$ and~$N^j(I)$.

Recall that the action with potential in its gauge fixed form still possesses one overall local Lorentz invariance. Part of this residual gauge symmetry can now be used to rotate away one of the $p^a(I)$. The remaining boosts can be solved for using $\mathcal{N}-1$ of the $N^j(I)$ equations. In this way all $p^a(I)$ are eliminated from the action. The last shift constraint together with one of the lapse constraints generate general coordinate transformations. The remaining $\mathcal{N}-1$ lapse equations are the secondary constraints that remove the Boulware-Deser ghosts.

The degree-of-freedom counting in the vielbein theory therefore goes as follows: To start with, there are $(d-1)^2$ components in each of the $\mathcal{N}$ spatial vielbeins, along with corresponding $\mathcal{N}(d-1)^2$ canonical momenta. 
The residual overall gauge invariance under spatial rotations gives rise to first class constraint $\sum_I\mathcal{P}_{ab}(I)$ and remove $2\cdot (d-1)(d-2)/2$ degrees of freedom in total. The remaining $\mathcal{N}-1$ spatial Lorentz transformations have been used for gauge fixing and therefore now give rise to second class constraints upon variation with respect to $\lambda^{ab}(I)$. This reduces the phase space by another $2\cdot (\mathcal{N}-1)(d-1)(d-2)/2$ dimensions.
The overall general coordinate transformations again give first class constraints and take away $2d$ variables. Finally, the $\mathcal{N}-1$ lapse constraints are assumed (although not shown) to also give rise to secondary constraints, which then together remove another $2(\mathcal{N}-1)$ degrees of freedom. 
Putting everything together, we find that the dimension of phase space is 
\begin{align}
D_\mathrm{p.s.}=2\cdot (\mathcal{N}-1)\Big(d(d-1)/2-1\Big)+2\cdot d(d-3)/2\,.
\end{align}
This is the correct number of degrees of freedom for describing $\mathcal{N}-1$ massive and one massless spin-2 particle.











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multimetric theory}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Let us briefly outline how this equivalence follows in a theory with only two interacting vielbeins ${E^a}_\mu\equiv{E^a}_\mu(1)$ and ${\bar{E}^a}_\mu\equiv{E^a}_\mu(2)$  (the more general case of multiple two-point interactions is very similar).  As demonstrated in~\cite{Hinterbichler:2012cn}, the equations of motion are solved by vielbeins that satisfy\footnote{There may also be other branches of solutions that lead to a theories which are not equivalent to the bimetric description, see~\cite{deffayet}.}
%\beqn
%{(E^{-1})^\mu}_a{\bar{E}^a}_\nu
%\eeqn  



The structure of (\ref{vielbeinpot}) is reminiscent of the ghost-free bimetric interaction potential (\ref{potantisym}), and for certain choices of $T^{I_1\hdots I_d}$ the vielbein and metric theories are indeed equivalent. More precisely, this is true whenever the interactions consist only of two-point vertices and contain no loops, i.e.~gives rise to the graphs of Figure~3.1. In that case, the constraints~(\ref{constvierb}) give rise to a symmetrization condition on the vielbeins which allows certain combinations of them to be expressed as square root matrices of the type $\sqrt{g^{-1}f}$. This explains why it is possible to have loop interactions in the vielbein theory despite the no-go statement we made about the metric formulation. We will see how this works in more detail below, after we have discussed the general case.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Obtaining a metric formulation}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In {\protect{\hyperref[papIV]{Paper IV}}} we show that it is always possible to reexpress the vielbein theory in terms of the corresponding metrics together with a set of St\"uckelberg fields. The main idea is to move away from the gauge fixed form of the vielbein that lead to the potential~(\ref{vielbeinpot}), and instead consider $\mathcal{N}$ general vielbeins ${e^a}_\mu(I)$ along with $\mathcal{N}$ independent Lorentz frames. 
The ${e^a}_\mu(I)$ are related to the  gauge fixed ${E^a}_\mu(I)$ by a local Lorentz transformation ${\Lambda^a}_b(I)$ through ${E^a}_\mu(I)={\Lambda^a}_b(I){e^b}_\mu(I)$. Since the corresponding metrics are Lorentz invariant, we again have
\beqn\label{defvielbein2}
g_{\mu\nu}(I)={e^a}_\mu(I)\eta_{ab}{e^b}_\nu(I)\,,
\eeqn 
and the kinetic terms are do not involve the local Lorentz matrices. On the other hand, the interaction potential~(\ref{vielbeinpot}) is now given in terms of
\beqn\label{unfixpot}
U_{I_1\hdots I_d}&=\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{a_1\hdots a_d}{\Lambda^{a_1}}_{b_1}{e^{b_1}}_{\mu_1}(I_1)\hdots{\Lambda^{a_d}}_{b_d}{e^{b_d}}_{\mu_d}(I_d)\,.
\eeqn
The local Lorentz matrices ${\Lambda^a}_b(I)$ appear in the action as St\"uckelberg fields\footnote{For recent references that make use of our method of using St\"uckelberg fields to restore the local Lorentz symmetries in multivielbein theory, see \cite{Gabadadze:2013ria, Ondo:2013wka}.} that restore the full set of $\mathcal{N}$ local Lorentz invariances in the theory. Their indices transform in two different frames, namely those of $\tilde{\epsilon}_{a_1\hdots a_d}$ and ${e^b_i}_{\mu_i}(I)$, respectively. The gauge choice that corresponds to~(\ref{vielbeinpot}) is the one in which all ${\Lambda^a}_b(I)$ are equal since in that case the $\tilde{\epsilon}$ contractions reduce them to a factor $\det\Lambda=1$.

The fully gauge invariant potential given in terms of (\ref{unfixpot}) is the starting point for converting the vielbein into a metric theory. The important point is that it allows us to choose any convenient gauge for the vielbeins ${e^a}_{\mu}(I)$, which is of course not possible in its gauge fixed form~(\ref{vielbeinpot}). As we will see now, the freedom of choosing a gauge is essential for the theory being expressible in terms of metrics.

From the gauge invariant form we proceed by identifying the frames of one of the vielbeins, say ${e^b}_{\mu}(1)$, and $\tilde{\epsilon}_{a_1\hdots a_d}$ . Then, due to the invariance of the totally antisymmetric tensor density, we can rewrite (\ref{unfixpot}) as
\beqn\label{newpotga}
U_{I_1\hdots I_d}&=\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{c_1\hdots c_d}{\Lambda^{c_1}}_{b_1}(1,I_1){e^{b_1}}_{\mu_1}(I_1)\hdots{\Lambda^{c_d}}_{b_d}(1,I_d){e^{b_d}}_{\mu_d}(I_d)\,.\nn\\
\eeqn
Here we have defined the combined Lorentz matrices,
\beqn
{\Lambda^{c}}_{b}(1,I)\equiv{(\Lambda^{-1})^c}_a(1){\Lambda^{a}}_{b}(I)\,,
\eeqn
whose indices transform in the frame of ${e^b}_{\mu}(1)$ and ${e^b}_{\mu}(I)$, respectively. Note that ${\Lambda^{c}}_{b}(1,1)=\delta^c_b$ such that there are only $\mathcal{N}-1$ nontrivial matrices. With the interaction potential brought into the form (\ref{newpotga}), we now again pick a gauge for the vielbeins ${e^b}_{\mu}(I)$, $I=2,\hdots,\mathcal{N}$. Namely, we introduce gauge fixed vielbeins ${\overline{e}^a}_{\rho}(I)$ that satisfy the following symmetry condition,
\beqn
{\overline{e}^b}_{\rho}(I){(e^{-1})^\rho}_c(1)\eta^{ca}={\overline{e}^a}_\rho(I){(e^{-1})^\rho}_c(1)\eta^{cb}\,.
\eeqn
This is sometimes referred to as the Deser-van-Nieuwenhuizen gauge.\footnote{It has been argued in \cite{Deffayet:2012zc} that it might not always be possible to choose this gauge in general. For instance, in four space-time dimensions it requires the existence of the square root matrix $\sqrt{g^{-1}(1)g(I)}$.}
In particular, it again identifies all of the Lorentz frames with that of ${e^a}_{\mu}(1)$. In this specific frame one then has
\begin{align}
g^{\mu\rho}(1)g_{\rho\nu}(I)&={(e^{-1})^\mu}_a(1){\overline{e}^b}_{\rho}(I){(e^{-1})^\rho}_c(1)\eta^{ca}\eta_{bd}{\overline{e}^d}_{\nu}(I)\nn\\
&={(e^{-1})^\mu}_a(1){\overline{e}^a}_\mu(I){(e^{-1})^\mu}_c(1){\overline{e}^c}_{\nu}(I)\nn\\
&=\left(\left[e^{-1}(1)\overline{e}(I)\right]^2\right)^\mu_{~\rho}\,,
\end{align}
or, equivalently, in matrix notation,
\beqn
\sqrt{g^{-1}(1)g(I)}=e^{-1}(1)\overline{e}(I)\,.
\eeqn
Using ${\overline{e}(I)^a}_\mu$ in (\ref{newpotga}) as well as the identity
\beqn
\tilde{\epsilon}_{c_1\hdots c_d}=\sqrt{-\det g(1)}\,\tilde{\epsilon}_{\nu_1\hdots \nu_d}{(e^{-1})^{\nu_1}}_{c_1}(1)\hdots{(e^{-1})^{\nu_d}}_{c_d}(1)\,,
\eeqn
we can finally express the gauge invariant potential as 
\begin{align}\label{metrexp}
U_{I_1\hdots I_d}
=\sqrt{-\det g(1)}\,&\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{\nu_1\hdots \nu_d}
{L^{\nu_1}}_{\lambda_1}(I_1)\left[\sqrt{g^{-1}(1)g(I_1)}\right]^{\lambda_1}_{~\mu_1}\hdots \nn\\
&\hdots{L^{\nu_d}}_{\lambda_d}(I_d)\left[\sqrt{g^{-1}(1)g(I_d)}\right]^{\lambda_d}_{~\mu_d}\,.
\end{align}
Here we have defined new St\"uckelberg fields with coordinate indices,
\beqn
{L^{\nu}}_{\lambda}(I)\equiv{(e^{-1})^{\nu}}_{a}(1){\Lambda^{a}}_{b}(1,I){e^b}_{\lambda}(1)\,.
\eeqn
Equation~(\ref{metrexp}) is the metric expression for the multivielbein theory of~\cite{Hinterbichler:2012cn}. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The ${L^{\nu}}_{\lambda}(I)$ equations.}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Varying the multivielbein action~(\ref{multac}) with interaction potential~(\ref{metrexp}) with respect to the ${L^{\nu}}_{\lambda}(I)$ gives $d(d-1)/2$ constraint equations for each~$I=2,\hdots,\mathcal{N}$, that can be used to eliminate the St\"uckelberg fields from the action. These equations replace the constraints~(\ref{constvierb}) that arose in the gauge fixed version of the theory. 

When trying to solve the ${L^{\nu}}_{\lambda}(I)$ equations for Lorentz degrees of freedom, one encounters a subtlety. Namely, the conditions that follow from the invariance of $\eta_{ab}$ under Lorentz transformations and reduce the number of independent components in ${L^{\nu}}_{\lambda}(I)$ to $d(d-1)/2$ read 
\beqn
{(L^\mathrm{T})_\mu}^\rho(I)g_{\rho\sigma}(1){L^\sigma}_\nu(I)=g_{\mu\nu}(1)\,,
\eeqn 
which imply that ${L^{\nu}}_{\lambda}(I)$ depends on the metric $\gmn(1)$. In order to extract the metric independent part, we therefore use the Caley transform of a Lorentz transformation to express the St\"uckelberg fields in terms of antisymmetric matrices $A_{\mu\nu}(I)$,
\beqn
{L^{\nu}}_{\lambda}(I)=\Big(\big[g(1)+A(I)\big]^{-1}\big[g(1)-A(I)\big]\Big)^\mu_{~\nu}\,.
\eeqn
Since the antisymmetry condition on $A_{\mu\nu}(I)$ is completely independent of the metric $\gmn(1)$, we can parameterize the gauge degrees of freedom in terms of its components.
The equations for the $A_{\rho\sigma}(I)$ are then obtained from
\beqn
\frac{\delta S_\mathrm{multi}}{\delta A_{\rho\sigma}(I)}=\frac{\delta {L^{\mu}}_{\nu}(I)}{\delta A_{\rho\sigma}(I)}\frac{\delta S_\mathrm{int}}{\delta {L^{\mu}}_{\nu}(I)}=0 \,.
\eeqn
Multiplying by $(g(1)-A(I))_{\rho\alpha}(g(1)-A(I))_{\sigma\beta}$ and evaluating the first factor results in
\beqn\label{Lconstr}
\Big({L^\mu}_\alpha(I)g_{\beta\nu}(1)-{L^\mu}_\beta(I)g_{\alpha\nu}(1)\Big)\frac{\delta S_\mathrm{int}}{\delta {L^{\mu}}_{\nu}}=0\,.
\eeqn
As explained in {\protect{\hyperref[papIV]{Paper IV}}}, these $(\mathcal{N}-1)\cdot d(d-1)/2$ equations can indeed be shown to be equivalent to the constraints~(\ref{constvierb}) on the gauge fixed vielbeins ${E^a}_\mu(I)$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Recovering bimetric interactions}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We would now like to address the question under what circumstances the interaction potential~(\ref{metrexp}) is writable in terms of metrics alone without having to introduce St\"uckelberg fields. 
In principle, plugging back the solution to the constraint equations~(\ref{Lconstr}) into the action will always result in a theory involving only the metrics, but in reality the explicit solution for the St\"uckelberg fields is difficult to obtain in the general case. In particular, the constraints may need to be solved componentwise, resulting in a noncovariant expressions for the interaction potential in terms of metrics alone.

Nevertheless, there is one case in which the situation is greatly simplified. Suppose we demand the interactions to be expressible in terms of $\sqrt{g^{-1}(1)g(I)}$ after integrating out the St\"uckelberg fields . The only obvious situation in which this requirement is satisfied is when the constraint equations~(\ref{Lconstr}) allow for solutions ${L^{\nu}}_{\lambda}(I)=\delta^\nu_\lambda$, or, equivalently, $A_{\mu\nu}(I)=0$. If that is the case, then on this solution~(\ref{Lconstr}) reduces to
\beqn\label{LconstrA0}
\left.\left(\frac{\delta S_\mathrm{int}}{\delta L^{\mu\nu}}-\frac{\delta S_\mathrm{int}}{\delta L^{\nu\mu}}\right)\right|_{A=0}=0\,,
\eeqn
where we have raised the index on ${L^{\nu}}_{\lambda}(I)$ with $g(1)^{\lambda\mu}$.
We will now argue that (\ref{LconstrA0}) together with $A_{\mu\nu}(I)=0$ is a consistent solution if the interaction potential contains only interactions between two vierbeins ${e^a}_\mu(1)$ and ${e^a}_\mu(2)$. In that case, namely, a generic term in the potential reads
\begin{align}\label{potfortv}
\sqrt{-\det g(1)}~&\tilde{\epsilon}^{\mu_1\hdots\mu_n\lambda_{n+1}\hdots\lambda_{d}}\tilde{\epsilon}_{\nu_1\hdots \nu_d \lambda_{n+1}\hdots\lambda_{d}}\nn\\
&~~~~~~~~~~~~\cdot L^{\nu_1\kappa_1}(2)S_{\kappa_1\mu_1}
\hdots 
L^{\nu_n\kappa_n}(2)S_{\kappa_n\mu_n}\,,
\end{align}
where we have defined the symmetric matrix
\beqn
S_{\kappa\mu}\equiv g(1)_{\kappa\rho}\left(\sqrt{g^{-1}(1)g(2)}\right)^\rho_{~\mu}\,.
\eeqn
Now take the variation of (\ref{potfortv}) with respect to $L^{\mu\nu}$ and in that set $A_{\mu\nu}(2)=0$, i.e.~$L^{\mu\nu}(2)=g^{\mu\nu}$. This gives an expression involving terms that are proportional to powers of $S_{\mu\nu}$. As a consequence of the symmetry of $S_{\mu\nu}$, this expression is symmetric itself. Therefore all terms in the variation of $S_\mathrm{int}$ with respect to $L^{\mu\nu}$ are symmetric when evaluated on $A_{\mu\nu}(2)=0$ and hence (\ref{LconstrA0}) holds. This shows that $A_{\mu\nu}(2)=0$ is indeed a solution to the constraint equations in this case, and thus integrating out the St\"uckelberg fields results in the Hassan-Rosen bimetric action with potential~(\ref{potantisym}).

Using the same arguments as above, it is easy to see that this result carries over to the case of $\mathcal{N}$ vielbeins with only bimetric interactions. The equivalent metric description is of the form~(\ref{gencv}). We conclude that the vielbein theories that possess straightforward reformulations in terms of metrics alone precisely correspond to graphs of the form shown in the left panel of Figure~4.2. In order to build more complicated interactions, such as loops and $n$-point vertices with $n>2$, one must invoke the St\"uckelberg fields ${L^{\nu}}_{\lambda}$ and solve their equations in a nontrivial way.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Bimetric Cosmology}
\label{ch:cosmo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


On small scales General Relativity makes very good predictions and, from a phenomenological point of view, there is no need to look for a modification of the theory. On cosmological states, however, it seems that either quantum field theory or gravity (or both) have to be modified in order to explain the observed value of the cosmic acceleration. Therefore, once a consistent theory of modified gravity has been constructed, its implications for cosmology are of great interest. Self-accelerating solutions of massive gravity have, for instance, been considered in \cite{deRham:2010tw, Gumrukcuoglu:2011ew}, and the hope was that a large cosmological constant could be screened out by the graviton mass that weakens gravity at large scales. However, this does not seem to be possible without fine tuning \cite{Hassan:2011vm}. In \cite{D'Amico:2011jj} the authors show that there exist no homogeneous and isotropic solutions in the dRGT model of Massive Gravity with flat reference metric. On the other hand, our analysis of bimetric theory with dynamical reference metric shows that in this framework such solutions do exist. The simplest examples are the proportional backgrounds considered in section~\ref{secpropbg} which, however, exist only for proportional sources. In this chapter we consider a different class of solutions for which one of the sources is set to zero. 
The existence of cosmological solutions in bimetric theory, in turn, implies their presence in Massive Gravity with a general homogeneous and isotropic reference frame. Homogeneous and isotropic solutions in bimetric gravity are the subject of {\protect{\hyperref[papII]{Paper~II}}} and have also been investigated in two further articles~\cite{Volkov:2011an, Comelli:2011zm} that appeared roughly at the same time. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Standard cosmology in General Relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Before discussing homogeneous and isotropic solutions in bimetric gravity, let us briefly review the derivation of the cosmological evolution equations in GR. To this end, we consider the Einstein-Hilbert action in $d=4$ including a cosmological constant term as well as a standard coupling of the metric $\gmn$ to matter,
\beqn
S_\mathrm{EH+m}=\frac{1}{M_\mathrm{PL}^2}\int\dd^4x\sqrt{-g}~\big(R-2\Lambda\big)+\int\dd^4x\sqrt{-g}~\mathcal{L}_m
\eeqn
The equations of motions for $\gmn$ obtained from this action read
\beqn\label{einsteq}
R_{\mu\nu}-\frac{1}{2}\gmn R=\frac{1}{M_\mathrm{PL}^2}\left(T_{\mu\nu}-\rho_\Lambda\,\gmn\right)\,,
\eeqn
where $T_{\mu\nu}$ is the stress-energy tensor obtained from variation of the matter Lagrangian as in (\ref{strente}) and we have defined the constant energy density $\rho_\Lambda\equiv\Lambda M_\mathrm{PL}^2$. 

When looking for homogeneous and isotropic solutions in general relativity, one makes a Friedmann-Robertson-Walker ansatz for the metric,
\beqn\label{FRWg}
\gmn \md x^\mu\md x^\nu=-\md t^2+a(t)^2\left(\frac{1}{1-kr^2}\md r^2+r^2\md \Omega\right)\,,
\eeqn
in which $k=0,-1,+1$ parameterizes the curvature of the universe (flat, open, closed), $a(t)$ is the scale factor, and $\md \Omega=\md \theta^2+\sin^2 \theta\,\md \varphi^2$. 
In accordance with homogeneity and isotropy, the stress-energy tensor is taken to be that of a perfect fluid, 
\beqn\label{setans}
{(T^g)^{\mu}}_\nu=\mathrm{diag}(-\rho, p, p, p)\,,
\eeqn
where $\rho(t)$ and $p(t)$ are the time dependent energy density and pressure of the fluid, respectively. As a consequence of the Bianchi identity the source is automatically covariantly conserved which implies the continuity equation,
\beqn\label{conteq}
\dot{\rho}+3\frac{\dot{a}}{a}\big(\rho+p\big)=0\,,
\eeqn
where dots denote time derivatives. This equation is actually nothing but the first law of thermodynamics, $\dd E=-p\,\dd V$, for an adiabatic expansion with volume $V=a^3$ and energy $E=\rho a^3$. 

Plugging the diagonal ans\"atze~(\ref{FRWg}) and~(\ref{setans}) into Einstein's equations~(\ref{einsteq}) gives a set of four equations. The 00-component is Friedmann's equation,
\beqn\label{Friedmann}
\left(\frac{\dot{a}}{a}\right)^2+\frac{k}{a^2}=\frac{\rho+\rho_\Lambda}{3M_\mathrm{PL}^2}\,,
\eeqn 
which is often expressed in terms of the Hubble parameter $H\equiv \dot{a}/a$.
Due to the isotropic ansatz, the $ii$-components of the equations are all equivalent and therefore only provide one additional independent equation. The most common way to present it is by taking the traced Einstein equations and using~(\ref{Friedmann}) to arrive at the acceleration equation,
\beqn\label{acceq}
\frac{\ddot{a}}{a}=-\frac{1}{6M_\mathrm{PL}^2}\left(\rho+\rho_\Lambda+3p\right)\,.
\eeqn
In fact, integrating the acceleration equation~(\ref{acceq}) and using the continuity equation~(\ref{conteq}) gives back the Friedmann equation~(\ref{Friedmann}), where $k$ enters as an integration constant. This is expected because the continuity equation is obtained from taking the divergence of Einstein's equations and is therefore already contained in the equations of motion. To specify a solution it is therefore sufficient to consider only two out of the three equations. 

In order to characterize different components of the cosmological fluid, one introduces the equation of state parameter $w$ defined as the ratio of pressure and energy density, $p=w\rho$. One can then rewrite the continuity equation~(\ref{conteq}) as 
\beqn
\frac{\dd \rho}{\dd a}+3(1+w)\frac{\rho}{a}=0\,,
\eeqn
which is solved by
\beqn
\rho=\rho_0\, a^{-3(1+w)}\,.
\eeqn
Here, $\rho_0$ is a constant to be determined by boundary conditions. Inserting this solution into the Friedmann equation~(\ref{Friedmann}) with $k=0$ and $\rho_\Lambda=0$ gives the following evolution of the scale factor for $w\neq -1$,
\beqn
a~\propto~ t^{\frac{2}{3(1+w)}}\,.
\eeqn
The behaviour for $w=-1$ is
\beqn
a~\propto~ e^{Ht}\,,\qquad H\equiv \frac{\dot{a}}{a}=\mathrm{const}.
\eeqn
Moreover, from the acceleration equation~(\ref{acceq}) we infer that, in the absence of a bare cosmological constant, the expansion of the universe accelerates for $w<-1/3$ and decelerates for $w>-1/3$. Three cases are of particular interest: $w=0$ characterizes nonrelativistic matter, $w=1/3$ corresponds to relativistic matter (``radiation"),  and $w=-1$ describes a cosmological constant. The energy density for nonrelativistic matter therefore scales as $a^{-3}$, i.e.~inversely proportional to the volume. Nonrelativistic matter experiences an additional redshift and its energy density goes as $a^{-4}$. None of these can explain an accelerated expansion of the universe. In contrast, a cosmological constant which of course has constant energy density leads to an exponentially accelerated expansion. 

It is common to measure the contributions of different fluid components in terms of their density parameters,
\beqn
\Omega_i=\frac{\rho_i}{3M_\mathrm{PL}^2 H_0^2},
\eeqn
where $i$ stands for either radiation, nonrelativistic matter or the cosmological constant and $H_0$ denotes the Hubble parameter at the present time. One also defines a curvature contribution, $\Omega_k=-\tfrac{k}{a^2H_0^2}$, and in terms of these the Friedmann equation becomes
\beqn
\Omega_\mathrm{rad}+\Omega_\mathrm{mat}+\Omega_\Lambda+\Omega_k=\frac{H^2}{H^2_0}\,.
\eeqn 
In particular, at the present time the density parameters add up to one. Latest observational data \cite{Hinshaw:2012aka, Ade:2013ktc} suggest the following values for the cosmological parameters at the present time,
\beqn
&~&H_0\sim 70\, \mathrm{km/s/Mpc}\,,\qquad \Omega_\mathrm{rad}\sim 10^{-5}\,,\qquad \Omega_\mathrm{mat}\sim 0.3 \,,\nn\\
&~&\Omega_\Lambda\sim 0.7\,,\qquad\qquad\qquad~~~\,   \Omega_k< 10^{-3}\,.
\eeqn
These values imply that our universe is flat and dominated by a cosmological constant component. As already discussed in the introduction, the energy density corresponding to this cosmological constant is extremely small compared to energy scales of the Standard Model of Particle Physics. Since so far we lack an explanation for this small value, the curious energy component $\rho_\Lambda$ is often referred to as \textit{Dark Energy}. On top of that, observations also show that the matter component $\Omega_\mathrm{m}$ is not dominated by familiar baryonic matter, but rather mainly consists of an unknown \textit{Dark Matter} component. These findings are summarized in the pie chart of Figure~5.1. 
 \begin{figure}[ht]
    \begin{center}
    \includegraphics[width=220pt]{Pictures/WMAP.pdf}
    \caption{Distribution of energy in the present universe. \textit{Credit: NASA/WMAP Science Team.}}
    \end{center}\label{figWMAP}
    \end{figure}
Consequently, under the assumption that General Relativity is indeed the theory of gravity, we must accept that 95$\%$ of the universe's energy content is not at all understood. Nevertheless, when this obscurity is ignored, the so-called $\Lambda$CDM model (GR with a cosmological constant and cold dark matter) fits the observational data very well.

Alternatively, we may question the validity of Einstein's theory of gravity and try to modify it on small distance scales such that it can account for one or both of the dark components in our universe. An example for a consistent infrared modification is bimetric gravity, which motivates us to derive and study the analogue of Friedmann's equation in this model. 

 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Cosmological evolution in bimetric theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In all of this chapter we work with the bimetric action (\ref{HR}) in four dimensions. Furthermore, in order to use the same conventions as in {\protect{\hyperref[papV]{Paper~V}}}, we replace the mass scale $m^4$ by $m^2m_g^2$. 
The coupling of $\fmn$ to matter is set to zero, which is of course a rather restrictive assumption. On the other hand, it allows us to interpret $\gmn$ as the metric in the usual way, provided that it has standard matter couplings.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsection{Homogeneous and isotropic ansatz} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

To keep the comparison of the bimetric solutions to those of General Relativity as simple as possible, we choose to make the usual Friedmann-Robertson-Walker ansatz for the metric $\gmn$ which is coupled to matter,
\beqn\label{FRWg}
\gmn \md x^\mu\md x^\nu=-\md t^2+a(t)^2\left(\frac{1}{1-kr^2}\md r^2+r^2\md \Omega\right)\,,
\eeqn 
It is now important to notice that, in order to arrive at this form, we have used time reparametrizations to remove one time-dependent function in the most general homogeneous and isotropic ansatz. We have therefore fixed the entire diffeomorphism invariance and there is no gauge symmetry left to do the same to $\fmn$.
As a result the most general homogeneous and isotropic ansatz for the second metric reads
\beqn\label{FRWf}
\fmn\md x^\mu\md x^\nu=-X(t)^2\md t^2+Y(t)^2\left(\frac{1}{1-kr^2}\md r^2+r^2\md \Omega\right)\,,
\eeqn
involving two time dependent functions $X(t)$ and $Y(t)$. Note also that we have assumed the curvatures $k$ of the two metrics to be the same. 

Furthermore, we use the perfect fluid form (\ref{setans}) for the stress-energy tensor ${(T^g)^{\mu}}_\nu$ of matter coupled to $\gmn$.
In GR any source is automatically covariantly conserved as a consequence of the Bianchi identity whereas in bimetric gravity the two sources for $\gmn$ and $\fmn$ are not necessarily separately conserved. But since here we have set $T^f_{\mu\nu}=0$, the diffeomorphism invariance of the Einstein Hilbert term and the interaction potential again imply $\nabla_g^\mu T_{\mu\nu}=0$ on-shell. 
This implies that the continuity equation~(\ref{conteq}) is also valid in the model under consideration.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evolution equations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, we consider the bimetric equations of motion, (\ref{geq}) and (\ref{feq}), with one index raised with the respective inverse metrics. Similarly to what we saw in GR, the symmetries of the cosmological ansatz ensure that it is sufficient to work with only part of the equations. Here, these are taken to be the $00$-components of the equations of motion, together with the continuity equation for the source, as well as the Bianchi constraint~(\ref{Bianchi}). The latter needs to be included because now the continuity equation makes up only a part of the divergence of the $\gmn$ equation. The $ii$-components of the equations of motion are then redundant. 

In what follows we shall refer to the $00$-components as simply the $\gmn$ and~$\fmn$ equation. Plugging the ans\"atze of the previous section into (\ref{geq}) we can make use of known GR results to straightforwardly obtain the $\gmn$ equation,
\beqn\label{gmncos}
\left(\tfrac{\dot{a}}{a}\right)^2+\tfrac{k}{a^2}-\tfrac{m^2}{3}\left[\beta_0+3\beta_1\tfrac{Y}{a}+3\beta_2\left(\tfrac{Y}{a}\right)^2+\beta_3\left(\tfrac{Y}{a}\right)^3\right]=\tfrac{\rho}{3m_g^2}\,.
\eeqn
In order to determine how different source components influence the cosmological evolution, we need to determine the function $Y(t)$ from the other equations. We start with the Bianchi constraint~(\ref{Bianchi}), evaluated on the homogeneous and isotropic ansatz, 
\beqn\label{bianchiev}
\tfrac{3m^2}{a}\left[\beta_1+2\beta_2\tfrac{Y}{a}+\beta_3\left(\tfrac{Y}{a}\right)^2\right]\left(\dot{Y}-\dot{a}X\right)=0\,.
\eeqn
There are two options to satisfy this equation; either the first or the second bracket must vanish: 
%%%%%%%%%%%%%%%%
\begin{itemize}

\item[\textbf{(1)}] If the parameters of the theory obey $\beta_1+2c\beta_2+c^2\beta_3=0$ for some constant $c$, then one solution is provided by $Y(t)=c \,a(t)$. In this case, the contribution from the interaction potential in~(\ref{gmncos}) reduces to a cosmological constant term. The $\gmn$ equation hence simply becomes the Friedmann equation~(\ref{Friedmann}) with a cosmological constant $\Lambda=m^2(\beta_0+3c\beta_1+3c^2\beta_2+c^3\beta_3)$. Interestingly, around proportional backgrounds, $\fmn=c^2\gmn$, the Fierz-Pauli mass of the massive perturbation is proportional to the combination of $\beta_n$ parameters in~(\ref{bianchiev}). It therefore vanishes on this particular background if the Bianchi constraint is satisfied by setting the first bracket in~(\ref{bianchiev}) to zero. This may imply an interesting phenomenology for the perturbations, but due to its degeneracy with GR at the background level, the solution is not of great interest to us here. 


\item[\textbf{(2)}] The alternative solution to the Bianchi constraint is $X(t)={\dot{Y}}/{\dot{a}}$. In contrast to the above, this is a dynamical equation and allows for much more general solutions. Since we are mostly interested in solutions that do not show the exact same behaviour as in GR, we focus on this branch in the following. Note also that, in fact, this constitutes no loss of generality because
setting the second bracket in~(\ref{bianchiev}) to zero still includes the proportional spatial metrics as possible solutions.

\end{itemize}
%%%%%%%%%%%%%%%%
Next, we turn to the $\fmn$ equation. Since the ansatz for $\fmn$ contains an extra time-dependent function in the 00-component, the derivative terms in this equation will look more complicated than the expressions familiar from GR. We derive them in the appendix of {\protect{\hyperref[papV]{Paper~V}}}. 
After eliminating $X(t)$ using the solution to the Bianchi constraint, the $\fmn$ equation reads 
\beqn
\left(\tfrac{\dot{a}}{Y}\right)^2+\tfrac{k}{Y^2}-\tfrac{m^2}{3\alpha^2}\left[\beta_1\left(\tfrac{a}{Y}\right)^3+3\beta_2\left(\tfrac{a}{Y}\right)^2+3\beta_3\tfrac{a}{Y}+\beta_4\right]=0\,,
\eeqn
where, as usual,\footnote{Note that in {\protect{\hyperref[papV]{Paper~V}}} the ratio of the Planck masses is denoted by $M_*$ instead of~$\alpha$.} $\alpha\equiv m_f/m_g$.
Multiplying this equation by $Y^2/a^2$ and subtracting it from the $\gmn$ equation (\ref{gmncos}) yields an algebraic equation,
\begin{align}\label{polynom}
\frac{\beta_3}{3}\Upsilon^4+\left(\beta_2-\tfrac{\beta_4}{3\alpha^2}\right)\Upsilon^3&+\left(\beta_1-\tfrac{\beta_3}{\alpha^2}\right)\Upsilon^2\nn\\
&+\left(\rho_*+\tfrac{\beta_0}{3}-\tfrac{\beta_2}{\alpha^2}\right)\Upsilon-\tfrac{\beta_1}{3\alpha^2}=0\,.
\end{align}
We have expressed this in terms of the dimensionless quantities,
\beqn
\Upsilon=\frac{Y}{a}\,,\qquad \rho_*=\frac{\rho}{3m_g^2m^2}\,.
\eeqn
Now we would like to solve equation (\ref{polynom}) for $\Upsilon$ and plug the solution back into the $\gmn$ equation~(\ref{gmncos}). After that, this equation will only contain $a(t)$, $\dot{a}(t)$ and $\rho(t)$ and thus becomes a modified Friedmann equation. The quartic polynomial equation (\ref{polynom}) can be solved numerically for $\Upsilon$. The general solution, however, is not very transparent. Instead, one can fix one or several of the $\beta_n$ parameters and investigate these constrained parameter spaces for simpler solutions. In {\protect{\hyperref[papII]{Paper~II}}}, we focus on parameter choices that allow for solutions close to those of GR.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Degeneracy with General Relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Consider, for example, the choice $\beta_3=0$. In this case, (\ref{polynom}) reduces to a cubic equation for $\Upsilon$ whose solutions will already look simpler. An even greater simplification is achieved if we in addition put $\beta_1=0$. Then the equation for $\Upsilon$ is a quadratic and a solution is readily obtained. Plugging it into the $\gmn$ equation~(\ref{gmncos}) then gives
\beqn\label{deggrcase}
\left(\frac{\dot{a}}{a}\right)^2+\frac{k}{a^2}=\frac{\rho}{3\bar{M}_\mathrm{Pl}^2}+\frac{\rho_\Lambda}{3\bar{M}_\mathrm{Pl}^2}\,,
\eeqn
where we have introduced a modified Planck mass and an effective constant energy density,
\beqn
\bar{M}_\mathrm{Pl}^2=\frac{m_g^2(\beta_4-3\beta_2\alpha^2)}{\beta_4}\,,\quad~~~~ \rho_\Lambda=\frac{m^2(\beta_0\beta_4-9\beta_2^2)}{\beta_4}\,.
\eeqn
Evidently, this is simply the usual Friedmann equation~(\ref{Friedmann}). The bimetric solution in this model is therefore indistinguishable from standard GR cosmology. This is a nontrivial result because the nonlinear theories themselves are very different due to the $\beta_2$-interaction term of bimetric theory. These differences are expected to show up at the level of perturbations. Bimetric perturbation theory around homogeneous and isotropic solutions has been studied in~\cite{Comelli:2012db, Berg:2012kn}. 

Turning on $\beta_1$ takes us smoothly away from the solutions that are degenerate with GR. Consequently, as shown in {\protect{\hyperref[papV]{Paper~V}}}, for small values of $\beta_1$ it is still possible to fit the model to cosmological data. For larger values the predictions of the bimetric model become incompatible with observations.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To summarize, the main conclusion of {\protect{\hyperref[papII]{Paper~II}}} is that there exist nontrivial (i.e.~interacting) models of bimetric gravity with cosmological solutions in agreement with observational data. Hence, the Hassan-Rosen bimetric theory passes one of the first tests for being a valid theory of gravity. In the model where $\beta_1=\beta_3=0$, the cosmological constant is a combination of contributions from the matter source   (which can be absorbed in $\beta_0$) and the bimetric interaction potential. Fitting it to its observed value still involves fine tuning of the parameters and the cosmological constant problem remains unsolved. The situation is somewhat improved for other choices of $\beta_n$, as will be discussed in the next section. 

Another important point is that it is far from clear whether the effective Planck mass in~(\ref{deggrcase}) is the same as the one that would enter spherically symmetric solutions. In GR the Planck mass in Friedmann's equation is the same as the one that enters the gravitational constant in the Newtonian limit and it is this value that has been used to fit the cosmological data. However, if in bimetric gravity the effective Planck mass on cosmological scales turns out to be different than the one on smaller scales, the model would most likely not be compatible with observations. Since so far not much is known about spherically symmetric solutions in bimetric gravity,\footnote{See however \cite{Comelli:2011wq, Volkov:2012wp}, where some progress has been made towards finding spherically symmetric solutions.} this investigation is still an open task.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Self-acceleration}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The purpose of~{\protect{\hyperref[papII]{Paper~II}}} was to demonstrate the existence of viable cosmological solutions in bimetric gravity. A more thorough statistical analysis of the whole parameter space was conducted in~\cite{Akrami:2012vf}. The authors used data from observations of the cosmic microwave background, baryon acoustic oscillations, type Ia supernovae, and the present value of the Hubble parameter to constrain different bimetric models.\footnote{See also~\cite{Akrami:2013ffa} where a similar analysis is performed in a model including matter couplings for $\fmn$ .} In particular, they investigate whether models with $\beta_0=0$ and no cosmological constant contribution from the matter source can give rise an expansion history compatible with observations. In the absence of a constant vacuum energy density driving the acceleration of the universe's expansion, the model has to be \textit{self-accelerating}, i.e.~the observed acceleration must stem from modified terms in Friedmann's equation. Indeed, self-accelerating solutions are found for many different combinations of nonzero $\beta_n$ parameters in bimetric gravity and, in fact, the fits to data are just as good as for the ordinary $\Lambda$CDM model.

The best fit value for the mass of the massive spin-2 field is on the order of the Hubble scale $H_0$. Since in the zero-mass limit the full diffeomorphism symmetry that transforms the two metrics separately is restored, a small spin-2 mass is technically natural. In the ideal case, bimetric theory should also explain why we do not observe the large cosmological constant predicted by quantum field theory, for instance it should provide a mechanism to screen out a large vacuum energy. To our present knowledge, this is not the case, except maybe for the parameters of the partially massless theory, discussed in chapter~\ref{ch:PM}. However, if an explanation for the absence of a large cosmological constant was found elsewhere, the Hubble scale set by the spin-2 mass could be radiatively stable, which would be a large step towards solving the cosmological constant problem.  



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Partially Massless Bimetric Theory}
\label{ch:PM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A massive spin-2 field in de Sitter (dS) background exhibits several interesting features that are neither shared by lower-spin particles nor by spin-2 excitations in flat space. For a special value of the Fierz-Pauli mass in units of the background curvature, the linear theory possesses an additional gauge symmetry which removes one of the spin-2 helicity components. In this case, where the field loses one propagating degree of freedom, it is referred to as \textit{partially massless} (PM). The particular mass value for which this situation occurs is called \textit{Higuchi bound} because it divides the parameter region into unitary and nonunitary subsectors~\cite{Higuchi:1986py}. 
%Below the Higuchi bound the helicity-zero mode of the spin-2 particle develops a ghost instability, whereas above the bound the the theory is healthy. 
%The Higuchi bound is therefore a particularly interesting line in parameter space. 

Being in the possession of a nonlinear theory that involves a massive spin-2 field, we are able to address the following question: Is the concept of partial masslessness restricted to the linear theory around de Sitter backgrounds or can it be extended to the nonlinear level? The demand on a nonlinear PM theory is the presence of an extra gauge symmetry, even away from de Sitter backgrounds. In {\protect{\hyperref[papVI]{Paper~VI}}} we develop a method to identify a unique candidate for a nonlinear PM bimetric theory in four spacetime dimensions. The analysis is extended to higher dimensions in {\protect{\hyperref[papVII]{Paper~VII}}}, where it is found that pure bimetric theory cannot give rise to partial masslessness at the nonlinear level. We therefore modify the bimetric action by adding the Lanczos-Lovelock terms and show that in this generalized framework it again becomes possible to single out PM candidates .




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Partial masslessness in de Sitter background}\label{seclinPM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us begin by reviewing the linear theory of a PM spin-2 particle in a de Sitter background, which was first discussed in a sequence of papers by Deser et.al.~\cite{Deser:1983mm, Deser:2001pe, Deser:2001us, Deser:2001wx, Deser:2001xr, Deser:2004ji, Deser:2006zx}. 
The equation of motion for a massive spin-2 fluctuation $h_{\mu\nu}$ in a de Sitter background $\bar{G}_{\mu\nu}$ with positive cosmological constant $\Lambda$ is given by
\beqn\label{lineqds}
{\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}h_{\rho\sigma}-\tfrac{2\Lambda}{d-2}\left(h_{\mu\nu}-\tfrac{1}{2}\bar{G}_{\mu\nu} h\right)
+\tfrac{m^2_\mathrm{FP}}{2}\Big(h_{\mu\nu}-\bar{G}_{\mu\nu} h\Big)=0\,,
\eeqn
where the derivative operator ${\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}$ is given in (\ref{kinopds}). For general values of the Fierz-Pauli mass, the equation possesses no gauge symmetries. Similarly to its analogue in flat space that was discussed in detail in section~\ref{sec:FP}, it contains $d+1$ constraint equations that reduce the number of propagating degrees of freedom to $(d(d-1)/2-1)$, appropriate for a massive spin-2 particle.

A feature of (\ref{lineqds}) without any analogue in flat space is that if the Fierz-Pauli mass saturates the Higuchi bound, $m^2_\mathrm{FP}=\frac{2}{d-1}\Lambda$, the equation is invariant under a new gauge symmetry. The corresponding linear gauge transformation reads
\beqn\label{linPMsym}
\Delta (\hmn) = \bar{\nabla}_\mu\partial_\nu\xi(x)+\tfrac{2\Lambda}{(d-1)(d-2)} \bar{G}_{\mu\nu}\, \xi(x)\,,
\eeqn
in which $\xi(x)$ is a local gauge parameter.
Moreover, if the value for the mass lies below the bound, the theory is nonunitary because the helicity-zero mode of the massive spin-2 field becomes a ghost \cite{Higuchi:1986py, Higuchi:1989gz}. Above the Higuchi bound the theory is well-behaved. 

Besides computing the variation of~(\ref{lineqds}) under the gauge transformation explicitly, there is another straightforward way to see the existence of a gauge symmetry in the equation for the massive spin-2 field with mass at the Higuchi bound. First take the double divergence of~(\ref{lineqds}) to arrive at
\beqn\label{doublediv}
\bar{\nabla}_\nu\bar{\nabla}_\mu\left(\bar{G}^{\mu\nu} \bar{G}^{\rho\sigma}-\bar{G}^{\mu\rho}\bar{G}^{\nu\sigma}\right)h_{\rho\sigma}=0\,.
\eeqn
The kinetic terms have dropped out after using the linearized Bianchi identity.
Furthermore, the trace of (\ref{lineqds}) is given by
\beqn
\tfrac{d-2}{2}\,\bar{\nabla}_\nu\bar{\nabla}_\mu\left(\bar{G}^{\mu\nu} \bar{G}^{\rho\sigma}-\bar{G}^{\mu\rho}\bar{G}^{\nu\sigma}\right)h_{\rho\sigma}+\left(\Lambda-\tfrac{d-1}{2}m^2_\mathrm{FP}\right)h=0\,.
\eeqn
If the mass is at the Higuchi bound, the terms without derivatives in this equation vanish identically, while the derivative terms are zero due to~(\ref{doublediv}).
Hence we find that for $m^2_\mathrm{FP}=\frac{2}{d-1}\Lambda$ the traced equations of motion are identical to their double divergence. Put differently, when multiplied by the appropriate factors, the difference of the trace and the double divergence is identically zero.
This identity signals the presence of a gauge symmetry. Since one particular combination of the equations of motion is identically satisfied, one component of $\hmn$ remains undetermined.  
In fact, a gauge identity of the above type even implies that the action is invariant under the corresponding gauge transformation. This follows from the fact that invariance of the action under~(\ref{linPMsym}) requires
\beqn
\Delta S=\frac{\delta S}{\delta \hmn}\Delta (\hmn)=0\,.
\eeqn
Since $\tfrac{\delta S}{\delta \hmn}$ is nothing else than the equation of motion for $\hmn$, after integrating by parts, we find that $\Delta S$ indeed vanishes due to the gauge identity. 

The conclusion is that the massive spin-2 field described by (\ref{lineqds}) with mass at the Higuchi bound has only $(d(d-1)/2-2)$ degrees of freedom, one less than is usually the case. Let us also remark that the existence of the gauge symmetry around de Sitter backgrounds is in agreement with the representation theory of the de Sitter group SO$(1,d)$, which allows for so-called \textit{partially massless} (PM) representations of higher-spin fields. For a discussion of this topic, consult e.g.~\cite{Garidi:2003ys}. The whole situation is summarized in Figure~6.1, where for definiteness we fix $d=4$.
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=200pt]{Pictures/dSPM.pdf}
    \caption{Unitary and nonunitary regions in the $\Lambda$-$m_\mathrm{FP}^2$-plane in $d=4$. The boundary of the shaded region corresponds to the Higuchi bound.}
    \end{center}
    \end{figure}

After the linear PM theory for spin-2 fields on de Sitter background had been established, it was attempted to construct higher order interactions for the perturbation $\hmn$ that would leave the gauge symmetry intact. At cubic order in $\hmn$ such a construction turned out to be possible in $d=4$~\cite{Zinoviev:2006im, Joung:2012rv}. In $d>4$, however, it was found that gauge invariant cubic vertices can only exist if one also includes higher derivative terms into the theory \cite{Zinoviev:2006im}. The construction of a fully nonlinear theory with a PM gauge symmetry remained an open task.



The remainder of this chapter summarizes the findings of {\protect{\hyperref[papVI]{Paper~VI}}} and {\protect{\hyperref[papVII]{Paper~VII}}} where we propose a nonlinear PM theory within the family of ghost-free bimetric theories. In particular, we show that in this framework it is possible to understand the outcome of the cubic-vertex analyses of~\cite{Zinoviev:2006im, Joung:2012rv}. We begin by explaining the properties of the candidate PM theory for the most relevant case of four space-time dimensions, before we generalize the arguments to $d>4$. Further remarkable features of the theory in $d=4$ will be presented in chapter~\ref{ch:HD} in the context of higher-curvature actions.


 
  
   
   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
\section{Towards a nonlinear PM theory}\label{secPmnonlin}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
It is natural to expect the nonlinear PM theory (if it exists) to be found within the family of ghost-free nonlinear theories for massive spin-2 fields. A first investigation of this possibility was carried out in \cite{deRham:2012kf} where the authors aimed to identify a PM theory in nonlinear Massive Gravity with the reference metric taken to be a fixed de Sitter background. Their construction used St\"uckelberg fields in a generalized decoupling limit and showed that, for a certain choice of the $\beta_n$-parameters, a scalar degree of freedom is not propagating. Although this seemed to be a solid argument for the presence of a gauge symmetry in the decoupling limit, it was later argued in \cite{Deser:2013uy, deRham:2013wv} that constructing a PM theory in the full theory of nonlinear Massive Gravity is impossible. Inspite of lacking a proof, another article also made similar negative statements about PM bimetric theory~\cite{Deser:2013gpa}.

Taking into account these objections, one could be worried about the possibility of constructing a PM bimetric theory. 
However, there are several reasons why the above no-go results need not concern us here:
First of all, the results of \cite{Deser:2013uy, deRham:2013wv} hold only for nonlinear Massive Gravity with fixed reference metric $\fmn$, and do not directly carry over to the ghost-free bimetric gravity where both metrics are dynamical. In fact, the analyses in these references merely show that in a nonlinear PM theory none of the metrics can be held fixed because both of them are expected to transform under the PM gauge symmetry. We will come back to this point in section~\ref{sec:PMMG}. Apart from this, the authors of \cite{Deser:2013uy, Deser:2013gpa} search for a nonlinear action with invariance under an infinitesimal PM gauge transformation and are unable to find it. The action will, however, not be invariant if the invariance is an on-shell symmetry of the equations of motion. In fact, it is possible to use the results we derive below to demonstrate that the nonlinear PM theory can only be invariant on-shell. This is part of an upcoming publication and beyond the scope of this thesis. However, we emphasize one more time that the no-go results of \cite{Deser:2013uy, deRham:2013wv, Deser:2013gpa} simply do not apply to the theory under consideration here.





In {\protect{\hyperref[papVI]{Paper~VI}}} we develop a method that allows us to identify a candidate PM theory within the family of ghost-free bimetric theories. To this end, we consider the proportional background solutions as well as the spectrum of linear perturbations around these that were discussed in section~\ref{sec:massspec}. This is a natural setup for extending the PM symmetry of perturbations around dS space because these backgrounds have constant curvature and, in particular, they are the only ones around which a massive fluctuation with Fierz-Pauli mass term exists. Our method is suitable for identifying or excluding PM candidates in bimetric theory in any space-time dimension. In this section, however, after outlining the general idea, we restrict to the case $d=4$. Dimensions greater than four will be the focus of section~\ref{PMdgf}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Identifying PM candidates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The equation of motion (\ref{dMeq}) for the massive fluctuation $\delta M_{\mu\nu}$ around proportional backgrounds is of the same form as (\ref{lineqds}) with $\Lambda=\bar{\Lambda}_g$.  
As a consequence, if the cosmological constant is assumed to be positive and if the Fierz-Pauli mass (\ref{FPmass}) is on the Higuchi bound, a gauge symmetry of the form (\ref{linPMsym}) is present in the linear theory around proportional backgrounds. In bimetric notation, the corresponding infinitesimal gauge transformation of the massive fluctuation reads
\beqn\label{linPMsym2}
\Delta (\delta M_{\mu\nu}) = \bar{\nabla}_\mu\partial_\nu\xi(x)+\tfrac{2\bar{\Lambda}_g}{(d-1)(d-2)} \bar{G}_{\mu\nu}\, \xi(x)\,.
\eeqn
On the other hand, the massless fluctuation does not transform under the PM symmetry, 
\beqn
\Delta (\delta G_{\mu\nu}) = 0\,.
\eeqn
This follows from the fact that its equation of motion (\ref{dGeq}) does not have any extra gauge symmetry besides the usual linearized diffeomorphism invariance. Therefore, $\delta G_{\mu\nu}$ itself must be invariant under the PM symmetry. 
The question is now under what conditions the above symmetry transformations for the fluctuations around dS background have a chance to be generalizable to the nonlinear level. 

Since the theory in terms of the nonlinear fields $M^G_{\mu\nu}$ and $G_{\mu\nu}$ has a very complicated form, we find it easier to work with the variables $\gmn$ and $\fmn$ instead. 
The above transformations of the mass eigenstates $\delta M_{\mu\nu}$ and $\delta G_{\mu\nu}$ allow us to uniquely determine the transformations of the fluctuations of $\gmn$ and $\fmn$ using the expressions for the massive and massless fluctuations given in (\ref{dGanddM}). The result is
\beqn\label{fgtrans}
\Delta (\delta\gmn)=-(\alpha c)^{\frac{d-2}{2}}\Delta (\delta\fmn)=\tfrac{-2(\alpha c)^{d-2}}{c(1+(\alpha c)^{d-2})}\Delta (\delta M_{\mu\nu})\,.
\eeqn
The crucial observation is now that in a theory with a gauge symmetry at the nonlinear level, it must be possible to shift these transformations of the fluctuations $\delta\gmn$ and $\delta\fmn$ to the backgrounds $\bgmn$ and $\bfmn$. This follows from the fact that the split into background and fluctuations is not unique and one can always take out part of the fluctuation to redefine the background. Therefore we demand that the symmetry transformations (\ref{fgtrans}) should also leave the background equations invariant. But since we are dealing with the proportional backgrounds, where the background equation is simply $\Lambda_g=\Lambda_f$ (c.f.~(\ref{propbackeq})), determining the proportionality constant $c^2$, we restrict ourselves to constant gauge transformations $\bar{\Delta}$ with $\xi(x)=$\,const. In this way we ensure that the transformation does not take us away from the proportional backgrounds and avoid unnecessary complication. 
The restriction to constant gauge transformations is a strong simplification, but as we will see now, demanding the background equation to be invariant under these is constraining enough to identify the PM candidate theory. Namely, it should be evident from (\ref{fgtrans}) that shifting the constant transformations to the backgrounds $\bgmn$ and $\bfmn=c^2\bgmn$ results in a shift in $c^2$,
\beqn
\bgmn\bar{\Delta}(c^2)= \bar{\Delta}(\bfmn)-c^2\bar{\Delta}(\bgmn)\,.
\eeqn
However, in general this cannot lead to an integrable\footnote{Integrability of the symmetry transformation means that it can be performed more than once and still leave the equations invariant. This is a natural requirement on any gauge symmetry. Without the integrability condition it is sufficient to set the mass to the Higuchi bound in order to have an invariant background.} symmetry of the background equations because $c$ is determined by $\Lambda_g=\Lambda_f$ and can therefore not be shifted. 
If this is the case, then a nonlinear PM symmetry cannot exist. The only possibility to avoid this immediate no-go statement is to demand that $c$ is not fixed by the background equation. 
Then, the equation $\Lambda_g=\Lambda_f$ that is automatically satisfied in this case (i.e.~without fixing $c$) is the gauge identity evaluated on the proportional backgrounds. Since making the proportional ansatz for the two metrics partly fixes the gauge, only constant scalings are left as residual transformations. The component of the metrics that remains undetermined by the equations therefore simply reduces to the constant $c$ on this solution. 

 
The whole idea will be made more explicit in the following, where we identify PM candidates in $d=4$, before we discuss the general case in the next section.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{PM candidate in $d=4$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In four space-time dimensions, the explicit expressions~(\ref{lambdas}) for the cosmological constants in terms of the $\beta_n$ parameters, the ratio of Planck masses $\alpha$ and the proportionality constant $c$ can be used to write the background condition $\Lambda_g=\Lambda_f$ as a polynomial equation for $c$,
\begin{align}
\beta_1+c(3\beta_2-\alpha^2\beta_0)&+3c^2(\beta_3-\alpha^2\beta_1)\nn\\
&+c^3(\beta_4-3\alpha^2\beta_2)-c^4\alpha^2\beta_3=0\,.
\end{align}
This equation clearly fixes $c$ unless all coefficients of different powers of $c$ vanish separately. A proportionality constant $c$ that is undetermined by the background equation therefore requires the following parameter choices in the bimetric interaction potential,
\beqn\label{PMpara}
\beta_1=\beta_3=0\,,\qquad \alpha^2\beta_0=3\beta_2=\alpha^{-2}\beta_4\,.
\eeqn
We will frequently refer to these values as the \textit{PM parameters}. Note that our requirement on the $\beta_n$-parameters fixes all but one of them uniquely in terms of the others and $\alpha$. The one remaining parameter is of course degenerate with the energy scale $m^4$ in the interaction potential and sets the scale for the Fierz-Pauli mass and the cosmological constant. Moreover, it is easy to check using the expressions (\ref{FPmass}) and (\ref{lambdas}) for $m_\mathrm{FP}^2$ and $\Lambda_g$, that the parameter choice (\ref{PMpara}) automatically puts the mass on the Higuchi bound. Therefore the theory of linear perturbations around the backgrounds at hand exhibits the usual PM gauge symmetry. It is worth emphasizing that we did not demand this in any way; it followed from an independent requirement on the background equations. 

On the other hand, we also make the following interesting observation: If we assume that there is a \textit{unique} PM theory, then satisfying the Higuchi bound is sufficient to determine its parameters. Namely, in this case, the symmetry (\ref{symbg}) of the interaction potential enforces $\alpha^{4-n}\beta_n=\alpha^{n}\beta_{4-n}$ because otherwise the theory obtained from replacing $\alpha^{4-n}\beta_n\rightarrow\alpha^{n}\beta_{4-n}$ would also be PM, contradicting the uniqueness requirement.
It is easy to see that this constraint on the $\beta_n$ parameters together with the Higuchi bound condition already implies (\ref{PMpara}).

We now turn to the requirement of integrability of the symmetry transformation. The constant parts of the PM symmetry transformations of the fluctuations can be written as 
\beqn\label{consttraf}
\Delta (\delta\gmn)=-\frac{2c\alpha^2}{1+(\alpha c)^2}\delta a\,\bgmn\,,\qquad \Delta (\delta\fmn)=\frac{2c}{1+(\alpha c)^2}\delta a\,\bgmn\,,
\eeqn
with  infinitesimal constant gauge parameter $\delta a$.
Furthermore, it is easy to check that with the PM parameters the background equations (\ref{bgeq}) are invariant under the nonlinear scaling transformations,
\beqn
\bgmn\rightarrow\frac{1+(\alpha c)^2}{1+\alpha^2(c+a)^2}\,\bgmn\,,\qquad \bfmn\rightarrow\frac{1+(\alpha c)^{-2}}{1+\alpha^{-2}(c+a)^{-2}}\,\bfmn
\eeqn
with finite constant gauge parameter $a$. Of course, these are simply the integrated versions of (\ref{consttraf}), verifying that the constant part of the gauge transformation is indeed integrable.
If the nonlinear PM symmetry exists, the above transformations constitute its form on the proportional backgrounds.

It is furthermore important to note that the Fierz-Pauli mass and cosmological constant, when taken with respect to the background metric~$\bar{G}_{\mu\nu}$, become independent of $c$,
\beqn
\bar{m}_\mathrm{FP}^2=\frac{2}{3}\bar{\Lambda}_g=2\beta_2\frac{m^4}{m_g^2}\,.
\eeqn
Hence, these can be regarded as physical quantities that do not depend on the gauge parameter $a$ that shifts the value of $c$.



By restricting to constant gauge transformations, clearly, we are not dealing with the full PM symmetry at the nonlinear level. Note, however, that since the set of constant transformations is a subset of the full gauge group, the theory we obtain by requiring invariance under this subset must contain the theory with the full gauge group (if it exists). Moreover, since in four dimensions the restriction to constant gauge transformations is sufficient to uniquely determine the $\beta_n$ parameters, we conclude that the resulting theory is already the unique candidate for having the full PM symmetry.

The scale invariance of the equations of motion for proportional backgrounds is not the only interesting property of the theory specified by the PM parameters. The PM candidate exhibits additional astonishing features that further support the existence of a gauge symmetry at the nonlinear level. For instance, consider again the homogeneous and isotropic solutions of {\protect{\hyperref[papII]{Paper~II}}} which we presented in chapter~\ref{ch:cosmo}. We saw that, after solving the Bianchi constraint, it was possible to arrive at (\ref{polynom}), an algebraic equation for the ratio of the two scale factors, $Y(t)/a(t)$. Inserting the PM parameters (\ref{PMpara}) into this equation, we find that it becomes an identity. Clearly, it is the analogue of the equation $\Lambda_g=\Lambda_f$ for proportional backgrounds. But instead of a constant, the equations evaluated on the cosmological ansatz now leave a time-dependent function undetermined. This shows that the cosmological evolution equations of PM bimetric theory are invariant under a symmetry that is local in time. Even if it eventually turns out that a PM symmetry does not exist in the nonlinear theory, a cosmological gauge symmetry could already be of interest on its own. 

Since, in four dimensions, the proportional backgrounds correspond to maximally symmetric space-times with ten independent Killing vectors and the homogeneous and isotropic solutions still possess six isometries, one might speculate that the presence of a symmetry on these solutions could somehow be related to the amount of symmetry of the underlying geometry. Then one could argue that a general solution with less symmetries than the above would not be invariant under any PM symmetry transformation. To invalidate this argument, it is therefore important to investigate the structure of our PM candidate theory away from the proportional and the cosmological backgrounds. This has been done in {\protect{\hyperref[papVIII]{Paper~VIII}}} which considers general perturbative solutions to the bimetric equations of motion. It turns out that the equations in the PM theory are conformally invariant to lowest order in a derivative expansion.
These remarkable results will be presented in section~\ref{secPMCG}.



To conclude this discussion, let us briefly mention that a PM candidate can also be obtained in $d=3$ where the background equation reads
\beqn
c(\beta_1-\alpha\beta_0)+2c^2(\beta_2-\alpha\beta_1)+c^3(\beta_3-\alpha\beta_2)=0\,.
\eeqn
Demanding this to leave $c$ undetermined results in the following PM parameters, 
\beqn
\beta_3=\alpha\beta_2=\alpha^2\beta_1=\alpha^3\beta_0\,.
\eeqn
Again, all but one of the $\beta_n$ parameters are fixed, and the Fierz-Pauli mass sits precisely on the Higuchi bound. 


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Massive gravity limit}\label{sec:PMMG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The PM parameters (\ref{PMpara}) in four space-time dimensions provide an example for a theory in which the coefficients in the interaction potential depend on the mass scale $m_f$ that is taken to infinity in the massive gravity limit that we discussed in section~\ref{sec:MGlim}. In this case, we have to be more careful when taking the limit because the $\beta_n$ parameters will scale as well. The conditions (\ref{PMpara}) fix the relative scale among them but their absolute scale may still be chosen freely. Suppose that $\beta_2$ does not scale when the limit $\alpha=m_f/m_g\rightarrow\infty$ is taken. Then $\beta_0\rightarrow 0$ and $\beta_4\rightarrow\infty$, whereas $\Lambda={\beta_4\,m^4}/{m_f^2}=\,$const.  In the Massive Gravity limit, the equations of motion for the PM theory thus reduce to
\beqn
\mathcal{G}_{\mu\nu}(g)
+\frac{\Lambda}{3}\,g_{\mu\lambda}{\big(Y^{(2)}\big)^\lambda}_{\nu}(S)&=&0\,, \label{gpm} \\
\mathcal{G}_{\mu\nu}(f)
+\Lambda\fmn&=&0 \,.\label{fpm}
\eeqn
Remarkably, these are exactly the equations singled out in \cite{deRham:2012kf, Deser:2013uy, deRham:2013wv} which investigated the possibility of realizing nonlinear partial masslessness in Massive Gravity with fixed reference metric. The methods invoked in those references are completely different from ours and hence provide independent support for the existence of a nonlinear PM symmetry. 

On the other hand, as we already mentioned previously, in \cite{Deser:2013uy, deRham:2013wv} it was also claimed that there is no nonlinear gauge symmetry present in (\ref{gpm}) and (\ref{fpm}). If correct, at first sight, this result might seem to rule out a nonlinear PM symmetry even in bimetric gravity because it should be possible to take the massive gravity limit to arrive at the above equations. There is, however, a caveat in this argument: If the symmetry transformation in PM bimetric gravity itself depends on $\alpha=m_f/m_g$, then it may become singular in the $\alpha\rightarrow\infty$ limit. In this case, it would not be consistent to only look for an invariance in (\ref{gpm}) and (\ref{fpm}) because terms in the original bimetric equations, that were neglected when taking the limit, could become relevant again due to the singular nature of the gauge transformation. In fact, our findings in chapter~\ref{ch:HD} suggest that the transformation of $\fmn$ indeed contains such singular terms and therefore the conclusions of \cite{Deser:2013uy, deRham:2013wv} are irrelevant for bimetric gravity. 


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
\section{Generalization to arbitrary dimensions}\label{PMdgf}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


In {\protect{\hyperref[papVII]{Paper~VII}}} we apply the procedure of identifying the candidate PM theories that we introduced in the previous section to bimetric theory in an arbitrary number of space-time dimensions. We find that in pure Hassan-Rosen bimetric theory there is no nonlinear PM theory for $d>4$. This outcome is in agreement with 3-vertex calculations~\cite{Zinoviev:2006im, Joung:2012rv}, which also suggest that it could be possible to find a nonlinear PM theory in higher dimensions if higher order derivative couplings are included into the theory. Inspired by these results we augment the bimetric action by the ghost-free Lanczos-Lovelock (LL) terms. In this LL-extended bimetric theory it is then possible to identify PM candidates even for $d>4$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background equation}\label{noPMdgeq5}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Let us first argue why in pure bimetric theory there is no PM candidate in dimensions greater than four. To this end, consider again the background equation $\Lambda_g=\Lambda_f$ which in $d$ dimensions assumes the following form,
\beqn\label{eqlad}
(\alpha c)^{d-2}\sum_{n=0}^{d-1}{d-1\choose n}c^n\beta_n
= \sum_{n=1}^{d}{d-1\choose n-1}c^n\beta_n\,.
\eeqn
As in the four-dimensional case, for $c$ to be undetermined by this polynomial equation, the coefficients of different powers of $c$ have to vanish separately. This requirement will again put constraints on the $\beta_n$-parameters and the ratio of Planck masses $\alpha$. It should be obvious that, for large $d$, the factor $c^{d-2}$ on the left-hand side produces a large number of terms with coefficients proportional to just one $\beta_n$-parameter. These $\beta_n$-parameters will then immediately forced to be zero. 
Explicitly, when multiplied by $c^{2-d}$, the above equation can be rewritten as
\beqn
\left( \alpha^{d-2}\sum_{n=0}^{d-1}{d-1\choose n}\beta_n-\sum_{n=3-d}^2{d-1\choose d+n-3}\beta_{n+d-2} \right)c^n=0\,.
\eeqn
In $d\geq 5$, demanding the coefficients of $c^n$ to vanish for $3-d\leq n\leq d-1$ then leads to the following constraints on the parameters,
\begin{align}
0&=\alpha^{d-2}{d-1\choose n}\beta_n-{d-1\choose d+n-3}\beta_{n+d-2} \qquad\text{for}\quad0\leq n\leq 2\,.,\nn\\
0&=\beta_m\qquad\text{for}\quad 1\leq m\leq d-1\,.
\end{align}
The second set of conditions inserted into the first also gives $\beta_0=\beta_d=0$ and hence for $d\geq 5$ all $\beta_n$ must vanish. This choice of parameters of course trivializes the interaction potential. Our conclusion therefore is that there exist no nontrivial parameter values for which the constant part of the gauge transformation leaves the background equations invariant. Hence there is no PM candidate in pure bimetric theory in dimensions greater than four. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bimetric theory with Lanczos-Lovelock terms}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

According to the constructive consistency proof in chapter~\ref{ch:MG}, the interaction potential of the Hassan-Rosen bimetric theory includes all  consistent non-derivative terms. Therefore, the only option to obtain an extended version of the theory is to add more derivative terms to the action. At this point, the only such terms that are expected to be ghost-free consist of the Lanczos-Lovelock invariants which are defined as totally antisymmetric contractions of Riemann tensors $R^{\alpha\beta}_{\phantom{\alpha\beta}\mu\nu}$,
\beqn\label{LLdef}
\mathcal{L}_{(n)}=\frac{1}{2^nn!}\delta^{\mu_1}_{[\alpha_1}\delta^{\nu_1}_{\beta_1}\hdots\delta^{\mu_n}_{\alpha_n}\delta^{\nu_n}_{\beta_n]}
\prod_{k=1}^nR^{\alpha_k\beta_k}_{\phantom{\alpha_k\beta_k}\mu_k\nu_k}\,.
\eeqn
In spite of being higher derivative operators, the LL invariants are believed to avoid inconsistencies that are usually introduced by such terms. This is due to the antisymmetric structure in (\ref{LLdef}) which ensures the absence of more than two time derivatives acting on one field in the action. It is interesting that the same structure appears in the interaction potential of ghost-free bimetric theory, but of course this is not really a coincidence: In the decoupling limit of nonlinear massive gravity it can be seen that the antisymmetric structure removes higher time derivatives from the longitudinal modes of the St\"uckelberg fields.  

Hoping to rediscover the possibility of finding PM candidates in $d>4$, we thus choose to extend the Hassan-Rosen bimetric action by the following terms,\footnote{In a different context, consistent bimetric theory extended by LL terms has already been considered in~\cite{Paulos:2012xe}.}
\begin{align}\label{LLaction}
S_\mathrm{LL}~&=~~m_g^{d-2}\int\dd^dx\sum_{n=2}^{[d/2]}\sqrt{-g}~l_n^g\,\mathcal{L}_{(n)}(g)\nn\\
&~+~m_f^{d-2}\int\dd^dx\sum_{n=2}^{[d/2]}\sqrt{-f}~l_n^f\,\mathcal{L}_{(n)}(f)\,,
\end{align}
where we have introduced two sets of couplings, $l_n^g$ and $l_n^f$, of mass dimension $2(1-n)$.
Furthermore, it is well known that the LL invariant $\mathcal{L}_{(n)}$ is topological in $d=2n$ and vanishes for $2n>d$ which is why the sums in (\ref{LLaction}) terminate at integer part of $d/2$. 



The equations of motion for $\gmn$ and $\fmn$ that follow from the LL extended bimetric action are
\beqn\label{LLeom}
\mathcal{G}_{\mu\nu}(g)+\sum_{n=2}^{[d/2]}l_n^g\mathcal{G}^{(n)}_{\mu\nu}(g)+\frac{m^d}{m_g^{d-2}}V^g_{\mu\nu}&=&0\,, \nn\\
\mathcal{G}_{\mu\nu}(f)+\sum_{n=2}^{[d/2]}l_n^f\mathcal{G}^{(n)}_{\mu\nu}(f)+\frac{m^d}{m_g^{d-2}}V^f_{\mu\nu}&=&0\,.
\eeqn
Here, $\mathcal{G}^{(n)}_{\mu\nu}$ are the Lovelock tensors that follow from variation of (\ref{LLaction}) and $V^g_{\mu\nu}$ and $V^f_{\mu\nu}$ are the contributions from the interaction potential which were defined in (\ref{poteom}). We will not need the explicit expressions for the Lovelock tensors, but let us note the important property,
\beqn\label{usefid}
g^{\mu\nu}\mathcal{G}^{(n)}_{\mu\nu}(g)=\frac{2n-d}{2}\mathcal{L}_{(n)}(g)\,,
\eeqn
which will be useful in what follows.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proportional backgrounds}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As in pure bimetric theory we are interested in the proportional background solutions to (\ref{LLeom}) and perturbations around those. Again, these backgrounds correspond to maximally symmetric spacetimes, for which the curvatures satisfy
\beqn\label{bgcurv}
R_{\mu\nu\rho\sigma}(\bar{g})&=&\frac{2\lambda}{(d-1)(d-2)}(\bar{g}_{\mu\rho}\bar{g}_{\nu\sigma}-\bar{g}_{\nu\rho}\bar{g}_{\mu\sigma})\,,\nn\\
R_{\mu\nu}(\bar{g})&=&\frac{2\lambda}{d-2}\bgmn\,,\qquad R(\bar{g})~=~\frac{2d\,\lambda}{d-2}\,,
\eeqn
with cosmological constant $\lambda$. On such backgrounds with constant curvature, the $n$-th order LL invariant is proportional to $\lambda^n$,
\beqn\label{LLbg}
\mathcal{L}_{(n)}=N_n(d)\,\lambda^n\,,\quad\text{with}~~N_n(d)\equiv\frac{2^n d!}{(d-1)^n(d-2)^n(d-2n)!}\,.
\eeqn
Next, we trace the equations of motion (\ref{LLeom}) in order to obtain two scalar equations and insert (\ref{bgcurv}) for the curvatures.
Furthermore, we make use of the identity (\ref{usefid}) and plug in the proportional ansatz, $\bfmn=c^2\bgmn$. 
Finally, in the equation for $\fmn$, we use $\mathcal{L}_{(n)}(c^2 \bar{g})=c^{-2n}\mathcal{L}_{(n)}( \bar{g})$. The resulting two equations read
\beqn\label{LLbgeq}
\lambda + \sum_{n=2}^{[d/2]}l^g_n\frac{d-2n}{2d}N_n(d)\lambda^n - \Lambda_g&=&0\,,\nn\\
\lambda + \sum_{n=2}^{[d/2]}c^{2-2n}l^f_n\frac{d-2n}{2d}N_n(d)\lambda^n - \Lambda_f&=&0\,.
\eeqn
Here, $\Lambda_g$ and $\Lambda_f$ are the contributions from the potential evaluated on the proportional backgrounds which defined earlier in (\ref{lambdas}). Note, however, that these no longer correspond to the physical cosmological constants and are not necessarily equal. 

For general parameters $\beta_n$, $l_n^g$, and $l_n^f$, the two algebraic equations in (\ref{LLbgeq}) serve to determine the background curvature $\lambda$ as well as the proportionality constant $c^2$. Note also that in the absence of the LL contributions, i.e.~for $l_n^g=l_n^f=0$, we rearrive at the bimetric background equations, $R(\bar{g})=\tfrac{2d}{d-2}\Lambda_g$ and $\Lambda_g=\Lambda_f$. Eventually, we will again be looking for the parameter values for which the equations (\ref{LLbgeq}) leave $c$ undetermined.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear Perturbations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Computing the linearized equations of motion from (\ref{LLeom}) is quite involved. Fortunately, it has been observed in \cite{Sisman:2012rc} that, around constant curvature backgrounds with cosmological constant $\lambda$, the fluctuation equations of General Relativity augmented by the LL terms with couplings $l_n^g$ assume the same form as the ones obtained from Einstein's equations. The only difference is that, in the linearized equations of the LL extended theory, the Planck mass $m_g$ needs to be replaced by an effective mass parameter $\tilde{m}_g$ defined through
\beqn\label{modmg}
\frac{\tilde{m}_g^{d-2}}{m_g^{d-2}}=1+(d-3)!\sum_{n=2}^{[d/2]}\frac{n(d-2n)l_n^g}{(d-2n)!}\left(\frac{2\lambda}{(d-1)(d-2)}\right)^{n-1}.
\eeqn
It is a remarkable feature of the Lovelock invariants that, in spite of being higher-derivative operators in the nonlinear theory, they give rise to linearized equations that are only second order in derivatives.

For the bimetric case the above result implies that the linear equations for the theory with LL terms are the same as in pure bimetric theory if one replaces $m_g$ by $\tilde{m}_g$ as above and $m_f$ by $\tilde{m}_f$ given by
\beqn\label{modmf}
\frac{\tilde{m}_f^{d-2}}{m_f^{d-2}}=1+(d-3)!\sum_{n=2}^{[d/2]}\frac{n(d-2n)c^{2-2n}l_n^f}{(d-2n)!}\left(\frac{2\lambda}{(d-1)(d-2)}\right)^{n-1}.
\eeqn
Hence, thanks to the results of~\cite{Sisman:2012rc}, without any computation we can conclude that the linear equations in a maximally symmetric background with cosmological constant $\lambda$ will again diagonalize into a massless and massive equation, where in the latter the Fierz-Pauli mass (\ref{FPmass}) is now given in terms of $\tilde{m}_g$ and $\tilde{m}_f$. Due to this similarity, the linear equations are again invariant under the usual PM symmetry (\ref{linPMsym}) if the mass is on the Higuchi bound, $m_{\mathrm{FP}}^2=\frac{2}{d-1}\lambda$. One can then hope that it is possible to find a nonlinear candidate PM theory within this generalized setup.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{PM candidates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We apply the same logic as in the four-dimensional case to LL extended bimetric theory:
For extending the linear PM symmetry to the nonlinear level, we need to be able to shift the proportionality constant $c^2$ and hence, in a PM candidate theory, the background equations (\ref{LLbgeq}) must not determine it. In order to see for which parameter values this is possible, we must first solve a combination of the two equations for $\lambda$, eliminate it from the remaining equation, and demand the result to be independent of $c$. 

Although this procedure sounds again straightforward, in practice, it cannot always be carried out immediately. Complications arise because the background equations (\ref{LLbgeq}) are polynomials of order $[d/2]$ in $\lambda$ and solving them does not result in a polynomial expression for $\lambda$ as a function of $c$. Therefore, generically, the equation that is supposed to leave $c$ undetermined is not a polynomial in $c$ and it becomes difficult to impose the requirement on the PM theory. 

Nevertheless, for small enough $d$ it is possible to arrive at a polynomial equation in $c$ and the analysis can be carried out. As an example, we present the analytical results in $d=5$ before summarizing the outcome of a computer-based analysis for dimensions up to $d=8$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Partial masslessness in $d=5$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In five space-time dimensions the equations are still simple enough to be solved by hand. The only nontrivial LL term is $\mathcal{L}_{(2)}$, also known as the Gauss-Bonnet combination,
\beqn\label{gaussbonnet}
\mathcal{L}_{(2)}=R^2-4R_{\mu\nu}R^{\mu\nu}+R_{\mu\nu\rho\sigma}R^{\mu\nu\rho\sigma}\,,
\eeqn
which is topological in $d=4$. 
When terms of this kind for both $\gmn$ and $\fmn$ are added to the bimetric action, the background equations (\ref{LLbgeq}) take the following form,
\beqn\label{bgeqLL5}
\lambda+\frac{l_2^g}{3}\lambda^2-\Lambda_g=0\,,\qquad
\lambda+\frac{l_2^f}{3c^2}\lambda^2-\Lambda_f=0\,.
\eeqn
Here the contributions from the interaction potential read
\beqn\label{contpotf}
\Lambda_g&=&\frac{m^5}{m_g^3}(\beta_0+4c\beta_1+6c^2\beta_2+4c^3\beta_3+c^4\beta_4)\,,\nn\\
\Lambda_f&=&\frac{m^5}{m_g^3(\alpha c)^3}(c\beta_1+4c^2\beta_2+6c^3\beta_3+4c^4\beta_4+c^5\beta_5)\,.
\eeqn
The system (\ref{bgeqLL5}) can easily be solved for $\lambda$ by building a linear combination of the equations in which the quadratic terms cancel out. This gives
\beqn
\lambda=\frac{c^2l_2^g\Lambda_f-l_2^f\Lambda_g}{c^2l_2^g-l_2^f}\,.
\eeqn
Plugging this result back into the difference of the two equations in (\ref{bgeqLL5}) results in a polynomial equation for $c$,
\beqn
l_2^g(l\Lambda_g-c^2\Lambda_f)^2+3(c^4-lc^2)(\Lambda_g-\Lambda_f)=0\,,
\eeqn
where, for notational simplicity, we have defined $l\equiv l_2^f/l_2^g$. After the expressions in (\ref{contpotf}) have been inserted, the left-hand side of this equation contains nine different powers of $c$. Demanding each coefficient to vanish, we obtain nine constraints on the parameters of the theory. As in the four-dimensional case, these constraints are not all independent, but they fix exactly seven out of the eight parameters $\{\beta_n, l_2^g, l_2^f\}$. The resulting values are
\begin{align}\label{PMvalf}
-\tfrac{1}{10}\beta_0&=\tfrac{1}{2\alpha}\beta_1=-\tfrac{1}{\alpha^2}\beta_2=-\tfrac{1}{\alpha^3}\beta_3=\tfrac{1}{2\alpha^4}\beta_4=-\tfrac{1}{10\alpha^5}\beta_5=\tfrac{m_g^3}{l_2^gm^5}\,,\nn\\
l_2^g&=\alpha^2l_f\,.
\end{align}
These parameters satisfy $\alpha^{5-n}\beta_n=\alpha^n\beta_{5-n}$ as well as $l_f=\alpha^{2-2n}l_n^g$, and hence the PM candidate theory is again symmetric under the interchange $\alpha^{-1}\gmn \leftrightarrow \alpha\fmn$. Using expression~(\ref{FPmass}) for the Fierz-Pauli mass with $m_g$ and $m_f$ replaced by the modified Planck masses given in (\ref{modmg}) and (\ref{modmf}), it is also straightforward to check that the Higuchi bound, $m_\mathrm{FP}^2=\frac{1}{2}\lambda$, is saturated. 

Note furthermore that one cannot set the Lovelock couplings $l_2^g$ and $l^f_2$ to zero because the $\beta_n$-parameters are inversely proportional to them. This is of course consistent with our findings in section \ref{noPMdgeq5}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Partial masslessness in $d>5$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The analysis in $d=6$ is very similar to the five-dimensional case since the only contributing LL term is still $\mathcal{L}_{(2)}$. Up to the sign of $\beta_3$, all but one of the parameters become fixed again. Their values are given in {\protect{\hyperref[papVII]{Paper VII}}}.

For dimensions greater than six, the cubic LL term $\mathcal{L}_{(3)}$ needs to be included into the action. According to (\ref{LLbg}), on the proportional backgrounds it reduces to $N_3(d)\lambda^3$. Hence the background equations (\ref{LLbgeq}) will now be cubic polynomials in $\lambda$. One can subtract the cubic term by building a linear combination of the two equations to arrive at a quadratic equation. But then the solution for $\lambda$ will invole a square root and, as a result, the equation determining $c$ will no longer be a polynomial. This complicates the determination of the PM parameters because we cannot apply our method, which proved successful in $d\leq 6$, to a non-polynomial equation. However, there is another possibility of solving the background equations (\ref{LLbgeq}): One can decompose them into a Gr\"obner basis of equivalent polynomial equations and thereby reduce the equation for $\lambda$ to a linear one. In addition, one obtains a consistency condition that is a polynomial in $c$ and can be used to impose the requirement for partial masslessness. Following this strategy, it is in principle possible to identify PM candidates in any dimension. The computational effort, however, becomes very large already when the quartic LL term $\mathcal{L}_{(4)}$ is included in the theory. Even with the help of a computer it was therefore only possible to determine the PM parameters in dimensions up to $d=8$ where $\mathcal{L}_{(4)}$ still does not contribute to the equations of motion. The results are summarized in Table~1 of {\protect{\hyperref[papVII]{Paper~VII}}}.  

As could have been anticipated, the PM parameters always satisfy the symmetry relations $\alpha^{d-n}\beta_n=\alpha^n\beta_{d-n}$ as well as $l_n^f=\alpha^{2-2n}l_n^g$.
The value for the Fierz-Pauli mass turns out to saturate the Higuchi bound in all cases. The fact that the scale invariance of the background and the PM gauge symmetry at the level of perturbations always coincide is entirely nontrivial and supports the validity of our approach.
Interestingly, there is no PM candidate in seven spacetime dimensions.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Relation to Higher-Curvature Gravity}
\label{ch:HD}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this chapter we discuss modified theories of gravity with higher powers of curvatures. A particular class of theories with at most four derivatives, including the famous examples of New Massive Gravity and Conformal Gravity, is known to be free of the Boulware-Deser ghost. However, one of the two spin-2 modes in these theories shows unavoidable ghost instabilities in all its helicity components. This has been an unresolved problem challenging the otherwise promising models of modified gravity. 

On the other hand, bimetric gravity with a large value for the Fierz-Pauli mass contains a heavy spin-2 excitation, and integrating out this field results in an effective theory for just one rank-2 tensor. In general, this effective action will be nonlocal, i.e.~it will not simply be an expansion in higher curvatures but involve inverted differential operators. However, in {\protect{\hyperref[papVIII]{Paper~VIII}}} we point out a definite relation among an effective action obtained from bimetric theory and the higher-curvature theories that avoid the Boulware-Deser ghost. We obtain a mapping between the two classes of theories and thereby also solve the ghost problem of the quadratic curvature theories by completing them into an infinite series of curvature terms. Furthermore, it is shown that, to lowest order in a derivative expansion, the effective theory obtained from the PM candidate introduced in chapter~\ref{ch:PM} is equivalent to Conformal Gravity.

Before explaining our method and presenting the results, we begin this chapter with a brief review of the relevant higher-curvature theories.  





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Higher-curvature gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
When viewed as a quantum theory, General Relativity is nonrenormalizable in the usual power-counting sense, which can be seen from the fact that, after canonical normalization of the fluctuations, the coupling constants of the nonlinear interactions have negative mass dimensions. Therefore the theory can be meaningful only as an effective theory which is valid at low energies and possesses a fully consistent (yet unknown) UV completion. One promising candidate for the theory at high energies is String Theory which is indeed a consistent quantum theory containing gravity as well as gauge theories that could reduce to the Standard Model of Particle Physics at low energies. In the framework of String Theory it is possible to derive the effective low-energy action for the metric $\gmn$ by integrating out heavy string states, which results in an expansion in curvatures suppressed by the mass scale of the heavy string excitations. String Theory theorefore constitutes one example of how higher-curvature terms enter the effective action. In general, the concept of effective field theory tells us that such corrections to the Einstein-Hilbert term are expected to arise from any UV completion. 


The most relevant correction to Einstein gravity is quadratic in curvatures for $\gmn$. The only possible (local) terms that can arise at this order are $R_{\mu\nu\rho\sigma}R^{\mu\nu\rho\sigma}$, $R_{\mu\nu}R^{\mu\nu}$ and $R^2$. In principle, we should also expect covariant derivatives acting on curvatures in the action, but due to the Bianchi identity the only possible term at quadratic order is $\Box R$ which is a total derivative. Also note that we can choose to complete the term $R_{\mu\nu\rho\sigma}R^{\mu\nu\rho\sigma}$ into the quadratic Lanczos-Lovelock combination~(\ref{gaussbonnet}) which we do not consider in this chapter but in principle can always be added to the action in $d>4$. One therefore only needs to take into account the terms $R_{\mu\nu}R^{\mu\nu}$ and $R^2$. It then turns out that the relative coefficient between these two contributions in the action is fixed by demanding the absence of the Boulware-Deser ghost, and the corresponding effective action truncated to a four-derivative theory is given by~\cite{Stelle:1976gc, Stelle:1977ry},
\begin{align}\label{HDact}
    S_\mathrm{HD}^{(2)}=m_g^{d-2}\int\dd^dx\sqrt{g}\,\Big[ &c_\Lambda+c_RR(g)\nn\\
    &-\frac{c_{RR}}{m^2}\left(R^{\mu\nu}R_{\mu\nu}-\frac{d}{4(d-1)}R^2\right) \Big]\,.
\end{align}
Here, $c_\Lambda$ is a cosmological constant term with mass dimension two, while $c_R$ and $c_{RR}$ are dimensionless coefficients. Furthermore, $m$ is the energy scale at which the effective field theory looses its validity. The relative coefficient between the two quadratic curvature terms is fixed to be equal to~$\frac{-d}{4(d-1)}$ which, as we shall now demonstrate, results in a mass term with the Fierz-Pauli combination at the linearized level. In order to see this, let us introduce an auxiliary tensor field $\varphi_{\mu\nu}$ into the theory, which we take to be symmetric in its indices. In terms of this new field we can write an equivalent action as follows,
\begin{align}\label{auxact}
    S_\mathrm{aux}=m_g^{d-2}\int\dd^dx\sqrt{g}\,\Big[ c_\Lambda+c_R&R(g) -\mathcal{G}_{\mu\nu}\varphi^{\mu\nu} \nn\\
    &+\frac{m^2}{4c_{RR}}(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,.
\end{align}
Here, $\mathcal{G}_{\mu\nu}$ is the Einstein tensor for $\gmn$ and the indices on the symmetric tensor $\varphi_{\mu\nu}$ are raised and lowered with~$\gmn$. As is easily verified, the solution to the equations of motion for $\varphi_{\mu\nu}$ reads
\beqn\label{phiauxeom}
\varphi_{\mu\nu}=\frac{2c_{RR}}{m^2}\left(\mathcal{G}_{\mu\nu}-\frac{1}{d-1}\mathcal{G}\gmn\right)\,,
\eeqn
which can be plugged back into (\ref{auxact}) to rearrive at (\ref{HDact}). Hence, we have defined a two-derivative theory involving an auxiliary field which can be integrated out to return to the higher-derivative action.

If now $c_\Lambda=0$ then $\bgmn=\emn$ and $\bar{\varphi}_{\mu\nu}=0$ solve both~(\ref{phiauxeom}) as well as the $\gmn$ equations. We then consider the quadratic action for fluctuations~$\varphi_{\mu\nu}$ and $\hmn=\gmn-\emn$ around this background, 
\begin{align}\label{quadactaux}
S_\mathrm{aux}^{\mathrm{lin}}=\tfrac{m_g^{d-2}}{4}\int\dd^dx\Big[h_{\mu\nu}\mathcal{E}^{\mu\nu\rho\sigma}\Big(c_{R}&h_{\rho\sigma}+\tfrac{d-2}{2}\varphi_{\rho\sigma}\Big)\nn\\
&+\tfrac{m^2}{c_{RR}}(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,,
\end{align}
where the linearized Einstein operator $\mathcal{E}^{\mu\nu\rho\sigma}$ in flat space was already given in (\ref{kinstruc1}). The kinetic terms are not diagonal, which motivates us to make the following linear redefinitions,
\beqn
\hmn'\equiv\tfrac{1}{2}m_g^{(d-2)/2} \hmn+\tfrac{d-2}{4}\tfrac{1}{c_R}\varphi_{\mu\nu}\,,\quad~~
 \varphi_{\mu\nu}'\equiv\tfrac{d-2}{4\sqrt{2}}\,m_g^{(d-2)/2}\varphi_{\mu\nu}\,,
\eeqn
where the normalizations in front have been chosen conveniently. These redefinitions diagonalize $S_\mathrm{aux}^{\mathrm{lin}}$ into an action for a massless spin-2 fluctuation $h'_{\mu\nu}$ and a massive spin-2 fluctuation $\varphi'_{\mu\nu}$,
\begin{align}\label{diagactaux}
S_\mathrm{aux}^{\mathrm{lin}}=\int\dd^dx\Big(c_Rh'_{\mu\nu}\mathcal{E}^{\mu\nu\rho\sigma}&h'_{\rho\sigma}-\tfrac{1}{c_R}\varphi'^{\mu\nu}\mathcal{E}^{\mu\nu\rho\sigma}\varphi'_{\rho\sigma}\nn\\
&+\tfrac{(d-2)^2}{16}\tfrac{m^2}{c_{RR}}(\varphi'^{\mu\nu}\varphi'_{\mu\nu}-\varphi'^2)\Big)\,.
\end{align}
As promised, the mass term has the Fierz-Pauli structure, which would not have been the case had we started with a different relative coefficient between the two quadratic-curvature terms in (\ref{HDact}). Furthermore, the sign of $c_{RR}$ determines the sign of the squared Fierz-Pauli mass and can be adjusted such that it is non-tachyonic.
On the other hand, the signs of the kinetic terms for the massless and massive spin-2 fluctuations are determined by the coefficient $c_R$ alone, and it is evident that they will always have opposite signs. As a consequence, it is unavoidable that either the massless or the massive fluctuation will be a ghost. Note that this ghost is not an extra degree of freedom and, in particular, it does not correspond to the Boulware-Deser instability. Instead, all helicity components of the massless or massive spin-2 fluctuation themselves suffer from a ghost-like kinetic term. This is a manifestation of Ostrogradski's theorem~\cite{Ostrogradski} which states that any theory with $N$ time derivatives, for $2<N<\infty$, is plagued by ghosts. Therefore the above higher-curvature action, despite being free of the Boulware-Deser ghost, is not consistent.
 
Before presenting the relation among higher-curvature gravity and Hassan-Rosen bimetric theory, let us briefly mention two popular examples for actions of the type (\ref{HDact}): New Massive Gravity in three and Conformal Gravity in four space-time dimensions.



    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsubsection{New Massive Gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As we already explained in section \ref{sec:FP}, the number degrees of freedom of a massless spin-2 particle in $d$ dimensions is $d(d-3)/2$. It follows that in $d=3$, there is no propagating massless spin-2 mode. This observation motivated the authors of \cite{Bergshoeff:2009hq, Bergshoeff:2009aq} to choose $c_R<0$ and $c_{RR}<0$ in the higher-curvature action~(\ref{HDact}) for the case $d=3$. As can be seen in the linearized auxiliary action~(\ref{diagactaux}), this choice renders the massive field healthy and turns the massless field into a ghost. However, since the massless field is not a propagating degree of freedom, the wrong sign in front of its kinetic term does not lead to an inconsistency in the theory. The higher-derivative action with these sign choices became very popular under the name \textit{New Massive Gravity}. Of course, the trick employed in \cite{Bergshoeff:2009hq, Bergshoeff:2009aq} fails to work in dimensions greater than three where the massless mode is propagating and ghost-like for $c_R<0$. In the past, the construction of a consistent higher-derivative theory in $d>3$ has therefore not been successful~\cite{Kleinschmidt:2012rs}. There have also been attempts to complete New Massive Gravity to a theory with infinitely many derivatives (see e.g.~\cite{Gullu:2010pc, Paulos:2010ke}) which could in principle avoid Ostrogradski's theorem and cure the ghost problem even in higher dimensions. We obtain such a completion in {\protect{\hyperref[papVIII]{Paper~VIII}}} where we show that the Hassan-Rosen bimetric theory when written as an effective theory for one of the metrics is closely related to New Massive Gravity in three and its generalized form in higher dimensions. Moreover, the spin-2 ghost that is unavoidably contained in (\ref{HDact}) is argued to arise from the truncation of an infinite derivative expansion to a four-derivative theory. This proposes the Hassan-Rosen bimetric action as a consistent nonlinear completion of the higher-derivative theory~(\ref{HDact}) in any number of space-time dimensions.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Conformal Gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In four spacetime dimensions, there is a particular choice of parameters for which the higher-derivative action (\ref{HDact}) develops a new gauge symmetry. 
Namely, if we set $c_\Lambda=c_R=0$ then the only terms left in the action are the four-derivative terms,~\cite{Bach} 
\beqn\label{CGact}
    S_\mathrm{CG}=-\frac{m_g^2c_{RR}}{m^2}\int\dd^4x\sqrt{g}\,\left(R^{\mu\nu}R_{\mu\nu}-\frac{1}{3}R^2\right)\,.
\eeqn
With help of the curvature relations (\ref{curvrel}) it is straightforward to show that this action is invariant under conformal transformations of the metric, 
\beqn\label{conftrafo}
\gmn\rightarrow \xi^2(x)\gmn\,,
\eeqn
where $\xi(x)$ is a local gauge parameter.
The theory therefore goes under the name of \textit{Conformal Gravity}. The cosmological constant and the Einstein-Hilbert term are not invariant under the transformation (\ref{conftrafo}) which is why their coefficients had to be set to zero.


The equations of motions that follow from variation of the conformal gravity action (\ref{CGact}) imply the vanishing of the Bach tensor for~$\gmn$,
\beqn\label{Bacheq}
   B_{\mu\nu}\equiv -\nabla^2 P_{\mu\nu}+\nabla^{\rho}\nabla_{(\mu}P_{\nu)\rho}+W_{\rho\mu\nu\sigma}P^{\rho\sigma}=0\,.
\eeqn 
Here, we have given the definition of $B_{\mu\nu}$ in terms of the Schouten tensor,
\beqn\label{schouten}
P_{\mu\nu}\equiv R_{\mu\nu}-\frac{1}{2(d-1)}\gmn R\,,
\eeqn
as well as the Weyl tensor,\footnote{In the literature, the Conformal Gravity action~(\ref{CGact}) is sometimes also expressed as the square of the Weyl tensor, $\mathcal{L}_\mathrm{CG}\propto\sqrt{g}\,W_{\rho\mu\nu\sigma}W^{\rho\mu\nu\sigma}$.}
\beqn
W_{\rho\mu\nu\sigma}\equiv R_{\rho\mu\nu\sigma}+g_{\mu[\nu}R_{\sigma]\rho}-g_{\rho[\nu}R_{\sigma]\mu}+\frac{1}{3}g_{\rho[\nu}g_{\sigma]\mu}R\,.
\eeqn 
The Bach tensor is invariant under conformal transformations in four space-time dimensions~\cite{Bach}.


The Conformal Gravity action is closely related to the linear theory for a partially massless spin-2 field discussed in section~\ref{seclinPM}. In order to see this, we again need to introduce an auxiliary field $\varphi_{\mu\nu}$. But since the equations of motion that follow from the above auxiliary action are consistent with vanishing background for $\varphi_{\mu\nu}$ only if $\gmn$ is flat, $S_\mathrm{aux}$ in (\ref{auxact}) needs to be slightly modified in order to give rise to more general de Sitter solutions for which the linear PM symmetry is known to exist. More precisely, one needs to add a linear term proportional to $\varphi=g^{\mu\nu} \varphi_{\mu\nu}$ such that $\mathcal{G}_{\mu\nu}(\bar{g})=\Lambda\bgmn$ with $\Lambda=$ const.~and $\bar{\varphi}_{\mu\nu}=0$ now solve the equations of motion. Instead of writing down the auxiliary action in the general case, here we only give the expression for Conformal Gravity which reads~\cite{Kaku:1977pa}
\begin{align}\label{CGauxact}
    S_\mathrm{CG}^{(2)}=\tfrac{4c_{RR}m_g^{2}\Lambda}{m^2}\int\dd^dx\sqrt{g}\,\Big[ \tfrac{1}{6}(R&-2\Lambda)+\varphi^{\mu\nu}\mathcal{G}_{\mu\nu} \nn\\
    &+ \Lambda\varphi+ \Lambda(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,.
\end{align}
Linearization around the constant curvature background and diagonalization into mass eigenstates shows that, for $c_{RR}>0$, the theory propagates a healthy massless and a ghost-like massive spin-2 particle. Moreover, the Fierz-Pauli mass of the massive fluctuation has the value corresponding to the Higuchi bound, $m_\mathrm{FP}^2=\frac{2}{3}\Lambda$, which implies the presence of the PM gauge symmetry (\ref{linPMsym}) for $\varphi_{\mu\nu}$. The massless fluctuation $\hmn'$ does not transform under this symmetry.
In fact, it is a simple exercise to check that, in addition to the obvious diffeomorphism invariance, the full nonlinear auxiliary action (\ref{CGauxact}) is invariant under the following linear gauge transformations~\cite{Deser:2012qg},
\beqn
\delta\gmn=2\xi(x)\gmn\,,\qquad \delta\varphi_{\mu\nu}=(\nabla_\mu\partial_\nu+\tfrac{\Lambda}{3})\xi(x)\,.
\eeqn
Note that the nonlinear field $\gmn$ transforms under the PM symmetry because its fluctuation does not correspond to the massless mode but is a linear superposition of mass eigenstates. Its transformation is of course nothing but the linear version of the conformal transformation (\ref{conftrafo}).

Conformal Gravity, or its equivalent form (\ref{CGauxact}), therefore describes only six propagating degrees of freedom instead of seven that would correspond to a massless and a massive spin-2 field. For more detailed discussions of its spectrum we refer the reader to \cite{Fradkin:1981iu, Lee:1982cp, Riegert:1984hf, Maldacena:2011mk}. 

Like any other conformal field theory, $S_\mathrm{CG}$ does not contain any dimensionful couplings and therefore avoids the nonrenormalizibility problem of General Relativity. Being a renormalizable field theory, conformal gravity has been suggested as a quantum theory for gravity. It has also been shown to allow for viable cosmological solutions and even fit galaxy rotation curves, providing a possible solution for at least part of the dark matter problem~\cite{Mannheim:2011ds}. 

Unfortunately, all of these promising features remain irrelevant unless a cure for the ghost problem is found. Suggestions for altering the theory in order to make it healthy include, for instance, a modification of quantum mechanics~\cite{Bender:2007wu} and the addition of specific boundary conditions~\cite{Maldacena:2011mk}, but none of these seemed sufficiently convincing for the theory to be accepted as a consistent alternative to General Relativity. 

In order to avoid the inconsistencies that plague theories with a finite number of higher derivatives, another possible solution is to complete the equations of motion~(\ref{Bacheq}) of Conformal Gravity with an infinite number of derivatives for which Ostrodgradski's theorem does not hold. Higher-derivative terms will, of course, break the conformal symmetry because they necessarily enter with a suppressing mass scale. On the other hand, one could imagine that the symmetry transformation needs to be completed with an infinite number of higher-derivative terms as well, in order to be a gauge symmetry of the full theory. In that case, both the equations of motion and the symmetry transformation could be thought of as a perturbative expansion in derivatives. Order by order, the equations would be invariant under the gauge symmetry, starting with the Bach tensor and its conformal invariance at lowest order. Although this idea sounds promising, without any further input it is difficult to guess the form of the higher-derivative corrections to the Bach equation that could give rise to such a gauge symmetry. It would therefore be helpful to have a guideline telling us how to construct these terms.

In section~\ref{secPMCG} we will see that the candidate for partially massless bimetric gravity introduced in section~\ref{secPmnonlin}, when written as an effective theory for $\gmn$, is equivalent to Conformal Gravity to lowest order in a derivative expansion. 
This observation motivates us to propose PM bimetric theory as a nonlinear ghost-free completion of Conformal Gravity. 
As in the case of general $\beta_n$ parameters that lead to the higher-curvature theory in (\ref{HDact}), the spin-2 ghost in Conformal Gravity is argued to be an artifact of truncating the full bimetric action to a four-derivative theory.
If our PM model possesses a nonlinear gauge symmetry then so does the corresponding effective theory for $\gmn$. Moreover, the derivative expansions of both the equations of motions for $\gmn$ and of the gauge symmetry can be constructed in a straightforward way.
This relation to the successful (but inconsistent) theory of Conformal Gravity turns ghost-free PM bimetric theory into a particularly interesting model.

   



%\begin{align}\label{auxactn}
    %S_\mathrm{aux}=m_g^{d-2}\int\dd^dx\sqrt{g}\,\Big[ \Big(&c_\Lambda+\tfrac{d}{d-1}c_{RR}m^2\Big)+\left(c_R-\tfrac{d-2}{d-1}c_{RR} \right)R(g) 
    %\nn\\
    %+\mathcal{G}_{\mu\nu}\varphi^{\mu\nu} &+m^2\varphi
    %-\frac{m^2}{4c_{RR}}(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,.
%\end{align}
%Here $\mathcal{G}_{\mu\nu}$ is the Einstein tensor for $\gmn$ and the indices on the symmetric tensor $\varphi_{\mu\nu}$ are raised and lowered with~$\gmn$. As is easily verified, the solution to the equations of motion for $\varphi_{\mu\nu}$ reads
%\beqn\label{phiauxeom}
%\varphi_{\mu\nu}=\frac{2c_{RR}}{m^2}\left(\mathcal{G}_{\mu\nu}-\frac{1}{d-1}\mathcal{G}\gmn-\frac{m^2}{d-1}\gmn\right)\,,
%\eeqn
%which can be plugged back into (\ref{auxact}) to reobtain (\ref{HDact}). 










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Relation to bimetric theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We now return to Hassan-Rosen bimetric gravity with the intention to demonstrate its close relation to the higher-curvature actions discussed above. First we outline two not entirely equivalent procedures of obtaining an effective action for one of the metrics by integrating out the other. Then we show that one of the procedures leads to the higher-derivative theory in~(\ref{HDact}) plus higher curvature corrections. Finally, we consider the PM bimetric theory as a particular example and demonstrate its equivalence to Conformal Gravity to lowest order in derivatives both at the level of the action and the equations of motion.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effective theories for $\gmn$}\label{sec:outl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Consider the two equations of motion obtained from varying the bimetric action (\ref{HR}) with respect to one of the two metrics while the other is held constant. Schematically, we write them as
\beqn
\mathcal{E}^g_{\mu\nu}(g,f)\equiv\left.\frac{\delta S_\mathrm{HR}}{\delta g^{\mu\nu}}\right|_{f}=0\,,\qquad \mathcal{E}^f_{\mu\nu}(g,f)\equiv\left.\frac{\delta S_\mathrm{HR}}{\delta f^{\mu\nu}}\right|_{g}=0\,.
\eeqn
Their explicit forms are given in (\ref{geq}) and (\ref{feq}), respectively, but are not important to us at this stage because our considerations here will be completely general. Suppose now that we intend to use one of the equations to express $\fmn$ in terms of $\gmn$ and then eliminate it in the second equation. For instance, we can think of obtaining a solution for $\fmn$ from its own equation of motion and plugging it into the $\gmn$ equation, such that we get an effective equation for $\gmn$,
\beqn\label{effeq1}
\mathcal{E}^g_{\mu\nu}(g, f(g))=0\,.
\eeqn
This equation will be nonlocal because solving the~$\fmn$ equation for $\fmn$ requires inverting derivative operators, leading to a nonlocal expression for $\fmn$ as a function of $\gmn$.

A more convenient way to arrive at an effective equation for $\gmn$ is to start instead by solving the $\gmn$ equation for $\fmn$, because this equation does not involve derivatives of $\fmn$.  This strategy therefore leads to an algebraic expression for $\fmn$ in terms of curvatures of $\gmn$. For general parameters in the potential, this solution can be obtained perturbatively as an infinite series in $R_{\mu\nu}(g)/m^2$. Plugging it into the other equation then results in a local effective equation for $\gmn$,
\beqn\label{effeq2}
\mathcal{E}^f_{\mu\nu}(g, f(g))=0\,,
\eeqn
which will acquire the form of a derivative expansion. Note that the two procedures of deriving an effective equation for $\gmn$ are completely equivalent: Both methods involved solving one subset of the system of equations and using these solutions in the remaining equations. Hence, the solutions to the two different effective equations for $\gmn$ will be identical in both cases.

Next let us address the question whether it is possible to derive equations (\ref{effeq1}) and (\ref{effeq2}) from an action principle. In both cases this clearly requires finding an effective action for $\gmn$. Let us first suppose that we have solved for $\fmn$ using its own equation of motion. Then we can plug this solution back into the action to obtain an effective action $S_\mathrm{eff}(g)=S_\mathrm{HR}(g, f(g))$ for $\gmn$. Variation of $S_\mathrm{eff}(g)$ then gives
\beqn\label{fpvar}
\frac{\delta S_\mathrm{eff}(g)}{\delta g^{\mu\nu}}&=&\left.\frac{\delta S_\mathrm{HR}(g, f(g))}{\delta g^{\mu\nu}}\right|_{f(g)}+\left.\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\frac{\delta S_\mathrm{HR}(g, f(g))}{\delta f^{\alpha\beta}}\right|_{g}\nn\\
&=& \mathcal{E}^g_{\mu\nu}(g, f(g))+\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\mathcal{E}^f_{\alpha\beta}(g, f(g))\,.
\eeqn
Here we have made use of the following short-hand notation for combining functional derivatives,
\beqn
\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\frac{\delta S}{\delta f^{\alpha\beta}}\equiv \int d^dy\, \frac{\delta f^{\alpha\beta}(y)}{\delta g^{\mu\nu}(x)}\frac{\delta S}{\delta f^{\alpha\beta}(y)}\,.
\eeqn
By definition, $f_{\mu\nu}(g)$ satisfies $\mathcal{E}^f_{\alpha\beta}(g, f(g))=0$. Using this in~(\ref{fpvar}) implies that, in fact, we have 
\beqn
\frac{\delta S_\mathrm{eff}(g)}{\delta g^{\mu\nu}}=\mathcal{E}^g_{\mu\nu}(g, f(g))\,.
\eeqn
This little exercise shows that the equation of motion obtained from $S_\mathrm{eff}(g)$ is precisely equation (\ref{effeq1}). We conclude that integrating out $\fmn$ in the action by using its own equation of motion is equivalent to plugging the solution directly into the $\gmn$ equation. 

Clearly, due to the nonlocality of the solution to the $\fmn$ equation, the action $S_\mathrm{eff}(g)$ will also be nonlocal and can thus not have the form of the higher-derivative theories discussed in the previous section. Let us therefore try to obtain a different effective action by integrating out $\fmn$ using the $\gmn$ equation. Since in this case the solution for $\fmn$ is an algebraic expression in terms of curvatures of $\gmn$, we can hope to arrive at a standard higher derivative theory. The variation of the effective action $S_\mathrm{HD}(g)=S_\mathrm{HR}(g, f(g))$ again reads
\beqn
\frac{\delta S_\mathrm{HD}(g)}{\delta g^{\mu\nu}}= \mathcal{E}^g_{\mu\nu}(g, f(g))+\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\mathcal{E}^f_{\alpha\beta}(g, f(g))\,.
\eeqn
But since now $f_{\mu\nu}(g)$ is defined to satisfy $\mathcal{E}^g_{\alpha\beta}(g, f(g))=0$, we have
\beqn\label{HDactvar}
\frac{\delta S_\mathrm{HD}(g)}{\delta g^{\mu\nu}}= \frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\mathcal{E}^f_{\alpha\beta}(g, f(g))\,.
\eeqn
Obviously, this is not exactly equivalent to (\ref{feq}). The equations of motion obtained from the effective action $S_\mathrm{HD}(g)$ differ from the effective bimetric equations by an operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$. Therefore the solutions to these equations will differ by functions $\chi(x)$ that are annihilated by this operator, which means that instead of the bimetric equation $\mathcal{E}^f_{\alpha\beta}=0$ we now have
\beqn
\mathcal{E}^f_{\alpha\beta}(g, f(g))=\chi(x)\,,\quad \int d^dy\, \frac{\delta f^{\alpha\beta}(y)}{\delta g^{\mu\nu}(x)}\chi(y)=0\,.
\eeqn
Since $\fmn$ is a function of curvatures of $\gmn$, the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ will introduce derivative terms into the effective action that would not be present in the higher-derivative theory that is truly equivalent to bimetric gravity. Separating off these extra terms is a tedious task which we choose not to pursue. Instead we try to find out what features of the bimetric theory carry over to the local higher-derivative theory despite their inequivalence. In particular, we are interested in making statements about the consistency of the higher-derivative action $S_\mathrm{HD}(g)$. 

While it is clear that the nonlocal action $S_\mathrm{eff}(g)$ that is equivalent to the ghost-free bimetric theory must be consistent and propagate seven healthy degrees of freedom, it is an important to understand whether the local action $S_\mathrm{HD}(g)$ that differs from the Hassan-Rosen theory by an extra operator can contain ghosts. This question is difficult to answer for nonlinear spin-2 fields because the nonlinearities and the tensor structures complicate the analysis. In the appendix of {\protect{\hyperref[papVIII]{Paper VIII}}} we therefore address this issue only in two simplified models: an action for two scalar fields with linear mixing term and linearized bimetric gravity. The outcome of the analysis in both models shows that the analogue of the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ does not alter the vacuum persistence amplitude and therefore does not introduce ghosts into the theory. We therefore expect (but do not prove) that the nonlinear theory with action $S_\mathrm{HD}(g)$, obtained from integrating out $\fmn$ using the $\gmn$ equation, is also ghost-free. 

On the other hand, our examples in the appendix of {\protect{\hyperref[papVIII]{Paper VIII}}} also show that, besides shifting the mass pole in the massive field's propagator, a truncation of the derivative expansion can easily lead to ghost instabilities. This explains the presence of the spin-2 ghost in the New Massive Gravity and Conformal Gravity actions. In order to avoid Ostrogradski's theorem, the ghost-free theory certainly needs the infinite number of higher-derivative terms.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Perturbative solution to the $\gmn$ equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our focus in the following lies on the second of the two procedures outlined above, which will lead to a local effective action with higher derivatives for $\gmn$. We will apply it to bimetric gravity and explicitly work out the resulting higher-curvature terms. The first step in our declared strategy is to obtain an algebraic solution for $\fmn$ using the $\gmn$ equation, which is the purpose of this section. In order to present an instructive example, we start with a simple bimetric model in which the solution for $\fmn$ in terms of $\gmn$ curvatures has a closed and finite expression. Then we turn to the general case. In this whole chapter, as in {\protect{\hyperref[papVIII]{Paper VIII}}}, we replace the mass parameter $m^d$ in the bimetric action by $m^2m_g^{d-2}$ which slightly simplifies the expressions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{A simple example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

There is one choice of parameters for which the algebraic solution for $\fmn$ derived from the $\gmn$ equation is particularly simple and can be obtained in closed form straightforwardly. Namely, let us consider the $\gmn$ equation (\ref{geq}) in which we set all $\beta_n$ with $n=2,3\hdots d-1$ to zero. Only the contributions from $(Y^{(0)})^\mu_{~\nu}$ and $(Y^{(1)})^\mu_{~\nu}$ remain\footnote{Note that the $\gmn$ equation does not contain $\beta_d$ and hence the perturbative solution for $\fmn$ does not depend on it.} and the equation simply reads 
\beqn
\frac{1}{m^2}{\mathcal{G}^\mu}_\nu(g)+\beta_0\delta^\mu_\nu-\beta_1({S^\mu}_\nu-\Tr\,S~{\delta^\mu}_\nu)=0\,.
\eeqn
Here we have used the definition $S=\sqrt{g^{-1}f}$, as usual, and raised one index with $g^{\mu\nu}$. The trace of this equation may be used to eliminate $\Tr\,S$ and in this way the solution for ${S^\mu}_\nu$ is obtained as
\beqn\label{ssolbeta1}
{S^\mu}_\nu=\frac{1}{1-d}\frac{\beta_0}{\beta_1}\delta^\mu_\nu+\frac{1}{\beta_1m^2}{P^\mu}_\nu(g)\,,
\eeqn
which we we have expressed in terms of the Schouten tensor defined in~(\ref{schouten}).
Since $\fmn=g_{\mu\rho}{(S^2)^\rho}_\nu$ the corresponding solution for $\fmn$ immediately follows from (\ref{ssolbeta1}) and reads 
\beqn
\fmn=\left(\frac{1}{d-1}\frac{\beta_0}{\beta_1}\right)^2\gmn-\frac{2}{d-1}\frac{\beta_0}{\beta^2_1m^2}P_{\mu\nu}+\frac{1}{\beta^2_1m^4}{P_\mu}^\rho P_{\rho\nu}\,.
\eeqn
This expression already has the form of a perturbative expansion in curvatures. Remarkably, in this particular model the series terminates at quartic order in derivatives. As we will see below, for general $\beta_n$, it is not possible to solve the $\gmn$ equation for $\fmn$ exactly, but we can obtain a perturbative solution, i.e.~an expression for $\fmn$ as an infinite series in~$P/m^{2}$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{General case}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

After having explored the nature of the $\fmn$ solution in an instructive example, we now turn to the case of general $\beta_n$ parameters.
Our aim is to solve the $\gmn$ equation perturbatively for ${S^\mu}_\nu$. It will prove convenient to first rewrite the Einstein tensor in (\ref{geq}) in terms of the Schouten tensor and raise one index with $g^{\mu\nu}$. This gives
\beqn\label{eomrewr}
\Tr\,P\,\delta^\mu_\nu-{P^\mu}_\nu=m^2\sum_{n=0}^{d-1}(-1)^n\beta_n {(Y^{(n)})^\mu}_\nu(S)\,.
\eeqn
Note that for the sake of notational simplicity we have set the source for $\gmn$ to zero. This simplification constitutes no loss of generality because in the final results of our computation it can always be reinstated by making the following replacement,
\beqn\label{sourcerepl}
{P^\mu}_\nu~\longrightarrow~ {P^\mu}_\nu-m^{2-d}\left( {T^{g\mu}}_\nu -\tfrac{1}{d-1}\Tr\,T^g\,\delta^\mu_\nu\right)\,.
\eeqn
Equation (\ref{eomrewr}) is linear in curvatures for $\gmn$, but it is highly nonlinear in $\fmn$ which appears under a square-root within the tensor-valued functions~$(Y^{(n)})^\mu_{~\nu}$. It is not obvious how to obtain a closed-form solution for~$\fmn$ from it, but we can easily arrive at a perturbative solution:
As in our simple example, we first solve (\ref{eomrewr}) algebraically for ${S^\mu}_\nu$ and afterwards square the result to obtain the solution for $\fmn$. To this end, we make the following perturbative ansatz
\begin{align}\label{ansatzs}
{S^\mu}_\nu=a\delta^\mu_\nu&+\tfrac{1}{m^2}\Big(b_1{P^\mu}_\nu+b_2\Tr\,P\,\delta^\mu_\nu\Big)
+ \tfrac{1}{m^4}\Big( c_1{(P^2)^\mu}_\nu+c_2\Tr\,P\,{P^\mu}_\nu   \nn\\
&+c_3\Tr\,P^2\delta^\mu_\nu+c_4(\Tr\,P)^2\delta^\mu_\nu \Big) 
+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,,
\end{align}
with arbitrary complex coefficients $a, b_i, c_i,\hdots$ Allowing the parameters to assume complex values is reasonable as long as the coefficients that will finally appear in the effective action remain real. One can think of complex parameters in the solution for ${S^\mu}_\nu$ as being merely a tool to arrive at the most general solution. 
As we will see in section~\ref{secPMCG}, an example for a case with complex coefficients is the PM theory in which the perturbative solution for ${S^\mu}_\nu$ turns out to be purely imaginary. This leads to a real solution for $\fmn$ as well as a real effective action for $\gmn$. 

In what follows, the strategy will be to plug the above ansatz for ${S^\mu}_\nu$ into the $\gmn$ equation (\ref{eomrewr}) and fix its coefficients by satisfying the equation at each order in $P/m^2$ separately. 
In order to simplify the expressions in the following, we introduce two new sets of linear combinations of the $\beta_n$ parameters,
\beqn\label{snalphan}
s_n\equiv \sum_{k=n}^{d-1}{d-1-n\choose k-n}a^k\beta_k\,,\qquad \alpha_n=\sum_{k=n}^d {d-n \choose k-n} a^k\beta_k\,.
\eeqn
It is easy to show that these obey
\beqn\label{salphaid}
s_n=\alpha_n-\alpha_{n+1}\,.
\eeqn
On proportional backgrounds, $\fmn=c^2\gmn$ and $s_0$ is proportional to the cosmological constant $\Lambda_g$ defined in~(\ref{lambdas}) if in that expression one replaces $c$ by $a$. As we will see below, the equation of motion enforces $s_0=0$, and hence if $c=a$ the solutions for both of the metrics are flat. 
On these backgrounds then $s_1$ is proportional to the Fierz-Pauli mass~(\ref{FPmass}). In general, however, $c\neq a$ and the sums $s_n$ have no direct interpretation.

In the following it will be convenient to work with ${M^\mu}_\nu\equiv{S^\mu}_\nu/a- \delta^\mu_\nu$, for which the ansatz~(\ref{ansatzs}) starts at linear order in curvatures. In terms of this matrix we can rewrite powers and symmetric polynomials of ${S^\mu}_\nu$ as follows,
\begin{align}
 {(S^{n-k})^\mu}_\nu&=a^{n-k}\sum_{r=0}^{n-k}{n-k\choose r}{(M^r)^\mu}_\nu\,,\nn  \\
 e_k(S)&=a^k\sum_{m=0}^k{d-m\choose k-m}e_m(M)\,. \label{eitoM}
 \end{align}
These expressions enter the $\gmn$ equation of motion through the definition~(\ref{defY}) of ${(Y^{(n)})^\mu}_\nu$.
At this point let us also remark that from the latter equation in (\ref{eitoM}) it follows that the interaction potential in the bimetric action written in terms of ${M^\mu}_\nu$ becomes
 \beqn
\sum_{n=0}^{d}\beta_ne_n(S)=\sum_{n=0}^d\alpha_ne_n(M)\,,\label{senwM} 
\eeqn
which involves the $\alpha_n$ parameters defined above.
This identity will become useful in the next section when we derive the effective action for $\gmn$.

Next we use (\ref{eitoM}) in the definitions (\ref{defY}) of the matrices ${(Y^{(n)})^\mu}_\nu$ and plug the resulting expressions into the $\gmn$ equation of motion (\ref{eomrewr}). The outcome is  
\beqn
&~&m^2\sum_{n=0}^{d-1}a^n\beta_n \sum_{k=0}^n \sum_{m=0}^k \sum_{r=0}^{n-k}   (-1)^{n+k}{d-m\choose k-m}{n-k\choose r} e_m(M){(M^r)^\mu}_\nu\nn\\
&=&\Tr\,P~\delta^\mu_\nu-{P^\mu}_\nu\,.
\eeqn
The right-hand side of this equation is linear in curvatures for $\gmn$, whereas the left-hand side is a polynomial of degree $(d-1)$ in ${M^\mu}_\nu$.
In order to solve the equation perturbatively, we now insert our ansatz (\ref{ansatzs}) and compare the coefficients of $\delta^\mu_\nu$, ${P^\mu}_\nu$, $\Tr\,P\,\delta^\mu_\nu$, etc.~on both sides. For this, of course, one also needs to invoke the explicit expressions of the elementary symmetric polynomials $e_m$ that we list in (\ref{listesp}) for $m\leq4$.


For the lowest three orders it is simple to carry out this procedure by hand. The results are
\begin{align}\label{parsollo}
\mathcal{O}(1):&~~~~s_0\equiv\sum_{n=0}^{d-1} {d-1\choose n}\beta_na^n=0\,,\nn\\
\mathcal{O}\left(\tfrac{P}{m^2}\right):&~~~~  b_1=\frac{a}{s_1}\,,\quad  b_2=0\,,\nn\\
\mathcal{O}\left(\tfrac{P^2}{m^4}\right):&~~~~ 2(d-1)c_4=-2(d-1)c_3=-c_2=c_1=\frac{as_2}{s_1^3}\,.
\end{align}
The equation at lowest order, $s_0=0$, is a polynomial in $a$ that determines $a$ in terms of the $\beta_n$. Here we see explicitly that it is possible to have complex solutions for $a$ which, as stated before, do not cause any problems as long as all parameters appearing in the effective action and equations for $\gmn$ remain real. We will encounter an example for this situation in the next section. Order by order, the other equations determine the coefficients in the ansatz for ${S^\mu}_\nu$. 
Hence the perturbative solution that we have been looking for is of the following form,
\begin{align}\label{sols}
{S^\mu}_\nu=a\delta^\mu_\nu&+\tfrac{a}{s_1m^2}{P^\mu}_\nu +\tfrac{as_2}{s_1^3m^4}\Big[{(P^2)^\mu}_\nu-\Tr\,P\,{P^\mu}_\nu+\tfrac{1}{d-1}e_2( P)\delta^\mu_\nu\Big] \nn\\
&+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,.
\end{align}
For general $\beta_n$ the right-hand side is an infinite expansion in curvatures. The only case for which the series is known to terminate is the model with $\beta_n=0$ for $n=2,3\hdots d-1$ that we discussed previously.
Furthermore, the suppressing mass scale is $s_1m^2$ which, as we argued before, is proportional to the Fierz-Pauli mass of the massive fluctuation in flat space. Note also the absence of a term proportional to $\Tr\,P$ in~(\ref{sols}) as well as the fact that all relative coefficients between the quadratic curvature contributions are simply numbers independent of the parameters of the theory. For higher curvature corrections, which we have found with the help of a computer up to fifth order in curvatures, this is no longer true because some of the ratios between coefficients will become parameter dependent. 


Finally, we use $\fmn=g_{\mu\rho}{(S^2)^\rho}_\nu$ to arrive at
\begin{align}\label{fsolP}
\fmn=a^2\gmn&+\tfrac{2a^2}{s_1m^2}P_{\mu\nu}+\tfrac{a^2(s_1+2s_2)}{s_1^3m^4}{(P^2)^\mu}_\nu\nn\\
&+\tfrac{2a^2s_2}{s_1^3m^4}\Big[\tfrac{1}{d-1}e_2( P)\delta^\mu_\nu-\Tr\,P\,{P^\mu}_\nu\Big]
+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,.
\end{align}
This is the most general perturbative solution for $\fmn$ obtained from the $\gmn$ equation.

At this point let us make the remark that there are special corners in parameter space for which the perturbative solution does not exist. For instance, if $\beta_0=0$ then $a=0$ is a solution to $s_0=0$ and in this case it is not possible to find a perturbative solution for~$\fmn$. Another example of this type is a set of $\beta_n$ parameters such that $s_1=0$. In this case the perturbative solution at $\mathcal{O}(P/m^2)$ enforces $R_{\mu\nu}(g)=0$, i.e.~the solution for $\gmn$ has to be flat. It is certainly interesting to understand the nature of these special cases, but here our main focus lies on generic values for the parameters of the theory for which the perturbative solution exists.

An immediate consequence of the existence of the solution (\ref{fsolP}) is that if the solution for $\gmn$ has constant curvature, $P_{\mu\nu}\propto\gmn$, then it follows from (\ref{fsolP}) that $\fmn\propto\gmn$, i.e.~the two metrics are proportional to each other. But, as we saw in section~\ref{secpropbg}, this implies that also $\fmn$ has constant curvature. Of course, we can just as well solve the~$\fmn$ equation algebraically for $\gmn$ and interchange the roles of $\gmn$ and $\fmn$ in the argument, and hence a constant curvature solution for one of the metrics always implies proportional backgrounds and a constant curvature solution for the other metric.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Resulting theory for $\gmn$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Following the strategy described in section~\ref{sec:outl}, we now use the solution~(\ref{fsolP}) for $\fmn$ to eliminate it in the bimetric action~(\ref{HR}). 
In the interaction potential this is straightforward: One simply uses~(\ref{senwM}) to obtain an expansion in curvatures of~$\gmn$. Since the expansion of the matrix ${M^\mu}_\nu\equiv{S^\mu}_\nu/a- \delta^\mu_\nu$ starts with a term linear in~${P^\mu}_\nu$, only $e_n(M)$ with $n=0,1,2$ contribute to quadratic order in $P/m^2$. 

The kinetic term for $\fmn$ is a bit more tricky. First, we need to evaluate the inverse and the Jacobian determinant of $\fmn$. The result for the inverse reads
\beqn
(f^{-1})^{\mu\nu}=a^{-2}g^{\mu\nu}-\frac{2}{a^2s_1m^2}P^{\mu\nu}+\mathcal{O}\left(\tfrac{P^2}{m^4}\right)\,.
\eeqn
It is sufficient to expand this to first order in curvatures because in the kinetic term it is contracted with the Ricci tensor for $\fmn$ which involves no constant term. Furthermore, we have
\beqn 
\sqrt{f}=\sqrt{g}\,\det S=\sqrt{g}\,\det(a\mathbb{1}+aM)=a^d\sqrt{g}\sum_{n=0}^de_n(M)\,,
\eeqn
in which now only terms with $n=0,1$ contribute to quadratic order in curvatures.

In order to evaluate the Ricci tensor for $\fmn$, we invoke once more the curvature relations (\ref{curvrel}). With their help we can express $R_{\mu\nu}(f)$ as $R_{\mu\nu}(g)$ plus terms with covariant derivatives acting on $\gmn$ curvatures. It turns out that terms involving $\gmn$-covariant derivatives (which anyway would only give a total derivative contribution) drop out of the action upon use of the Bianchi identity. More details are provided in {\protect{\hyperref[papVIII]{Paper~VIII}}}, here we simply present the final result.
Putting everything together gives the following effective action for~$\gmn$,
\begin{align}\label{HDactobt}
    S_\mathrm{HD}=m_g^{d-2}&\int\dd^dx\sqrt{g}\,\Big[ c_\Lambda+c_RR(g)\nn\\
    &-\frac{c_{RR}}{m^2}\Big(R^{\mu\nu}R_{\mu\nu}-\frac{d}{4(d-1)}R^2\Big) \Big]~+~\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,.
\end{align}
The coefficients of different orders in curvatures are related to the original bimetric parameters through
\begin{align}
c_\Lambda&=-2m^2\alpha_0\,, \qquad c_R=1+(\alpha a)^{d-2}-\frac{\alpha_1(d-2)}{s_1(d-1)}\,,\nn\\
c_{RR}&=\frac{1}{s_1^2}\left( 2s_1(\alpha a)^{d-2}-\alpha_2+\frac{\alpha_1s_2(d-2)}{s_1(d-1)} \right)\,.
\end{align}
Remarkably, the effective action (\ref{HDactobt}) is exactly of the form (\ref{HDact}). In particular, the relative coefficient in between the two quadratic curvature coefficients is independent of the parameters of the theory and fixed to the value that removes the Boulware-Deser ghost from the spectrum. This is of course expected considering the fact that we started from the ghost-free bimetric theory. 

In the beginning of this chapter we showed that the quadratic curvature action (\ref{HDact}) always contains a spin-2 ghost. Clearly, this is not the case in bimetric gravity which gives rise to two healthy spin-2 modes at the linearized level. In {\protect{\hyperref[papVIII]{Paper~VIII}}} we  try to localize the origin of the inconsistency using a simplified model of two scalar fields. This example shows that the ghost is most likely not introduced by our procedure of obtaining the effective action for $\gmn$. That is to say,  we believe that the extra zero modes to the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ that appear in the solution are not responsible for the inconsistency. Rather, the scalar field model suggests that the ghost instability arises when the theory with infinitely many derivatives is truncated to the four-derivative level. This result is also in accordance with Ostrogradski's theorem.  We are thus lead to making the following conjecture: The local higher derivative theory with action $S_\mathrm{HD}$ obtained from bimetric gravity by integrating out $\fmn$ using the $\gmn$ equation provides a ghost-free extension of the incomplete quadratic curvature action~$S_\mathrm{HD}^{(2)}$.

Note also that the sources may be included into the theory by making the replacement~(\ref{sourcerepl}) in~(\ref{HDactobt}). As a result, in the effective action, the ghost-free coupling to matter sources is highly nontrivial. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Partially massless case}\label{secPMCG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now specialize to four space-time dimensions where, as we demonstrated in chapter~\ref{ch:PM}, the family of bimetric theories contains a candidate for the nonlinear theory of a partially massless field. But instead of fixing the parameters in the interaction potential immediately to their PM values, let us start from a different direction: Suppose our interest lies in finding the parameter values for which the higher-derivative action~(\ref{HDactobt}) obtained from bimetric gravity reduces to the Conformal Gravity action~(\ref{CGact}) at lowest order in derivatives. Clearly, this means that we must have
\beqn\label{condCG}
c_\Lambda=-2m^2\alpha_0=0\,,\qquad c_R=1+(\alpha a)^2-\frac{2\alpha_1}{3s_1}=0\,.
\eeqn
Recall that satisfying the $\gmn$ equation required $s_0=0$. Then, the identity (\ref{salphaid}) together with the first of the above conditions, $\alpha_0=0$, imply that also $\alpha_1=0$. Using this in the second condition we see that we must have $a=\pm i\alpha^{-1}$. Now we plug this value for $a$ into $s_0=0$ and $\alpha_0=0$ which we evaluate in terms of the $\beta_n$ parameters. This gives two complex equations,
\beqn
\beta_0+\frac{3i}{\alpha}\beta_1-\frac{3}{\alpha^2}\beta_2-\frac{i}{\alpha^3}\beta_3&=&0\,,\nn\\
\beta_0+\frac{4i}{\alpha}\beta_1-\frac{6}{\alpha^2}\beta_2-\frac{4i}{\alpha^3}\beta_3+\frac{1}{\alpha^4}\beta_4&=&0\,.
\eeqn
The real and imaginary parts must vanish separately and the unique solution is
\beqn\label{PMparz}
\beta_1=\beta_3=0\,,\qquad \alpha^2\beta_0=3\beta_2=\alpha^{-2}\beta_4\,.
\eeqn
Remarkably, these values precisely corresponds to the PM parameter choice in $d=4$ that we found in chapter~\ref{ch:PM}. We conclude that the PM candidate is the unique member of the family of bimetric theories with the feature that to lowest order in a derivative expansion the effective action for $\gmn$ is conformally invariant. To lowest order, the corresponding equations of motion obtained from the effective action for $\gmn$ are those of Conformal Gravity,
\beqn
B_{\mu\nu}+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)=0\,.
\eeqn
Moreover, it is straightforward to show that the first method that we explained in section~\ref{sec:outl} yields a similar result:
The effective equation for $\gmn$, obtained from solving the $\gmn$ equation for $\fmn$ and plugging the solution into the $\fmn$ equation, also sets the Bach tensor to zero at lowest order in derivatives.
This is expected since the first term in the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ in (\ref{HDactvar}) is proportional to the identity and hence the lowest-order terms are the same for both ways of integrating out $\fmn$.  

The nonlinear PM bimetric theory therefore proposes a ghost-free completion of Conformal Gravity. The presence of a gauge symmetry to lowest order in a derivative expansion further supports the existence of a PM gauge symmetry in the theory. In turn, if it exists, the PM symmetry constitutes the generalization of the gauge invariance of Conformal Gravity to higher orders in derivatives.

\subsubsection{Constructing the PM symmetry} 

The perturbative solution to the $\gmn$ equation and the analogous solution to the $\fmn$ equation can be used to construct the PM symmetry transformation order by order in derivatives. In fact, this method is powerful enough to prove the existence of a PM symmetry perturbatively. This is the subject of an upcoming publication and will not be discussed in detail in this thesis. However, since it strengthens the importance of {\protect{\hyperref[papVI]{Paper~VI}}}, {\protect{\hyperref[papVII]{Paper~VII}}} and {\protect{\hyperref[papVIII]{Paper~VIII}}}, let us briefly outline the idea of the proof.

An important tool in what follows is the discrete interchange symmetry of the PM candidate theory. Namely, recall that the action and the equations of motions are invariant under
\beqn\label{intsymPM}
\alpha^{-1}\gmn\longleftrightarrow \alpha \fmn\,.
\eeqn
With the PM parameters~(\ref{PMparz}), the perturbative solutions to the $\gmn$ and $\fmn$ equations of motion, respectively, assume the form,
\beqn\label{pertsolpm}
\fmn&=&-\alpha^{-2}\gmn+\frac{1}{\beta_2m^2}P_{\mu\nu}+\gamma_{\mu\nu}(\alpha^{-1}g,P)\,,\nn\\
\gmn&=&-\alpha^2\fmn+\frac{\alpha^2}{\beta_2m^2}\tilde{P}_{\mu\nu}+\alpha^2\gamma_{\mu\nu}(\alpha f,\tilde{P})\,,
\eeqn
where $\tilde{P}$ denote curvatures for $\fmn$. Furthermore, the function $\gamma_{\mu\nu}$ contains all higher-order contributions, starting at the four-derivative level. Due to the interchange symmetry (\ref{intsymPM}) the higher orders have the same functional form in both equations. 


It is easy to see that, to lowest order in derivatives, the perturbative solutions in (\ref{pertsolpm}) are invariant under two conformal transformations,
\begin{align}
\Delta\gmn&=\phi(x)\gmn + \mathcal{O}\left(\tfrac{P}{m^2}\right)\,,\nn\\
\Delta\fmn&=\phi(x)\fmn + \mathcal{O}\left(\tfrac{\tilde{P}}{m^2}\right)=-\alpha^{-2}\phi(x)\gmn+ \mathcal{O}\left(\tfrac{P}{m^2}\right)\,.
\end{align}
In the second line, we have used the solution for $\fmn$ to give two different expressions for its transformation: one that can be obtained from the $\gmn$ transformation via the interchange symmetry (\ref{intsymPM}) and one for which the invariance of the perturbative solutions is manifest. 
 
Although the conformal transformations are a symmetry of the lowest order terms in the above equations, it is clear that they will not leave the higher-order contributions invariant. In order to cancel the effects of the conformal transformations in higher orders, we need to include higher-derivative terms into the symmetry transformations of the metrics.

The next order of the transformations has two derivatives and consists of terms involving covariant derivatives acting on $\phi$ or curvatures multiplying $\phi$. They are constructed by plugging the lowest order of the transformation into the two-derivative terms of the equations. In order to cancel out these contributions one then adds corresponding terms in the transformations for $\gmn$ and $\fmn$. In fact, it is sufficient to consider only one of the above equations, say the solution for $\fmn$, and write down the necessary terms in the transformations to guarantee invariance of this equation. Then, for each type of term, there will still be an arbitrary relative coefficient between the $\gmn$ and $\fmn$ transformation. 
This coefficient is then fixed by imposing the interchange symmetry (\ref{intsymPM}). In this way, since it can be obtained from the solution for $\fmn$ through the interchange symmetry, the solution for $\gmn$ will also be invariant under the PM symmetry by construction. 

The results for the transformations to second order in derivatives derived in this manner have the following form,
\beqn\label{PMtrafso}
\Delta\gmn&=&\phi\gmn - \frac{\alpha^2}{2\beta_2m^2}\nabla_\mu\partial_\nu \phi-\frac{\alpha^2}{2\beta_2m^2}P_{\mu\nu}\phi+ \mathcal{O}\left(\tfrac{P^2}{m^4}\right)\,,\nn\\
\Delta\fmn&=&\phi\fmn - \frac{1}{2\beta_2m^2}\tilde{\nabla}_\mu\partial_\nu \phi-\frac{1}{2\beta_2m^2}\tilde{P}_{\mu\nu}\phi+\mathcal{O}\left(\tfrac{\tilde{P}^2}{m^4}\right)\nn\\
&=&-\alpha^{-2}\phi\gmn - \frac{1}{2\beta_2m^2}\nabla_\mu\partial_\nu \phi+\frac{1}{2\beta_2m^2}P_{\mu\nu}\phi+\mathcal{O}\left(\tfrac{\tilde{P}^2}{m^4}\right)\,.\nn\\
\eeqn
Again, we have expressed the $\fmn$ transformation in two different ways that are equivalent on-shell. The expression in the last line can be used to check the invariance of the perturbative solutions explicitly. When using the solution for $\fmn$ to rewrite its transformation in terms of only $\gmn$ and its curvatures, one introduces new higher-derivative terms that need to be taken care of at the next orders. This is how, for example, the term proportional to $P_{\mu\nu}\phi$ enters the transformations. 
A term $P\gmn\phi$ is absent because it is not introduced by using the perturbative solution for~$\fmn$.

The above construction of the transformations can be continued step by step at each order in derivatives, resulting in a perturbative expression for the PM gauge symmetry. Performing this construction explicitly is intricate already at the four-derivative level. Nevertheless, the mere fact that it is possible to construct the symmetry in a derivative expansion proves its existence on the perturbative solutions. Although these solutions are not the most general ones\footnote{For example, the perturbative solutions imply that if the curvatures are diagonal then so are the metrics, whereas bimetric theory is known to also contain solutions for which this is not the case, see e.g.~\cite{Volkov:2013roa}. However, in $d=4$, these are not continuously connected to the perturbative solutions above.}, they make up a large isolated class of all possible solutions. The existence of a gauge symmetry on this class of solutions is therefore highly nontrivial and furthermore supports its presence in the full theory.

Note that the precise form of the perturbative solutions in~(\ref{pertsolpm}) is unique to the PM parameters. It is quite simple to show that, for any other values of the $\beta_n$ parameters, the construction of a gauge symmetry fails latest at the two-derivative level. This could have been expected, since it was only the PM parameters that lead to the conformally invariant Bach equation when the $\gmn$ and $\fmn$ equations where combined. We conclude that our PM candidate theory is the unique theory with a scalar gauge symmetry in the perturbative solutions to its equations of motion.

To conclude this discussion, let us demonstrate that the above transformations reduce to the well-known PM gauge symmetry in the linear theory around a de Sitter background.
To this end, recall the transformation for the massive fluctuation $\delta M_{\mu\nu}$ around proportional backgrounds which, in $d=4$, can be written as
\beqn\label{linPMsym3}
\Delta (\delta M_{\mu\nu}) =  \phi(x)\bar{g}_{\mu\nu} +\frac{3}{\Lambda_g}\bar{\nabla}_\mu\partial_\nu\phi(x)\,.
\eeqn
According to its definition in (\ref{dGanddM}), the massive fluctuation satisfies $\delta M_{\mu\nu}\propto \delta\fmn-c^2\delta\gmn$. This implies that its transformation under the PM symmetry must be proportional to $\Delta\fmn-c^2\Delta\gmn$ evaluated on the proportional backgrounds. 
For $\bar{f}_{\mu\nu}=c^2\bar{g}_{\mu\nu}$ we have that
\beqn
P_{\mu\nu}(\bar{g})=\tilde{P}_{\mu\nu}(\bar{f})= \frac{\Lambda_g}{3}\bar{g}_{\mu\nu}\qquad \Lambda_g=3\beta_2m^2(1+\alpha^2c^2)\,.
\eeqn
Using these results in (\ref{PMtrafso}) it can easily be checked that on these backgrounds one obtains
\beqn
\left.\left(\Delta\fmn-c^2\Delta\gmn\right)\right|_{\bar{f}_{\mu\nu}=c^2\bar{g}_{\mu\nu}}=\frac{1}{2}(\alpha^4c^4-1)\left[\phi\bar{g}_{\mu\nu}+\frac{3}{\Lambda_g}\bar{\nabla}_\mu\partial_\nu\phi\right]\,,
\eeqn
which is indeed proportional to (\ref{linPMsym3}).
Hence, the above nonlinear transformations generate precisely the PM transformation of the massive fluctuation. As a side remark, let us point out that this also means that the higher-order terms of the PM transformation of $\delta M_{\mu\nu}$ must vanish on the proportional backgrounds.

The fact that we arrive at the correct form (\ref{linPMsym3}) starting from the nonlinear transformations shows that the gauge symmetry we constructed above corresponds precisely to the PM invariance of the linear theory. 
Our nonlinear PM candidate thus explains the origin of the PM symmetry around de Sitter backgrounds and, even at the nonlinear level, a gauge symmetry removes one degree of freedom. 


 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Summary $\&$ Outlook}
\label{ch:concl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this thesis, we discussed ghost-free nonlinear theories involving massive spin-2 fields. Our findings are summarized below.


\begin{itemize}

\item[$\diamond$] There are two classes of consistent nonlinear theories for massive spin-2 fields of rather distinct nature: Nonlinear Massive Gravity~\cite{deRham:2010kj, Hassan:2011vm} contains self-interactions of a massive spin-2 field in a background that is fixed by hand, whereas bimetric theory~\cite{Hassan:2011zd} describes two dynamical spin-2 fields, one with massive and one with massless fluctuation around maximally symmetric backgrounds. We demonstrated the absence of the Boulware-Deser ghost instability in nonlinear Massive Gravity both in the physical gauge and in a diffeomorphism invariant formulation. 

\item[$\diamond$] We computed the mass spectrum of bimetric theory around proportional background solutions and identified nonlinear fields with massive and massless fluctuations around these backgrounds. A Hamiltonian analysis revealed that the nonlinear massless field cannot have standard matter couplings, which suggested that, in the presence of a massive spin-2 field, the gravitational metric is a superposition of mass eigenstates.

\item[$\diamond$] In the vielbein formulation, bimetric theory can be generalized to describe interactions of multiple spin-2 fields~\cite{Hinterbichler:2012cn}. We introduced a set of St\"uckelberg fields to reinstore the broken local Lorentz symmetry in the theory, which enabled us to reformulate the multivielbein theory in terms of the respective metrics.


\item[$\diamond$] The most general homogeneous and isotropic solutions to the bimetric equations of motion were derived and in some special cases discussed in more detail. The parameters of the interaction potential could be fitted to observational data and thus, at the background level, bimetric theory could account for the observed cosmologial evolution. Certain parameter subspaces even gave rise to a viable self-accelerating cosmological expansion without the need to include vacuum energy~\cite{Akrami:2012vf}.

\item[$\diamond$] We developed a method to identify nonlinear candidate theories for a partially massless spin-2 field within the family of bimetric actions. The equations of motion in such a theory should be invariant under a generalization of the gauge symmetry for linear PM fields in de Sitter backgrounds.
In the four-dimensional candidate theory, several aspects pointed towards the presence of a gauge symmetry at the nonlinear level. 
In space-time dimensions greater than four, it was necessary to extend the bimetric action by the Lanczos-Lovelock terms in order to obtain nontrivial results.


\item[$\diamond$] Bimetric theory was shown to be closely related to a certain class of higher-curvature theories for gravity which are known to be free of the Boulware-Deser ghost. On the other hand, these theories contain a spin-2 field whose helicity components all show instabilities. We argued that this problem may be cured by completing the quadratic curvature terms in the action into an infinite expansion in derivatives whose form can be derived from bimetric gravity. 

\item[$\diamond$] A close connection between our candidate theory for nonlinear partial masslessness and Conformal Gravity was established. The equations of motion of PM bimetric theory were shown to be conformally invariant at the four-derivative level in a perturbative expansion. This observation further allowed us to explicitly construct the PM gauge symmetry perturbatively to second-order in derivatives, which resulted in an expression compatible with the well-known transformation of linear PM fields. Moreover, the perturbative solutions to the equations of motion in the PM bimetric theory opened up the possibility to prove the existence of a gauge symmetry at the nonlinear level.
\end{itemize}


Open issues in the field of nonlinear Massive Gravity and bimetric theory can be divided into phenomenological and more theoretical questions. On the phenomenology side, further investigation of classical solutions to the equations of motion is of great interest. On the theory side, it is most interesting to look for extensions of the consistent theories in order to fit them into a larger framework. In the following we mention some of the vividly ongoing research. 

\vspace*{5mm}

Having found viable cosmological background solutions to the bimetric equations, the next test the theory needs to pass is whether it can explain growth of structure in the universe. In order to address this question, one needs to study perturbations around the cosmological solutions. Unfortunately, this type of analysis is complicated by the square-root matrix in the interaction potential. First attempts to derive and solve the perturbation equations have been made in~\cite{Comelli:2012db, Berg:2012kn}, but the compatibility of bimetric theory with constraints from structure formation is still an open question.

Another important issue in theories with massive spin-2 fields coupled to matter is the existence of a Vainshtein mechanism in order to avoid the observationally discarded vDVZ discontinuity. Spherically symmetric solutions to the bimetric equations have been investigated in \cite{Comelli:2011wq, Volkov:2013roa, Volkov:2012wp}. The possibility for a Vainshtein mechanism and the reconcilability with astrophysical data were shown to be given both in Massive Gravity~\cite{Sjors:2011iv} and in bimetric theory~\cite{Enander:2013kza}.


The evidence for the existence of a gauge symmetry, which we discovered in several independent approaches, exposes the exceptional nature of the nonlinear PM bimetric theory. It would be of great interest to derive the explicit non-perturbative form of the gauge transformations that leave the bimetric equations invariant. But even without the knowledge of the exact transformations, physical aspects of the theory can be studied. An analysis of implications for cosmology has been started, for example, in~\cite{Akrami:2013ffa}. Moreover, in \cite{Brito:2013yxa} it was shown that the PM theory avoids the Gregory-Laflamme instability~\cite{Gregory:1993vy} which is a generic undesirable feature of black-hole solutions in nonlinear Massive Gravity and bimetric theory~\cite{Babichev:2013una, Brito:2013wya}.

Eventually, one would of course also like to return to the original motivation for constructing a nonlinear Massive Gravity theory and readdress the cosmological constant problem. So far, an obvious solution to the problem has been found neither in Massive Gravity nor in bimetric gravity. The self-accelerating cosmological backgrounds discussed in \cite{Akrami:2012vf, Akrami:2013ffa} demonstrate that bimetric theory can account for the observed rate of cosmic acceleration without any vacuum energy.
The acceleration is due to a spin-2 field with mass at the Hubble scale, which mildens the cosmological constant problem because a small spin-2 mass is technically natural. On the other hand, the origin of the small value for the graviton mass as well as the disappearance of vacuum energy from quantum field theory remain unexplained in this setup. 






\vspace*{5mm}


Turning to the prospects on the theory side, we emphasize that extensions of the bimetric action primarily need to maintain the consistency of the theory. In particular, they must not reintroduce the Boulware-Deser ghost instability. One possibility of extending the theory is then given by the Lanczos-Lovelock terms that we already considered in {\protect{\hyperref[papVII]{Paper~VII}}}. These are commonly believed to avoid the Boulware-Deser ghost and therefore provide a viable generalization of the Hassan-Rosen action. 
Another conceivable extension is the addition of further derivative interactions that respect the antisymmetric structure of the interaction potential and the LL terms. The consistency of such new interactions has recently been suggested in a pseudo-linear analysis~\cite{Hinterbichler:2013eza}, while their precise nonlinear form is still unknown.

Other extensions involving additional scalar fields have been introduced mainly in the context of nonlinear Massive Gravity. For example, it has been suggested to promote the $\beta_n$-parameters to functions of a scalar field~\cite{Huang:2012pe, Huang:2013mha}.
Furthermore, the proposals involve coupling the metric $\gmn$ to fields with Galileon symmetry~\cite{Gabadadze:2012tr} and to a quasi-dilaton~\cite{D'Amico:2012zv}. If the quasi-dilaton is self-interacting, the theory is classically equivalent to the Massive Gravity action extended by functions of the Ricci scalar~\cite{Cai:2013lqa}. A similar $f( R)$ generalization has also been considered for bimetric gravity~\cite{Nojiri:2013zza}.


Another important issue is the computation of quantum corrections to the consistent nonlinear actions for spin-2 fields. A first attempt to this effect has been made in~\cite{Buchbinder:2012wb} which, however, worked with the auxiliary model that we discussed in section~\ref{hamstuck}. Although, classically, this model is equivalent to the Massive Gravity action with a certain parameter choice, the two theories may differ at the quantum level. More recently, the one-loop effective action of the dRGT model was computed in~\cite{deRham:2013qqa}. There it was demonstrated that, at one-loop level, matter fields running in the loop do not change the structure of the interaction potential for the metric, whereas the ghost-free configuration does get modified by gravitons in the loop. Fortunately, the authors also argue that the mass of the ghost is never below the Planck scale and therefore does not propagate in the effective theory. These promising results suggest that consistent nonlinear Massive Gravity may be stable under quantum corrections. Besides the computation of higher-order loop diagrams in the dRGT model with fixed Minkowski background, it would be interesting to investigate whether this feature is shared by the fully dynamical bimetric theory.


Finally, one could explore the possibility of embedding the consistent bimetric models in String Theory. The most promising candidate for a unified description of particle physics and quantum gravity possesses a rich spectrum of massless and massive higher-spin fields. In particular, it contains a massless spin-2 field whose low-energy effective action is Einstein-Hilbert plus higher-curvature corrections. But the spectrum also includes a massive spin-2 field whose effective action has not been computed.
%\footnote{Derivations of effective actions in String Theory are very involved and usually the focus lies on massless fields that are most relevant in the low-energy limit.} 
It is therefore an interesting open question whether the ghost-free structure of the nonlinear massive spin-2 theories discussed in this thesis can be reproduced in String Theory. If this is the case, then, since phenomenologically viable String Theory requires Supersymmetry, it will contain a supersymmetrized version of bimetric theory. This motivates the search for a supersymmetric theory involving massive spin-2 fields which, even without String Theory, could be an interesting subject on its own. Interestingly, such a theory was already suggested several decades ago in~\cite{Chamseddine:1978yu} but without addressing the ghost issue.

Concluding remarks





 



\begin{thebibliography}{999}
\bibitem{Einstein:1916vd}
  A.~Einstein,
  %``The Foundation of the General Theory of Relativity,''
  Annalen Phys.\  {\bf 49} (1916) 769
   [Annalen Phys.\  {\bf 14} (2005) 517].
  %%CITATION = ANPYA,49,769;%%   
\bibitem{Fierz:1939ix}
  M.~Fierz and W.~Pauli,
  %``On relativistic wave equations for particles of arbitrary spin in 
  %an electromagnetic field,'' 
  Proc.\ Roy.\ Soc.\ Lond.\ A {\bf 173} (1939) 211.
  %%CITATION = PRSLA,A173,211;%%
\bibitem{vanDam:1970vg}
  H.~van Dam and M.~J.~G.~Veltman,
  %``Massive and massless Yang-Mills and gravitational fields,''
  Nucl.\ Phys.\ B {\bf 22} (1970) 397.
  %%CITATION = NUPHA,B22,397;%%
\bibitem{Zakharov:1970cc}
  V.~I.~Zakharov,
  %``Linearized gravitation theory and the graviton mass,''
  JETP Lett.\  {\bf 12} (1970) 312
   [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 12} (1970) 447].
  %%CITATION = JTPLA,12,312;%%
\bibitem{Vainshtein:1972sx}
  A.~I.~Vainshtein,
  %``To the problem of nonvanishing gravitation mass,''
  Phys.\ Lett.\ B {\bf 39} (1972) 393.
  %%CITATION = PHLTA,B39,393;%%
\bibitem{Boulware:1972zf}
  D.~G.~Boulware and S.~Deser,
  %``Inconsistency of finite range gravitation,''
  Phys.\ Lett.\ B {\bf 40} (1972) 227.
  %%CITATION = PHLTA,B40,227;%%
\bibitem{Boulware:1973my}
  D.~G.~Boulware and S.~Deser,
  %``Can gravitation have a finite range?,''
  Phys.\ Rev.\ D {\bf 6} (1972) 3368.
  %%CITATION = PHRVA,D6,3368;%%
\bibitem{ArkaniHamed:2002sp}
  N.~Arkani-Hamed, H.~Georgi and M.~D.~Schwartz,
  %``Effective field theory for massive gravitons and gravity in
  %theory space,'' 
  Annals Phys.\  {\bf 305} (2003) 96
  [hep-th/0210184].
  %%CITATION = HEP-TH/0210184;%%
\bibitem{de Urries:1998bi}
  F.~J.~de Urries and J.~Julve,
  %``Ostrogradski formalism for higher derivative scalar field theories,''
  J.\ Phys.\ A {\bf 31} (1998) 6949
  [hep-th/9802115].
  %%CITATION = HEP-TH/9802115;%%
\bibitem{deRham:2010ik}
  C.~de Rham and G.~Gabadadze,
  %``Generalization of the Fierz-Pauli Action,''
  Phys.\ Rev.\ D {\bf 82} (2010) 044020
  [arXiv:1007.0443 [hep-th]].
  %%CITATION = ARXIV:1007.0443;%%
\bibitem{deRham:2010kj}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Resummation of Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 106} (2011) 231101
  [arXiv:1011.1232 [hep-th]].
  %%CITATION = ARXIV:1011.1232;%%
\bibitem{Hassan:2011vm}
  S.~F.~Hassan and R.~A.~Rosen,
  %``On nonlinear Actions for Massive Gravity,''
  JHEP {\bf 1107} (2011) 009
  [arXiv:1103.6055 [hep-th]].
  %%CITATION = ARXIV:1103.6055;%%
\bibitem{Hassan:2011hr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Resolving the Ghost Problem in nonlinear Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 108} (2012) 041101
  [arXiv:1106.3344 [hep-th]].
  %%CITATION = ARXIV:1106.3344;%%
\bibitem{Hassan:2011ea}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Confirmation of the Secondary Constraint and Absence of Ghost in Massive Gravity and Bimetric Gravity,''
  JHEP {\bf 1204} (2012) 123
  [arXiv:1111.2070 [hep-th]].
  %%CITATION = ARXIV:1111.2070;%%
\bibitem{Hassan:2011zd}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Bimetric Gravity from Ghost-free Massive Gravity,''
  JHEP {\bf 1202} (2012) 126
  [arXiv:1109.3515 [hep-th]].
  %%CITATION = ARXIV:1109.3515;%%
\bibitem{Rosen:1940zz}
  N.~Rosen,
  %``General Relativity and Flat Space. II,''
  Phys.\ Rev.\  {\bf 57} (1940) 150.
  %%CITATION = PHRVA,57,150;%%
\bibitem{Rosen:1975kk}
  N.~Rosen,
  %``Bimetric Theory of Gravitation,''
  In *Erice 1975, Proceedings, Topics In Theoretical and Experimental
  Gravitation Physics*, New York 1977, 273-294 
 \bibitem{Aragone:1971kh}
  C.~Aragone and S.~Deser,
  %``Constraints on gravitationally coupled tensor fields,''
  Nuovo Cim.\ A {\bf 3} (1971) 709.
  %%CITATION = NUCIA,A3,709;%%
\bibitem{Isham:1971gm}
  C.~J.~Isham, A.~Salam and J.~A.~Strathdee,
  %``F-dominance of gravity,''
  Phys.\ Rev.\ D {\bf 3} (1971) 867.
  %%CITATION = PHRVA,D3,867;%%  
\bibitem{Chamseddine:1978yu}
  A.~H.~Chamseddine, A.~Salam and J.~A.~Strathdee,
  %``Strong Gravity and Supersymmetry,''
  Nucl.\ Phys.\ B {\bf 136} (1978) 248.
  %%CITATION = NUPHA,B136,248;%%
\bibitem{Dvali:2000rv}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``Metastable gravitons and infinite volume extra dimensions,''
  Phys.\ Lett.\ B {\bf 484} (2000) 112
  [hep-th/0002190].
  %%CITATION = HEP-TH/0002190;%%
\bibitem{Dvali:2000hr}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``4-D gravity on a brane in 5-D Minkowski space,''
  Phys.\ Lett.\ B {\bf 485} (2000) 208
  [hep-th/0005016].
  %%CITATION = HEP-TH/0005016;%%
\bibitem{Kaluza:1921tu}
  T.~Kaluza,
  %``On the Problem of Unity in Physics,''
  Sitzungsber.\ Preuss.\ Akad.\ Wiss.\ Berlin (Math.\ Phys.\ ) {\bf 1921} (1921) 966.
  %%CITATION = SPWPA,1921,966;%%  
\bibitem{Klein:1926tv}
  O.~Klein,
  %``Quantum Theory and Five-Dimensional Theory of Relativity. (In German and English),''
  Z.\ Phys.\  {\bf 37} (1926) 895
   [Surveys High Energ.\ Phys.\  {\bf 5} (1986) 241].
  %%CITATION = ZEPYA,37,895;%% 
\bibitem{Bergshoeff:2009hq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``Massive Gravity in Three Dimensions,''
  Phys.\ Rev.\ Lett.\  {\bf 102} (2009) 201301
  [arXiv:0901.1766 [hep-th]].
  %%CITATION = ARXIV:0901.1766;%%
\bibitem{Deser:1981wh}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Topologically Massive Gauge Theories,''
  Annals Phys.\  {\bf 140} (1982) 372
   [Erratum-ibid.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 281} (2000) 409].
  %%CITATION = APNYA,140,372;%%
\bibitem{Deser:1982vy}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Three-Dimensional Massive Gauge Theories,''
  Phys.\ Rev.\ Lett.\  {\bf 48} (1982) 975.
  %%CITATION = PRLTA,48,975;%%
\bibitem{ArkaniHamed:2003uy}
  N.~Arkani-Hamed, H.~-C.~Cheng, M.~A.~Luty and S.~Mukohyama,
  %``Ghost condensation and a consistent infrared modification of gravity,''
  JHEP {\bf 0405} (2004) 074
  [hep-th/0312099].
  %%CITATION = HEP-TH/0312099;%%
\bibitem{Riess:1998cb}
  A.~G.~Riess {\it et al.}  [Supernova Search Team Collaboration],
  %``Observational evidence from supernovae for an accelerating universe and a cosmological constant,''
  Astron.\ J.\  {\bf 116} (1998) 1009
  [astro-ph/9805201].
  %%CITATION = ASTRO-PH/9805201;%%
\bibitem{Perlmutter:1998np}
  S.~Perlmutter {\it et al.}  [Supernova Cosmology Project Collaboration],
  %``Measurements of Omega and Lambda from 42 high redshift supernovae,''
  Astrophys.\ J.\  {\bf 517} (1999) 565
  [astro-ph/9812133].
  %%CITATION = ASTRO-PH/9812133;%%
\bibitem{Martin:2012bt}
  J.~Martin,
  %``Everything You Always Wanted To Know About The Cosmological Constant Problem (But Were Afraid To Ask),''
  Comptes Rendus Physique {\bf 13} (2012) 566
  [arXiv:1205.3365 [astro-ph.CO]].
  %%CITATION = ARXIV:1205.3365;%%
\bibitem{Wigner:1939cj}
  E.~P.~Wigner,
  %``On Unitary Representations of the Inhomogeneous Lorentz Group,''
  Annals Math.\  {\bf 40} (1939) 149
   [Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 6} (1989) 9].
  %%CITATION = ANMAA,40,149;%%
\bibitem{Henneaux:1997bm}
  M.~Henneaux,
  %``Consistent interactions between gauge fields: The Cohomological approach,''
  Contemp.\ Math.\  {\bf 219} (1998) 93
  [hep-th/9712226].
  %%CITATION = HEP-TH/9712226;%%
\bibitem{Ruegg:2003ps}
  H.~Ruegg and M.~Ruiz-Altaba,
  %``The Stueckelberg field,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 19} (2004) 3265
  [hep-th/0304245].
  %%CITATION = HEP-TH/0304245;%%
\bibitem{Hinterbichler:2011tt}
  K.~Hinterbichler,
  %``Theoretical Aspects of Massive Gravity,''
  Rev.\ Mod.\ Phys.\  {\bf 84} (2012) 671
  [arXiv:1105.3735 [hep-th]].
  %%CITATION = ARXIV:1105.3735;%%
\bibitem{Arnowitt:1962hi}
  R.~L.~Arnowitt, S.~Deser and C.~W.~Misner,
  %``The Dynamics of general relativity,''
  [gr-qc/0405109].
  %%CITATION = GR-QC/0405109;%%
\bibitem{Date:2010xr}
  G.~Date,
  %``Lectures on Constrained Systems,''
  arXiv:1010.2062 [gr-qc].
  %%CITATION = ARXIV:1010.2062;%%
\bibitem{Khoury:2011ay}
  J.~Khoury, G.~E.~J.~Miller and A.~J.~Tolley,
  %``Spatially Covariant Theories of a Transverse, Traceless Graviton, Part I: Formalism,''
  Phys.\ Rev.\ D {\bf 85} (2012) 084002
  [arXiv:1108.1397 [hep-th]].
  %%CITATION = ARXIV:1108.1397;%%
\bibitem{Deffayet:2012nr}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``Covariant constraints in ghost free massive gravity,''
  JCAP {\bf 1301} (2013) 032
  [arXiv:1207.6338 [hep-th]].
  %%CITATION = ARXIV:1207.6338;%%
\bibitem{Kluson:2011qe}
  J.~Kluson,
  %``Note About Hamiltonian Structure of Non-Linear Massive Gravity,''
  JHEP {\bf 1201} (2012) 013
  [arXiv:1109.3052 [hep-th]].
  %%CITATION = ARXIV:1109.3052;%%
\bibitem{Chamseddine:2011mu}
  A.~H.~Chamseddine and V.~Mukhanov,
  %``Massive Gravity Simplified: A Quadratic Action,''
  JHEP {\bf 1108} (2011) 091
  [arXiv:1106.5868 [hep-th]].
  %%CITATION = ARXIV:1106.5868;%%
\bibitem{Kluson:2011rt}
  J.~Kluson,
  %``Comments About Hamiltonian Formulation of Non-Linear Massive Gravity with Stuckelberg Fields,''
  JHEP {\bf 1206} (2012) 170
  [arXiv:1112.5267 [hep-th]].
  %%CITATION = ARXIV:1112.5267;%%
\bibitem{Kluson:2012gz}
  J.~Kluson,
  %``Remark About Hamiltonian Formulation of Non-Linear Massive Gravity in Stuckelberg Formalism,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124005
  [arXiv:1202.5899 [hep-th]].
  %%CITATION = ARXIV:1202.5899;%%  
\bibitem{Lee:1977yc}
  B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
  %``The Strength of Weak Interactions at Very High-Energies and the Higgs Boson Mass,''
  Phys.\ Rev.\ Lett.\  {\bf 38} (1977) 883.
  %%CITATION = PRLTA,38,883;%%  
\bibitem{Chanowitz:1985hj}
  M.~S.~Chanowitz and M.~K.~Gaillard,
  %``The TeV Physics of Strongly Interacting W's and Z's,''
  Nucl.\ Phys.\ B {\bf 261} (1985) 379.
  %%CITATION = NUPHA,B261,379;%%
\bibitem{Creminelli:2005qk}
  P.~Creminelli, A.~Nicolis, M.~Papucci and E.~Trincherini,
  %``Ghosts in massive gravity,''
  JHEP {\bf 0509} (2005) 003
  [hep-th/0505147].
  %%CITATION = HEP-TH/0505147;%%
\bibitem{Ondo:2013wka}
  N.~A.~Ondo and A.~J.~Tolley,
  %``Complete Decoupling Limit of Ghost-free Massive Gravity,''
  arXiv:1307.4769 [hep-th]. 
\bibitem{deRham:2011rn}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Ghost free Massive Gravity in the St\'uckelberg language,''
  Phys.\ Lett.\ B {\bf 711} (2012) 190
  [arXiv:1107.3820 [hep-th]].
  %%CITATION = ARXIV:1107.3820;%%
\bibitem{Golovnev:2011aa}
  A.~Golovnev,
  %``On the Hamiltonian analysis of non-linear massive gravity,''
  Phys.\ Lett.\ B {\bf 707} (2012) 404
  [arXiv:1112.2134 [gr-qc]].
  %%CITATION = ARXIV:1112.2134;%%
\bibitem{Buchbinder:2012wb}
  I.~L.~Buchbinder, D.~D.~Pereira and I.~L.~Shapiro,
  %``One-loop divergences in massive gravity theory,''
  Phys.\ Lett.\ B {\bf 712} (2012) 104
  [arXiv:1201.3145 [hep-th]].
  %%CITATION = ARXIV:1201.3145;%%
\bibitem{Boulanger:2000rq}
  N.~Boulanger, T.~Damour, L.~Gualtieri and M.~Henneaux,
  %``Inconsistency of interacting, multigraviton theories,''
  Nucl.\ Phys.\ B {\bf 597} (2001) 127
  [hep-th/0007220].
  %%CITATION = HEP-TH/0007220;%%  
\bibitem{Damour:2002wu}
  T.~Damour, I.~I.~Kogan and A.~Papazoglou,
  %``Nonlinear bigravity and cosmic acceleration,''
  Phys.\ Rev.\ D {\bf 66} (2002) 104025
  [hep-th/0206044].
  %%CITATION = HEP-TH/0206044;%%
\bibitem{Nibbelink:2006sz}
  S.~Nibbelink Groot, M.~Peloso and M.~Sexton,
  %``Nonlinear Properties of Vielbein Massive Gravity,''
  Eur.\ Phys.\ J.\ C {\bf 51} (2007) 741
  [hep-th/0610169].
  %%CITATION = HEP-TH/0610169;%%
\bibitem{Damour:2002ws}
  T.~Damour and I.~I.~Kogan,
  %``Effective Lagrangians and universality classes of nonlinear
  %bigravity,'' 
  Phys.\ Rev.\ D {\bf 66} (2002) 104024
  [hep-th/0206042].
  %%CITATION = HEP-TH/0206042;%%
\bibitem{Akrami:2013ffa}
  Y.~Akrami, T.~S.~Koivisto, D.~F.~Mota and M.~Sandstad,
  %``Bimetric gravity doubly coupled to matter: theory and cosmological implications,''
  arXiv:1306.0004 [hep-th].
  %%CITATION = ARXIV:1306.0004;%%
\bibitem{Baccetti:2012bk}
  V.~Baccetti, P.~Martin-Moruno and M.~Visser,
  %``Massive gravity from bimetric gravity,''
  arXiv:1205.2158 [gr-qc].
  %%CITATION = ARXIV:1205.2158;%%
\bibitem{Hinterbichler:2012cn}
  K.~Hinterbichler and R.~A.~Rosen,
  %``Interacting Spin-2 Fields,''
  JHEP {\bf 1207} (2012) 047
  [arXiv:1203.5783 [hep-th]].
  %%CITATION = ARXIV:1203.5783;%%
\bibitem{Nomura:2012xr}
  K.~Nomura and J.~Soda,
  %``When is Multimetric Gravity Ghost-free?,''
  Phys.\ Rev.\ D {\bf 86} (2012) 084052
  [arXiv:1207.3637 [hep-th]].
  %%CITATION = ARXIV:1207.3637;%%    
\bibitem{Gabadadze:2013ria}
  G.~Gabadadze, K.~Hinterbichler, D.~Pirtskhalava and Y.~Shang,
  %``On the Potential for General Relativity and its Geometry,''
  arXiv:1307.2245 [hep-th].
  %%CITATION = ARXIV:1307.2245;%%    
\bibitem{Deffayet:2012zc}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``A note on 'symmetric' vielbeins in bimetric, massive, perturbative and non perturbative gravities,''
  JHEP {\bf 1303} (2013) 086
  [arXiv:1208.4493 [gr-qc]].
  %%CITATION = ARXIV:1208.4493;%% 
\bibitem{deRham:2010tw}
  C.~de Rham, G.~Gabadadze, L.~Heisenberg and D.~Pirtskhalava,
  %``Cosmic Acceleration and the Helicity-0 Graviton,''
  Phys.\ Rev.\ D {\bf 83} (2011) 103516
  [arXiv:1010.1780 [hep-th]].
  %%CITATION = ARXIV:1010.1780;%%  
\bibitem{Gumrukcuoglu:2011ew}
  A.~E.~Gumrukcuoglu, C.~Lin and S.~Mukohyama,
  %``Open FRW universes and self-acceleration from nonlinear massive gravity,''
  JCAP {\bf 1111} (2011) 030
  [arXiv:1109.3845 [hep-th]].
  %%CITATION = ARXIV:1109.3845;%%
\bibitem{D'Amico:2011jj}
  G.~D'Amico, C.~de Rham, S.~Dubovsky, G.~Gabadadze, D.~Pirtskhalava and A.~J.~Tolley,
  %``Massive Cosmologies,''
  Phys.\ Rev.\ D {\bf 84} (2011) 124046
  [arXiv:1108.5231 [hep-th]].
  %%CITATION = ARXIV:1108.5231;%%    
\bibitem{Volkov:2011an}
  M.~S.~Volkov,
  %``Cosmological solutions with massive gravitons in the bigravity
  %theory,'' 
  JHEP {\bf 1201} (2012) 035
  [arXiv:1110.6153 [hep-th]].
  %%CITATION = ARXIV:1110.6153;%%
\bibitem{Comelli:2011zm}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``FRW Cosmology in ghost-free Massive Gravity,''
  JHEP {\bf 1203} (2012) 067
   [Erratum-ibid.\  {\bf 1206} (2012) 020]
  [arXiv:1111.1983 [hep-th]].
  %%CITATION = ARXIV:1111.1983;%%
\bibitem{Hinshaw:2012aka}
  G.~Hinshaw {\it et al.}  [WMAP Collaboration],
  %``Nine-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Parameter Results,''
  arXiv:1212.5226 [astro-ph.CO].
  %%CITATION = ARXIV:1212.5226;%% 
\bibitem{Ade:2013ktc}
  P.~A.~R.~Ade {\it et al.}  [Planck Collaboration],
  %``Planck 2013 results. I. Overview of products and scientific results,''
  arXiv:1303.5062 [astro-ph.CO].
  %%CITATION = ARXIV:1303.5062;%%  
\bibitem{Comelli:2012db}
  D.~Comelli, M.~Crisostomi and L.~Pilo,
  %``Perturbations in Massive Gravity Cosmology,''
  JHEP {\bf 1206} (2012) 085
  [arXiv:1202.1986 [hep-th]].
  %%CITATION = ARXIV:1202.1986;%%
\bibitem{Berg:2012kn}
  M.~Berg, I.~Buchberger, J.~Enander, E.~Mortsell and S.~Sjors,
  %``Growth Histories in Bimetric Massive Gravity,''
  arXiv:1206.3496 [gr-qc].
  %%CITATION = ARXIV:1206.3496;%%
\bibitem{Comelli:2011wq}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``Spherically Symmetric Solutions in Ghost-Free Massive Gravity,''
  Phys.\ Rev.\ D {\bf 85} (2012) 024044
  [arXiv:1110.4967 [hep-th]].
  %%CITATION = ARXIV:1110.4967;%%
\bibitem{Volkov:2012wp}
  M.~S.~Volkov,
  %``Hairy black holes in the ghost-free bigravity theory,''
  Phys.\ Rev.\ D {\bf 85} (2012) 124043
  [arXiv:1202.6682 [hep-th]].
  %%CITATION = ARXIV:1202.6682;%%
\bibitem{Akrami:2012vf}
  Y.~Akrami, T.~S.~Koivisto and M.~Sandstad,
  %``Accelerated expansion from ghost-free bigravity: a statistical analysis with improved generality,''
  arXiv:1209.0457 [astro-ph.CO].
  %%CITATION = ARXIV:1209.0457;%%
\bibitem{Higuchi:1986py}
  A.~Higuchi,
  %``Forbidden Mass Range For Spin-2 Field Theory In De Sitter Space-time,''
  Nucl.\ Phys.\ B {\bf 282} (1987) 397.
  %%CITATION = NUPHA,B282,397;%%
\bibitem{Deser:1983mm}
  S.~Deser and R.~I.~Nepomechie,
  %``Gauge Invariance Versus Masslessness In De Sitter Space,''
  Annals Phys.\  {\bf 154} (1984) 396.
  %%CITATION = APNYA,154,396;%%
\bibitem{Deser:2001pe}
  S.~Deser and A.~Waldron,
  %``Gauge invariances and phases of massive higher spins in (A)dS,''
  Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 031601
  [hep-th/0102166].
  %%CITATION = HEP-TH/0102166;%%
\bibitem{Deser:2001us}
  S.~Deser and A.~Waldron,
  %``Partial masslessness of higher spins in (A)dS,''
  Nucl.\ Phys.\ B {\bf 607} (2001) 577
  [hep-th/0103198].
  %%CITATION = HEP-TH/0103198;%%
\bibitem{Deser:2001wx}
  S.~Deser and A.~Waldron,
  %``Stability of massive cosmological gravitons,''
  Phys.\ Lett.\ B {\bf 508} (2001) 347
  [hep-th/0103255].
  %%CITATION = HEP-TH/0103255;%%
\bibitem{Deser:2001xr}
  S.~Deser and A.~Waldron,
  %``Null propagation of partially massless higher spins in (A)dS and cosmological constant speculations,''
  Phys.\ Lett.\ B {\bf 513} (2001) 137
  [hep-th/0105181].
  %%CITATION = HEP-TH/0105181;%%
\bibitem{Deser:2004ji}
  S.~Deser and A.~Waldron,
  %``Conformal invariance of partially massless higher spins,''
  Phys.\ Lett.\ B {\bf 603} (2004) 30
  [hep-th/0408155].
  %%CITATION = HEP-TH/0408155;%%  
\bibitem{Deser:2006zx}
  S.~Deser and A.~Waldron,
  %``Partially Massless Spin 2 Electrodynamics,''
  Phys.\ Rev.\ D {\bf 74} (2006) 084036
  [hep-th/0609113].
  %%CITATION = HEP-TH/0609113;%%
\bibitem{Higuchi:1989gz}
  A.~Higuchi,
  %``Massive Symmetric Tensor Field In Space-times With A Positive Cosmological Constant,''
  Nucl.\ Phys.\ B {\bf 325} (1989) 745.
  %%CITATION = NUPHA,B325,745;%%
\bibitem{Garidi:2003ys}
  T.~Garidi,
  %``What is mass in de Sitterian physics?,''
  hep-th/0309104.
  %%CITATION = HEP-TH/0309104;%%  
\bibitem{Zinoviev:2006im}
  Y.~.M.~Zinoviev,
  %``On massive spin 2 interactions,''
  Nucl.\ Phys.\ B {\bf 770} (2007) 83
  [hep-th/0609170].
  %%CITATION = HEP-TH/0609170;%%
\bibitem{Joung:2012rv}
  E.~Joung, L.~Lopez and M.~Taronna,
  %``On the cubic interactions of massive and partially-massless higher spins in (A)dS,''
  JHEP {\bf 1207} (2012) 041
  [arXiv:1203.6578 [hep-th]].
  %%CITATION = ARXIV:1203.6578;%%
\bibitem{deRham:2012kf}
  C.~de Rham and S.~Renaux-Petel,
  %``Massive Gravity on de Sitter and Unique Candidate for Partially
  %Massless Gravity,'' 
  arXiv:1206.3482 [hep-th].
  %%CITATION = ARXIV:1206.3482;%%
\bibitem{Deser:2013uy}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``Nonlinear Partially Massless from Massive Gravity?,''
  Phys.\  Rev.\  D 87, {\bf 101501} (R) (2013)
  [arXiv:1301.5621 [hep-th]].
  %%CITATION = ARXIV:1301.5621;%%
\bibitem{deRham:2013wv}
  C.~de Rham, K.~Hinterbichler, R.~A.~Rosen and A.~J.~Tolley,
  %``Evidence for and Obstructions to Non-Linear Partially Massless Gravity,''
  arXiv:1302.0025 [hep-th].
  %%CITATION = ARXIV:1302.0025;%%  
\bibitem{Deser:2013gpa}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``No consistent bimetric gravity?,''
  arXiv:1306.0647 [hep-th].
  %%CITATION = ARXIV:1306.0647;%%
\bibitem{Paulos:2012xe}
  M.~F.~Paulos and A.~J.~Tolley,
  %``Massive Gravity Theories and limits of Ghost-free Bigravity models,''
  arXiv:1203.4268 [hep-th].
  %%CITATION = ARXIV:1203.4268;%%
\bibitem{Sisman:2012rc}
  T.~C.~Sisman, I.~Gullu and B.~Tekin,
  %``Spectra, vacua and the unitarity of Lovelock gravity in D-dimensional AdS spacetimes,''
  Phys.\ Rev.\ D {\bf 86} (2012) 044041
  [arXiv:1204.3814 [hep-th]].
  %%CITATION = ARXIV:1204.3814;%%  
\bibitem{Stelle:1976gc}
  K.~S.~Stelle,
  %``Renormalization of Higher Derivative Quantum Gravity,''
  Phys.\ Rev.\ D {\bf 16} (1977) 953.
  %%CITATION = PHRVA,D16,953;%%
\bibitem{Stelle:1977ry}
  K.~S.~Stelle,
  %``Classical Gravity with Higher Derivatives,''
  Gen.\ Rel.\ Grav.\  {\bf 9} (1978) 353.
  %%CITATION = GRGVA,9,353;%%
\bibitem{Ostrogradski}
  M.~Ostrogradski,
  Mem.\ Ac.\ St.~Petersbourg  {\bf VI} (1850) 385. 
\bibitem{Bergshoeff:2009aq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``More on Massive 3D Gravity,''
  Phys.\ Rev.\ D {\bf 79} (2009) 124042
  [arXiv:0905.1259 [hep-th]].
  %%CITATION = ARXIV:0905.1259;%%
\bibitem{Kleinschmidt:2012rs}
  A.~Kleinschmidt, T.~Nutma and A.~Virmani,
  %``On unitary subsectors of polycritical gravities,''
  Gen.\  Rel.\  Grav.\  {\bf 45} (2013) 727
  [arXiv:1206.7095 [hep-th]].
  %%CITATION = ARXIV:1206.7095;%%
\bibitem{Gullu:2010pc}
  I.~Gullu, T.~C.~Sisman and B.~Tekin,
  %``Born-Infeld extension of new massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 27} (2010) 162001
  [arXiv:1003.3935 [hep-th]].
  %%CITATION = ARXIV:1003.3935;%%
\bibitem{Paulos:2010ke}
  M.~F.~Paulos,
  %``New massive gravity extended with an arbitrary number of curvature corrections,''
  Phys.\ Rev.\ D {\bf 82} (2010) 084042
  [arXiv:1005.1646 [hep-th]].
  %%CITATION = ARXIV:1005.1646;%%
\bibitem{Bach}
  R.~Bach,
  Math.\ Zeitschr.\ {\bf 9} (1921) 110.
  %%CITATION = GRGVA,9,353;%%  
\bibitem{Kaku:1977pa}
  M.~Kaku, P.~K.~Townsend and P.~van Nieuwenhuizen,
  %``Gauge Theory of the Conformal and Superconformal Group,''
  Phys.\ Lett.\ B {\bf 69} (1977) 304.
  %%CITATION = PHLTA,B69,304;%%
\bibitem{Deser:2012qg}
  S.~Deser, E.~Joung and A.~Waldron,
  %``Partial Masslessness and Conformal Gravity,''
  J.\ Phys.\ A (2012)
  [arXiv:1208.1307 [hep-th]].
  %%CITATION = ARXIV:1208.1307;%%
\bibitem{Fradkin:1981iu}
  E.~S.~Fradkin and A.~A.~Tseytlin,
  %``Renormalizable asymptotically free quantum theory of gravity,''
  Nucl.\ Phys.\ B {\bf 201} (1982) 469.
  %%CITATION = NUPHA,B201,469;%%  
\bibitem{Lee:1982cp}
  S.~C.~Lee and P.~van Nieuwenhuizen,
  %``Counting Of States In Higher Derivative Field Theories,''
  Phys.\ Rev.\ D {\bf 26} (1982) 934.
  %%CITATION = PHRVA,D26,934;%%
\bibitem{Riegert:1984hf}
  R.~J.~Riegert,
  %``The Particle Content Of Linearized Conformal Gravity,''
  Phys.\ Lett.\ A {\bf 105} (1984) 110.
  %%CITATION = PHLTA,A105,110;%%
\bibitem{Maldacena:2011mk}
  J.~Maldacena,
  %``Einstein Gravity from Conformal Gravity,''
  arXiv:1105.5632 [hep-th].
  %%CITATION = ARXIV:1105.5632;%%
\bibitem{Mannheim:2011ds}
  P.~D.~Mannheim,
  %``Making the Case for Conformal Gravity,''
  Found.\ Phys.\  {\bf 42} (2012) 388
  [arXiv:1101.2186 [hep-th]].
  %%CITATION = ARXIV:1101.2186;%%  
\bibitem{Bender:2007wu}
  C.~M.~Bender and P.~D.~Mannheim,
  %``No-ghost theorem for the fourth-order derivative Pais-Uhlenbeck oscillator model,''
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 110402
  [arXiv:0706.0207 [hep-th]].    
\bibitem{Volkov:2013roa}
  M.~S.~Volkov,
  %``Self-accelerating cosmologies and hairy black holes in ghost-free bigravity and massive gravity,''
  arXiv:1304.0238 [hep-th].
  %%CITATION = ARXIV:1304.0238;%% 
\bibitem{Sjors:2011iv}
  S.~Sjors and E.~Mortsell,
  %``Spherically Symmetric Solutions in Massive Gravity and Constraints from Galaxies,''
  JHEP {\bf 1302} (2013) 080
  [arXiv:1111.5961 [gr-qc]].
  %%CITATION = ARXIV:1111.5961;%%
\bibitem{Enander:2013kza}
  J.~Enander and E.~Mortsell,
  %``Strong lensing constraints on bimetric massive gravity,''
  arXiv:1306.1086 [astro-ph.CO].
  %%CITATION = ARXIV:1306.1086;%%   
\bibitem{Brito:2013yxa}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Partially massless gravitons do not destroy general relativity black holes,''
  Phys.\  Rev.\ D {\bf 87} (2013) 124024
  [arXiv:1306.0908 [gr-qc]].
  %%CITATION = ARXIV:1306.0908;%%   
\bibitem{Gregory:1993vy}
  R.~Gregory and R.~Laflamme,
  %``Black strings and p-branes are unstable,''
  Phys.\ Rev.\ Lett.\  {\bf 70} (1993) 2837
  [hep-th/9301052].
  %%CITATION = HEP-TH/9301052;%% 
\bibitem{Babichev:2013una}
  E.~Babichev and A.~Fabbri,
  %``Instability of black holes in massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 30} (2013) 152001
  [arXiv:1304.5992 [gr-qc]].
  %%CITATION = ARXIV:1304.5992;%%
\bibitem{Brito:2013wya}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Massive spin-2 fields on black hole spacetimes: Instability of the Schwarzschild and Kerr solutions and bounds on the graviton mass,''
  Phys.\  Rev.\ D {\bf 88} (2013) 023514
  [arXiv:1304.6725 [gr-qc]].
  %%CITATION = ARXIV:1304.6725;%% 
\bibitem{Hinterbichler:2013eza}
  K.~Hinterbichler,
  %``Ghost-Free Derivative Interactions for a Massive Graviton,''
  arXiv:1305.7227 [hep-th].
  %%CITATION = ARXIV:1305.7227;%%      
\bibitem{Huang:2012pe}
  Q.~-G.~Huang, Y.~-S.~Piao and S.~-Y.~Zhou,
  %``Mass-Varying Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124014
  [arXiv:1206.5678 [hep-th]].
  %%CITATION = ARXIV:1206.5678;%% 
\bibitem{Huang:2013mha}
  Q.~-G.~Huang, K.~-C.~Zhang and S.~-Y.~Zhou,
  %``Generalized massive gravity in arbitrary dimensions and its Hamiltonian formulation,''
  arXiv:1306.4740 [hep-th].
  %%CITATION = ARXIV:1306.4740;%%   
\bibitem{Gabadadze:2012tr}
  G.~Gabadadze, K.~Hinterbichler, J.~Khoury, D.~Pirtskhalava and M.~Trodden,
  %``A Covariant Master Theory for Novel Galilean Invariant Models and Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124004
  [arXiv:1208.5773 [hep-th]].
  %%CITATION = ARXIV:1208.5773;%%
\bibitem{D'Amico:2012zv}
  G.~D'Amico, G.~Gabadadze, L.~Hui and D.~Pirtskhalava,
  %``Quasi-Dilaton: Theory and Cosmology,''
  arXiv:1206.4253 [hep-th].
  %%CITATION = ARXIV:1206.4253;%%   
%\cite{Ondo:2013wka}
\bibitem{Cai:2013lqa}
  Y.~-F.~Cai, F.~Duplessis and E.~N.~Saridakis,
  %``$F(R)$ nonlinear massive gravity and cosmological implications,''
  arXiv:1307.7150 [hep-th].
  %%CITATION = ARXIV:1307.7150;%%  
\bibitem{Nojiri:2013zza}
  S.~'I.~Nojiri and S.~D.~Odintsov,
  %``Accelerating cosmology in modified gravity: from convenient $F(R)$ or string-inspired theory to bimetric $F(R)$ gravity,''
  arXiv:1306.4426 [gr-qc].
  %%CITATION = ARXIV:1306.4426;%% 
\bibitem{deRham:2013qqa}
  C.~de Rham, L.~Heisenberg and R.~H.~Ribeiro,
  %``Quantum Corrections in Massive Gravity,''
  arXiv:1307.7169 [hep-th].
  %%CITATION = ARXIV:1307.7169;%% 
\bibitem{Wald:1984rg}
  R.~M.~Wald,
  %``General Relativity,''
  Chicago, Usa: Univ. Pr. ( 1984) 491p.  
  
  

\end{thebibliography}


    
    

    
    
    
    

        
        
        
    




==> Bibliography/OrderReferences/all-new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Introduction}
\label{intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





Since its introduction in 1916~\cite{Einstein:1916vd}, Einstein's theory of General Relativity (GR) has successfully explained the majority of gravity-related phenomena. It reproduces Newtonian dynamics in the weak-gravity limit, makes observable predictions, such as the bending of light by massive objects, and until today it withstands solar system tests to a very high precision. At the same time, containing the scalar curvature of a metric tensor, the Einstein-Hilbert action for GR offers an intuitive geometrical interpretation of the theory and Einstein's field equations can be regarded as capturing the interplay between matter and space-time geometry. 

On scales larger than the solar system, however, astrophysical observations have posed questions that to a large extend remain unanswered in the context of GR. These enigmas include the cosmological constant problem, which we will explain in more detail below, as well as the nature of dark matter. 
While there exists a large variety of promising candidates for dark matter particles in various extensions of the Standard Model of Particle Physics, so far there is no convincing explanation for the smallness of the observed cosmological constant. Unless they eventually both turn out to be resolved on the particle physics side, the severeness of the phenomenological problems challenges GR as the ultimate and complete theory of gravity. Therefore, it is reasonable to investigate the possibility of modifying Einstein's beautiful theory with the goal to provide explanations for the perplexing astrophysical observations. 

Of course, such a modification of the theory of gravity is already heavily constrained from the observational side since it must not alter the well-tested predictions of GR at solar-system scales.  
From a more theoretical perpective, looking for alternatives beyond GR is also motivated by String Theory, the most promising candidate for a quantum theory of gravity. GR itself cannot be promoted into a renormalizable quantum theory; it can at most be an effective theory that requires an ultraviolet (UV) completion. 
String Theory in the UV predicts an effective action at low energies that includes the Einstein-Hilbert term of GR plus higher-curvature corrections, as well as couplings to many fields of different spin. Computing this effective action explicitly in string perturbation theory is tedious but, alternatively, one can choose to search for consistent effective theories in a bottom-up approach. 
Following this strategy reveals that modifying GR is surprisingly difficult; almost any alteration of the Einstein-Hilbert action leads to inconsistencies in the theory. Moreover, the nonlinearities of GR often complicate consistency analyses of suggested modified theories and it happens rather rarely that a modification is proven to be consistent. Finding an alternative theory of gravity without inconsistencies is therefore always an important achievement and it is worth investigating the new theory in detail.

As a field theory, GR describes nonlinear self-interactions of a massless spin-2 excitation. A logical first guess for a modification of this setup would be the addition of a mass term for the spin-2 field. The resulting theory should describe nonlinear interactions of a massive spin-2 field and is commonly referred to as \textit{Massive Gravity}. However, the problem with a massive graviton is that a generic mass term introduces ghosts into the physical spectrum. Ghosts correspond to fields with negative kinetic energy that lead to instabilities at the classical and nonunitarity at the quantum level. In a consistent theory, it is necessary to avoid the presence of ghost-fields which puts severe constraints on the mass term and interaction potential of the spin-2 field.

To summarize, the search for a consistent theory of an interacting massive spin-2 field is motivated by the following question:
\begin{itemize}
\item[] Can a massive graviton explain unresolved puzzles in cosmology? 
\end{itemize}
But due to the difficulty of consistently modifying GR, before we can address this question, we need to answer an even more fundamental one:
\begin{itemize}
\item[] How can we describe massive spin-2 particles in field theory?
\end{itemize}
Even without a cosmological constant or Dark Matter problem, this task is interesting from a purely theoretical point of view: It is well-known how to describe massless and massive particles with spin $<2$ in field theory, and there is no obvious reason why there should not exist a corresponding model for spin 2.

Discussing consistency proofs and special features of recently discovered nonlinear theories for massive spin-2 fields, this thesis is mostly devoted to the latter of the two problems, although basic applications to cosmology are also provided. Before diving into this engrossing new subject we present the history of Massive Gravity, explain the cosmological constant problem and provide the basics of theories with spin-2 fields in the remainder of the introduction.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Historical development}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Finding a consistent theory that describes a massive spin-2 field is an old problem. In the year 1939, Fierz and Pauli wrote down the unique ghost-free mass term for a linearized spin-2 fluctuation~\cite{Fierz:1939ix}. An a priori arbitrary coefficient in the mass term needs to be tuned to a specific value in order to remove inconsistencies. 
About 30 years later, in two independent articles, van Dam and Veltman as well as Zakharov discovered that in the zero-mass limit the Fierz-Pauli theory coupled to sources does not converge to the massless theory~\cite{vanDam:1970vg, Zakharov:1970cc}. Namely, the helicity-zero mode of the massive spin-2 field does not decouple in this limit but gives an additional contribution to the vacuum amplitude of two interacting sources. Therefore, this \textit{vDVZ discontinuity} implies that even a very small graviton mass has significant impact on gravitational interactions between sources. In particular, in the zero-mass limit, GR augmented by the Fierz-Pauli term predicts different gravitational constants for conformal and non-conformal matter. Such a difference would be observable in measurements of the gravitational constant for light bending, whose value in the Fierz-Pauli theory with infinitely small mass differs by 25$\%$ from the one predicted by GR. Observations clearly rule out this possibility and a massive graviton would have been discarded decades ago had Vainshtein not found his famous loophole which suggested that a nonlinear completion of the Fierz-Pauli theory could avoid the vDVZ discontinuity~\cite{Vainshtein:1972sx}. Vainshtein showed that around massive sources the linear approximation loses its validity below a certain distance scale. This \textit{Vainshtein radius} becomes infinitely large in the limit of zero Fierz-Pauli mass and in this case there is no regime where the linear theory is valid. Clearly, such a \textit{Vainshtein mechanism} requires a nonlinear extension of the Fierz-Pauli mass term which, not unexpectedly, generically reintroduces inconsistencies. In fact, already in 1972, Boulware and Deser claimed that any nonlinear completion of Fierz-Pauli theory would exhibit a ghost instability~\cite{Boulware:1972zf, Boulware:1973my}. Their results were trusted and for almost 40 years there was little progress in the field of Massive Gravity. Moreover, in 2005, an analysis by Creminelli et.~al.~that was based on earlier work by Arkani-Hamed et.~al.~\cite{ArkaniHamed:2002sp} seemingly confirmed the unavoidable presence of the Boulware-Deser ghost in any nonlinear extension of the Fierz-Pauli theory.

The peripeteia came in 2010, when de Rham, Gabadadze and Tolley (dRGT) revisited the analysis of Creminelli et.~al.~and discovered a minor sign mistake which unfortunately had a large impact on the paper's final conclusion \cite{deRham:2010ik, deRham:2010kj}. After correcting the sign, they found that it is possible to construct a theory of nonlinear Massive Gravity which is ghost-free in a certain decoupling limit. This alone did not guarantee the consistency of the full theory away from the decoupling limit but, in the following year, their reformulation of the dRGT theory~\cite{Hassan:2011vm} enabled Hassan and Rosen to prove the absence of the Boulware-Deser ghost in a Hamiltonian constraint analysis~\cite{Hassan:2011hr, Hassan:2011ea}. Furthermore, they generalized the dRGT setup, which describes a nonlinearly interacting massive spin-2 field in flat space, to a ghost-free bimetric theory containing nonlinear interactions of a massless and massive spin-2 field in a dynamical background~\cite{Hassan:2011zd}. These works established the first consistent nonlinear theory for massive spin-2 fields. 

%The discovery of a consistent nonlinear theory for massive spin-2 fields opened up a new research area. Of particular interest were classical solutions within the dRGT and the Hassan-Rosen model~\cite{} as well as perturbations around them~\cite{}.

Inconsistent models with bimetric interactions had been considered earlier in the literature, for the first time by Rosen in 1940~\cite{Rosen:1940zz,Rosen:1975kk} and later by Aragone and Deser~\cite{Aragone:1971kh} as well as Isham, Salaam and Strathdee~\cite{Isham:1971gm}. The consistent bimetric model had actually already appeared in \cite{Chamseddine:1978yu} where, however, the ghost issue was not addressed.
Besides these, alternative theories with massive gravitons have also been under investigation. These include the DGP model~\cite{Dvali:2000rv,Dvali:2000hr}, Kaluza-Klein scenarios~\cite{Kaluza:1921tu, Klein:1926tv}, New Massive Gravity~\cite{Bergshoeff:2009hq}, Topological Massive Gravity~\cite{Deser:1981wh,Deser:1982vy} and Lorentz violating models~\cite{ArkaniHamed:2003uy}.











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The cosmological constant problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Einstein's equations, the equations of motion for the metric tensor $\gmn$ that follow from the Einstein-Hilbert action of General Relativity, are of the form
\beqn\label{ee}
R_{\mu\nu}-\frac{1}{2}R\,\gmn=\frac{1}{M_{\mathrm{Pl}}^{2}}T_{\mu\nu}-\Lambda\gmn\,.
\eeqn 
The left-hand side contains the Ricci curvature tensor and scalar of $\gmn$ and hence describes the dynamics of space-time geometry. The right-hand side consists of matter sources with stress energy tensor $T_{\mu\nu}$ to which we have added a cosmological constant term. 

In the absence of local sources, there is still a contribution from the matter sector to Einstein's equations because quantum field theory predicts a vacuum expectation value $\braket{T_{\mu\nu}}$ for the source. In particular, the component $\braket{T_{00}}$ is the vacuum energy density that includes contributions from normal ordering of operators in the Hamiltonian and from expectation values of scalar potentials after symmetry breaking. The size of these contributions depends on the specific model, its symmetry breaking mechanisms and UV cutoff, but generically it certainly satisfies $\braket{T_{00}}>(1\,\text{TeV})^4$. In the worst case, it is as large as the Planck density, $\braket{T_{00}}\sim (10^{18}\text{GeV})^4$. As we will review in chapter~\ref{ch:cosmo}, such a huge value for the vacuum energy density would make the expansion of the universe accelerate at an immense rate. Although in the late 1990's observational data revealed that the cosmological expansion is indeed accelerating~\cite{Riess:1998cb, Perlmutter:1998np}, the vacuum energy density driving this acceleration must be as tiny as $10^{-47}(\text{GeV})^4$. The theoretical prediction and the observed value therefore differ by 60 to 120 orders of magnitude. 

In principle, there is a way to cure the discrepancy by hand: One could simply adjust the free parameter $\Lambda$ in (\ref{ee}) such that it cancels the large number in $\braket{T_{00}}$ up to 60-120 decimal places. Obviously this method of dealing with the difference in observed and measured vacuum energies requires an enormous amount of fine-tuning. Although there is no mathematical inconsistency in this procedure, the inexplicable almost exact cancellation is a thorn in the flesh of most theoretical physicists. 
The \textit{cosmological constant problem} has become one of the greatest challenges of modern theoretical physics and there is a countless number of proposals for solutions in the literature. For a recent review we refer the reader to~\cite{Martin:2012bt}.  


A priori, there is good reason to believe that a theory of Massive Gravity could be a step towards explaining the smallness of the observed vacuum energy. 
The main idea is that a small graviton mass is protected against quantum corrections, which relies on the appearance of a gauge symmetry (namely diffeomorphism invariance) in the zero-mass limit. Contrarily, when the cosmological constant is taken to zero, no such symmetry emerges and hence the value for the vacuum energy is unprotected. A tiny graviton mass is therefore considered less unnatural than a cosmological constant of the same scale. The smallness of the mass parameter would still have to be explained, but once it is small at the classical level, quantum corrections will be of the same order of magnitude and not drive it to the cut-off scale. 
If now, in a Massive Gravity theory, a large vacuum energy $\braket{T_{00}}$ generated on the matter side is somehow ``screened" by a mass term with a small graviton mass in the modified Einstein equations, the effect of the vacuum energy on the acceleration of the cosmological expansion could be small. Despite these promising ideas, it seems that a straightforward screening mechnanism does not exist in the dRGT and Hassan-Rosen models to be considered in this thesis. However, this question is not yet finally settled and, moreover, there appear to exist other interesting possibilities to address the cosmological constant problem. 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Massless and massive field theories}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The modern description of particle physics is based on the extremely successful framework of quantum field theory (QFT). Quantum states that correspond to physical particles are created and annihilated by local operators, or quantum fields, that transform in irreducible unitary representations of the Poincar\'e group which, in turn, characterizes the isometries of the underlying Minkowski space time. According to Wigner's classification~\cite{Wigner:1939cj}, the irreducible unitary representations with non-negative energy can be labelled by two Casimir invariants related to mass and spin (or helicity) of the corresponding particle. 
%It is furthermore important to distinguish between the massless and massive case which correspond to different little groups that leave the particle's four-momentum invariant.  

The construction of a QFT with a Hilbert space of particle states is usually achieved in two steps:  
One begins by writing down a Lagrangian of a consistent classical field theory for which the Hamiltonian is bounded from below. Then one quantizes the theory either in the path integral formalism or by imposing canonical (anti)commutation relations for the fields. The process of quantization can in principle reintroduce inconsistencies that render the theory nonunitary but, if one is lucky, it is possible to avoid these. Then, in the absence of gauge anomalies, there may exist a consistent quantum version of the classical theory. The crucial point is that for the existence of a unitary description of particles in a QFT framework, it is absolutely necessary to start from a classically consistent field theory. 

Apart from the problem of nonunitarity in its quantum version, a classical field theory with a Hamiltonian that is not bounded from below is not even meaningful on its own. The instability allows the field to transfer an infinite amount of energy to other fields it interacts with and hence the theory cannot make any useful predictions. Thus, a Hamiltonian that is bounded from below is required from any feasible field theory (classical or quantum). In particular, one must demand the absence of fields that have wrong signs in front of their mass terms (\textit{tachyons}) or kinetic terms (\textit{ghosts}).  

Consistent classical theories for both massless and massive fields with spin 0, 1/2 and 1 are well-known\footnote{Note also that a consistent classical theory for a massive/massless gravitino with spin 3/2 exists in the form of broken/unbroken supergravity.} and their quantum versions play an important role in theoretical particle physics. In fact, the Standard Model of Particle Physics is a consistent quantum theory of fields with spin~1/2 (fermions), spin~1 (gauge bosons) and spin~0 (Higgs boson). Table~\ref{fttable} displays the structure of Lagrangians for fields of different spin.

\begin{table}[htdp]
\caption{Lagrangians for fields of different spin. The massless theories correspond to setting $m=0$.}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline && \\
spin 0& scalar field $\phi$ & $\mathcal{L}_\phi=-\partial_\mu\phi\partial^\mu\phi-m^2\phi^2$
 \\ &&\\
\hline && \\
spin $\tfrac{1}{2}$&  spinor field $\psi^\alpha$ & $\mathcal{L}_\psi=-\bar{\psi}\gamma^\mu\partial_\mu\psi-m\bar{\psi}\psi$ \\ &&\\
\hline &&\\
spin 1& vector field $A_\mu$& $\mathcal{L}_A=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-\frac{m^2}{2}A^\mu A_\mu$ \\ &&\\
\hline 
\end{tabular}
\end{center}
\label{fttable}
\end{table}%

Compared to its lower-spin companions, spin-2 fields turn out to be much more difficult to handle. The consistent classical theory for a massless spin-2 particle with nonlinear self-interactions is General Relativity. However, when trying to quantize the theory one faces another problem because the Lagrangian for GR is nonrenormalizable. This means that predictions for scattering cross sections contain infinities that cannot be absorbed into perturbatively renormalized coupling constants. Due to this obstruction, GR makes sense only as an effective field theory valid at low energies which is believed to have a consistent, renormalizable completion in the ultraviolet regime. For massive spin-2 fields the situation is even worse: Adding a mass term to the Einstein-Hilbert action of GR generically introduces ghost instabilities that render the theory inconsistent already at the classical level. 

In the following we discuss classical field theories of massless and massive spin-1 and spin-2 particles in more detail. In particular we review the degree-of-freedom counting in these theories using gauge invariances and constraints in the equations of motion. 

















%%%%%%%%%%%%%%%%%%%%%
\subsection{Spin-1}
%%%%%%%%%%%%%%%%%%%%%

Before coming to the more relevant example of linear spin-2 theories, it is instructive to begin by considering spin-1 fields that share several features with their spin-2 analogues. Unlike in the theories for spin-0 and spin-1/2 fields, gauge invariance is needed in the massless case to obtain the correct number of propagating degrees of freedom.
We first discuss the massless vector field that appears in classical electrodynamics and then present the Proca theory for massive spin-1 fields.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Massless theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The theory for a massless spin-1 field $A_\mu(x)$ in flat space is given by Maxwell's Lagrangian,
\beqn
\mathcal{L}_\mathrm{Maxwell}=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-J^\mu A_\mu\,,\qquad F_{\mu\nu}\equiv \partial_\mu A_\nu-\partial_\nu A_\mu\,,
\eeqn
where $J^\mu$ is an external source and indices are contracted with the Minkowski metric $\emn$. 
The equations of motion obtained from varying with respect to $A_\nu$ are
\beqn
\partial^\mu F_{\mu\nu}=J_\nu\,.
\eeqn
Due the identity $\partial^\nu\partial^\mu F_{\mu\nu}=0$, the divergence of the equations implies that the source must be conserved, $\partial^\mu J_\mu=0$.
With the help of this conservation law\footnote{In general, the source is not necessarily conserved off-shell since its conservation is an on-shell constraint. For a Lagrangian with off-shell gauge-invariance we need to require off-shell conservation of $J_\mu$ or, equivalently, off-shell gauge-invariance of the source term $J^\mu A_\mu$.} it can be shown that both the above Lagrangian and the equations are invariant under a U(1) gauge transformation,
\beqn\label{gtso}
A_\mu(x)\longrightarrow A_\mu(x)+\partial_\mu\phi(x)\,,
\eeqn
where $\phi(x)$ is a scalar gauge parameter. The symmetry transformation may be used to choose the Lorenz gauge which is defined through the condition $\partial^\mu A_\mu=0$.
In this gauge the equations of motion reduce to 
\beqn
\Box A_\mu=J_\mu\,,
\eeqn
which is simply a sourced Klein-Gordon equation for a massless field.
However, the gauge is not yet fixed completely because we can still perform gauge transformations~(\ref{gtso}) with $\Box\phi=0$ that do not take us out of the Lorenz gauge. The gauge condition $\partial^\mu A_\mu=0$ together with this residual gauge transformation remove two degrees of freedom from $A_\mu$. In~$d$ dimensions the theory for a massless spin-1 particle therefore propagates $d-2$ degrees of freedom.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Massive theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, let us turn to the massive spin-1 particle. It is described by the Proca Lagrangian,
\beqn
\mathcal{L}_\mathrm{Proca}=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-\frac{m^2}{2}A^\mu A_\mu-J^\mu A_\mu\,.
\eeqn
Clearly, this is the same as Maxwell's Lagrangian with an additional mass term quadratic in the field.
The equations of motion in the Proca theory read 
\beqn
\partial^\mu F_{\mu\nu}-m^2A_\nu=J_\nu\,.
\eeqn
The mass term breaks the above U(1) symmetry and the Lagrangian is no longer gauge invariant. Hence, this time there is no symmetry that can be used to remove redundant components of the field.
On the other hand, taking the divergence of the equations of motion we now obtain a constraint equation that contains the field,
\beqn\label{constAmu}
\partial^\mu A_\mu=-\frac{1}{m^2}\partial^\mu J_\mu\,.
\eeqn
The source is no longer necessarily conserved but, if we anyway assume $\partial^\mu J_\mu=0$, then the constraint corresponds precisely to the above Lorenz gauge condition. Plugging it back into the equations of motion we obtain (for a conserved source)
\beqn
(\Box-m^2)A_\mu=J_\mu\,.
\eeqn
Thus the massive spin-1 field again satisfies a sourced Klein-Gordon equation. Since one degree of freedom is removed by the constraint, the theory has $d-1$ propagating degrees of freedom.

 








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Spin-2}\label{sec:FP}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Now we are ready to perform the degree-of-freedom counting in the linear spin-2 theory. Once more, we begin with the massless case before turning to the massive Fierz-Pauli theory. Eventually, we draw the connection between the linear massless theory and nonlinear General Relativity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear massless theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The Lagrangian for a massless spin-2 field in flat space to quadratic order in the field reads
\beqn\label{masslesslin}
\mathcal{L}_\mathrm{lin}=h^{\mu\nu}\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}-\kappa h^{\mu\nu} T_{\mu\nu}\,,
\eeqn
where $T^{\mu\nu}$ is an external source and the structure of the kinetic terms is captured by the two-derivative operator,
\begin{align}\label{kinstruc1}
	\mathcal{E}_{\mu\nu}^{\phantom\mu\phantom\nu\rho\sigma} = \tfrac{1}{2}\Big(
	\eta_\mu^{\phantom\mu\rho}\eta_\nu^{\phantom\nu\sigma}\Box
	&-\eta_\nu^{\phantom\nu\sigma}\partial_\mu\partial^\rho
	-\eta_\mu^{\phantom\mu\sigma}\partial_\nu\partial^\rho\nn\\
	&+\eta_{\mu\nu} \partial^\sigma\partial^\rho
	+\eta^{\rho\sigma}\partial_\mu\partial_\nu
	-\eta^{\rho\sigma}\eta_{\mu\nu}\Box\Big)
	\,. 
\end{align}
The corresponding equations of motion are 
\beqn
\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}=\frac{\kappa}{2} T_{\mu\nu}\,.
\eeqn
The linear Bianchi identity, $\partial^\mu \mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}=0$, implies conservation of the source, $\partial^\mu T_{\mu\nu}=0$. Using this it can easily be verified that the Lagrangian and equations for the massless spin-2 particle are invariant under the following gauge transformations,
\beqn\label{lindiff}
\hmn(x)\longrightarrow \hmn(x) + \partial_\mu\xi_\nu(x)+\partial_\nu\xi_\mu(x)\,,
\eeqn
with vector gauge parameter $\xi_\mu(x)$. As in the spin-1 case, we can use this symmetry to pick a convenient gauge. The Lorenz gauge condition for the spin-2 field is $\partial^\mu\hmn-\frac{1}{2}\partial_\nu h=0$, and, in this gauge, the equations of motion can be written as
\beqn
\Box\hmn=\kappa T_{\mu\nu}-\frac{\kappa}{d-2}T\,.
\eeqn
Again, there exist residual gauge transformations, namely those with $\Box\xi_\mu=0$, that leave the Lorenz gauge intact and correspond to further redundant degrees of freedom.
In total, gauge invariance therefore removes $2d$ of the $d(d+1)/2$ components in $\hmn$, and the only propagating modes are the $d(d-3)/2$ degrees of freedom of a massless spin-2 particle.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear massive theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As has been known since the work of Fierz and Pauli from 1939~\cite{Fierz:1939ix}, the quadratic Lagrangian for a massive spin-2 particle in flat space has the form
\beqn\label{FPlag}
\mathcal{L}_\mathrm{FP}=h^{\mu\nu}\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}-\frac{m_\mathrm{FP}^2}{2}(h^{\mu\nu}\hmn-h^2)-\kappa h^{\mu\nu} T_{\mu\nu}\,,
\eeqn
where the kinetic operator is the same as in the massless case, given by (\ref{kinstruc1}).
The equations of motion obtained from the Lagrangian for the massive particle are
\beqn
\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}-\frac{m_\mathrm{FP}^2}{2}(\hmn-\emn h)=\frac{\kappa}{2} T_{\mu\nu}\,.
\eeqn
The mass term breaks the gauge invariance of the massless theory but, as a consequence of the linearized Bianchi identity, the divergence and trace of these equations give rise to $d+1$ constraints,
\beqn\label{twoconstr}
\partial^\mu \hmn-\partial_\nu h&=&-\frac{\kappa}{m_\mathrm{FP}^2}\partial_\mu T^{\mu\nu}\,,\nn\\
h&=&\frac{1}{d-1}\frac{\kappa}{m_\mathrm{FP}^2}T+\frac{d-2}{d-1}\frac{\kappa}{m_\mathrm{FP}^4}\partial^\nu\partial^\mu T_{\mu\nu}\,.
\eeqn
The source is not necessarily conserved but we shall anyway assume $\partial_\mu T^{\mu\nu}=0$.
Then, unlike in the spin-1 example, the constraint equation obtained from taking the divergence of the equations of motion does not resemble the Lorenz gauge condition but differs by a factor of $1/2$ in front of the trace. For vanishing sources, the constraints imply that the massive spin-2 field is transverse and traceless. 

Using (\ref{twoconstr}) in the equations of motion, we arrive at
\beqn
(\Box-m_\mathrm{FP}^2)\hmn=\kappa\left(T_{\mu\nu}-\frac{1}{d-1}\left[\eta_{\mu\nu}-\frac{1}{m_\mathrm{FP}^2}\partial_\mu\partial_\nu T\right]\right) \,.
\eeqn
Therefore the massive spin-2 field also satisfies a sourced Klein-Gordon equation.
The constraints (\ref{twoconstr}) remove $d+1$ of the $d(d+1)/2$ components in $\hmn$, leaving us with the $d(d-1)/2-1$ propagating degrees of freedom of a massive spin-2 particle. 

An important observation is that modifying the structure of the mass term, i.e.~changing the numerical factor in front of $h^2$ in (\ref{FPlag}), introduces an additional degree of freedom into the theory. This happens because the trace constraint in (\ref{twoconstr}) is lost and $h$ satisfies a dynamical equation of motion instead. It can also be shown that the propagator corresponding to the extra degree of freedom comes with a residue of the wrong sign and therefore gives rise to a ghost instability. This unwanted dynamical field is referred to as the \textit{Boulware-Deser-ghost}. It is this ghost mode that complicates the construction of a nonlinear interaction potential for a spin-2 field because, even when banned from the linear theory, the ghost notoriously reappears through the higher-order interactions.

On the other hand, tuning the linear mass potential to the Fierz-Pauli structure comes with its own problems that threaten the phenomenological viability of the theory as a modification of general relativity. Namely, as already mentioned, it was shown by van Dam, Veltman and Zakharov (vDVZ) \cite{vanDam:1970vg, Zakharov:1970cc} that the $m_\mathrm{FP}\rightarrow 0$ limit of linear massive gravity is discontinuous. More precisely, the helicity-zero mode does not decouple from the sources in this limit and gives an extra contribution to the gravitational force for matter sources whose stress-energy tensors has nonvanishing trace. This leads to a substantial difference between the interactions of massive objects and massless particles, such as photons. This difference can be tested, for instance, by observing light bending by heavy objects. Such tests clearly rule out the existence of a vDVZ discontinuity.

Fortunately, it has been demonstrated by Vainshtein in that nonlinear self-interaction for the spin-2 field may be able to cure this problem~\cite{Vainshtein:1972sx}: The nonlinear theory becomes strongly coupled and the linear approximation breaks down at disctance scales smaller than the \textit{Vainshtein radius}. This radius is large for small $m_\mathrm{FP}$ and goes to infinity in the zero-mass limit. If it is large enough then, although beyond it the linear theory is valid, the vDVZ discontinuity cannot be observed.  
The existence of such a \textit{Vainshtein mechanism} requires a nonlinear completion of the Fierz-Pauli mass term which is one of the main motivations for the construction of a nonlinear theory of Massive Gravity.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Nonlinear massless theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To conclude the introduction, we outline the relation between the linear theory for massless spin-2 fields discussed above and Einstein's General Relativity.
The graviton in GR is a massless spin-2 particle and should hence be described by the Lagrangian~(\ref{masslesslin}). However, the equivalence principle tells us that the field should couple to all kinds of energy in the same manner, including its own stress-energy tensor. Implementing this requirement in~(\ref{masslesslin}) iteratively introduces nonlinearities and eventually leads to the Einstein-Hilbert action for GR.
In turn, the quadratic Lagrangian for a massless spin-2 particle follows from linearizing the Einstein-Hilbert action,
\beqn\label{EHGR}
S_{\mathrm{GR}}=M_{\mathrm{Pl}}^{d-2}\int \mathrm{d}^dx\,\sqrt{-g}~R ~+ \int \mathrm{d}^dx\,\sqrt{-g}~\mathcal{L}_\mathrm{m} \,,
\eeqn
in the perturbation $\hmn=\kappa^{-1}(\gmn-\emn)$ with $\kappa=M^{(2-d)/2}_{\mathrm{Pl}}$. The source is related to the matter Lagrangian~$\mathcal{L}_\mathrm{m}$ through the definition of the stress-energy tensor,
\beqn
T_{\mu\nu}\equiv-\frac{1}{\sqrt{-g}}\frac{\partial(\sqrt{-g}\,\mathcal{L}_\mathrm{m})}{\partial g^{\mu\nu}}\,.
\eeqn
The Einstein-Hilbert action is the gauge invariant nonlinear extension\footnote{One can also include self-interactions into the theory for the massless spin-1 field considered above. In order for the field to remain massless, these interactions must respect gauge invariance and this requirement leads to the structure of Yang-Mills theories~\cite{Henneaux:1997bm}. In the quantum theory, giving mass to non-Abelian spin-1 fields in a unitary and renormalizable way requires a Higgs mechanism, see e.g.~\cite{Ruegg:2003ps}.} of~(\ref{masslesslin}). It can be defined uniquely, as the field theory that describes nonlinear self-interactions of a massless spin-2 particle \cite{Hinterbichler:2011tt}. The gauge transformations~(\ref{lindiff}) are linearized general coordinate transformations (GCTs), under which the metric at the nonlinear level transforms as
\beqn
\gmn\longrightarrow\gmn+\nabla_\mu\xi_\nu+\nabla_\nu\xi_\mu\,.
\eeqn
The presence of a gauge symmetry at the nonlinear level ensures that the full theory propagates the same number of degrees of freedom as its linear version.

Naturally, the existence of a nonlinear closed form for the kinetic terms of a spin-2 particle motivates the search for a nonlinear completion of the Fierz-Pauli mass term. As we saw above, consistency of linearized Massive Gravity requires tuning of a coefficient in the mass potential. One can therefore expect that a consistent (i.e.~ghost-free) nonlinear potential cannot contain arbitrary interaction terms, but that the coefficients of certain terms will be related to each other by demanding the absence of the extra degree of freedom. We shall see in the next chapter that this is precisely what happens. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\chapter{Consistent Nonlinear Massive Gravity}
\label{ch:MG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

In this chapter we introduce the recently discovered consistent theory of nonlinear Massive Gravity. Its nonlinear interaction potential is the unique ghost-free completion of the Fierz-Pauli mass term and contains $(d-2)$ independent parameters in $d$ dimensions. Proving the consistency of the theory in two different formulations was the purpose of {\protect{\hyperref[papI]{Paper~I}}} and~{\protect{\hyperref[papIII]{III}}}.

We begin the discussion by pointing out some general features of nonlinear spin-2 interactions, emphasizing the necessity of a second rank-2 tensor in the theory.
Afterwards, we use insights from the Hamiltonian formulation of General Relativity to construct the ghost-free nonlinear mass potential. 
The resulting Massive Gravity action is the model constructed by de Rham, Gabadadze and Tolley (dRGT) in \cite{deRham:2010ik, deRham:2010kj}, generalized to arbitrary backgrounds. 
The interaction term manifestly breaks diffeomorphism invariance which can be restored using St\"uckelberg fields. The consistency proof in the gauge invariant formulation of nonlinear Massive Gravity is subject of the second half of this chapter.



  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\section{Construction of the ghost-free nonlinear theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 This section is devoted to the construction of the dRGT model for nonlinear Massive Gravity~\cite{deRham:2010ik, deRham:2010kj} as well as its generalization to arbitrary backgrounds by Hassan and Rosen~\cite{Hassan:2011vm}.
  The constructive consistency proof presented here is neither part of any of the papers accompanying the thesis nor has it appeared anywhere else in the literature. Nevertheless, it constitutes the most efficient and straightforward way to arrive at the consistent theory. 
Before we come to the proof, it is worthwile to make a few remarks on general properties of spin-2 interaction potentials.
 
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{General remarks on nonlinear interactions}\label{sec:nonlin}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the introduction we considered massless and massive theories for a linear fluctuation $\hmn$ in a fixed Minkowski background $\emn$. In the nonlinear massless theory given by the Einstein-Hilbert action of GR, it was possible to combine the background and the fluctuation into a single field $\gmn$. We would now like to do something similar in the massive case.

What we call a mass term for a rank-2 tensor $\gmn$ must be a scalar density, i.e.~it has to be a nontrivial scalar function $V(g)$ multiplied by the scalar density $\sqrt{-g}$. Obviously, the scalar function $V(g)$ cannot have any loose covariant indices. Moreover, it should not contain any derivatives. But then, the only object at hand to contract the indices of the metric tensor $\gmn$ is the metric itself which, since $g^{\mu\nu}\gmn=d$, leads to a trivial cosmological constant contribution in the action. We conclude that there is no possibility to construct a covariant nonlinear interaction term for a spin-2 field using only one tensor field.\footnote{Note the difference to e.g.~the vector example, where the metric $\gmn$ can be used to contract the indices in nonlinear interaction terms for $A_\mu$ in a nontrivial way. Furthermore, in the massless spin-2 theory this problem did not occur because in the kinetic terms the indices of the metric could be contracted with derivative operators.} 
Hence, we are forced to introduce a second rank-2 tensor, which we shall call $\fmn$ and which can be used to build nonlinear contractions with $\gmn$. The interaction potential will then be given by $\sqrt{-g}$ multiplying a scalar function of $g^{\rho\mu}\fmn$. 
  

In summary, we expect the nonlinear massive gravity action to be of the form,
\beqn\label{mggenact}
S_\mathrm{MG}=\int \mathrm{d}^dx~\sqrt{-g}~\left[M_{\mathrm{Pl}}^{d-2}R(g) - m^d\, V(g^{-1}f)\right]\,,
\eeqn
where $m$ is an arbitrary energy scale that sets the mass of the spin-2 field. In this setup, the second ``metric" $\fmn$ is a fixed background field that needs to be put into the theory by hand. From the viewpoint of field theory this seems unfamiliar because $\fmn$ is not determined by an equation of motion. But, in fact, there is no need to worry about this, since we will resolve this slightly confusing point in the next chapter, when we introduce the fully dynamical bimetric theory that treats $\gmn$ and $\fmn$ on the same footing. For now, let us accept the possibility to work with a fixed reference metric $\fmn$ and investigate the consistency of this class of theories. 

Obviously, a necessary requirement on the interaction potential in (\ref{mggenact}) is that it reduces to the Fierz-Pauli mass term when linearized around flat space (i.e.~with flat reference metric $\fmn$ and flat background for $\gmn$), otherwise it will certainly propagate the Boulware-Deser ghost. As it will turn out in a nonlinear constraint analysis, a generic interaction potential, even if it incorporates the Fierz-Pauli structure around flat space, will reintroduce this extra degree of freedom at the nonlinear level. This is anticipated from a simple degree-of-freedom counting:
The introduction of the interaction potential breaks the diffeomorphism invariance of general relativity. Therefore the $d$ gauge symmetries are lost and the theory generically will propagate $d$ additional degrees of freedom. Since $d(d-3)/2+d=d(d-1)/2$, this does not give the correct number for a massive spin-2 particle, but there is an extra degree of freedom in the theory. This is the nonlinear Boulware-Deser ghost and an extra constraint is needed to remove it from the spectrum of propagating modes. Tuning the linear mass term to the Fierz-Pauli combination ensured the presence of this constraint in the linear theory.
In section~\ref{sec:conspot} we will demonstrate that, in order to obtain an additional constraint and thereby ensure the absence of the ghost, it is necessary to impose strong restrictions on the structure of nonlinear interactions. In fact, demanding the presence of a constraint will fix all but $(d-2)$ coefficients of all possible interaction terms.
 
 
In the construction of the consistent theory, we will follow the approach of Boulware and Deser who studied Massive Gravity in the Hamiltonian formulation~\cite{Boulware:1972zf, Boulware:1973my}. They claimed that, even though it is possible to remove the ghost from the spectrum of propagating modes at the linear level, it will return for any nonlinear interaction terms that are added to the Lagrangian (\ref{FPlag}). In order to show that this result is in fact incorrect, we first need to familiarize us with variables suitable for the Hamiltonian formulation of GR.
   
  
   


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
\subsection{ADM variables for General Relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  




The Hamiltonian formulation of GR traces back to work by Arnowitt, Deser, and Misner (ADM) from 1962~\cite{Arnowitt:1962hi}. The authors decomposed the metric $\gmn$ into a scalar $N$, a symmetric $(d-1)\times (d-1)$ matrix $\gamma_{ij}$, and a vector $N_i$ with $(d-1)$ components as follows: 
\beqn\label{admmetr}
\gmn=\begin{pmatrix}
-N^2+N_i \gamma^{ij}N_j& N_j\\
N_i & \gamma_{ij}
\end{pmatrix}\,,
\eeqn
where $\gamma^{ij}$ denotes the inverse of $\gamma_{ij}$. This parametrization essentially splits the metric into its time ($0\mu$) and spatial ($ij$) components; in $d=4$ it is therefore also referred to as \textit{(3+1)-decomposition}. From (\ref{admmetr}) we can also compute the inverse of the metric,
\beqn\label{invadm}
g^{\mu\nu}=\frac{1}{N^2}\begin{pmatrix}
-1& N^j\\
N^i & N^2\gamma^{ij}-N^iN^j
\end{pmatrix}\,.
\eeqn
It turns out that, in any theory with kinetic structure given by the Einstein-Hilbert term, the $0\mu$-components are nondynamical gauge degrees of freedom because the Ricci scalar of $\gmn$ contains no derivatives of those components. Hence, all of the propagating modes are contained in the spatial metric $\gamma_{ij}$ which has $d(d-1)/2$ independent components. As we will see now, the gauge invariance of GR will reduce the number of propagating degrees of freedom to $d(d-3)/2$, along with the same number of corresponding canonical momenta.


In terms of the ADM variables the Einstein-Hilbert action (\ref{EHGR}) becomes (up to total derivatives that can be discarded) \cite{Arnowitt:1962hi}
\beqn\label{gradm}
S_{\mathrm{GR}}%=M_\mathrm{P}^{d-2}\int \mathrm{d}^4x~\sqrt{-g}~R
=M_\mathrm{P}^{d-2}\int \mathrm{d}^dx~\left(\pi^{ij}\partial_t \gamma_{ij}-NR^0-N_iR^i\right)\,,
\eeqn
where, in terms of the curvature scalar $R_{(d-1)}$ of the metric $\gamma_{ij}$,
\beqn
R^0&=& -\sqrt{\gamma}~ \left[R_{(d-1)} +\gamma^{-1}\left(\frac{1}{2}({\pi^i}_i)^2-\pi^{ij}\pi_{ij}\right)\right] \,,\nonumber\\
R^i&=& -2\partial_j\pi^{ij}.
\eeqn
The conjugate momenta $\pi^{ij}$ of the $d(d-1)/2$ metric components $\gamma_{ij}$ are computed from the GR Lagrangian in the standard way which leads to expressions in terms of derivatives of the $d$-dimensional metric.

As pointed out before, the action (\ref{gradm}) does not contain dynamical terms for the scalar $N$ nor for the vector $N^i$. On top of that, these variables appear only linearly.
Therefore they act as Lagrange multipliers, and their equations of motion do not contain $N$ and $N^i$ themselves. This means that these equations
constitute $d$ primary constraints~$R^\mu=(R^0, R^i)$ on the remaining $d(d-1)$ variables $\gamma_{ij}$ and $\pi^{ij}$. 

According to the theory of constrained Hamiltonian systems,\footnote{For review of this subject see~\cite{Date:2010xr}.} the presence of a gauge symmetry can now be seen in the Poisson algebra of the constraints, $\{R^\mu, R^\nu\}$. Here, the Poisson bracket for functions $A,B$ is defined as
\beqn\label{defpoisb}
\{A(x), B(y)\}\equiv\int \mathrm{d}^3z~\left(  \frac{\delta A(x)}{\delta g_{ij}(z)}\frac{\delta B(y)}{\delta \pi^{ij}(z)} -\frac{\delta A(y)}{\delta \pi^{ij}(z)}\frac{\delta B(x)}{\delta g_{ij}(z)}\right)\,.
\eeqn
The result for the constraint algebra of GR reads~(see e.g.~\cite{Khoury:2011ay})
\beqn
\{R^0(x), R^0(y)\}&=& R^i(y)\frac{\partial}{\partial y^i}\delta^3(x-y)-R^i(x)\frac{\partial}{\partial x^i}\delta^3(x-y)\, , \nonumber\\
\{R_i(x), R_j(y)\}&=& R_i(y)\frac{\partial}{\partial y^j}\delta^3(x-y)-R_j(x)\frac{\partial}{\partial x^i}\delta^3(x-y)\,,\nonumber\\
\{R^0(x), R_i(y)\}&=& -R^0(y)\frac{\partial}{\partial x^i}\delta^3(x-y)\,.
\eeqn
Since these brackets are proportional to the constraints themselves, they vanish on the constraint surface, as they should in the presence of a gauge symmetry. This implies that all $d$ primary constraints will serve to put conditions on the remaining variables $\gamma_{ij}$ and $\pi^{ij}$, while the Lagrange multipliers $N$ and $N^i$ remain undetermined. There will be no secondary constraints because the primary constraints are automatically preserved in time.

After imposing the $d$ conditions on $\gamma_{ij}$ and $\pi^{ij}$, we can still use gauge transformations to remove $d$ more degrees of freedom. In total we therefore end up with $d(d-3)$ variables, corresponding to the helicity states of the massless graviton and their canonical momenta. This shows that, even nonlinearly, GR propagates the correct number of degrees of freedom for describing a massless spin-2 particle.

Note that throughout the above discussion we never actually wrote down the Hamiltonian, but remained in the Lagrangian formulation. In order to investigate the positivity of the energy, this is naturally insufficient, but since here we were only interested in counting degrees of freedom there was no need to work with the Hamiltonian, which can trivially be obtained from (\ref{gradm}). 


        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%         
\subsection{ADM variables for Massive Gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

In a general nonlinearly interacting theory of the form (\ref{mggenact}), the lapse and shift functions $N$ and $N^i$ will still appear without derivatives. However, the interaction potential will in general no longer be linear in these functions. Therefore, their equations of motion, instead of imposing constraints on the remaining variables, will now determine $N$ and $N^i$ themselves. The $d$ gauge constraints are lost and, as already explained in section \ref{sec:nonlin}, the number of propagating modes will now be $d(d-1)/2$, plus the corresponding canonical momenta. These are two phase-space degrees of freedom too many for the theory of a massive spin-2 particle. Moreover, the Hamiltonian of a generic theory will not be positive definite~\cite{Boulware:1972zf, Boulware:1973my}, signaling that the extra propagating mode is a ghost.  
The necessary requirement on a consistent interaction potential is therefore the presence of an additional constraint that removes the nonlinear Boulware-Deser ghost.

In order to investigate the posibility for a potential in~(\ref{mggenact}) that gives rise to a constraint, we first decompose the second rank-2 tensor $f_{\mu\nu}$ into its own ADM variables,
\beqn\label{admf}
f_{\mu\nu}=\begin{pmatrix}
-L^2+L_l \tilde{f}^{lk}L_k& L_j\\
L_i & \tilde{f}_{ij}
\end{pmatrix}\,.
\eeqn
Here, $\tilde{f}^{ij}$ denote the inverse of the $(d-1)\times (d-1)$ matrix $\tilde{f}_{ij}$, $L_i$ is the shift, and $L$ is the lapse of~$f_{\mu\nu}$. 
We furthermore express the measure factor $\sqrt{-g}$ in terms of the lapse $N$ and the determinant $\gamma$ of $\gamma_{ij}$,
\beqn\label{measur}
\sqrt{-g}=N \sqrt{\gamma}\,.
\eeqn
With these expressions at hand, we can write a generic interaction potential in terms of ADM variables,
\beqn
\sqrt{-g}~V(g^{-1}f)=N \sqrt{\gamma}~V(\gamma_{ij}, N, N^i; \tilde{f}_{ij}, L, L^i)\,.
\eeqn
In order to provide a constraint, the right-hand side of this equation needs to be linear in the lapse $N$. In fact, the necessary condition on the potential is slightly weaker than that because the constraint may be obtained after combining several of the equations for $N$ and $N^i$. If there exists a combination of these equations that is independent of $N^i$ and $N$, then this equation will constrain the remaining variables. At the level of the action, this means that we should allow for a field-dependent redefinition of the shift, $N^i\rightarrow n^i$, that renders the Lagrangian linear in the lapse $N$. Certainly, such a redefinition must be linear in $N$ itself since $N^i$ appears linearly in the kinetic term. Furthermore, since the redefined shift $n^i$ is expected to appear in the constraint, it must be fully determined by its own equation of motion which therefore must not depend on $N$.  To summarize, we make two requirements on the potential in terms of the redefined shift $n^i$:
\begin{itemize}
\item[(i)] linearity of the Lagrangian in $N$,
\item[(ii)]  absence of $N$ in the $n^i$ equations of motion.
\end{itemize} 
Next, we observe that the interaction potential already has a factor of $N$ in front coming from the measure factor (\ref{measur}). Hence, in order to satisfy requirement (i), the potential $V(g^{-1}f)$ written in ADM variables must be of the form
\beqn
V(g^{-1}f)=\frac{1}{N}V_1+V_2
\eeqn
where $V_1$ and $V_2$ are functions of $(\gamma_{ij}, n^i; \tilde{f}_{ij}, L, L^i)$, i.e.~independent of~$N$. Recalling the ADM decomposition (\ref{admmetr}) of $\gmn$, it is clear that the only object that has the chance of giving something linear in $1/N$ is the square root of the inverse metric~(\ref{invadm}). We are thus lead to consider a potential~$V$ that is a function of the matrix $S\equiv\sqrt{g^{-1}f}$, defined via $S^2=g^{-1}f$. This square-root matrix has a very nontrivial ADM decomposition and is certainly highly nonlinear in $1/N$. However, we will now make use of the allowed redefinition of the shift $N^i$ in order to write $S$ in the form
\beqn\label{sadm}
S=\frac{1}{N}\mA+\mB\,,
\eeqn
where $\mA$ and $\mB$ are matrix-valued functions of $(\gamma_{ij}, n^i; \tilde{f}_{ij}, L, L^i)$. The redefinition that leads to (\ref{sadm}) as well as the explicit expressions for $\mA$ and $\mB$ can be obtained straightforwardly by the following method: Square the right-hand side of the ansatz (\ref{sadm}) and equate it with the ADM expression for $g^{-1}f$ obtained from (\ref{admmetr}) and (\ref{admf}). Then compare the expressions on both sides order by order in $1/N$ to read off the shift redefinition as well as the matrices $\mA$ and $\mB$.
This derivation is discussed in more detail in {\protect{\hyperref[papI]{Paper~I}}}; here we simply state the result. The redefinition that renders the square-root matrix $S$ linear in $1/N$ takes the rather simple form
\beqn\label{shiftred}
N^i=Ln^i+L^i+N{D^i}_kn^k\,.
\eeqn
The $(d-1)\times(d-1)$ matrix $D$ on the right-hand side is a function of the variables $(\gamma_{ij}, n^i; \tilde{f}_{ij})$. Explicitly, it is given by
\beqn
D=\sqrt{\gamma^{-1}\tilde{f}Q}\,Q^{-1}\,,
\eeqn
where we have defined another matrix $Q$ through
\beqn
{Q^i}_j=x{\delta^i}_j+n^in^k\tilde{f}_{kj}\,,\qquad x=1-n^i\tilde{f}_{ij}n^j\,.
\eeqn
The matrices $\mA$ and $\mB$ then turn out to be
\beqn
\mA=\frac{1}{L\sqrt{x}}
\begin{pmatrix}
a_0&a_j\\
-a_0c^i&-c^ia_j
\end{pmatrix}\,,~~\quad~~
\mB=\sqrt{x}
\begin{pmatrix}
0&0\\
{D^i}_jL^j&{D^i}_j
\end{pmatrix}\,,
\eeqn
in which
\beqn\label{defa}
a_0=L+n^kL_k\,,\qquad a_i=n^kf_{ki}\,,\qquad
c^i=Ln^i+L^i\,.
\eeqn
The form of the redefinition is not entirely unique. In {\protect{\hyperref[papI]{Paper~I}}} we mainly work with a set of variables that slightly differs from the one presented here. This difference does not affect any of the conclusions drawn in the following, but the choice of variables we made here is more suitable for application to bimetric theory in the next chapter.  

Although the above expressions seem rather complicated, what is essential for the construction of the ghost-free potential is the structure of the matrices $\mA$ and $\mB$. Most importantly, $\mA$ has rank one, i.e.~it can be written as the outer product of two vectors,
\beqn\label{vwa}
\mA=v w^\mathrm{T}\,,~~\quad~~\text{where}~~v=\begin{pmatrix}1\\-c^i \end{pmatrix}\,~~\text{and}~~~w=\frac{1}{\sqrt{x}}\begin{pmatrix}a_0\\a^i\end{pmatrix}\,.
\eeqn
Having obtained the suitable ADM expression (\ref{sadm}) for the square-root matrix $S=\sqrt{g^{-1}f}$, we are ready to construct the interactions which give rise to an additional constraint that removes the Boulware-Deser ghost.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%         
\subsection{Construction of the interaction potential}\label{sec:conspot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As explained above, the mass potential has to be a function of the square-root matrix $S=\sqrt{g^{-1}f}=\frac{1}{N}\mA+\mB$, multiplied by $\sqrt{-g}=N\sqrt{\gamma}$\,. We assume this function to be expandable as a Taylor series in $S$. Generically, this will give an expression that is nonlinear in the lapse $N$. 
The only way to ensure linearity in $N$ is to demand the absence of higher powers of~$\frac{1}{N}\mA$ in the expansion. Obviously, the simplest possible term is $\sqrt{-g}~\tr~(\frac{1}{N}\mA+\mB)$. At first sight it seems that all higher powers of $\frac{1}{N}\mA+\mB$ will involve higher powers of~$1/N$. However, due to the special structure of the matrix $\mA$ there is a caveat here:
Since $\mA$ has rank one, it is a projection operator on a one-dimensional subspace. Because of that, there is a unique way of building polynomials of $\frac{1}{N}\mA+\mB$ that are linear in $\frac{1}{N}\mA$. Namely, an antisymmetric product of $\mA$'s will automatically contain only one power of~$\mA$. Let us see how this works in detail. In $d$ dimensions we consider
\beqn\label{potantisym}
V(S)=\sum_{k=0}^d ~b_n~\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d}~{S^{\nu_1}}_{\mu_1}\hdots{S^{\nu_n}}_{\mu_n}\,,
\eeqn
with arbitrary coefficients $b_n$.
Since the simultaneous exchange of $\mu_i$, $\mu_j$ and $\nu_i$, $\nu_j$ only changes the sign of both $\epsilon$-tensors, it leaves the whole term invariant.
Therefore, at $n$th order, the product of $S$'s under the sum can be written in the form,
\beqn
\sum_{l=0}^n {n \choose l}\left(\frac{1}{N}\right)^l   {\mA^{\nu_1}}_{\mu_1}\hdots {\mA^{\nu_l}}_{\mu_l}{\mB^{\nu_{l+1}}}_{\mu_{l+1}}\hdots {\mB^{\nu_n}}_{\mu_n}\,.      
\eeqn
We insert this expression into (\ref{potantisym}) and obtain
\beqn
V(S)=\sum_{n=0}^d b_n\sum_{l=0}^n {n \choose l}\left(\frac{1}{N}\right)^l V_n(\mA,\mB)\,,
\eeqn
with
\beqn
V_n(\mA,\mB)&=&\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d} \nn\\
&~&\hspace{50pt}\cdot~{\mA ^{\nu_1}}_{\mu_1}\hdots {\mA ^{\nu_l}}_{\mu_l}{\mB^{\nu_{l+1}}}_{\mu_{l+1}}\hdots {\mB^{\nu_n}}_{\mu_n}  \nonumber\\
&=&\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d}\nn\\
&~&\hspace{50pt} \cdot~{v ^{\nu_1}}w_{\mu_1}\hdots {v ^{\nu_l}}w_{\mu_l}{\mB^{\nu_{l+1}}}_{\mu_{l+1}}\hdots {\mB^{\nu_n}}_{\mu_n}\,.
\eeqn
Here we have used (\ref{vwa}).
Since all indices of the symmetric product of $v^{\nu_i}$ are contracted with the totally antisymmetric indices of $\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d} $, we find that in $V_n(\mA,\mB)$ only terms with at most one $\mA$ contribute. This is precisely the property that we were looking for.  
We conclude that the most general form of the potential that is linear in $N$ after the redefinition (\ref{shiftred}) is
\beqn
\sqrt{-g}\,\sum_{n=0}^d ~b_n~\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d}~{S^{\nu_1}}_{\mu_1}\hdots{S^{\nu_n}}_{\mu_n}\,,
\eeqn
with $S=\sqrt{g^{-1}f}$. A more convenient way of writing this is by introducing the elementary symmetric polynomials of the matrix $S$ that can be defined through a recursion formula,
\beqn
e_n(S)=\frac{(-1)^{n+1}}{n}\sum_{k=0}^{n-1}(-1)^{k}\tr (S^{n-k})e_k(S)\,,\quad \text{with}~~e_0(S)=1\,.
\eeqn
Properties of the elementary symmetric polynomials are summarized in appendix~\ref{app:el}.
In terms of these the potential takes the simple form,
\beqn\label{potsympol}
\sqrt{-g}~V(S)=\sqrt{-g}\,\sum_{n=0}^d ~\beta_ne_n(S)\,,
\eeqn
where we have introduced the rescaled coefficients $\beta_n=\frac{n!(d-n)!}{2}b_n$. Since the elementary symmetric polynomials also appear in the expansion of the determinant, the above potential can be regarded as a \textit{deformed determinant}. Note in particular that there is only a finite number of terms giving a potential which is linear in $N$. Due to the antisymmetric structure of the interactions, the possible terms are limited by the dimension of space time. Moreover, out of the $d$ parameters $\beta_n$, only $(d-2)$ are truely measuring interaction strengths: Since $e_0(S)=1$, the $\beta_0$-term is simply a cosmological constant. Also, the last term in the sum that is proportional to $\beta_d$ is just a cosmological constant term for $\fmn$ because $e_d(S)=\det S$. It is therefore independent of $\gmn$ and does not contribute to the equation of motion. Nonetheless, we choose to include it in the action because it will become relevant when we give dynamics to $\fmn$ in the next chapter.

As we have argued, (\ref{potsympol}) is the most general potential that satisfies the above criterion (i). We now explain why requirement (ii) follows automatically. Namely, we can write the equations of motion for $n^i$ obtained from the nonlinear massive gravity action $S_\mathrm{MG}$ as
\beqn
\frac{\delta S_\mathrm{MG}}{\delta n^i}=\frac{\delta N^j}{\delta n^i}\frac{\delta S_\mathrm{MG}}{\delta N^j}=0\,.
\eeqn
Observe that these equations can depend on $N$ at most linearly because the action is linear in $N$. But since the redefinition (\ref{shiftred}) is already linear in $N$, so is $\frac{\delta N^j}{\delta n^i}$ and consequently $\frac{\delta S_\mathrm{MG}}{\delta N^j}$ is independent of $N$. Furthermore, $\frac{\delta N^j}{\delta n^i}$ is nonzero since it is the Jacobian of the redefinition. The $n^i$ equations of motion are therefore equivalent to $\frac{\delta S_\mathrm{MG}}{\delta N^j}=0$ which is independent of~$N$. Hence, by constructing a potential that meets requirement (i), we automatically satisfy criterion (ii). This has also been shown explicitly in {\protect{\hyperref[papI]{Paper~I}}}. 
 

To summarize, we have derived the nonlinear massive gravity action equipped with an additional constraint that removes the Boulware-Deser ghost,
\beqn\label{HRMG}
S_\mathrm{MG}=\int \mathrm{d}^dx\,\sqrt{-g}\,\left[M_{\mathrm{Pl}}^{d-2}R(g) -2 m^d\sum_{n=0}^d ~\beta_ne_n\left(S\right)\right]\,,
\eeqn
with $S=\sqrt{g^{-1}f}$. Once the structure of the theory was known, it was also possible to derive the constraint in a purely covariant formulation for some simplifying parameter choices~\cite{Deffayet:2012nr}. 
In the literature, the above action has been widely referred to as the dRGT model. However, it should be stressed that the theory derived by de Rham, Gabadadze and Tolley in \cite{deRham:2010ik, deRham:2010kj} was defined with flat reference metric $\fmn=\emn$ only. The dRGT construction uses St\"uckelberg fields (see section~\ref{sec:stuck}) and is valid only in a certain decoupling limit that strongly relies on the flat reference metric. In contrast, the construction we have presented here is valid for all reference metrics and demonstrates the consistency of the fully nonlinear theory away from any limiting approximation.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The secondary constraint}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The above requirements on the consistent interaction potential were necessary but not sufficient: A secondary constraint is crucial for the absence of the Boulware-Deser ghost because two constraints are needed to remove both the ghost mode and its canonical momentum from the set of dynamical variables.

It was motivated in Paper I that there is in fact a secondary constraint arising from demanding the primary constraint to be constant in time.  In order to compute the time evolution of the constraint one uses the Poisson bracket (\ref{defpoisb}) and the Hamiltonian, which for the above Massive Gravity action is of the form
 \beqn\label{hamsecc}
H=\int \mathrm{d}^{d-1} y~(\mathcal{H}_0-N\mathcal{C})\,.
\eeqn
Here $\mathcal{H}_0$ is independent of $N$ and $\mathcal{C}$ is the Hamiltonian constraint obtained from varying the action with respect to $N$. The time evolution of $\mathcal{C}$ then reads
\beqn\label{seccons}
\frac{\mathrm{d}\mathcal{C}(x)}{\mathrm{d}t}=\{\mathcal{C}(x),H\}=0\,.
\eeqn  
As in the case of the primary constraint, this equation should be independent of $N$, because otherwise it would determine $N$ instead of constraining $\gamma_{ij}$ and $\pi^{ij}$. Inserting~(\ref{seccons}) into~(\ref{hamsecc}) gives
\beqn
\int \mathrm{d}^{d-1} x~\Big(\{\mathcal{C}(x),\mathcal{H}_0(y)\}-N\{\mathcal{C}(x),\mathcal{C}(y)\}\Big)=0\,.
\eeqn  
Since $\mathcal{C}$ and $\mathcal{H}_0$ are independent of $N$, we therefore need the Poisson bracket among the constraints $\{\mathcal{C}(x),\mathcal{C}(y)\}$ to vanish because the secondary constraint cannot depend on $N$. Before this was actually demonstrated to be the case, there had been objections against the theory claiming that $\{\mathcal{C}(x),\mathcal{C}(y)\}$ could be nonzero \cite{Kluson:2011qe}. The issue was resolved when the secondary constraint was eventually shown to exist in a detailed calculation in~\cite{Hassan:2011ea}. With this, the consistency of the nonlinear Massive Gravity action (\ref{HRMG}) was fully proven.




 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%        
\section{Consistency in the St\"uckelberg formulation}\label{sec:stuck}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As stated earlier, the invariance under general coordinate transformations of General Relativity is broken by the mass term for the graviton. This is because the metric $\gmn$ itself transforms as a covariant rank-two tensor under GCTs while the fixed background metric $\fmn$ does not. Therefore objects like $g^{\mu\nu}\fmn$ are not diffeomorphism invariant. However, there exist a method to restore the gauge symmetry in the action: By introducing new gauge degrees of freedom, so-called St\"uckelberg fields, that transform in a certain way under the gauge group, one can rewrite the theory in a manifestly gauge invariant way. In turn, fixing the so-called physical gauge will give back the original action.

While the proof of absence of the Boulware-Deser ghost given in {\protect{\hyperref[papI]{Paper~I}}} was formulated in the gauge-fixed version of massive gravity, i.e.~without introducing the St\"uckelberg fields, it is expected that restoring the gauge invariance does not alter the dynamics of the theory. In fact, since gauge symmetry is merely a redundancy in the description of the underlying physics, the two formulations are completely equivalent. In particular, absence of ghost in the gauge fixed version of Massive Gravity implies that the St\"uckelberg formulation cannot exhibit the instability either.

Nevertheless, before the constraint needed to remove the ghost was computed explicitly in the St\"uckelberg formulation, there had been some confusion regarding this issue. Namely, in \cite{Chamseddine:2011mu, Kluson:2011rt, Kluson:2012gz}, it was claimed that the Boulware-Deser ghost seems to reappear in the gauge invariant theory. If this was true, it would have suggested a flaw in the consistency proof of gauge fixed Massive Gravity. Fortunately, we were eventually able to prove the absence of ghost in the St\"uckelberg formulation in {\protect{\hyperref[papIII]{Paper~III}}}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The St\"uckelberg trick}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
One possibility to reintroduce diffeomorphism invariance in Massive Gravity is to perform a gauge transformation on the dynamical metric~$\gmn$ and treat the gauge parameters as new fields in the action. Under a GCT, $x^\alpha\rightarrow x'^\alpha(x)$, the metric transforms as
\beqn
\gmn(x)\rightarrow\frac{\partial x'^\alpha}{\partial x^\mu}\frac{\partial x'^\beta}{\partial x^\nu}g_{\alpha\beta}(\phi)\,.
\eeqn
After performing this GCT, one interprets the $x'^\alpha$ as dynamical fields. Another equivalent way, that will be more convenient for our purposes, is to mimic this kind of transformation on the reference metric $\fmn$, which, of course, actually does not transform under GCTs.  But since a simultaneous coordinate transformation of $\gmn$ and $\fmn$ would be a symmetry of the Massive Gravity action, instead of transforming $\gmn$ we can choose to perform the transformation on $\fmn$. 
That is to say, we replace $\fmn$ by its covariantized form
\beqn\label{etcov}
\fmn\rightarrow\frac{\partial \varphi^\alpha}{\partial x^\mu}\frac{\partial \varphi^\beta}{\partial x^\nu}\bar{f}_{\alpha\beta}\,.
\eeqn
Here, $\bar{f}_{\alpha\beta}$ is a new fixed background metric that does not transform under the gauge group. The ``coordinates'' $\varphi^\alpha$ are promoted to dynamical fields that transform as scalars under GCTs. Introducing these St\"uckelberg fields ensures that objects such as
\beqn
 \Tr\, (g^{-1}f) =g^{\mu\nu}\frac{\partial \varphi^\alpha}{\partial x^\mu}\frac{\partial \varphi^\beta}{\partial x^\nu}\bar{f}_{\alpha\beta}
 \eeqn
are diffeomorphism invariant. In addition to the equations of motion for the metric $\gmn$, we now also consider the $\varphi^\alpha$ equations and, as we will see below, this system of equations is equivalent to the original $\gmn$ equation without St\"uckelberg fields.
 
Let us expand the St\"uckelberg fields around the identity transformation, which corresponds to considering infinitesimal GCTs,
\beqn
\varphi^\alpha=x^\alpha-\pi^\alpha\,.
\eeqn 
Furthermore, we decompose the perturbations into a transverse and a longitudinal mode,
\beqn\label{decpi}
\pi^\alpha=\hat{\pi}^\alpha+\partial^\alpha\pi\,.
\eeqn
The power of the St\"uckelberg formalism lies in the conjecture that the ghost instability of nonlinear Massive Gravity can be traced back to higher derivative interactions of the $\pi$ fields in flat space, where $\bar{f}_{\alpha\beta}=\eta_{\alpha\beta}$ \cite{ArkaniHamed:2002sp}. This assumption relies on an analogy to the Goldstone equivalence theorem for spin-1 fields \cite{Lee:1977yc, Chanowitz:1985hj}. In that case, the longitudinal modes of the gauge fields have been shown to carry all information needed for computing scattering processes at high energies. Although the theorem has not been proven for the spin-2 case, it is reasonable to start with the assumption of its validity in order to investigate the stability of Massive Gravity in a certain high energy limit. This limit (also referred to as \textit{decoupling limit}) essentially corresponds to setting the metric perturbation to zero and also ignoring all terms involving the transverse components of the St\"uckelberg fields. Then the conjecture of \cite{ArkaniHamed:2002sp} suggests to construct the interaction potential in such a way that there appear no higher-order interactions of the longitudinal modes. Since each of these modes always comes with two derivatives, their interactions generically give rise to higher derivative terms. These can be shown to lead to ghosts and must therefore be avoided in a consistent theory.
The conclusion of an exhaustive analysis in \cite{Creminelli:2005qk} was that avoiding the higher derivative terms was impossible, and once more it seemed that there exists no consistent nonlinear theory for Massive Gravity. However, it turned out that the authors of~\cite{Creminelli:2005qk} had made sign mistake, and after correcting that flaw, de Rham, Gabadadze and Tolley were indeed able to construct a theory without higher-derivative interactions of the $\pi$ fields. The trick they employed was to tune the coefficients of the interaction terms in such a way that the higher derivative terms combined into total derivatives that could be dropped from the action. 
This lead to the nonlinear Massive Gravity action (\ref{HRMG}) with flat $\fmn$ (and limited parameter space since one of the $\beta_n$ was fixed to ensure a flat background solution for $\gmn$). The complete expression for its decoupling limit, including the transverse vector modes in~(\ref{decpi}), was worked out in~\cite{Ondo:2013wka}.
 
Being free of ghost instabilities in the decoupling limit, the dRGT model is definitely a promising candidate for a consistent theory of nonlinear Massive Gravity in flat space. However, consistency of the theory in all its interactions, that is, away from the decoupling limit, is difficult to prove in the St\"uckelberg formulation, in particular for general $\beta_n$ parameters. The main complication arises due to the square-root matrices appearing in the potential. However, as we explain in the following, it is easy to see that the ghost proof of the gauge fixed theory carries over to the gauge invariant mass potential.
Thereafter, in order to support our arguments even further, we demonstrate the consistency of Massive Gravity in the St\"uckelberg formulation explicitly by identifying the constraint that removes the ghost.  



        
                

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{General arguments for consistency}\label{secgenargst}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
The fact that the dynamics remain unaltered in the gauge invariant theory can be demonstrated by considering the equations of motions for the St\"uckelberg fields. After making the replacement (\ref{etcov}) for $f_{\mu\nu}$, the mass potential $V(g,f)$  becomes a function of the scalar fields and their equations of motions read
\beqn\label{varphieoms}
\frac{\delta}{\delta\varphi^A} V(g,\varphi^B)=0\,.
\eeqn
However, this equation will not give rise to any new dynamics because it is, in fact, already implied by the Bianchi constraint of the gauge fixed theory,
\beqn
&~&\nabla^\mu V_{\mu\nu}(g,\varphi^B)=0\,,\nn\\
&~& \text{where}~~~V_{\mu\nu}(g,\varphi^B)\equiv\frac{1}{\sqrt{-g}}\frac{\delta}{\delta g^{\mu\nu}}\left(\sqrt{-g}~ V(g,\varphi^B)\right)\,.
\eeqn
This constraint follows from the divergence of the $\gmn$ equations after using the Bianchi identity $\nabla^\mu G_{\mu\nu}=0$.
In order to see the equivalence, consider a gauge transformation $\delta x^\mu=\xi^\mu$ of the action involving St\"uckelberg fields,
\begin{align}
&\delta S=\int\mathrm{d}^dx\sqrt{-g}\left[\left(\mpl^{d-2} G_{\mu\nu}
-2m^dV_{\mu\nu}\right)\delta g^{\mu\nu}
-2m^d\frac{\delta V}{\delta\varphi^A}\delta\varphi^A\right]\,.
\end{align}
Here $G_{\mu\nu}$ is the Einstein tensor and the variations under the gauge transformation read $\delta g^{\mu\nu}=-2\nabla^{(\mu} \xi^{\nu)}$ and $\delta\varphi^A=-\xi^\mu\partial_\mu\varphi^A$. As the action is invariant under GCTs, integrating by parts and using the Bianchi identity shows that
\beqn\label{coordconst}
\nabla^\mu V_{\mu\nu} = \frac{\delta V}{\delta\varphi^A}\partial_\nu\varphi^A\,,
\eeqn
identically.
Since the St\"uckelberg fields were introduced to mimic nonsingular coordinate transformations, the matrix $\partial_\nu\varphi^A$ is invertible and hence the Bianchi constraint $\nabla^\mu V_{\mu\nu}=0$ is equivalent to the $\varphi^A$ equations of motion~(\ref{varphieoms}). As expected, the redundant gauge degrees of freedom $\varphi^A$ therefore do not introduce new dynamics into the theory.

From these general arguments we thus expect the consistency proof of Paper~I to be valid for both the gauge fixed and the gauge invariant version of Massive Gravity.
Nonetheless there had been some work arguing against the consistency of the action involving St\"uckelberg fields: In \cite{Chamseddine:2011mu} it was claimed that the ghost generically reappears in the St\"uckelberg sector and the author of \cite{Kluson:2011rt, Kluson:2012gz} could not find a constraint to remove the ghost. Although this constraint was shown to be present in a two-dimensional toy model and to fourth order in perturbation theory in four dimensions \cite{deRham:2011rn}, the issue remained unresolved until we performed the full Hamiltonian analysis in Paper~II. The following section summarizes our findings.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%       
\subsection{Hamiltonian analysis}\label{hamstuck}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

For the sake of simplicity, in {\protect{\hyperref[papIII]{Paper~III}}} we restrict the constraint analysis of Massive Gravity with St\"uckelberg fields to an interaction potential with only $\beta_1\neq 0$. The analysis for general $\beta_n$ is much more involved and has not been carried out yet. Also, here we focus on $d=4$ although the results straightforwardly generalize to arbitrary number of space-time dimensions. 

The reason why the so-called \textit{minimal model} with only $\beta_1\neq 0$ is simpler, is that, as has been noticed in \cite{Golovnev:2011aa, Buchbinder:2012wb}, in this case the action involving St\"uckelberg fields is equivalent to
\beqn\label{phistuckact}
S_\Phi=M_\mathrm{g}^2\int \md^4 x\sqrt{-g}\left(R-m^4\left[{\Phi^A}_A+{(\Phi^{-1})^A}_B {{\bf A}^B}_A\right]\right)\,,
\eeqn
where ${{\bf A}^B}_A\equiv g^{\mu\nu}\partial_\mu\varphi^B\partial_\nu\varphi^C\bar{f}_{CA}$ and ${\Phi^A}_B$ is an auxiliary field that has been introduced in order to remove the square root. Integrating out ${\Phi^A}_B$ gives back the original action involving $\sqrt{g^{-1}f}$ with $\beta_1=1$. This formulation of the minimal model greatly simplifies the ADM analysis. 
In the following, we raise and lower indices on the St\"uckelberg fields as well as on the auxiliary field with the background metric $\bar{f}_{AB}$.

Using the ADM variables (\ref{admmetr}) for the metric $\gmn$ and computing the canonical momenta $p_A$ conjugate to the St\"uckelberg fields $\varphi^A$, we obtain the Hamiltonian corresponding to (\ref{phistuckact}),
\beqn
\mathcal{H}=-NR_0-N^iR_i+N\mathcal{H}_T^\mathrm{sc}+N^i\mathcal{H}^\mathrm{sc}_i\,,
\eeqn
in which the first two pieces are the familiar ones coming from the Einstein-Hilbert term and where
\beqn
\mathcal{H}_T^\mathrm{sc}&=&\sqrt{\gamma}M_\mathrm{P}^2m^2\big({\Phi^A}_A+{(\Phi^{-1})^A}_B{V^B}_A\big)+\frac{1}{4m^2M_\mathrm{P}^2\sqrt{\gamma}}\Phi^{AB}p_Ap_B\,, \nonumber\\
\mathcal{H}^\mathrm{sc}_i&=& p_A\partial_i\varphi^A\,.
\eeqn
Here we have also defined 
\beqn\label{defvab}
{V^B}_A\equiv \gamma^{ij}\partial_i\varphi^B\partial_j\varphi^C\bar{f}_{CA}\,.
\eeqn
Note that in this formulation involving the auxiliary field ${\Phi^A}_B$ the Hamiltonian is manifestly linear in $N$ and $N^i$. There is no need for a field redefinition in order to demonstrate the linearity in the lapse. The linearity in $N^i$ is of course due to the fact that we have reintroduced the gauge invariance and now, as in General Relativity, expect to encounter four first class constraints. They can be thought of as removing the St\"uckelberg fields from the set of dynamical variables. Gauge fixing then serves to also remove their canonical momenta. However, the Hamiltonian constraint that is needed to remove the Boulware-Deser ghost mode within the metric $\gamma_{ij}$ is not among the gauge constraints but has to arise separately. Hence, as in the gauge fixed case, a generic theory would be inconsistent and an extra constraint is present only for special choices of the potential. 

The important observation that was missed in \cite{Kluson:2011rt, Kluson:2012gz} is now that, besides the constraints imposed by the equations of motion for $N$ and $N^i$, the 10 equations of motion for the symmetric field $\Phi^{AB}$ actually only determine 9 independent combinations of the $\Phi^{AB}$. One equation is independent of $\Phi^{AB}$ and therefore constrains the remaining variables. The reason for this is the singularity of the matrix ${V^B}_A$ defined in (\ref{defvab}). The equations of motion obtained from varying (\ref{phistuckact}) with respect to $\Phi^{AB}$ read
\beqn\label{capphieom}
%\Psi_{AB}\equiv
\sqrt{\gamma}\,M_\mathrm{P}^2m^2\Big(\bar{f}_{AB}-
(\Phi^{-1})_{AC}V^{CD}(\Phi^{-1})_{DB}\Big)&~&
\nn\\ 
+~\frac{1}{4m^2M_\mathrm{P}^2\sqrt{\gamma}}\,p_A\,p_B&=&0\,.
\eeqn
Being composed of two $3\times 4$ matrices and a $3\times 3$ matrix, ${V^B}_A$ can at most have rank three. The same is true for the combination of matrices $(\Phi^{-1})_{AC}V^{CD}(\Phi^{-1})_{DB}$ that appears in (\ref{capphieom}). A generic $4\times 4$ symmetric matrix of rank-three has only nine independent components and therefore the ten equations of motion for $\Phi^{AB}$ determine only nine independent combinations of $\Phi^{AB}$. The tenth equation serves to constrain the remaining variables.

Moreover, it is straightforward to extract the constraint from~(\ref{capphieom}) by taking the determinant of the equation. Since the determinant of a matrix that does not have full rank is zero, we obtain the following constraint equation,
\beqn\label{cconstrainteq}
\mathcal{C}\equiv\det{\bar{f}}\left(\bar{f}_{AB}\frac{p^Ap^B}{\gamma}+4(m^2M_\mathrm{P}^2)^2\right)\approx 0\,.
\eeqn
This extra constraint is not first class, it does not arise from the presence of a gauge symmetry. Just as in the gauge fixed version of the theory, it is therefore necessary to show the existence of a secondary constraint generated by the time evolution of (\ref{cconstrainteq}). This second constraint is needed to remove the canonical momentum of the ghost. From the general arguments given in section \ref{secgenargst} we know that the secondary constraint has to be there, and it can be found explicitly in a straightforward way. The time evolution of the primary constraint (\ref{cconstrainteq}) is given by the Poisson bracket $\{\mathcal{C}(x),H_\mathrm{tot}\}$, in which the total Hamiltonian reads
\beqn\label{htot2}
H_\mathrm{tot}=\int \mathrm{d}^3 x \left[N(\mathcal{H}_T^\mathrm{sc}-R_0+{\Gamma^A}_{B}{\Psi^B}_A)+N^i(\mathcal{H}^\mathrm{sc}_i-R_i)\right]\,.
\eeqn
In this we have included 10 Lagrange multipliers ${\Gamma^A}_{B}$ that enforce the ${\Phi^A}_B$ equations of motion. In fact, we really need to include only the constraint (\ref{cconstrainteq}), i.e.~add a term $\lambda \mathcal{C}$ with one Lagrange multiplier $\lambda$. The two approaches are equivalent and their connection is discussed in {\protect{\hyperref[papIII]{Paper~III}}}. Here we only give the arguments for the absence of the ghost and its momentum. 

The crucial point that still needs to be proven is that the secondary constraint $\mathcal{C}_2=\{\mathcal{C},H_\mathrm{tot}\}\approx 0$ must be independent of $N$ and $N^i$, or otherwise it would determine the classical value for these fields instead of constraining the canonical momentum of the ghost mode. Fortunately, it is quite straightforward to show that the pieces in $\mathcal{C}_2$ that involve $N^i$ cancel out on-shell. Moreover, all remaining terms in $\mathcal{C}_2$ are proportional to $N$ which can therefore be divided out. Hence the secondary constraint is indeed independent of the lapse and shift. Furthermore, all dependence on the Lagrange multipliers ${\Gamma^A}_{B}$ drops out upon use of the ${\Phi^A}_B$ equations of motion. Plugging in the solutions\footnote{In fact, we never derive these solutions explicitly. All that is needed for the proof are some general relations from linear algebra.} to the ${\Phi^A}_B$ equations therefore leaves us with a constraint on the remaining variables that will remove the ghost momentum,
\beqn
\mathcal{C}_2\approx-2\alpha\gamma^{-{1/2}}\bar{f}{(\Phi^{-1})^B}_{D}\partial_j\varphi^D\gamma^{jk}\nabla^{(f)}_kp_B-\alpha^2  \gamma^{-1/2}\bar{f} \pi\,.
\eeqn
Here, we have defined $\nabla^{(f)}_kp_B=\partial_kp_B-\Gamma^D_{AB}p_D\partial_k\varphi^A$, with $\Gamma^D_{AB}$ being the Levi-Civita connection of the metric~$\bar{f}_{AB}$.

Of course, this proof is valid only for the special parameter choice $\beta_1\neq 0$ and all other~$\beta_n$ equal to zero. But from the general arguments given in section \ref{secgenargst} it should be clear that, although it may be harder to find, a constraint is also present in the St\"uckelberg formulation of the full theory. This proves that nonlinear Massive Gravity is ghost-free both in its gauge-fixed and gauge invariant version.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Consistent Bimetric Theory}
\label{ch:HR}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the previous chapter we dealt with the nonlinear theory for a massive spin-2 field~$\gmn$, embedded in some arbitrary but fixed reference frame, set by a second rank-two tensor $f_{\mu\nu}$. The important question that we are about to address now is whether this reference metric can be given dynamics on its own without reintroducing instabilities. From a field-theoretical point of view this would result in a much more natural setup: All fields in the action would be determined dynamically without the need of fixing any of their values by hand. A priori, since the constraint analysis of {\protect{\hyperref[papI]{Paper~I}}} assumed a fixed reference frame, it is not clear whether the Massive Gravity action with dynamical $\fmn$ will still avoid the Boulware-Deser ghost instability. Certainly, the consistency of the theory with two dynamical metrics will depend on the kinetic structure assumed for the second rank-2 tensor. 

The ADM variables introduced above for the constraint analysis of nonlinear Massive Gravity enabled Hassan and Rosen to demonstrate the possibility of promoting $\fmn$ to a dynamical field by simply adding its own Einstein-Hilbert term to the Massive Gravity action~\cite{Hassan:2011zd}. The resulting theory contains two interacting spin-2 fields, one massive and one massless one, as expected from general arguments \cite{Boulanger:2000rq}. Such theories had been under consideration for a long time (see e.g.~\cite{Rosen:1940zz}, \cite{Isham:1971gm}, \cite{Damour:2002wu}), but never with the correct consistent interaction potential (except for very few accidental exceptions~\cite{Chamseddine:1978yu, Nibbelink:2006sz}). It required the discovery of ghost-free Massive Gravity to find the unique consistent bimetric theory. 


%In recent years, bimetric theories were mainly considered in relation to the dark matter problem \cite{Banados:2008fi, Milgrom:2009gv} and in the context of spontaneous Lorentz symmetry breaking \cite{Berezhiani:2007zf, Blas:2009my}. 
%Furthermore, the consistency of effective Lagrangians for interacting spin-2 fields, that could arise in brane models or string theory, has been investigated in~\cite{PhysRevD.40.1095, Buchbinder:1999be, Buchbinder:1999ar, Damour:2002ws}.









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Hassan-Rosen action}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   

The Hassan-Rosen action for bimetric gravity consists of two Einstein-Hilbert terms for $\gmn$ and $\fmn$ as well as non-derivative interactions between the two tensor fields. The interaction potential is given by (\ref{potsympol}), i.e.~it has exactly the same form as in nonlinear Massive Gravity.
Hence the bimetric action reads
\begin{align}\label{HR}
S_\mathrm{HR}~=~m_g^{d-2}\int \mathrm{d}^dx\,\sqrt{-g}&\,R(g)~+~m_f^{d-2}\int \mathrm{d}^dx\,\sqrt{-f}\,R(f) \nn\\
&-~2 m^d\sum_{n=0}^d ~\beta_ne_n(S)\,.
\end{align}  
Here we used again the definition of the matrix square root, $S=\sqrt{g^{-1}f}$. Moreover, $m_g$,$m_f$ denote the Planck masses for $\gmn$ and $\fmn$, respectively.

Na\"ively, there seems to be a straightforward argument why this action cannot be consistent: Suppose we go backwards and freeze one of the two metrics to rearrive at a theory for one spin-two field $\gmn$ in a fixed background. For example, we could set $f_{\mu\nu}=\emn$ which gives back the dRGT action that is known to be consistent. Contrarily, freezing $\gmn$ leads to an action for $f_{\mu\nu}$ whose interaction potential does not seem to resemble the form that is known to be the only consistent one. One could be lead to conclude that bimetric theory therefore has to be inconsistent. However, it turns out that the elementary symmetric polynomials possess a rather unexpected property,
\beqn\label{symprop}
e_n(S)=e_{d-n}(S^{-1})\cdot\det S\qquad \text{for}\quad n=0,\hdots, d\,.
\eeqn
Owing to these identities, Hassan-Rosen bimetric gravity is invariant under the following discrete symmetry,
\beqn\label{symbg}
\gmn \longleftrightarrow \fmn\,,\quad m_g \longleftrightarrow m_f\,,\quad \beta_n\longrightarrow\beta_{d-n}\,. 
\eeqn
This interchange symmetry guarantees that freezing $\gmn$ also gives back the consistent Massive Gravity theory for $f_{\mu\nu}$. Of course, this observation does not automatically prove that the theory with both $\gmn$ and $f_{\mu\nu}$ taken to be dynamical is consistent. It merely shows that one necessary condition on a consistent bimetric theory is indeed satisfied. The actual consistency can only be proven in an ADM analysis, which has been performed in \cite{Hassan:2011zd}. Since now both metrics are dynamical, there are two potential Boulware-Deser ghosts within the theory, the usual one coming from $g_{\mu\nu}$ and another one coming from $f_{\mu\nu}$. One therefore has to show that the action is linear in both of the lapses~$N$ and~$L$. Furthermore, in contrast to the action for massive gravity, the bimetric action (\ref{HR}) has a gauge symmetry: It is invariant under diffeomorphisms, under which~$\gmn$ and~$\fmn$ transform simultaneously. 
It is therefore expected that the bimetric action, if consistent, should describe the $(d(d-2)-1)$ degrees of freedom of a massive and a massless spin-2 field.

Indeed, in \cite{Hassan:2011zd} it has been shown that the action (\ref{HR}) becomes linear in both of the lapses $N$ and $L$. It further turns out that the action becomes also linear in $L^i$. As in general relativity, the shift vectors of $\fmn$ now give rise to three further constraints. In addition to this, the presence of a secondary constraint for the Hamiltonian constraint has been demonstrated in \cite{Hassan:2011ea}. Both of the Boulware-Deser ghosts are therefore absent and the number of degrees of freedom is $(d(d-2)-1)$, the correct number for a massive and a massless spin-2 field. In section~\ref{sec:massspec}, we will see that at the linear level these mass eigenstates are neither the fluctuations of $\gmn$ nor those of $\fmn$ but a superposition of the two. Before we turn to the mass spectrum, however, we need to address the question of how the metrics should couple to matter.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsubsection{Including matter sources}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

So far, the bimetric action in the form (\ref{HR}) does not take into account couplings of $\gmn$ and $\fmn$ to other fields. For phenomenological purposes the nature of the matter couplings is of great importance. The only presently known couplings that can be added to (\ref{HR}) without reintroducing the ghost instabilities are the standard minimal couplings familiar from general relativity,
\beqn\label{matcoup}
S_\mathrm{m}=\int\dd^dx~\sqrt{-g}\,\mathcal{L}^g_m+\int\dd^dx~\sqrt{-f}\,\mathcal{L}^f_m\,.
\eeqn
Here, $\mathcal{L}^g_m$ and $\mathcal{L}^f_m$ are Lagrangians involving matter fields as well as the respective metrics.
The variations of $S_\mathrm{m}$ define the two stress-energy tensors,
\beqn\label{strente}
T^{g}_{\mu\nu}\equiv-\frac{1}{\sqrt{-g}}\frac{\delta S_\mathrm{m}}{\delta g^{\mu\nu}}\,,\qquad 
T^{f}_{\mu\nu}\equiv-\frac{1}{\sqrt{-f}}\frac{\delta S_\mathrm{m}}{\delta f^{\mu\nu}}\,.
\eeqn
We shall not discuss the phenomenological implications of a second metric coupled to matter. In {\protect{\hyperref[papII]{Paper II}}}, where we derive homogeneous and isotropic solutions to the bimetric equations of motion, we set the matter coupling of $\fmn$ to zero. This is always a consistent choice and results in a theory for a spin-2 field that only couples to matter indirectly through gravity. For recent work dealing with both of the couplings, see~\cite{Akrami:2013ffa}.

   
    
    
    
    
 
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\section{Equations of motion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
    
We now turn to the equations of motions for $\gmn$ and $\fmn$, obtained from the Hassan-Rosen action (\ref{HR}) including the matter couplings (\ref{matcoup}). When computing these, the only complication arises from variation of the square-root matrix $S=\sqrt{g^{-1}f}$. However, since this matrix only appears under the trace, one can make use of $\delta (S^2)=(\delta S)S+S(\delta S)$ to obtain $\delta(\Tr\,S)=\Tr(\delta S)=\tfrac{1}{2}\Tr(S^{-1}\delta (S^2))$, and similarly for higher powers of $S$ under the trace~\cite{Hassan:2011vm}. Then it is easy to derive the equations of motion, wich in terms of the Einstein tensor $\mathcal{G}_{\mu\nu}(g)\equiv R_{\mu\nu}(g)-\frac{1}{2}\gmn R(g)$ read
\beqn
\mathcal{G}_{\mu\nu}(g) + \frac{m^d}{m_g^{d-2}}V^g_{\mu\nu}(g,f)&=&\frac{1}{m_g^{d-2}}T^g_{\mu\nu}\,,\label{geq} \\
\mathcal{G}_{\mu\nu}(f)+\frac{m^d}{m_f^{d-2}}V^f_{\mu\nu}(g,f)&=&\frac{1}{m_f^{d-2}}T^f_{\mu\nu}\,.\label{feq}
\eeqn
The contributions coming from the bimetric interaction potential are of the following form,
\beqn\label{poteom}
V^g_{\mu\nu}(g,f)&\equiv& \sum_{n=0}^{d-1}(-1)^n\beta_n \,g_{\mu\lambda}{\big(Y^{(n)}\big)^\lambda}_{\nu}(S)\,,\nn\\
V^f_{\mu\nu}(g,f)&\equiv&\sum_{n=0}^{d-1}(-1)^n\beta_{d-n} \,f_{\mu\lambda}{\big(Y^{(n)}\big)^\lambda}_{\nu}(S^{-1})\,,
\eeqn
in which the matrix functions ${(Y^{(n)})^\lambda}_{\nu}$ are defined in terms of the elementary symmetric polynomials through
\beqn\label{defY}
{\big(Y^{(n)}\big)^\lambda}_{\nu}(S)=\sum_{k=0}^n(-1)^ke_k(S){(S^{n-k})^\lambda}_{\nu}\,.
\eeqn
An immediate consequence of the interchange symmetry (\ref{symbg}) in the bimetric action, which of course carries over to the equations of motion, is the identity $V^f_{\mu\nu}(g,f; \beta_{d-n})=V^g_{\mu\nu}(f,g, ; \beta_{n})$.

Note that in nonlinear Massive Gravity with fixed reference metric $\fmn$, there is only one equation of motion for $\gmn$, given by (\ref{geq}).
In contrast, bimetric gravity has two sets of equations of motion and is therefore much more constrained. Moreover, the $\beta_4$-term enters the $\fmn$ equation and is thus no longer nondynamical but rather appears as a cosmological constant term in the equation for $\fmn$. We will have to say more about the important differences between the two theories in section~(\ref{sec:MGlim}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bianchi constraints}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $\nabla$ and $\tilde{\nabla}$ denote the covariant derivatives compatible with the metrics $\gmn$ and $\fmn$, respectively. In General Relativity without interaction term, covariant conservation of the stress-energy tensor, $\nabla^\mu T^{g}_{\mu\nu}=0$, is a consequence of the equations of motion because the Einstein tensor satisfies the Bianchi identity $\nabla^\mu \mathcal{G}_{\mu\nu}=0$. In other words, a massless spin-2 field can only couple to conserved matter sources. In bimetric gravity the condition is weaker: Invariance of the interaction potential under simultaneous diffeomorphisms of $\gmn$ and $\fmn$ implies 
\beqn\label{bicog}
\sqrt{-g}\,\nabla^\mu V^g_{\mu\nu}+\sqrt{-f}\,\tilde{\nabla}^\mu V^f_{\mu\nu}=0\,.
\eeqn
The constraint on the sources enforced by the equations of motion then reads
\beqn
\sqrt{-g}\,\nabla^\mu T^{g}_{\mu\nu}+\sqrt{-f}\,\tilde{\nabla}^\mu T^{f}_{\mu\nu}=0,
\eeqn
meaning that in bimetric gravity the two source contributions are not forced to be separately conserved by the equations. 
Nevertheless, we shall always assume their separate conservation, that is $\nabla^\mu T^{g}_{\mu\nu}=\tilde{\nabla}^\mu T^{f}_{\mu\nu}=0$. This is equivalent to imposing the separate invariance of the two matter Lagrangians $\mathcal{L}^g_\mathrm{m}$ and $\mathcal{L}^f_\mathrm{m}$ under diffeomorphisms, which appears to be a natural requirement.
In this case, the equations of motion for $\gmn$ then give rise to $d$ Bianchi constraints,
\beqn\label{Bianchi}
\nabla^\mu \sum_{n=0}^{d-1}(-1)^n\beta_n \,g_{\mu\lambda}{(Y^{(n)})^\lambda}_{\nu}(S)&=&0\,.
\eeqn 
Accordingly, there is a set of similar constraints arising from the $\fmn$ equation which, as a consequence of the identity (\ref{bicog}), is equivalent to (\ref{Bianchi}). In summary, under the assumption of separate covariant conservation of the stress-energy tensors, the equations of motion contain $d$ constraints~(\ref{Bianchi}) following from diffeomorphism invariance.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Massive Gravity limit}\label{sec:MGlim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

An intriguing question is whether there exist a limit in the Hassan-Rosen theory in which one of the metrics decouples and the remaining metric describes a massive excitation. It turns out that this is indeed possible, but as always the exact limit needs to be treated with care. Massive Gravity limits of bimetric gravity have been studied in~\cite{Baccetti:2012bk}, where it was shown that only one of two possible limiting procedures leads to a nontrivial theory.

Consider again the nonlinear equations of motion (\ref{geq}) and (\ref{feq}) for $\gmn$ and $\fmn$, respectively. In these we now take the following limit,
\beqn\label{mglimit}
\frac{m_f}{M}\rightarrow \infty\,,\qquad \beta_d\rightarrow \infty\,,\qquad \text{such~that}\quad \frac{\beta_dM}{m_f}=\text{const.}
\eeqn
Here, $M$ denotes any other mass scale in the theory, such as $m_g$, $m$ and the energy scale of the sources. Provided that the $\beta_n$ parameters are independent of $m_f/M$, then the equations of motion in this limit reduce to
\begin{align}
\mathcal{G}_{\mu\nu}(g)
+\tfrac{m^d}{m_g^{d-2}}\sum_{n=0}^{d-1}(-1)^n\beta_n \,g_{\mu\lambda}{(Y^{(n)})^\lambda}_{\nu}(S)=\tfrac{1}{m_g^{d-2}}T^{g}_{\mu\nu}\,, \label{gdrgt} \\
\mathcal{G}_{\mu\nu}(f)
+\Lambda\fmn=0 \,,\label{fdrgt}
\end{align}
where $\Lambda\equiv{\beta_d\,m^d}/{m_f^{d-2}}$. The equation for $\gmn$ is unaltered, while the equation for $\fmn$ decouples and simply becomes an ordinary Einstein equation with cosmological constant $\Lambda$. Hence, the solution for $\fmn$ will be an Einstein metric which can be plugged into the $\gmn$ equation. The resulting equation for $\gmn$ is exactly the same as in the nonlinear Massive Gravity where the auxiliary metric $\fmn$ is fixed to be an Einstein metric. Note, however, that it is not possible to derive the equations (\ref{gdrgt}) and (\ref{gdrgt}) from an action principle. 
One may therefore think that a more natural limit would be given by $m_f/M\rightarrow 0$ which could directly be taken in the bimetric action. However, it is quite easy to see that in this limit the equations of motion admit only GR solutions for $\gmn$~\cite{Baccetti:2012bk}.

Another important observation is that, as long as the above limit~(\ref{mglimit}) is not taken exactly, the bimetric equations of motion always force both metrics to be Einstein solutions if one of them is. This follows, for example, from the perturbative solutions that we obtain in chapter~\ref{ch:HD} and can also be shown explicitly for certain parameter choices. Therefore the Massive Gravity limit is a singular point in parameter space, where an important relation among the two metrics is lost.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
\section{Mass spectrum}\label{sec:massspec}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

From the nonlinear ADM analysis of \cite{Hassan:2011zd} it is known that ghost-free bimetric theory propgates $(d(d-2)-1)$ degrees of freedom. At the linear level around a certain class of backgrounds, these can be attributed to a massless and massive fluctuation. Around general backgrounds or at the nonlinear level, however, such a split is usually not well-defined. In {\protect{\hyperref[papV]{Paper V}}} we identify the backgrounds suitable for discussing the theory's mass spectrum in four dimensions. Then we perturb around these backgrounds and show how to diagonalize the fluctuations into modes with definite mass. {\protect{\hyperref[papVII]{Paper VII}}} generalizes these findings to an arbitrary number of space-time dimensions. Both papers also discuss possible nonlinear extensions of mass eigenstates, a topic which we leave for the next section.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Proportional backgrounds}\label{secpropbg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

A simple, yet very important class of solutions to the bimetric equations of motion is obtained by making an ansatz that conformally relates the two metrics, $\bfmn=c(x)^2\bgmn$, where $c(x)$ is a space-time dependent function. Having plugged this ansatz into the equations of motion, we first note that the Bianchi constraint~(\ref{Bianchi}) immediately enforces $\partial_\mu c(x)=0$ and hence $c(x)=$\,const. This restricts our ansatz to proportional metrics,
\beqn
\bfmn=c^2\bgmn\qquad \text{with}\quad c=\mathrm{const.}
\eeqn
Using this in (\ref{geq}) and (\ref{feq}) we find that the equations of motion simply reduce to two copies of Einstein's equations,
\begin{align}\label{bgeq}
\mathcal{G}_{\mu\nu}(\bar{g})
+\Lambda_g\bgmn=\frac{1}{m_g^{d-2}}\bar{T}^{g}_{\mu\nu}\,, \quad
\mathcal{G}_{\mu\nu}(\bar{g})
+\Lambda_f\bgmn=\frac{1}{m_f^{d-2}}\bar{T}^{f}_{\mu\nu} \,.
\end{align}
In this we have defined the cosmological constant contributions arising from the interaction potential,
\beqn\label{lambdas}
\Lambda_g&\equiv&\frac{m^d}{m_g^{d-2}}\sum_{n=0}^{d-1}{d-1\choose n}c^n\beta_n\,,\nn\\
\Lambda_f&\equiv&\frac{m^d}{(m_f c)^{d-2}}\sum_{n=1}^{d}{d-1\choose n-1}c^n\beta_n\,,
\eeqn
Proportional backgrounds thus simply correspond to solutions to Einstein's equations in General Relativity.
After all constant contributions in the stress-energy tensors have been shifted into $\Lambda_g$ and $\Lambda_f$, respectively,\footnote{This can always be achieved by redefining $\beta_0$ and $\beta_d$.} the difference of the above background equations implies that
\beqn\label{propbackeq}
\Lambda_g=\Lambda_f\,,\qquad
\bar{T}^{f}_{\mu\nu}=\alpha^{d-2}\bar{T}^{g}_{\mu\nu}\,,~~~~~\text{where}~~\alpha\equiv \frac{m_f}{m_g}\,.
\eeqn
From (\ref{lambdas}) it is clear that the first equation relating the cosmological constants is a polynomial in $c$ with coefficients depending on the $\beta_n$ parameters. In general, this equation serves to determine the proportionality constant $c$ of our ansatz in terms of the parameters of the theory and thereby specifies the solution completely. An important exception to this generic situation is the partially massless case, to be introduced in chapter~\ref{ch:PM}.  

The second equation in (\ref{propbackeq}) that relates the sources for the two metrics is very constraining. From a phenomenological point of view, there is no reason to believe that the matter sources satisfy such a strong constraint. Proportional background solutions, however, only exist in this case. Since any deviation from the proportional backgrounds constitutes a deviation from GR solutions, the difference in the source terms may be regarded as a measure for the difference of bimetric solutions from those of GR. 
 
The proportional background solutions are of particular interest because they allow for a definite mass spectrum of fluctuations around them. In general, the linear perturbation equations have a rather complicated structure because in order to derive them one needs to vary the square-root matrix $S=\sqrt{g^{-1}f}$. This is always possible but, for backgrounds giving rise to matrices $\bar{g}^{-1}\bar{f}$ that do not commute with the fluctuations, the resulting expressions are lengthy and not illuminating. In particular, the equations will not contain a mass term with Fierz-Pauli structure which makes it difficult to identify the massive field. In contrast, for the proportional backgrounds we have $\bar{g}^{-1}\bar{f}=c^2\mathbb{1}$ which does commute with any other matrix and hence drastically simplifies the perturbation equations which now will exhibit the Fierz-Pauli structure. Moreover, in the absence of sources, these backgrounds correspond to maximally symmetric ones for which the concept of mass as a label of representations of the underlying isometry group is well-defined. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsection{Linear perturbations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

We shall now consider small perturbations around the proportional backgrounds for both of the metrics as well as the sources,
\beqn
\gmn&=&\bgmn+\dg_{\mu\nu}\,,\qquad \fmn~=~c^2\bgmn+\df_{\mu\nu}\,,\nn\\
T^{g}_{\mu\nu}&=&\bar{T}^{g}_{\mu\nu}+\delta T^{g}_{\mu\nu}\,,\qquad T^{f}_{\mu\nu}~=~\alpha^{d-2}\bar{T}^{g}_{\mu\nu}+\delta T^{f}_{\mu\nu}\,.
\eeqn
In the following we set the background values of the sources to zero, $\bar{T}^{g}_{\mu\nu}=0$. In {\protect{\hyperref[papV]{Paper V}}} we keep them in the equations, which modifies the structure of the kinetic operator (\ref{kinopds}) below. As a consequence, the coupling of the fluctuations to the cosmological constant term assumes a less familiar form, which is our main motivation to present the equations without background sources here. Note however that their inclusion does not alter any of the results.


As stated earlier, around the proportional backgrounds the linearized equations of motion can be diagonalized into an equation for a massless and a massive perturbation. To this end, consider the following redefinitions of fluctuations,
\beqn\label{dGanddM}
\delta G_{\mu\nu} &\equiv&\left[1+(\alpha c )^{d-2}\right]^{\frac{4-d}{d-2}}\big(\dg_{\mu\nu}+c^{d-4}\alpha^{d-2}\df_{\mu\nu}\big)\,,\nn\\
\delta M_{\mu\nu} &\equiv& \frac{1}{2c}\big(\df_{\mu\nu}-c^2 \dg_{\mu\nu}\big)\,,
\eeqn
in which the overall normalizations have been chosen conveniently. Now, taking the appropriate linear combinations of the original fluctuation equations for $\delta\gmn$ and $\delta\fmn$ decouples the massless from the massive mode. The resulting equations read
\begin{align}
{\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}\delta G_{\rho\sigma}&-\tfrac{2}{d-2}\bar{\Lambda}_g\left(\delta G_{\mu\nu}-\tfrac{1}{2}\bar{G}_{\mu\nu}\delta G\right) \nn\\
& \hspace{75pt}=\left(\tfrac{1}{m_g}\right)^{\frac{d-2}{2}}\left(\delta T^g_{\mu\nu}+c^{d-2}\delta T^f_{\mu\nu}\right)\,, \label{dGeq}\\
{\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}\delta M_{\rho\sigma}&-\tfrac{2}{d-2}\bar{\Lambda}_g\left(\delta M_{\mu\nu}-\tfrac{1}{2}\bar{G}_{\mu\nu}\delta M\right)
+\tfrac{\bar{m}^2_\mathrm{FP}}{2}\Big(\delta M_{\mu\nu}-\bgmn\delta M\Big)\nn\\
& \hspace{75pt}=\left(\tfrac{c}{m_f}\right)^{\frac{d-2}{2}}\left(\delta T^f_{\mu\nu}-\alpha^{d-2}\delta T^g_{\mu\nu}\right)\,.\label{dMeq}
\end{align}
Here, the traces of the fluctuations are taken with respect to a redefined background metric, 
\beqn
\bar{G}_{\mu\nu}\equiv \big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}\bgmn\,,
\eeqn
that is $\delta G=\bar{G}^{\mu\nu}\delta G_{\mu\nu}$ and $\delta M=\bar{G}^{\mu\nu}\delta M_{\mu\nu}$. Also, we have redefined the cosmological constant with respect to this background,
\beqn
\bar{\Lambda}_g\equiv \big(1+(\alpha c)^2\big)^{-\frac{2}{d-2}} \Lambda_g  \,, \qquad R_{\mu\nu}(\bar{G})=\frac{2\bar{\Lambda}_g}{d-2}\bar{G}_{\mu\nu}\,.
\eeqn
Furthermore, the kinetic operator ${\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}$ with respect to the $\bar{G}_{\mu\nu}$ background is defined as
\begin{align}\label{kinopds}
\bar{\mathcal{E}}^{\rho\sigma}_{\mu\nu}\delta G_{\rho\sigma} 
=-\tfrac{1}{2}\Big[\delta^\rho_\mu\delta^\sigma_\nu\bar{\nabla}^2
&+\bar G^{\rho\sigma}\bar{\nabla}_\mu\bar{\nabla}_\nu 
-\delta^\rho_\mu\bar{\nabla}^\sigma\bar{\nabla}_\nu
-\delta^\rho_\nu\bar{\nabla}^\sigma\bar{\nabla}_\mu \nn\\
&-\bar{G}_{\mu\nu}\bar G^{\rho\sigma}\bar{\nabla}^2 
+\bar{G}_{\mu\nu}\bar{\nabla}^\rho\bar{\nabla}^\sigma\Big]\delta G_{\rho\sigma}\,,
\end{align}
in which $\bar{\nabla}$ is the covariant derivative compatible with $\bar{G}_{\mu\nu}$. Finally, the Fierz-Pauli mass is given in terms of the parameters of the theory through
\beqn\label{FPmass}
\bar{m}^2_\mathrm{FP}=\frac{m^d}{m_g^{d-2}} \big(1+(\alpha c)^2\big)^{-\frac{2}{d-2}}\left(1+(\alpha c)^{2-d}\right)\sum_{n=1}^{d-1}{d-2\choose n-1}c^n\beta_n\,.
\eeqn
Recall that in the above expressions $c$ is to be regarded as a function of the Planck masses and the $\beta_n$ parameters, determined by the background equation $\Lambda_g=\Lambda_f$. At this stage, the main reason for choosing the new background $\bar{G}_{\mu\nu}$ is to render the equations as simple as possible. However, as our notation already indicates, $\bar{G}_{\mu\nu}$ will also turn out to be the background of the nonlinear massless field that we identify below. Alternatively, we could have written the equations with respect to the original background $\bgmn$, in terms of $\Lambda_g$ and a properly rescaled Fierz-Pauli mass, $m^2_\mathrm{FP}\equiv \big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}\bar{m}^2_\mathrm{FP}$. In addition, there would be a factor of $\big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}$ in front of the source terms, modifying the effective Planck masses of the theory. In {\protect{\hyperref[papV]{Paper V}}} (and also in {\protect{\hyperref[papVI]{Paper VI}}}) we use $\bgmn$ as the background metric, whereas in {\protect{\hyperref[papVII]{Paper VII}}} we express the equations in terms of $\bar{G}_{\mu\nu}$. 

As promised, (\ref{dGeq}) and (\ref{dMeq}), respectively,  describe a massless and a massive spin-2 fluctuation in (Anti-) de Sitter background. At the linear level around proportional backgrounds, one can therefore assign $d(d-3)/2$ degrees of freedom to a massless fluctuation $\delta G_{\mu\nu}$ and the remaining $(d(d-1)/2-1)$ ones to a massive fluctuation $\delta M_{\mu\nu}$.

Observe that in the limit of small $\alpha$ (which is the limit opposite to the massive gravity limit discussed in section~\ref{sec:MGlim}), we have that $\delta G_{\mu\nu}\sim\delta \gmn$ and hence the fluctuation for the metric $\gmn$ becomes mostly massless. This is important because, at least to our present knowledge, only the couplings of the original metrics to matter are ghost-free, whereas on the other hand the gravitational metric needs to be mostly massless for phenomenological reasons. Fortunately, the limit in which the perturbation of $\gmn$ is dominated by the massless mode corresponds to a large Planck mass $m_g$, which is required for having a weak gravitational force anyway. We will come back to this point when discussing the nonlinear extension of the massless field below.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
\section{Nonlinear extensions of mass eigenstates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

In the previous section, we saw that the fluctuations of $\gmn$ and $\fmn$ around proportional backgrounds are not mass eigenstates, whereas certain linear combinations of them do satisfy the equations for massless and massive spin-2 fields. We now turn to the derivation of nonlinear fields  $G_{\mu\nu}$ and $M^G_{\mu\nu}$ that, when linearized around the proportional background solutions, give rise to these massless and massive perturbations. Having obtained expressions for these we are also able to address the question whether it is possible to couple the massless field to matter without reintroducing the Boulware-Deser ghost.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
\subsection{Identifying the nonlinear fields}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

In the following we will see that, as may have been anticipated, there are infinitely many possibilities to define nonlinear fields with massless or massive fluctuations around the proportional backgrounds. In {\protect{\hyperref[papVI]{Paper VI}}} and {\protect{\hyperref[papVII]{Paper VII}}}, we therefore invoke additional criteria of simplicity and invertibility which allow us to single out unique nonlinear extensions of the linear mass eigenstates.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsubsection{The massless field}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

General covariance implies that the most general ansatz for the nonlinear field $G_{\mu\nu}$ with massless fluctuation around proportional backgrounds is of the form
\beqn\label{ansatzG}
G_{\mu\nu}=g_{\mu\rho}{\Phi^\rho}_\nu(S)\,.
\eeqn
Here, ${\Phi^\rho}_\nu(S)$ is an arbitrary matrix-valued function of the square-root matrix $S=\sqrt{g^{-1}f}$. The transposed matrix $S^\mathrm{T}$ does not appear in the ansatz due to the symmetry property $gS=S^\mathrm{T}g$. Now, on the proportional backgrounds, any function of $S$ is proportional to the unit matrix and hence $\Phi(\bar{S})\equiv\phi( c)\mathbb{1}$, where $\phi( c)$ is just a scalar function of $c$. With (\ref{ansatzG}) the fluctuation of $G_{\mu\nu}$ can thus be written as
\beqn
\delta G_{\mu\nu}=\phi( c)\delta g_{\mu\nu}+\bar{g}_{\mu\rho}\left.\frac{\delta {\Phi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}\delta {S^\alpha}_\beta\,.
\eeqn
Using the variation of the square root around proportional backgrounds,
\beqn\label{sfluc}
\delta {S^\alpha}_\beta=\frac{1}{2c}\bar{g}^{\alpha\lambda}(\delta f_{\lambda\beta}-c^2\delta g_{\lambda\beta})\,,
\eeqn
we can compare this expression to the definition of the massless fluctuation in~(\ref{dGanddM}). This gives
\beqn
\phi(s)&=&\big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}\,,\nn\\
 \left.\frac{\delta {\Phi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}&=& 2\left[1+(\alpha c )^{d-2}\right]^{\frac{4-d}{d-2}}c^{d-3}\alpha^{d-2}\delta^\rho_\alpha\delta^\nu_\beta\,.
\eeqn
These constraints on the matrix function ${\Phi^\rho}_\nu(S)$ have an infinite number of solutions given through power series of the matrix $S$ with mildly constrained coefficients. We present their general form in the case of four space-time dimensions in {\protect{\hyperref[papV]{Paper V}}}. From all of these possible definitions for the nonlinear massless field we choose the one that gives the simplest invertible relation to the original variables $\gmn$ and $\fmn$. This particular choice corresponds to
\beqn\label{defG}
G_{\mu\nu} = \left[1+(\alpha c )^{d-2}\right]^{\frac{4-d}{d-2}}\big(g_{\mu\nu}+c^{d-4}\alpha^{d-2}f_{\mu\nu}\big)\,.
\eeqn
Remarkably, it turns out to be simply a linear combination of the original metrics.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsubsection{The massive field}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to identify a nonlinear extension of the massive fluctuation, we make an ansatz similar to the one for the massless field above,
\beqn\label{ansatzM}
M_{\mu\nu}=g_{\mu\rho}{\Psi^\rho}_\nu(S)\,,
\eeqn
where ${\Psi^\rho}_\nu(S)$ is an arbitrary matrix-valued function of the square-root matrix ${S^\mu}_\nu$. Again, on the background we have $\Psi(\bar{S})=\psi( c)\mathbb{1}$ with $\psi( c)$ being a scalar function. The variation of the ansatz therefore reads
\beqn
\delta M_{\mu\nu}=\psi( c)\delta g_{\mu\nu}+\bar{g}_{\mu\rho}\left.\frac{\delta {\Psi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}\delta {S^\alpha}_\beta\,.
\eeqn
Comparing this to the definition of the massive fluctuation in (\ref{dGanddM}), we see that
\beqn\label{constdm}
\psi( c)=0\,,\qquad \left.\frac{\delta {\Psi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}=\delta^\rho_\alpha\delta^\beta_\nu\,. 
\eeqn
As in the massless case, there are infinitely many solutions to these constraints whose general form is provided in {\protect{\hyperref[papV]{Paper V}}} for $d=4$.
In order to single out a nonlinear extension of the massive fluctuation, we first observe that the interaction potential in the action is a polynomial in the square-root matrix ${S^\mu}_\nu$. Moreover, as can be seen by comparing~(\ref{dGanddM}) and~(\ref{sfluc}), the variation of this matrix gives the massive fluctuation up to normalization. However, ${S^\mu}_\nu$ is a (1,1)-tensor which furthermore satisfies the symmetry property $G_{\rho\mu}{S^\mu}_\nu=G_{\nu\mu}{S^\mu}_\rho$ and can therefore not be regarded as independent of the massless field. We would like the massive field to be a (0,2)-tensor that is independent of $G_{\mu\nu}$. On the other hand, lowering an index ${S^\mu}_\nu$ with $G_{\mu\nu}$ modifies the expression of its variation in terms of $\delta\gmn$ and $\delta\fmn$. According to (\ref{constdm}), in oder to obtain the massive fluctuation in~(\ref{dGanddM}) we must subtract the field's background value. 
Hence, our choice for the nonlinear massive fields is given by
\beqn
M^G_{\mu\nu} \equiv \left[1+(\alpha c )^{d-2}\right]^{-\frac{2}{d-2}}\left(G_{\mu\rho} {S^\rho}_\sigma-cG_{\mu\nu}\right)\,.
\eeqn
The reader is reminded once again that in this definition (and in the one for the massless field above), $c$ is a function of the $\beta_n$ parameters obtained by setting $\Lambda_g=\Lambda_f$.

In the next section it will be shown that the massless field $G_{\mu\nu}$, as defined in~(\ref{defG}), cannot consistently couple to matter sources. It is therefore not a suitable candidate for the gravitational metric and rewriting the bimetric theory in terms of $G_{\mu\nu}$ and $M^G_{\mu\nu}$ is probably not useful for phenomenological purposes. On the other hand, $\gmn$ can couple to matter without introducing inconsistencies and a formulation of the theory in terms of $\gmn$ and a corresponding massive field $M_{\mu\nu}$ may be of use for applications. A definition for this new field $M_{\mu\nu}$ which can be considered as independent of $\gmn$ while being compatible with (\ref{constdm}) is
\beqn\label{defMg}
M_{\mu\nu} \equiv g_{\mu\rho} {S^\rho}_\sigma-cg_{\mu\nu}\,.
\eeqn
A particular feature, shared by all possible definitions of the nonlinear massive fields, is that their background value vanishes on the proportional backgrounds. Because these backgrounds precisely corresponds to GR solutions, a nonzero background value for the nonlinear massive field is a measure for deviations of bimetric theory from General Relativity.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Inconsistency of coupling the massless field to matter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   

Astrophysical observations show that the mass of the graviton cannot be larger than the Hubble scale $\sim 10^{-33}$eV. A massless gravitational metric would therefore be favoured from a phenomenological point of view. Having obtained an expression for a nonlinear massless spin-2 field in the bimetric setup, we are therefore interested in the question whether this field could consistently be coupled to matter alone and hence represent the gravitational metric.
This motivates an ADM analysis of interactions between the massless field $G_{\mu\nu}$ and matter sources. To this end, consider the addition of a standard minimal matter coupling of the form
\beqn\label{mmcoup}
S^G_\mathrm{m}=\int \dd^d x~\sqrt{-G}\,\mathcal{L}^G_\mathrm{m}
\eeqn 
to the bimetric action. Since the Hamiltonian analysis of the latter has been performed in the original formulation of the theory, the simplest route to follow is to use the definition (\ref{defG}) of the massless field to obtain its ADM variables as functions of the ADM variables of $\gmn$ and $\fmn$. In fact, since constant factors are not of interest in the ADM analysis, we can simply rescale the metrics such that we have $G_{\mu\nu}=\gmn'+\fmn'$, where $\gmn'$ and $\fmn'$ possess ADM decompositions as in (\ref{admmetr}) and (\ref{admf}), respectively.
That is to say, we define 
\beqn
G_{\mu\nu}=\begin{pmatrix}
-K^2+K_m\Gamma^{mn}K_n&K_j\\ K_i & \Gamma_{ij}
\end{pmatrix}\,,
\eeqn
whose components obey
\beqn\label{ADMG}
K_i&=&N_i+L_i\,,\qquad \Gamma_{ij}~=~\gamma_{ij}+\tilde{f}_{ij}\,,\nn\\
K^2&=&N^2+L^2+\Gamma^{ij}K_iK_j-\gamma_{ij}N^iN^j-\tilde{f}_{ij}L^iL^j\,.
\eeqn
In these, the shift $N_i$ of $\gmn$ should be understood as a function of the other ADM variables and the redefined shift vectors $n_i$, according to~(\ref{shiftred}).  
After this redefinition the bimetric action is linear in the lapses $N$ and $L$ of $\gmn$ and $\fmn$ as well as the shift $L_i$ of $\fmn$. In order not to reintroduce the Boulware-Deser ghosts and maintain diffeomorphism invariance, the coupling (\ref{mmcoup}) must also be linear in these variables. 
On the other hand, since we take the couplings (\ref{mmcoup}) to resemble those of the metric in General Relativity, we know that due to general covariance of GR they have to be linear in the lapse $K$ and shift $K_i$ of $G_{\mu\nu}$.\footnote{For instance, this can explicitly be verified for the standard coupling of a massless scalar field, $\mathcal{L}^G_\mathrm{m}=G^{\mu\nu}\partial_\mu\phi\partial_\nu\phi$.} But from~(\ref{ADMG}) it is clear that the lapse $K$ is a nonlinear function of $N$, $L$ and $L^i$. In order to demonstrate the consistency bimetric action without matter coupling, so far we have only redefined $N_i$. We therefore still have the freedom to perform a redefinition of $L_i$ which possibly could render the expression for $K$ linear in $N$, $L$ and $L^i$. However, as we will now argue, such a redefintion does not exist. To see this, rewrite the above expression for~$K^2$ as
\beqn\label{defk2} 
K^2=N^2+L^2+(N^i-L^i) (\gamma_{ij}-\gamma_{ik} \Gamma^{kl} \gamma_{lj}) (N^j-L^j)  \,.
\eeqn
The redefinition of $L^i$ would have to turn the right-hand side of this equation into a perfect square of a function linear in $N$, $L$ and $L^i$. 
But due to the form of the redefinition~(\ref{shiftred}) required by the bimetric interaction potential, we have that 
\beqn 
N^i-L^i=Ln^i-N{D^i}_kn^k\,,
\eeqn
implying that the above expression for $K^2$ does not depend on $L^i$. Consequently, redefining $L^i$ cannot change the fact that $K$ is nonlinear in $N$ and $L$ and hence a coupling term of the form (\ref{mmcoup}) cannot be consistent.


Of course, we have not shown that a massless field in bimetric theory can never couple to matter in a ghost-free manner.
The above proof only applies to standard matter couplings and to the massless field singled out in the previous section. It is possible that other types of couplings or more complicated choices for the field remedy the above conclusion and there exist a way to obtain a massless gravitational metric.\footnote{Another option is to tune the $\beta_n$ parameters such that the Fierz-Pauli mass (\ref{FPmass}) vanishes. In this case, both $\gmn$ and $\fmn$ have massless fluctuations and the graviton could be massless while still interacting nontrivially with another spin-2 field at the nonlinear level.}  




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Massive spin-2 interactions with gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

Owing to the absence of ghost-free matter couplings for the nonlinear massless field, we choose to consider the standard consistent interactions of the metric $\gmn$ with matter sources. In this case, $\gmn$ is the gravitational metric with geometric interpretation. Its fluctuations, however, are neither massless nor massive; they are superpositions of mass eigenstates. Nonetheless, it is still possible to consider a nonlinear version of the massive spin-2 perturbation in this gravitational background. The appropriate nonlinear field which is independent of $\gmn$ is the one given in~(\ref{defMg}). 

In {\protect{\hyperref[papV]{Paper V}}} we rewrite the Hassan-Rosen bimetric action in terms of the variables $\gmn$ and $M_{\mu\nu}$. In the interaction potential, implementing the field redefinition is straightforward,
\beqn
\sum_{n=0}^d\beta_ne_n(S)=\sum_{n=0}^d\beta_ne_n(c\mathbb{1}+g^{-1}M)=\sum_{n=0}^d\alpha_n^ce_n(g^{-1}M)\,.
\eeqn
Here the new parameters $\alpha_n^c$ depend on the original $\beta_n$-parameters in the following way,
\beqn
\alpha^c_n\equiv\sum_{k=n}^d {d-n \choose k-n} c^k\beta_k\,.
\eeqn
The potential is therefore simply a polynomial in $M_{\mu\nu}$. In the kinetic term for $\fmn$ we invoke the curvature relations~(\ref{curvrel}) to rewrite it in terms of $\gmn$-covariant derivatives acting on $M_{\mu\nu}$. For notational simplicity, we present the result in terms of the matrix $S=c\mathbb{1}+g^{-1}M$,
\beqn
\sqrt{-f}\,R(f)=\sqrt{-g}\,(\det S)\left[\phi^{\mu\nu}R_{\mu\nu}(g)+\Pi_{\rho\omega}^{\sigma\pi\alpha\beta}\nabla_\alpha{S^\rho}_\sigma\nabla_\beta{S^\omega}_\pi\right]\,.
\eeqn
Here we have used the abbreviation,
\beqn
\phi^{\mu\nu}\equiv{(S^{-2})^\mu}_\rho g^{\rho\nu}\,,
\eeqn
as well as defined a nonlinear polarization tensor,
\begin{align}
\Pi_{\rho\omega}^{\sigma\pi\alpha\beta}
\equiv\big(2&\phi^{\alpha\mu}\phi^{\kappa\delta}\phi^{\beta\nu}
-2\phi^{\alpha\mu}\phi^{\beta\kappa}\phi^{\delta\nu}
\nn\\
&-\phi^{\alpha\beta}\phi^{\kappa\delta}\phi^{\mu\nu}
+\phi^{\alpha\beta}\phi^{\kappa\mu}\phi^{\delta\nu}\big)
\delta^\sigma_{(\kappa}\delta^\gamma_{\delta)}\,  
\delta^\pi_{(\mu} \delta^\lambda_{\nu)}\, S_{\gamma\rho}\,
S_{\lambda\omega}. 
\end{align}
Collecting all the terms we arrive at the nonlinear action for a massive spin-2 field $M_{\mu\nu}$ in a gravitational background $\gmn$,
\begin{align}\label{sp2gr}
&S_{M,g}~=~m_g^{d-2}\int\dd^d x~\sqrt{-g}\,R(g) +\int\dd^d x~\sqrt{-g}\,\mathcal{L}^g_\mathrm{m}\nn\\
&~+~m_f^{d-2}\int\dd^d x~\sqrt{-g}\,(\det S)\left[\phi^{\mu\nu}R_{\mu\nu}(g)+\Pi_{\rho\omega}^{\sigma\pi\alpha\beta}\nabla_\alpha{S^\rho}_\sigma\nabla_\beta{S^\omega}_\pi\right] \nn\\
&~-~2m^d\int\dd^dx~\sqrt{-g}\,\sum_{n=0}^d\alpha_n^ce_n(g^{-1}M)\,.
\end{align}
While in the bimetric formulation of the theory in terms of $\gmn$ and $\fmn$ the kinetic terms are diagonal, the massive spin-2 field shows highly nontrivial kinetic mixing with the gravitational metric. Moreover, as already stated above, $\gmn$ does not give rise to a massless fluctuation around maximally symmetric backgrounds, which could endanger the compatibility of the theory with observations. However, we also already observed that gravity becomes essentially massless in the limit where its interactions are weak, $m_g/m_f\rightarrow \infty$. Hence, although the presence of a massive spin-2 field always implies that the graviton is a superposition of mass eigenstates, the effects of this mixing are expected to be small due to the weakly interacting nature of gravity.

Of course, it is also possible to formulate the theory in terms of the nonlinear fields $G_{\mu\nu}$ and $M^G_{\mu\nu}$. The structure of the resulting action is even more involved than in~(\ref{sp2gr}) and we refrain from presenting it here. Its expression in four space-time dimensions can be found in {\protect{\hyperref[papV]{Paper V}}}.

From the consistent matter couplings in the original bimetric formulation one can furthermore derive ghost-free interactions between the massive spin-2 field $M_{\mu\nu}$ and arbitrary types of matter fields. For interactions with bosonic matter this is straightforwardly realized by making the replacement $\fmn=g_{\mu\alpha}{S^\alpha}_\beta{S^\beta}_\nu$ in the standard matter couplings $\int\dd^dx\, \sqrt{-f}\,\mathcal{L}^f_\mathrm{m}$ for $\fmn$. In {\protect{\hyperref[papV]{Paper V}}} we give an explicit example of coupling $M_{\mu\nu}$ to a massive spin-1 field and also work out the slightly more complicated couplings of the massive spin-2 field to fermions. The latter requires working in the vielbein formulation and making appropriate replacements in the $\gamma^\mu$ matrices as well as the spin connections.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Generalization to Multimetric Theory} 
\label{ch:MV}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Ghost-free bimetric theory describes the interaction of two spin-2 fields, one with massless and one with massive fluctuations around proportional backgrounds. In this section we discuss a generalization of the Hassan-Rosen action to an interacting theory for an arbitrary number of spin-2 fields as introduced in~\cite{Hinterbichler:2012cn}. In general, such a theory will contain one massless spin-2 mode along with many massive ones and, again, one has to ensure the absence of the corresponding Boulware-Deser ghosts. A formulation of the theory in terms of vielbeins turns out to be very convenient for the ghost proof, but reexpressing the consistent multivielbein action in terms of metrics is not entirely trivial.
In {\protect{\hyperref[papIV]{Paper IV}}} we develop a method to rewrite the multivielbein theory of~\cite{Hinterbichler:2012cn} in terms of the corresponding metrics as well as St\"uckelberg fields that take care of local Lorentz invariances. 
We begin the discussion with a demonstration of consistent and inconsistent multimetric couplings before going over to the multivielbein formulation. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multiple bimetric couplings}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

When constructing a theory for more than two spin-2 fields, of course, the main requirement on its structure remains the absence of the Boulware-Deser ghosts. The interaction potential for $\mathcal{N}$ fields therefore has to be chosen such that the action in Hamiltonian formulation gives rise to $(d+\mathcal{N}-1)$ constraints. Out of these,  $d$ should be first class constraints, generating the group of general coordinate transformations, while the remaining $(\mathcal{N}-1)$ are expected to be second class and serve to remove all Boulware-Deser ghosts from the spectrum. 


An obvious way to satisfy these requirements is to simply add up several copies of the Hassan-Rosen action for fields $\fmn$ and $\gmn^{(i)}$ with $i=1,\hdots, \mathcal{N}-1$, to obtain a theory in which one of the metrics coupled to all the others,
\beqn\label{centercoup}
S_\mathrm{center}(f,\{g^{(i)}\})=\sum_{i=1}^{\mathcal{N}-1}S_{\mathrm{HR}}(g^{(i)},f)\,.
\eeqn
This will be consistent because in every interaction potential one can redefine the ADM variables for $\gmn^{(i)}$ to make it linear in the lapse and shift of~$\fmn$ as well as the lapse of $\gmn^{(i)}$, such that one obtains the desired $(d+\mathcal{N}-1)$ constraints. 

The left panel of Figure~4.1 shows how such a coupling can be visualized in a graph~\cite{Hinterbichler:2012cn}. Each solid dot represents a different spin-2 field and the lines stand for standard Hassan-Rosen bimetric couplings between them. Fields corresponding to dots that are not connected by a line do not directly interact. Due to the corresponding picture with one metric in the center, we shall refer to interactions of the form~(\ref{centercoup}) as ``center couplings".

Another option to obtain consistent multiple bimetric interactions is to build a ``chain" of $\mathcal{N}$ coupled spin-2 fields $\gmn^{(k)}$ where $k=1,\hdots,\mathcal{N}$. That is to say, we take an action is of the form,
\beqn
S_\mathrm{chain}(\{g^{(k)}\})=\sum_{k=1}^{\mathcal{N}-1}S_{\mathrm{HR}}(g^{(k)},g^{(k+1)})\,,
\eeqn
for which the corresponding graph is depicted in the right panel of Figure~4.1.
This construction works because in the first term one can redefine the ADM variables for $g^{(1)}$ such that it becomes linear in the lapse and shift of $g^{(2)}$ as well as the lapse of $g^{(1)}$. In the second term one performs a similiar redefinition for the shift of $g^{(2)}$ which, since the redefinition is linear in the lapses, does not destroy the linearity in the lapse of $g^{(2)}$ in the first term. Note however that the second term will no longer be linear in the shift of $g^{(2)}$. Continuing with this procedure in all the terms results in an action that is linear in the lapse and shift of $g^{(\mathcal{N})}$ and in all the other lapses. 



    \begin{figure}[h]
    \begin{center}
    \includegraphics[width=210pt]{Pictures/vbvertex.pdf}
    \caption{The center couplings \textit{(left)} and the chain couplings \textit{(right)}.}
    \end{center}\label{figcentchaint}
    \end{figure}
    
  

In fact, it is also possible to combine the two above constructions in the following manner: First introduce a chain coupling for fields $f^{(k)}$, $k=1,\hdots,\mathcal{K}$, and then to each $f^{(k)}$ attach $I_k$ fields $g_{(k)}^{(i_k)}$, $i_k=1,\hdots\mathcal{I}_k$, in a center coupling. This gives 
\beqn\label{gencv}
S_\mathrm{c-v}~=~S_\mathrm{chain}(\{f^{(k)}\})+\sum_{k=1}^\mathcal{K}S_\mathrm{center}(f^{(k)},\{g_{(k)}^{(i_k)}\})\,.
\eeqn
In this theory the total number of fields is $\mathcal{N}=\mathcal{K}+\sum_{k=1}^\mathcal{K}\mathcal{I}_k$. An example for a graph is shown in the left panel of Figure~4.2.
  \begin{figure}[h]
    \begin{center}$
    \begin{array}{cc}
    \includegraphics[width=140pt]{Pictures/vbchainvertex.pdf}~~~~~ & ~~~~~
    \includegraphics[width=45pt]{Pictures/vbloop.pdf}
    \end{array}$
    \caption{The combined chain and center couplings \textit{(left)} and a forbidden loop coupling \textit{(right)}.}
    \end{center}
    \end{figure}
Note that the action~$S_\mathrm{c-v}$ still consists purely of multiple copies of the Hassan-Rosen bimetric action; we have not introduced any type of new interaction term. 
Of course, in the above construction, it is also possible to add further center couplings to each of the $g_{(k)}^{(i_k)}$.
However, it is important to realize that not all possible bimetric couplings are allowed. In particular, one may not couple the metrics in a ``loop", which means adding terms such as $S_{\mathrm{HR}}(f^{(k)},f^{(k+2)})$ or $S_{\mathrm{HR}}(f^{(k+1)},g_{(k)}^{(i_k)})$ to (\ref{gencv}). To see why this fails, consider a simple loop coupling among three metrics,
\beqn\label{loopact}
S_\mathrm{loop}(g,f,h)=S_{\mathrm{HR}}(g,f)+ S_{\mathrm{HR}}(f,h)+S_{\mathrm{HR}}(h,g)\,,
\eeqn
whose graph is depicted in the right panel of Figure~4.2.
Now imagine that in the first term one redefines the shift of $g$ to render it linear in the lapse and shift of $f$ and the lapse of $g$. Then, in the second term redefine the shift of $f$ such that the first two terms afterwards are linear in the lapse and shift of $h$ and the lapses of $g$ and $f$. In the third term, one would now have to redefine the shift of $h$, but from the particular form~(\ref{shiftred}) of the redefinition it is clear that afterwards, the action will again contain the original shift variable for $g$ which cannot be expressed in terms of the redefined variables only. Therefore there is at least no obvious consistent redefinition of ADM variables that renders (\ref{loopact}) linear in all the lapses and we conclude that the loop couplings most likely give rise to Boulware-Deser ghosts. This is in agreement with results of a similar analysis performed in~\cite{Nomura:2012xr}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multivielbein couplings}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

So far we have used the earlier results of the bimetric ADM analysis in order to couple several spin-2 fields to each other using only bimetric interactions. Now we would like to address the question whether there exist more general couplings than the bimetric vertex. We introduce graphs for two examples of such $n$-point vertices in Figure~4.3. 
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=150pt]{Pictures/vbmulti1.pdf}
       \caption{A three- and a four-point vertex.}
    \end{center}
    \end{figure}
A priori, such couplings could be very different from the bimetric ones and the ADM analysis has to be redone from the start.

The problem is simplified when working with vielbeins ${E^a}_\mu(I)$, labeled by an index $I=1,\hdots,\mathcal{N}$, instead of the corresponding metrics $g_{\mu\nu}(I)$. The metrics expressed in terms of the vielbeins read
\beqn\label{defvielbein}
g_{\mu\nu}(I)={E^a}_\mu(I)\eta_{ab}{E^b}_\nu(I)\,.
\eeqn 
The vielbeins have a coordinate index $\mu$ as well as a Lorentz index $a$ and the definition of the metric is invariant under local Lorentz transformations.
Their kinetic terms are simply taken to be the Einstein-Hilbert terms $S_\mathrm{EH}(I)$ for the metrics expressed in terms of~${E^a}_\mu(I)$ through~(\ref{defvielbein}).
In~\cite{Hinterbichler:2012cn} it is shown that then the interactions of vielbeins that lead to ghost-free theories are of the form
\begin{align}\label{vielbeinpot}
S_\mathrm{int}&=\frac{m^2}{4}\sum_{\{I\}}\int\dd^dx~T^{I_1\hdots I_d}U_{I_1\hdots I_d}\,,\nn\\
\text{with}~~~~U_{I_1\hdots I_d}&=\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{a_1\hdots a_d}{E^{a_1}}_{\mu_1}(I_1)\hdots{E^{a_d}}_{\mu_d}(I_d)\,,
\end{align}
where $T^{I_1\hdots I_d}$ are coupling constants, and $\tilde{\epsilon}^{\mu_1\hdots\mu_d}$ and $\tilde{\epsilon}_{a_1\hdots a_d}$ are the totally antisymmetric tensor densities with respect to GCT and Lorentz transformations, respectively. The total multivielbein action is then given by
\beqn\label{multac}
S_\mathrm{multi}=\sum_{I=1}^\mathcal{N}S_\mathrm{EH}(I)+S_\mathrm{int}\,.
\eeqn
Note that the antisymmetric structure of (\ref{vielbeinpot}) ensures that there cannot be more than $d$ vielbeins interacting in one vertex. The ghost-free theory therefore gives rise to diagrams of the type displayed in Figure~3.3 with at most $d$ lines ending in one vertex. 
%We will summarize the consistency proof of~\cite{Hinterbichler:2012cn} in section~\ref{secvbghost}. 

A few remarks on degree-of-freedom counting in the vielbein theory are in order. A general vielbein has no symmetry properties and therefore consists of $d^2$ independent components, whereas the corresponding metric is symmetric and thus only $d(d+1)/2$ of its components are independent. This discrepancy can of course be explained by the presence of additional gauge symmetries in the vielbein theory which serve to remove the redundant degrees of freedom. These $d(d-1)/2$ gauge transformations are the local Lorentz transformations ${\Lambda^b}_a(I)$ that act on the upper index of the vielbein ${E^a}_\mu(I)$. A general theory for $\mathcal{N}$ vielbeins ${E^a}_\mu(I)$ will therefore be invariant under $\mathcal{N}$ distinct local Lorentz transformations. Note however that in (\ref{vielbeinpot}), $\mathcal{N}-1$ of the local Lorentz gauges have already been fixed in order to identify the different Lorentz frames for each vielbein with each other and contract all their indices with a common antisymmetric tensor. Only one overall Lorentz invariance is left over. As discussed in~\cite{Hinterbichler:2012cn} and reviewed in {\protect{\hyperref[papIV]{Paper IV}}}, for each vielbein there exist $d(d-1)/2$ combinations of its equations of motion following from (\ref{multac}) that do not contain any derivatives. These read
\beqn\label{constvierb}
\frac{\delta S_\mathrm{int}}{\delta {E^a}_\mu(I)}{E^c}_\mu(I)\eta_{cb}-\frac{\delta S_\mathrm{int}}{\delta {E^b}_\mu(I)}{E^c}_\mu(I)\eta_{ca}=0\,,
\eeqn
and give the correct number of constraints to reduce the number of independent components of each vielbein to $d(d+1)/2$, as expected in a gauge-fixed theory. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Hamiltonian analysis of the vielbein theory}
\label{secvbghost}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Before we come to its metric formulation, we review the ADM analysis of the multivielbein theory as presented in~\cite{Hinterbichler:2012cn}, which proves the absence of the Boulware-Deser ghosts. 
The Hamiltonian analysis is carried out for the vielbein action with interaction potential in its gauge fixed form~(\ref{vielbeinpot}). It makes use of the fact that the vielbein ${E^a}_\mu$ can be decomposed as 
\beqn\label{decvbla}
{E^a}_\mu(I)={\hat{\Lambda}^a}_{~b}(I){\hat{E}^b}_{~\mu}(I)\,,
\eeqn
where ${\hat{\Lambda}^a}_{~b}(I)$ is a Lorentz transformation and ${\hat{E}^b}_{~\mu}(I)$ is a constrained vielbein for which the following ADM parameterization may be chosen,
\beqn\label{ADMvb}
{\hat{E}^b}_{~\mu}(I)=\begin{pmatrix}
N(I)&0\\ {\hat{e}^s}_{~j}(I)N^j(I)&{\hat{e}^s}_{~i}(I)
\end{pmatrix}\,.
\eeqn
At this point it becomes evident why the vielbein formulation significantly simplifies the Hamiltonian analysis: In contrast to the ADM parameterization of the metric, c.f.~(\ref{admmetr}), the expression for the vielbein is itself already linear in lapse and shift. 
When $d$ vielbeins are contracted with the totally antisymmetric $\tilde{\epsilon}$-tensors in~(\ref{vielbeinpot}), the resulting expression will be linear in all ${E^a}_0(I)$, which implies linearity in $N(I)$ and $N^j(I)$. This certainly is a great advantage over the metric formulation because, due to the absence of square root matrices, no redefinition of ADM variables is needed. However, the simplification does not come without a price, because one still has to deal with the Lorentz matrices ${\hat{\Lambda}^a}_{~b}(I)$ and the extra gauge invariances, as we will explain now. 

The parameterization (\ref{ADMvb}) does not fix the gauge completely but is invariant under the residual gauge group of spatial rotations. To the action one should therefore add a term $\lambda^{ab}(I)\mathcal{P}_{ab}(I)$ for each vielbein, where $\lambda^{ab}(I)$ is a Lagrange multiplier and $\mathcal{P}_{ab}(I)$ are the $\mathcal{N}$ first class constraints that generate the residual gauge group of spatial rotations. The explicit expressions for the matrices $\mathcal{P}_{ab}(I)$ are not important to us but we emphasize that they are functions of the spatial vielbeins and there canonical momenta alone.
It also follows that each ${\hat{\Lambda}^a}_{~b}(I)$ can be parameterized by $d-1$ boosts~$p^a(I)$ which, when the decomposition (\ref{decvbla}) is plugged into the interaction potential~(\ref{vielbeinpot}), enter as St\"uckelberg fields. 

Thus, the potential in ADM variables is of the form
\beqn
S_\mathrm{int}=\int\dd^dx~\sum_{I=1}^{\mathcal{N}}\Big(N(I)\mathcal{C}(I)+N^j(I)\mathcal{C}_j(I)\Big)\,,
\eeqn
where the lapse and shift constraints $\mathcal{C}(I)$ and $\mathcal{C}_j(I)$ are functions of the spatial vielbeins ${\hat{e}^s}_{~i}(I)$ and the boosts $p^a(I)$.  When expressed in terms of vielbeins, the ADM form of the Lorentz invariant kinetic terms is similar to~(\ref{gradm}) in the metric theory, and the full action is linear in all~$N(I)$ and~$N^j(I)$.

Recall that the action with potential in its gauge fixed form still possesses one overall local Lorentz invariance. Part of this residual gauge symmetry can now be used to rotate away one of the $p^a(I)$. The remaining boosts can be solved for using $\mathcal{N}-1$ of the $N^j(I)$ equations. In this way all $p^a(I)$ are eliminated from the action. The last shift constraint together with one of the lapse constraints generate general coordinate transformations. The remaining $\mathcal{N}-1$ lapse equations are the secondary constraints that remove the Boulware-Deser ghosts.

The degree-of-freedom counting in the vielbein theory therefore goes as follows: To start with, there are $(d-1)^2$ components in each of the $\mathcal{N}$ spatial vielbeins, along with corresponding $\mathcal{N}(d-1)^2$ canonical momenta. 
The residual overall gauge invariance under spatial rotations gives rise to first class constraint $\sum_I\mathcal{P}_{ab}(I)$ and remove $2\cdot (d-1)(d-2)/2$ degrees of freedom in total. The remaining $\mathcal{N}-1$ spatial Lorentz transformations have been used for gauge fixing and therefore now give rise to second class constraints upon variation with respect to $\lambda^{ab}(I)$. This reduces the phase space by another $2\cdot (\mathcal{N}-1)(d-1)(d-2)/2$ dimensions.
The overall general coordinate transformations again give first class constraints and take away $2d$ variables. Finally, the $\mathcal{N}-1$ lapse constraints are assumed (although not shown) to also give rise to secondary constraints, which then together remove another $2(\mathcal{N}-1)$ degrees of freedom. 
Putting everything together, we find that the dimension of phase space is 
\begin{align}
D_\mathrm{p.s.}=2\cdot (\mathcal{N}-1)\Big(d(d-1)/2-1\Big)+2\cdot d(d-3)/2\,.
\end{align}
This is the correct number of degrees of freedom for describing $\mathcal{N}-1$ massive and one massless spin-2 particle.











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multimetric theory}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Let us briefly outline how this equivalence follows in a theory with only two interacting vielbeins ${E^a}_\mu\equiv{E^a}_\mu(1)$ and ${\bar{E}^a}_\mu\equiv{E^a}_\mu(2)$  (the more general case of multiple two-point interactions is very similar).  As demonstrated in~\cite{Hinterbichler:2012cn}, the equations of motion are solved by vielbeins that satisfy\footnote{There may also be other branches of solutions that lead to a theories which are not equivalent to the bimetric description, see~\cite{deffayet}.}
%\beqn
%{(E^{-1})^\mu}_a{\bar{E}^a}_\nu
%\eeqn  



The structure of (\ref{vielbeinpot}) is reminiscent of the ghost-free bimetric interaction potential (\ref{potantisym}), and for certain choices of $T^{I_1\hdots I_d}$ the vielbein and metric theories are indeed equivalent. More precisely, this is true whenever the interactions consist only of two-point vertices and contain no loops, i.e.~gives rise to the graphs of Figure~3.1. In that case, the constraints~(\ref{constvierb}) give rise to a symmetrization condition on the vielbeins which allows certain combinations of them to be expressed as square root matrices of the type $\sqrt{g^{-1}f}$. This explains why it is possible to have loop interactions in the vielbein theory despite the no-go statement we made about the metric formulation. We will see how this works in more detail below, after we have discussed the general case.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Obtaining a metric formulation}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In {\protect{\hyperref[papIV]{Paper IV}}} we show that it is always possible to reexpress the vielbein theory in terms of the corresponding metrics together with a set of St\"uckelberg fields. The main idea is to move away from the gauge fixed form of the vielbein that lead to the potential~(\ref{vielbeinpot}), and instead consider $\mathcal{N}$ general vielbeins ${e^a}_\mu(I)$ along with $\mathcal{N}$ independent Lorentz frames. 
The ${e^a}_\mu(I)$ are related to the  gauge fixed ${E^a}_\mu(I)$ by a local Lorentz transformation ${\Lambda^a}_b(I)$ through ${E^a}_\mu(I)={\Lambda^a}_b(I){e^b}_\mu(I)$. Since the corresponding metrics are Lorentz invariant, we again have
\beqn\label{defvielbein2}
g_{\mu\nu}(I)={e^a}_\mu(I)\eta_{ab}{e^b}_\nu(I)\,,
\eeqn 
and the kinetic terms are do not involve the local Lorentz matrices. On the other hand, the interaction potential~(\ref{vielbeinpot}) is now given in terms of
\beqn\label{unfixpot}
U_{I_1\hdots I_d}&=\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{a_1\hdots a_d}{\Lambda^{a_1}}_{b_1}{e^{b_1}}_{\mu_1}(I_1)\hdots{\Lambda^{a_d}}_{b_d}{e^{b_d}}_{\mu_d}(I_d)\,.
\eeqn
The local Lorentz matrices ${\Lambda^a}_b(I)$ appear in the action as St\"uckelberg fields\footnote{For recent references that make use of our method of using St\"uckelberg fields to restore the local Lorentz symmetries in multivielbein theory, see \cite{Gabadadze:2013ria, Ondo:2013wka}.} that restore the full set of $\mathcal{N}$ local Lorentz invariances in the theory. Their indices transform in two different frames, namely those of $\tilde{\epsilon}_{a_1\hdots a_d}$ and ${e^b_i}_{\mu_i}(I)$, respectively. The gauge choice that corresponds to~(\ref{vielbeinpot}) is the one in which all ${\Lambda^a}_b(I)$ are equal since in that case the $\tilde{\epsilon}$ contractions reduce them to a factor $\det\Lambda=1$.

The fully gauge invariant potential given in terms of (\ref{unfixpot}) is the starting point for converting the vielbein into a metric theory. The important point is that it allows us to choose any convenient gauge for the vielbeins ${e^a}_{\mu}(I)$, which is of course not possible in its gauge fixed form~(\ref{vielbeinpot}). As we will see now, the freedom of choosing a gauge is essential for the theory being expressible in terms of metrics.

From the gauge invariant form we proceed by identifying the frames of one of the vielbeins, say ${e^b}_{\mu}(1)$, and $\tilde{\epsilon}_{a_1\hdots a_d}$ . Then, due to the invariance of the totally antisymmetric tensor density, we can rewrite (\ref{unfixpot}) as
\beqn\label{newpotga}
U_{I_1\hdots I_d}&=\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{c_1\hdots c_d}{\Lambda^{c_1}}_{b_1}(1,I_1){e^{b_1}}_{\mu_1}(I_1)\hdots{\Lambda^{c_d}}_{b_d}(1,I_d){e^{b_d}}_{\mu_d}(I_d)\,.\nn\\
\eeqn
Here we have defined the combined Lorentz matrices,
\beqn
{\Lambda^{c}}_{b}(1,I)\equiv{(\Lambda^{-1})^c}_a(1){\Lambda^{a}}_{b}(I)\,,
\eeqn
whose indices transform in the frame of ${e^b}_{\mu}(1)$ and ${e^b}_{\mu}(I)$, respectively. Note that ${\Lambda^{c}}_{b}(1,1)=\delta^c_b$ such that there are only $\mathcal{N}-1$ nontrivial matrices. With the interaction potential brought into the form (\ref{newpotga}), we now again pick a gauge for the vielbeins ${e^b}_{\mu}(I)$, $I=2,\hdots,\mathcal{N}$. Namely, we introduce gauge fixed vielbeins ${\overline{e}^a}_{\rho}(I)$ that satisfy the following symmetry condition,
\beqn
{\overline{e}^b}_{\rho}(I){(e^{-1})^\rho}_c(1)\eta^{ca}={\overline{e}^a}_\rho(I){(e^{-1})^\rho}_c(1)\eta^{cb}\,.
\eeqn
This is sometimes referred to as the Deser-van-Nieuwenhuizen gauge.\footnote{It has been argued in \cite{Deffayet:2012zc} that it might not always be possible to choose this gauge in general. For instance, in four space-time dimensions it requires the existence of the square root matrix $\sqrt{g^{-1}(1)g(I)}$.}
In particular, it again identifies all of the Lorentz frames with that of ${e^a}_{\mu}(1)$. In this specific frame one then has
\begin{align}
g^{\mu\rho}(1)g_{\rho\nu}(I)&={(e^{-1})^\mu}_a(1){\overline{e}^b}_{\rho}(I){(e^{-1})^\rho}_c(1)\eta^{ca}\eta_{bd}{\overline{e}^d}_{\nu}(I)\nn\\
&={(e^{-1})^\mu}_a(1){\overline{e}^a}_\mu(I){(e^{-1})^\mu}_c(1){\overline{e}^c}_{\nu}(I)\nn\\
&=\left(\left[e^{-1}(1)\overline{e}(I)\right]^2\right)^\mu_{~\rho}\,,
\end{align}
or, equivalently, in matrix notation,
\beqn
\sqrt{g^{-1}(1)g(I)}=e^{-1}(1)\overline{e}(I)\,.
\eeqn
Using ${\overline{e}(I)^a}_\mu$ in (\ref{newpotga}) as well as the identity
\beqn
\tilde{\epsilon}_{c_1\hdots c_d}=\sqrt{-\det g(1)}\,\tilde{\epsilon}_{\nu_1\hdots \nu_d}{(e^{-1})^{\nu_1}}_{c_1}(1)\hdots{(e^{-1})^{\nu_d}}_{c_d}(1)\,,
\eeqn
we can finally express the gauge invariant potential as 
\begin{align}\label{metrexp}
U_{I_1\hdots I_d}
=\sqrt{-\det g(1)}\,&\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{\nu_1\hdots \nu_d}
{L^{\nu_1}}_{\lambda_1}(I_1)\left[\sqrt{g^{-1}(1)g(I_1)}\right]^{\lambda_1}_{~\mu_1}\hdots \nn\\
&\hdots{L^{\nu_d}}_{\lambda_d}(I_d)\left[\sqrt{g^{-1}(1)g(I_d)}\right]^{\lambda_d}_{~\mu_d}\,.
\end{align}
Here we have defined new St\"uckelberg fields with coordinate indices,
\beqn
{L^{\nu}}_{\lambda}(I)\equiv{(e^{-1})^{\nu}}_{a}(1){\Lambda^{a}}_{b}(1,I){e^b}_{\lambda}(1)\,.
\eeqn
Equation~(\ref{metrexp}) is the metric expression for the multivielbein theory of~\cite{Hinterbichler:2012cn}. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The ${L^{\nu}}_{\lambda}(I)$ equations.}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Varying the multivielbein action~(\ref{multac}) with interaction potential~(\ref{metrexp}) with respect to the ${L^{\nu}}_{\lambda}(I)$ gives $d(d-1)/2$ constraint equations for each~$I=2,\hdots,\mathcal{N}$, that can be used to eliminate the St\"uckelberg fields from the action. These equations replace the constraints~(\ref{constvierb}) that arose in the gauge fixed version of the theory. 

When trying to solve the ${L^{\nu}}_{\lambda}(I)$ equations for Lorentz degrees of freedom, one encounters a subtlety. Namely, the conditions that follow from the invariance of $\eta_{ab}$ under Lorentz transformations and reduce the number of independent components in ${L^{\nu}}_{\lambda}(I)$ to $d(d-1)/2$ read 
\beqn
{(L^\mathrm{T})_\mu}^\rho(I)g_{\rho\sigma}(1){L^\sigma}_\nu(I)=g_{\mu\nu}(1)\,,
\eeqn 
which imply that ${L^{\nu}}_{\lambda}(I)$ depends on the metric $\gmn(1)$. In order to extract the metric independent part, we therefore use the Caley transform of a Lorentz transformation to express the St\"uckelberg fields in terms of antisymmetric matrices $A_{\mu\nu}(I)$,
\beqn
{L^{\nu}}_{\lambda}(I)=\Big(\big[g(1)+A(I)\big]^{-1}\big[g(1)-A(I)\big]\Big)^\mu_{~\nu}\,.
\eeqn
Since the antisymmetry condition on $A_{\mu\nu}(I)$ is completely independent of the metric $\gmn(1)$, we can parameterize the gauge degrees of freedom in terms of its components.
The equations for the $A_{\rho\sigma}(I)$ are then obtained from
\beqn
\frac{\delta S_\mathrm{multi}}{\delta A_{\rho\sigma}(I)}=\frac{\delta {L^{\mu}}_{\nu}(I)}{\delta A_{\rho\sigma}(I)}\frac{\delta S_\mathrm{int}}{\delta {L^{\mu}}_{\nu}(I)}=0 \,.
\eeqn
Multiplying by $(g(1)-A(I))_{\rho\alpha}(g(1)-A(I))_{\sigma\beta}$ and evaluating the first factor results in
\beqn\label{Lconstr}
\Big({L^\mu}_\alpha(I)g_{\beta\nu}(1)-{L^\mu}_\beta(I)g_{\alpha\nu}(1)\Big)\frac{\delta S_\mathrm{int}}{\delta {L^{\mu}}_{\nu}}=0\,.
\eeqn
As explained in {\protect{\hyperref[papIV]{Paper IV}}}, these $(\mathcal{N}-1)\cdot d(d-1)/2$ equations can indeed be shown to be equivalent to the constraints~(\ref{constvierb}) on the gauge fixed vielbeins ${E^a}_\mu(I)$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Recovering bimetric interactions}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We would now like to address the question under what circumstances the interaction potential~(\ref{metrexp}) is writable in terms of metrics alone without having to introduce St\"uckelberg fields. 
In principle, plugging back the solution to the constraint equations~(\ref{Lconstr}) into the action will always result in a theory involving only the metrics, but in reality the explicit solution for the St\"uckelberg fields is difficult to obtain in the general case. In particular, the constraints may need to be solved componentwise, resulting in a noncovariant expressions for the interaction potential in terms of metrics alone.

Nevertheless, there is one case in which the situation is greatly simplified. Suppose we demand the interactions to be expressible in terms of $\sqrt{g^{-1}(1)g(I)}$ after integrating out the St\"uckelberg fields . The only obvious situation in which this requirement is satisfied is when the constraint equations~(\ref{Lconstr}) allow for solutions ${L^{\nu}}_{\lambda}(I)=\delta^\nu_\lambda$, or, equivalently, $A_{\mu\nu}(I)=0$. If that is the case, then on this solution~(\ref{Lconstr}) reduces to
\beqn\label{LconstrA0}
\left.\left(\frac{\delta S_\mathrm{int}}{\delta L^{\mu\nu}}-\frac{\delta S_\mathrm{int}}{\delta L^{\nu\mu}}\right)\right|_{A=0}=0\,,
\eeqn
where we have raised the index on ${L^{\nu}}_{\lambda}(I)$ with $g(1)^{\lambda\mu}$.
We will now argue that (\ref{LconstrA0}) together with $A_{\mu\nu}(I)=0$ is a consistent solution if the interaction potential contains only interactions between two vierbeins ${e^a}_\mu(1)$ and ${e^a}_\mu(2)$. In that case, namely, a generic term in the potential reads
\begin{align}\label{potfortv}
\sqrt{-\det g(1)}~&\tilde{\epsilon}^{\mu_1\hdots\mu_n\lambda_{n+1}\hdots\lambda_{d}}\tilde{\epsilon}_{\nu_1\hdots \nu_d \lambda_{n+1}\hdots\lambda_{d}}\nn\\
&~~~~~~~~~~~~\cdot L^{\nu_1\kappa_1}(2)S_{\kappa_1\mu_1}
\hdots 
L^{\nu_n\kappa_n}(2)S_{\kappa_n\mu_n}\,,
\end{align}
where we have defined the symmetric matrix
\beqn
S_{\kappa\mu}\equiv g(1)_{\kappa\rho}\left(\sqrt{g^{-1}(1)g(2)}\right)^\rho_{~\mu}\,.
\eeqn
Now take the variation of (\ref{potfortv}) with respect to $L^{\mu\nu}$ and in that set $A_{\mu\nu}(2)=0$, i.e.~$L^{\mu\nu}(2)=g^{\mu\nu}$. This gives an expression involving terms that are proportional to powers of $S_{\mu\nu}$. As a consequence of the symmetry of $S_{\mu\nu}$, this expression is symmetric itself. Therefore all terms in the variation of $S_\mathrm{int}$ with respect to $L^{\mu\nu}$ are symmetric when evaluated on $A_{\mu\nu}(2)=0$ and hence (\ref{LconstrA0}) holds. This shows that $A_{\mu\nu}(2)=0$ is indeed a solution to the constraint equations in this case, and thus integrating out the St\"uckelberg fields results in the Hassan-Rosen bimetric action with potential~(\ref{potantisym}).

Using the same arguments as above, it is easy to see that this result carries over to the case of $\mathcal{N}$ vielbeins with only bimetric interactions. The equivalent metric description is of the form~(\ref{gencv}). We conclude that the vielbein theories that possess straightforward reformulations in terms of metrics alone precisely correspond to graphs of the form shown in the left panel of Figure~4.2. In order to build more complicated interactions, such as loops and $n$-point vertices with $n>2$, one must invoke the St\"uckelberg fields ${L^{\nu}}_{\lambda}$ and solve their equations in a nontrivial way.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Bimetric Cosmology}
\label{ch:cosmo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


On small scales General Relativity makes very good predictions and, from a phenomenological point of view, there is no need to look for a modification of the theory. On cosmological states, however, it seems that either quantum field theory or gravity (or both) have to be modified in order to explain the observed value of the cosmic acceleration. Therefore, once a consistent theory of modified gravity has been constructed, its implications for cosmology are of great interest. Self-accelerating solutions of massive gravity have, for instance, been considered in \cite{deRham:2010tw, Gumrukcuoglu:2011ew}, and the hope was that a large cosmological constant could be screened out by the graviton mass that weakens gravity at large scales. However, this does not seem to be possible without fine tuning \cite{Hassan:2011vm}. In \cite{D'Amico:2011jj} the authors show that there exist no homogeneous and isotropic solutions in the dRGT model of Massive Gravity with flat reference metric. On the other hand, our analysis of bimetric theory with dynamical reference metric shows that in this framework such solutions do exist. The simplest examples are the proportional backgrounds considered in section~\ref{secpropbg} which, however, exist only for proportional sources. In this chapter we consider a different class of solutions for which one of the sources is set to zero. 
The existence of cosmological solutions in bimetric theory, in turn, implies their presence in Massive Gravity with a general homogeneous and isotropic reference frame. Homogeneous and isotropic solutions in bimetric gravity are the subject of {\protect{\hyperref[papII]{Paper~II}}} and have also been investigated in two further articles~\cite{Volkov:2011an, Comelli:2011zm} that appeared roughly at the same time. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Standard cosmology in General Relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Before discussing homogeneous and isotropic solutions in bimetric gravity, let us briefly review the derivation of the cosmological evolution equations in GR. To this end, we consider the Einstein-Hilbert action in $d=4$ including a cosmological constant term as well as a standard coupling of the metric $\gmn$ to matter,
\beqn
S_\mathrm{EH+m}=\frac{1}{M_\mathrm{PL}^2}\int\dd^4x\sqrt{-g}~\big(R-2\Lambda\big)+\int\dd^4x\sqrt{-g}~\mathcal{L}_m
\eeqn
The equations of motions for $\gmn$ obtained from this action read
\beqn\label{einsteq}
R_{\mu\nu}-\frac{1}{2}\gmn R=\frac{1}{M_\mathrm{PL}^2}\left(T_{\mu\nu}-\rho_\Lambda\,\gmn\right)\,,
\eeqn
where $T_{\mu\nu}$ is the stress-energy tensor obtained from variation of the matter Lagrangian as in (\ref{strente}) and we have defined the constant energy density $\rho_\Lambda\equiv\Lambda M_\mathrm{PL}^2$. 

When looking for homogeneous and isotropic solutions in general relativity, one makes a Friedmann-Robertson-Walker ansatz for the metric,
\beqn\label{FRWg}
\gmn \md x^\mu\md x^\nu=-\md t^2+a(t)^2\left(\frac{1}{1-kr^2}\md r^2+r^2\md \Omega\right)\,,
\eeqn
in which $k=0,-1,+1$ parameterizes the curvature of the universe (flat, open, closed), $a(t)$ is the scale factor, and $\md \Omega=\md \theta^2+\sin^2 \theta\,\md \varphi^2$. 
In accordance with homogeneity and isotropy, the stress-energy tensor is taken to be that of a perfect fluid, 
\beqn\label{setans}
{(T^g)^{\mu}}_\nu=\mathrm{diag}(-\rho, p, p, p)\,,
\eeqn
where $\rho(t)$ and $p(t)$ are the time dependent energy density and pressure of the fluid, respectively. As a consequence of the Bianchi identity the source is automatically covariantly conserved which implies the continuity equation,
\beqn\label{conteq}
\dot{\rho}+3\frac{\dot{a}}{a}\big(\rho+p\big)=0\,,
\eeqn
where dots denote time derivatives. This equation is actually nothing but the first law of thermodynamics, $\dd E=-p\,\dd V$, for an adiabatic expansion with volume $V=a^3$ and energy $E=\rho a^3$. 

Plugging the diagonal ans\"atze~(\ref{FRWg}) and~(\ref{setans}) into Einstein's equations~(\ref{einsteq}) gives a set of four equations. The 00-component is Friedmann's equation,
\beqn\label{Friedmann}
\left(\frac{\dot{a}}{a}\right)^2+\frac{k}{a^2}=\frac{\rho+\rho_\Lambda}{3M_\mathrm{PL}^2}\,,
\eeqn 
which is often expressed in terms of the Hubble parameter $H\equiv \dot{a}/a$.
Due to the isotropic ansatz, the $ii$-components of the equations are all equivalent and therefore only provide one additional independent equation. The most common way to present it is by taking the traced Einstein equations and using~(\ref{Friedmann}) to arrive at the acceleration equation,
\beqn\label{acceq}
\frac{\ddot{a}}{a}=-\frac{1}{6M_\mathrm{PL}^2}\left(\rho+\rho_\Lambda+3p\right)\,.
\eeqn
In fact, integrating the acceleration equation~(\ref{acceq}) and using the continuity equation~(\ref{conteq}) gives back the Friedmann equation~(\ref{Friedmann}), where $k$ enters as an integration constant. This is expected because the continuity equation is obtained from taking the divergence of Einstein's equations and is therefore already contained in the equations of motion. To specify a solution it is therefore sufficient to consider only two out of the three equations. 

In order to characterize different components of the cosmological fluid, one introduces the equation of state parameter $w$ defined as the ratio of pressure and energy density, $p=w\rho$. One can then rewrite the continuity equation~(\ref{conteq}) as 
\beqn
\frac{\dd \rho}{\dd a}+3(1+w)\frac{\rho}{a}=0\,,
\eeqn
which is solved by
\beqn
\rho=\rho_0\, a^{-3(1+w)}\,.
\eeqn
Here, $\rho_0$ is a constant to be determined by boundary conditions. Inserting this solution into the Friedmann equation~(\ref{Friedmann}) with $k=0$ and $\rho_\Lambda=0$ gives the following evolution of the scale factor for $w\neq -1$,
\beqn
a~\propto~ t^{\frac{2}{3(1+w)}}\,.
\eeqn
The behaviour for $w=-1$ is
\beqn
a~\propto~ e^{Ht}\,,\qquad H\equiv \frac{\dot{a}}{a}=\mathrm{const}.
\eeqn
Moreover, from the acceleration equation~(\ref{acceq}) we infer that, in the absence of a bare cosmological constant, the expansion of the universe accelerates for $w<-1/3$ and decelerates for $w>-1/3$. Three cases are of particular interest: $w=0$ characterizes nonrelativistic matter, $w=1/3$ corresponds to relativistic matter (``radiation"),  and $w=-1$ describes a cosmological constant. The energy density for nonrelativistic matter therefore scales as $a^{-3}$, i.e.~inversely proportional to the volume. Nonrelativistic matter experiences an additional redshift and its energy density goes as $a^{-4}$. None of these can explain an accelerated expansion of the universe. In contrast, a cosmological constant which of course has constant energy density leads to an exponentially accelerated expansion. 

It is common to measure the contributions of different fluid components in terms of their density parameters,
\beqn
\Omega_i=\frac{\rho_i}{3M_\mathrm{PL}^2 H_0^2},
\eeqn
where $i$ stands for either radiation, nonrelativistic matter or the cosmological constant and $H_0$ denotes the Hubble parameter at the present time. One also defines a curvature contribution, $\Omega_k=-\tfrac{k}{a^2H_0^2}$, and in terms of these the Friedmann equation becomes
\beqn
\Omega_\mathrm{rad}+\Omega_\mathrm{mat}+\Omega_\Lambda+\Omega_k=\frac{H^2}{H^2_0}\,.
\eeqn 
In particular, at the present time the density parameters add up to one. Latest observational data \cite{Hinshaw:2012aka, Ade:2013ktc} suggest the following values for the cosmological parameters at the present time,
\beqn
&~&H_0\sim 70\, \mathrm{km/s/Mpc}\,,\qquad \Omega_\mathrm{rad}\sim 10^{-5}\,,\qquad \Omega_\mathrm{mat}\sim 0.3 \,,\nn\\
&~&\Omega_\Lambda\sim 0.7\,,\qquad\qquad\qquad~~~\,   \Omega_k< 10^{-3}\,.
\eeqn
These values imply that our universe is flat and dominated by a cosmological constant component. As already discussed in the introduction, the energy density corresponding to this cosmological constant is extremely small compared to energy scales of the Standard Model of Particle Physics. Since so far we lack an explanation for this small value, the curious energy component $\rho_\Lambda$ is often referred to as \textit{Dark Energy}. On top of that, observations also show that the matter component $\Omega_\mathrm{m}$ is not dominated by familiar baryonic matter, but rather mainly consists of an unknown \textit{Dark Matter} component. These findings are summarized in the pie chart of Figure~5.1. 
 \begin{figure}[ht]
    \begin{center}
    \includegraphics[width=220pt]{Pictures/WMAP.pdf}
    \caption{Distribution of energy in the present universe. \textit{Credit: NASA/WMAP Science Team.}}
    \end{center}\label{figWMAP}
    \end{figure}
Consequently, under the assumption that General Relativity is indeed the theory of gravity, we must accept that 95$\%$ of the universe's energy content is not at all understood. Nevertheless, when this obscurity is ignored, the so-called $\Lambda$CDM model (GR with a cosmological constant and cold dark matter) fits the observational data very well.

Alternatively, we may question the validity of Einstein's theory of gravity and try to modify it on small distance scales such that it can account for one or both of the dark components in our universe. An example for a consistent infrared modification is bimetric gravity, which motivates us to derive and study the analogue of Friedmann's equation in this model. 

 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Cosmological evolution in bimetric theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In all of this chapter we work with the bimetric action (\ref{HR}) in four dimensions. Furthermore, in order to use the same conventions as in {\protect{\hyperref[papV]{Paper~V}}}, we replace the mass scale $m^4$ by $m^2m_g^2$. 
The coupling of $\fmn$ to matter is set to zero, which is of course a rather restrictive assumption. On the other hand, it allows us to interpret $\gmn$ as the metric in the usual way, provided that it has standard matter couplings.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsection{Homogeneous and isotropic ansatz} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

To keep the comparison of the bimetric solutions to those of General Relativity as simple as possible, we choose to make the usual Friedmann-Robertson-Walker ansatz for the metric $\gmn$ which is coupled to matter,
\beqn\label{FRWg}
\gmn \md x^\mu\md x^\nu=-\md t^2+a(t)^2\left(\frac{1}{1-kr^2}\md r^2+r^2\md \Omega\right)\,,
\eeqn 
It is now important to notice that, in order to arrive at this form, we have used time reparametrizations to remove one time-dependent function in the most general homogeneous and isotropic ansatz. We have therefore fixed the entire diffeomorphism invariance and there is no gauge symmetry left to do the same to $\fmn$.
As a result the most general homogeneous and isotropic ansatz for the second metric reads
\beqn\label{FRWf}
\fmn\md x^\mu\md x^\nu=-X(t)^2\md t^2+Y(t)^2\left(\frac{1}{1-kr^2}\md r^2+r^2\md \Omega\right)\,,
\eeqn
involving two time dependent functions $X(t)$ and $Y(t)$. Note also that we have assumed the curvatures $k$ of the two metrics to be the same. 

Furthermore, we use the perfect fluid form (\ref{setans}) for the stress-energy tensor ${(T^g)^{\mu}}_\nu$ of matter coupled to $\gmn$.
In GR any source is automatically covariantly conserved as a consequence of the Bianchi identity whereas in bimetric gravity the two sources for $\gmn$ and $\fmn$ are not necessarily separately conserved. But since here we have set $T^f_{\mu\nu}=0$, the diffeomorphism invariance of the Einstein Hilbert term and the interaction potential again imply $\nabla_g^\mu T_{\mu\nu}=0$ on-shell. 
This implies that the continuity equation~(\ref{conteq}) is also valid in the model under consideration.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evolution equations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, we consider the bimetric equations of motion, (\ref{geq}) and (\ref{feq}), with one index raised with the respective inverse metrics. Similarly to what we saw in GR, the symmetries of the cosmological ansatz ensure that it is sufficient to work with only part of the equations. Here, these are taken to be the $00$-components of the equations of motion, together with the continuity equation for the source, as well as the Bianchi constraint~(\ref{Bianchi}). The latter needs to be included because now the continuity equation makes up only a part of the divergence of the $\gmn$ equation. The $ii$-components of the equations of motion are then redundant. 

In what follows we shall refer to the $00$-components as simply the $\gmn$ and~$\fmn$ equation. Plugging the ans\"atze of the previous section into (\ref{geq}) we can make use of known GR results to straightforwardly obtain the $\gmn$ equation,
\beqn\label{gmncos}
\left(\tfrac{\dot{a}}{a}\right)^2+\tfrac{k}{a^2}-\tfrac{m^2}{3}\left[\beta_0+3\beta_1\tfrac{Y}{a}+3\beta_2\left(\tfrac{Y}{a}\right)^2+\beta_3\left(\tfrac{Y}{a}\right)^3\right]=\tfrac{\rho}{3m_g^2}\,.
\eeqn
In order to determine how different source components influence the cosmological evolution, we need to determine the function $Y(t)$ from the other equations. We start with the Bianchi constraint~(\ref{Bianchi}), evaluated on the homogeneous and isotropic ansatz, 
\beqn\label{bianchiev}
\tfrac{3m^2}{a}\left[\beta_1+2\beta_2\tfrac{Y}{a}+\beta_3\left(\tfrac{Y}{a}\right)^2\right]\left(\dot{Y}-\dot{a}X\right)=0\,.
\eeqn
There are two options to satisfy this equation; either the first or the second bracket must vanish: 
%%%%%%%%%%%%%%%%
\begin{itemize}

\item[\textbf{(1)}] If the parameters of the theory obey $\beta_1+2c\beta_2+c^2\beta_3=0$ for some constant $c$, then one solution is provided by $Y(t)=c \,a(t)$. In this case, the contribution from the interaction potential in~(\ref{gmncos}) reduces to a cosmological constant term. The $\gmn$ equation hence simply becomes the Friedmann equation~(\ref{Friedmann}) with a cosmological constant $\Lambda=m^2(\beta_0+3c\beta_1+3c^2\beta_2+c^3\beta_3)$. Interestingly, around proportional backgrounds, $\fmn=c^2\gmn$, the Fierz-Pauli mass of the massive perturbation is proportional to the combination of $\beta_n$ parameters in~(\ref{bianchiev}). It therefore vanishes on this particular background if the Bianchi constraint is satisfied by setting the first bracket in~(\ref{bianchiev}) to zero. This may imply an interesting phenomenology for the perturbations, but due to its degeneracy with GR at the background level, the solution is not of great interest to us here. 


\item[\textbf{(2)}] The alternative solution to the Bianchi constraint is $X(t)={\dot{Y}}/{\dot{a}}$. In contrast to the above, this is a dynamical equation and allows for much more general solutions. Since we are mostly interested in solutions that do not show the exact same behaviour as in GR, we focus on this branch in the following. Note also that, in fact, this constitutes no loss of generality because
setting the second bracket in~(\ref{bianchiev}) to zero still includes the proportional spatial metrics as possible solutions.

\end{itemize}
%%%%%%%%%%%%%%%%
Next, we turn to the $\fmn$ equation. Since the ansatz for $\fmn$ contains an extra time-dependent function in the 00-component, the derivative terms in this equation will look more complicated than the expressions familiar from GR. We derive them in the appendix of {\protect{\hyperref[papV]{Paper~V}}}. 
After eliminating $X(t)$ using the solution to the Bianchi constraint, the $\fmn$ equation reads 
\beqn
\left(\tfrac{\dot{a}}{Y}\right)^2+\tfrac{k}{Y^2}-\tfrac{m^2}{3\alpha^2}\left[\beta_1\left(\tfrac{a}{Y}\right)^3+3\beta_2\left(\tfrac{a}{Y}\right)^2+3\beta_3\tfrac{a}{Y}+\beta_4\right]=0\,,
\eeqn
where, as usual,\footnote{Note that in {\protect{\hyperref[papV]{Paper~V}}} the ratio of the Planck masses is denoted by $M_*$ instead of~$\alpha$.} $\alpha\equiv m_f/m_g$.
Multiplying this equation by $Y^2/a^2$ and subtracting it from the $\gmn$ equation (\ref{gmncos}) yields an algebraic equation,
\begin{align}\label{polynom}
\frac{\beta_3}{3}\Upsilon^4+\left(\beta_2-\tfrac{\beta_4}{3\alpha^2}\right)\Upsilon^3&+\left(\beta_1-\tfrac{\beta_3}{\alpha^2}\right)\Upsilon^2\nn\\
&+\left(\rho_*+\tfrac{\beta_0}{3}-\tfrac{\beta_2}{\alpha^2}\right)\Upsilon-\tfrac{\beta_1}{3\alpha^2}=0\,.
\end{align}
We have expressed this in terms of the dimensionless quantities,
\beqn
\Upsilon=\frac{Y}{a}\,,\qquad \rho_*=\frac{\rho}{3m_g^2m^2}\,.
\eeqn
Now we would like to solve equation (\ref{polynom}) for $\Upsilon$ and plug the solution back into the $\gmn$ equation~(\ref{gmncos}). After that, this equation will only contain $a(t)$, $\dot{a}(t)$ and $\rho(t)$ and thus becomes a modified Friedmann equation. The quartic polynomial equation (\ref{polynom}) can be solved numerically for $\Upsilon$. The general solution, however, is not very transparent. Instead, one can fix one or several of the $\beta_n$ parameters and investigate these constrained parameter spaces for simpler solutions. In {\protect{\hyperref[papII]{Paper~II}}}, we focus on parameter choices that allow for solutions close to those of GR.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Degeneracy with General Relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Consider, for example, the choice $\beta_3=0$. In this case, (\ref{polynom}) reduces to a cubic equation for $\Upsilon$ whose solutions will already look simpler. An even greater simplification is achieved if we in addition put $\beta_1=0$. Then the equation for $\Upsilon$ is a quadratic and a solution is readily obtained. Plugging it into the $\gmn$ equation~(\ref{gmncos}) then gives
\beqn\label{deggrcase}
\left(\frac{\dot{a}}{a}\right)^2+\frac{k}{a^2}=\frac{\rho}{3\bar{M}_\mathrm{Pl}^2}+\frac{\rho_\Lambda}{3\bar{M}_\mathrm{Pl}^2}\,,
\eeqn
where we have introduced a modified Planck mass and an effective constant energy density,
\beqn
\bar{M}_\mathrm{Pl}^2=\frac{m_g^2(\beta_4-3\beta_2\alpha^2)}{\beta_4}\,,\quad~~~~ \rho_\Lambda=\frac{m^2(\beta_0\beta_4-9\beta_2^2)}{\beta_4}\,.
\eeqn
Evidently, this is simply the usual Friedmann equation~(\ref{Friedmann}). The bimetric solution in this model is therefore indistinguishable from standard GR cosmology. This is a nontrivial result because the nonlinear theories themselves are very different due to the $\beta_2$-interaction term of bimetric theory. These differences are expected to show up at the level of perturbations. Bimetric perturbation theory around homogeneous and isotropic solutions has been studied in~\cite{Comelli:2012db, Berg:2012kn}. 

Turning on $\beta_1$ takes us smoothly away from the solutions that are degenerate with GR. Consequently, as shown in {\protect{\hyperref[papV]{Paper~V}}}, for small values of $\beta_1$ it is still possible to fit the model to cosmological data. For larger values the predictions of the bimetric model become incompatible with observations.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To summarize, the main conclusion of {\protect{\hyperref[papII]{Paper~II}}} is that there exist nontrivial (i.e.~interacting) models of bimetric gravity with cosmological solutions in agreement with observational data. Hence, the Hassan-Rosen bimetric theory passes one of the first tests for being a valid theory of gravity. In the model where $\beta_1=\beta_3=0$, the cosmological constant is a combination of contributions from the matter source   (which can be absorbed in $\beta_0$) and the bimetric interaction potential. Fitting it to its observed value still involves fine tuning of the parameters and the cosmological constant problem remains unsolved. The situation is somewhat improved for other choices of $\beta_n$, as will be discussed in the next section. 

Another important point is that it is far from clear whether the effective Planck mass in~(\ref{deggrcase}) is the same as the one that would enter spherically symmetric solutions. In GR the Planck mass in Friedmann's equation is the same as the one that enters the gravitational constant in the Newtonian limit and it is this value that has been used to fit the cosmological data. However, if in bimetric gravity the effective Planck mass on cosmological scales turns out to be different than the one on smaller scales, the model would most likely not be compatible with observations. Since so far not much is known about spherically symmetric solutions in bimetric gravity,\footnote{See however \cite{Comelli:2011wq, Volkov:2012wp}, where some progress has been made towards finding spherically symmetric solutions.} this investigation is still an open task.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Self-acceleration}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The purpose of~{\protect{\hyperref[papII]{Paper~II}}} was to demonstrate the existence of viable cosmological solutions in bimetric gravity. A more thorough statistical analysis of the whole parameter space was conducted in~\cite{Akrami:2012vf}. The authors used data from observations of the cosmic microwave background, baryon acoustic oscillations, type Ia supernovae, and the present value of the Hubble parameter to constrain different bimetric models.\footnote{See also~\cite{Akrami:2013ffa} where a similar analysis is performed in a model including matter couplings for $\fmn$ .} In particular, they investigate whether models with $\beta_0=0$ and no cosmological constant contribution from the matter source can give rise an expansion history compatible with observations. In the absence of a constant vacuum energy density driving the acceleration of the universe's expansion, the model has to be \textit{self-accelerating}, i.e.~the observed acceleration must stem from modified terms in Friedmann's equation. Indeed, self-accelerating solutions are found for many different combinations of nonzero $\beta_n$ parameters in bimetric gravity and, in fact, the fits to data are just as good as for the ordinary $\Lambda$CDM model.

The best fit value for the mass of the massive spin-2 field is on the order of the Hubble scale $H_0$. Since in the zero-mass limit the full diffeomorphism symmetry that transforms the two metrics separately is restored, a small spin-2 mass is technically natural. In the ideal case, bimetric theory should also explain why we do not observe the large cosmological constant predicted by quantum field theory, for instance it should provide a mechanism to screen out a large vacuum energy. To our present knowledge, this is not the case, except maybe for the parameters of the partially massless theory, discussed in chapter~\ref{ch:PM}. However, if an explanation for the absence of a large cosmological constant was found elsewhere, the Hubble scale set by the spin-2 mass could be radiatively stable, which would be a large step towards solving the cosmological constant problem.  



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Partially Massless Bimetric Theory}
\label{ch:PM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A massive spin-2 field in de Sitter (dS) background exhibits several interesting features that are neither shared by lower-spin particles nor by spin-2 excitations in flat space. For a special value of the Fierz-Pauli mass in units of the background curvature, the linear theory possesses an additional gauge symmetry which removes one of the spin-2 helicity components. In this case, where the field loses one propagating degree of freedom, it is referred to as \textit{partially massless} (PM). The particular mass value for which this situation occurs is called \textit{Higuchi bound} because it divides the parameter region into unitary and nonunitary subsectors~\cite{Higuchi:1986py}. 
%Below the Higuchi bound the helicity-zero mode of the spin-2 particle develops a ghost instability, whereas above the bound the the theory is healthy. 
%The Higuchi bound is therefore a particularly interesting line in parameter space. 

Being in the possession of a nonlinear theory that involves a massive spin-2 field, we are able to address the following question: Is the concept of partial masslessness restricted to the linear theory around de Sitter backgrounds or can it be extended to the nonlinear level? The demand on a nonlinear PM theory is the presence of an extra gauge symmetry, even away from de Sitter backgrounds. In {\protect{\hyperref[papVI]{Paper~VI}}} we develop a method to identify a unique candidate for a nonlinear PM bimetric theory in four spacetime dimensions. The analysis is extended to higher dimensions in {\protect{\hyperref[papVII]{Paper~VII}}}, where it is found that pure bimetric theory cannot give rise to partial masslessness at the nonlinear level. We therefore modify the bimetric action by adding the Lanczos-Lovelock terms and show that in this generalized framework it again becomes possible to single out PM candidates .




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Partial masslessness in de Sitter background}\label{seclinPM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us begin by reviewing the linear theory of a PM spin-2 particle in a de Sitter background, which was first discussed in a sequence of papers by Deser et.al.~\cite{Deser:1983mm, Deser:2001pe, Deser:2001us, Deser:2001wx, Deser:2001xr, Deser:2004ji, Deser:2006zx}. 
The equation of motion for a massive spin-2 fluctuation $h_{\mu\nu}$ in a de Sitter background $\bar{G}_{\mu\nu}$ with positive cosmological constant $\Lambda$ is given by
\beqn\label{lineqds}
{\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}h_{\rho\sigma}-\tfrac{2\Lambda}{d-2}\left(h_{\mu\nu}-\tfrac{1}{2}\bar{G}_{\mu\nu} h\right)
+\tfrac{m^2_\mathrm{FP}}{2}\Big(h_{\mu\nu}-\bar{G}_{\mu\nu} h\Big)=0\,,
\eeqn
where the derivative operator ${\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}$ is given in (\ref{kinopds}). For general values of the Fierz-Pauli mass, the equation possesses no gauge symmetries. Similarly to its analogue in flat space that was discussed in detail in section~\ref{sec:FP}, it contains $d+1$ constraint equations that reduce the number of propagating degrees of freedom to $(d(d-1)/2-1)$, appropriate for a massive spin-2 particle.

A feature of (\ref{lineqds}) without any analogue in flat space is that if the Fierz-Pauli mass saturates the Higuchi bound, $m^2_\mathrm{FP}=\frac{2}{d-1}\Lambda$, the equation is invariant under a new gauge symmetry. The corresponding linear gauge transformation reads
\beqn\label{linPMsym}
\Delta (\hmn) = \bar{\nabla}_\mu\partial_\nu\xi(x)+\tfrac{2\Lambda}{(d-1)(d-2)} \bar{G}_{\mu\nu}\, \xi(x)\,,
\eeqn
in which $\xi(x)$ is a local gauge parameter.
Moreover, if the value for the mass lies below the bound, the theory is nonunitary because the helicity-zero mode of the massive spin-2 field becomes a ghost \cite{Higuchi:1986py, Higuchi:1989gz}. Above the Higuchi bound the theory is well-behaved. 

Besides computing the variation of~(\ref{lineqds}) under the gauge transformation explicitly, there is another straightforward way to see the existence of a gauge symmetry in the equation for the massive spin-2 field with mass at the Higuchi bound. First take the double divergence of~(\ref{lineqds}) to arrive at
\beqn\label{doublediv}
\bar{\nabla}_\nu\bar{\nabla}_\mu\left(\bar{G}^{\mu\nu} \bar{G}^{\rho\sigma}-\bar{G}^{\mu\rho}\bar{G}^{\nu\sigma}\right)h_{\rho\sigma}=0\,.
\eeqn
The kinetic terms have dropped out after using the linearized Bianchi identity.
Furthermore, the trace of (\ref{lineqds}) is given by
\beqn
\tfrac{d-2}{2}\,\bar{\nabla}_\nu\bar{\nabla}_\mu\left(\bar{G}^{\mu\nu} \bar{G}^{\rho\sigma}-\bar{G}^{\mu\rho}\bar{G}^{\nu\sigma}\right)h_{\rho\sigma}+\left(\Lambda-\tfrac{d-1}{2}m^2_\mathrm{FP}\right)h=0\,.
\eeqn
If the mass is at the Higuchi bound, the terms without derivatives in this equation vanish identically, while the derivative terms are zero due to~(\ref{doublediv}).
Hence we find that for $m^2_\mathrm{FP}=\frac{2}{d-1}\Lambda$ the traced equations of motion are identical to their double divergence. Put differently, when multiplied by the appropriate factors, the difference of the trace and the double divergence is identically zero.
This identity signals the presence of a gauge symmetry. Since one particular combination of the equations of motion is identically satisfied, one component of $\hmn$ remains undetermined.  
In fact, a gauge identity of the above type even implies that the action is invariant under the corresponding gauge transformation. This follows from the fact that invariance of the action under~(\ref{linPMsym}) requires
\beqn
\Delta S=\frac{\delta S}{\delta \hmn}\Delta (\hmn)=0\,.
\eeqn
Since $\tfrac{\delta S}{\delta \hmn}$ is nothing else than the equation of motion for $\hmn$, after integrating by parts, we find that $\Delta S$ indeed vanishes due to the gauge identity. 

The conclusion is that the massive spin-2 field described by (\ref{lineqds}) with mass at the Higuchi bound has only $(d(d-1)/2-2)$ degrees of freedom, one less than is usually the case. Let us also remark that the existence of the gauge symmetry around de Sitter backgrounds is in agreement with the representation theory of the de Sitter group SO$(1,d)$, which allows for so-called \textit{partially massless} (PM) representations of higher-spin fields. For a discussion of this topic, consult e.g.~\cite{Garidi:2003ys}. The whole situation is summarized in Figure~6.1, where for definiteness we fix $d=4$.
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=200pt]{Pictures/dSPM.pdf}
    \caption{Unitary and nonunitary regions in the $\Lambda$-$m_\mathrm{FP}^2$-plane in $d=4$. The boundary of the shaded region corresponds to the Higuchi bound.}
    \end{center}
    \end{figure}

After the linear PM theory for spin-2 fields on de Sitter background had been established, it was attempted to construct higher order interactions for the perturbation $\hmn$ that would leave the gauge symmetry intact. At cubic order in $\hmn$ such a construction turned out to be possible in $d=4$~\cite{Zinoviev:2006im, Joung:2012rv}. In $d>4$, however, it was found that gauge invariant cubic vertices can only exist if one also includes higher derivative terms into the theory \cite{Zinoviev:2006im}. The construction of a fully nonlinear theory with a PM gauge symmetry remained an open task.



The remainder of this chapter summarizes the findings of {\protect{\hyperref[papVI]{Paper~VI}}} and {\protect{\hyperref[papVII]{Paper~VII}}} where we propose a nonlinear PM theory within the family of ghost-free bimetric theories. In particular, we show that in this framework it is possible to understand the outcome of the cubic-vertex analyses of~\cite{Zinoviev:2006im, Joung:2012rv}. We begin by explaining the properties of the candidate PM theory for the most relevant case of four space-time dimensions, before we generalize the arguments to $d>4$. Further remarkable features of the theory in $d=4$ will be presented in chapter~\ref{ch:HD} in the context of higher-curvature actions.


 
  
   
   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
\section{Towards a nonlinear PM theory}\label{secPmnonlin}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
It is natural to expect the nonlinear PM theory (if it exists) to be found within the family of ghost-free nonlinear theories for massive spin-2 fields. A first investigation of this possibility was carried out in \cite{deRham:2012kf} where the authors aimed to identify a PM theory in nonlinear Massive Gravity with the reference metric taken to be a fixed de Sitter background. Their construction used St\"uckelberg fields in a generalized decoupling limit and showed that, for a certain choice of the $\beta_n$-parameters, a scalar degree of freedom is not propagating. Although this seemed to be a solid argument for the presence of a gauge symmetry in the decoupling limit, it was later argued in \cite{Deser:2013uy, deRham:2013wv} that constructing a PM theory in the full theory of nonlinear Massive Gravity is impossible. Inspite of lacking a proof, another article also made similar negative statements about PM bimetric theory~\cite{Deser:2013gpa}.

Taking into account these objections, one could be worried about the possibility of constructing a PM bimetric theory. 
However, there are several reasons why the above no-go results need not concern us here:
First of all, the results of \cite{Deser:2013uy, deRham:2013wv} hold only for nonlinear Massive Gravity with fixed reference metric $\fmn$, and do not directly carry over to the ghost-free bimetric gravity where both metrics are dynamical. In fact, the analyses in these references merely show that in a nonlinear PM theory none of the metrics can be held fixed because both of them are expected to transform under the PM gauge symmetry. We will come back to this point in section~\ref{sec:PMMG}. Apart from this, the authors of \cite{Deser:2013uy, Deser:2013gpa} search for a nonlinear action with invariance under an infinitesimal PM gauge transformation and are unable to find it. The action will, however, not be invariant if the invariance is an on-shell symmetry of the equations of motion. In fact, it is possible to use the results we derive below to demonstrate that the nonlinear PM theory can only be invariant on-shell. This is part of an upcoming publication and beyond the scope of this thesis. However, we emphasize one more time that the no-go results of \cite{Deser:2013uy, deRham:2013wv, Deser:2013gpa} simply do not apply to the theory under consideration here.





In {\protect{\hyperref[papVI]{Paper~VI}}} we develop a method that allows us to identify a candidate PM theory within the family of ghost-free bimetric theories. To this end, we consider the proportional background solutions as well as the spectrum of linear perturbations around these that were discussed in section~\ref{sec:massspec}. This is a natural setup for extending the PM symmetry of perturbations around dS space because these backgrounds have constant curvature and, in particular, they are the only ones around which a massive fluctuation with Fierz-Pauli mass term exists. Our method is suitable for identifying or excluding PM candidates in bimetric theory in any space-time dimension. In this section, however, after outlining the general idea, we restrict to the case $d=4$. Dimensions greater than four will be the focus of section~\ref{PMdgf}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Identifying PM candidates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The equation of motion (\ref{dMeq}) for the massive fluctuation $\delta M_{\mu\nu}$ around proportional backgrounds is of the same form as (\ref{lineqds}) with $\Lambda=\bar{\Lambda}_g$.  
As a consequence, if the cosmological constant is assumed to be positive and if the Fierz-Pauli mass (\ref{FPmass}) is on the Higuchi bound, a gauge symmetry of the form (\ref{linPMsym}) is present in the linear theory around proportional backgrounds. In bimetric notation, the corresponding infinitesimal gauge transformation of the massive fluctuation reads
\beqn\label{linPMsym2}
\Delta (\delta M_{\mu\nu}) = \bar{\nabla}_\mu\partial_\nu\xi(x)+\tfrac{2\bar{\Lambda}_g}{(d-1)(d-2)} \bar{G}_{\mu\nu}\, \xi(x)\,.
\eeqn
On the other hand, the massless fluctuation does not transform under the PM symmetry, 
\beqn
\Delta (\delta G_{\mu\nu}) = 0\,.
\eeqn
This follows from the fact that its equation of motion (\ref{dGeq}) does not have any extra gauge symmetry besides the usual linearized diffeomorphism invariance. Therefore, $\delta G_{\mu\nu}$ itself must be invariant under the PM symmetry. 
The question is now under what conditions the above symmetry transformations for the fluctuations around dS background have a chance to be generalizable to the nonlinear level. 

Since the theory in terms of the nonlinear fields $M^G_{\mu\nu}$ and $G_{\mu\nu}$ has a very complicated form, we find it easier to work with the variables $\gmn$ and $\fmn$ instead. 
The above transformations of the mass eigenstates $\delta M_{\mu\nu}$ and $\delta G_{\mu\nu}$ allow us to uniquely determine the transformations of the fluctuations of $\gmn$ and $\fmn$ using the expressions for the massive and massless fluctuations given in (\ref{dGanddM}). The result is
\beqn\label{fgtrans}
\Delta (\delta\gmn)=-(\alpha c)^{\frac{d-2}{2}}\Delta (\delta\fmn)=\tfrac{-2(\alpha c)^{d-2}}{c(1+(\alpha c)^{d-2})}\Delta (\delta M_{\mu\nu})\,.
\eeqn
The crucial observation is now that in a theory with a gauge symmetry at the nonlinear level, it must be possible to shift these transformations of the fluctuations $\delta\gmn$ and $\delta\fmn$ to the backgrounds $\bgmn$ and $\bfmn$. This follows from the fact that the split into background and fluctuations is not unique and one can always take out part of the fluctuation to redefine the background. Therefore we demand that the symmetry transformations (\ref{fgtrans}) should also leave the background equations invariant. But since we are dealing with the proportional backgrounds, where the background equation is simply $\Lambda_g=\Lambda_f$ (c.f.~(\ref{propbackeq})), determining the proportionality constant $c^2$, we restrict ourselves to constant gauge transformations $\bar{\Delta}$ with $\xi(x)=$\,const. In this way we ensure that the transformation does not take us away from the proportional backgrounds and avoid unnecessary complication. 
The restriction to constant gauge transformations is a strong simplification, but as we will see now, demanding the background equation to be invariant under these is constraining enough to identify the PM candidate theory. Namely, it should be evident from (\ref{fgtrans}) that shifting the constant transformations to the backgrounds $\bgmn$ and $\bfmn=c^2\bgmn$ results in a shift in $c^2$,
\beqn
\bgmn\bar{\Delta}(c^2)= \bar{\Delta}(\bfmn)-c^2\bar{\Delta}(\bgmn)\,.
\eeqn
However, in general this cannot lead to an integrable\footnote{Integrability of the symmetry transformation means that it can be performed more than once and still leave the equations invariant. This is a natural requirement on any gauge symmetry. Without the integrability condition it is sufficient to set the mass to the Higuchi bound in order to have an invariant background.} symmetry of the background equations because $c$ is determined by $\Lambda_g=\Lambda_f$ and can therefore not be shifted. 
If this is the case, then a nonlinear PM symmetry cannot exist. The only possibility to avoid this immediate no-go statement is to demand that $c$ is not fixed by the background equation. 
Then, the equation $\Lambda_g=\Lambda_f$ that is automatically satisfied in this case (i.e.~without fixing $c$) is the gauge identity evaluated on the proportional backgrounds. Since making the proportional ansatz for the two metrics partly fixes the gauge, only constant scalings are left as residual transformations. The component of the metrics that remains undetermined by the equations therefore simply reduces to the constant $c$ on this solution. 

 
The whole idea will be made more explicit in the following, where we identify PM candidates in $d=4$, before we discuss the general case in the next section.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{PM candidate in $d=4$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In four space-time dimensions, the explicit expressions~(\ref{lambdas}) for the cosmological constants in terms of the $\beta_n$ parameters, the ratio of Planck masses $\alpha$ and the proportionality constant $c$ can be used to write the background condition $\Lambda_g=\Lambda_f$ as a polynomial equation for $c$,
\begin{align}
\beta_1+c(3\beta_2-\alpha^2\beta_0)&+3c^2(\beta_3-\alpha^2\beta_1)\nn\\
&+c^3(\beta_4-3\alpha^2\beta_2)-c^4\alpha^2\beta_3=0\,.
\end{align}
This equation clearly fixes $c$ unless all coefficients of different powers of $c$ vanish separately. A proportionality constant $c$ that is undetermined by the background equation therefore requires the following parameter choices in the bimetric interaction potential,
\beqn\label{PMpara}
\beta_1=\beta_3=0\,,\qquad \alpha^2\beta_0=3\beta_2=\alpha^{-2}\beta_4\,.
\eeqn
We will frequently refer to these values as the \textit{PM parameters}. Note that our requirement on the $\beta_n$-parameters fixes all but one of them uniquely in terms of the others and $\alpha$. The one remaining parameter is of course degenerate with the energy scale $m^4$ in the interaction potential and sets the scale for the Fierz-Pauli mass and the cosmological constant. Moreover, it is easy to check using the expressions (\ref{FPmass}) and (\ref{lambdas}) for $m_\mathrm{FP}^2$ and $\Lambda_g$, that the parameter choice (\ref{PMpara}) automatically puts the mass on the Higuchi bound. Therefore the theory of linear perturbations around the backgrounds at hand exhibits the usual PM gauge symmetry. It is worth emphasizing that we did not demand this in any way; it followed from an independent requirement on the background equations. 

On the other hand, we also make the following interesting observation: If we assume that there is a \textit{unique} PM theory, then satisfying the Higuchi bound is sufficient to determine its parameters. Namely, in this case, the symmetry (\ref{symbg}) of the interaction potential enforces $\alpha^{4-n}\beta_n=\alpha^{n}\beta_{4-n}$ because otherwise the theory obtained from replacing $\alpha^{4-n}\beta_n\rightarrow\alpha^{n}\beta_{4-n}$ would also be PM, contradicting the uniqueness requirement.
It is easy to see that this constraint on the $\beta_n$ parameters together with the Higuchi bound condition already implies (\ref{PMpara}).

We now turn to the requirement of integrability of the symmetry transformation. The constant parts of the PM symmetry transformations of the fluctuations can be written as 
\beqn\label{consttraf}
\Delta (\delta\gmn)=-\frac{2c\alpha^2}{1+(\alpha c)^2}\delta a\,\bgmn\,,\qquad \Delta (\delta\fmn)=\frac{2c}{1+(\alpha c)^2}\delta a\,\bgmn\,,
\eeqn
with  infinitesimal constant gauge parameter $\delta a$.
Furthermore, it is easy to check that with the PM parameters the background equations (\ref{bgeq}) are invariant under the nonlinear scaling transformations,
\beqn
\bgmn\rightarrow\frac{1+(\alpha c)^2}{1+\alpha^2(c+a)^2}\,\bgmn\,,\qquad \bfmn\rightarrow\frac{1+(\alpha c)^{-2}}{1+\alpha^{-2}(c+a)^{-2}}\,\bfmn
\eeqn
with finite constant gauge parameter $a$. Of course, these are simply the integrated versions of (\ref{consttraf}), verifying that the constant part of the gauge transformation is indeed integrable.
If the nonlinear PM symmetry exists, the above transformations constitute its form on the proportional backgrounds.

It is furthermore important to note that the Fierz-Pauli mass and cosmological constant, when taken with respect to the background metric~$\bar{G}_{\mu\nu}$, become independent of $c$,
\beqn
\bar{m}_\mathrm{FP}^2=\frac{2}{3}\bar{\Lambda}_g=2\beta_2\frac{m^4}{m_g^2}\,.
\eeqn
Hence, these can be regarded as physical quantities that do not depend on the gauge parameter $a$ that shifts the value of $c$.



By restricting to constant gauge transformations, clearly, we are not dealing with the full PM symmetry at the nonlinear level. Note, however, that since the set of constant transformations is a subset of the full gauge group, the theory we obtain by requiring invariance under this subset must contain the theory with the full gauge group (if it exists). Moreover, since in four dimensions the restriction to constant gauge transformations is sufficient to uniquely determine the $\beta_n$ parameters, we conclude that the resulting theory is already the unique candidate for having the full PM symmetry.

The scale invariance of the equations of motion for proportional backgrounds is not the only interesting property of the theory specified by the PM parameters. The PM candidate exhibits additional astonishing features that further support the existence of a gauge symmetry at the nonlinear level. For instance, consider again the homogeneous and isotropic solutions of {\protect{\hyperref[papII]{Paper~II}}} which we presented in chapter~\ref{ch:cosmo}. We saw that, after solving the Bianchi constraint, it was possible to arrive at (\ref{polynom}), an algebraic equation for the ratio of the two scale factors, $Y(t)/a(t)$. Inserting the PM parameters (\ref{PMpara}) into this equation, we find that it becomes an identity. Clearly, it is the analogue of the equation $\Lambda_g=\Lambda_f$ for proportional backgrounds. But instead of a constant, the equations evaluated on the cosmological ansatz now leave a time-dependent function undetermined. This shows that the cosmological evolution equations of PM bimetric theory are invariant under a symmetry that is local in time. Even if it eventually turns out that a PM symmetry does not exist in the nonlinear theory, a cosmological gauge symmetry could already be of interest on its own. 

Since, in four dimensions, the proportional backgrounds correspond to maximally symmetric space-times with ten independent Killing vectors and the homogeneous and isotropic solutions still possess six isometries, one might speculate that the presence of a symmetry on these solutions could somehow be related to the amount of symmetry of the underlying geometry. Then one could argue that a general solution with less symmetries than the above would not be invariant under any PM symmetry transformation. To invalidate this argument, it is therefore important to investigate the structure of our PM candidate theory away from the proportional and the cosmological backgrounds. This has been done in {\protect{\hyperref[papVIII]{Paper~VIII}}} which considers general perturbative solutions to the bimetric equations of motion. It turns out that the equations in the PM theory are conformally invariant to lowest order in a derivative expansion.
These remarkable results will be presented in section~\ref{secPMCG}.



To conclude this discussion, let us briefly mention that a PM candidate can also be obtained in $d=3$ where the background equation reads
\beqn
c(\beta_1-\alpha\beta_0)+2c^2(\beta_2-\alpha\beta_1)+c^3(\beta_3-\alpha\beta_2)=0\,.
\eeqn
Demanding this to leave $c$ undetermined results in the following PM parameters, 
\beqn
\beta_3=\alpha\beta_2=\alpha^2\beta_1=\alpha^3\beta_0\,.
\eeqn
Again, all but one of the $\beta_n$ parameters are fixed, and the Fierz-Pauli mass sits precisely on the Higuchi bound. 


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Massive gravity limit}\label{sec:PMMG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The PM parameters (\ref{PMpara}) in four space-time dimensions provide an example for a theory in which the coefficients in the interaction potential depend on the mass scale $m_f$ that is taken to infinity in the massive gravity limit that we discussed in section~\ref{sec:MGlim}. In this case, we have to be more careful when taking the limit because the $\beta_n$ parameters will scale as well. The conditions (\ref{PMpara}) fix the relative scale among them but their absolute scale may still be chosen freely. Suppose that $\beta_2$ does not scale when the limit $\alpha=m_f/m_g\rightarrow\infty$ is taken. Then $\beta_0\rightarrow 0$ and $\beta_4\rightarrow\infty$, whereas $\Lambda={\beta_4\,m^4}/{m_f^2}=\,$const.  In the Massive Gravity limit, the equations of motion for the PM theory thus reduce to
\beqn
\mathcal{G}_{\mu\nu}(g)
+\frac{\Lambda}{3}\,g_{\mu\lambda}{\big(Y^{(2)}\big)^\lambda}_{\nu}(S)&=&0\,, \label{gpm} \\
\mathcal{G}_{\mu\nu}(f)
+\Lambda\fmn&=&0 \,.\label{fpm}
\eeqn
Remarkably, these are exactly the equations singled out in \cite{deRham:2012kf, Deser:2013uy, deRham:2013wv} which investigated the possibility of realizing nonlinear partial masslessness in Massive Gravity with fixed reference metric. The methods invoked in those references are completely different from ours and hence provide independent support for the existence of a nonlinear PM symmetry. 

On the other hand, as we already mentioned previously, in \cite{Deser:2013uy, deRham:2013wv} it was also claimed that there is no nonlinear gauge symmetry present in (\ref{gpm}) and (\ref{fpm}). If correct, at first sight, this result might seem to rule out a nonlinear PM symmetry even in bimetric gravity because it should be possible to take the massive gravity limit to arrive at the above equations. There is, however, a caveat in this argument: If the symmetry transformation in PM bimetric gravity itself depends on $\alpha=m_f/m_g$, then it may become singular in the $\alpha\rightarrow\infty$ limit. In this case, it would not be consistent to only look for an invariance in (\ref{gpm}) and (\ref{fpm}) because terms in the original bimetric equations, that were neglected when taking the limit, could become relevant again due to the singular nature of the gauge transformation. In fact, our findings in chapter~\ref{ch:HD} suggest that the transformation of $\fmn$ indeed contains such singular terms and therefore the conclusions of \cite{Deser:2013uy, deRham:2013wv} are irrelevant for bimetric gravity. 


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
\section{Generalization to arbitrary dimensions}\label{PMdgf}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


In {\protect{\hyperref[papVII]{Paper~VII}}} we apply the procedure of identifying the candidate PM theories that we introduced in the previous section to bimetric theory in an arbitrary number of space-time dimensions. We find that in pure Hassan-Rosen bimetric theory there is no nonlinear PM theory for $d>4$. This outcome is in agreement with 3-vertex calculations~\cite{Zinoviev:2006im, Joung:2012rv}, which also suggest that it could be possible to find a nonlinear PM theory in higher dimensions if higher order derivative couplings are included into the theory. Inspired by these results we augment the bimetric action by the ghost-free Lanczos-Lovelock (LL) terms. In this LL-extended bimetric theory it is then possible to identify PM candidates even for $d>4$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background equation}\label{noPMdgeq5}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Let us first argue why in pure bimetric theory there is no PM candidate in dimensions greater than four. To this end, consider again the background equation $\Lambda_g=\Lambda_f$ which in $d$ dimensions assumes the following form,
\beqn\label{eqlad}
(\alpha c)^{d-2}\sum_{n=0}^{d-1}{d-1\choose n}c^n\beta_n
= \sum_{n=1}^{d}{d-1\choose n-1}c^n\beta_n\,.
\eeqn
As in the four-dimensional case, for $c$ to be undetermined by this polynomial equation, the coefficients of different powers of $c$ have to vanish separately. This requirement will again put constraints on the $\beta_n$-parameters and the ratio of Planck masses $\alpha$. It should be obvious that, for large $d$, the factor $c^{d-2}$ on the left-hand side produces a large number of terms with coefficients proportional to just one $\beta_n$-parameter. These $\beta_n$-parameters will then immediately forced to be zero. 
Explicitly, when multiplied by $c^{2-d}$, the above equation can be rewritten as
\beqn
\left( \alpha^{d-2}\sum_{n=0}^{d-1}{d-1\choose n}\beta_n-\sum_{n=3-d}^2{d-1\choose d+n-3}\beta_{n+d-2} \right)c^n=0\,.
\eeqn
In $d\geq 5$, demanding the coefficients of $c^n$ to vanish for $3-d\leq n\leq d-1$ then leads to the following constraints on the parameters,
\begin{align}
0&=\alpha^{d-2}{d-1\choose n}\beta_n-{d-1\choose d+n-3}\beta_{n+d-2} \qquad\text{for}\quad0\leq n\leq 2\,.,\nn\\
0&=\beta_m\qquad\text{for}\quad 1\leq m\leq d-1\,.
\end{align}
The second set of conditions inserted into the first also gives $\beta_0=\beta_d=0$ and hence for $d\geq 5$ all $\beta_n$ must vanish. This choice of parameters of course trivializes the interaction potential. Our conclusion therefore is that there exist no nontrivial parameter values for which the constant part of the gauge transformation leaves the background equations invariant. Hence there is no PM candidate in pure bimetric theory in dimensions greater than four. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bimetric theory with Lanczos-Lovelock terms}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

According to the constructive consistency proof in chapter~\ref{ch:MG}, the interaction potential of the Hassan-Rosen bimetric theory includes all  consistent non-derivative terms. Therefore, the only option to obtain an extended version of the theory is to add more derivative terms to the action. At this point, the only such terms that are expected to be ghost-free consist of the Lanczos-Lovelock invariants which are defined as totally antisymmetric contractions of Riemann tensors $R^{\alpha\beta}_{\phantom{\alpha\beta}\mu\nu}$,
\beqn\label{LLdef}
\mathcal{L}_{(n)}=\frac{1}{2^nn!}\delta^{\mu_1}_{[\alpha_1}\delta^{\nu_1}_{\beta_1}\hdots\delta^{\mu_n}_{\alpha_n}\delta^{\nu_n}_{\beta_n]}
\prod_{k=1}^nR^{\alpha_k\beta_k}_{\phantom{\alpha_k\beta_k}\mu_k\nu_k}\,.
\eeqn
In spite of being higher derivative operators, the LL invariants are believed to avoid inconsistencies that are usually introduced by such terms. This is due to the antisymmetric structure in (\ref{LLdef}) which ensures the absence of more than two time derivatives acting on one field in the action. It is interesting that the same structure appears in the interaction potential of ghost-free bimetric theory, but of course this is not really a coincidence: In the decoupling limit of nonlinear massive gravity it can be seen that the antisymmetric structure removes higher time derivatives from the longitudinal modes of the St\"uckelberg fields.  

Hoping to rediscover the possibility of finding PM candidates in $d>4$, we thus choose to extend the Hassan-Rosen bimetric action by the following terms,\footnote{In a different context, consistent bimetric theory extended by LL terms has already been considered in~\cite{Paulos:2012xe}.}
\begin{align}\label{LLaction}
S_\mathrm{LL}~&=~~m_g^{d-2}\int\dd^dx\sum_{n=2}^{[d/2]}\sqrt{-g}~l_n^g\,\mathcal{L}_{(n)}(g)\nn\\
&~+~m_f^{d-2}\int\dd^dx\sum_{n=2}^{[d/2]}\sqrt{-f}~l_n^f\,\mathcal{L}_{(n)}(f)\,,
\end{align}
where we have introduced two sets of couplings, $l_n^g$ and $l_n^f$, of mass dimension $2(1-n)$.
Furthermore, it is well known that the LL invariant $\mathcal{L}_{(n)}$ is topological in $d=2n$ and vanishes for $2n>d$ which is why the sums in (\ref{LLaction}) terminate at integer part of $d/2$. 



The equations of motion for $\gmn$ and $\fmn$ that follow from the LL extended bimetric action are
\beqn\label{LLeom}
\mathcal{G}_{\mu\nu}(g)+\sum_{n=2}^{[d/2]}l_n^g\mathcal{G}^{(n)}_{\mu\nu}(g)+\frac{m^d}{m_g^{d-2}}V^g_{\mu\nu}&=&0\,, \nn\\
\mathcal{G}_{\mu\nu}(f)+\sum_{n=2}^{[d/2]}l_n^f\mathcal{G}^{(n)}_{\mu\nu}(f)+\frac{m^d}{m_g^{d-2}}V^f_{\mu\nu}&=&0\,.
\eeqn
Here, $\mathcal{G}^{(n)}_{\mu\nu}$ are the Lovelock tensors that follow from variation of (\ref{LLaction}) and $V^g_{\mu\nu}$ and $V^f_{\mu\nu}$ are the contributions from the interaction potential which were defined in (\ref{poteom}). We will not need the explicit expressions for the Lovelock tensors, but let us note the important property,
\beqn\label{usefid}
g^{\mu\nu}\mathcal{G}^{(n)}_{\mu\nu}(g)=\frac{2n-d}{2}\mathcal{L}_{(n)}(g)\,,
\eeqn
which will be useful in what follows.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proportional backgrounds}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As in pure bimetric theory we are interested in the proportional background solutions to (\ref{LLeom}) and perturbations around those. Again, these backgrounds correspond to maximally symmetric spacetimes, for which the curvatures satisfy
\beqn\label{bgcurv}
R_{\mu\nu\rho\sigma}(\bar{g})&=&\frac{2\lambda}{(d-1)(d-2)}(\bar{g}_{\mu\rho}\bar{g}_{\nu\sigma}-\bar{g}_{\nu\rho}\bar{g}_{\mu\sigma})\,,\nn\\
R_{\mu\nu}(\bar{g})&=&\frac{2\lambda}{d-2}\bgmn\,,\qquad R(\bar{g})~=~\frac{2d\,\lambda}{d-2}\,,
\eeqn
with cosmological constant $\lambda$. On such backgrounds with constant curvature, the $n$-th order LL invariant is proportional to $\lambda^n$,
\beqn\label{LLbg}
\mathcal{L}_{(n)}=N_n(d)\,\lambda^n\,,\quad\text{with}~~N_n(d)\equiv\frac{2^n d!}{(d-1)^n(d-2)^n(d-2n)!}\,.
\eeqn
Next, we trace the equations of motion (\ref{LLeom}) in order to obtain two scalar equations and insert (\ref{bgcurv}) for the curvatures.
Furthermore, we make use of the identity (\ref{usefid}) and plug in the proportional ansatz, $\bfmn=c^2\bgmn$. 
Finally, in the equation for $\fmn$, we use $\mathcal{L}_{(n)}(c^2 \bar{g})=c^{-2n}\mathcal{L}_{(n)}( \bar{g})$. The resulting two equations read
\beqn\label{LLbgeq}
\lambda + \sum_{n=2}^{[d/2]}l^g_n\frac{d-2n}{2d}N_n(d)\lambda^n - \Lambda_g&=&0\,,\nn\\
\lambda + \sum_{n=2}^{[d/2]}c^{2-2n}l^f_n\frac{d-2n}{2d}N_n(d)\lambda^n - \Lambda_f&=&0\,.
\eeqn
Here, $\Lambda_g$ and $\Lambda_f$ are the contributions from the potential evaluated on the proportional backgrounds which defined earlier in (\ref{lambdas}). Note, however, that these no longer correspond to the physical cosmological constants and are not necessarily equal. 

For general parameters $\beta_n$, $l_n^g$, and $l_n^f$, the two algebraic equations in (\ref{LLbgeq}) serve to determine the background curvature $\lambda$ as well as the proportionality constant $c^2$. Note also that in the absence of the LL contributions, i.e.~for $l_n^g=l_n^f=0$, we rearrive at the bimetric background equations, $R(\bar{g})=\tfrac{2d}{d-2}\Lambda_g$ and $\Lambda_g=\Lambda_f$. Eventually, we will again be looking for the parameter values for which the equations (\ref{LLbgeq}) leave $c$ undetermined.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear Perturbations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Computing the linearized equations of motion from (\ref{LLeom}) is quite involved. Fortunately, it has been observed in \cite{Sisman:2012rc} that, around constant curvature backgrounds with cosmological constant $\lambda$, the fluctuation equations of General Relativity augmented by the LL terms with couplings $l_n^g$ assume the same form as the ones obtained from Einstein's equations. The only difference is that, in the linearized equations of the LL extended theory, the Planck mass $m_g$ needs to be replaced by an effective mass parameter $\tilde{m}_g$ defined through
\beqn\label{modmg}
\frac{\tilde{m}_g^{d-2}}{m_g^{d-2}}=1+(d-3)!\sum_{n=2}^{[d/2]}\frac{n(d-2n)l_n^g}{(d-2n)!}\left(\frac{2\lambda}{(d-1)(d-2)}\right)^{n-1}.
\eeqn
It is a remarkable feature of the Lovelock invariants that, in spite of being higher-derivative operators in the nonlinear theory, they give rise to linearized equations that are only second order in derivatives.

For the bimetric case the above result implies that the linear equations for the theory with LL terms are the same as in pure bimetric theory if one replaces $m_g$ by $\tilde{m}_g$ as above and $m_f$ by $\tilde{m}_f$ given by
\beqn\label{modmf}
\frac{\tilde{m}_f^{d-2}}{m_f^{d-2}}=1+(d-3)!\sum_{n=2}^{[d/2]}\frac{n(d-2n)c^{2-2n}l_n^f}{(d-2n)!}\left(\frac{2\lambda}{(d-1)(d-2)}\right)^{n-1}.
\eeqn
Hence, thanks to the results of~\cite{Sisman:2012rc}, without any computation we can conclude that the linear equations in a maximally symmetric background with cosmological constant $\lambda$ will again diagonalize into a massless and massive equation, where in the latter the Fierz-Pauli mass (\ref{FPmass}) is now given in terms of $\tilde{m}_g$ and $\tilde{m}_f$. Due to this similarity, the linear equations are again invariant under the usual PM symmetry (\ref{linPMsym}) if the mass is on the Higuchi bound, $m_{\mathrm{FP}}^2=\frac{2}{d-1}\lambda$. One can then hope that it is possible to find a nonlinear candidate PM theory within this generalized setup.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{PM candidates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We apply the same logic as in the four-dimensional case to LL extended bimetric theory:
For extending the linear PM symmetry to the nonlinear level, we need to be able to shift the proportionality constant $c^2$ and hence, in a PM candidate theory, the background equations (\ref{LLbgeq}) must not determine it. In order to see for which parameter values this is possible, we must first solve a combination of the two equations for $\lambda$, eliminate it from the remaining equation, and demand the result to be independent of $c$. 

Although this procedure sounds again straightforward, in practice, it cannot always be carried out immediately. Complications arise because the background equations (\ref{LLbgeq}) are polynomials of order $[d/2]$ in $\lambda$ and solving them does not result in a polynomial expression for $\lambda$ as a function of $c$. Therefore, generically, the equation that is supposed to leave $c$ undetermined is not a polynomial in $c$ and it becomes difficult to impose the requirement on the PM theory. 

Nevertheless, for small enough $d$ it is possible to arrive at a polynomial equation in $c$ and the analysis can be carried out. As an example, we present the analytical results in $d=5$ before summarizing the outcome of a computer-based analysis for dimensions up to $d=8$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Partial masslessness in $d=5$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In five space-time dimensions the equations are still simple enough to be solved by hand. The only nontrivial LL term is $\mathcal{L}_{(2)}$, also known as the Gauss-Bonnet combination,
\beqn\label{gaussbonnet}
\mathcal{L}_{(2)}=R^2-4R_{\mu\nu}R^{\mu\nu}+R_{\mu\nu\rho\sigma}R^{\mu\nu\rho\sigma}\,,
\eeqn
which is topological in $d=4$. 
When terms of this kind for both $\gmn$ and $\fmn$ are added to the bimetric action, the background equations (\ref{LLbgeq}) take the following form,
\beqn\label{bgeqLL5}
\lambda+\frac{l_2^g}{3}\lambda^2-\Lambda_g=0\,,\qquad
\lambda+\frac{l_2^f}{3c^2}\lambda^2-\Lambda_f=0\,.
\eeqn
Here the contributions from the interaction potential read
\beqn\label{contpotf}
\Lambda_g&=&\frac{m^5}{m_g^3}(\beta_0+4c\beta_1+6c^2\beta_2+4c^3\beta_3+c^4\beta_4)\,,\nn\\
\Lambda_f&=&\frac{m^5}{m_g^3(\alpha c)^3}(c\beta_1+4c^2\beta_2+6c^3\beta_3+4c^4\beta_4+c^5\beta_5)\,.
\eeqn
The system (\ref{bgeqLL5}) can easily be solved for $\lambda$ by building a linear combination of the equations in which the quadratic terms cancel out. This gives
\beqn
\lambda=\frac{c^2l_2^g\Lambda_f-l_2^f\Lambda_g}{c^2l_2^g-l_2^f}\,.
\eeqn
Plugging this result back into the difference of the two equations in (\ref{bgeqLL5}) results in a polynomial equation for $c$,
\beqn
l_2^g(l\Lambda_g-c^2\Lambda_f)^2+3(c^4-lc^2)(\Lambda_g-\Lambda_f)=0\,,
\eeqn
where, for notational simplicity, we have defined $l\equiv l_2^f/l_2^g$. After the expressions in (\ref{contpotf}) have been inserted, the left-hand side of this equation contains nine different powers of $c$. Demanding each coefficient to vanish, we obtain nine constraints on the parameters of the theory. As in the four-dimensional case, these constraints are not all independent, but they fix exactly seven out of the eight parameters $\{\beta_n, l_2^g, l_2^f\}$. The resulting values are
\begin{align}\label{PMvalf}
-\tfrac{1}{10}\beta_0&=\tfrac{1}{2\alpha}\beta_1=-\tfrac{1}{\alpha^2}\beta_2=-\tfrac{1}{\alpha^3}\beta_3=\tfrac{1}{2\alpha^4}\beta_4=-\tfrac{1}{10\alpha^5}\beta_5=\tfrac{m_g^3}{l_2^gm^5}\,,\nn\\
l_2^g&=\alpha^2l_f\,.
\end{align}
These parameters satisfy $\alpha^{5-n}\beta_n=\alpha^n\beta_{5-n}$ as well as $l_f=\alpha^{2-2n}l_n^g$, and hence the PM candidate theory is again symmetric under the interchange $\alpha^{-1}\gmn \leftrightarrow \alpha\fmn$. Using expression~(\ref{FPmass}) for the Fierz-Pauli mass with $m_g$ and $m_f$ replaced by the modified Planck masses given in (\ref{modmg}) and (\ref{modmf}), it is also straightforward to check that the Higuchi bound, $m_\mathrm{FP}^2=\frac{1}{2}\lambda$, is saturated. 

Note furthermore that one cannot set the Lovelock couplings $l_2^g$ and $l^f_2$ to zero because the $\beta_n$-parameters are inversely proportional to them. This is of course consistent with our findings in section \ref{noPMdgeq5}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Partial masslessness in $d>5$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The analysis in $d=6$ is very similar to the five-dimensional case since the only contributing LL term is still $\mathcal{L}_{(2)}$. Up to the sign of $\beta_3$, all but one of the parameters become fixed again. Their values are given in {\protect{\hyperref[papVII]{Paper VII}}}.

For dimensions greater than six, the cubic LL term $\mathcal{L}_{(3)}$ needs to be included into the action. According to (\ref{LLbg}), on the proportional backgrounds it reduces to $N_3(d)\lambda^3$. Hence the background equations (\ref{LLbgeq}) will now be cubic polynomials in $\lambda$. One can subtract the cubic term by building a linear combination of the two equations to arrive at a quadratic equation. But then the solution for $\lambda$ will invole a square root and, as a result, the equation determining $c$ will no longer be a polynomial. This complicates the determination of the PM parameters because we cannot apply our method, which proved successful in $d\leq 6$, to a non-polynomial equation. However, there is another possibility of solving the background equations (\ref{LLbgeq}): One can decompose them into a Gr\"obner basis of equivalent polynomial equations and thereby reduce the equation for $\lambda$ to a linear one. In addition, one obtains a consistency condition that is a polynomial in $c$ and can be used to impose the requirement for partial masslessness. Following this strategy, it is in principle possible to identify PM candidates in any dimension. The computational effort, however, becomes very large already when the quartic LL term $\mathcal{L}_{(4)}$ is included in the theory. Even with the help of a computer it was therefore only possible to determine the PM parameters in dimensions up to $d=8$ where $\mathcal{L}_{(4)}$ still does not contribute to the equations of motion. The results are summarized in Table~1 of {\protect{\hyperref[papVII]{Paper~VII}}}.  

As could have been anticipated, the PM parameters always satisfy the symmetry relations $\alpha^{d-n}\beta_n=\alpha^n\beta_{d-n}$ as well as $l_n^f=\alpha^{2-2n}l_n^g$.
The value for the Fierz-Pauli mass turns out to saturate the Higuchi bound in all cases. The fact that the scale invariance of the background and the PM gauge symmetry at the level of perturbations always coincide is entirely nontrivial and supports the validity of our approach.
Interestingly, there is no PM candidate in seven spacetime dimensions.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Relation to Higher-Curvature Gravity}
\label{ch:HD}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this chapter we discuss modified theories of gravity with higher powers of curvatures. A particular class of theories with at most four derivatives, including the famous examples of New Massive Gravity and Conformal Gravity, is known to be free of the Boulware-Deser ghost. However, one of the two spin-2 modes in these theories shows unavoidable ghost instabilities in all its helicity components. This has been an unresolved problem challenging the otherwise promising models of modified gravity. 

On the other hand, bimetric gravity with a large value for the Fierz-Pauli mass contains a heavy spin-2 excitation, and integrating out this field results in an effective theory for just one rank-2 tensor. In general, this effective action will be nonlocal, i.e.~it will not simply be an expansion in higher curvatures but involve inverted differential operators. However, in {\protect{\hyperref[papVIII]{Paper~VIII}}} we point out a definite relation among an effective action obtained from bimetric theory and the higher-curvature theories that avoid the Boulware-Deser ghost. We obtain a mapping between the two classes of theories and thereby also solve the ghost problem of the quadratic curvature theories by completing them into an infinite series of curvature terms. Furthermore, it is shown that, to lowest order in a derivative expansion, the effective theory obtained from the PM candidate introduced in chapter~\ref{ch:PM} is equivalent to Conformal Gravity.

Before explaining our method and presenting the results, we begin this chapter with a brief review of the relevant higher-curvature theories.  





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Higher-curvature gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
When viewed as a quantum theory, General Relativity is nonrenormalizable in the usual power-counting sense, which can be seen from the fact that, after canonical normalization of the fluctuations, the coupling constants of the nonlinear interactions have negative mass dimensions. Therefore the theory can be meaningful only as an effective theory which is valid at low energies and possesses a fully consistent (yet unknown) UV completion. One promising candidate for the theory at high energies is String Theory which is indeed a consistent quantum theory containing gravity as well as gauge theories that could reduce to the Standard Model of Particle Physics at low energies. In the framework of String Theory it is possible to derive the effective low-energy action for the metric $\gmn$ by integrating out heavy string states, which results in an expansion in curvatures suppressed by the mass scale of the heavy string excitations. String Theory theorefore constitutes one example of how higher-curvature terms enter the effective action. In general, the concept of effective field theory tells us that such corrections to the Einstein-Hilbert term are expected to arise from any UV completion. 


The most relevant correction to Einstein gravity is quadratic in curvatures for $\gmn$. The only possible (local) terms that can arise at this order are $R_{\mu\nu\rho\sigma}R^{\mu\nu\rho\sigma}$, $R_{\mu\nu}R^{\mu\nu}$ and $R^2$. In principle, we should also expect covariant derivatives acting on curvatures in the action, but due to the Bianchi identity the only possible term at quadratic order is $\Box R$ which is a total derivative. Also note that we can choose to complete the term $R_{\mu\nu\rho\sigma}R^{\mu\nu\rho\sigma}$ into the quadratic Lanczos-Lovelock combination~(\ref{gaussbonnet}) which we do not consider in this chapter but in principle can always be added to the action in $d>4$. One therefore only needs to take into account the terms $R_{\mu\nu}R^{\mu\nu}$ and $R^2$. It then turns out that the relative coefficient between these two contributions in the action is fixed by demanding the absence of the Boulware-Deser ghost, and the corresponding effective action truncated to a four-derivative theory is given by~\cite{Stelle:1976gc, Stelle:1977ry},
\begin{align}\label{HDact}
    S_\mathrm{HD}^{(2)}=m_g^{d-2}\int\dd^dx\sqrt{g}\,\Big[ &c_\Lambda+c_RR(g)\nn\\
    &-\frac{c_{RR}}{m^2}\left(R^{\mu\nu}R_{\mu\nu}-\frac{d}{4(d-1)}R^2\right) \Big]\,.
\end{align}
Here, $c_\Lambda$ is a cosmological constant term with mass dimension two, while $c_R$ and $c_{RR}$ are dimensionless coefficients. Furthermore, $m$ is the energy scale at which the effective field theory looses its validity. The relative coefficient between the two quadratic curvature terms is fixed to be equal to~$\frac{-d}{4(d-1)}$ which, as we shall now demonstrate, results in a mass term with the Fierz-Pauli combination at the linearized level. In order to see this, let us introduce an auxiliary tensor field $\varphi_{\mu\nu}$ into the theory, which we take to be symmetric in its indices. In terms of this new field we can write an equivalent action as follows,
\begin{align}\label{auxact}
    S_\mathrm{aux}=m_g^{d-2}\int\dd^dx\sqrt{g}\,\Big[ c_\Lambda+c_R&R(g) -\mathcal{G}_{\mu\nu}\varphi^{\mu\nu} \nn\\
    &+\frac{m^2}{4c_{RR}}(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,.
\end{align}
Here, $\mathcal{G}_{\mu\nu}$ is the Einstein tensor for $\gmn$ and the indices on the symmetric tensor $\varphi_{\mu\nu}$ are raised and lowered with~$\gmn$. As is easily verified, the solution to the equations of motion for $\varphi_{\mu\nu}$ reads
\beqn\label{phiauxeom}
\varphi_{\mu\nu}=\frac{2c_{RR}}{m^2}\left(\mathcal{G}_{\mu\nu}-\frac{1}{d-1}\mathcal{G}\gmn\right)\,,
\eeqn
which can be plugged back into (\ref{auxact}) to rearrive at (\ref{HDact}). Hence, we have defined a two-derivative theory involving an auxiliary field which can be integrated out to return to the higher-derivative action.

If now $c_\Lambda=0$ then $\bgmn=\emn$ and $\bar{\varphi}_{\mu\nu}=0$ solve both~(\ref{phiauxeom}) as well as the $\gmn$ equations. We then consider the quadratic action for fluctuations~$\varphi_{\mu\nu}$ and $\hmn=\gmn-\emn$ around this background, 
\begin{align}\label{quadactaux}
S_\mathrm{aux}^{\mathrm{lin}}=\tfrac{m_g^{d-2}}{4}\int\dd^dx\Big[h_{\mu\nu}\mathcal{E}^{\mu\nu\rho\sigma}\Big(c_{R}&h_{\rho\sigma}+\tfrac{d-2}{2}\varphi_{\rho\sigma}\Big)\nn\\
&+\tfrac{m^2}{c_{RR}}(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,,
\end{align}
where the linearized Einstein operator $\mathcal{E}^{\mu\nu\rho\sigma}$ in flat space was already given in (\ref{kinstruc1}). The kinetic terms are not diagonal, which motivates us to make the following linear redefinitions,
\beqn
\hmn'\equiv\tfrac{1}{2}m_g^{(d-2)/2} \hmn+\tfrac{d-2}{4}\tfrac{1}{c_R}\varphi_{\mu\nu}\,,\quad~~
 \varphi_{\mu\nu}'\equiv\tfrac{d-2}{4\sqrt{2}}\,m_g^{(d-2)/2}\varphi_{\mu\nu}\,,
\eeqn
where the normalizations in front have been chosen conveniently. These redefinitions diagonalize $S_\mathrm{aux}^{\mathrm{lin}}$ into an action for a massless spin-2 fluctuation $h'_{\mu\nu}$ and a massive spin-2 fluctuation $\varphi'_{\mu\nu}$,
\begin{align}\label{diagactaux}
S_\mathrm{aux}^{\mathrm{lin}}=\int\dd^dx\Big(c_Rh'_{\mu\nu}\mathcal{E}^{\mu\nu\rho\sigma}&h'_{\rho\sigma}-\tfrac{1}{c_R}\varphi'^{\mu\nu}\mathcal{E}^{\mu\nu\rho\sigma}\varphi'_{\rho\sigma}\nn\\
&+\tfrac{(d-2)^2}{16}\tfrac{m^2}{c_{RR}}(\varphi'^{\mu\nu}\varphi'_{\mu\nu}-\varphi'^2)\Big)\,.
\end{align}
As promised, the mass term has the Fierz-Pauli structure, which would not have been the case had we started with a different relative coefficient between the two quadratic-curvature terms in (\ref{HDact}). Furthermore, the sign of $c_{RR}$ determines the sign of the squared Fierz-Pauli mass and can be adjusted such that it is non-tachyonic.
On the other hand, the signs of the kinetic terms for the massless and massive spin-2 fluctuations are determined by the coefficient $c_R$ alone, and it is evident that they will always have opposite signs. As a consequence, it is unavoidable that either the massless or the massive fluctuation will be a ghost. Note that this ghost is not an extra degree of freedom and, in particular, it does not correspond to the Boulware-Deser instability. Instead, all helicity components of the massless or massive spin-2 fluctuation themselves suffer from a ghost-like kinetic term. This is a manifestation of Ostrogradski's theorem~\cite{Ostrogradski} which states that any theory with $N$ time derivatives, for $2<N<\infty$, is plagued by ghosts. Therefore the above higher-curvature action, despite being free of the Boulware-Deser ghost, is not consistent.
 
Before presenting the relation among higher-curvature gravity and Hassan-Rosen bimetric theory, let us briefly mention two popular examples for actions of the type (\ref{HDact}): New Massive Gravity in three and Conformal Gravity in four space-time dimensions.



    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsubsection{New Massive Gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As we already explained in section \ref{sec:FP}, the number degrees of freedom of a massless spin-2 particle in $d$ dimensions is $d(d-3)/2$. It follows that in $d=3$, there is no propagating massless spin-2 mode. This observation motivated the authors of \cite{Bergshoeff:2009hq, Bergshoeff:2009aq} to choose $c_R<0$ and $c_{RR}<0$ in the higher-curvature action~(\ref{HDact}) for the case $d=3$. As can be seen in the linearized auxiliary action~(\ref{diagactaux}), this choice renders the massive field healthy and turns the massless field into a ghost. However, since the massless field is not a propagating degree of freedom, the wrong sign in front of its kinetic term does not lead to an inconsistency in the theory. The higher-derivative action with these sign choices became very popular under the name \textit{New Massive Gravity}. Of course, the trick employed in \cite{Bergshoeff:2009hq, Bergshoeff:2009aq} fails to work in dimensions greater than three where the massless mode is propagating and ghost-like for $c_R<0$. In the past, the construction of a consistent higher-derivative theory in $d>3$ has therefore not been successful~\cite{Kleinschmidt:2012rs}. There have also been attempts to complete New Massive Gravity to a theory with infinitely many derivatives (see e.g.~\cite{Gullu:2010pc, Paulos:2010ke}) which could in principle avoid Ostrogradski's theorem and cure the ghost problem even in higher dimensions. We obtain such a completion in {\protect{\hyperref[papVIII]{Paper~VIII}}} where we show that the Hassan-Rosen bimetric theory when written as an effective theory for one of the metrics is closely related to New Massive Gravity in three and its generalized form in higher dimensions. Moreover, the spin-2 ghost that is unavoidably contained in (\ref{HDact}) is argued to arise from the truncation of an infinite derivative expansion to a four-derivative theory. This proposes the Hassan-Rosen bimetric action as a consistent nonlinear completion of the higher-derivative theory~(\ref{HDact}) in any number of space-time dimensions.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Conformal Gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In four spacetime dimensions, there is a particular choice of parameters for which the higher-derivative action (\ref{HDact}) develops a new gauge symmetry. 
Namely, if we set $c_\Lambda=c_R=0$ then the only terms left in the action are the four-derivative terms,~\cite{Bach} 
\beqn\label{CGact}
    S_\mathrm{CG}=-\frac{m_g^2c_{RR}}{m^2}\int\dd^4x\sqrt{g}\,\left(R^{\mu\nu}R_{\mu\nu}-\frac{1}{3}R^2\right)\,.
\eeqn
With help of the curvature relations (\ref{curvrel}) it is straightforward to show that this action is invariant under conformal transformations of the metric, 
\beqn\label{conftrafo}
\gmn\rightarrow \xi^2(x)\gmn\,,
\eeqn
where $\xi(x)$ is a local gauge parameter.
The theory therefore goes under the name of \textit{Conformal Gravity}. The cosmological constant and the Einstein-Hilbert term are not invariant under the transformation (\ref{conftrafo}) which is why their coefficients had to be set to zero.


The equations of motions that follow from variation of the conformal gravity action (\ref{CGact}) imply the vanishing of the Bach tensor for~$\gmn$,
\beqn\label{Bacheq}
   B_{\mu\nu}\equiv -\nabla^2 P_{\mu\nu}+\nabla^{\rho}\nabla_{(\mu}P_{\nu)\rho}+W_{\rho\mu\nu\sigma}P^{\rho\sigma}=0\,.
\eeqn 
Here, we have given the definition of $B_{\mu\nu}$ in terms of the Schouten tensor,
\beqn\label{schouten}
P_{\mu\nu}\equiv R_{\mu\nu}-\frac{1}{2(d-1)}\gmn R\,,
\eeqn
as well as the Weyl tensor,\footnote{In the literature, the Conformal Gravity action~(\ref{CGact}) is sometimes also expressed as the square of the Weyl tensor, $\mathcal{L}_\mathrm{CG}\propto\sqrt{g}\,W_{\rho\mu\nu\sigma}W^{\rho\mu\nu\sigma}$.}
\beqn
W_{\rho\mu\nu\sigma}\equiv R_{\rho\mu\nu\sigma}+g_{\mu[\nu}R_{\sigma]\rho}-g_{\rho[\nu}R_{\sigma]\mu}+\frac{1}{3}g_{\rho[\nu}g_{\sigma]\mu}R\,.
\eeqn 
The Bach tensor is invariant under conformal transformations in four space-time dimensions~\cite{Bach}.


The Conformal Gravity action is closely related to the linear theory for a partially massless spin-2 field discussed in section~\ref{seclinPM}. In order to see this, we again need to introduce an auxiliary field $\varphi_{\mu\nu}$. But since the equations of motion that follow from the above auxiliary action are consistent with vanishing background for $\varphi_{\mu\nu}$ only if $\gmn$ is flat, $S_\mathrm{aux}$ in (\ref{auxact}) needs to be slightly modified in order to give rise to more general de Sitter solutions for which the linear PM symmetry is known to exist. More precisely, one needs to add a linear term proportional to $\varphi=g^{\mu\nu} \varphi_{\mu\nu}$ such that $\mathcal{G}_{\mu\nu}(\bar{g})=\Lambda\bgmn$ with $\Lambda=$ const.~and $\bar{\varphi}_{\mu\nu}=0$ now solve the equations of motion. Instead of writing down the auxiliary action in the general case, here we only give the expression for Conformal Gravity which reads~\cite{Kaku:1977pa}
\begin{align}\label{CGauxact}
    S_\mathrm{CG}^{(2)}=\tfrac{4c_{RR}m_g^{2}\Lambda}{m^2}\int\dd^dx\sqrt{g}\,\Big[ \tfrac{1}{6}(R&-2\Lambda)+\varphi^{\mu\nu}\mathcal{G}_{\mu\nu} \nn\\
    &+ \Lambda\varphi+ \Lambda(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,.
\end{align}
Linearization around the constant curvature background and diagonalization into mass eigenstates shows that, for $c_{RR}>0$, the theory propagates a healthy massless and a ghost-like massive spin-2 particle. Moreover, the Fierz-Pauli mass of the massive fluctuation has the value corresponding to the Higuchi bound, $m_\mathrm{FP}^2=\frac{2}{3}\Lambda$, which implies the presence of the PM gauge symmetry (\ref{linPMsym}) for $\varphi_{\mu\nu}$. The massless fluctuation $\hmn'$ does not transform under this symmetry.
In fact, it is a simple exercise to check that, in addition to the obvious diffeomorphism invariance, the full nonlinear auxiliary action (\ref{CGauxact}) is invariant under the following linear gauge transformations~\cite{Deser:2012qg},
\beqn
\delta\gmn=2\xi(x)\gmn\,,\qquad \delta\varphi_{\mu\nu}=(\nabla_\mu\partial_\nu+\tfrac{\Lambda}{3})\xi(x)\,.
\eeqn
Note that the nonlinear field $\gmn$ transforms under the PM symmetry because its fluctuation does not correspond to the massless mode but is a linear superposition of mass eigenstates. Its transformation is of course nothing but the linear version of the conformal transformation (\ref{conftrafo}).

Conformal Gravity, or its equivalent form (\ref{CGauxact}), therefore describes only six propagating degrees of freedom instead of seven that would correspond to a massless and a massive spin-2 field. For more detailed discussions of its spectrum we refer the reader to \cite{Fradkin:1981iu, Lee:1982cp, Riegert:1984hf, Maldacena:2011mk}. 

Like any other conformal field theory, $S_\mathrm{CG}$ does not contain any dimensionful couplings and therefore avoids the nonrenormalizibility problem of General Relativity. Being a renormalizable field theory, conformal gravity has been suggested as a quantum theory for gravity. It has also been shown to allow for viable cosmological solutions and even fit galaxy rotation curves, providing a possible solution for at least part of the dark matter problem~\cite{Mannheim:2011ds}. 

Unfortunately, all of these promising features remain irrelevant unless a cure for the ghost problem is found. Suggestions for altering the theory in order to make it healthy include, for instance, a modification of quantum mechanics~\cite{Bender:2007wu} and the addition of specific boundary conditions~\cite{Maldacena:2011mk}, but none of these seemed sufficiently convincing for the theory to be accepted as a consistent alternative to General Relativity. 

In order to avoid the inconsistencies that plague theories with a finite number of higher derivatives, another possible solution is to complete the equations of motion~(\ref{Bacheq}) of Conformal Gravity with an infinite number of derivatives for which Ostrodgradski's theorem does not hold. Higher-derivative terms will, of course, break the conformal symmetry because they necessarily enter with a suppressing mass scale. On the other hand, one could imagine that the symmetry transformation needs to be completed with an infinite number of higher-derivative terms as well, in order to be a gauge symmetry of the full theory. In that case, both the equations of motion and the symmetry transformation could be thought of as a perturbative expansion in derivatives. Order by order, the equations would be invariant under the gauge symmetry, starting with the Bach tensor and its conformal invariance at lowest order. Although this idea sounds promising, without any further input it is difficult to guess the form of the higher-derivative corrections to the Bach equation that could give rise to such a gauge symmetry. It would therefore be helpful to have a guideline telling us how to construct these terms.

In section~\ref{secPMCG} we will see that the candidate for partially massless bimetric gravity introduced in section~\ref{secPmnonlin}, when written as an effective theory for $\gmn$, is equivalent to Conformal Gravity to lowest order in a derivative expansion. 
This observation motivates us to propose PM bimetric theory as a nonlinear ghost-free completion of Conformal Gravity. 
As in the case of general $\beta_n$ parameters that lead to the higher-curvature theory in (\ref{HDact}), the spin-2 ghost in Conformal Gravity is argued to be an artifact of truncating the full bimetric action to a four-derivative theory.
If our PM model possesses a nonlinear gauge symmetry then so does the corresponding effective theory for $\gmn$. Moreover, the derivative expansions of both the equations of motions for $\gmn$ and of the gauge symmetry can be constructed in a straightforward way.
This relation to the successful (but inconsistent) theory of Conformal Gravity turns ghost-free PM bimetric theory into a particularly interesting model.

   



%\begin{align}\label{auxactn}
    %S_\mathrm{aux}=m_g^{d-2}\int\dd^dx\sqrt{g}\,\Big[ \Big(&c_\Lambda+\tfrac{d}{d-1}c_{RR}m^2\Big)+\left(c_R-\tfrac{d-2}{d-1}c_{RR} \right)R(g) 
    %\nn\\
    %+\mathcal{G}_{\mu\nu}\varphi^{\mu\nu} &+m^2\varphi
    %-\frac{m^2}{4c_{RR}}(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,.
%\end{align}
%Here $\mathcal{G}_{\mu\nu}$ is the Einstein tensor for $\gmn$ and the indices on the symmetric tensor $\varphi_{\mu\nu}$ are raised and lowered with~$\gmn$. As is easily verified, the solution to the equations of motion for $\varphi_{\mu\nu}$ reads
%\beqn\label{phiauxeom}
%\varphi_{\mu\nu}=\frac{2c_{RR}}{m^2}\left(\mathcal{G}_{\mu\nu}-\frac{1}{d-1}\mathcal{G}\gmn-\frac{m^2}{d-1}\gmn\right)\,,
%\eeqn
%which can be plugged back into (\ref{auxact}) to reobtain (\ref{HDact}). 










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Relation to bimetric theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We now return to Hassan-Rosen bimetric gravity with the intention to demonstrate its close relation to the higher-curvature actions discussed above. First we outline two not entirely equivalent procedures of obtaining an effective action for one of the metrics by integrating out the other. Then we show that one of the procedures leads to the higher-derivative theory in~(\ref{HDact}) plus higher curvature corrections. Finally, we consider the PM bimetric theory as a particular example and demonstrate its equivalence to Conformal Gravity to lowest order in derivatives both at the level of the action and the equations of motion.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effective theories for $\gmn$}\label{sec:outl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Consider the two equations of motion obtained from varying the bimetric action (\ref{HR}) with respect to one of the two metrics while the other is held constant. Schematically, we write them as
\beqn
\mathcal{E}^g_{\mu\nu}(g,f)\equiv\left.\frac{\delta S_\mathrm{HR}}{\delta g^{\mu\nu}}\right|_{f}=0\,,\qquad \mathcal{E}^f_{\mu\nu}(g,f)\equiv\left.\frac{\delta S_\mathrm{HR}}{\delta f^{\mu\nu}}\right|_{g}=0\,.
\eeqn
Their explicit forms are given in (\ref{geq}) and (\ref{feq}), respectively, but are not important to us at this stage because our considerations here will be completely general. Suppose now that we intend to use one of the equations to express $\fmn$ in terms of $\gmn$ and then eliminate it in the second equation. For instance, we can think of obtaining a solution for $\fmn$ from its own equation of motion and plugging it into the $\gmn$ equation, such that we get an effective equation for $\gmn$,
\beqn\label{effeq1}
\mathcal{E}^g_{\mu\nu}(g, f(g))=0\,.
\eeqn
This equation will be nonlocal because solving the~$\fmn$ equation for $\fmn$ requires inverting derivative operators, leading to a nonlocal expression for $\fmn$ as a function of $\gmn$.

A more convenient way to arrive at an effective equation for $\gmn$ is to start instead by solving the $\gmn$ equation for $\fmn$, because this equation does not involve derivatives of $\fmn$.  This strategy therefore leads to an algebraic expression for $\fmn$ in terms of curvatures of $\gmn$. For general parameters in the potential, this solution can be obtained perturbatively as an infinite series in $R_{\mu\nu}(g)/m^2$. Plugging it into the other equation then results in a local effective equation for $\gmn$,
\beqn\label{effeq2}
\mathcal{E}^f_{\mu\nu}(g, f(g))=0\,,
\eeqn
which will acquire the form of a derivative expansion. Note that the two procedures of deriving an effective equation for $\gmn$ are completely equivalent: Both methods involved solving one subset of the system of equations and using these solutions in the remaining equations. Hence, the solutions to the two different effective equations for $\gmn$ will be identical in both cases.

Next let us address the question whether it is possible to derive equations (\ref{effeq1}) and (\ref{effeq2}) from an action principle. In both cases this clearly requires finding an effective action for $\gmn$. Let us first suppose that we have solved for $\fmn$ using its own equation of motion. Then we can plug this solution back into the action to obtain an effective action $S_\mathrm{eff}(g)=S_\mathrm{HR}(g, f(g))$ for $\gmn$. Variation of $S_\mathrm{eff}(g)$ then gives
\beqn\label{fpvar}
\frac{\delta S_\mathrm{eff}(g)}{\delta g^{\mu\nu}}&=&\left.\frac{\delta S_\mathrm{HR}(g, f(g))}{\delta g^{\mu\nu}}\right|_{f(g)}+\left.\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\frac{\delta S_\mathrm{HR}(g, f(g))}{\delta f^{\alpha\beta}}\right|_{g}\nn\\
&=& \mathcal{E}^g_{\mu\nu}(g, f(g))+\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\mathcal{E}^f_{\alpha\beta}(g, f(g))\,.
\eeqn
Here we have made use of the following short-hand notation for combining functional derivatives,
\beqn
\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\frac{\delta S}{\delta f^{\alpha\beta}}\equiv \int d^dy\, \frac{\delta f^{\alpha\beta}(y)}{\delta g^{\mu\nu}(x)}\frac{\delta S}{\delta f^{\alpha\beta}(y)}\,.
\eeqn
By definition, $f_{\mu\nu}(g)$ satisfies $\mathcal{E}^f_{\alpha\beta}(g, f(g))=0$. Using this in~(\ref{fpvar}) implies that, in fact, we have 
\beqn
\frac{\delta S_\mathrm{eff}(g)}{\delta g^{\mu\nu}}=\mathcal{E}^g_{\mu\nu}(g, f(g))\,.
\eeqn
This little exercise shows that the equation of motion obtained from $S_\mathrm{eff}(g)$ is precisely equation (\ref{effeq1}). We conclude that integrating out $\fmn$ in the action by using its own equation of motion is equivalent to plugging the solution directly into the $\gmn$ equation. 

Clearly, due to the nonlocality of the solution to the $\fmn$ equation, the action $S_\mathrm{eff}(g)$ will also be nonlocal and can thus not have the form of the higher-derivative theories discussed in the previous section. Let us therefore try to obtain a different effective action by integrating out $\fmn$ using the $\gmn$ equation. Since in this case the solution for $\fmn$ is an algebraic expression in terms of curvatures of $\gmn$, we can hope to arrive at a standard higher derivative theory. The variation of the effective action $S_\mathrm{HD}(g)=S_\mathrm{HR}(g, f(g))$ again reads
\beqn
\frac{\delta S_\mathrm{HD}(g)}{\delta g^{\mu\nu}}= \mathcal{E}^g_{\mu\nu}(g, f(g))+\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\mathcal{E}^f_{\alpha\beta}(g, f(g))\,.
\eeqn
But since now $f_{\mu\nu}(g)$ is defined to satisfy $\mathcal{E}^g_{\alpha\beta}(g, f(g))=0$, we have
\beqn\label{HDactvar}
\frac{\delta S_\mathrm{HD}(g)}{\delta g^{\mu\nu}}= \frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\mathcal{E}^f_{\alpha\beta}(g, f(g))\,.
\eeqn
Obviously, this is not exactly equivalent to (\ref{feq}). The equations of motion obtained from the effective action $S_\mathrm{HD}(g)$ differ from the effective bimetric equations by an operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$. Therefore the solutions to these equations will differ by functions $\chi(x)$ that are annihilated by this operator, which means that instead of the bimetric equation $\mathcal{E}^f_{\alpha\beta}=0$ we now have
\beqn
\mathcal{E}^f_{\alpha\beta}(g, f(g))=\chi(x)\,,\quad \int d^dy\, \frac{\delta f^{\alpha\beta}(y)}{\delta g^{\mu\nu}(x)}\chi(y)=0\,.
\eeqn
Since $\fmn$ is a function of curvatures of $\gmn$, the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ will introduce derivative terms into the effective action that would not be present in the higher-derivative theory that is truly equivalent to bimetric gravity. Separating off these extra terms is a tedious task which we choose not to pursue. Instead we try to find out what features of the bimetric theory carry over to the local higher-derivative theory despite their inequivalence. In particular, we are interested in making statements about the consistency of the higher-derivative action $S_\mathrm{HD}(g)$. 

While it is clear that the nonlocal action $S_\mathrm{eff}(g)$ that is equivalent to the ghost-free bimetric theory must be consistent and propagate seven healthy degrees of freedom, it is an important to understand whether the local action $S_\mathrm{HD}(g)$ that differs from the Hassan-Rosen theory by an extra operator can contain ghosts. This question is difficult to answer for nonlinear spin-2 fields because the nonlinearities and the tensor structures complicate the analysis. In the appendix of {\protect{\hyperref[papVIII]{Paper VIII}}} we therefore address this issue only in two simplified models: an action for two scalar fields with linear mixing term and linearized bimetric gravity. The outcome of the analysis in both models shows that the analogue of the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ does not alter the vacuum persistence amplitude and therefore does not introduce ghosts into the theory. We therefore expect (but do not prove) that the nonlinear theory with action $S_\mathrm{HD}(g)$, obtained from integrating out $\fmn$ using the $\gmn$ equation, is also ghost-free. 

On the other hand, our examples in the appendix of {\protect{\hyperref[papVIII]{Paper VIII}}} also show that, besides shifting the mass pole in the massive field's propagator, a truncation of the derivative expansion can easily lead to ghost instabilities. This explains the presence of the spin-2 ghost in the New Massive Gravity and Conformal Gravity actions. In order to avoid Ostrogradski's theorem, the ghost-free theory certainly needs the infinite number of higher-derivative terms.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Perturbative solution to the $\gmn$ equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our focus in the following lies on the second of the two procedures outlined above, which will lead to a local effective action with higher derivatives for $\gmn$. We will apply it to bimetric gravity and explicitly work out the resulting higher-curvature terms. The first step in our declared strategy is to obtain an algebraic solution for $\fmn$ using the $\gmn$ equation, which is the purpose of this section. In order to present an instructive example, we start with a simple bimetric model in which the solution for $\fmn$ in terms of $\gmn$ curvatures has a closed and finite expression. Then we turn to the general case. In this whole chapter, as in {\protect{\hyperref[papVIII]{Paper VIII}}}, we replace the mass parameter $m^d$ in the bimetric action by $m^2m_g^{d-2}$ which slightly simplifies the expressions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{A simple example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

There is one choice of parameters for which the algebraic solution for $\fmn$ derived from the $\gmn$ equation is particularly simple and can be obtained in closed form straightforwardly. Namely, let us consider the $\gmn$ equation (\ref{geq}) in which we set all $\beta_n$ with $n=2,3\hdots d-1$ to zero. Only the contributions from $(Y^{(0)})^\mu_{~\nu}$ and $(Y^{(1)})^\mu_{~\nu}$ remain\footnote{Note that the $\gmn$ equation does not contain $\beta_d$ and hence the perturbative solution for $\fmn$ does not depend on it.} and the equation simply reads 
\beqn
\frac{1}{m^2}{\mathcal{G}^\mu}_\nu(g)+\beta_0\delta^\mu_\nu-\beta_1({S^\mu}_\nu-\Tr\,S~{\delta^\mu}_\nu)=0\,.
\eeqn
Here we have used the definition $S=\sqrt{g^{-1}f}$, as usual, and raised one index with $g^{\mu\nu}$. The trace of this equation may be used to eliminate $\Tr\,S$ and in this way the solution for ${S^\mu}_\nu$ is obtained as
\beqn\label{ssolbeta1}
{S^\mu}_\nu=\frac{1}{1-d}\frac{\beta_0}{\beta_1}\delta^\mu_\nu+\frac{1}{\beta_1m^2}{P^\mu}_\nu(g)\,,
\eeqn
which we we have expressed in terms of the Schouten tensor defined in~(\ref{schouten}).
Since $\fmn=g_{\mu\rho}{(S^2)^\rho}_\nu$ the corresponding solution for $\fmn$ immediately follows from (\ref{ssolbeta1}) and reads 
\beqn
\fmn=\left(\frac{1}{d-1}\frac{\beta_0}{\beta_1}\right)^2\gmn-\frac{2}{d-1}\frac{\beta_0}{\beta^2_1m^2}P_{\mu\nu}+\frac{1}{\beta^2_1m^4}{P_\mu}^\rho P_{\rho\nu}\,.
\eeqn
This expression already has the form of a perturbative expansion in curvatures. Remarkably, in this particular model the series terminates at quartic order in derivatives. As we will see below, for general $\beta_n$, it is not possible to solve the $\gmn$ equation for $\fmn$ exactly, but we can obtain a perturbative solution, i.e.~an expression for $\fmn$ as an infinite series in~$P/m^{2}$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{General case}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

After having explored the nature of the $\fmn$ solution in an instructive example, we now turn to the case of general $\beta_n$ parameters.
Our aim is to solve the $\gmn$ equation perturbatively for ${S^\mu}_\nu$. It will prove convenient to first rewrite the Einstein tensor in (\ref{geq}) in terms of the Schouten tensor and raise one index with $g^{\mu\nu}$. This gives
\beqn\label{eomrewr}
\Tr\,P\,\delta^\mu_\nu-{P^\mu}_\nu=m^2\sum_{n=0}^{d-1}(-1)^n\beta_n {(Y^{(n)})^\mu}_\nu(S)\,.
\eeqn
Note that for the sake of notational simplicity we have set the source for $\gmn$ to zero. This simplification constitutes no loss of generality because in the final results of our computation it can always be reinstated by making the following replacement,
\beqn\label{sourcerepl}
{P^\mu}_\nu~\longrightarrow~ {P^\mu}_\nu-m^{2-d}\left( {T^{g\mu}}_\nu -\tfrac{1}{d-1}\Tr\,T^g\,\delta^\mu_\nu\right)\,.
\eeqn
Equation (\ref{eomrewr}) is linear in curvatures for $\gmn$, but it is highly nonlinear in $\fmn$ which appears under a square-root within the tensor-valued functions~$(Y^{(n)})^\mu_{~\nu}$. It is not obvious how to obtain a closed-form solution for~$\fmn$ from it, but we can easily arrive at a perturbative solution:
As in our simple example, we first solve (\ref{eomrewr}) algebraically for ${S^\mu}_\nu$ and afterwards square the result to obtain the solution for $\fmn$. To this end, we make the following perturbative ansatz
\begin{align}\label{ansatzs}
{S^\mu}_\nu=a\delta^\mu_\nu&+\tfrac{1}{m^2}\Big(b_1{P^\mu}_\nu+b_2\Tr\,P\,\delta^\mu_\nu\Big)
+ \tfrac{1}{m^4}\Big( c_1{(P^2)^\mu}_\nu+c_2\Tr\,P\,{P^\mu}_\nu   \nn\\
&+c_3\Tr\,P^2\delta^\mu_\nu+c_4(\Tr\,P)^2\delta^\mu_\nu \Big) 
+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,,
\end{align}
with arbitrary complex coefficients $a, b_i, c_i,\hdots$ Allowing the parameters to assume complex values is reasonable as long as the coefficients that will finally appear in the effective action remain real. One can think of complex parameters in the solution for ${S^\mu}_\nu$ as being merely a tool to arrive at the most general solution. 
As we will see in section~\ref{secPMCG}, an example for a case with complex coefficients is the PM theory in which the perturbative solution for ${S^\mu}_\nu$ turns out to be purely imaginary. This leads to a real solution for $\fmn$ as well as a real effective action for $\gmn$. 

In what follows, the strategy will be to plug the above ansatz for ${S^\mu}_\nu$ into the $\gmn$ equation (\ref{eomrewr}) and fix its coefficients by satisfying the equation at each order in $P/m^2$ separately. 
In order to simplify the expressions in the following, we introduce two new sets of linear combinations of the $\beta_n$ parameters,
\beqn\label{snalphan}
s_n\equiv \sum_{k=n}^{d-1}{d-1-n\choose k-n}a^k\beta_k\,,\qquad \alpha_n=\sum_{k=n}^d {d-n \choose k-n} a^k\beta_k\,.
\eeqn
It is easy to show that these obey
\beqn\label{salphaid}
s_n=\alpha_n-\alpha_{n+1}\,.
\eeqn
On proportional backgrounds, $\fmn=c^2\gmn$ and $s_0$ is proportional to the cosmological constant $\Lambda_g$ defined in~(\ref{lambdas}) if in that expression one replaces $c$ by $a$. As we will see below, the equation of motion enforces $s_0=0$, and hence if $c=a$ the solutions for both of the metrics are flat. 
On these backgrounds then $s_1$ is proportional to the Fierz-Pauli mass~(\ref{FPmass}). In general, however, $c\neq a$ and the sums $s_n$ have no direct interpretation.

In the following it will be convenient to work with ${M^\mu}_\nu\equiv{S^\mu}_\nu/a- \delta^\mu_\nu$, for which the ansatz~(\ref{ansatzs}) starts at linear order in curvatures. In terms of this matrix we can rewrite powers and symmetric polynomials of ${S^\mu}_\nu$ as follows,
\begin{align}
 {(S^{n-k})^\mu}_\nu&=a^{n-k}\sum_{r=0}^{n-k}{n-k\choose r}{(M^r)^\mu}_\nu\,,\nn  \\
 e_k(S)&=a^k\sum_{m=0}^k{d-m\choose k-m}e_m(M)\,. \label{eitoM}
 \end{align}
These expressions enter the $\gmn$ equation of motion through the definition~(\ref{defY}) of ${(Y^{(n)})^\mu}_\nu$.
At this point let us also remark that from the latter equation in (\ref{eitoM}) it follows that the interaction potential in the bimetric action written in terms of ${M^\mu}_\nu$ becomes
 \beqn
\sum_{n=0}^{d}\beta_ne_n(S)=\sum_{n=0}^d\alpha_ne_n(M)\,,\label{senwM} 
\eeqn
which involves the $\alpha_n$ parameters defined above.
This identity will become useful in the next section when we derive the effective action for $\gmn$.

Next we use (\ref{eitoM}) in the definitions (\ref{defY}) of the matrices ${(Y^{(n)})^\mu}_\nu$ and plug the resulting expressions into the $\gmn$ equation of motion (\ref{eomrewr}). The outcome is  
\beqn
&~&m^2\sum_{n=0}^{d-1}a^n\beta_n \sum_{k=0}^n \sum_{m=0}^k \sum_{r=0}^{n-k}   (-1)^{n+k}{d-m\choose k-m}{n-k\choose r} e_m(M){(M^r)^\mu}_\nu\nn\\
&=&\Tr\,P~\delta^\mu_\nu-{P^\mu}_\nu\,.
\eeqn
The right-hand side of this equation is linear in curvatures for $\gmn$, whereas the left-hand side is a polynomial of degree $(d-1)$ in ${M^\mu}_\nu$.
In order to solve the equation perturbatively, we now insert our ansatz (\ref{ansatzs}) and compare the coefficients of $\delta^\mu_\nu$, ${P^\mu}_\nu$, $\Tr\,P\,\delta^\mu_\nu$, etc.~on both sides. For this, of course, one also needs to invoke the explicit expressions of the elementary symmetric polynomials $e_m$ that we list in (\ref{listesp}) for $m\leq4$.


For the lowest three orders it is simple to carry out this procedure by hand. The results are
\begin{align}\label{parsollo}
\mathcal{O}(1):&~~~~s_0\equiv\sum_{n=0}^{d-1} {d-1\choose n}\beta_na^n=0\,,\nn\\
\mathcal{O}\left(\tfrac{P}{m^2}\right):&~~~~  b_1=\frac{a}{s_1}\,,\quad  b_2=0\,,\nn\\
\mathcal{O}\left(\tfrac{P^2}{m^4}\right):&~~~~ 2(d-1)c_4=-2(d-1)c_3=-c_2=c_1=\frac{as_2}{s_1^3}\,.
\end{align}
The equation at lowest order, $s_0=0$, is a polynomial in $a$ that determines $a$ in terms of the $\beta_n$. Here we see explicitly that it is possible to have complex solutions for $a$ which, as stated before, do not cause any problems as long as all parameters appearing in the effective action and equations for $\gmn$ remain real. We will encounter an example for this situation in the next section. Order by order, the other equations determine the coefficients in the ansatz for ${S^\mu}_\nu$. 
Hence the perturbative solution that we have been looking for is of the following form,
\begin{align}\label{sols}
{S^\mu}_\nu=a\delta^\mu_\nu&+\tfrac{a}{s_1m^2}{P^\mu}_\nu +\tfrac{as_2}{s_1^3m^4}\Big[{(P^2)^\mu}_\nu-\Tr\,P\,{P^\mu}_\nu+\tfrac{1}{d-1}e_2( P)\delta^\mu_\nu\Big] \nn\\
&+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,.
\end{align}
For general $\beta_n$ the right-hand side is an infinite expansion in curvatures. The only case for which the series is known to terminate is the model with $\beta_n=0$ for $n=2,3\hdots d-1$ that we discussed previously.
Furthermore, the suppressing mass scale is $s_1m^2$ which, as we argued before, is proportional to the Fierz-Pauli mass of the massive fluctuation in flat space. Note also the absence of a term proportional to $\Tr\,P$ in~(\ref{sols}) as well as the fact that all relative coefficients between the quadratic curvature contributions are simply numbers independent of the parameters of the theory. For higher curvature corrections, which we have found with the help of a computer up to fifth order in curvatures, this is no longer true because some of the ratios between coefficients will become parameter dependent. 


Finally, we use $\fmn=g_{\mu\rho}{(S^2)^\rho}_\nu$ to arrive at
\begin{align}\label{fsolP}
\fmn=a^2\gmn&+\tfrac{2a^2}{s_1m^2}P_{\mu\nu}+\tfrac{a^2(s_1+2s_2)}{s_1^3m^4}{(P^2)^\mu}_\nu\nn\\
&+\tfrac{2a^2s_2}{s_1^3m^4}\Big[\tfrac{1}{d-1}e_2( P)\delta^\mu_\nu-\Tr\,P\,{P^\mu}_\nu\Big]
+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,.
\end{align}
This is the most general perturbative solution for $\fmn$ obtained from the $\gmn$ equation.

At this point let us make the remark that there are special corners in parameter space for which the perturbative solution does not exist. For instance, if $\beta_0=0$ then $a=0$ is a solution to $s_0=0$ and in this case it is not possible to find a perturbative solution for~$\fmn$. Another example of this type is a set of $\beta_n$ parameters such that $s_1=0$. In this case the perturbative solution at $\mathcal{O}(P/m^2)$ enforces $R_{\mu\nu}(g)=0$, i.e.~the solution for $\gmn$ has to be flat. It is certainly interesting to understand the nature of these special cases, but here our main focus lies on generic values for the parameters of the theory for which the perturbative solution exists.

An immediate consequence of the existence of the solution (\ref{fsolP}) is that if the solution for $\gmn$ has constant curvature, $P_{\mu\nu}\propto\gmn$, then it follows from (\ref{fsolP}) that $\fmn\propto\gmn$, i.e.~the two metrics are proportional to each other. But, as we saw in section~\ref{secpropbg}, this implies that also $\fmn$ has constant curvature. Of course, we can just as well solve the~$\fmn$ equation algebraically for $\gmn$ and interchange the roles of $\gmn$ and $\fmn$ in the argument, and hence a constant curvature solution for one of the metrics always implies proportional backgrounds and a constant curvature solution for the other metric.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Resulting theory for $\gmn$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Following the strategy described in section~\ref{sec:outl}, we now use the solution~(\ref{fsolP}) for $\fmn$ to eliminate it in the bimetric action~(\ref{HR}). 
In the interaction potential this is straightforward: One simply uses~(\ref{senwM}) to obtain an expansion in curvatures of~$\gmn$. Since the expansion of the matrix ${M^\mu}_\nu\equiv{S^\mu}_\nu/a- \delta^\mu_\nu$ starts with a term linear in~${P^\mu}_\nu$, only $e_n(M)$ with $n=0,1,2$ contribute to quadratic order in $P/m^2$. 

The kinetic term for $\fmn$ is a bit more tricky. First, we need to evaluate the inverse and the Jacobian determinant of $\fmn$. The result for the inverse reads
\beqn
(f^{-1})^{\mu\nu}=a^{-2}g^{\mu\nu}-\frac{2}{a^2s_1m^2}P^{\mu\nu}+\mathcal{O}\left(\tfrac{P^2}{m^4}\right)\,.
\eeqn
It is sufficient to expand this to first order in curvatures because in the kinetic term it is contracted with the Ricci tensor for $\fmn$ which involves no constant term. Furthermore, we have
\beqn 
\sqrt{f}=\sqrt{g}\,\det S=\sqrt{g}\,\det(a\mathbb{1}+aM)=a^d\sqrt{g}\sum_{n=0}^de_n(M)\,,
\eeqn
in which now only terms with $n=0,1$ contribute to quadratic order in curvatures.

In order to evaluate the Ricci tensor for $\fmn$, we invoke once more the curvature relations (\ref{curvrel}). With their help we can express $R_{\mu\nu}(f)$ as $R_{\mu\nu}(g)$ plus terms with covariant derivatives acting on $\gmn$ curvatures. It turns out that terms involving $\gmn$-covariant derivatives (which anyway would only give a total derivative contribution) drop out of the action upon use of the Bianchi identity. More details are provided in {\protect{\hyperref[papVIII]{Paper~VIII}}}, here we simply present the final result.
Putting everything together gives the following effective action for~$\gmn$,
\begin{align}\label{HDactobt}
    S_\mathrm{HD}=m_g^{d-2}&\int\dd^dx\sqrt{g}\,\Big[ c_\Lambda+c_RR(g)\nn\\
    &-\frac{c_{RR}}{m^2}\Big(R^{\mu\nu}R_{\mu\nu}-\frac{d}{4(d-1)}R^2\Big) \Big]~+~\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,.
\end{align}
The coefficients of different orders in curvatures are related to the original bimetric parameters through
\begin{align}
c_\Lambda&=-2m^2\alpha_0\,, \qquad c_R=1+(\alpha a)^{d-2}-\frac{\alpha_1(d-2)}{s_1(d-1)}\,,\nn\\
c_{RR}&=\frac{1}{s_1^2}\left( 2s_1(\alpha a)^{d-2}-\alpha_2+\frac{\alpha_1s_2(d-2)}{s_1(d-1)} \right)\,.
\end{align}
Remarkably, the effective action (\ref{HDactobt}) is exactly of the form (\ref{HDact}). In particular, the relative coefficient in between the two quadratic curvature coefficients is independent of the parameters of the theory and fixed to the value that removes the Boulware-Deser ghost from the spectrum. This is of course expected considering the fact that we started from the ghost-free bimetric theory. 

In the beginning of this chapter we showed that the quadratic curvature action (\ref{HDact}) always contains a spin-2 ghost. Clearly, this is not the case in bimetric gravity which gives rise to two healthy spin-2 modes at the linearized level. In {\protect{\hyperref[papVIII]{Paper~VIII}}} we  try to localize the origin of the inconsistency using a simplified model of two scalar fields. This example shows that the ghost is most likely not introduced by our procedure of obtaining the effective action for $\gmn$. That is to say,  we believe that the extra zero modes to the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ that appear in the solution are not responsible for the inconsistency. Rather, the scalar field model suggests that the ghost instability arises when the theory with infinitely many derivatives is truncated to the four-derivative level. This result is also in accordance with Ostrogradski's theorem.  We are thus lead to making the following conjecture: The local higher derivative theory with action $S_\mathrm{HD}$ obtained from bimetric gravity by integrating out $\fmn$ using the $\gmn$ equation provides a ghost-free extension of the incomplete quadratic curvature action~$S_\mathrm{HD}^{(2)}$.

Note also that the sources may be included into the theory by making the replacement~(\ref{sourcerepl}) in~(\ref{HDactobt}). As a result, in the effective action, the ghost-free coupling to matter sources is highly nontrivial. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Partially massless case}\label{secPMCG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now specialize to four space-time dimensions where, as we demonstrated in chapter~\ref{ch:PM}, the family of bimetric theories contains a candidate for the nonlinear theory of a partially massless field. But instead of fixing the parameters in the interaction potential immediately to their PM values, let us start from a different direction: Suppose our interest lies in finding the parameter values for which the higher-derivative action~(\ref{HDactobt}) obtained from bimetric gravity reduces to the Conformal Gravity action~(\ref{CGact}) at lowest order in derivatives. Clearly, this means that we must have
\beqn\label{condCG}
c_\Lambda=-2m^2\alpha_0=0\,,\qquad c_R=1+(\alpha a)^2-\frac{2\alpha_1}{3s_1}=0\,.
\eeqn
Recall that satisfying the $\gmn$ equation required $s_0=0$. Then, the identity (\ref{salphaid}) together with the first of the above conditions, $\alpha_0=0$, imply that also $\alpha_1=0$. Using this in the second condition we see that we must have $a=\pm i\alpha^{-1}$. Now we plug this value for $a$ into $s_0=0$ and $\alpha_0=0$ which we evaluate in terms of the $\beta_n$ parameters. This gives two complex equations,
\beqn
\beta_0+\frac{3i}{\alpha}\beta_1-\frac{3}{\alpha^2}\beta_2-\frac{i}{\alpha^3}\beta_3&=&0\,,\nn\\
\beta_0+\frac{4i}{\alpha}\beta_1-\frac{6}{\alpha^2}\beta_2-\frac{4i}{\alpha^3}\beta_3+\frac{1}{\alpha^4}\beta_4&=&0\,.
\eeqn
The real and imaginary parts must vanish separately and the unique solution is
\beqn\label{PMparz}
\beta_1=\beta_3=0\,,\qquad \alpha^2\beta_0=3\beta_2=\alpha^{-2}\beta_4\,.
\eeqn
Remarkably, these values precisely corresponds to the PM parameter choice in $d=4$ that we found in chapter~\ref{ch:PM}. We conclude that the PM candidate is the unique member of the family of bimetric theories with the feature that to lowest order in a derivative expansion the effective action for $\gmn$ is conformally invariant. To lowest order, the corresponding equations of motion obtained from the effective action for $\gmn$ are those of Conformal Gravity,
\beqn
B_{\mu\nu}+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)=0\,.
\eeqn
Moreover, it is straightforward to show that the first method that we explained in section~\ref{sec:outl} yields a similar result:
The effective equation for $\gmn$, obtained from solving the $\gmn$ equation for $\fmn$ and plugging the solution into the $\fmn$ equation, also sets the Bach tensor to zero at lowest order in derivatives.
This is expected since the first term in the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ in (\ref{HDactvar}) is proportional to the identity and hence the lowest-order terms are the same for both ways of integrating out $\fmn$.  

The nonlinear PM bimetric theory therefore proposes a ghost-free completion of Conformal Gravity. The presence of a gauge symmetry to lowest order in a derivative expansion further supports the existence of a PM gauge symmetry in the theory. In turn, if it exists, the PM symmetry constitutes the generalization of the gauge invariance of Conformal Gravity to higher orders in derivatives.

\subsubsection{Constructing the PM symmetry} 

The perturbative solution to the $\gmn$ equation and the analogous solution to the $\fmn$ equation can be used to construct the PM symmetry transformation order by order in derivatives. In fact, this method is powerful enough to prove the existence of a PM symmetry perturbatively. This is the subject of an upcoming publication and will not be discussed in detail in this thesis. However, since it strengthens the importance of {\protect{\hyperref[papVI]{Paper~VI}}}, {\protect{\hyperref[papVII]{Paper~VII}}} and {\protect{\hyperref[papVIII]{Paper~VIII}}}, let us briefly outline the idea of the proof.

An important tool in what follows is the discrete interchange symmetry of the PM candidate theory. Namely, recall that the action and the equations of motions are invariant under
\beqn\label{intsymPM}
\alpha^{-1}\gmn\longleftrightarrow \alpha \fmn\,.
\eeqn
With the PM parameters~(\ref{PMparz}), the perturbative solutions to the $\gmn$ and $\fmn$ equations of motion, respectively, assume the form,
\beqn\label{pertsolpm}
\fmn&=&-\alpha^{-2}\gmn+\frac{1}{\beta_2m^2}P_{\mu\nu}+\gamma_{\mu\nu}(\alpha^{-1}g,P)\,,\nn\\
\gmn&=&-\alpha^2\fmn+\frac{\alpha^2}{\beta_2m^2}\tilde{P}_{\mu\nu}+\alpha^2\gamma_{\mu\nu}(\alpha f,\tilde{P})\,,
\eeqn
where $\tilde{P}$ denote curvatures for $\fmn$. Furthermore, the function $\gamma_{\mu\nu}$ contains all higher-order contributions, starting at the four-derivative level. Due to the interchange symmetry (\ref{intsymPM}) the higher orders have the same functional form in both equations. 


It is easy to see that, to lowest order in derivatives, the perturbative solutions in (\ref{pertsolpm}) are invariant under two conformal transformations,
\begin{align}
\Delta\gmn&=\phi(x)\gmn + \mathcal{O}\left(\tfrac{P}{m^2}\right)\,,\nn\\
\Delta\fmn&=\phi(x)\fmn + \mathcal{O}\left(\tfrac{\tilde{P}}{m^2}\right)=-\alpha^{-2}\phi(x)\gmn+ \mathcal{O}\left(\tfrac{P}{m^2}\right)\,.
\end{align}
In the second line, we have used the solution for $\fmn$ to give two different expressions for its transformation: one that can be obtained from the $\gmn$ transformation via the interchange symmetry (\ref{intsymPM}) and one for which the invariance of the perturbative solutions is manifest. 
 
Although the conformal transformations are a symmetry of the lowest order terms in the above equations, it is clear that they will not leave the higher-order contributions invariant. In order to cancel the effects of the conformal transformations in higher orders, we need to include higher-derivative terms into the symmetry transformations of the metrics.

The next order of the transformations has two derivatives and consists of terms involving covariant derivatives acting on $\phi$ or curvatures multiplying $\phi$. They are constructed by plugging the lowest order of the transformation into the two-derivative terms of the equations. In order to cancel out these contributions one then adds corresponding terms in the transformations for $\gmn$ and $\fmn$. In fact, it is sufficient to consider only one of the above equations, say the solution for $\fmn$, and write down the necessary terms in the transformations to guarantee invariance of this equation. Then, for each type of term, there will still be an arbitrary relative coefficient between the $\gmn$ and $\fmn$ transformation. 
This coefficient is then fixed by imposing the interchange symmetry (\ref{intsymPM}). In this way, since it can be obtained from the solution for $\fmn$ through the interchange symmetry, the solution for $\gmn$ will also be invariant under the PM symmetry by construction. 

The results for the transformations to second order in derivatives derived in this manner have the following form,
\beqn\label{PMtrafso}
\Delta\gmn&=&\phi\gmn - \frac{\alpha^2}{2\beta_2m^2}\nabla_\mu\partial_\nu \phi-\frac{\alpha^2}{2\beta_2m^2}P_{\mu\nu}\phi+ \mathcal{O}\left(\tfrac{P^2}{m^4}\right)\,,\nn\\
\Delta\fmn&=&\phi\fmn - \frac{1}{2\beta_2m^2}\tilde{\nabla}_\mu\partial_\nu \phi-\frac{1}{2\beta_2m^2}\tilde{P}_{\mu\nu}\phi+\mathcal{O}\left(\tfrac{\tilde{P}^2}{m^4}\right)\nn\\
&=&-\alpha^{-2}\phi\gmn - \frac{1}{2\beta_2m^2}\nabla_\mu\partial_\nu \phi+\frac{1}{2\beta_2m^2}P_{\mu\nu}\phi+\mathcal{O}\left(\tfrac{\tilde{P}^2}{m^4}\right)\,.\nn\\
\eeqn
Again, we have expressed the $\fmn$ transformation in two different ways that are equivalent on-shell. The expression in the last line can be used to check the invariance of the perturbative solutions explicitly. When using the solution for $\fmn$ to rewrite its transformation in terms of only $\gmn$ and its curvatures, one introduces new higher-derivative terms that need to be taken care of at the next orders. This is how, for example, the term proportional to $P_{\mu\nu}\phi$ enters the transformations. 
A term $P\gmn\phi$ is absent because it is not introduced by using the perturbative solution for~$\fmn$.

The above construction of the transformations can be continued step by step at each order in derivatives, resulting in a perturbative expression for the PM gauge symmetry. Performing this construction explicitly is intricate already at the four-derivative level. Nevertheless, the mere fact that it is possible to construct the symmetry in a derivative expansion proves its existence on the perturbative solutions. Although these solutions are not the most general ones\footnote{For example, the perturbative solutions imply that if the curvatures are diagonal then so are the metrics, whereas bimetric theory is known to also contain solutions for which this is not the case, see e.g.~\cite{Volkov:2013roa}. However, in $d=4$, these are not continuously connected to the perturbative solutions above.}, they make up a large isolated class of all possible solutions. The existence of a gauge symmetry on this class of solutions is therefore highly nontrivial and furthermore supports its presence in the full theory.

Note that the precise form of the perturbative solutions in~(\ref{pertsolpm}) is unique to the PM parameters. It is quite simple to show that, for any other values of the $\beta_n$ parameters, the construction of a gauge symmetry fails latest at the two-derivative level. This could have been expected, since it was only the PM parameters that lead to the conformally invariant Bach equation when the $\gmn$ and $\fmn$ equations where combined. We conclude that our PM candidate theory is the unique theory with a scalar gauge symmetry in the perturbative solutions to its equations of motion.

To conclude this discussion, let us demonstrate that the above transformations reduce to the well-known PM gauge symmetry in the linear theory around a de Sitter background.
To this end, recall the transformation for the massive fluctuation $\delta M_{\mu\nu}$ around proportional backgrounds which, in $d=4$, can be written as
\beqn\label{linPMsym3}
\Delta (\delta M_{\mu\nu}) =  \phi(x)\bar{g}_{\mu\nu} +\frac{3}{\Lambda_g}\bar{\nabla}_\mu\partial_\nu\phi(x)\,.
\eeqn
According to its definition in (\ref{dGanddM}), the massive fluctuation satisfies $\delta M_{\mu\nu}\propto \delta\fmn-c^2\delta\gmn$. This implies that its transformation under the PM symmetry must be proportional to $\Delta\fmn-c^2\Delta\gmn$ evaluated on the proportional backgrounds. 
For $\bar{f}_{\mu\nu}=c^2\bar{g}_{\mu\nu}$ we have that
\beqn
P_{\mu\nu}(\bar{g})=\tilde{P}_{\mu\nu}(\bar{f})= \frac{\Lambda_g}{3}\bar{g}_{\mu\nu}\qquad \Lambda_g=3\beta_2m^2(1+\alpha^2c^2)\,.
\eeqn
Using these results in (\ref{PMtrafso}) it can easily be checked that on these backgrounds one obtains
\beqn
\left.\left(\Delta\fmn-c^2\Delta\gmn\right)\right|_{\bar{f}_{\mu\nu}=c^2\bar{g}_{\mu\nu}}=\frac{1}{2}(\alpha^4c^4-1)\left[\phi\bar{g}_{\mu\nu}+\frac{3}{\Lambda_g}\bar{\nabla}_\mu\partial_\nu\phi\right]\,,
\eeqn
which is indeed proportional to (\ref{linPMsym3}).
Hence, the above nonlinear transformations generate precisely the PM transformation of the massive fluctuation. As a side remark, let us point out that this also means that the higher-order terms of the PM transformation of $\delta M_{\mu\nu}$ must vanish on the proportional backgrounds.

The fact that we arrive at the correct form (\ref{linPMsym3}) starting from the nonlinear transformations shows that the gauge symmetry we constructed above corresponds precisely to the PM invariance of the linear theory. 
Our nonlinear PM candidate thus explains the origin of the PM symmetry around de Sitter backgrounds and, even at the nonlinear level, a gauge symmetry removes one degree of freedom. 


 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Summary $\&$ Outlook}
\label{ch:concl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this thesis, we discussed ghost-free nonlinear theories involving massive spin-2 fields. Our findings are summarized below.


\begin{itemize}

\item[$\diamond$] There are two classes of consistent nonlinear theories for massive spin-2 fields of rather distinct nature: Nonlinear Massive Gravity~\cite{deRham:2010kj, Hassan:2011vm} contains self-interactions of a massive spin-2 field in a background that is fixed by hand, whereas bimetric theory~\cite{Hassan:2011zd} describes two dynamical spin-2 fields, one with massive and one with massless fluctuation around maximally symmetric backgrounds. We demonstrated the absence of the Boulware-Deser ghost instability in nonlinear Massive Gravity both in the physical gauge and in a diffeomorphism invariant formulation. 

\item[$\diamond$] We computed the mass spectrum of bimetric theory around proportional background solutions and identified nonlinear fields with massive and massless fluctuations around these backgrounds. A Hamiltonian analysis revealed that the nonlinear massless field cannot have standard matter couplings, which suggested that, in the presence of a massive spin-2 field, the gravitational metric is a superposition of mass eigenstates.

\item[$\diamond$] In the vielbein formulation, bimetric theory can be generalized to describe interactions of multiple spin-2 fields~\cite{Hinterbichler:2012cn}. We introduced a set of St\"uckelberg fields to reinstore the broken local Lorentz symmetry in the theory, which enabled us to reformulate the multivielbein theory in terms of the respective metrics.


\item[$\diamond$] The most general homogeneous and isotropic solutions to the bimetric equations of motion were derived and in some special cases discussed in more detail. The parameters of the interaction potential could be fitted to observational data and thus, at the background level, bimetric theory could account for the observed cosmologial evolution. Certain parameter subspaces even gave rise to a viable self-accelerating cosmological expansion without the need to include vacuum energy~\cite{Akrami:2012vf}.

\item[$\diamond$] We developed a method to identify nonlinear candidate theories for a partially massless spin-2 field within the family of bimetric actions. The equations of motion in such a theory should be invariant under a generalization of the gauge symmetry for linear PM fields in de Sitter backgrounds.
In the four-dimensional candidate theory, several aspects pointed towards the presence of a gauge symmetry at the nonlinear level. 
In space-time dimensions greater than four, it was necessary to extend the bimetric action by the Lanczos-Lovelock terms in order to obtain nontrivial results.


\item[$\diamond$] Bimetric theory was shown to be closely related to a certain class of higher-curvature theories for gravity which are known to be free of the Boulware-Deser ghost. On the other hand, these theories contain a spin-2 field whose helicity components all show instabilities. We argued that this problem may be cured by completing the quadratic curvature terms in the action into an infinite expansion in derivatives whose form can be derived from bimetric gravity. 

\item[$\diamond$] A close connection between our candidate theory for nonlinear partial masslessness and Conformal Gravity was established. The equations of motion of PM bimetric theory were shown to be conformally invariant at the four-derivative level in a perturbative expansion. This observation further allowed us to explicitly construct the PM gauge symmetry perturbatively to second-order in derivatives, which resulted in an expression compatible with the well-known transformation of linear PM fields. Moreover, the perturbative solutions to the equations of motion in the PM bimetric theory opened up the possibility to prove the existence of a gauge symmetry at the nonlinear level.
\end{itemize}


Open issues in the field of nonlinear Massive Gravity and bimetric theory can be divided into phenomenological and more theoretical questions. On the phenomenology side, further investigation of classical solutions to the equations of motion is of great interest. On the theory side, it is most interesting to look for extensions of the consistent theories in order to fit them into a larger framework. In the following we mention some of the vividly ongoing research. 

\vspace*{5mm}

Having found viable cosmological background solutions to the bimetric equations, the next test the theory needs to pass is whether it can explain growth of structure in the universe. In order to address this question, one needs to study perturbations around the cosmological solutions. Unfortunately, this type of analysis is complicated by the square-root matrix in the interaction potential. First attempts to derive and solve the perturbation equations have been made in~\cite{Comelli:2012db, Berg:2012kn}, but the compatibility of bimetric theory with constraints from structure formation is still an open question.

Another important issue in theories with massive spin-2 fields coupled to matter is the existence of a Vainshtein mechanism in order to avoid the observationally discarded vDVZ discontinuity. Spherically symmetric solutions to the bimetric equations have been investigated in \cite{Comelli:2011wq, Volkov:2013roa, Volkov:2012wp}. The possibility for a Vainshtein mechanism and the reconcilability with astrophysical data were shown to be given both in Massive Gravity~\cite{Sjors:2011iv} and in bimetric theory~\cite{Enander:2013kza}.


The evidence for the existence of a gauge symmetry, which we discovered in several independent approaches, exposes the exceptional nature of the nonlinear PM bimetric theory. It would be of great interest to derive the explicit non-perturbative form of the gauge transformations that leave the bimetric equations invariant. But even without the knowledge of the exact transformations, physical aspects of the theory can be studied. An analysis of implications for cosmology has been started, for example, in~\cite{Akrami:2013ffa}. Moreover, in \cite{Brito:2013yxa} it was shown that the PM theory avoids the Gregory-Laflamme instability~\cite{Gregory:1993vy} which is a generic undesirable feature of black-hole solutions in nonlinear Massive Gravity and bimetric theory~\cite{Babichev:2013una, Brito:2013wya}.

Eventually, one would of course also like to return to the original motivation for constructing a nonlinear Massive Gravity theory and readdress the cosmological constant problem. So far, an obvious solution to the problem has been found neither in Massive Gravity nor in bimetric gravity. The self-accelerating cosmological backgrounds discussed in \cite{Akrami:2012vf, Akrami:2013ffa} demonstrate that bimetric theory can account for the observed rate of cosmic acceleration without any vacuum energy.
The acceleration is due to a spin-2 field with mass at the Hubble scale, which mildens the cosmological constant problem because a small spin-2 mass is technically natural. On the other hand, the origin of the small value for the graviton mass as well as the disappearance of vacuum energy from quantum field theory remain unexplained in this setup. 






\vspace*{5mm}


Turning to the prospects on the theory side, we emphasize that extensions of the bimetric action primarily need to maintain the consistency of the theory. In particular, they must not reintroduce the Boulware-Deser ghost instability. One possibility of extending the theory is then given by the Lanczos-Lovelock terms that we already considered in {\protect{\hyperref[papVII]{Paper~VII}}}. These are commonly believed to avoid the Boulware-Deser ghost and therefore provide a viable generalization of the Hassan-Rosen action. 
Another conceivable extension is the addition of further derivative interactions that respect the antisymmetric structure of the interaction potential and the LL terms. The consistency of such new interactions has recently been suggested in a pseudo-linear analysis~\cite{Hinterbichler:2013eza}, while their precise nonlinear form is still unknown.

Other extensions involving additional scalar fields have been introduced mainly in the context of nonlinear Massive Gravity. For example, it has been suggested to promote the $\beta_n$-parameters to functions of a scalar field~\cite{Huang:2012pe, Huang:2013mha}.
Furthermore, the proposals involve coupling the metric $\gmn$ to fields with Galileon symmetry~\cite{Gabadadze:2012tr} and to a quasi-dilaton~\cite{D'Amico:2012zv}. If the quasi-dilaton is self-interacting, the theory is classically equivalent to the Massive Gravity action extended by functions of the Ricci scalar~\cite{Cai:2013lqa}. A similar $f( R)$ generalization has also been considered for bimetric gravity~\cite{Nojiri:2013zza}.


Another important issue is the computation of quantum corrections to the consistent nonlinear actions for spin-2 fields. A first attempt to this effect has been made in~\cite{Buchbinder:2012wb} which, however, worked with the auxiliary model that we discussed in section~\ref{hamstuck}. Although, classically, this model is equivalent to the Massive Gravity action with a certain parameter choice, the two theories may differ at the quantum level. More recently, the one-loop effective action of the dRGT model was computed in~\cite{deRham:2013qqa}. There it was demonstrated that, at one-loop level, matter fields running in the loop do not change the structure of the interaction potential for the metric, whereas the ghost-free configuration does get modified by gravitons in the loop. Fortunately, the authors also argue that the mass of the ghost is never below the Planck scale and therefore does not propagate in the effective theory. These promising results suggest that consistent nonlinear Massive Gravity may be stable under quantum corrections. Besides the computation of higher-order loop diagrams in the dRGT model with fixed Minkowski background, it would be interesting to investigate whether this feature is shared by the fully dynamical bimetric theory.


Finally, one could explore the possibility of embedding the consistent bimetric models in String Theory. The most promising candidate for a unified description of particle physics and quantum gravity possesses a rich spectrum of massless and massive higher-spin fields. In particular, it contains a massless spin-2 field whose low-energy effective action is Einstein-Hilbert plus higher-curvature corrections. But the spectrum also includes a massive spin-2 field whose effective action has not been computed.
%\footnote{Derivations of effective actions in String Theory are very involved and usually the focus lies on massless fields that are most relevant in the low-energy limit.} 
It is therefore an interesting open question whether the ghost-free structure of the nonlinear massive spin-2 theories discussed in this thesis can be reproduced in String Theory. If this is the case, then, since phenomenologically viable String Theory requires Supersymmetry, it will contain a supersymmetrized version of bimetric theory. This motivates the search for a supersymmetric theory involving massive spin-2 fields which, even without String Theory, could be an interesting subject on its own. Interestingly, such a theory was already suggested several decades ago in~\cite{Chamseddine:1978yu} but without addressing the ghost issue.

Concluding remarks





 



\begin{thebibliography}{999}
\bibitem{Einstein:1916vd}
  A.~Einstein,
  %``The Foundation of the General Theory of Relativity,''
  Annalen Phys.\  {\bf 49} (1916) 769
   [Annalen Phys.\  {\bf 14} (2005) 517].
  %%CITATION = ANPYA,49,769;%%   
\bibitem{Fierz:1939ix}
  M.~Fierz and W.~Pauli,
  %``On relativistic wave equations for particles of arbitrary spin in 
  %an electromagnetic field,'' 
  Proc.\ Roy.\ Soc.\ Lond.\ A {\bf 173} (1939) 211.
  %%CITATION = PRSLA,A173,211;%%
\bibitem{vanDam:1970vg}
  H.~van Dam and M.~J.~G.~Veltman,
  %``Massive and massless Yang-Mills and gravitational fields,''
  Nucl.\ Phys.\ B {\bf 22} (1970) 397.
  %%CITATION = NUPHA,B22,397;%%
\bibitem{Zakharov:1970cc}
  V.~I.~Zakharov,
  %``Linearized gravitation theory and the graviton mass,''
  JETP Lett.\  {\bf 12} (1970) 312
   [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 12} (1970) 447].
  %%CITATION = JTPLA,12,312;%%
\bibitem{Vainshtein:1972sx}
  A.~I.~Vainshtein,
  %``To the problem of nonvanishing gravitation mass,''
  Phys.\ Lett.\ B {\bf 39} (1972) 393.
  %%CITATION = PHLTA,B39,393;%%
\bibitem{Boulware:1972zf}
  D.~G.~Boulware and S.~Deser,
  %``Inconsistency of finite range gravitation,''
  Phys.\ Lett.\ B {\bf 40} (1972) 227.
  %%CITATION = PHLTA,B40,227;%%
\bibitem{Boulware:1973my}
  D.~G.~Boulware and S.~Deser,
  %``Can gravitation have a finite range?,''
  Phys.\ Rev.\ D {\bf 6} (1972) 3368.
  %%CITATION = PHRVA,D6,3368;%%
\bibitem{ArkaniHamed:2002sp}
  N.~Arkani-Hamed, H.~Georgi and M.~D.~Schwartz,
  %``Effective field theory for massive gravitons and gravity in
  %theory space,'' 
  Annals Phys.\  {\bf 305} (2003) 96
  [hep-th/0210184].
  %%CITATION = HEP-TH/0210184;%%
\bibitem{de Urries:1998bi}
  F.~J.~de Urries and J.~Julve,
  %``Ostrogradski formalism for higher derivative scalar field theories,''
  J.\ Phys.\ A {\bf 31} (1998) 6949
  [hep-th/9802115].
  %%CITATION = HEP-TH/9802115;%%
\bibitem{deRham:2010ik}
  C.~de Rham and G.~Gabadadze,
  %``Generalization of the Fierz-Pauli Action,''
  Phys.\ Rev.\ D {\bf 82} (2010) 044020
  [arXiv:1007.0443 [hep-th]].
  %%CITATION = ARXIV:1007.0443;%%
\bibitem{deRham:2010kj}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Resummation of Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 106} (2011) 231101
  [arXiv:1011.1232 [hep-th]].
  %%CITATION = ARXIV:1011.1232;%%
\bibitem{Hassan:2011vm}
  S.~F.~Hassan and R.~A.~Rosen,
  %``On nonlinear Actions for Massive Gravity,''
  JHEP {\bf 1107} (2011) 009
  [arXiv:1103.6055 [hep-th]].
  %%CITATION = ARXIV:1103.6055;%%
\bibitem{Hassan:2011hr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Resolving the Ghost Problem in nonlinear Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 108} (2012) 041101
  [arXiv:1106.3344 [hep-th]].
  %%CITATION = ARXIV:1106.3344;%%
\bibitem{Hassan:2011ea}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Confirmation of the Secondary Constraint and Absence of Ghost in Massive Gravity and Bimetric Gravity,''
  JHEP {\bf 1204} (2012) 123
  [arXiv:1111.2070 [hep-th]].
  %%CITATION = ARXIV:1111.2070;%%
\bibitem{Hassan:2011zd}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Bimetric Gravity from Ghost-free Massive Gravity,''
  JHEP {\bf 1202} (2012) 126
  [arXiv:1109.3515 [hep-th]].
  %%CITATION = ARXIV:1109.3515;%%
\bibitem{Rosen:1940zz}
  N.~Rosen,
  %``General Relativity and Flat Space. II,''
  Phys.\ Rev.\  {\bf 57} (1940) 150.
  %%CITATION = PHRVA,57,150;%%
\bibitem{Rosen:1975kk}
  N.~Rosen,
  %``Bimetric Theory of Gravitation,''
  In *Erice 1975, Proceedings, Topics In Theoretical and Experimental
  Gravitation Physics*, New York 1977, 273-294 
 \bibitem{Aragone:1971kh}
  C.~Aragone and S.~Deser,
  %``Constraints on gravitationally coupled tensor fields,''
  Nuovo Cim.\ A {\bf 3} (1971) 709.
  %%CITATION = NUCIA,A3,709;%%
\bibitem{Isham:1971gm}
  C.~J.~Isham, A.~Salam and J.~A.~Strathdee,
  %``F-dominance of gravity,''
  Phys.\ Rev.\ D {\bf 3} (1971) 867.
  %%CITATION = PHRVA,D3,867;%%  
\bibitem{Chamseddine:1978yu}
  A.~H.~Chamseddine, A.~Salam and J.~A.~Strathdee,
  %``Strong Gravity and Supersymmetry,''
  Nucl.\ Phys.\ B {\bf 136} (1978) 248.
  %%CITATION = NUPHA,B136,248;%%
\bibitem{Dvali:2000rv}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``Metastable gravitons and infinite volume extra dimensions,''
  Phys.\ Lett.\ B {\bf 484} (2000) 112
  [hep-th/0002190].
  %%CITATION = HEP-TH/0002190;%%
\bibitem{Dvali:2000hr}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``4-D gravity on a brane in 5-D Minkowski space,''
  Phys.\ Lett.\ B {\bf 485} (2000) 208
  [hep-th/0005016].
  %%CITATION = HEP-TH/0005016;%%
\bibitem{Kaluza:1921tu}
  T.~Kaluza,
  %``On the Problem of Unity in Physics,''
  Sitzungsber.\ Preuss.\ Akad.\ Wiss.\ Berlin (Math.\ Phys.\ ) {\bf 1921} (1921) 966.
  %%CITATION = SPWPA,1921,966;%%  
\bibitem{Klein:1926tv}
  O.~Klein,
  %``Quantum Theory and Five-Dimensional Theory of Relativity. (In German and English),''
  Z.\ Phys.\  {\bf 37} (1926) 895
   [Surveys High Energ.\ Phys.\  {\bf 5} (1986) 241].
  %%CITATION = ZEPYA,37,895;%% 
\bibitem{Bergshoeff:2009hq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``Massive Gravity in Three Dimensions,''
  Phys.\ Rev.\ Lett.\  {\bf 102} (2009) 201301
  [arXiv:0901.1766 [hep-th]].
  %%CITATION = ARXIV:0901.1766;%%
\bibitem{Deser:1981wh}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Topologically Massive Gauge Theories,''
  Annals Phys.\  {\bf 140} (1982) 372
   [Erratum-ibid.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 281} (2000) 409].
  %%CITATION = APNYA,140,372;%%
\bibitem{Deser:1982vy}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Three-Dimensional Massive Gauge Theories,''
  Phys.\ Rev.\ Lett.\  {\bf 48} (1982) 975.
  %%CITATION = PRLTA,48,975;%%
\bibitem{ArkaniHamed:2003uy}
  N.~Arkani-Hamed, H.~-C.~Cheng, M.~A.~Luty and S.~Mukohyama,
  %``Ghost condensation and a consistent infrared modification of gravity,''
  JHEP {\bf 0405} (2004) 074
  [hep-th/0312099].
  %%CITATION = HEP-TH/0312099;%%
\bibitem{Riess:1998cb}
  A.~G.~Riess {\it et al.}  [Supernova Search Team Collaboration],
  %``Observational evidence from supernovae for an accelerating universe and a cosmological constant,''
  Astron.\ J.\  {\bf 116} (1998) 1009
  [astro-ph/9805201].
  %%CITATION = ASTRO-PH/9805201;%%
\bibitem{Perlmutter:1998np}
  S.~Perlmutter {\it et al.}  [Supernova Cosmology Project Collaboration],
  %``Measurements of Omega and Lambda from 42 high redshift supernovae,''
  Astrophys.\ J.\  {\bf 517} (1999) 565
  [astro-ph/9812133].
  %%CITATION = ASTRO-PH/9812133;%%
\bibitem{Martin:2012bt}
  J.~Martin,
  %``Everything You Always Wanted To Know About The Cosmological Constant Problem (But Were Afraid To Ask),''
  Comptes Rendus Physique {\bf 13} (2012) 566
  [arXiv:1205.3365 [astro-ph.CO]].
  %%CITATION = ARXIV:1205.3365;%%
\bibitem{Wigner:1939cj}
  E.~P.~Wigner,
  %``On Unitary Representations of the Inhomogeneous Lorentz Group,''
  Annals Math.\  {\bf 40} (1939) 149
   [Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 6} (1989) 9].
  %%CITATION = ANMAA,40,149;%%
\bibitem{Henneaux:1997bm}
  M.~Henneaux,
  %``Consistent interactions between gauge fields: The Cohomological approach,''
  Contemp.\ Math.\  {\bf 219} (1998) 93
  [hep-th/9712226].
  %%CITATION = HEP-TH/9712226;%%
\bibitem{Ruegg:2003ps}
  H.~Ruegg and M.~Ruiz-Altaba,
  %``The Stueckelberg field,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 19} (2004) 3265
  [hep-th/0304245].
  %%CITATION = HEP-TH/0304245;%%
\bibitem{Hinterbichler:2011tt}
  K.~Hinterbichler,
  %``Theoretical Aspects of Massive Gravity,''
  Rev.\ Mod.\ Phys.\  {\bf 84} (2012) 671
  [arXiv:1105.3735 [hep-th]].
  %%CITATION = ARXIV:1105.3735;%%
\bibitem{Arnowitt:1962hi}
  R.~L.~Arnowitt, S.~Deser and C.~W.~Misner,
  %``The Dynamics of general relativity,''
  [gr-qc/0405109].
  %%CITATION = GR-QC/0405109;%%
\bibitem{Date:2010xr}
  G.~Date,
  %``Lectures on Constrained Systems,''
  arXiv:1010.2062 [gr-qc].
  %%CITATION = ARXIV:1010.2062;%%
\bibitem{Khoury:2011ay}
  J.~Khoury, G.~E.~J.~Miller and A.~J.~Tolley,
  %``Spatially Covariant Theories of a Transverse, Traceless Graviton, Part I: Formalism,''
  Phys.\ Rev.\ D {\bf 85} (2012) 084002
  [arXiv:1108.1397 [hep-th]].
  %%CITATION = ARXIV:1108.1397;%%
\bibitem{Deffayet:2012nr}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``Covariant constraints in ghost free massive gravity,''
  JCAP {\bf 1301} (2013) 032
  [arXiv:1207.6338 [hep-th]].
  %%CITATION = ARXIV:1207.6338;%%
\bibitem{Kluson:2011qe}
  J.~Kluson,
  %``Note About Hamiltonian Structure of Non-Linear Massive Gravity,''
  JHEP {\bf 1201} (2012) 013
  [arXiv:1109.3052 [hep-th]].
  %%CITATION = ARXIV:1109.3052;%%
\bibitem{Chamseddine:2011mu}
  A.~H.~Chamseddine and V.~Mukhanov,
  %``Massive Gravity Simplified: A Quadratic Action,''
  JHEP {\bf 1108} (2011) 091
  [arXiv:1106.5868 [hep-th]].
  %%CITATION = ARXIV:1106.5868;%%
\bibitem{Kluson:2011rt}
  J.~Kluson,
  %``Comments About Hamiltonian Formulation of Non-Linear Massive Gravity with Stuckelberg Fields,''
  JHEP {\bf 1206} (2012) 170
  [arXiv:1112.5267 [hep-th]].
  %%CITATION = ARXIV:1112.5267;%%
\bibitem{Kluson:2012gz}
  J.~Kluson,
  %``Remark About Hamiltonian Formulation of Non-Linear Massive Gravity in Stuckelberg Formalism,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124005
  [arXiv:1202.5899 [hep-th]].
  %%CITATION = ARXIV:1202.5899;%%  
\bibitem{Lee:1977yc}
  B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
  %``The Strength of Weak Interactions at Very High-Energies and the Higgs Boson Mass,''
  Phys.\ Rev.\ Lett.\  {\bf 38} (1977) 883.
  %%CITATION = PRLTA,38,883;%%  
\bibitem{Chanowitz:1985hj}
  M.~S.~Chanowitz and M.~K.~Gaillard,
  %``The TeV Physics of Strongly Interacting W's and Z's,''
  Nucl.\ Phys.\ B {\bf 261} (1985) 379.
  %%CITATION = NUPHA,B261,379;%%
\bibitem{Creminelli:2005qk}
  P.~Creminelli, A.~Nicolis, M.~Papucci and E.~Trincherini,
  %``Ghosts in massive gravity,''
  JHEP {\bf 0509} (2005) 003
  [hep-th/0505147].
  %%CITATION = HEP-TH/0505147;%%
\bibitem{Ondo:2013wka}
  N.~A.~Ondo and A.~J.~Tolley,
  %``Complete Decoupling Limit of Ghost-free Massive Gravity,''
  arXiv:1307.4769 [hep-th]. 
\bibitem{deRham:2011rn}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Ghost free Massive Gravity in the St\'uckelberg language,''
  Phys.\ Lett.\ B {\bf 711} (2012) 190
  [arXiv:1107.3820 [hep-th]].
  %%CITATION = ARXIV:1107.3820;%%
\bibitem{Golovnev:2011aa}
  A.~Golovnev,
  %``On the Hamiltonian analysis of non-linear massive gravity,''
  Phys.\ Lett.\ B {\bf 707} (2012) 404
  [arXiv:1112.2134 [gr-qc]].
  %%CITATION = ARXIV:1112.2134;%%
\bibitem{Buchbinder:2012wb}
  I.~L.~Buchbinder, D.~D.~Pereira and I.~L.~Shapiro,
  %``One-loop divergences in massive gravity theory,''
  Phys.\ Lett.\ B {\bf 712} (2012) 104
  [arXiv:1201.3145 [hep-th]].
  %%CITATION = ARXIV:1201.3145;%%
\bibitem{Boulanger:2000rq}
  N.~Boulanger, T.~Damour, L.~Gualtieri and M.~Henneaux,
  %``Inconsistency of interacting, multigraviton theories,''
  Nucl.\ Phys.\ B {\bf 597} (2001) 127
  [hep-th/0007220].
  %%CITATION = HEP-TH/0007220;%%  
\bibitem{Damour:2002wu}
  T.~Damour, I.~I.~Kogan and A.~Papazoglou,
  %``Nonlinear bigravity and cosmic acceleration,''
  Phys.\ Rev.\ D {\bf 66} (2002) 104025
  [hep-th/0206044].
  %%CITATION = HEP-TH/0206044;%%
\bibitem{Nibbelink:2006sz}
  S.~Nibbelink Groot, M.~Peloso and M.~Sexton,
  %``Nonlinear Properties of Vielbein Massive Gravity,''
  Eur.\ Phys.\ J.\ C {\bf 51} (2007) 741
  [hep-th/0610169].
  %%CITATION = HEP-TH/0610169;%%
\bibitem{Banados:2008fi} {\bfseries MISSING REFERENCE!!!}

\bibitem{Milgrom:2009gv} {\bfseries MISSING REFERENCE!!!}

\bibitem{Berezhiani:2007zf} {\bfseries MISSING REFERENCE!!!}

\bibitem{Blas:2009my} {\bfseries MISSING REFERENCE!!!}

\bibitem{PhysRevD.40.1095} {\bfseries MISSING REFERENCE!!!}

\bibitem{Buchbinder:1999be} {\bfseries MISSING REFERENCE!!!}

\bibitem{Buchbinder:1999ar} {\bfseries MISSING REFERENCE!!!}

\bibitem{Damour:2002ws}
  T.~Damour and I.~I.~Kogan,
  %``Effective Lagrangians and universality classes of nonlinear
  %bigravity,'' 
  Phys.\ Rev.\ D {\bf 66} (2002) 104024
  [hep-th/0206042].
  %%CITATION = HEP-TH/0206042;%%
\bibitem{Akrami:2013ffa}
  Y.~Akrami, T.~S.~Koivisto, D.~F.~Mota and M.~Sandstad,
  %``Bimetric gravity doubly coupled to matter: theory and cosmological implications,''
  arXiv:1306.0004 [hep-th].
  %%CITATION = ARXIV:1306.0004;%%
\bibitem{Baccetti:2012bk}
  V.~Baccetti, P.~Martin-Moruno and M.~Visser,
  %``Massive gravity from bimetric gravity,''
  arXiv:1205.2158 [gr-qc].
  %%CITATION = ARXIV:1205.2158;%%
\bibitem{Hinterbichler:2012cn}
  K.~Hinterbichler and R.~A.~Rosen,
  %``Interacting Spin-2 Fields,''
  JHEP {\bf 1207} (2012) 047
  [arXiv:1203.5783 [hep-th]].
  %%CITATION = ARXIV:1203.5783;%%
\bibitem{Nomura:2012xr}
  K.~Nomura and J.~Soda,
  %``When is Multimetric Gravity Ghost-free?,''
  Phys.\ Rev.\ D {\bf 86} (2012) 084052
  [arXiv:1207.3637 [hep-th]].
  %%CITATION = ARXIV:1207.3637;%%    
  
  
    
  


\bibitem{Gabadadze:2013ria}
  G.~Gabadadze, K.~Hinterbichler, D.~Pirtskhalava and Y.~Shang,
  %``On the Potential for General Relativity and its Geometry,''
  arXiv:1307.2245 [hep-th].
  %%CITATION = ARXIV:1307.2245;%%    
\bibitem{Deffayet:2012zc}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``A note on 'symmetric' vielbeins in bimetric, massive, perturbative and non perturbative gravities,''
  JHEP {\bf 1303} (2013) 086
  [arXiv:1208.4493 [gr-qc]].
  %%CITATION = ARXIV:1208.4493;%% 
\bibitem{deRham:2010tw}
  C.~de Rham, G.~Gabadadze, L.~Heisenberg and D.~Pirtskhalava,
  %``Cosmic Acceleration and the Helicity-0 Graviton,''
  Phys.\ Rev.\ D {\bf 83} (2011) 103516
  [arXiv:1010.1780 [hep-th]].
  %%CITATION = ARXIV:1010.1780;%%  
\bibitem{Gumrukcuoglu:2011ew}
  A.~E.~Gumrukcuoglu, C.~Lin and S.~Mukohyama,
  %``Open FRW universes and self-acceleration from nonlinear massive gravity,''
  JCAP {\bf 1111} (2011) 030
  [arXiv:1109.3845 [hep-th]].
  %%CITATION = ARXIV:1109.3845;%%
\bibitem{D'Amico:2011jj}
  G.~D'Amico, C.~de Rham, S.~Dubovsky, G.~Gabadadze, D.~Pirtskhalava and A.~J.~Tolley,
  %``Massive Cosmologies,''
  Phys.\ Rev.\ D {\bf 84} (2011) 124046
  [arXiv:1108.5231 [hep-th]].
  %%CITATION = ARXIV:1108.5231;%%    
\bibitem{Volkov:2011an}
  M.~S.~Volkov,
  %``Cosmological solutions with massive gravitons in the bigravity
  %theory,'' 
  JHEP {\bf 1201} (2012) 035
  [arXiv:1110.6153 [hep-th]].
  %%CITATION = ARXIV:1110.6153;%%
\bibitem{Comelli:2011zm}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``FRW Cosmology in ghost-free Massive Gravity,''
  JHEP {\bf 1203} (2012) 067
   [Erratum-ibid.\  {\bf 1206} (2012) 020]
  [arXiv:1111.1983 [hep-th]].
  %%CITATION = ARXIV:1111.1983;%%
\bibitem{Hinshaw:2012aka}
  G.~Hinshaw {\it et al.}  [WMAP Collaboration],
  %``Nine-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Parameter Results,''
  arXiv:1212.5226 [astro-ph.CO].
  %%CITATION = ARXIV:1212.5226;%% 
\bibitem{Ade:2013ktc}
  P.~A.~R.~Ade {\it et al.}  [Planck Collaboration],
  %``Planck 2013 results. I. Overview of products and scientific results,''
  arXiv:1303.5062 [astro-ph.CO].
  %%CITATION = ARXIV:1303.5062;%%  
\bibitem{Comelli:2012db}
  D.~Comelli, M.~Crisostomi and L.~Pilo,
  %``Perturbations in Massive Gravity Cosmology,''
  JHEP {\bf 1206} (2012) 085
  [arXiv:1202.1986 [hep-th]].
  %%CITATION = ARXIV:1202.1986;%%
\bibitem{Berg:2012kn}
  M.~Berg, I.~Buchberger, J.~Enander, E.~Mortsell and S.~Sjors,
  %``Growth Histories in Bimetric Massive Gravity,''
  arXiv:1206.3496 [gr-qc].
  %%CITATION = ARXIV:1206.3496;%%
\bibitem{Comelli:2011wq}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``Spherically Symmetric Solutions in Ghost-Free Massive Gravity,''
  Phys.\ Rev.\ D {\bf 85} (2012) 024044
  [arXiv:1110.4967 [hep-th]].
  %%CITATION = ARXIV:1110.4967;%%
\bibitem{Volkov:2012wp}
  M.~S.~Volkov,
  %``Hairy black holes in the ghost-free bigravity theory,''
  Phys.\ Rev.\ D {\bf 85} (2012) 124043
  [arXiv:1202.6682 [hep-th]].
  %%CITATION = ARXIV:1202.6682;%%
\bibitem{Akrami:2012vf}
  Y.~Akrami, T.~S.~Koivisto and M.~Sandstad,
  %``Accelerated expansion from ghost-free bigravity: a statistical analysis with improved generality,''
  arXiv:1209.0457 [astro-ph.CO].
  %%CITATION = ARXIV:1209.0457;%%
\bibitem{Higuchi:1986py}
  A.~Higuchi,
  %``Forbidden Mass Range For Spin-2 Field Theory In De Sitter Space-time,''
  Nucl.\ Phys.\ B {\bf 282} (1987) 397.
  %%CITATION = NUPHA,B282,397;%%
\bibitem{Deser:1983mm}
  S.~Deser and R.~I.~Nepomechie,
  %``Gauge Invariance Versus Masslessness In De Sitter Space,''
  Annals Phys.\  {\bf 154} (1984) 396.
  %%CITATION = APNYA,154,396;%%
\bibitem{Deser:2001pe}
  S.~Deser and A.~Waldron,
  %``Gauge invariances and phases of massive higher spins in (A)dS,''
  Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 031601
  [hep-th/0102166].
  %%CITATION = HEP-TH/0102166;%%
\bibitem{Deser:2001us}
  S.~Deser and A.~Waldron,
  %``Partial masslessness of higher spins in (A)dS,''
  Nucl.\ Phys.\ B {\bf 607} (2001) 577
  [hep-th/0103198].
  %%CITATION = HEP-TH/0103198;%%
\bibitem{Deser:2001wx}
  S.~Deser and A.~Waldron,
  %``Stability of massive cosmological gravitons,''
  Phys.\ Lett.\ B {\bf 508} (2001) 347
  [hep-th/0103255].
  %%CITATION = HEP-TH/0103255;%%
\bibitem{Deser:2001xr}
  S.~Deser and A.~Waldron,
  %``Null propagation of partially massless higher spins in (A)dS and cosmological constant speculations,''
  Phys.\ Lett.\ B {\bf 513} (2001) 137
  [hep-th/0105181].
  %%CITATION = HEP-TH/0105181;%%
\bibitem{Deser:2004ji}
  S.~Deser and A.~Waldron,
  %``Conformal invariance of partially massless higher spins,''
  Phys.\ Lett.\ B {\bf 603} (2004) 30
  [hep-th/0408155].
  %%CITATION = HEP-TH/0408155;%%  
\bibitem{Deser:2006zx}
  S.~Deser and A.~Waldron,
  %``Partially Massless Spin 2 Electrodynamics,''
  Phys.\ Rev.\ D {\bf 74} (2006) 084036
  [hep-th/0609113].
  %%CITATION = HEP-TH/0609113;%%
\bibitem{Higuchi:1989gz}
  A.~Higuchi,
  %``Massive Symmetric Tensor Field In Space-times With A Positive Cosmological Constant,''
  Nucl.\ Phys.\ B {\bf 325} (1989) 745.
  %%CITATION = NUPHA,B325,745;%%
\bibitem{Garidi:2003ys}
  T.~Garidi,
  %``What is mass in de Sitterian physics?,''
  hep-th/0309104.
  %%CITATION = HEP-TH/0309104;%%  
\bibitem{Zinoviev:2006im}
  Y.~.M.~Zinoviev,
  %``On massive spin 2 interactions,''
  Nucl.\ Phys.\ B {\bf 770} (2007) 83
  [hep-th/0609170].
  %%CITATION = HEP-TH/0609170;%%
\bibitem{Joung:2012rv}
  E.~Joung, L.~Lopez and M.~Taronna,
  %``On the cubic interactions of massive and partially-massless higher spins in (A)dS,''
  JHEP {\bf 1207} (2012) 041
  [arXiv:1203.6578 [hep-th]].
  %%CITATION = ARXIV:1203.6578;%%
\bibitem{deRham:2012kf}
  C.~de Rham and S.~Renaux-Petel,
  %``Massive Gravity on de Sitter and Unique Candidate for Partially
  %Massless Gravity,'' 
  arXiv:1206.3482 [hep-th].
  %%CITATION = ARXIV:1206.3482;%%
\bibitem{Deser:2013uy}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``Nonlinear Partially Massless from Massive Gravity?,''
  Phys.\  Rev.\  D 87, {\bf 101501} (R) (2013)
  [arXiv:1301.5621 [hep-th]].
  %%CITATION = ARXIV:1301.5621;%%
\bibitem{deRham:2013wv}
  C.~de Rham, K.~Hinterbichler, R.~A.~Rosen and A.~J.~Tolley,
  %``Evidence for and Obstructions to Non-Linear Partially Massless Gravity,''
  arXiv:1302.0025 [hep-th].
  %%CITATION = ARXIV:1302.0025;%%  
\bibitem{Deser:2013gpa}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``No consistent bimetric gravity?,''
  arXiv:1306.0647 [hep-th].
  %%CITATION = ARXIV:1306.0647;%%
\bibitem{Paulos:2012xe}
  M.~F.~Paulos and A.~J.~Tolley,
  %``Massive Gravity Theories and limits of Ghost-free Bigravity models,''
  arXiv:1203.4268 [hep-th].
  %%CITATION = ARXIV:1203.4268;%%
\bibitem{Sisman:2012rc}
  T.~C.~Sisman, I.~Gullu and B.~Tekin,
  %``Spectra, vacua and the unitarity of Lovelock gravity in D-dimensional AdS spacetimes,''
  Phys.\ Rev.\ D {\bf 86} (2012) 044041
  [arXiv:1204.3814 [hep-th]].
  %%CITATION = ARXIV:1204.3814;%%  
\bibitem{Stelle:1976gc}
  K.~S.~Stelle,
  %``Renormalization of Higher Derivative Quantum Gravity,''
  Phys.\ Rev.\ D {\bf 16} (1977) 953.
  %%CITATION = PHRVA,D16,953;%%
\bibitem{Stelle:1977ry}
  K.~S.~Stelle,
  %``Classical Gravity with Higher Derivatives,''
  Gen.\ Rel.\ Grav.\  {\bf 9} (1978) 353.
  %%CITATION = GRGVA,9,353;%%
\bibitem{Ostrogradski}
  M.~Ostrogradski,
  Mem.\ Ac.\ St.~Petersbourg  {\bf VI} (1850) 385. 
\bibitem{Bergshoeff:2009aq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``More on Massive 3D Gravity,''
  Phys.\ Rev.\ D {\bf 79} (2009) 124042
  [arXiv:0905.1259 [hep-th]].
  %%CITATION = ARXIV:0905.1259;%%
\bibitem{Kleinschmidt:2012rs}
  A.~Kleinschmidt, T.~Nutma and A.~Virmani,
  %``On unitary subsectors of polycritical gravities,''
  Gen.\  Rel.\  Grav.\  {\bf 45} (2013) 727
  [arXiv:1206.7095 [hep-th]].
  %%CITATION = ARXIV:1206.7095;%%
\bibitem{Gullu:2010pc}
  I.~Gullu, T.~C.~Sisman and B.~Tekin,
  %``Born-Infeld extension of new massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 27} (2010) 162001
  [arXiv:1003.3935 [hep-th]].
  %%CITATION = ARXIV:1003.3935;%%
\bibitem{Paulos:2010ke}
  M.~F.~Paulos,
  %``New massive gravity extended with an arbitrary number of curvature corrections,''
  Phys.\ Rev.\ D {\bf 82} (2010) 084042
  [arXiv:1005.1646 [hep-th]].
  %%CITATION = ARXIV:1005.1646;%%
\bibitem{Bach}
  R.~Bach,
  Math.\ Zeitschr.\ {\bf 9} (1921) 110.
  %%CITATION = GRGVA,9,353;%%  
\bibitem{Kaku:1977pa}
  M.~Kaku, P.~K.~Townsend and P.~van Nieuwenhuizen,
  %``Gauge Theory of the Conformal and Superconformal Group,''
  Phys.\ Lett.\ B {\bf 69} (1977) 304.
  %%CITATION = PHLTA,B69,304;%%
\bibitem{Deser:2012qg}
  S.~Deser, E.~Joung and A.~Waldron,
  %``Partial Masslessness and Conformal Gravity,''
  J.\ Phys.\ A (2012)
  [arXiv:1208.1307 [hep-th]].
  %%CITATION = ARXIV:1208.1307;%%
\bibitem{Fradkin:1981iu}
  E.~S.~Fradkin and A.~A.~Tseytlin,
  %``Renormalizable asymptotically free quantum theory of gravity,''
  Nucl.\ Phys.\ B {\bf 201} (1982) 469.
  %%CITATION = NUPHA,B201,469;%%  
\bibitem{Lee:1982cp}
  S.~C.~Lee and P.~van Nieuwenhuizen,
  %``Counting Of States In Higher Derivative Field Theories,''
  Phys.\ Rev.\ D {\bf 26} (1982) 934.
  %%CITATION = PHRVA,D26,934;%%
\bibitem{Riegert:1984hf}
  R.~J.~Riegert,
  %``The Particle Content Of Linearized Conformal Gravity,''
  Phys.\ Lett.\ A {\bf 105} (1984) 110.
  %%CITATION = PHLTA,A105,110;%%
\bibitem{Maldacena:2011mk}
  J.~Maldacena,
  %``Einstein Gravity from Conformal Gravity,''
  arXiv:1105.5632 [hep-th].
  %%CITATION = ARXIV:1105.5632;%%
\bibitem{Mannheim:2011ds}
  P.~D.~Mannheim,
  %``Making the Case for Conformal Gravity,''
  Found.\ Phys.\  {\bf 42} (2012) 388
  [arXiv:1101.2186 [hep-th]].
  %%CITATION = ARXIV:1101.2186;%%  
\bibitem{Bender:2007wu}
  C.~M.~Bender and P.~D.~Mannheim,
  %``No-ghost theorem for the fourth-order derivative Pais-Uhlenbeck oscillator model,''
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 110402
  [arXiv:0706.0207 [hep-th]].    
\bibitem{Volkov:2013roa}
  M.~S.~Volkov,
  %``Self-accelerating cosmologies and hairy black holes in ghost-free bigravity and massive gravity,''
  arXiv:1304.0238 [hep-th].
  %%CITATION = ARXIV:1304.0238;%% 
\bibitem{Sjors:2011iv}
  S.~Sjors and E.~Mortsell,
  %``Spherically Symmetric Solutions in Massive Gravity and Constraints from Galaxies,''
  JHEP {\bf 1302} (2013) 080
  [arXiv:1111.5961 [gr-qc]].
  %%CITATION = ARXIV:1111.5961;%%
\bibitem{Enander:2013kza}
  J.~Enander and E.~Mortsell,
  %``Strong lensing constraints on bimetric massive gravity,''
  arXiv:1306.1086 [astro-ph.CO].
  %%CITATION = ARXIV:1306.1086;%%   
\bibitem{Brito:2013yxa}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Partially massless gravitons do not destroy general relativity black holes,''
  Phys.\  Rev.\ D {\bf 87} (2013) 124024
  [arXiv:1306.0908 [gr-qc]].
  %%CITATION = ARXIV:1306.0908;%%   
\bibitem{Gregory:1993vy}
  R.~Gregory and R.~Laflamme,
  %``Black strings and p-branes are unstable,''
  Phys.\ Rev.\ Lett.\  {\bf 70} (1993) 2837
  [hep-th/9301052].
  %%CITATION = HEP-TH/9301052;%% 
\bibitem{Babichev:2013una}
  E.~Babichev and A.~Fabbri,
  %``Instability of black holes in massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 30} (2013) 152001
  [arXiv:1304.5992 [gr-qc]].
  %%CITATION = ARXIV:1304.5992;%%
\bibitem{Brito:2013wya}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Massive spin-2 fields on black hole spacetimes: Instability of the Schwarzschild and Kerr solutions and bounds on the graviton mass,''
  Phys.\  Rev.\ D {\bf 88} (2013) 023514
  [arXiv:1304.6725 [gr-qc]].
  %%CITATION = ARXIV:1304.6725;%% 
\bibitem{Hinterbichler:2013eza}
  K.~Hinterbichler,
  %``Ghost-Free Derivative Interactions for a Massive Graviton,''
  arXiv:1305.7227 [hep-th].
  %%CITATION = ARXIV:1305.7227;%%      
\bibitem{Huang:2012pe}
  Q.~-G.~Huang, Y.~-S.~Piao and S.~-Y.~Zhou,
  %``Mass-Varying Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124014
  [arXiv:1206.5678 [hep-th]].
  %%CITATION = ARXIV:1206.5678;%% 
\bibitem{Huang:2013mha}
  Q.~-G.~Huang, K.~-C.~Zhang and S.~-Y.~Zhou,
  %``Generalized massive gravity in arbitrary dimensions and its Hamiltonian formulation,''
  arXiv:1306.4740 [hep-th].
  %%CITATION = ARXIV:1306.4740;%%   
\bibitem{Gabadadze:2012tr}
  G.~Gabadadze, K.~Hinterbichler, J.~Khoury, D.~Pirtskhalava and M.~Trodden,
  %``A Covariant Master Theory for Novel Galilean Invariant Models and Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124004
  [arXiv:1208.5773 [hep-th]].
  %%CITATION = ARXIV:1208.5773;%%
\bibitem{D'Amico:2012zv}
  G.~D'Amico, G.~Gabadadze, L.~Hui and D.~Pirtskhalava,
  %``Quasi-Dilaton: Theory and Cosmology,''
  arXiv:1206.4253 [hep-th].
  %%CITATION = ARXIV:1206.4253;%%   
%\cite{Ondo:2013wka}
\bibitem{Cai:2013lqa}
  Y.~-F.~Cai, F.~Duplessis and E.~N.~Saridakis,
  %``$F(R)$ nonlinear massive gravity and cosmological implications,''
  arXiv:1307.7150 [hep-th].
  %%CITATION = ARXIV:1307.7150;%%  
\bibitem{Nojiri:2013zza}
  S.~'I.~Nojiri and S.~D.~Odintsov,
  %``Accelerating cosmology in modified gravity: from convenient $F(R)$ or string-inspired theory to bimetric $F(R)$ gravity,''
  arXiv:1306.4426 [gr-qc].
  %%CITATION = ARXIV:1306.4426;%% 
\bibitem{deRham:2013qqa}
  C.~de Rham, L.~Heisenberg and R.~H.~Ribeiro,
  %``Quantum Corrections in Massive Gravity,''
  arXiv:1307.7169 [hep-th].
  %%CITATION = ARXIV:1307.7169;%%  
\bibitem{Srednicki:2007qs}
  M.~Srednicki,
  %``Quantum field theory,''
  Cambridge, UK: Univ. Pr. (2007) 641 p
  
  
  
  
  
\bibitem{???} {\bfseries THE REMAINING CITATIONS ARE NEVER REFERED TO.}





\bibitem{Wald:1984rg}
  R.~M.~Wald,
  %``General Relativity,''
  Chicago, Usa: Univ. Pr. ( 1984) 491p.

\bibitem{Ondo:2013wka}
  N.~A.~Ondo and A.~J.~Tolley,
  %``Complete Decoupling Limit of Ghost-free Massive Gravity,''
  arXiv:1307.4769 [hep-th].
  %%CITATION = ARXIV:1307.4769;%%  
  
  
  


\end{thebibliography}


    
    

    
    
    
    

        
        
        
    




==> Bibliography/OrderReferences/all.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Introduction}
\label{intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





Since its introduction in 1916~\cite{Einstein:1916vd}, Einstein's theory of General Relativity (GR) has successfully explained the majority of gravity-related phenomena. It reproduces Newtonian dynamics in the weak-gravity limit, makes observable predictions, such as the bending of light by massive objects, and until today it withstands solar system tests to a very high precision. At the same time, containing the scalar curvature of a metric tensor, the Einstein-Hilbert action for GR offers an intuitive geometrical interpretation of the theory and Einstein's field equations can be regarded as capturing the interplay between matter and space-time geometry. 

On scales larger than the solar system, however, astrophysical observations have posed questions that to a large extend remain unanswered in the context of GR. These enigmas include the cosmological constant problem, which we will explain in more detail below, as well as the nature of dark matter. 
While there exists a large variety of promising candidates for dark matter particles in various extensions of the Standard Model of Particle Physics, so far there is no convincing explanation for the smallness of the observed cosmological constant. Unless they eventually both turn out to be resolved on the particle physics side, the severeness of the phenomenological problems challenges GR as the ultimate and complete theory of gravity. Therefore, it is reasonable to investigate the possibility of modifying Einstein's beautiful theory with the goal to provide explanations for the perplexing astrophysical observations. 

Of course, such a modification of the theory of gravity is already heavily constrained from the observational side since it must not alter the well-tested predictions of GR at solar-system scales.  
From a more theoretical perpective, looking for alternatives beyond GR is also motivated by String Theory, the most promising candidate for a quantum theory of gravity. GR itself cannot be promoted into a renormalizable quantum theory; it can at most be an effective theory that requires an ultraviolet (UV) completion. 
String Theory in the UV predicts an effective action at low energies that includes the Einstein-Hilbert term of GR plus higher-curvature corrections, as well as couplings to many fields of different spin. Computing this effective action explicitly in string perturbation theory is tedious but, alternatively, one can choose to search for consistent effective theories in a bottom-up approach. 
Following this strategy reveals that modifying GR is surprisingly difficult; almost any alteration of the Einstein-Hilbert action leads to inconsistencies in the theory. Moreover, the nonlinearities of GR often complicate consistency analyses of suggested modified theories and it happens rather rarely that a modification is proven to be consistent. Finding an alternative theory of gravity without inconsistencies is therefore always an important achievement and it is worth investigating the new theory in detail.

As a field theory, GR describes nonlinear self-interactions of a massless spin-2 excitation. A logical first guess for a modification of this setup would be the addition of a mass term for the spin-2 field. The resulting theory should describe nonlinear interactions of a massive spin-2 field and is commonly referred to as \textit{Massive Gravity}. However, the problem with a massive graviton is that a generic mass term introduces ghosts into the physical spectrum. Ghosts correspond to fields with negative kinetic energy that lead to instabilities at the classical and nonunitarity at the quantum level. In a consistent theory, it is necessary to avoid the presence of ghost-fields which puts severe constraints on the mass term and interaction potential of the spin-2 field.

To summarize, the search for a consistent theory of an interacting massive spin-2 field is motivated by the following question:
\begin{itemize}
\item[] Can a massive graviton explain unresolved puzzles in cosmology? 
\end{itemize}
But due to the difficulty of consistently modifying GR, before we can address this question, we need to answer an even more fundamental one:
\begin{itemize}
\item[] How can we describe massive spin-2 particles in field theory?
\end{itemize}
Even without a cosmological constant or Dark Matter problem, this task is interesting from a purely theoretical point of view: It is well-known how to describe massless and massive particles with spin $<2$ in field theory, and there is no obvious reason why there should not exist a corresponding model for spin 2.

Discussing consistency proofs and special features of recently discovered nonlinear theories for massive spin-2 fields, this thesis is mostly devoted to the latter of the two problems, although basic applications to cosmology are also provided. Before diving into this engrossing new subject we present the history of Massive Gravity, explain the cosmological constant problem and provide the basics of theories with spin-2 fields in the remainder of the introduction.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Historical development}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Finding a consistent theory that describes a massive spin-2 field is an old problem. In the year 1939, Fierz and Pauli wrote down the unique ghost-free mass term for a linearized spin-2 fluctuation~\cite{Fierz:1939ix}. An a priori arbitrary coefficient in the mass term needs to be tuned to a specific value in order to remove inconsistencies. 
About 30 years later, in two independent articles, van Dam and Veltman as well as Zakharov discovered that in the zero-mass limit the Fierz-Pauli theory coupled to sources does not converge to the massless theory~\cite{vanDam:1970vg, Zakharov:1970cc}. Namely, the helicity-zero mode of the massive spin-2 field does not decouple in this limit but gives an additional contribution to the vacuum amplitude of two interacting sources. Therefore, this \textit{vDVZ discontinuity} implies that even a very small graviton mass has significant impact on gravitational interactions between sources. In particular, in the zero-mass limit, GR augmented by the Fierz-Pauli term predicts different gravitational constants for conformal and non-conformal matter. Such a difference would be observable in measurements of the gravitational constant for light bending, whose value in the Fierz-Pauli theory with infinitely small mass differs by 25$\%$ from the one predicted by GR. Observations clearly rule out this possibility and a massive graviton would have been discarded decades ago had Vainshtein not found his famous loophole which suggested that a nonlinear completion of the Fierz-Pauli theory could avoid the vDVZ discontinuity~\cite{Vainshtein:1972sx}. Vainshtein showed that around massive sources the linear approximation loses its validity below a certain distance scale. This \textit{Vainshtein radius} becomes infinitely large in the limit of zero Fierz-Pauli mass and in this case there is no regime where the linear theory is valid. Clearly, such a \textit{Vainshtein mechanism} requires a nonlinear extension of the Fierz-Pauli mass term which, not unexpectedly, generically reintroduces inconsistencies. In fact, already in 1972, Boulware and Deser claimed that any nonlinear completion of Fierz-Pauli theory would exhibit a ghost instability~\cite{Boulware:1972zf, Boulware:1973my}. Their results were trusted and for almost 40 years there was little progress in the field of Massive Gravity. Moreover, in 2005, an analysis by Creminelli et.~al.~that was based on earlier work by Arkani-Hamed et.~al.~\cite{ArkaniHamed:2002sp} seemingly confirmed the unavoidable presence of the Boulware-Deser ghost in any nonlinear extension of the Fierz-Pauli theory.

The peripeteia came in 2010, when de Rham, Gabadadze and Tolley (dRGT) revisited the analysis of Creminelli et.~al.~and discovered a minor sign mistake which unfortunately had a large impact on the paper's final conclusion \cite{deRham:2010ik, deRham:2010kj}. After correcting the sign, they found that it is possible to construct a theory of nonlinear Massive Gravity which is ghost-free in a certain decoupling limit. This alone did not guarantee the consistency of the full theory away from the decoupling limit but, in the following year, their reformulation of the dRGT theory~\cite{Hassan:2011vm} enabled Hassan and Rosen to prove the absence of the Boulware-Deser ghost in a Hamiltonian constraint analysis~\cite{Hassan:2011hr, Hassan:2011ea}. Furthermore, they generalized the dRGT setup, which describes a nonlinearly interacting massive spin-2 field in flat space, to a ghost-free bimetric theory containing nonlinear interactions of a massless and massive spin-2 field in a dynamical background~\cite{Hassan:2011zd}. These works established the first consistent nonlinear theory for massive spin-2 fields. 

%The discovery of a consistent nonlinear theory for massive spin-2 fields opened up a new research area. Of particular interest were classical solutions within the dRGT and the Hassan-Rosen model~\cite{} as well as perturbations around them~\cite{}.

Inconsistent models with bimetric interactions had been considered earlier in the literature, for the first time by Rosen in 1940~\cite{Rosen:1940zz,Rosen:1975kk} and later by Aragone and Deser~\cite{Aragone:1971kh} as well as Isham, Salaam and Strathdee~\cite{Isham:1971gm}. The consistent bimetric model had actually already appeared in \cite{Chamseddine:1978yu} where, however, the ghost issue was not addressed.
Besides these, alternative theories with massive gravitons have also been under investigation. These include the DGP model~\cite{Dvali:2000rv,Dvali:2000hr}, Kaluza-Klein scenarios~\cite{Kaluza:1921tu, Klein:1926tv}, New Massive Gravity~\cite{Bergshoeff:2009hq}, Topological Massive Gravity~\cite{Deser:1981wh,Deser:1982vy} and Lorentz violating models~\cite{ArkaniHamed:2003uy}.











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The cosmological constant problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Einstein's equations, the equations of motion for the metric tensor $\gmn$ that follow from the Einstein-Hilbert action of General Relativity, are of the form
\beqn\label{ee}
R_{\mu\nu}-\frac{1}{2}R\,\gmn=\frac{1}{M_{\mathrm{Pl}}^{2}}T_{\mu\nu}-\Lambda\gmn\,.
\eeqn 
The left-hand side contains the Ricci curvature tensor and scalar of $\gmn$ and hence describes the dynamics of space-time geometry. The right-hand side consists of matter sources with stress energy tensor $T_{\mu\nu}$ to which we have added a cosmological constant term. 

In the absence of local sources, there is still a contribution from the matter sector to Einstein's equations because quantum field theory predicts a vacuum expectation value $\braket{T_{\mu\nu}}$ for the source. In particular, the component $\braket{T_{00}}$ is the vacuum energy density that includes contributions from normal ordering of operators in the Hamiltonian and from expectation values of scalar potentials after symmetry breaking. The size of these contributions depends on the specific model, its symmetry breaking mechanisms and UV cutoff, but generically it certainly satisfies $\braket{T_{00}}>(1\,\text{TeV})^4$. In the worst case, it is as large as the Planck density, $\braket{T_{00}}\sim (10^{18}\text{GeV})^4$. As we will review in chapter~\ref{ch:cosmo}, such a huge value for the vacuum energy density would make the expansion of the universe accelerate at an immense rate. Although in the late 1990's observational data revealed that the cosmological expansion is indeed accelerating~\cite{Riess:1998cb, Perlmutter:1998np}, the vacuum energy density driving this acceleration must be as tiny as $10^{-47}(\text{GeV})^4$. The theoretical prediction and the observed value therefore differ by 60 to 120 orders of magnitude. 

In principle, there is a way to cure the discrepancy by hand: One could simply adjust the free parameter $\Lambda$ in (\ref{ee}) such that it cancels the large number in $\braket{T_{00}}$ up to 60-120 decimal places. Obviously this method of dealing with the difference in observed and measured vacuum energies requires an enormous amount of fine-tuning. Although there is no mathematical inconsistency in this procedure, the inexplicable almost exact cancellation is a thorn in the flesh of most theoretical physicists. 
The \textit{cosmological constant problem} has become one of the greatest challenges of modern theoretical physics and there is a countless number of proposals for solutions in the literature. For a recent review we refer the reader to~\cite{Martin:2012bt}.  


A priori, there is good reason to believe that a theory of Massive Gravity could be a step towards explaining the smallness of the observed vacuum energy. 
The main idea is that a small graviton mass is protected against quantum corrections, which relies on the appearance of a gauge symmetry (namely diffeomorphism invariance) in the zero-mass limit. Contrarily, when the cosmological constant is taken to zero, no such symmetry emerges and hence the value for the vacuum energy is unprotected. A tiny graviton mass is therefore considered less unnatural than a cosmological constant of the same scale. The smallness of the mass parameter would still have to be explained, but once it is small at the classical level, quantum corrections will be of the same order of magnitude and not drive it to the cut-off scale. 
If now, in a Massive Gravity theory, a large vacuum energy $\braket{T_{00}}$ generated on the matter side is somehow ``screened" by a mass term with a small graviton mass in the modified Einstein equations, the effect of the vacuum energy on the acceleration of the cosmological expansion could be small. Despite these promising ideas, it seems that a straightforward screening mechnanism does not exist in the dRGT and Hassan-Rosen models to be considered in this thesis. However, this question is not yet finally settled and, moreover, there appear to exist other interesting possibilities to address the cosmological constant problem. 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Massless and massive field theories}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The modern description of particle physics is based on the extremely successful framework of quantum field theory (QFT). Quantum states that correspond to physical particles are created and annihilated by local operators, or quantum fields, that transform in irreducible unitary representations of the Poincar\'e group which, in turn, characterizes the isometries of the underlying Minkowski space time. According to Wigner's classification~\cite{Wigner:1939cj}, the irreducible unitary representations with non-negative energy can be labelled by two Casimir invariants related to mass and spin (or helicity) of the corresponding particle. 
%It is furthermore important to distinguish between the massless and massive case which correspond to different little groups that leave the particle's four-momentum invariant.  

The construction of a QFT with a Hilbert space of particle states is usually achieved in two steps:  
One begins by writing down a Lagrangian of a consistent classical field theory for which the Hamiltonian is bounded from below. Then one quantizes the theory either in the path integral formalism or by imposing canonical (anti)commutation relations for the fields. The process of quantization can in principle reintroduce inconsistencies that render the theory nonunitary but, if one is lucky, it is possible to avoid these. Then, in the absence of gauge anomalies, there may exist a consistent quantum version of the classical theory. The crucial point is that for the existence of a unitary description of particles in a QFT framework, it is absolutely necessary to start from a classically consistent field theory. 

Apart from the problem of nonunitarity in its quantum version, a classical field theory with a Hamiltonian that is not bounded from below is not even meaningful on its own. The instability allows the field to transfer an infinite amount of energy to other fields it interacts with and hence the theory cannot make any useful predictions. Thus, a Hamiltonian that is bounded from below is required from any feasible field theory (classical or quantum). In particular, one must demand the absence of fields that have wrong signs in front of their mass terms (\textit{tachyons}) or kinetic terms (\textit{ghosts}).  

Consistent classical theories for both massless and massive fields with spin 0, 1/2 and 1 are well-known\footnote{Note also that a consistent classical theory for a massive/massless gravitino with spin 3/2 exists in the form of broken/unbroken supergravity.} and their quantum versions play an important role in theoretical particle physics. In fact, the Standard Model of Particle Physics is a consistent quantum theory of fields with spin~1/2 (fermions), spin~1 (gauge bosons) and spin~0 (Higgs boson). Table~\ref{fttable} displays the structure of Lagrangians for fields of different spin.

\begin{table}[htdp]
\caption{Lagrangians for fields of different spin. The massless theories correspond to setting $m=0$.}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline && \\
spin 0& scalar field $\phi$ & $\mathcal{L}_\phi=-\partial_\mu\phi\partial^\mu\phi-m^2\phi^2$
 \\ &&\\
\hline && \\
spin $\tfrac{1}{2}$&  spinor field $\psi^\alpha$ & $\mathcal{L}_\psi=-\bar{\psi}\gamma^\mu\partial_\mu\psi-m\bar{\psi}\psi$ \\ &&\\
\hline &&\\
spin 1& vector field $A_\mu$& $\mathcal{L}_A=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-\frac{m^2}{2}A^\mu A_\mu$ \\ &&\\
\hline 
\end{tabular}
\end{center}
\label{fttable}
\end{table}%

Compared to its lower-spin companions, spin-2 fields turn out to be much more difficult to handle. The consistent classical theory for a massless spin-2 particle with nonlinear self-interactions is General Relativity. However, when trying to quantize the theory one faces another problem because the Lagrangian for GR is nonrenormalizable. This means that predictions for scattering cross sections contain infinities that cannot be absorbed into perturbatively renormalized coupling constants. Due to this obstruction, GR makes sense only as an effective field theory valid at low energies which is believed to have a consistent, renormalizable completion in the ultraviolet regime. For massive spin-2 fields the situation is even worse: Adding a mass term to the Einstein-Hilbert action of GR generically introduces ghost instabilities that render the theory inconsistent already at the classical level. 

In the following we discuss classical field theories of massless and massive spin-1 and spin-2 particles in more detail. In particular we review the degree-of-freedom counting in these theories using gauge invariances and constraints in the equations of motion. 

















%%%%%%%%%%%%%%%%%%%%%
\subsection{Spin-1}
%%%%%%%%%%%%%%%%%%%%%

Before coming to the more relevant example of linear spin-2 theories, it is instructive to begin by considering spin-1 fields that share several features with their spin-2 analogues. Unlike in the theories for spin-0 and spin-1/2 fields, gauge invariance is needed in the massless case to obtain the correct number of propagating degrees of freedom.
We first discuss the massless vector field that appears in classical electrodynamics and then present the Proca theory for massive spin-1 fields.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Massless theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The theory for a massless spin-1 field $A_\mu(x)$ in flat space is given by Maxwell's Lagrangian,
\beqn
\mathcal{L}_\mathrm{Maxwell}=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-J^\mu A_\mu\,,\qquad F_{\mu\nu}\equiv \partial_\mu A_\nu-\partial_\nu A_\mu\,,
\eeqn
where $J^\mu$ is an external source and indices are contracted with the Minkowski metric $\emn$. 
The equations of motion obtained from varying with respect to $A_\nu$ are
\beqn
\partial^\mu F_{\mu\nu}=J_\nu\,.
\eeqn
Due the identity $\partial^\nu\partial^\mu F_{\mu\nu}=0$, the divergence of the equations implies that the source must be conserved, $\partial^\mu J_\mu=0$.
With the help of this conservation law\footnote{In general, the source is not necessarily conserved off-shell since its conservation is an on-shell constraint. For a Lagrangian with off-shell gauge-invariance we need to require off-shell conservation of $J_\mu$ or, equivalently, off-shell gauge-invariance of the source term $J^\mu A_\mu$.} it can be shown that both the above Lagrangian and the equations are invariant under a U(1) gauge transformation,
\beqn\label{gtso}
A_\mu(x)\longrightarrow A_\mu(x)+\partial_\mu\phi(x)\,,
\eeqn
where $\phi(x)$ is a scalar gauge parameter. The symmetry transformation may be used to choose the Lorenz gauge which is defined through the condition $\partial^\mu A_\mu=0$.
In this gauge the equations of motion reduce to 
\beqn
\Box A_\mu=J_\mu\,,
\eeqn
which is simply a sourced Klein-Gordon equation for a massless field.
However, the gauge is not yet fixed completely because we can still perform gauge transformations~(\ref{gtso}) with $\Box\phi=0$ that do not take us out of the Lorenz gauge. The gauge condition $\partial^\mu A_\mu=0$ together with this residual gauge transformation remove two degrees of freedom from $A_\mu$. In~$d$ dimensions the theory for a massless spin-1 particle therefore propagates $d-2$ degrees of freedom.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Massive theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, let us turn to the massive spin-1 particle. It is described by the Proca Lagrangian,
\beqn
\mathcal{L}_\mathrm{Proca}=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-\frac{m^2}{2}A^\mu A_\mu-J^\mu A_\mu\,.
\eeqn
Clearly, this is the same as Maxwell's Lagrangian with an additional mass term quadratic in the field.
The equations of motion in the Proca theory read 
\beqn
\partial^\mu F_{\mu\nu}-m^2A_\nu=J_\nu\,.
\eeqn
The mass term breaks the above U(1) symmetry and the Lagrangian is no longer gauge invariant. Hence, this time there is no symmetry that can be used to remove redundant components of the field.
On the other hand, taking the divergence of the equations of motion we now obtain a constraint equation that contains the field,
\beqn\label{constAmu}
\partial^\mu A_\mu=-\frac{1}{m^2}\partial^\mu J_\mu\,.
\eeqn
The source is no longer necessarily conserved but, if we anyway assume $\partial^\mu J_\mu=0$, then the constraint corresponds precisely to the above Lorenz gauge condition. Plugging it back into the equations of motion we obtain (for a conserved source)
\beqn
(\Box-m^2)A_\mu=J_\mu\,.
\eeqn
Thus the massive spin-1 field again satisfies a sourced Klein-Gordon equation. Since one degree of freedom is removed by the constraint, the theory has $d-1$ propagating degrees of freedom.

 








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Spin-2}\label{sec:FP}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Now we are ready to perform the degree-of-freedom counting in the linear spin-2 theory. Once more, we begin with the massless case before turning to the massive Fierz-Pauli theory. Eventually, we draw the connection between the linear massless theory and nonlinear General Relativity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear massless theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The Lagrangian for a massless spin-2 field in flat space to quadratic order in the field reads
\beqn\label{masslesslin}
\mathcal{L}_\mathrm{lin}=h^{\mu\nu}\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}-\kappa h^{\mu\nu} T_{\mu\nu}\,,
\eeqn
where $T^{\mu\nu}$ is an external source and the structure of the kinetic terms is captured by the two-derivative operator,
\begin{align}\label{kinstruc1}
	\mathcal{E}_{\mu\nu}^{\phantom\mu\phantom\nu\rho\sigma} = \tfrac{1}{2}\Big(
	\eta_\mu^{\phantom\mu\rho}\eta_\nu^{\phantom\nu\sigma}\Box
	&-\eta_\nu^{\phantom\nu\sigma}\partial_\mu\partial^\rho
	-\eta_\mu^{\phantom\mu\sigma}\partial_\nu\partial^\rho\nn\\
	&+\eta_{\mu\nu} \partial^\sigma\partial^\rho
	+\eta^{\rho\sigma}\partial_\mu\partial_\nu
	-\eta^{\rho\sigma}\eta_{\mu\nu}\Box\Big)
	\,. 
\end{align}
The corresponding equations of motion are 
\beqn
\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}=\frac{\kappa}{2} T_{\mu\nu}\,.
\eeqn
The linear Bianchi identity, $\partial^\mu \mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}=0$, implies conservation of the source, $\partial^\mu T_{\mu\nu}=0$. Using this it can easily be verified that the Lagrangian and equations for the massless spin-2 particle are invariant under the following gauge transformations,
\beqn\label{lindiff}
\hmn(x)\longrightarrow \hmn(x) + \partial_\mu\xi_\nu(x)+\partial_\nu\xi_\mu(x)\,,
\eeqn
with vector gauge parameter $\xi_\mu(x)$. As in the spin-1 case, we can use this symmetry to pick a convenient gauge. The Lorenz gauge condition for the spin-2 field is $\partial^\mu\hmn-\frac{1}{2}\partial_\nu h=0$, and, in this gauge, the equations of motion can be written as
\beqn
\Box\hmn=\kappa T_{\mu\nu}-\frac{\kappa}{d-2}T\,.
\eeqn
Again, there exist residual gauge transformations, namely those with $\Box\xi_\mu=0$, that leave the Lorenz gauge intact and correspond to further redundant degrees of freedom.
In total, gauge invariance therefore removes $2d$ of the $d(d+1)/2$ components in $\hmn$, and the only propagating modes are the $d(d-3)/2$ degrees of freedom of a massless spin-2 particle.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear massive theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As has been known since the work of Fierz and Pauli from 1939~\cite{Fierz:1939ix}, the quadratic Lagrangian for a massive spin-2 particle in flat space has the form
\beqn\label{FPlag}
\mathcal{L}_\mathrm{FP}=h^{\mu\nu}\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}-\frac{m_\mathrm{FP}^2}{2}(h^{\mu\nu}\hmn-h^2)-\kappa h^{\mu\nu} T_{\mu\nu}\,,
\eeqn
where the kinetic operator is the same as in the massless case, given by (\ref{kinstruc1}).
The equations of motion obtained from the Lagrangian for the massive particle are
\beqn
\mathcal{E}_{\mu\nu}^{\phantom{\mu\nu}\rho\sigma}h_{\rho\sigma}-\frac{m_\mathrm{FP}^2}{2}(\hmn-\emn h)=\frac{\kappa}{2} T_{\mu\nu}\,.
\eeqn
The mass term breaks the gauge invariance of the massless theory but, as a consequence of the linearized Bianchi identity, the divergence and trace of these equations give rise to $d+1$ constraints,
\beqn\label{twoconstr}
\partial^\mu \hmn-\partial_\nu h&=&-\frac{\kappa}{m_\mathrm{FP}^2}\partial_\mu T^{\mu\nu}\,,\nn\\
h&=&\frac{1}{d-1}\frac{\kappa}{m_\mathrm{FP}^2}T+\frac{d-2}{d-1}\frac{\kappa}{m_\mathrm{FP}^4}\partial^\nu\partial^\mu T_{\mu\nu}\,.
\eeqn
The source is not necessarily conserved but we shall anyway assume $\partial_\mu T^{\mu\nu}=0$.
Then, unlike in the spin-1 example, the constraint equation obtained from taking the divergence of the equations of motion does not resemble the Lorenz gauge condition but differs by a factor of $1/2$ in front of the trace. For vanishing sources, the constraints imply that the massive spin-2 field is transverse and traceless. 

Using (\ref{twoconstr}) in the equations of motion, we arrive at
\beqn
(\Box-m_\mathrm{FP}^2)\hmn=\kappa\left(T_{\mu\nu}-\frac{1}{d-1}\left[\eta_{\mu\nu}-\frac{1}{m_\mathrm{FP}^2}\partial_\mu\partial_\nu T\right]\right) \,.
\eeqn
Therefore the massive spin-2 field also satisfies a sourced Klein-Gordon equation.
The constraints (\ref{twoconstr}) remove $d+1$ of the $d(d+1)/2$ components in $\hmn$, leaving us with the $d(d-1)/2-1$ propagating degrees of freedom of a massive spin-2 particle. 

An important observation is that modifying the structure of the mass term, i.e.~changing the numerical factor in front of $h^2$ in (\ref{FPlag}), introduces an additional degree of freedom into the theory. This happens because the trace constraint in (\ref{twoconstr}) is lost and $h$ satisfies a dynamical equation of motion instead. It can also be shown that the propagator corresponding to the extra degree of freedom comes with a residue of the wrong sign and therefore gives rise to a ghost instability. This unwanted dynamical field is referred to as the \textit{Boulware-Deser-ghost}. It is this ghost mode that complicates the construction of a nonlinear interaction potential for a spin-2 field because, even when banned from the linear theory, the ghost notoriously reappears through the higher-order interactions.

On the other hand, tuning the linear mass potential to the Fierz-Pauli structure comes with its own problems that threaten the phenomenological viability of the theory as a modification of general relativity. Namely, as already mentioned, it was shown by van Dam, Veltman and Zakharov (vDVZ) \cite{vanDam:1970vg, Zakharov:1970cc} that the $m_\mathrm{FP}\rightarrow 0$ limit of linear massive gravity is discontinuous. More precisely, the helicity-zero mode does not decouple from the sources in this limit and gives an extra contribution to the gravitational force for matter sources whose stress-energy tensors has nonvanishing trace. This leads to a substantial difference between the interactions of massive objects and massless particles, such as photons. This difference can be tested, for instance, by observing light bending by heavy objects. Such tests clearly rule out the existence of a vDVZ discontinuity.

Fortunately, it has been demonstrated by Vainshtein in that nonlinear self-interaction for the spin-2 field may be able to cure this problem~\cite{Vainshtein:1972sx}: The nonlinear theory becomes strongly coupled and the linear approximation breaks down at disctance scales smaller than the \textit{Vainshtein radius}. This radius is large for small $m_\mathrm{FP}$ and goes to infinity in the zero-mass limit. If it is large enough then, although beyond it the linear theory is valid, the vDVZ discontinuity cannot be observed.  
The existence of such a \textit{Vainshtein mechanism} requires a nonlinear completion of the Fierz-Pauli mass term which is one of the main motivations for the construction of a nonlinear theory of Massive Gravity.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Nonlinear massless theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To conclude the introduction, we outline the relation between the linear theory for massless spin-2 fields discussed above and Einstein's General Relativity.
The graviton in GR is a massless spin-2 particle and should hence be described by the Lagrangian~(\ref{masslesslin}). However, the equivalence principle tells us that the field should couple to all kinds of energy in the same manner, including its own stress-energy tensor. Implementing this requirement in~(\ref{masslesslin}) iteratively introduces nonlinearities and eventually leads to the Einstein-Hilbert action for GR.
In turn, the quadratic Lagrangian for a massless spin-2 particle follows from linearizing the Einstein-Hilbert action,
\beqn\label{EHGR}
S_{\mathrm{GR}}=M_{\mathrm{Pl}}^{d-2}\int \mathrm{d}^dx\,\sqrt{-g}~R ~+ \int \mathrm{d}^dx\,\sqrt{-g}~\mathcal{L}_\mathrm{m} \,,
\eeqn
in the perturbation $\hmn=\kappa^{-1}(\gmn-\emn)$ with $\kappa=M^{(2-d)/2}_{\mathrm{Pl}}$. The source is related to the matter Lagrangian~$\mathcal{L}_\mathrm{m}$ through the definition of the stress-energy tensor,
\beqn
T_{\mu\nu}\equiv-\frac{1}{\sqrt{-g}}\frac{\partial(\sqrt{-g}\,\mathcal{L}_\mathrm{m})}{\partial g^{\mu\nu}}\,.
\eeqn
The Einstein-Hilbert action is the gauge invariant nonlinear extension\footnote{One can also include self-interactions into the theory for the massless spin-1 field considered above. In order for the field to remain massless, these interactions must respect gauge invariance and this requirement leads to the structure of Yang-Mills theories~\cite{Henneaux:1997bm}. In the quantum theory, giving mass to non-Abelian spin-1 fields in a unitary and renormalizable way requires a Higgs mechanism, see e.g.~\cite{Ruegg:2003ps}.} of~(\ref{masslesslin}). It can be defined uniquely, as the field theory that describes nonlinear self-interactions of a massless spin-2 particle \cite{Hinterbichler:2011tt}. The gauge transformations~(\ref{lindiff}) are linearized general coordinate transformations (GCTs), under which the metric at the nonlinear level transforms as
\beqn
\gmn\longrightarrow\gmn+\nabla_\mu\xi_\nu+\nabla_\nu\xi_\mu\,.
\eeqn
The presence of a gauge symmetry at the nonlinear level ensures that the full theory propagates the same number of degrees of freedom as its linear version.

Naturally, the existence of a nonlinear closed form for the kinetic terms of a spin-2 particle motivates the search for a nonlinear completion of the Fierz-Pauli mass term. As we saw above, consistency of linearized Massive Gravity requires tuning of a coefficient in the mass potential. One can therefore expect that a consistent (i.e.~ghost-free) nonlinear potential cannot contain arbitrary interaction terms, but that the coefficients of certain terms will be related to each other by demanding the absence of the extra degree of freedom. We shall see in the next chapter that this is precisely what happens. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\chapter{Consistent Nonlinear Massive Gravity}
\label{ch:MG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

In this chapter we introduce the recently discovered consistent theory of nonlinear Massive Gravity. Its nonlinear interaction potential is the unique ghost-free completion of the Fierz-Pauli mass term and contains $(d-2)$ independent parameters in $d$ dimensions. Proving the consistency of the theory in two different formulations was the purpose of {\protect{\hyperref[papI]{Paper~I}}} and~{\protect{\hyperref[papIII]{III}}}.

We begin the discussion by pointing out some general features of nonlinear spin-2 interactions, emphasizing the necessity of a second rank-2 tensor in the theory.
Afterwards, we use insights from the Hamiltonian formulation of General Relativity to construct the ghost-free nonlinear mass potential. 
The resulting Massive Gravity action is the model constructed by de Rham, Gabadadze and Tolley (dRGT) in \cite{deRham:2010ik, deRham:2010kj}, generalized to arbitrary backgrounds. 
The interaction term manifestly breaks diffeomorphism invariance which can be restored using St\"uckelberg fields. The consistency proof in the gauge invariant formulation of nonlinear Massive Gravity is subject of the second half of this chapter.



  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\section{Construction of the ghost-free nonlinear theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 This section is devoted to the construction of the dRGT model for nonlinear Massive Gravity~\cite{deRham:2010ik, deRham:2010kj} as well as its generalization to arbitrary backgrounds by Hassan and Rosen~\cite{Hassan:2011vm}.
  The constructive consistency proof presented here is neither part of any of the papers accompanying the thesis nor has it appeared anywhere else in the literature. Nevertheless, it constitutes the most efficient and straightforward way to arrive at the consistent theory. 
Before we come to the proof, it is worthwile to make a few remarks on general properties of spin-2 interaction potentials.
 
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{General remarks on nonlinear interactions}\label{sec:nonlin}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the introduction we considered massless and massive theories for a linear fluctuation $\hmn$ in a fixed Minkowski background $\emn$. In the nonlinear massless theory given by the Einstein-Hilbert action of GR, it was possible to combine the background and the fluctuation into a single field $\gmn$. We would now like to do something similar in the massive case.

What we call a mass term for a rank-2 tensor $\gmn$ must be a scalar density, i.e.~it has to be a nontrivial scalar function $V(g)$ multiplied by the scalar density $\sqrt{-g}$. Obviously, the scalar function $V(g)$ cannot have any loose covariant indices. Moreover, it should not contain any derivatives. But then, the only object at hand to contract the indices of the metric tensor $\gmn$ is the metric itself which, since $g^{\mu\nu}\gmn=d$, leads to a trivial cosmological constant contribution in the action. We conclude that there is no possibility to construct a covariant nonlinear interaction term for a spin-2 field using only one tensor field.\footnote{Note the difference to e.g.~the vector example, where the metric $\gmn$ can be used to contract the indices in nonlinear interaction terms for $A_\mu$ in a nontrivial way. Furthermore, in the massless spin-2 theory this problem did not occur because in the kinetic terms the indices of the metric could be contracted with derivative operators.} 
Hence, we are forced to introduce a second rank-2 tensor, which we shall call $\fmn$ and which can be used to build nonlinear contractions with $\gmn$. The interaction potential will then be given by $\sqrt{-g}$ multiplying a scalar function of $g^{\rho\mu}\fmn$. 
  

In summary, we expect the nonlinear massive gravity action to be of the form,
\beqn\label{mggenact}
S_\mathrm{MG}=\int \mathrm{d}^dx~\sqrt{-g}~\left[M_{\mathrm{Pl}}^{d-2}R(g) - m^d\, V(g^{-1}f)\right]\,,
\eeqn
where $m$ is an arbitrary energy scale that sets the mass of the spin-2 field. In this setup, the second ``metric" $\fmn$ is a fixed background field that needs to be put into the theory by hand. From the viewpoint of field theory this seems unfamiliar because $\fmn$ is not determined by an equation of motion. But, in fact, there is no need to worry about this, since we will resolve this slightly confusing point in the next chapter, when we introduce the fully dynamical bimetric theory that treats $\gmn$ and $\fmn$ on the same footing. For now, let us accept the possibility to work with a fixed reference metric $\fmn$ and investigate the consistency of this class of theories. 

Obviously, a necessary requirement on the interaction potential in (\ref{mggenact}) is that it reduces to the Fierz-Pauli mass term when linearized around flat space (i.e.~with flat reference metric $\fmn$ and flat background for $\gmn$), otherwise it will certainly propagate the Boulware-Deser ghost. As it will turn out in a nonlinear constraint analysis, a generic interaction potential, even if it incorporates the Fierz-Pauli structure around flat space, will reintroduce this extra degree of freedom at the nonlinear level. This is anticipated from a simple degree-of-freedom counting:
The introduction of the interaction potential breaks the diffeomorphism invariance of general relativity. Therefore the $d$ gauge symmetries are lost and the theory generically will propagate $d$ additional degrees of freedom. Since $d(d-3)/2+d=d(d-1)/2$, this does not give the correct number for a massive spin-2 particle, but there is an extra degree of freedom in the theory. This is the nonlinear Boulware-Deser ghost and an extra constraint is needed to remove it from the spectrum of propagating modes. Tuning the linear mass term to the Fierz-Pauli combination ensured the presence of this constraint in the linear theory.
In section~\ref{sec:conspot} we will demonstrate that, in order to obtain an additional constraint and thereby ensure the absence of the ghost, it is necessary to impose strong restrictions on the structure of nonlinear interactions. In fact, demanding the presence of a constraint will fix all but $(d-2)$ coefficients of all possible interaction terms.
 
 
In the construction of the consistent theory, we will follow the approach of Boulware and Deser who studied Massive Gravity in the Hamiltonian formulation~\cite{Boulware:1972zf, Boulware:1973my}. They claimed that, even though it is possible to remove the ghost from the spectrum of propagating modes at the linear level, it will return for any nonlinear interaction terms that are added to the Lagrangian (\ref{FPlag}). In order to show that this result is in fact incorrect, we first need to familiarize us with variables suitable for the Hamiltonian formulation of GR.
   
  
   


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
\subsection{ADM variables for General Relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  




The Hamiltonian formulation of GR traces back to work by Arnowitt, Deser, and Misner (ADM) from 1962~\cite{Arnowitt:1962hi}. The authors decomposed the metric $\gmn$ into a scalar $N$, a symmetric $(d-1)\times (d-1)$ matrix $\gamma_{ij}$, and a vector $N_i$ with $(d-1)$ components as follows: 
\beqn\label{admmetr}
\gmn=\begin{pmatrix}
-N^2+N_i \gamma^{ij}N_j& N_j\\
N_i & \gamma_{ij}
\end{pmatrix}\,,
\eeqn
where $\gamma^{ij}$ denotes the inverse of $\gamma_{ij}$. This parametrization essentially splits the metric into its time ($0\mu$) and spatial ($ij$) components; in $d=4$ it is therefore also referred to as \textit{(3+1)-decomposition}. From (\ref{admmetr}) we can also compute the inverse of the metric,
\beqn\label{invadm}
g^{\mu\nu}=\frac{1}{N^2}\begin{pmatrix}
-1& N^j\\
N^i & N^2\gamma^{ij}-N^iN^j
\end{pmatrix}\,.
\eeqn
It turns out that, in any theory with kinetic structure given by the Einstein-Hilbert term, the $0\mu$-components are nondynamical gauge degrees of freedom because the Ricci scalar of $\gmn$ contains no derivatives of those components. Hence, all of the propagating modes are contained in the spatial metric $\gamma_{ij}$ which has $d(d-1)/2$ independent components. As we will see now, the gauge invariance of GR will reduce the number of propagating degrees of freedom to $d(d-3)/2$, along with the same number of corresponding canonical momenta.


In terms of the ADM variables the Einstein-Hilbert action (\ref{EHGR}) becomes (up to total derivatives that can be discarded) \cite{Arnowitt:1962hi}
\beqn\label{gradm}
S_{\mathrm{GR}}%=M_\mathrm{P}^{d-2}\int \mathrm{d}^4x~\sqrt{-g}~R
=M_\mathrm{P}^{d-2}\int \mathrm{d}^dx~\left(\pi^{ij}\partial_t \gamma_{ij}-NR^0-N_iR^i\right)\,,
\eeqn
where, in terms of the curvature scalar $R_{(d-1)}$ of the metric $\gamma_{ij}$,
\beqn
R^0&=& -\sqrt{\gamma}~ \left[R_{(d-1)} +\gamma^{-1}\left(\frac{1}{2}({\pi^i}_i)^2-\pi^{ij}\pi_{ij}\right)\right] \,,\nonumber\\
R^i&=& -2\partial_j\pi^{ij}.
\eeqn
The conjugate momenta $\pi^{ij}$ of the $d(d-1)/2$ metric components $\gamma_{ij}$ are computed from the GR Lagrangian in the standard way which leads to expressions in terms of derivatives of the $d$-dimensional metric.

As pointed out before, the action (\ref{gradm}) does not contain dynamical terms for the scalar $N$ nor for the vector $N^i$. On top of that, these variables appear only linearly.
Therefore they act as Lagrange multipliers, and their equations of motion do not contain $N$ and $N^i$ themselves. This means that these equations
constitute $d$ primary constraints~$R^\mu=(R^0, R^i)$ on the remaining $d(d-1)$ variables $\gamma_{ij}$ and $\pi^{ij}$. 

According to the theory of constrained Hamiltonian systems,\footnote{For review of this subject see~\cite{Date:2010xr}.} the presence of a gauge symmetry can now be seen in the Poisson algebra of the constraints, $\{R^\mu, R^\nu\}$. Here, the Poisson bracket for functions $A,B$ is defined as
\beqn\label{defpoisb}
\{A(x), B(y)\}\equiv\int \mathrm{d}^3z~\left(  \frac{\delta A(x)}{\delta g_{ij}(z)}\frac{\delta B(y)}{\delta \pi^{ij}(z)} -\frac{\delta A(y)}{\delta \pi^{ij}(z)}\frac{\delta B(x)}{\delta g_{ij}(z)}\right)\,.
\eeqn
The result for the constraint algebra of GR reads~(see e.g.~\cite{Khoury:2011ay})
\beqn
\{R^0(x), R^0(y)\}&=& R^i(y)\frac{\partial}{\partial y^i}\delta^3(x-y)-R^i(x)\frac{\partial}{\partial x^i}\delta^3(x-y)\, , \nonumber\\
\{R_i(x), R_j(y)\}&=& R_i(y)\frac{\partial}{\partial y^j}\delta^3(x-y)-R_j(x)\frac{\partial}{\partial x^i}\delta^3(x-y)\,,\nonumber\\
\{R^0(x), R_i(y)\}&=& -R^0(y)\frac{\partial}{\partial x^i}\delta^3(x-y)\,.
\eeqn
Since these brackets are proportional to the constraints themselves, they vanish on the constraint surface, as they should in the presence of a gauge symmetry. This implies that all $d$ primary constraints will serve to put conditions on the remaining variables $\gamma_{ij}$ and $\pi^{ij}$, while the Lagrange multipliers $N$ and $N^i$ remain undetermined. There will be no secondary constraints because the primary constraints are automatically preserved in time.

After imposing the $d$ conditions on $\gamma_{ij}$ and $\pi^{ij}$, we can still use gauge transformations to remove $d$ more degrees of freedom. In total we therefore end up with $d(d-3)$ variables, corresponding to the helicity states of the massless graviton and their canonical momenta. This shows that, even nonlinearly, GR propagates the correct number of degrees of freedom for describing a massless spin-2 particle.

Note that throughout the above discussion we never actually wrote down the Hamiltonian, but remained in the Lagrangian formulation. In order to investigate the positivity of the energy, this is naturally insufficient, but since here we were only interested in counting degrees of freedom there was no need to work with the Hamiltonian, which can trivially be obtained from (\ref{gradm}). 


        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%         
\subsection{ADM variables for Massive Gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

In a general nonlinearly interacting theory of the form (\ref{mggenact}), the lapse and shift functions $N$ and $N^i$ will still appear without derivatives. However, the interaction potential will in general no longer be linear in these functions. Therefore, their equations of motion, instead of imposing constraints on the remaining variables, will now determine $N$ and $N^i$ themselves. The $d$ gauge constraints are lost and, as already explained in section \ref{sec:nonlin}, the number of propagating modes will now be $d(d-1)/2$, plus the corresponding canonical momenta. These are two phase-space degrees of freedom too many for the theory of a massive spin-2 particle. Moreover, the Hamiltonian of a generic theory will not be positive definite~\cite{Boulware:1972zf, Boulware:1973my}, signaling that the extra propagating mode is a ghost.  
The necessary requirement on a consistent interaction potential is therefore the presence of an additional constraint that removes the nonlinear Boulware-Deser ghost.

In order to investigate the posibility for a potential in~(\ref{mggenact}) that gives rise to a constraint, we first decompose the second rank-2 tensor $f_{\mu\nu}$ into its own ADM variables,
\beqn\label{admf}
f_{\mu\nu}=\begin{pmatrix}
-L^2+L_l \tilde{f}^{lk}L_k& L_j\\
L_i & \tilde{f}_{ij}
\end{pmatrix}\,.
\eeqn
Here, $\tilde{f}^{ij}$ denote the inverse of the $(d-1)\times (d-1)$ matrix $\tilde{f}_{ij}$, $L_i$ is the shift, and $L$ is the lapse of~$f_{\mu\nu}$. 
We furthermore express the measure factor $\sqrt{-g}$ in terms of the lapse $N$ and the determinant $\gamma$ of $\gamma_{ij}$,
\beqn\label{measur}
\sqrt{-g}=N \sqrt{\gamma}\,.
\eeqn
With these expressions at hand, we can write a generic interaction potential in terms of ADM variables,
\beqn
\sqrt{-g}~V(g^{-1}f)=N \sqrt{\gamma}~V(\gamma_{ij}, N, N^i; \tilde{f}_{ij}, L, L^i)\,.
\eeqn
In order to provide a constraint, the right-hand side of this equation needs to be linear in the lapse $N$. In fact, the necessary condition on the potential is slightly weaker than that because the constraint may be obtained after combining several of the equations for $N$ and $N^i$. If there exists a combination of these equations that is independent of $N^i$ and $N$, then this equation will constrain the remaining variables. At the level of the action, this means that we should allow for a field-dependent redefinition of the shift, $N^i\rightarrow n^i$, that renders the Lagrangian linear in the lapse $N$. Certainly, such a redefinition must be linear in $N$ itself since $N^i$ appears linearly in the kinetic term. Furthermore, since the redefined shift $n^i$ is expected to appear in the constraint, it must be fully determined by its own equation of motion which therefore must not depend on $N$.  To summarize, we make two requirements on the potential in terms of the redefined shift $n^i$:
\begin{itemize}
\item[(i)] linearity of the Lagrangian in $N$,
\item[(ii)]  absence of $N$ in the $n^i$ equations of motion.
\end{itemize} 
Next, we observe that the interaction potential already has a factor of $N$ in front coming from the measure factor (\ref{measur}). Hence, in order to satisfy requirement (i), the potential $V(g^{-1}f)$ written in ADM variables must be of the form
\beqn
V(g^{-1}f)=\frac{1}{N}V_1+V_2
\eeqn
where $V_1$ and $V_2$ are functions of $(\gamma_{ij}, n^i; \tilde{f}_{ij}, L, L^i)$, i.e.~independent of~$N$. Recalling the ADM decomposition (\ref{admmetr}) of $\gmn$, it is clear that the only object that has the chance of giving something linear in $1/N$ is the square root of the inverse metric~(\ref{invadm}). We are thus lead to consider a potential~$V$ that is a function of the matrix $S\equiv\sqrt{g^{-1}f}$, defined via $S^2=g^{-1}f$. This square-root matrix has a very nontrivial ADM decomposition and is certainly highly nonlinear in $1/N$. However, we will now make use of the allowed redefinition of the shift $N^i$ in order to write $S$ in the form
\beqn\label{sadm}
S=\frac{1}{N}\mA+\mB\,,
\eeqn
where $\mA$ and $\mB$ are matrix-valued functions of $(\gamma_{ij}, n^i; \tilde{f}_{ij}, L, L^i)$. The redefinition that leads to (\ref{sadm}) as well as the explicit expressions for $\mA$ and $\mB$ can be obtained straightforwardly by the following method: Square the right-hand side of the ansatz (\ref{sadm}) and equate it with the ADM expression for $g^{-1}f$ obtained from (\ref{admmetr}) and (\ref{admf}). Then compare the expressions on both sides order by order in $1/N$ to read off the shift redefinition as well as the matrices $\mA$ and $\mB$.
This derivation is discussed in more detail in {\protect{\hyperref[papI]{Paper~I}}}; here we simply state the result. The redefinition that renders the square-root matrix $S$ linear in $1/N$ takes the rather simple form
\beqn\label{shiftred}
N^i=Ln^i+L^i+N{D^i}_kn^k\,.
\eeqn
The $(d-1)\times(d-1)$ matrix $D$ on the right-hand side is a function of the variables $(\gamma_{ij}, n^i; \tilde{f}_{ij})$. Explicitly, it is given by
\beqn
D=\sqrt{\gamma^{-1}\tilde{f}Q}\,Q^{-1}\,,
\eeqn
where we have defined another matrix $Q$ through
\beqn
{Q^i}_j=x{\delta^i}_j+n^in^k\tilde{f}_{kj}\,,\qquad x=1-n^i\tilde{f}_{ij}n^j\,.
\eeqn
The matrices $\mA$ and $\mB$ then turn out to be
\beqn
\mA=\frac{1}{L\sqrt{x}}
\begin{pmatrix}
a_0&a_j\\
-a_0c^i&-c^ia_j
\end{pmatrix}\,,~~\quad~~
\mB=\sqrt{x}
\begin{pmatrix}
0&0\\
{D^i}_jL^j&{D^i}_j
\end{pmatrix}\,,
\eeqn
in which
\beqn\label{defa}
a_0=L+n^kL_k\,,\qquad a_i=n^kf_{ki}\,,\qquad
c^i=Ln^i+L^i\,.
\eeqn
The form of the redefinition is not entirely unique. In {\protect{\hyperref[papI]{Paper~I}}} we mainly work with a set of variables that slightly differs from the one presented here. This difference does not affect any of the conclusions drawn in the following, but the choice of variables we made here is more suitable for application to bimetric theory in the next chapter.  

Although the above expressions seem rather complicated, what is essential for the construction of the ghost-free potential is the structure of the matrices $\mA$ and $\mB$. Most importantly, $\mA$ has rank one, i.e.~it can be written as the outer product of two vectors,
\beqn\label{vwa}
\mA=v w^\mathrm{T}\,,~~\quad~~\text{where}~~v=\begin{pmatrix}1\\-c^i \end{pmatrix}\,~~\text{and}~~~w=\frac{1}{\sqrt{x}}\begin{pmatrix}a_0\\a^i\end{pmatrix}\,.
\eeqn
Having obtained the suitable ADM expression (\ref{sadm}) for the square-root matrix $S=\sqrt{g^{-1}f}$, we are ready to construct the interactions which give rise to an additional constraint that removes the Boulware-Deser ghost.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%         
\subsection{Construction of the interaction potential}\label{sec:conspot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As explained above, the mass potential has to be a function of the square-root matrix $S=\sqrt{g^{-1}f}=\frac{1}{N}\mA+\mB$, multiplied by $\sqrt{-g}=N\sqrt{\gamma}$\,. We assume this function to be expandable as a Taylor series in $S$. Generically, this will give an expression that is nonlinear in the lapse $N$. 
The only way to ensure linearity in $N$ is to demand the absence of higher powers of~$\frac{1}{N}\mA$ in the expansion. Obviously, the simplest possible term is $\sqrt{-g}~\tr~(\frac{1}{N}\mA+\mB)$. At first sight it seems that all higher powers of $\frac{1}{N}\mA+\mB$ will involve higher powers of~$1/N$. However, due to the special structure of the matrix $\mA$ there is a caveat here:
Since $\mA$ has rank one, it is a projection operator on a one-dimensional subspace. Because of that, there is a unique way of building polynomials of $\frac{1}{N}\mA+\mB$ that are linear in $\frac{1}{N}\mA$. Namely, an antisymmetric product of $\mA$'s will automatically contain only one power of~$\mA$. Let us see how this works in detail. In $d$ dimensions we consider
\beqn\label{potantisym}
V(S)=\sum_{k=0}^d ~b_n~\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d}~{S^{\nu_1}}_{\mu_1}\hdots{S^{\nu_n}}_{\mu_n}\,,
\eeqn
with arbitrary coefficients $b_n$.
Since the simultaneous exchange of $\mu_i$, $\mu_j$ and $\nu_i$, $\nu_j$ only changes the sign of both $\epsilon$-tensors, it leaves the whole term invariant.
Therefore, at $n$th order, the product of $S$'s under the sum can be written in the form,
\beqn
\sum_{l=0}^n {n \choose l}\left(\frac{1}{N}\right)^l   {\mA^{\nu_1}}_{\mu_1}\hdots {\mA^{\nu_l}}_{\mu_l}{\mB^{\nu_{l+1}}}_{\mu_{l+1}}\hdots {\mB^{\nu_n}}_{\mu_n}\,.      
\eeqn
We insert this expression into (\ref{potantisym}) and obtain
\beqn
V(S)=\sum_{n=0}^d b_n\sum_{l=0}^n {n \choose l}\left(\frac{1}{N}\right)^l V_n(\mA,\mB)\,,
\eeqn
with
\beqn
V_n(\mA,\mB)&=&\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d} \nn\\
&~&\hspace{50pt}\cdot~{\mA ^{\nu_1}}_{\mu_1}\hdots {\mA ^{\nu_l}}_{\mu_l}{\mB^{\nu_{l+1}}}_{\mu_{l+1}}\hdots {\mB^{\nu_n}}_{\mu_n}  \nonumber\\
&=&\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d}\nn\\
&~&\hspace{50pt} \cdot~{v ^{\nu_1}}w_{\mu_1}\hdots {v ^{\nu_l}}w_{\mu_l}{\mB^{\nu_{l+1}}}_{\mu_{l+1}}\hdots {\mB^{\nu_n}}_{\mu_n}\,.
\eeqn
Here we have used (\ref{vwa}).
Since all indices of the symmetric product of $v^{\nu_i}$ are contracted with the totally antisymmetric indices of $\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d} $, we find that in $V_n(\mA,\mB)$ only terms with at most one $\mA$ contribute. This is precisely the property that we were looking for.  
We conclude that the most general form of the potential that is linear in $N$ after the redefinition (\ref{shiftred}) is
\beqn
\sqrt{-g}\,\sum_{n=0}^d ~b_n~\epsilon^{\mu_1\mu_2\hdots\mu_n\lambda_{n+1}\hdots\lambda_d}\epsilon_{\nu_1\nu_2\hdots\nu_n\lambda_{n+1}\hdots\lambda_d}~{S^{\nu_1}}_{\mu_1}\hdots{S^{\nu_n}}_{\mu_n}\,,
\eeqn
with $S=\sqrt{g^{-1}f}$. A more convenient way of writing this is by introducing the elementary symmetric polynomials of the matrix $S$ that can be defined through a recursion formula,
\beqn
e_n(S)=\frac{(-1)^{n+1}}{n}\sum_{k=0}^{n-1}(-1)^{k}\tr (S^{n-k})e_k(S)\,,\quad \text{with}~~e_0(S)=1\,.
\eeqn
Properties of the elementary symmetric polynomials are summarized in appendix~\ref{app:el}.
In terms of these the potential takes the simple form,
\beqn\label{potsympol}
\sqrt{-g}~V(S)=\sqrt{-g}\,\sum_{n=0}^d ~\beta_ne_n(S)\,,
\eeqn
where we have introduced the rescaled coefficients $\beta_n=\frac{n!(d-n)!}{2}b_n$. Since the elementary symmetric polynomials also appear in the expansion of the determinant, the above potential can be regarded as a \textit{deformed determinant}. Note in particular that there is only a finite number of terms giving a potential which is linear in $N$. Due to the antisymmetric structure of the interactions, the possible terms are limited by the dimension of space time. Moreover, out of the $d$ parameters $\beta_n$, only $(d-2)$ are truely measuring interaction strengths: Since $e_0(S)=1$, the $\beta_0$-term is simply a cosmological constant. Also, the last term in the sum that is proportional to $\beta_d$ is just a cosmological constant term for $\fmn$ because $e_d(S)=\det S$. It is therefore independent of $\gmn$ and does not contribute to the equation of motion. Nonetheless, we choose to include it in the action because it will become relevant when we give dynamics to $\fmn$ in the next chapter.

As we have argued, (\ref{potsympol}) is the most general potential that satisfies the above criterion (i). We now explain why requirement (ii) follows automatically. Namely, we can write the equations of motion for $n^i$ obtained from the nonlinear massive gravity action $S_\mathrm{MG}$ as
\beqn
\frac{\delta S_\mathrm{MG}}{\delta n^i}=\frac{\delta N^j}{\delta n^i}\frac{\delta S_\mathrm{MG}}{\delta N^j}=0\,.
\eeqn
Observe that these equations can depend on $N$ at most linearly because the action is linear in $N$. But since the redefinition (\ref{shiftred}) is already linear in $N$, so is $\frac{\delta N^j}{\delta n^i}$ and consequently $\frac{\delta S_\mathrm{MG}}{\delta N^j}$ is independent of $N$. Furthermore, $\frac{\delta N^j}{\delta n^i}$ is nonzero since it is the Jacobian of the redefinition. The $n^i$ equations of motion are therefore equivalent to $\frac{\delta S_\mathrm{MG}}{\delta N^j}=0$ which is independent of~$N$. Hence, by constructing a potential that meets requirement (i), we automatically satisfy criterion (ii). This has also been shown explicitly in {\protect{\hyperref[papI]{Paper~I}}}. 
 

To summarize, we have derived the nonlinear massive gravity action equipped with an additional constraint that removes the Boulware-Deser ghost,
\beqn\label{HRMG}
S_\mathrm{MG}=\int \mathrm{d}^dx\,\sqrt{-g}\,\left[M_{\mathrm{Pl}}^{d-2}R(g) -2 m^d\sum_{n=0}^d ~\beta_ne_n\left(S\right)\right]\,,
\eeqn
with $S=\sqrt{g^{-1}f}$. Once the structure of the theory was known, it was also possible to derive the constraint in a purely covariant formulation for some simplifying parameter choices~\cite{Deffayet:2012nr}. 
In the literature, the above action has been widely referred to as the dRGT model. However, it should be stressed that the theory derived by de Rham, Gabadadze and Tolley in \cite{deRham:2010ik, deRham:2010kj} was defined with flat reference metric $\fmn=\emn$ only. The dRGT construction uses St\"uckelberg fields (see section~\ref{sec:stuck}) and is valid only in a certain decoupling limit that strongly relies on the flat reference metric. In contrast, the construction we have presented here is valid for all reference metrics and demonstrates the consistency of the fully nonlinear theory away from any limiting approximation.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The secondary constraint}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The above requirements on the consistent interaction potential were necessary but not sufficient: A secondary constraint is crucial for the absence of the Boulware-Deser ghost because two constraints are needed to remove both the ghost mode and its canonical momentum from the set of dynamical variables.

It was motivated in Paper I that there is in fact a secondary constraint arising from demanding the primary constraint to be constant in time.  In order to compute the time evolution of the constraint one uses the Poisson bracket (\ref{defpoisb}) and the Hamiltonian, which for the above Massive Gravity action is of the form
 \beqn\label{hamsecc}
H=\int \mathrm{d}^{d-1} y~(\mathcal{H}_0-N\mathcal{C})\,.
\eeqn
Here $\mathcal{H}_0$ is independent of $N$ and $\mathcal{C}$ is the Hamiltonian constraint obtained from varying the action with respect to $N$. The time evolution of $\mathcal{C}$ then reads
\beqn\label{seccons}
\frac{\mathrm{d}\mathcal{C}(x)}{\mathrm{d}t}=\{\mathcal{C}(x),H\}=0\,.
\eeqn  
As in the case of the primary constraint, this equation should be independent of $N$, because otherwise it would determine $N$ instead of constraining $\gamma_{ij}$ and $\pi^{ij}$. Inserting~(\ref{seccons}) into~(\ref{hamsecc}) gives
\beqn
\int \mathrm{d}^{d-1} x~\Big(\{\mathcal{C}(x),\mathcal{H}_0(y)\}-N\{\mathcal{C}(x),\mathcal{C}(y)\}\Big)=0\,.
\eeqn  
Since $\mathcal{C}$ and $\mathcal{H}_0$ are independent of $N$, we therefore need the Poisson bracket among the constraints $\{\mathcal{C}(x),\mathcal{C}(y)\}$ to vanish because the secondary constraint cannot depend on $N$. Before this was actually demonstrated to be the case, there had been objections against the theory claiming that $\{\mathcal{C}(x),\mathcal{C}(y)\}$ could be nonzero \cite{Kluson:2011qe}. The issue was resolved when the secondary constraint was eventually shown to exist in a detailed calculation in~\cite{Hassan:2011ea}. With this, the consistency of the nonlinear Massive Gravity action (\ref{HRMG}) was fully proven.




 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%        
\section{Consistency in the St\"uckelberg formulation}\label{sec:stuck}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As stated earlier, the invariance under general coordinate transformations of General Relativity is broken by the mass term for the graviton. This is because the metric $\gmn$ itself transforms as a covariant rank-two tensor under GCTs while the fixed background metric $\fmn$ does not. Therefore objects like $g^{\mu\nu}\fmn$ are not diffeomorphism invariant. However, there exist a method to restore the gauge symmetry in the action: By introducing new gauge degrees of freedom, so-called St\"uckelberg fields, that transform in a certain way under the gauge group, one can rewrite the theory in a manifestly gauge invariant way. In turn, fixing the so-called physical gauge will give back the original action.

While the proof of absence of the Boulware-Deser ghost given in {\protect{\hyperref[papI]{Paper~I}}} was formulated in the gauge-fixed version of massive gravity, i.e.~without introducing the St\"uckelberg fields, it is expected that restoring the gauge invariance does not alter the dynamics of the theory. In fact, since gauge symmetry is merely a redundancy in the description of the underlying physics, the two formulations are completely equivalent. In particular, absence of ghost in the gauge fixed version of Massive Gravity implies that the St\"uckelberg formulation cannot exhibit the instability either.

Nevertheless, before the constraint needed to remove the ghost was computed explicitly in the St\"uckelberg formulation, there had been some confusion regarding this issue. Namely, in \cite{Chamseddine:2011mu, Kluson:2011rt, Kluson:2012gz}, it was claimed that the Boulware-Deser ghost seems to reappear in the gauge invariant theory. If this was true, it would have suggested a flaw in the consistency proof of gauge fixed Massive Gravity. Fortunately, we were eventually able to prove the absence of ghost in the St\"uckelberg formulation in {\protect{\hyperref[papIII]{Paper~III}}}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The St\"uckelberg trick}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
One possibility to reintroduce diffeomorphism invariance in Massive Gravity is to perform a gauge transformation on the dynamical metric~$\gmn$ and treat the gauge parameters as new fields in the action. Under a GCT, $x^\alpha\rightarrow x'^\alpha(x)$, the metric transforms as
\beqn
\gmn(x)\rightarrow\frac{\partial x'^\alpha}{\partial x^\mu}\frac{\partial x'^\beta}{\partial x^\nu}g_{\alpha\beta}(\phi)\,.
\eeqn
After performing this GCT, one interprets the $x'^\alpha$ as dynamical fields. Another equivalent way, that will be more convenient for our purposes, is to mimic this kind of transformation on the reference metric $\fmn$, which, of course, actually does not transform under GCTs.  But since a simultaneous coordinate transformation of $\gmn$ and $\fmn$ would be a symmetry of the Massive Gravity action, instead of transforming $\gmn$ we can choose to perform the transformation on $\fmn$. 
That is to say, we replace $\fmn$ by its covariantized form
\beqn\label{etcov}
\fmn\rightarrow\frac{\partial \varphi^\alpha}{\partial x^\mu}\frac{\partial \varphi^\beta}{\partial x^\nu}\bar{f}_{\alpha\beta}\,.
\eeqn
Here, $\bar{f}_{\alpha\beta}$ is a new fixed background metric that does not transform under the gauge group. The ``coordinates'' $\varphi^\alpha$ are promoted to dynamical fields that transform as scalars under GCTs. Introducing these St\"uckelberg fields ensures that objects such as
\beqn
 \Tr\, (g^{-1}f) =g^{\mu\nu}\frac{\partial \varphi^\alpha}{\partial x^\mu}\frac{\partial \varphi^\beta}{\partial x^\nu}\bar{f}_{\alpha\beta}
 \eeqn
are diffeomorphism invariant. In addition to the equations of motion for the metric $\gmn$, we now also consider the $\varphi^\alpha$ equations and, as we will see below, this system of equations is equivalent to the original $\gmn$ equation without St\"uckelberg fields.
 
Let us expand the St\"uckelberg fields around the identity transformation, which corresponds to considering infinitesimal GCTs,
\beqn
\varphi^\alpha=x^\alpha-\pi^\alpha\,.
\eeqn 
Furthermore, we decompose the perturbations into a transverse and a longitudinal mode,
\beqn\label{decpi}
\pi^\alpha=\hat{\pi}^\alpha+\partial^\alpha\pi\,.
\eeqn
The power of the St\"uckelberg formalism lies in the conjecture that the ghost instability of nonlinear Massive Gravity can be traced back to higher derivative interactions of the $\pi$ fields in flat space, where $\bar{f}_{\alpha\beta}=\eta_{\alpha\beta}$ \cite{ArkaniHamed:2002sp}. This assumption relies on an analogy to the Goldstone equivalence theorem for spin-1 fields \cite{Lee:1977yc, Chanowitz:1985hj}. In that case, the longitudinal modes of the gauge fields have been shown to carry all information needed for computing scattering processes at high energies. Although the theorem has not been proven for the spin-2 case, it is reasonable to start with the assumption of its validity in order to investigate the stability of Massive Gravity in a certain high energy limit. This limit (also referred to as \textit{decoupling limit}) essentially corresponds to setting the metric perturbation to zero and also ignoring all terms involving the transverse components of the St\"uckelberg fields. Then the conjecture of \cite{ArkaniHamed:2002sp} suggests to construct the interaction potential in such a way that there appear no higher-order interactions of the longitudinal modes. Since each of these modes always comes with two derivatives, their interactions generically give rise to higher derivative terms. These can be shown to lead to ghosts and must therefore be avoided in a consistent theory.
The conclusion of an exhaustive analysis in \cite{Creminelli:2005qk} was that avoiding the higher derivative terms was impossible, and once more it seemed that there exists no consistent nonlinear theory for Massive Gravity. However, it turned out that the authors of~\cite{Creminelli:2005qk} had made sign mistake, and after correcting that flaw, de Rham, Gabadadze and Tolley were indeed able to construct a theory without higher-derivative interactions of the $\pi$ fields. The trick they employed was to tune the coefficients of the interaction terms in such a way that the higher derivative terms combined into total derivatives that could be dropped from the action. 
This lead to the nonlinear Massive Gravity action (\ref{HRMG}) with flat $\fmn$ (and limited parameter space since one of the $\beta_n$ was fixed to ensure a flat background solution for $\gmn$). The complete expression for its decoupling limit, including the transverse vector modes in~(\ref{decpi}), was worked out in~\cite{Ondo:2013wka}.
 
Being free of ghost instabilities in the decoupling limit, the dRGT model is definitely a promising candidate for a consistent theory of nonlinear Massive Gravity in flat space. However, consistency of the theory in all its interactions, that is, away from the decoupling limit, is difficult to prove in the St\"uckelberg formulation, in particular for general $\beta_n$ parameters. The main complication arises due to the square-root matrices appearing in the potential. However, as we explain in the following, it is easy to see that the ghost proof of the gauge fixed theory carries over to the gauge invariant mass potential.
Thereafter, in order to support our arguments even further, we demonstrate the consistency of Massive Gravity in the St\"uckelberg formulation explicitly by identifying the constraint that removes the ghost.  



        
                

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{General arguments for consistency}\label{secgenargst}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
The fact that the dynamics remain unaltered in the gauge invariant theory can be demonstrated by considering the equations of motions for the St\"uckelberg fields. After making the replacement (\ref{etcov}) for $f_{\mu\nu}$, the mass potential $V(g,f)$  becomes a function of the scalar fields and their equations of motions read
\beqn\label{varphieoms}
\frac{\delta}{\delta\varphi^A} V(g,\varphi^B)=0\,.
\eeqn
However, this equation will not give rise to any new dynamics because it is, in fact, already implied by the Bianchi constraint of the gauge fixed theory,
\beqn
&~&\nabla^\mu V_{\mu\nu}(g,\varphi^B)=0\,,\nn\\
&~& \text{where}~~~V_{\mu\nu}(g,\varphi^B)\equiv\frac{1}{\sqrt{-g}}\frac{\delta}{\delta g^{\mu\nu}}\left(\sqrt{-g}~ V(g,\varphi^B)\right)\,.
\eeqn
This constraint follows from the divergence of the $\gmn$ equations after using the Bianchi identity $\nabla^\mu G_{\mu\nu}=0$.
In order to see the equivalence, consider a gauge transformation $\delta x^\mu=\xi^\mu$ of the action involving St\"uckelberg fields,
\begin{align}
&\delta S=\int\mathrm{d}^dx\sqrt{-g}\left[\left(\mpl^{d-2} G_{\mu\nu}
-2m^dV_{\mu\nu}\right)\delta g^{\mu\nu}
-2m^d\frac{\delta V}{\delta\varphi^A}\delta\varphi^A\right]\,.
\end{align}
Here $G_{\mu\nu}$ is the Einstein tensor and the variations under the gauge transformation read $\delta g^{\mu\nu}=-2\nabla^{(\mu} \xi^{\nu)}$ and $\delta\varphi^A=-\xi^\mu\partial_\mu\varphi^A$. As the action is invariant under GCTs, integrating by parts and using the Bianchi identity shows that
\beqn\label{coordconst}
\nabla^\mu V_{\mu\nu} = \frac{\delta V}{\delta\varphi^A}\partial_\nu\varphi^A\,,
\eeqn
identically.
Since the St\"uckelberg fields were introduced to mimic nonsingular coordinate transformations, the matrix $\partial_\nu\varphi^A$ is invertible and hence the Bianchi constraint $\nabla^\mu V_{\mu\nu}=0$ is equivalent to the $\varphi^A$ equations of motion~(\ref{varphieoms}). As expected, the redundant gauge degrees of freedom $\varphi^A$ therefore do not introduce new dynamics into the theory.

From these general arguments we thus expect the consistency proof of Paper~I to be valid for both the gauge fixed and the gauge invariant version of Massive Gravity.
Nonetheless there had been some work arguing against the consistency of the action involving St\"uckelberg fields: In \cite{Chamseddine:2011mu} it was claimed that the ghost generically reappears in the St\"uckelberg sector and the author of \cite{Kluson:2011rt, Kluson:2012gz} could not find a constraint to remove the ghost. Although this constraint was shown to be present in a two-dimensional toy model and to fourth order in perturbation theory in four dimensions \cite{deRham:2011rn}, the issue remained unresolved until we performed the full Hamiltonian analysis in Paper~II. The following section summarizes our findings.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%       
\subsection{Hamiltonian analysis}\label{hamstuck}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

For the sake of simplicity, in {\protect{\hyperref[papIII]{Paper~III}}} we restrict the constraint analysis of Massive Gravity with St\"uckelberg fields to an interaction potential with only $\beta_1\neq 0$. The analysis for general $\beta_n$ is much more involved and has not been carried out yet. Also, here we focus on $d=4$ although the results straightforwardly generalize to arbitrary number of space-time dimensions. 

The reason why the so-called \textit{minimal model} with only $\beta_1\neq 0$ is simpler, is that, as has been noticed in \cite{Golovnev:2011aa, Buchbinder:2012wb}, in this case the action involving St\"uckelberg fields is equivalent to
\beqn\label{phistuckact}
S_\Phi=M_\mathrm{g}^2\int \md^4 x\sqrt{-g}\left(R-m^4\left[{\Phi^A}_A+{(\Phi^{-1})^A}_B {{\bf A}^B}_A\right]\right)\,,
\eeqn
where ${{\bf A}^B}_A\equiv g^{\mu\nu}\partial_\mu\varphi^B\partial_\nu\varphi^C\bar{f}_{CA}$ and ${\Phi^A}_B$ is an auxiliary field that has been introduced in order to remove the square root. Integrating out ${\Phi^A}_B$ gives back the original action involving $\sqrt{g^{-1}f}$ with $\beta_1=1$. This formulation of the minimal model greatly simplifies the ADM analysis. 
In the following, we raise and lower indices on the St\"uckelberg fields as well as on the auxiliary field with the background metric $\bar{f}_{AB}$.

Using the ADM variables (\ref{admmetr}) for the metric $\gmn$ and computing the canonical momenta $p_A$ conjugate to the St\"uckelberg fields $\varphi^A$, we obtain the Hamiltonian corresponding to (\ref{phistuckact}),
\beqn
\mathcal{H}=-NR_0-N^iR_i+N\mathcal{H}_T^\mathrm{sc}+N^i\mathcal{H}^\mathrm{sc}_i\,,
\eeqn
in which the first two pieces are the familiar ones coming from the Einstein-Hilbert term and where
\beqn
\mathcal{H}_T^\mathrm{sc}&=&\sqrt{\gamma}M_\mathrm{P}^2m^2\big({\Phi^A}_A+{(\Phi^{-1})^A}_B{V^B}_A\big)+\frac{1}{4m^2M_\mathrm{P}^2\sqrt{\gamma}}\Phi^{AB}p_Ap_B\,, \nonumber\\
\mathcal{H}^\mathrm{sc}_i&=& p_A\partial_i\varphi^A\,.
\eeqn
Here we have also defined 
\beqn\label{defvab}
{V^B}_A\equiv \gamma^{ij}\partial_i\varphi^B\partial_j\varphi^C\bar{f}_{CA}\,.
\eeqn
Note that in this formulation involving the auxiliary field ${\Phi^A}_B$ the Hamiltonian is manifestly linear in $N$ and $N^i$. There is no need for a field redefinition in order to demonstrate the linearity in the lapse. The linearity in $N^i$ is of course due to the fact that we have reintroduced the gauge invariance and now, as in General Relativity, expect to encounter four first class constraints. They can be thought of as removing the St\"uckelberg fields from the set of dynamical variables. Gauge fixing then serves to also remove their canonical momenta. However, the Hamiltonian constraint that is needed to remove the Boulware-Deser ghost mode within the metric $\gamma_{ij}$ is not among the gauge constraints but has to arise separately. Hence, as in the gauge fixed case, a generic theory would be inconsistent and an extra constraint is present only for special choices of the potential. 

The important observation that was missed in \cite{Kluson:2011rt, Kluson:2012gz} is now that, besides the constraints imposed by the equations of motion for $N$ and $N^i$, the 10 equations of motion for the symmetric field $\Phi^{AB}$ actually only determine 9 independent combinations of the $\Phi^{AB}$. One equation is independent of $\Phi^{AB}$ and therefore constrains the remaining variables. The reason for this is the singularity of the matrix ${V^B}_A$ defined in (\ref{defvab}). The equations of motion obtained from varying (\ref{phistuckact}) with respect to $\Phi^{AB}$ read
\beqn\label{capphieom}
%\Psi_{AB}\equiv
\sqrt{\gamma}\,M_\mathrm{P}^2m^2\Big(\bar{f}_{AB}-
(\Phi^{-1})_{AC}V^{CD}(\Phi^{-1})_{DB}\Big)&~&
\nn\\ 
+~\frac{1}{4m^2M_\mathrm{P}^2\sqrt{\gamma}}\,p_A\,p_B&=&0\,.
\eeqn
Being composed of two $3\times 4$ matrices and a $3\times 3$ matrix, ${V^B}_A$ can at most have rank three. The same is true for the combination of matrices $(\Phi^{-1})_{AC}V^{CD}(\Phi^{-1})_{DB}$ that appears in (\ref{capphieom}). A generic $4\times 4$ symmetric matrix of rank-three has only nine independent components and therefore the ten equations of motion for $\Phi^{AB}$ determine only nine independent combinations of $\Phi^{AB}$. The tenth equation serves to constrain the remaining variables.

Moreover, it is straightforward to extract the constraint from~(\ref{capphieom}) by taking the determinant of the equation. Since the determinant of a matrix that does not have full rank is zero, we obtain the following constraint equation,
\beqn\label{cconstrainteq}
\mathcal{C}\equiv\det{\bar{f}}\left(\bar{f}_{AB}\frac{p^Ap^B}{\gamma}+4(m^2M_\mathrm{P}^2)^2\right)\approx 0\,.
\eeqn
This extra constraint is not first class, it does not arise from the presence of a gauge symmetry. Just as in the gauge fixed version of the theory, it is therefore necessary to show the existence of a secondary constraint generated by the time evolution of (\ref{cconstrainteq}). This second constraint is needed to remove the canonical momentum of the ghost. From the general arguments given in section \ref{secgenargst} we know that the secondary constraint has to be there, and it can be found explicitly in a straightforward way. The time evolution of the primary constraint (\ref{cconstrainteq}) is given by the Poisson bracket $\{\mathcal{C}(x),H_\mathrm{tot}\}$, in which the total Hamiltonian reads
\beqn\label{htot2}
H_\mathrm{tot}=\int \mathrm{d}^3 x \left[N(\mathcal{H}_T^\mathrm{sc}-R_0+{\Gamma^A}_{B}{\Psi^B}_A)+N^i(\mathcal{H}^\mathrm{sc}_i-R_i)\right]\,.
\eeqn
In this we have included 10 Lagrange multipliers ${\Gamma^A}_{B}$ that enforce the ${\Phi^A}_B$ equations of motion. In fact, we really need to include only the constraint (\ref{cconstrainteq}), i.e.~add a term $\lambda \mathcal{C}$ with one Lagrange multiplier $\lambda$. The two approaches are equivalent and their connection is discussed in {\protect{\hyperref[papIII]{Paper~III}}}. Here we only give the arguments for the absence of the ghost and its momentum. 

The crucial point that still needs to be proven is that the secondary constraint $\mathcal{C}_2=\{\mathcal{C},H_\mathrm{tot}\}\approx 0$ must be independent of $N$ and $N^i$, or otherwise it would determine the classical value for these fields instead of constraining the canonical momentum of the ghost mode. Fortunately, it is quite straightforward to show that the pieces in $\mathcal{C}_2$ that involve $N^i$ cancel out on-shell. Moreover, all remaining terms in $\mathcal{C}_2$ are proportional to $N$ which can therefore be divided out. Hence the secondary constraint is indeed independent of the lapse and shift. Furthermore, all dependence on the Lagrange multipliers ${\Gamma^A}_{B}$ drops out upon use of the ${\Phi^A}_B$ equations of motion. Plugging in the solutions\footnote{In fact, we never derive these solutions explicitly. All that is needed for the proof are some general relations from linear algebra.} to the ${\Phi^A}_B$ equations therefore leaves us with a constraint on the remaining variables that will remove the ghost momentum,
\beqn
\mathcal{C}_2\approx-2\alpha\gamma^{-{1/2}}\bar{f}{(\Phi^{-1})^B}_{D}\partial_j\varphi^D\gamma^{jk}\nabla^{(f)}_kp_B-\alpha^2  \gamma^{-1/2}\bar{f} \pi\,.
\eeqn
Here, we have defined $\nabla^{(f)}_kp_B=\partial_kp_B-\Gamma^D_{AB}p_D\partial_k\varphi^A$, with $\Gamma^D_{AB}$ being the Levi-Civita connection of the metric~$\bar{f}_{AB}$.

Of course, this proof is valid only for the special parameter choice $\beta_1\neq 0$ and all other~$\beta_n$ equal to zero. But from the general arguments given in section \ref{secgenargst} it should be clear that, although it may be harder to find, a constraint is also present in the St\"uckelberg formulation of the full theory. This proves that nonlinear Massive Gravity is ghost-free both in its gauge-fixed and gauge invariant version.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Consistent Bimetric Theory}
\label{ch:HR}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the previous chapter we dealt with the nonlinear theory for a massive spin-2 field~$\gmn$, embedded in some arbitrary but fixed reference frame, set by a second rank-two tensor $f_{\mu\nu}$. The important question that we are about to address now is whether this reference metric can be given dynamics on its own without reintroducing instabilities. From a field-theoretical point of view this would result in a much more natural setup: All fields in the action would be determined dynamically without the need of fixing any of their values by hand. A priori, since the constraint analysis of {\protect{\hyperref[papI]{Paper~I}}} assumed a fixed reference frame, it is not clear whether the Massive Gravity action with dynamical $\fmn$ will still avoid the Boulware-Deser ghost instability. Certainly, the consistency of the theory with two dynamical metrics will depend on the kinetic structure assumed for the second rank-2 tensor. 

The ADM variables introduced above for the constraint analysis of nonlinear Massive Gravity enabled Hassan and Rosen to demonstrate the possibility of promoting $\fmn$ to a dynamical field by simply adding its own Einstein-Hilbert term to the Massive Gravity action~\cite{Hassan:2011zd}. The resulting theory contains two interacting spin-2 fields, one massive and one massless one, as expected from general arguments \cite{Boulanger:2000rq}. Such theories had been under consideration for a long time (see e.g.~\cite{Rosen:1940zz}, \cite{Isham:1971gm}, \cite{Damour:2002wu}), but never with the correct consistent interaction potential (except for very few accidental exceptions~\cite{Chamseddine:1978yu, Nibbelink:2006sz}). It required the discovery of ghost-free Massive Gravity to find the unique consistent bimetric theory. 


%In recent years, bimetric theories were mainly considered in relation to the dark matter problem \cite{Banados:2008fi, Milgrom:2009gv} and in the context of spontaneous Lorentz symmetry breaking \cite{Berezhiani:2007zf, Blas:2009my}. 
%Furthermore, the consistency of effective Lagrangians for interacting spin-2 fields, that could arise in brane models or string theory, has been investigated in~\cite{PhysRevD.40.1095, Buchbinder:1999be, Buchbinder:1999ar, Damour:2002ws}.









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Hassan-Rosen action}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   

The Hassan-Rosen action for bimetric gravity consists of two Einstein-Hilbert terms for $\gmn$ and $\fmn$ as well as non-derivative interactions between the two tensor fields. The interaction potential is given by (\ref{potsympol}), i.e.~it has exactly the same form as in nonlinear Massive Gravity.
Hence the bimetric action reads
\begin{align}\label{HR}
S_\mathrm{HR}~=~m_g^{d-2}\int \mathrm{d}^dx\,\sqrt{-g}&\,R(g)~+~m_f^{d-2}\int \mathrm{d}^dx\,\sqrt{-f}\,R(f) \nn\\
&-~2 m^d\sum_{n=0}^d ~\beta_ne_n(S)\,.
\end{align}  
Here we used again the definition of the matrix square root, $S=\sqrt{g^{-1}f}$. Moreover, $m_g$,$m_f$ denote the Planck masses for $\gmn$ and $\fmn$, respectively.

Na\"ively, there seems to be a straightforward argument why this action cannot be consistent: Suppose we go backwards and freeze one of the two metrics to rearrive at a theory for one spin-two field $\gmn$ in a fixed background. For example, we could set $f_{\mu\nu}=\emn$ which gives back the dRGT action that is known to be consistent. Contrarily, freezing $\gmn$ leads to an action for $f_{\mu\nu}$ whose interaction potential does not seem to resemble the form that is known to be the only consistent one. One could be lead to conclude that bimetric theory therefore has to be inconsistent. However, it turns out that the elementary symmetric polynomials possess a rather unexpected property,
\beqn\label{symprop}
e_n(S)=e_{d-n}(S^{-1})\cdot\det S\qquad \text{for}\quad n=0,\hdots, d\,.
\eeqn
Owing to these identities, Hassan-Rosen bimetric gravity is invariant under the following discrete symmetry,
\beqn\label{symbg}
\gmn \longleftrightarrow \fmn\,,\quad m_g \longleftrightarrow m_f\,,\quad \beta_n\longrightarrow\beta_{d-n}\,. 
\eeqn
This interchange symmetry guarantees that freezing $\gmn$ also gives back the consistent Massive Gravity theory for $f_{\mu\nu}$. Of course, this observation does not automatically prove that the theory with both $\gmn$ and $f_{\mu\nu}$ taken to be dynamical is consistent. It merely shows that one necessary condition on a consistent bimetric theory is indeed satisfied. The actual consistency can only be proven in an ADM analysis, which has been performed in \cite{Hassan:2011zd}. Since now both metrics are dynamical, there are two potential Boulware-Deser ghosts within the theory, the usual one coming from $g_{\mu\nu}$ and another one coming from $f_{\mu\nu}$. One therefore has to show that the action is linear in both of the lapses~$N$ and~$L$. Furthermore, in contrast to the action for massive gravity, the bimetric action (\ref{HR}) has a gauge symmetry: It is invariant under diffeomorphisms, under which~$\gmn$ and~$\fmn$ transform simultaneously. 
It is therefore expected that the bimetric action, if consistent, should describe the $(d(d-2)-1)$ degrees of freedom of a massive and a massless spin-2 field.

Indeed, in \cite{Hassan:2011zd} it has been shown that the action (\ref{HR}) becomes linear in both of the lapses $N$ and $L$. It further turns out that the action becomes also linear in $L^i$. As in general relativity, the shift vectors of $\fmn$ now give rise to three further constraints. In addition to this, the presence of a secondary constraint for the Hamiltonian constraint has been demonstrated in \cite{Hassan:2011ea}. Both of the Boulware-Deser ghosts are therefore absent and the number of degrees of freedom is $(d(d-2)-1)$, the correct number for a massive and a massless spin-2 field. In section~\ref{sec:massspec}, we will see that at the linear level these mass eigenstates are neither the fluctuations of $\gmn$ nor those of $\fmn$ but a superposition of the two. Before we turn to the mass spectrum, however, we need to address the question of how the metrics should couple to matter.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsubsection{Including matter sources}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

So far, the bimetric action in the form (\ref{HR}) does not take into account couplings of $\gmn$ and $\fmn$ to other fields. For phenomenological purposes the nature of the matter couplings is of great importance. The only presently known couplings that can be added to (\ref{HR}) without reintroducing the ghost instabilities are the standard minimal couplings familiar from general relativity,
\beqn\label{matcoup}
S_\mathrm{m}=\int\dd^dx~\sqrt{-g}\,\mathcal{L}^g_m+\int\dd^dx~\sqrt{-f}\,\mathcal{L}^f_m\,.
\eeqn
Here, $\mathcal{L}^g_m$ and $\mathcal{L}^f_m$ are Lagrangians involving matter fields as well as the respective metrics.
The variations of $S_\mathrm{m}$ define the two stress-energy tensors,
\beqn\label{strente}
T^{g}_{\mu\nu}\equiv-\frac{1}{\sqrt{-g}}\frac{\delta S_\mathrm{m}}{\delta g^{\mu\nu}}\,,\qquad 
T^{f}_{\mu\nu}\equiv-\frac{1}{\sqrt{-f}}\frac{\delta S_\mathrm{m}}{\delta f^{\mu\nu}}\,.
\eeqn
We shall not discuss the phenomenological implications of a second metric coupled to matter. In {\protect{\hyperref[papII]{Paper II}}}, where we derive homogeneous and isotropic solutions to the bimetric equations of motion, we set the matter coupling of $\fmn$ to zero. This is always a consistent choice and results in a theory for a spin-2 field that only couples to matter indirectly through gravity. For recent work dealing with both of the couplings, see~\cite{Akrami:2013ffa}.

   
    
    
    
    
 
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\section{Equations of motion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
    
We now turn to the equations of motions for $\gmn$ and $\fmn$, obtained from the Hassan-Rosen action (\ref{HR}) including the matter couplings (\ref{matcoup}). When computing these, the only complication arises from variation of the square-root matrix $S=\sqrt{g^{-1}f}$. However, since this matrix only appears under the trace, one can make use of $\delta (S^2)=(\delta S)S+S(\delta S)$ to obtain $\delta(\Tr\,S)=\Tr(\delta S)=\tfrac{1}{2}\Tr(S^{-1}\delta (S^2))$, and similarly for higher powers of $S$ under the trace~\cite{Hassan:2011vm}. Then it is easy to derive the equations of motion, wich in terms of the Einstein tensor $\mathcal{G}_{\mu\nu}(g)\equiv R_{\mu\nu}(g)-\frac{1}{2}\gmn R(g)$ read
\beqn
\mathcal{G}_{\mu\nu}(g) + \frac{m^d}{m_g^{d-2}}V^g_{\mu\nu}(g,f)&=&\frac{1}{m_g^{d-2}}T^g_{\mu\nu}\,,\label{geq} \\
\mathcal{G}_{\mu\nu}(f)+\frac{m^d}{m_f^{d-2}}V^f_{\mu\nu}(g,f)&=&\frac{1}{m_f^{d-2}}T^f_{\mu\nu}\,.\label{feq}
\eeqn
The contributions coming from the bimetric interaction potential are of the following form,
\beqn\label{poteom}
V^g_{\mu\nu}(g,f)&\equiv& \sum_{n=0}^{d-1}(-1)^n\beta_n \,g_{\mu\lambda}{\big(Y^{(n)}\big)^\lambda}_{\nu}(S)\,,\nn\\
V^f_{\mu\nu}(g,f)&\equiv&\sum_{n=0}^{d-1}(-1)^n\beta_{d-n} \,f_{\mu\lambda}{\big(Y^{(n)}\big)^\lambda}_{\nu}(S^{-1})\,,
\eeqn
in which the matrix functions ${(Y^{(n)})^\lambda}_{\nu}$ are defined in terms of the elementary symmetric polynomials through
\beqn\label{defY}
{\big(Y^{(n)}\big)^\lambda}_{\nu}(S)=\sum_{k=0}^n(-1)^ke_k(S){(S^{n-k})^\lambda}_{\nu}\,.
\eeqn
An immediate consequence of the interchange symmetry (\ref{symbg}) in the bimetric action, which of course carries over to the equations of motion, is the identity $V^f_{\mu\nu}(g,f; \beta_{d-n})=V^g_{\mu\nu}(f,g, ; \beta_{n})$.

Note that in nonlinear Massive Gravity with fixed reference metric $\fmn$, there is only one equation of motion for $\gmn$, given by (\ref{geq}).
In contrast, bimetric gravity has two sets of equations of motion and is therefore much more constrained. Moreover, the $\beta_4$-term enters the $\fmn$ equation and is thus no longer nondynamical but rather appears as a cosmological constant term in the equation for $\fmn$. We will have to say more about the important differences between the two theories in section~(\ref{sec:MGlim}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bianchi constraints}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $\nabla$ and $\tilde{\nabla}$ denote the covariant derivatives compatible with the metrics $\gmn$ and $\fmn$, respectively. In General Relativity without interaction term, covariant conservation of the stress-energy tensor, $\nabla^\mu T^{g}_{\mu\nu}=0$, is a consequence of the equations of motion because the Einstein tensor satisfies the Bianchi identity $\nabla^\mu \mathcal{G}_{\mu\nu}=0$. In other words, a massless spin-2 field can only couple to conserved matter sources. In bimetric gravity the condition is weaker: Invariance of the interaction potential under simultaneous diffeomorphisms of $\gmn$ and $\fmn$ implies 
\beqn\label{bicog}
\sqrt{-g}\,\nabla^\mu V^g_{\mu\nu}+\sqrt{-f}\,\tilde{\nabla}^\mu V^f_{\mu\nu}=0\,.
\eeqn
The constraint on the sources enforced by the equations of motion then reads
\beqn
\sqrt{-g}\,\nabla^\mu T^{g}_{\mu\nu}+\sqrt{-f}\,\tilde{\nabla}^\mu T^{f}_{\mu\nu}=0,
\eeqn
meaning that in bimetric gravity the two source contributions are not forced to be separately conserved by the equations. 
Nevertheless, we shall always assume their separate conservation, that is $\nabla^\mu T^{g}_{\mu\nu}=\tilde{\nabla}^\mu T^{f}_{\mu\nu}=0$. This is equivalent to imposing the separate invariance of the two matter Lagrangians $\mathcal{L}^g_\mathrm{m}$ and $\mathcal{L}^f_\mathrm{m}$ under diffeomorphisms, which appears to be a natural requirement.
In this case, the equations of motion for $\gmn$ then give rise to $d$ Bianchi constraints,
\beqn\label{Bianchi}
\nabla^\mu \sum_{n=0}^{d-1}(-1)^n\beta_n \,g_{\mu\lambda}{(Y^{(n)})^\lambda}_{\nu}(S)&=&0\,.
\eeqn 
Accordingly, there is a set of similar constraints arising from the $\fmn$ equation which, as a consequence of the identity (\ref{bicog}), is equivalent to (\ref{Bianchi}). In summary, under the assumption of separate covariant conservation of the stress-energy tensors, the equations of motion contain $d$ constraints~(\ref{Bianchi}) following from diffeomorphism invariance.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Massive Gravity limit}\label{sec:MGlim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

An intriguing question is whether there exist a limit in the Hassan-Rosen theory in which one of the metrics decouples and the remaining metric describes a massive excitation. It turns out that this is indeed possible, but as always the exact limit needs to be treated with care. Massive Gravity limits of bimetric gravity have been studied in~\cite{Baccetti:2012bk}, where it was shown that only one of two possible limiting procedures leads to a nontrivial theory.

Consider again the nonlinear equations of motion (\ref{geq}) and (\ref{feq}) for $\gmn$ and $\fmn$, respectively. In these we now take the following limit,
\beqn\label{mglimit}
\frac{m_f}{M}\rightarrow \infty\,,\qquad \beta_d\rightarrow \infty\,,\qquad \text{such~that}\quad \frac{\beta_dM}{m_f}=\text{const.}
\eeqn
Here, $M$ denotes any other mass scale in the theory, such as $m_g$, $m$ and the energy scale of the sources. Provided that the $\beta_n$ parameters are independent of $m_f/M$, then the equations of motion in this limit reduce to
\begin{align}
\mathcal{G}_{\mu\nu}(g)
+\tfrac{m^d}{m_g^{d-2}}\sum_{n=0}^{d-1}(-1)^n\beta_n \,g_{\mu\lambda}{(Y^{(n)})^\lambda}_{\nu}(S)=\tfrac{1}{m_g^{d-2}}T^{g}_{\mu\nu}\,, \label{gdrgt} \\
\mathcal{G}_{\mu\nu}(f)
+\Lambda\fmn=0 \,,\label{fdrgt}
\end{align}
where $\Lambda\equiv{\beta_d\,m^d}/{m_f^{d-2}}$. The equation for $\gmn$ is unaltered, while the equation for $\fmn$ decouples and simply becomes an ordinary Einstein equation with cosmological constant $\Lambda$. Hence, the solution for $\fmn$ will be an Einstein metric which can be plugged into the $\gmn$ equation. The resulting equation for $\gmn$ is exactly the same as in the nonlinear Massive Gravity where the auxiliary metric $\fmn$ is fixed to be an Einstein metric. Note, however, that it is not possible to derive the equations (\ref{gdrgt}) and (\ref{gdrgt}) from an action principle. 
One may therefore think that a more natural limit would be given by $m_f/M\rightarrow 0$ which could directly be taken in the bimetric action. However, it is quite easy to see that in this limit the equations of motion admit only GR solutions for $\gmn$~\cite{Baccetti:2012bk}.

Another important observation is that, as long as the above limit~(\ref{mglimit}) is not taken exactly, the bimetric equations of motion always force both metrics to be Einstein solutions if one of them is. This follows, for example, from the perturbative solutions that we obtain in chapter~\ref{ch:HD} and can also be shown explicitly for certain parameter choices. Therefore the Massive Gravity limit is a singular point in parameter space, where an important relation among the two metrics is lost.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
\section{Mass spectrum}\label{sec:massspec}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

From the nonlinear ADM analysis of \cite{Hassan:2011zd} it is known that ghost-free bimetric theory propgates $(d(d-2)-1)$ degrees of freedom. At the linear level around a certain class of backgrounds, these can be attributed to a massless and massive fluctuation. Around general backgrounds or at the nonlinear level, however, such a split is usually not well-defined. In {\protect{\hyperref[papV]{Paper V}}} we identify the backgrounds suitable for discussing the theory's mass spectrum in four dimensions. Then we perturb around these backgrounds and show how to diagonalize the fluctuations into modes with definite mass. {\protect{\hyperref[papVII]{Paper VII}}} generalizes these findings to an arbitrary number of space-time dimensions. Both papers also discuss possible nonlinear extensions of mass eigenstates, a topic which we leave for the next section.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Proportional backgrounds}\label{secpropbg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

A simple, yet very important class of solutions to the bimetric equations of motion is obtained by making an ansatz that conformally relates the two metrics, $\bfmn=c(x)^2\bgmn$, where $c(x)$ is a space-time dependent function. Having plugged this ansatz into the equations of motion, we first note that the Bianchi constraint~(\ref{Bianchi}) immediately enforces $\partial_\mu c(x)=0$ and hence $c(x)=$\,const. This restricts our ansatz to proportional metrics,
\beqn
\bfmn=c^2\bgmn\qquad \text{with}\quad c=\mathrm{const.}
\eeqn
Using this in (\ref{geq}) and (\ref{feq}) we find that the equations of motion simply reduce to two copies of Einstein's equations,
\begin{align}\label{bgeq}
\mathcal{G}_{\mu\nu}(\bar{g})
+\Lambda_g\bgmn=\frac{1}{m_g^{d-2}}\bar{T}^{g}_{\mu\nu}\,, \quad
\mathcal{G}_{\mu\nu}(\bar{g})
+\Lambda_f\bgmn=\frac{1}{m_f^{d-2}}\bar{T}^{f}_{\mu\nu} \,.
\end{align}
In this we have defined the cosmological constant contributions arising from the interaction potential,
\beqn\label{lambdas}
\Lambda_g&\equiv&\frac{m^d}{m_g^{d-2}}\sum_{n=0}^{d-1}{d-1\choose n}c^n\beta_n\,,\nn\\
\Lambda_f&\equiv&\frac{m^d}{(m_f c)^{d-2}}\sum_{n=1}^{d}{d-1\choose n-1}c^n\beta_n\,,
\eeqn
Proportional backgrounds thus simply correspond to solutions to Einstein's equations in General Relativity.
After all constant contributions in the stress-energy tensors have been shifted into $\Lambda_g$ and $\Lambda_f$, respectively,\footnote{This can always be achieved by redefining $\beta_0$ and $\beta_d$.} the difference of the above background equations implies that
\beqn\label{propbackeq}
\Lambda_g=\Lambda_f\,,\qquad
\bar{T}^{f}_{\mu\nu}=\alpha^{d-2}\bar{T}^{g}_{\mu\nu}\,,~~~~~\text{where}~~\alpha\equiv \frac{m_f}{m_g}\,.
\eeqn
From (\ref{lambdas}) it is clear that the first equation relating the cosmological constants is a polynomial in $c$ with coefficients depending on the $\beta_n$ parameters. In general, this equation serves to determine the proportionality constant $c$ of our ansatz in terms of the parameters of the theory and thereby specifies the solution completely. An important exception to this generic situation is the partially massless case, to be introduced in chapter~\ref{ch:PM}.  

The second equation in (\ref{propbackeq}) that relates the sources for the two metrics is very constraining. From a phenomenological point of view, there is no reason to believe that the matter sources satisfy such a strong constraint. Proportional background solutions, however, only exist in this case. Since any deviation from the proportional backgrounds constitutes a deviation from GR solutions, the difference in the source terms may be regarded as a measure for the difference of bimetric solutions from those of GR. 
 
The proportional background solutions are of particular interest because they allow for a definite mass spectrum of fluctuations around them. In general, the linear perturbation equations have a rather complicated structure because in order to derive them one needs to vary the square-root matrix $S=\sqrt{g^{-1}f}$. This is always possible but, for backgrounds giving rise to matrices $\bar{g}^{-1}\bar{f}$ that do not commute with the fluctuations, the resulting expressions are lengthy and not illuminating. In particular, the equations will not contain a mass term with Fierz-Pauli structure which makes it difficult to identify the massive field. In contrast, for the proportional backgrounds we have $\bar{g}^{-1}\bar{f}=c^2\mathbb{1}$ which does commute with any other matrix and hence drastically simplifies the perturbation equations which now will exhibit the Fierz-Pauli structure. Moreover, in the absence of sources, these backgrounds correspond to maximally symmetric ones for which the concept of mass as a label of representations of the underlying isometry group is well-defined. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsection{Linear perturbations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

We shall now consider small perturbations around the proportional backgrounds for both of the metrics as well as the sources,
\beqn
\gmn&=&\bgmn+\dg_{\mu\nu}\,,\qquad \fmn~=~c^2\bgmn+\df_{\mu\nu}\,,\nn\\
T^{g}_{\mu\nu}&=&\bar{T}^{g}_{\mu\nu}+\delta T^{g}_{\mu\nu}\,,\qquad T^{f}_{\mu\nu}~=~\alpha^{d-2}\bar{T}^{g}_{\mu\nu}+\delta T^{f}_{\mu\nu}\,.
\eeqn
In the following we set the background values of the sources to zero, $\bar{T}^{g}_{\mu\nu}=0$. In {\protect{\hyperref[papV]{Paper V}}} we keep them in the equations, which modifies the structure of the kinetic operator (\ref{kinopds}) below. As a consequence, the coupling of the fluctuations to the cosmological constant term assumes a less familiar form, which is our main motivation to present the equations without background sources here. Note however that their inclusion does not alter any of the results.


As stated earlier, around the proportional backgrounds the linearized equations of motion can be diagonalized into an equation for a massless and a massive perturbation. To this end, consider the following redefinitions of fluctuations,
\beqn\label{dGanddM}
\delta G_{\mu\nu} &\equiv&\left[1+(\alpha c )^{d-2}\right]^{\frac{4-d}{d-2}}\big(\dg_{\mu\nu}+c^{d-4}\alpha^{d-2}\df_{\mu\nu}\big)\,,\nn\\
\delta M_{\mu\nu} &\equiv& \frac{1}{2c}\big(\df_{\mu\nu}-c^2 \dg_{\mu\nu}\big)\,,
\eeqn
in which the overall normalizations have been chosen conveniently. Now, taking the appropriate linear combinations of the original fluctuation equations for $\delta\gmn$ and $\delta\fmn$ decouples the massless from the massive mode. The resulting equations read
\begin{align}
{\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}\delta G_{\rho\sigma}&-\tfrac{2}{d-2}\bar{\Lambda}_g\left(\delta G_{\mu\nu}-\tfrac{1}{2}\bar{G}_{\mu\nu}\delta G\right) \nn\\
& \hspace{75pt}=\left(\tfrac{1}{m_g}\right)^{\frac{d-2}{2}}\left(\delta T^g_{\mu\nu}+c^{d-2}\delta T^f_{\mu\nu}\right)\,, \label{dGeq}\\
{\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}\delta M_{\rho\sigma}&-\tfrac{2}{d-2}\bar{\Lambda}_g\left(\delta M_{\mu\nu}-\tfrac{1}{2}\bar{G}_{\mu\nu}\delta M\right)
+\tfrac{\bar{m}^2_\mathrm{FP}}{2}\Big(\delta M_{\mu\nu}-\bgmn\delta M\Big)\nn\\
& \hspace{75pt}=\left(\tfrac{c}{m_f}\right)^{\frac{d-2}{2}}\left(\delta T^f_{\mu\nu}-\alpha^{d-2}\delta T^g_{\mu\nu}\right)\,.\label{dMeq}
\end{align}
Here, the traces of the fluctuations are taken with respect to a redefined background metric, 
\beqn
\bar{G}_{\mu\nu}\equiv \big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}\bgmn\,,
\eeqn
that is $\delta G=\bar{G}^{\mu\nu}\delta G_{\mu\nu}$ and $\delta M=\bar{G}^{\mu\nu}\delta M_{\mu\nu}$. Also, we have redefined the cosmological constant with respect to this background,
\beqn
\bar{\Lambda}_g\equiv \big(1+(\alpha c)^2\big)^{-\frac{2}{d-2}} \Lambda_g  \,, \qquad R_{\mu\nu}(\bar{G})=\frac{2\bar{\Lambda}_g}{d-2}\bar{G}_{\mu\nu}\,.
\eeqn
Furthermore, the kinetic operator ${\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}$ with respect to the $\bar{G}_{\mu\nu}$ background is defined as
\begin{align}\label{kinopds}
\bar{\mathcal{E}}^{\rho\sigma}_{\mu\nu}\delta G_{\rho\sigma} 
=-\tfrac{1}{2}\Big[\delta^\rho_\mu\delta^\sigma_\nu\bar{\nabla}^2
&+\bar G^{\rho\sigma}\bar{\nabla}_\mu\bar{\nabla}_\nu 
-\delta^\rho_\mu\bar{\nabla}^\sigma\bar{\nabla}_\nu
-\delta^\rho_\nu\bar{\nabla}^\sigma\bar{\nabla}_\mu \nn\\
&-\bar{G}_{\mu\nu}\bar G^{\rho\sigma}\bar{\nabla}^2 
+\bar{G}_{\mu\nu}\bar{\nabla}^\rho\bar{\nabla}^\sigma\Big]\delta G_{\rho\sigma}\,,
\end{align}
in which $\bar{\nabla}$ is the covariant derivative compatible with $\bar{G}_{\mu\nu}$. Finally, the Fierz-Pauli mass is given in terms of the parameters of the theory through
\beqn\label{FPmass}
\bar{m}^2_\mathrm{FP}=\frac{m^d}{m_g^{d-2}} \big(1+(\alpha c)^2\big)^{-\frac{2}{d-2}}\left(1+(\alpha c)^{2-d}\right)\sum_{n=1}^{d-1}{d-2\choose n-1}c^n\beta_n\,.
\eeqn
Recall that in the above expressions $c$ is to be regarded as a function of the Planck masses and the $\beta_n$ parameters, determined by the background equation $\Lambda_g=\Lambda_f$. At this stage, the main reason for choosing the new background $\bar{G}_{\mu\nu}$ is to render the equations as simple as possible. However, as our notation already indicates, $\bar{G}_{\mu\nu}$ will also turn out to be the background of the nonlinear massless field that we identify below. Alternatively, we could have written the equations with respect to the original background $\bgmn$, in terms of $\Lambda_g$ and a properly rescaled Fierz-Pauli mass, $m^2_\mathrm{FP}\equiv \big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}\bar{m}^2_\mathrm{FP}$. In addition, there would be a factor of $\big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}$ in front of the source terms, modifying the effective Planck masses of the theory. In {\protect{\hyperref[papV]{Paper V}}} (and also in {\protect{\hyperref[papVI]{Paper VI}}}) we use $\bgmn$ as the background metric, whereas in {\protect{\hyperref[papVII]{Paper VII}}} we express the equations in terms of $\bar{G}_{\mu\nu}$. 

As promised, (\ref{dGeq}) and (\ref{dMeq}), respectively,  describe a massless and a massive spin-2 fluctuation in (Anti-) de Sitter background. At the linear level around proportional backgrounds, one can therefore assign $d(d-3)/2$ degrees of freedom to a massless fluctuation $\delta G_{\mu\nu}$ and the remaining $(d(d-1)/2-1)$ ones to a massive fluctuation $\delta M_{\mu\nu}$.

Observe that in the limit of small $\alpha$ (which is the limit opposite to the massive gravity limit discussed in section~\ref{sec:MGlim}), we have that $\delta G_{\mu\nu}\sim\delta \gmn$ and hence the fluctuation for the metric $\gmn$ becomes mostly massless. This is important because, at least to our present knowledge, only the couplings of the original metrics to matter are ghost-free, whereas on the other hand the gravitational metric needs to be mostly massless for phenomenological reasons. Fortunately, the limit in which the perturbation of $\gmn$ is dominated by the massless mode corresponds to a large Planck mass $m_g$, which is required for having a weak gravitational force anyway. We will come back to this point when discussing the nonlinear extension of the massless field below.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
\section{Nonlinear extensions of mass eigenstates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

In the previous section, we saw that the fluctuations of $\gmn$ and $\fmn$ around proportional backgrounds are not mass eigenstates, whereas certain linear combinations of them do satisfy the equations for massless and massive spin-2 fields. We now turn to the derivation of nonlinear fields  $G_{\mu\nu}$ and $M^G_{\mu\nu}$ that, when linearized around the proportional background solutions, give rise to these massless and massive perturbations. Having obtained expressions for these we are also able to address the question whether it is possible to couple the massless field to matter without reintroducing the Boulware-Deser ghost.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
\subsection{Identifying the nonlinear fields}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

In the following we will see that, as may have been anticipated, there are infinitely many possibilities to define nonlinear fields with massless or massive fluctuations around the proportional backgrounds. In {\protect{\hyperref[papVI]{Paper VI}}} and {\protect{\hyperref[papVII]{Paper VII}}}, we therefore invoke additional criteria of simplicity and invertibility which allow us to single out unique nonlinear extensions of the linear mass eigenstates.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsubsection{The massless field}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

General covariance implies that the most general ansatz for the nonlinear field $G_{\mu\nu}$ with massless fluctuation around proportional backgrounds is of the form
\beqn\label{ansatzG}
G_{\mu\nu}=g_{\mu\rho}{\Phi^\rho}_\nu(S)\,.
\eeqn
Here, ${\Phi^\rho}_\nu(S)$ is an arbitrary matrix-valued function of the square-root matrix $S=\sqrt{g^{-1}f}$. The transposed matrix $S^\mathrm{T}$ does not appear in the ansatz due to the symmetry property $gS=S^\mathrm{T}g$. Now, on the proportional backgrounds, any function of $S$ is proportional to the unit matrix and hence $\Phi(\bar{S})\equiv\phi( c)\mathbb{1}$, where $\phi( c)$ is just a scalar function of $c$. With (\ref{ansatzG}) the fluctuation of $G_{\mu\nu}$ can thus be written as
\beqn
\delta G_{\mu\nu}=\phi( c)\delta g_{\mu\nu}+\bar{g}_{\mu\rho}\left.\frac{\delta {\Phi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}\delta {S^\alpha}_\beta\,.
\eeqn
Using the variation of the square root around proportional backgrounds,
\beqn\label{sfluc}
\delta {S^\alpha}_\beta=\frac{1}{2c}\bar{g}^{\alpha\lambda}(\delta f_{\lambda\beta}-c^2\delta g_{\lambda\beta})\,,
\eeqn
we can compare this expression to the definition of the massless fluctuation in~(\ref{dGanddM}). This gives
\beqn
\phi(s)&=&\big(1+(\alpha c)^2\big)^{\frac{2}{d-2}}\,,\nn\\
 \left.\frac{\delta {\Phi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}&=& 2\left[1+(\alpha c )^{d-2}\right]^{\frac{4-d}{d-2}}c^{d-3}\alpha^{d-2}\delta^\rho_\alpha\delta^\nu_\beta\,.
\eeqn
These constraints on the matrix function ${\Phi^\rho}_\nu(S)$ have an infinite number of solutions given through power series of the matrix $S$ with mildly constrained coefficients. We present their general form in the case of four space-time dimensions in {\protect{\hyperref[papV]{Paper V}}}. From all of these possible definitions for the nonlinear massless field we choose the one that gives the simplest invertible relation to the original variables $\gmn$ and $\fmn$. This particular choice corresponds to
\beqn\label{defG}
G_{\mu\nu} = \left[1+(\alpha c )^{d-2}\right]^{\frac{4-d}{d-2}}\big(g_{\mu\nu}+c^{d-4}\alpha^{d-2}f_{\mu\nu}\big)\,.
\eeqn
Remarkably, it turns out to be simply a linear combination of the original metrics.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsubsection{The massive field}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to identify a nonlinear extension of the massive fluctuation, we make an ansatz similar to the one for the massless field above,
\beqn\label{ansatzM}
M_{\mu\nu}=g_{\mu\rho}{\Psi^\rho}_\nu(S)\,,
\eeqn
where ${\Psi^\rho}_\nu(S)$ is an arbitrary matrix-valued function of the square-root matrix ${S^\mu}_\nu$. Again, on the background we have $\Psi(\bar{S})=\psi( c)\mathbb{1}$ with $\psi( c)$ being a scalar function. The variation of the ansatz therefore reads
\beqn
\delta M_{\mu\nu}=\psi( c)\delta g_{\mu\nu}+\bar{g}_{\mu\rho}\left.\frac{\delta {\Psi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}\delta {S^\alpha}_\beta\,.
\eeqn
Comparing this to the definition of the massive fluctuation in (\ref{dGanddM}), we see that
\beqn\label{constdm}
\psi( c)=0\,,\qquad \left.\frac{\delta {\Psi^\rho}_\nu(S)}{\delta {S^\alpha}_\beta}\right|_{\bar{S}}=\delta^\rho_\alpha\delta^\beta_\nu\,. 
\eeqn
As in the massless case, there are infinitely many solutions to these constraints whose general form is provided in {\protect{\hyperref[papV]{Paper V}}} for $d=4$.
In order to single out a nonlinear extension of the massive fluctuation, we first observe that the interaction potential in the action is a polynomial in the square-root matrix ${S^\mu}_\nu$. Moreover, as can be seen by comparing~(\ref{dGanddM}) and~(\ref{sfluc}), the variation of this matrix gives the massive fluctuation up to normalization. However, ${S^\mu}_\nu$ is a (1,1)-tensor which furthermore satisfies the symmetry property $G_{\rho\mu}{S^\mu}_\nu=G_{\nu\mu}{S^\mu}_\rho$ and can therefore not be regarded as independent of the massless field. We would like the massive field to be a (0,2)-tensor that is independent of $G_{\mu\nu}$. On the other hand, lowering an index ${S^\mu}_\nu$ with $G_{\mu\nu}$ modifies the expression of its variation in terms of $\delta\gmn$ and $\delta\fmn$. According to (\ref{constdm}), in oder to obtain the massive fluctuation in~(\ref{dGanddM}) we must subtract the field's background value. 
Hence, our choice for the nonlinear massive fields is given by
\beqn
M^G_{\mu\nu} \equiv \left[1+(\alpha c )^{d-2}\right]^{-\frac{2}{d-2}}\left(G_{\mu\rho} {S^\rho}_\sigma-cG_{\mu\nu}\right)\,.
\eeqn
The reader is reminded once again that in this definition (and in the one for the massless field above), $c$ is a function of the $\beta_n$ parameters obtained by setting $\Lambda_g=\Lambda_f$.

In the next section it will be shown that the massless field $G_{\mu\nu}$, as defined in~(\ref{defG}), cannot consistently couple to matter sources. It is therefore not a suitable candidate for the gravitational metric and rewriting the bimetric theory in terms of $G_{\mu\nu}$ and $M^G_{\mu\nu}$ is probably not useful for phenomenological purposes. On the other hand, $\gmn$ can couple to matter without introducing inconsistencies and a formulation of the theory in terms of $\gmn$ and a corresponding massive field $M_{\mu\nu}$ may be of use for applications. A definition for this new field $M_{\mu\nu}$ which can be considered as independent of $\gmn$ while being compatible with (\ref{constdm}) is
\beqn\label{defMg}
M_{\mu\nu} \equiv g_{\mu\rho} {S^\rho}_\sigma-cg_{\mu\nu}\,.
\eeqn
A particular feature, shared by all possible definitions of the nonlinear massive fields, is that their background value vanishes on the proportional backgrounds. Because these backgrounds precisely corresponds to GR solutions, a nonzero background value for the nonlinear massive field is a measure for deviations of bimetric theory from General Relativity.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Inconsistency of coupling the massless field to matter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   

Astrophysical observations show that the mass of the graviton cannot be larger than the Hubble scale $\sim 10^{-33}$eV. A massless gravitational metric would therefore be favoured from a phenomenological point of view. Having obtained an expression for a nonlinear massless spin-2 field in the bimetric setup, we are therefore interested in the question whether this field could consistently be coupled to matter alone and hence represent the gravitational metric.
This motivates an ADM analysis of interactions between the massless field $G_{\mu\nu}$ and matter sources. To this end, consider the addition of a standard minimal matter coupling of the form
\beqn\label{mmcoup}
S^G_\mathrm{m}=\int \dd^d x~\sqrt{-G}\,\mathcal{L}^G_\mathrm{m}
\eeqn 
to the bimetric action. Since the Hamiltonian analysis of the latter has been performed in the original formulation of the theory, the simplest route to follow is to use the definition (\ref{defG}) of the massless field to obtain its ADM variables as functions of the ADM variables of $\gmn$ and $\fmn$. In fact, since constant factors are not of interest in the ADM analysis, we can simply rescale the metrics such that we have $G_{\mu\nu}=\gmn'+\fmn'$, where $\gmn'$ and $\fmn'$ possess ADM decompositions as in (\ref{admmetr}) and (\ref{admf}), respectively.
That is to say, we define 
\beqn
G_{\mu\nu}=\begin{pmatrix}
-K^2+K_m\Gamma^{mn}K_n&K_j\\ K_i & \Gamma_{ij}
\end{pmatrix}\,,
\eeqn
whose components obey
\beqn\label{ADMG}
K_i&=&N_i+L_i\,,\qquad \Gamma_{ij}~=~\gamma_{ij}+\tilde{f}_{ij}\,,\nn\\
K^2&=&N^2+L^2+\Gamma^{ij}K_iK_j-\gamma_{ij}N^iN^j-\tilde{f}_{ij}L^iL^j\,.
\eeqn
In these, the shift $N_i$ of $\gmn$ should be understood as a function of the other ADM variables and the redefined shift vectors $n_i$, according to~(\ref{shiftred}).  
After this redefinition the bimetric action is linear in the lapses $N$ and $L$ of $\gmn$ and $\fmn$ as well as the shift $L_i$ of $\fmn$. In order not to reintroduce the Boulware-Deser ghosts and maintain diffeomorphism invariance, the coupling (\ref{mmcoup}) must also be linear in these variables. 
On the other hand, since we take the couplings (\ref{mmcoup}) to resemble those of the metric in General Relativity, we know that due to general covariance of GR they have to be linear in the lapse $K$ and shift $K_i$ of $G_{\mu\nu}$.\footnote{For instance, this can explicitly be verified for the standard coupling of a massless scalar field, $\mathcal{L}^G_\mathrm{m}=G^{\mu\nu}\partial_\mu\phi\partial_\nu\phi$.} But from~(\ref{ADMG}) it is clear that the lapse $K$ is a nonlinear function of $N$, $L$ and $L^i$. In order to demonstrate the consistency bimetric action without matter coupling, so far we have only redefined $N_i$. We therefore still have the freedom to perform a redefinition of $L_i$ which possibly could render the expression for $K$ linear in $N$, $L$ and $L^i$. However, as we will now argue, such a redefintion does not exist. To see this, rewrite the above expression for~$K^2$ as
\beqn\label{defk2} 
K^2=N^2+L^2+(N^i-L^i) (\gamma_{ij}-\gamma_{ik} \Gamma^{kl} \gamma_{lj}) (N^j-L^j)  \,.
\eeqn
The redefinition of $L^i$ would have to turn the right-hand side of this equation into a perfect square of a function linear in $N$, $L$ and $L^i$. 
But due to the form of the redefinition~(\ref{shiftred}) required by the bimetric interaction potential, we have that 
\beqn 
N^i-L^i=Ln^i-N{D^i}_kn^k\,,
\eeqn
implying that the above expression for $K^2$ does not depend on $L^i$. Consequently, redefining $L^i$ cannot change the fact that $K$ is nonlinear in $N$ and $L$ and hence a coupling term of the form (\ref{mmcoup}) cannot be consistent.


Of course, we have not shown that a massless field in bimetric theory can never couple to matter in a ghost-free manner.
The above proof only applies to standard matter couplings and to the massless field singled out in the previous section. It is possible that other types of couplings or more complicated choices for the field remedy the above conclusion and there exist a way to obtain a massless gravitational metric.\footnote{Another option is to tune the $\beta_n$ parameters such that the Fierz-Pauli mass (\ref{FPmass}) vanishes. In this case, both $\gmn$ and $\fmn$ have massless fluctuations and the graviton could be massless while still interacting nontrivially with another spin-2 field at the nonlinear level.}  




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Massive spin-2 interactions with gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

Owing to the absence of ghost-free matter couplings for the nonlinear massless field, we choose to consider the standard consistent interactions of the metric $\gmn$ with matter sources. In this case, $\gmn$ is the gravitational metric with geometric interpretation. Its fluctuations, however, are neither massless nor massive; they are superpositions of mass eigenstates. Nonetheless, it is still possible to consider a nonlinear version of the massive spin-2 perturbation in this gravitational background. The appropriate nonlinear field which is independent of $\gmn$ is the one given in~(\ref{defMg}). 

In {\protect{\hyperref[papV]{Paper V}}} we rewrite the Hassan-Rosen bimetric action in terms of the variables $\gmn$ and $M_{\mu\nu}$. In the interaction potential, implementing the field redefinition is straightforward,
\beqn
\sum_{n=0}^d\beta_ne_n(S)=\sum_{n=0}^d\beta_ne_n(c\mathbb{1}+g^{-1}M)=\sum_{n=0}^d\alpha_n^ce_n(g^{-1}M)\,.
\eeqn
Here the new parameters $\alpha_n^c$ depend on the original $\beta_n$-parameters in the following way,
\beqn
\alpha^c_n\equiv\sum_{k=n}^d {d-n \choose k-n} c^k\beta_k\,.
\eeqn
The potential is therefore simply a polynomial in $M_{\mu\nu}$. In the kinetic term for $\fmn$ we invoke the curvature relations~(\ref{curvrel}) to rewrite it in terms of $\gmn$-covariant derivatives acting on $M_{\mu\nu}$. For notational simplicity, we present the result in terms of the matrix $S=c\mathbb{1}+g^{-1}M$,
\beqn
\sqrt{-f}\,R(f)=\sqrt{-g}\,(\det S)\left[\phi^{\mu\nu}R_{\mu\nu}(g)+\Pi_{\rho\omega}^{\sigma\pi\alpha\beta}\nabla_\alpha{S^\rho}_\sigma\nabla_\beta{S^\omega}_\pi\right]\,.
\eeqn
Here we have used the abbreviation,
\beqn
\phi^{\mu\nu}\equiv{(S^{-2})^\mu}_\rho g^{\rho\nu}\,,
\eeqn
as well as defined a nonlinear polarization tensor,
\begin{align}
\Pi_{\rho\omega}^{\sigma\pi\alpha\beta}
\equiv\big(2&\phi^{\alpha\mu}\phi^{\kappa\delta}\phi^{\beta\nu}
-2\phi^{\alpha\mu}\phi^{\beta\kappa}\phi^{\delta\nu}
\nn\\
&-\phi^{\alpha\beta}\phi^{\kappa\delta}\phi^{\mu\nu}
+\phi^{\alpha\beta}\phi^{\kappa\mu}\phi^{\delta\nu}\big)
\delta^\sigma_{(\kappa}\delta^\gamma_{\delta)}\,  
\delta^\pi_{(\mu} \delta^\lambda_{\nu)}\, S_{\gamma\rho}\,
S_{\lambda\omega}. 
\end{align}
Collecting all the terms we arrive at the nonlinear action for a massive spin-2 field $M_{\mu\nu}$ in a gravitational background $\gmn$,
\begin{align}\label{sp2gr}
&S_{M,g}~=~m_g^{d-2}\int\dd^d x~\sqrt{-g}\,R(g) +\int\dd^d x~\sqrt{-g}\,\mathcal{L}^g_\mathrm{m}\nn\\
&~+~m_f^{d-2}\int\dd^d x~\sqrt{-g}\,(\det S)\left[\phi^{\mu\nu}R_{\mu\nu}(g)+\Pi_{\rho\omega}^{\sigma\pi\alpha\beta}\nabla_\alpha{S^\rho}_\sigma\nabla_\beta{S^\omega}_\pi\right] \nn\\
&~-~2m^d\int\dd^dx~\sqrt{-g}\,\sum_{n=0}^d\alpha_n^ce_n(g^{-1}M)\,.
\end{align}
While in the bimetric formulation of the theory in terms of $\gmn$ and $\fmn$ the kinetic terms are diagonal, the massive spin-2 field shows highly nontrivial kinetic mixing with the gravitational metric. Moreover, as already stated above, $\gmn$ does not give rise to a massless fluctuation around maximally symmetric backgrounds, which could endanger the compatibility of the theory with observations. However, we also already observed that gravity becomes essentially massless in the limit where its interactions are weak, $m_g/m_f\rightarrow \infty$. Hence, although the presence of a massive spin-2 field always implies that the graviton is a superposition of mass eigenstates, the effects of this mixing are expected to be small due to the weakly interacting nature of gravity.

Of course, it is also possible to formulate the theory in terms of the nonlinear fields $G_{\mu\nu}$ and $M^G_{\mu\nu}$. The structure of the resulting action is even more involved than in~(\ref{sp2gr}) and we refrain from presenting it here. Its expression in four space-time dimensions can be found in {\protect{\hyperref[papV]{Paper V}}}.

From the consistent matter couplings in the original bimetric formulation one can furthermore derive ghost-free interactions between the massive spin-2 field $M_{\mu\nu}$ and arbitrary types of matter fields. For interactions with bosonic matter this is straightforwardly realized by making the replacement $\fmn=g_{\mu\alpha}{S^\alpha}_\beta{S^\beta}_\nu$ in the standard matter couplings $\int\dd^dx\, \sqrt{-f}\,\mathcal{L}^f_\mathrm{m}$ for $\fmn$. In {\protect{\hyperref[papV]{Paper V}}} we give an explicit example of coupling $M_{\mu\nu}$ to a massive spin-1 field and also work out the slightly more complicated couplings of the massive spin-2 field to fermions. The latter requires working in the vielbein formulation and making appropriate replacements in the $\gamma^\mu$ matrices as well as the spin connections.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Generalization to Multimetric Theory} 
\label{ch:MV}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Ghost-free bimetric theory describes the interaction of two spin-2 fields, one with massless and one with massive fluctuations around proportional backgrounds. In this section we discuss a generalization of the Hassan-Rosen action to an interacting theory for an arbitrary number of spin-2 fields as introduced in~\cite{Hinterbichler:2012cn}. In general, such a theory will contain one massless spin-2 mode along with many massive ones and, again, one has to ensure the absence of the corresponding Boulware-Deser ghosts. A formulation of the theory in terms of vielbeins turns out to be very convenient for the ghost proof, but reexpressing the consistent multivielbein action in terms of metrics is not entirely trivial.
In {\protect{\hyperref[papIV]{Paper IV}}} we develop a method to rewrite the multivielbein theory of~\cite{Hinterbichler:2012cn} in terms of the corresponding metrics as well as St\"uckelberg fields that take care of local Lorentz invariances. 
We begin the discussion with a demonstration of consistent and inconsistent multimetric couplings before going over to the multivielbein formulation. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multiple bimetric couplings}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

When constructing a theory for more than two spin-2 fields, of course, the main requirement on its structure remains the absence of the Boulware-Deser ghosts. The interaction potential for $\mathcal{N}$ fields therefore has to be chosen such that the action in Hamiltonian formulation gives rise to $(d+\mathcal{N}-1)$ constraints. Out of these,  $d$ should be first class constraints, generating the group of general coordinate transformations, while the remaining $(\mathcal{N}-1)$ are expected to be second class and serve to remove all Boulware-Deser ghosts from the spectrum. 


An obvious way to satisfy these requirements is to simply add up several copies of the Hassan-Rosen action for fields $\fmn$ and $\gmn^{(i)}$ with $i=1,\hdots, \mathcal{N}-1$, to obtain a theory in which one of the metrics coupled to all the others,
\beqn\label{centercoup}
S_\mathrm{center}(f,\{g^{(i)}\})=\sum_{i=1}^{\mathcal{N}-1}S_{\mathrm{HR}}(g^{(i)},f)\,.
\eeqn
This will be consistent because in every interaction potential one can redefine the ADM variables for $\gmn^{(i)}$ to make it linear in the lapse and shift of~$\fmn$ as well as the lapse of $\gmn^{(i)}$, such that one obtains the desired $(d+\mathcal{N}-1)$ constraints. 

The left panel of Figure~4.1 shows how such a coupling can be visualized in a graph~\cite{Hinterbichler:2012cn}. Each solid dot represents a different spin-2 field and the lines stand for standard Hassan-Rosen bimetric couplings between them. Fields corresponding to dots that are not connected by a line do not directly interact. Due to the corresponding picture with one metric in the center, we shall refer to interactions of the form~(\ref{centercoup}) as ``center couplings".

Another option to obtain consistent multiple bimetric interactions is to build a ``chain" of $\mathcal{N}$ coupled spin-2 fields $\gmn^{(k)}$ where $k=1,\hdots,\mathcal{N}$. That is to say, we take an action is of the form,
\beqn
S_\mathrm{chain}(\{g^{(k)}\})=\sum_{k=1}^{\mathcal{N}-1}S_{\mathrm{HR}}(g^{(k)},g^{(k+1)})\,,
\eeqn
for which the corresponding graph is depicted in the right panel of Figure~4.1.
This construction works because in the first term one can redefine the ADM variables for $g^{(1)}$ such that it becomes linear in the lapse and shift of $g^{(2)}$ as well as the lapse of $g^{(1)}$. In the second term one performs a similiar redefinition for the shift of $g^{(2)}$ which, since the redefinition is linear in the lapses, does not destroy the linearity in the lapse of $g^{(2)}$ in the first term. Note however that the second term will no longer be linear in the shift of $g^{(2)}$. Continuing with this procedure in all the terms results in an action that is linear in the lapse and shift of $g^{(\mathcal{N})}$ and in all the other lapses. 



    \begin{figure}[h]
    \begin{center}
    \includegraphics[width=210pt]{Pictures/vbvertex.pdf}
    \caption{The center couplings \textit{(left)} and the chain couplings \textit{(right)}.}
    \end{center}\label{figcentchaint}
    \end{figure}
    
  

In fact, it is also possible to combine the two above constructions in the following manner: First introduce a chain coupling for fields $f^{(k)}$, $k=1,\hdots,\mathcal{K}$, and then to each $f^{(k)}$ attach $I_k$ fields $g_{(k)}^{(i_k)}$, $i_k=1,\hdots\mathcal{I}_k$, in a center coupling. This gives 
\beqn\label{gencv}
S_\mathrm{c-v}~=~S_\mathrm{chain}(\{f^{(k)}\})+\sum_{k=1}^\mathcal{K}S_\mathrm{center}(f^{(k)},\{g_{(k)}^{(i_k)}\})\,.
\eeqn
In this theory the total number of fields is $\mathcal{N}=\mathcal{K}+\sum_{k=1}^\mathcal{K}\mathcal{I}_k$. An example for a graph is shown in the left panel of Figure~4.2.
  \begin{figure}[h]
    \begin{center}$
    \begin{array}{cc}
    \includegraphics[width=140pt]{Pictures/vbchainvertex.pdf}~~~~~ & ~~~~~
    \includegraphics[width=45pt]{Pictures/vbloop.pdf}
    \end{array}$
    \caption{The combined chain and center couplings \textit{(left)} and a forbidden loop coupling \textit{(right)}.}
    \end{center}
    \end{figure}
Note that the action~$S_\mathrm{c-v}$ still consists purely of multiple copies of the Hassan-Rosen bimetric action; we have not introduced any type of new interaction term. 
Of course, in the above construction, it is also possible to add further center couplings to each of the $g_{(k)}^{(i_k)}$.
However, it is important to realize that not all possible bimetric couplings are allowed. In particular, one may not couple the metrics in a ``loop", which means adding terms such as $S_{\mathrm{HR}}(f^{(k)},f^{(k+2)})$ or $S_{\mathrm{HR}}(f^{(k+1)},g_{(k)}^{(i_k)})$ to (\ref{gencv}). To see why this fails, consider a simple loop coupling among three metrics,
\beqn\label{loopact}
S_\mathrm{loop}(g,f,h)=S_{\mathrm{HR}}(g,f)+ S_{\mathrm{HR}}(f,h)+S_{\mathrm{HR}}(h,g)\,,
\eeqn
whose graph is depicted in the right panel of Figure~4.2.
Now imagine that in the first term one redefines the shift of $g$ to render it linear in the lapse and shift of $f$ and the lapse of $g$. Then, in the second term redefine the shift of $f$ such that the first two terms afterwards are linear in the lapse and shift of $h$ and the lapses of $g$ and $f$. In the third term, one would now have to redefine the shift of $h$, but from the particular form~(\ref{shiftred}) of the redefinition it is clear that afterwards, the action will again contain the original shift variable for $g$ which cannot be expressed in terms of the redefined variables only. Therefore there is at least no obvious consistent redefinition of ADM variables that renders (\ref{loopact}) linear in all the lapses and we conclude that the loop couplings most likely give rise to Boulware-Deser ghosts. This is in agreement with results of a similar analysis performed in~\cite{Nomura:2012xr}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multivielbein couplings}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

So far we have used the earlier results of the bimetric ADM analysis in order to couple several spin-2 fields to each other using only bimetric interactions. Now we would like to address the question whether there exist more general couplings than the bimetric vertex. We introduce graphs for two examples of such $n$-point vertices in Figure~4.3. 
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=150pt]{Pictures/vbmulti1.pdf}
       \caption{A three- and a four-point vertex.}
    \end{center}
    \end{figure}
A priori, such couplings could be very different from the bimetric ones and the ADM analysis has to be redone from the start.

The problem is simplified when working with vielbeins ${E^a}_\mu(I)$, labeled by an index $I=1,\hdots,\mathcal{N}$, instead of the corresponding metrics $g_{\mu\nu}(I)$. The metrics expressed in terms of the vielbeins read
\beqn\label{defvielbein}
g_{\mu\nu}(I)={E^a}_\mu(I)\eta_{ab}{E^b}_\nu(I)\,.
\eeqn 
The vielbeins have a coordinate index $\mu$ as well as a Lorentz index $a$ and the definition of the metric is invariant under local Lorentz transformations.
Their kinetic terms are simply taken to be the Einstein-Hilbert terms $S_\mathrm{EH}(I)$ for the metrics expressed in terms of~${E^a}_\mu(I)$ through~(\ref{defvielbein}).
In~\cite{Hinterbichler:2012cn} it is shown that then the interactions of vielbeins that lead to ghost-free theories are of the form
\begin{align}\label{vielbeinpot}
S_\mathrm{int}&=\frac{m^2}{4}\sum_{\{I\}}\int\dd^dx~T^{I_1\hdots I_d}U_{I_1\hdots I_d}\,,\nn\\
\text{with}~~~~U_{I_1\hdots I_d}&=\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{a_1\hdots a_d}{E^{a_1}}_{\mu_1}(I_1)\hdots{E^{a_d}}_{\mu_d}(I_d)\,,
\end{align}
where $T^{I_1\hdots I_d}$ are coupling constants, and $\tilde{\epsilon}^{\mu_1\hdots\mu_d}$ and $\tilde{\epsilon}_{a_1\hdots a_d}$ are the totally antisymmetric tensor densities with respect to GCT and Lorentz transformations, respectively. The total multivielbein action is then given by
\beqn\label{multac}
S_\mathrm{multi}=\sum_{I=1}^\mathcal{N}S_\mathrm{EH}(I)+S_\mathrm{int}\,.
\eeqn
Note that the antisymmetric structure of (\ref{vielbeinpot}) ensures that there cannot be more than $d$ vielbeins interacting in one vertex. The ghost-free theory therefore gives rise to diagrams of the type displayed in Figure~3.3 with at most $d$ lines ending in one vertex. 
%We will summarize the consistency proof of~\cite{Hinterbichler:2012cn} in section~\ref{secvbghost}. 

A few remarks on degree-of-freedom counting in the vielbein theory are in order. A general vielbein has no symmetry properties and therefore consists of $d^2$ independent components, whereas the corresponding metric is symmetric and thus only $d(d+1)/2$ of its components are independent. This discrepancy can of course be explained by the presence of additional gauge symmetries in the vielbein theory which serve to remove the redundant degrees of freedom. These $d(d-1)/2$ gauge transformations are the local Lorentz transformations ${\Lambda^b}_a(I)$ that act on the upper index of the vielbein ${E^a}_\mu(I)$. A general theory for $\mathcal{N}$ vielbeins ${E^a}_\mu(I)$ will therefore be invariant under $\mathcal{N}$ distinct local Lorentz transformations. Note however that in (\ref{vielbeinpot}), $\mathcal{N}-1$ of the local Lorentz gauges have already been fixed in order to identify the different Lorentz frames for each vielbein with each other and contract all their indices with a common antisymmetric tensor. Only one overall Lorentz invariance is left over. As discussed in~\cite{Hinterbichler:2012cn} and reviewed in {\protect{\hyperref[papIV]{Paper IV}}}, for each vielbein there exist $d(d-1)/2$ combinations of its equations of motion following from (\ref{multac}) that do not contain any derivatives. These read
\beqn\label{constvierb}
\frac{\delta S_\mathrm{int}}{\delta {E^a}_\mu(I)}{E^c}_\mu(I)\eta_{cb}-\frac{\delta S_\mathrm{int}}{\delta {E^b}_\mu(I)}{E^c}_\mu(I)\eta_{ca}=0\,,
\eeqn
and give the correct number of constraints to reduce the number of independent components of each vielbein to $d(d+1)/2$, as expected in a gauge-fixed theory. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Hamiltonian analysis of the vielbein theory}
\label{secvbghost}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Before we come to its metric formulation, we review the ADM analysis of the multivielbein theory as presented in~\cite{Hinterbichler:2012cn}, which proves the absence of the Boulware-Deser ghosts. 
The Hamiltonian analysis is carried out for the vielbein action with interaction potential in its gauge fixed form~(\ref{vielbeinpot}). It makes use of the fact that the vielbein ${E^a}_\mu$ can be decomposed as 
\beqn\label{decvbla}
{E^a}_\mu(I)={\hat{\Lambda}^a}_{~b}(I){\hat{E}^b}_{~\mu}(I)\,,
\eeqn
where ${\hat{\Lambda}^a}_{~b}(I)$ is a Lorentz transformation and ${\hat{E}^b}_{~\mu}(I)$ is a constrained vielbein for which the following ADM parameterization may be chosen,
\beqn\label{ADMvb}
{\hat{E}^b}_{~\mu}(I)=\begin{pmatrix}
N(I)&0\\ {\hat{e}^s}_{~j}(I)N^j(I)&{\hat{e}^s}_{~i}(I)
\end{pmatrix}\,.
\eeqn
At this point it becomes evident why the vielbein formulation significantly simplifies the Hamiltonian analysis: In contrast to the ADM parameterization of the metric, c.f.~(\ref{admmetr}), the expression for the vielbein is itself already linear in lapse and shift. 
When $d$ vielbeins are contracted with the totally antisymmetric $\tilde{\epsilon}$-tensors in~(\ref{vielbeinpot}), the resulting expression will be linear in all ${E^a}_0(I)$, which implies linearity in $N(I)$ and $N^j(I)$. This certainly is a great advantage over the metric formulation because, due to the absence of square root matrices, no redefinition of ADM variables is needed. However, the simplification does not come without a price, because one still has to deal with the Lorentz matrices ${\hat{\Lambda}^a}_{~b}(I)$ and the extra gauge invariances, as we will explain now. 

The parameterization (\ref{ADMvb}) does not fix the gauge completely but is invariant under the residual gauge group of spatial rotations. To the action one should therefore add a term $\lambda^{ab}(I)\mathcal{P}_{ab}(I)$ for each vielbein, where $\lambda^{ab}(I)$ is a Lagrange multiplier and $\mathcal{P}_{ab}(I)$ are the $\mathcal{N}$ first class constraints that generate the residual gauge group of spatial rotations. The explicit expressions for the matrices $\mathcal{P}_{ab}(I)$ are not important to us but we emphasize that they are functions of the spatial vielbeins and there canonical momenta alone.
It also follows that each ${\hat{\Lambda}^a}_{~b}(I)$ can be parameterized by $d-1$ boosts~$p^a(I)$ which, when the decomposition (\ref{decvbla}) is plugged into the interaction potential~(\ref{vielbeinpot}), enter as St\"uckelberg fields. 

Thus, the potential in ADM variables is of the form
\beqn
S_\mathrm{int}=\int\dd^dx~\sum_{I=1}^{\mathcal{N}}\Big(N(I)\mathcal{C}(I)+N^j(I)\mathcal{C}_j(I)\Big)\,,
\eeqn
where the lapse and shift constraints $\mathcal{C}(I)$ and $\mathcal{C}_j(I)$ are functions of the spatial vielbeins ${\hat{e}^s}_{~i}(I)$ and the boosts $p^a(I)$.  When expressed in terms of vielbeins, the ADM form of the Lorentz invariant kinetic terms is similar to~(\ref{gradm}) in the metric theory, and the full action is linear in all~$N(I)$ and~$N^j(I)$.

Recall that the action with potential in its gauge fixed form still possesses one overall local Lorentz invariance. Part of this residual gauge symmetry can now be used to rotate away one of the $p^a(I)$. The remaining boosts can be solved for using $\mathcal{N}-1$ of the $N^j(I)$ equations. In this way all $p^a(I)$ are eliminated from the action. The last shift constraint together with one of the lapse constraints generate general coordinate transformations. The remaining $\mathcal{N}-1$ lapse equations are the secondary constraints that remove the Boulware-Deser ghosts.

The degree-of-freedom counting in the vielbein theory therefore goes as follows: To start with, there are $(d-1)^2$ components in each of the $\mathcal{N}$ spatial vielbeins, along with corresponding $\mathcal{N}(d-1)^2$ canonical momenta. 
The residual overall gauge invariance under spatial rotations gives rise to first class constraint $\sum_I\mathcal{P}_{ab}(I)$ and remove $2\cdot (d-1)(d-2)/2$ degrees of freedom in total. The remaining $\mathcal{N}-1$ spatial Lorentz transformations have been used for gauge fixing and therefore now give rise to second class constraints upon variation with respect to $\lambda^{ab}(I)$. This reduces the phase space by another $2\cdot (\mathcal{N}-1)(d-1)(d-2)/2$ dimensions.
The overall general coordinate transformations again give first class constraints and take away $2d$ variables. Finally, the $\mathcal{N}-1$ lapse constraints are assumed (although not shown) to also give rise to secondary constraints, which then together remove another $2(\mathcal{N}-1)$ degrees of freedom. 
Putting everything together, we find that the dimension of phase space is 
\begin{align}
D_\mathrm{p.s.}=2\cdot (\mathcal{N}-1)\Big(d(d-1)/2-1\Big)+2\cdot d(d-3)/2\,.
\end{align}
This is the correct number of degrees of freedom for describing $\mathcal{N}-1$ massive and one massless spin-2 particle.











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multimetric theory}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Let us briefly outline how this equivalence follows in a theory with only two interacting vielbeins ${E^a}_\mu\equiv{E^a}_\mu(1)$ and ${\bar{E}^a}_\mu\equiv{E^a}_\mu(2)$  (the more general case of multiple two-point interactions is very similar).  As demonstrated in~\cite{Hinterbichler:2012cn}, the equations of motion are solved by vielbeins that satisfy\footnote{There may also be other branches of solutions that lead to a theories which are not equivalent to the bimetric description, see~\cite{deffayet}.}
%\beqn
%{(E^{-1})^\mu}_a{\bar{E}^a}_\nu
%\eeqn  



The structure of (\ref{vielbeinpot}) is reminiscent of the ghost-free bimetric interaction potential (\ref{potantisym}), and for certain choices of $T^{I_1\hdots I_d}$ the vielbein and metric theories are indeed equivalent. More precisely, this is true whenever the interactions consist only of two-point vertices and contain no loops, i.e.~gives rise to the graphs of Figure~3.1. In that case, the constraints~(\ref{constvierb}) give rise to a symmetrization condition on the vielbeins which allows certain combinations of them to be expressed as square root matrices of the type $\sqrt{g^{-1}f}$. This explains why it is possible to have loop interactions in the vielbein theory despite the no-go statement we made about the metric formulation. We will see how this works in more detail below, after we have discussed the general case.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Obtaining a metric formulation}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In {\protect{\hyperref[papIV]{Paper IV}}} we show that it is always possible to reexpress the vielbein theory in terms of the corresponding metrics together with a set of St\"uckelberg fields. The main idea is to move away from the gauge fixed form of the vielbein that lead to the potential~(\ref{vielbeinpot}), and instead consider $\mathcal{N}$ general vielbeins ${e^a}_\mu(I)$ along with $\mathcal{N}$ independent Lorentz frames. 
The ${e^a}_\mu(I)$ are related to the  gauge fixed ${E^a}_\mu(I)$ by a local Lorentz transformation ${\Lambda^a}_b(I)$ through ${E^a}_\mu(I)={\Lambda^a}_b(I){e^b}_\mu(I)$. Since the corresponding metrics are Lorentz invariant, we again have
\beqn\label{defvielbein2}
g_{\mu\nu}(I)={e^a}_\mu(I)\eta_{ab}{e^b}_\nu(I)\,,
\eeqn 
and the kinetic terms are do not involve the local Lorentz matrices. On the other hand, the interaction potential~(\ref{vielbeinpot}) is now given in terms of
\beqn\label{unfixpot}
U_{I_1\hdots I_d}&=\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{a_1\hdots a_d}{\Lambda^{a_1}}_{b_1}{e^{b_1}}_{\mu_1}(I_1)\hdots{\Lambda^{a_d}}_{b_d}{e^{b_d}}_{\mu_d}(I_d)\,.
\eeqn
The local Lorentz matrices ${\Lambda^a}_b(I)$ appear in the action as St\"uckelberg fields\footnote{For recent references that make use of our method of using St\"uckelberg fields to restore the local Lorentz symmetries in multivielbein theory, see \cite{Gabadadze:2013ria, Ondo:2013wka}.} that restore the full set of $\mathcal{N}$ local Lorentz invariances in the theory. Their indices transform in two different frames, namely those of $\tilde{\epsilon}_{a_1\hdots a_d}$ and ${e^b_i}_{\mu_i}(I)$, respectively. The gauge choice that corresponds to~(\ref{vielbeinpot}) is the one in which all ${\Lambda^a}_b(I)$ are equal since in that case the $\tilde{\epsilon}$ contractions reduce them to a factor $\det\Lambda=1$.

The fully gauge invariant potential given in terms of (\ref{unfixpot}) is the starting point for converting the vielbein into a metric theory. The important point is that it allows us to choose any convenient gauge for the vielbeins ${e^a}_{\mu}(I)$, which is of course not possible in its gauge fixed form~(\ref{vielbeinpot}). As we will see now, the freedom of choosing a gauge is essential for the theory being expressible in terms of metrics.

From the gauge invariant form we proceed by identifying the frames of one of the vielbeins, say ${e^b}_{\mu}(1)$, and $\tilde{\epsilon}_{a_1\hdots a_d}$ . Then, due to the invariance of the totally antisymmetric tensor density, we can rewrite (\ref{unfixpot}) as
\beqn\label{newpotga}
U_{I_1\hdots I_d}&=\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{c_1\hdots c_d}{\Lambda^{c_1}}_{b_1}(1,I_1){e^{b_1}}_{\mu_1}(I_1)\hdots{\Lambda^{c_d}}_{b_d}(1,I_d){e^{b_d}}_{\mu_d}(I_d)\,.\nn\\
\eeqn
Here we have defined the combined Lorentz matrices,
\beqn
{\Lambda^{c}}_{b}(1,I)\equiv{(\Lambda^{-1})^c}_a(1){\Lambda^{a}}_{b}(I)\,,
\eeqn
whose indices transform in the frame of ${e^b}_{\mu}(1)$ and ${e^b}_{\mu}(I)$, respectively. Note that ${\Lambda^{c}}_{b}(1,1)=\delta^c_b$ such that there are only $\mathcal{N}-1$ nontrivial matrices. With the interaction potential brought into the form (\ref{newpotga}), we now again pick a gauge for the vielbeins ${e^b}_{\mu}(I)$, $I=2,\hdots,\mathcal{N}$. Namely, we introduce gauge fixed vielbeins ${\overline{e}^a}_{\rho}(I)$ that satisfy the following symmetry condition,
\beqn
{\overline{e}^b}_{\rho}(I){(e^{-1})^\rho}_c(1)\eta^{ca}={\overline{e}^a}_\rho(I){(e^{-1})^\rho}_c(1)\eta^{cb}\,.
\eeqn
This is sometimes referred to as the Deser-van-Nieuwenhuizen gauge.\footnote{It has been argued in \cite{Deffayet:2012zc} that it might not always be possible to choose this gauge in general. For instance, in four space-time dimensions it requires the existence of the square root matrix $\sqrt{g^{-1}(1)g(I)}$.}
In particular, it again identifies all of the Lorentz frames with that of ${e^a}_{\mu}(1)$. In this specific frame one then has
\begin{align}
g^{\mu\rho}(1)g_{\rho\nu}(I)&={(e^{-1})^\mu}_a(1){\overline{e}^b}_{\rho}(I){(e^{-1})^\rho}_c(1)\eta^{ca}\eta_{bd}{\overline{e}^d}_{\nu}(I)\nn\\
&={(e^{-1})^\mu}_a(1){\overline{e}^a}_\mu(I){(e^{-1})^\mu}_c(1){\overline{e}^c}_{\nu}(I)\nn\\
&=\left(\left[e^{-1}(1)\overline{e}(I)\right]^2\right)^\mu_{~\rho}\,,
\end{align}
or, equivalently, in matrix notation,
\beqn
\sqrt{g^{-1}(1)g(I)}=e^{-1}(1)\overline{e}(I)\,.
\eeqn
Using ${\overline{e}(I)^a}_\mu$ in (\ref{newpotga}) as well as the identity
\beqn
\tilde{\epsilon}_{c_1\hdots c_d}=\sqrt{-\det g(1)}\,\tilde{\epsilon}_{\nu_1\hdots \nu_d}{(e^{-1})^{\nu_1}}_{c_1}(1)\hdots{(e^{-1})^{\nu_d}}_{c_d}(1)\,,
\eeqn
we can finally express the gauge invariant potential as 
\begin{align}\label{metrexp}
U_{I_1\hdots I_d}
=\sqrt{-\det g(1)}\,&\tilde{\epsilon}^{\mu_1\hdots\mu_d}\tilde{\epsilon}_{\nu_1\hdots \nu_d}
{L^{\nu_1}}_{\lambda_1}(I_1)\left[\sqrt{g^{-1}(1)g(I_1)}\right]^{\lambda_1}_{~\mu_1}\hdots \nn\\
&\hdots{L^{\nu_d}}_{\lambda_d}(I_d)\left[\sqrt{g^{-1}(1)g(I_d)}\right]^{\lambda_d}_{~\mu_d}\,.
\end{align}
Here we have defined new St\"uckelberg fields with coordinate indices,
\beqn
{L^{\nu}}_{\lambda}(I)\equiv{(e^{-1})^{\nu}}_{a}(1){\Lambda^{a}}_{b}(1,I){e^b}_{\lambda}(1)\,.
\eeqn
Equation~(\ref{metrexp}) is the metric expression for the multivielbein theory of~\cite{Hinterbichler:2012cn}. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The ${L^{\nu}}_{\lambda}(I)$ equations.}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Varying the multivielbein action~(\ref{multac}) with interaction potential~(\ref{metrexp}) with respect to the ${L^{\nu}}_{\lambda}(I)$ gives $d(d-1)/2$ constraint equations for each~$I=2,\hdots,\mathcal{N}$, that can be used to eliminate the St\"uckelberg fields from the action. These equations replace the constraints~(\ref{constvierb}) that arose in the gauge fixed version of the theory. 

When trying to solve the ${L^{\nu}}_{\lambda}(I)$ equations for Lorentz degrees of freedom, one encounters a subtlety. Namely, the conditions that follow from the invariance of $\eta_{ab}$ under Lorentz transformations and reduce the number of independent components in ${L^{\nu}}_{\lambda}(I)$ to $d(d-1)/2$ read 
\beqn
{(L^\mathrm{T})_\mu}^\rho(I)g_{\rho\sigma}(1){L^\sigma}_\nu(I)=g_{\mu\nu}(1)\,,
\eeqn 
which imply that ${L^{\nu}}_{\lambda}(I)$ depends on the metric $\gmn(1)$. In order to extract the metric independent part, we therefore use the Caley transform of a Lorentz transformation to express the St\"uckelberg fields in terms of antisymmetric matrices $A_{\mu\nu}(I)$,
\beqn
{L^{\nu}}_{\lambda}(I)=\Big(\big[g(1)+A(I)\big]^{-1}\big[g(1)-A(I)\big]\Big)^\mu_{~\nu}\,.
\eeqn
Since the antisymmetry condition on $A_{\mu\nu}(I)$ is completely independent of the metric $\gmn(1)$, we can parameterize the gauge degrees of freedom in terms of its components.
The equations for the $A_{\rho\sigma}(I)$ are then obtained from
\beqn
\frac{\delta S_\mathrm{multi}}{\delta A_{\rho\sigma}(I)}=\frac{\delta {L^{\mu}}_{\nu}(I)}{\delta A_{\rho\sigma}(I)}\frac{\delta S_\mathrm{int}}{\delta {L^{\mu}}_{\nu}(I)}=0 \,.
\eeqn
Multiplying by $(g(1)-A(I))_{\rho\alpha}(g(1)-A(I))_{\sigma\beta}$ and evaluating the first factor results in
\beqn\label{Lconstr}
\Big({L^\mu}_\alpha(I)g_{\beta\nu}(1)-{L^\mu}_\beta(I)g_{\alpha\nu}(1)\Big)\frac{\delta S_\mathrm{int}}{\delta {L^{\mu}}_{\nu}}=0\,.
\eeqn
As explained in {\protect{\hyperref[papIV]{Paper IV}}}, these $(\mathcal{N}-1)\cdot d(d-1)/2$ equations can indeed be shown to be equivalent to the constraints~(\ref{constvierb}) on the gauge fixed vielbeins ${E^a}_\mu(I)$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Recovering bimetric interactions}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We would now like to address the question under what circumstances the interaction potential~(\ref{metrexp}) is writable in terms of metrics alone without having to introduce St\"uckelberg fields. 
In principle, plugging back the solution to the constraint equations~(\ref{Lconstr}) into the action will always result in a theory involving only the metrics, but in reality the explicit solution for the St\"uckelberg fields is difficult to obtain in the general case. In particular, the constraints may need to be solved componentwise, resulting in a noncovariant expressions for the interaction potential in terms of metrics alone.

Nevertheless, there is one case in which the situation is greatly simplified. Suppose we demand the interactions to be expressible in terms of $\sqrt{g^{-1}(1)g(I)}$ after integrating out the St\"uckelberg fields . The only obvious situation in which this requirement is satisfied is when the constraint equations~(\ref{Lconstr}) allow for solutions ${L^{\nu}}_{\lambda}(I)=\delta^\nu_\lambda$, or, equivalently, $A_{\mu\nu}(I)=0$. If that is the case, then on this solution~(\ref{Lconstr}) reduces to
\beqn\label{LconstrA0}
\left.\left(\frac{\delta S_\mathrm{int}}{\delta L^{\mu\nu}}-\frac{\delta S_\mathrm{int}}{\delta L^{\nu\mu}}\right)\right|_{A=0}=0\,,
\eeqn
where we have raised the index on ${L^{\nu}}_{\lambda}(I)$ with $g(1)^{\lambda\mu}$.
We will now argue that (\ref{LconstrA0}) together with $A_{\mu\nu}(I)=0$ is a consistent solution if the interaction potential contains only interactions between two vierbeins ${e^a}_\mu(1)$ and ${e^a}_\mu(2)$. In that case, namely, a generic term in the potential reads
\begin{align}\label{potfortv}
\sqrt{-\det g(1)}~&\tilde{\epsilon}^{\mu_1\hdots\mu_n\lambda_{n+1}\hdots\lambda_{d}}\tilde{\epsilon}_{\nu_1\hdots \nu_d \lambda_{n+1}\hdots\lambda_{d}}\nn\\
&~~~~~~~~~~~~\cdot L^{\nu_1\kappa_1}(2)S_{\kappa_1\mu_1}
\hdots 
L^{\nu_n\kappa_n}(2)S_{\kappa_n\mu_n}\,,
\end{align}
where we have defined the symmetric matrix
\beqn
S_{\kappa\mu}\equiv g(1)_{\kappa\rho}\left(\sqrt{g^{-1}(1)g(2)}\right)^\rho_{~\mu}\,.
\eeqn
Now take the variation of (\ref{potfortv}) with respect to $L^{\mu\nu}$ and in that set $A_{\mu\nu}(2)=0$, i.e.~$L^{\mu\nu}(2)=g^{\mu\nu}$. This gives an expression involving terms that are proportional to powers of $S_{\mu\nu}$. As a consequence of the symmetry of $S_{\mu\nu}$, this expression is symmetric itself. Therefore all terms in the variation of $S_\mathrm{int}$ with respect to $L^{\mu\nu}$ are symmetric when evaluated on $A_{\mu\nu}(2)=0$ and hence (\ref{LconstrA0}) holds. This shows that $A_{\mu\nu}(2)=0$ is indeed a solution to the constraint equations in this case, and thus integrating out the St\"uckelberg fields results in the Hassan-Rosen bimetric action with potential~(\ref{potantisym}).

Using the same arguments as above, it is easy to see that this result carries over to the case of $\mathcal{N}$ vielbeins with only bimetric interactions. The equivalent metric description is of the form~(\ref{gencv}). We conclude that the vielbein theories that possess straightforward reformulations in terms of metrics alone precisely correspond to graphs of the form shown in the left panel of Figure~4.2. In order to build more complicated interactions, such as loops and $n$-point vertices with $n>2$, one must invoke the St\"uckelberg fields ${L^{\nu}}_{\lambda}$ and solve their equations in a nontrivial way.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Bimetric Cosmology}
\label{ch:cosmo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


On small scales General Relativity makes very good predictions and, from a phenomenological point of view, there is no need to look for a modification of the theory. On cosmological states, however, it seems that either quantum field theory or gravity (or both) have to be modified in order to explain the observed value of the cosmic acceleration. Therefore, once a consistent theory of modified gravity has been constructed, its implications for cosmology are of great interest. Self-accelerating solutions of massive gravity have, for instance, been considered in \cite{deRham:2010tw, Gumrukcuoglu:2011ew}, and the hope was that a large cosmological constant could be screened out by the graviton mass that weakens gravity at large scales. However, this does not seem to be possible without fine tuning \cite{Hassan:2011vm}. In \cite{D'Amico:2011jj} the authors show that there exist no homogeneous and isotropic solutions in the dRGT model of Massive Gravity with flat reference metric. On the other hand, our analysis of bimetric theory with dynamical reference metric shows that in this framework such solutions do exist. The simplest examples are the proportional backgrounds considered in section~\ref{secpropbg} which, however, exist only for proportional sources. In this chapter we consider a different class of solutions for which one of the sources is set to zero. 
The existence of cosmological solutions in bimetric theory, in turn, implies their presence in Massive Gravity with a general homogeneous and isotropic reference frame. Homogeneous and isotropic solutions in bimetric gravity are the subject of {\protect{\hyperref[papII]{Paper~II}}} and have also been investigated in two further articles~\cite{Volkov:2011an, Comelli:2011zm} that appeared roughly at the same time. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Standard cosmology in General Relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Before discussing homogeneous and isotropic solutions in bimetric gravity, let us briefly review the derivation of the cosmological evolution equations in GR. To this end, we consider the Einstein-Hilbert action in $d=4$ including a cosmological constant term as well as a standard coupling of the metric $\gmn$ to matter,
\beqn
S_\mathrm{EH+m}=\frac{1}{M_\mathrm{PL}^2}\int\dd^4x\sqrt{-g}~\big(R-2\Lambda\big)+\int\dd^4x\sqrt{-g}~\mathcal{L}_m
\eeqn
The equations of motions for $\gmn$ obtained from this action read
\beqn\label{einsteq}
R_{\mu\nu}-\frac{1}{2}\gmn R=\frac{1}{M_\mathrm{PL}^2}\left(T_{\mu\nu}-\rho_\Lambda\,\gmn\right)\,,
\eeqn
where $T_{\mu\nu}$ is the stress-energy tensor obtained from variation of the matter Lagrangian as in (\ref{strente}) and we have defined the constant energy density $\rho_\Lambda\equiv\Lambda M_\mathrm{PL}^2$. 

When looking for homogeneous and isotropic solutions in general relativity, one makes a Friedmann-Robertson-Walker ansatz for the metric,
\beqn\label{FRWg}
\gmn \md x^\mu\md x^\nu=-\md t^2+a(t)^2\left(\frac{1}{1-kr^2}\md r^2+r^2\md \Omega\right)\,,
\eeqn
in which $k=0,-1,+1$ parameterizes the curvature of the universe (flat, open, closed), $a(t)$ is the scale factor, and $\md \Omega=\md \theta^2+\sin^2 \theta\,\md \varphi^2$. 
In accordance with homogeneity and isotropy, the stress-energy tensor is taken to be that of a perfect fluid, 
\beqn\label{setans}
{(T^g)^{\mu}}_\nu=\mathrm{diag}(-\rho, p, p, p)\,,
\eeqn
where $\rho(t)$ and $p(t)$ are the time dependent energy density and pressure of the fluid, respectively. As a consequence of the Bianchi identity the source is automatically covariantly conserved which implies the continuity equation,
\beqn\label{conteq}
\dot{\rho}+3\frac{\dot{a}}{a}\big(\rho+p\big)=0\,,
\eeqn
where dots denote time derivatives. This equation is actually nothing but the first law of thermodynamics, $\dd E=-p\,\dd V$, for an adiabatic expansion with volume $V=a^3$ and energy $E=\rho a^3$. 

Plugging the diagonal ans\"atze~(\ref{FRWg}) and~(\ref{setans}) into Einstein's equations~(\ref{einsteq}) gives a set of four equations. The 00-component is Friedmann's equation,
\beqn\label{Friedmann}
\left(\frac{\dot{a}}{a}\right)^2+\frac{k}{a^2}=\frac{\rho+\rho_\Lambda}{3M_\mathrm{PL}^2}\,,
\eeqn 
which is often expressed in terms of the Hubble parameter $H\equiv \dot{a}/a$.
Due to the isotropic ansatz, the $ii$-components of the equations are all equivalent and therefore only provide one additional independent equation. The most common way to present it is by taking the traced Einstein equations and using~(\ref{Friedmann}) to arrive at the acceleration equation,
\beqn\label{acceq}
\frac{\ddot{a}}{a}=-\frac{1}{6M_\mathrm{PL}^2}\left(\rho+\rho_\Lambda+3p\right)\,.
\eeqn
In fact, integrating the acceleration equation~(\ref{acceq}) and using the continuity equation~(\ref{conteq}) gives back the Friedmann equation~(\ref{Friedmann}), where $k$ enters as an integration constant. This is expected because the continuity equation is obtained from taking the divergence of Einstein's equations and is therefore already contained in the equations of motion. To specify a solution it is therefore sufficient to consider only two out of the three equations. 

In order to characterize different components of the cosmological fluid, one introduces the equation of state parameter $w$ defined as the ratio of pressure and energy density, $p=w\rho$. One can then rewrite the continuity equation~(\ref{conteq}) as 
\beqn
\frac{\dd \rho}{\dd a}+3(1+w)\frac{\rho}{a}=0\,,
\eeqn
which is solved by
\beqn
\rho=\rho_0\, a^{-3(1+w)}\,.
\eeqn
Here, $\rho_0$ is a constant to be determined by boundary conditions. Inserting this solution into the Friedmann equation~(\ref{Friedmann}) with $k=0$ and $\rho_\Lambda=0$ gives the following evolution of the scale factor for $w\neq -1$,
\beqn
a~\propto~ t^{\frac{2}{3(1+w)}}\,.
\eeqn
The behaviour for $w=-1$ is
\beqn
a~\propto~ e^{Ht}\,,\qquad H\equiv \frac{\dot{a}}{a}=\mathrm{const}.
\eeqn
Moreover, from the acceleration equation~(\ref{acceq}) we infer that, in the absence of a bare cosmological constant, the expansion of the universe accelerates for $w<-1/3$ and decelerates for $w>-1/3$. Three cases are of particular interest: $w=0$ characterizes nonrelativistic matter, $w=1/3$ corresponds to relativistic matter (``radiation"),  and $w=-1$ describes a cosmological constant. The energy density for nonrelativistic matter therefore scales as $a^{-3}$, i.e.~inversely proportional to the volume. Nonrelativistic matter experiences an additional redshift and its energy density goes as $a^{-4}$. None of these can explain an accelerated expansion of the universe. In contrast, a cosmological constant which of course has constant energy density leads to an exponentially accelerated expansion. 

It is common to measure the contributions of different fluid components in terms of their density parameters,
\beqn
\Omega_i=\frac{\rho_i}{3M_\mathrm{PL}^2 H_0^2},
\eeqn
where $i$ stands for either radiation, nonrelativistic matter or the cosmological constant and $H_0$ denotes the Hubble parameter at the present time. One also defines a curvature contribution, $\Omega_k=-\tfrac{k}{a^2H_0^2}$, and in terms of these the Friedmann equation becomes
\beqn
\Omega_\mathrm{rad}+\Omega_\mathrm{mat}+\Omega_\Lambda+\Omega_k=\frac{H^2}{H^2_0}\,.
\eeqn 
In particular, at the present time the density parameters add up to one. Latest observational data \cite{Hinshaw:2012aka, Ade:2013ktc} suggest the following values for the cosmological parameters at the present time,
\beqn
&~&H_0\sim 70\, \mathrm{km/s/Mpc}\,,\qquad \Omega_\mathrm{rad}\sim 10^{-5}\,,\qquad \Omega_\mathrm{mat}\sim 0.3 \,,\nn\\
&~&\Omega_\Lambda\sim 0.7\,,\qquad\qquad\qquad~~~\,   \Omega_k< 10^{-3}\,.
\eeqn
These values imply that our universe is flat and dominated by a cosmological constant component. As already discussed in the introduction, the energy density corresponding to this cosmological constant is extremely small compared to energy scales of the Standard Model of Particle Physics. Since so far we lack an explanation for this small value, the curious energy component $\rho_\Lambda$ is often referred to as \textit{Dark Energy}. On top of that, observations also show that the matter component $\Omega_\mathrm{m}$ is not dominated by familiar baryonic matter, but rather mainly consists of an unknown \textit{Dark Matter} component. These findings are summarized in the pie chart of Figure~5.1. 
 \begin{figure}[ht]
    \begin{center}
    \includegraphics[width=220pt]{Pictures/WMAP.pdf}
    \caption{Distribution of energy in the present universe. \textit{Credit: NASA/WMAP Science Team.}}
    \end{center}\label{figWMAP}
    \end{figure}
Consequently, under the assumption that General Relativity is indeed the theory of gravity, we must accept that 95$\%$ of the universe's energy content is not at all understood. Nevertheless, when this obscurity is ignored, the so-called $\Lambda$CDM model (GR with a cosmological constant and cold dark matter) fits the observational data very well.

Alternatively, we may question the validity of Einstein's theory of gravity and try to modify it on small distance scales such that it can account for one or both of the dark components in our universe. An example for a consistent infrared modification is bimetric gravity, which motivates us to derive and study the analogue of Friedmann's equation in this model. 

 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Cosmological evolution in bimetric theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In all of this chapter we work with the bimetric action (\ref{HR}) in four dimensions. Furthermore, in order to use the same conventions as in {\protect{\hyperref[papV]{Paper~V}}}, we replace the mass scale $m^4$ by $m^2m_g^2$. 
The coupling of $\fmn$ to matter is set to zero, which is of course a rather restrictive assumption. On the other hand, it allows us to interpret $\gmn$ as the metric in the usual way, provided that it has standard matter couplings.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsection{Homogeneous and isotropic ansatz} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

To keep the comparison of the bimetric solutions to those of General Relativity as simple as possible, we choose to make the usual Friedmann-Robertson-Walker ansatz for the metric $\gmn$ which is coupled to matter,
\beqn\label{FRWg}
\gmn \md x^\mu\md x^\nu=-\md t^2+a(t)^2\left(\frac{1}{1-kr^2}\md r^2+r^2\md \Omega\right)\,,
\eeqn 
It is now important to notice that, in order to arrive at this form, we have used time reparametrizations to remove one time-dependent function in the most general homogeneous and isotropic ansatz. We have therefore fixed the entire diffeomorphism invariance and there is no gauge symmetry left to do the same to $\fmn$.
As a result the most general homogeneous and isotropic ansatz for the second metric reads
\beqn\label{FRWf}
\fmn\md x^\mu\md x^\nu=-X(t)^2\md t^2+Y(t)^2\left(\frac{1}{1-kr^2}\md r^2+r^2\md \Omega\right)\,,
\eeqn
involving two time dependent functions $X(t)$ and $Y(t)$. Note also that we have assumed the curvatures $k$ of the two metrics to be the same. 

Furthermore, we use the perfect fluid form (\ref{setans}) for the stress-energy tensor ${(T^g)^{\mu}}_\nu$ of matter coupled to $\gmn$.
In GR any source is automatically covariantly conserved as a consequence of the Bianchi identity whereas in bimetric gravity the two sources for $\gmn$ and $\fmn$ are not necessarily separately conserved. But since here we have set $T^f_{\mu\nu}=0$, the diffeomorphism invariance of the Einstein Hilbert term and the interaction potential again imply $\nabla_g^\mu T_{\mu\nu}=0$ on-shell. 
This implies that the continuity equation~(\ref{conteq}) is also valid in the model under consideration.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evolution equations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, we consider the bimetric equations of motion, (\ref{geq}) and (\ref{feq}), with one index raised with the respective inverse metrics. Similarly to what we saw in GR, the symmetries of the cosmological ansatz ensure that it is sufficient to work with only part of the equations. Here, these are taken to be the $00$-components of the equations of motion, together with the continuity equation for the source, as well as the Bianchi constraint~(\ref{Bianchi}). The latter needs to be included because now the continuity equation makes up only a part of the divergence of the $\gmn$ equation. The $ii$-components of the equations of motion are then redundant. 

In what follows we shall refer to the $00$-components as simply the $\gmn$ and~$\fmn$ equation. Plugging the ans\"atze of the previous section into (\ref{geq}) we can make use of known GR results to straightforwardly obtain the $\gmn$ equation,
\beqn\label{gmncos}
\left(\tfrac{\dot{a}}{a}\right)^2+\tfrac{k}{a^2}-\tfrac{m^2}{3}\left[\beta_0+3\beta_1\tfrac{Y}{a}+3\beta_2\left(\tfrac{Y}{a}\right)^2+\beta_3\left(\tfrac{Y}{a}\right)^3\right]=\tfrac{\rho}{3m_g^2}\,.
\eeqn
In order to determine how different source components influence the cosmological evolution, we need to determine the function $Y(t)$ from the other equations. We start with the Bianchi constraint~(\ref{Bianchi}), evaluated on the homogeneous and isotropic ansatz, 
\beqn\label{bianchiev}
\tfrac{3m^2}{a}\left[\beta_1+2\beta_2\tfrac{Y}{a}+\beta_3\left(\tfrac{Y}{a}\right)^2\right]\left(\dot{Y}-\dot{a}X\right)=0\,.
\eeqn
There are two options to satisfy this equation; either the first or the second bracket must vanish: 
%%%%%%%%%%%%%%%%
\begin{itemize}

\item[\textbf{(1)}] If the parameters of the theory obey $\beta_1+2c\beta_2+c^2\beta_3=0$ for some constant $c$, then one solution is provided by $Y(t)=c \,a(t)$. In this case, the contribution from the interaction potential in~(\ref{gmncos}) reduces to a cosmological constant term. The $\gmn$ equation hence simply becomes the Friedmann equation~(\ref{Friedmann}) with a cosmological constant $\Lambda=m^2(\beta_0+3c\beta_1+3c^2\beta_2+c^3\beta_3)$. Interestingly, around proportional backgrounds, $\fmn=c^2\gmn$, the Fierz-Pauli mass of the massive perturbation is proportional to the combination of $\beta_n$ parameters in~(\ref{bianchiev}). It therefore vanishes on this particular background if the Bianchi constraint is satisfied by setting the first bracket in~(\ref{bianchiev}) to zero. This may imply an interesting phenomenology for the perturbations, but due to its degeneracy with GR at the background level, the solution is not of great interest to us here. 


\item[\textbf{(2)}] The alternative solution to the Bianchi constraint is $X(t)={\dot{Y}}/{\dot{a}}$. In contrast to the above, this is a dynamical equation and allows for much more general solutions. Since we are mostly interested in solutions that do not show the exact same behaviour as in GR, we focus on this branch in the following. Note also that, in fact, this constitutes no loss of generality because
setting the second bracket in~(\ref{bianchiev}) to zero still includes the proportional spatial metrics as possible solutions.

\end{itemize}
%%%%%%%%%%%%%%%%
Next, we turn to the $\fmn$ equation. Since the ansatz for $\fmn$ contains an extra time-dependent function in the 00-component, the derivative terms in this equation will look more complicated than the expressions familiar from GR. We derive them in the appendix of {\protect{\hyperref[papV]{Paper~V}}}. 
After eliminating $X(t)$ using the solution to the Bianchi constraint, the $\fmn$ equation reads 
\beqn
\left(\tfrac{\dot{a}}{Y}\right)^2+\tfrac{k}{Y^2}-\tfrac{m^2}{3\alpha^2}\left[\beta_1\left(\tfrac{a}{Y}\right)^3+3\beta_2\left(\tfrac{a}{Y}\right)^2+3\beta_3\tfrac{a}{Y}+\beta_4\right]=0\,,
\eeqn
where, as usual,\footnote{Note that in {\protect{\hyperref[papV]{Paper~V}}} the ratio of the Planck masses is denoted by $M_*$ instead of~$\alpha$.} $\alpha\equiv m_f/m_g$.
Multiplying this equation by $Y^2/a^2$ and subtracting it from the $\gmn$ equation (\ref{gmncos}) yields an algebraic equation,
\begin{align}\label{polynom}
\frac{\beta_3}{3}\Upsilon^4+\left(\beta_2-\tfrac{\beta_4}{3\alpha^2}\right)\Upsilon^3&+\left(\beta_1-\tfrac{\beta_3}{\alpha^2}\right)\Upsilon^2\nn\\
&+\left(\rho_*+\tfrac{\beta_0}{3}-\tfrac{\beta_2}{\alpha^2}\right)\Upsilon-\tfrac{\beta_1}{3\alpha^2}=0\,.
\end{align}
We have expressed this in terms of the dimensionless quantities,
\beqn
\Upsilon=\frac{Y}{a}\,,\qquad \rho_*=\frac{\rho}{3m_g^2m^2}\,.
\eeqn
Now we would like to solve equation (\ref{polynom}) for $\Upsilon$ and plug the solution back into the $\gmn$ equation~(\ref{gmncos}). After that, this equation will only contain $a(t)$, $\dot{a}(t)$ and $\rho(t)$ and thus becomes a modified Friedmann equation. The quartic polynomial equation (\ref{polynom}) can be solved numerically for $\Upsilon$. The general solution, however, is not very transparent. Instead, one can fix one or several of the $\beta_n$ parameters and investigate these constrained parameter spaces for simpler solutions. In {\protect{\hyperref[papII]{Paper~II}}}, we focus on parameter choices that allow for solutions close to those of GR.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Degeneracy with General Relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Consider, for example, the choice $\beta_3=0$. In this case, (\ref{polynom}) reduces to a cubic equation for $\Upsilon$ whose solutions will already look simpler. An even greater simplification is achieved if we in addition put $\beta_1=0$. Then the equation for $\Upsilon$ is a quadratic and a solution is readily obtained. Plugging it into the $\gmn$ equation~(\ref{gmncos}) then gives
\beqn\label{deggrcase}
\left(\frac{\dot{a}}{a}\right)^2+\frac{k}{a^2}=\frac{\rho}{3\bar{M}_\mathrm{Pl}^2}+\frac{\rho_\Lambda}{3\bar{M}_\mathrm{Pl}^2}\,,
\eeqn
where we have introduced a modified Planck mass and an effective constant energy density,
\beqn
\bar{M}_\mathrm{Pl}^2=\frac{m_g^2(\beta_4-3\beta_2\alpha^2)}{\beta_4}\,,\quad~~~~ \rho_\Lambda=\frac{m^2(\beta_0\beta_4-9\beta_2^2)}{\beta_4}\,.
\eeqn
Evidently, this is simply the usual Friedmann equation~(\ref{Friedmann}). The bimetric solution in this model is therefore indistinguishable from standard GR cosmology. This is a nontrivial result because the nonlinear theories themselves are very different due to the $\beta_2$-interaction term of bimetric theory. These differences are expected to show up at the level of perturbations. Bimetric perturbation theory around homogeneous and isotropic solutions has been studied in~\cite{Comelli:2012db, Berg:2012kn}. 

Turning on $\beta_1$ takes us smoothly away from the solutions that are degenerate with GR. Consequently, as shown in {\protect{\hyperref[papV]{Paper~V}}}, for small values of $\beta_1$ it is still possible to fit the model to cosmological data. For larger values the predictions of the bimetric model become incompatible with observations.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To summarize, the main conclusion of {\protect{\hyperref[papII]{Paper~II}}} is that there exist nontrivial (i.e.~interacting) models of bimetric gravity with cosmological solutions in agreement with observational data. Hence, the Hassan-Rosen bimetric theory passes one of the first tests for being a valid theory of gravity. In the model where $\beta_1=\beta_3=0$, the cosmological constant is a combination of contributions from the matter source   (which can be absorbed in $\beta_0$) and the bimetric interaction potential. Fitting it to its observed value still involves fine tuning of the parameters and the cosmological constant problem remains unsolved. The situation is somewhat improved for other choices of $\beta_n$, as will be discussed in the next section. 

Another important point is that it is far from clear whether the effective Planck mass in~(\ref{deggrcase}) is the same as the one that would enter spherically symmetric solutions. In GR the Planck mass in Friedmann's equation is the same as the one that enters the gravitational constant in the Newtonian limit and it is this value that has been used to fit the cosmological data. However, if in bimetric gravity the effective Planck mass on cosmological scales turns out to be different than the one on smaller scales, the model would most likely not be compatible with observations. Since so far not much is known about spherically symmetric solutions in bimetric gravity,\footnote{See however \cite{Comelli:2011wq, Volkov:2012wp}, where some progress has been made towards finding spherically symmetric solutions.} this investigation is still an open task.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Self-acceleration}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The purpose of~{\protect{\hyperref[papII]{Paper~II}}} was to demonstrate the existence of viable cosmological solutions in bimetric gravity. A more thorough statistical analysis of the whole parameter space was conducted in~\cite{Akrami:2012vf}. The authors used data from observations of the cosmic microwave background, baryon acoustic oscillations, type Ia supernovae, and the present value of the Hubble parameter to constrain different bimetric models.\footnote{See also~\cite{Akrami:2013ffa} where a similar analysis is performed in a model including matter couplings for $\fmn$ .} In particular, they investigate whether models with $\beta_0=0$ and no cosmological constant contribution from the matter source can give rise an expansion history compatible with observations. In the absence of a constant vacuum energy density driving the acceleration of the universe's expansion, the model has to be \textit{self-accelerating}, i.e.~the observed acceleration must stem from modified terms in Friedmann's equation. Indeed, self-accelerating solutions are found for many different combinations of nonzero $\beta_n$ parameters in bimetric gravity and, in fact, the fits to data are just as good as for the ordinary $\Lambda$CDM model.

The best fit value for the mass of the massive spin-2 field is on the order of the Hubble scale $H_0$. Since in the zero-mass limit the full diffeomorphism symmetry that transforms the two metrics separately is restored, a small spin-2 mass is technically natural. In the ideal case, bimetric theory should also explain why we do not observe the large cosmological constant predicted by quantum field theory, for instance it should provide a mechanism to screen out a large vacuum energy. To our present knowledge, this is not the case, except maybe for the parameters of the partially massless theory, discussed in chapter~\ref{ch:PM}. However, if an explanation for the absence of a large cosmological constant was found elsewhere, the Hubble scale set by the spin-2 mass could be radiatively stable, which would be a large step towards solving the cosmological constant problem.  



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Partially Massless Bimetric Theory}
\label{ch:PM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A massive spin-2 field in de Sitter (dS) background exhibits several interesting features that are neither shared by lower-spin particles nor by spin-2 excitations in flat space. For a special value of the Fierz-Pauli mass in units of the background curvature, the linear theory possesses an additional gauge symmetry which removes one of the spin-2 helicity components. In this case, where the field loses one propagating degree of freedom, it is referred to as \textit{partially massless} (PM). The particular mass value for which this situation occurs is called \textit{Higuchi bound} because it divides the parameter region into unitary and nonunitary subsectors~\cite{Higuchi:1986py}. 
%Below the Higuchi bound the helicity-zero mode of the spin-2 particle develops a ghost instability, whereas above the bound the the theory is healthy. 
%The Higuchi bound is therefore a particularly interesting line in parameter space. 

Being in the possession of a nonlinear theory that involves a massive spin-2 field, we are able to address the following question: Is the concept of partial masslessness restricted to the linear theory around de Sitter backgrounds or can it be extended to the nonlinear level? The demand on a nonlinear PM theory is the presence of an extra gauge symmetry, even away from de Sitter backgrounds. In {\protect{\hyperref[papVI]{Paper~VI}}} we develop a method to identify a unique candidate for a nonlinear PM bimetric theory in four spacetime dimensions. The analysis is extended to higher dimensions in {\protect{\hyperref[papVII]{Paper~VII}}}, where it is found that pure bimetric theory cannot give rise to partial masslessness at the nonlinear level. We therefore modify the bimetric action by adding the Lanczos-Lovelock terms and show that in this generalized framework it again becomes possible to single out PM candidates .




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Partial masslessness in de Sitter background}\label{seclinPM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us begin by reviewing the linear theory of a PM spin-2 particle in a de Sitter background, which was first discussed in a sequence of papers by Deser et.al.~\cite{Deser:1983mm, Deser:2001pe, Deser:2001us, Deser:2001wx, Deser:2001xr, Deser:2004ji, Deser:2006zx}. 
The equation of motion for a massive spin-2 fluctuation $h_{\mu\nu}$ in a de Sitter background $\bar{G}_{\mu\nu}$ with positive cosmological constant $\Lambda$ is given by
\beqn\label{lineqds}
{\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}h_{\rho\sigma}-\tfrac{2\Lambda}{d-2}\left(h_{\mu\nu}-\tfrac{1}{2}\bar{G}_{\mu\nu} h\right)
+\tfrac{m^2_\mathrm{FP}}{2}\Big(h_{\mu\nu}-\bar{G}_{\mu\nu} h\Big)=0\,,
\eeqn
where the derivative operator ${\bar{\mathcal{E}}_{\mu\nu}}^{\rho\sigma}$ is given in (\ref{kinopds}). For general values of the Fierz-Pauli mass, the equation possesses no gauge symmetries. Similarly to its analogue in flat space that was discussed in detail in section~\ref{sec:FP}, it contains $d+1$ constraint equations that reduce the number of propagating degrees of freedom to $(d(d-1)/2-1)$, appropriate for a massive spin-2 particle.

A feature of (\ref{lineqds}) without any analogue in flat space is that if the Fierz-Pauli mass saturates the Higuchi bound, $m^2_\mathrm{FP}=\frac{2}{d-1}\Lambda$, the equation is invariant under a new gauge symmetry. The corresponding linear gauge transformation reads
\beqn\label{linPMsym}
\Delta (\hmn) = \bar{\nabla}_\mu\partial_\nu\xi(x)+\tfrac{2\Lambda}{(d-1)(d-2)} \bar{G}_{\mu\nu}\, \xi(x)\,,
\eeqn
in which $\xi(x)$ is a local gauge parameter.
Moreover, if the value for the mass lies below the bound, the theory is nonunitary because the helicity-zero mode of the massive spin-2 field becomes a ghost \cite{Higuchi:1986py, Higuchi:1989gz}. Above the Higuchi bound the theory is well-behaved. 

Besides computing the variation of~(\ref{lineqds}) under the gauge transformation explicitly, there is another straightforward way to see the existence of a gauge symmetry in the equation for the massive spin-2 field with mass at the Higuchi bound. First take the double divergence of~(\ref{lineqds}) to arrive at
\beqn\label{doublediv}
\bar{\nabla}_\nu\bar{\nabla}_\mu\left(\bar{G}^{\mu\nu} \bar{G}^{\rho\sigma}-\bar{G}^{\mu\rho}\bar{G}^{\nu\sigma}\right)h_{\rho\sigma}=0\,.
\eeqn
The kinetic terms have dropped out after using the linearized Bianchi identity.
Furthermore, the trace of (\ref{lineqds}) is given by
\beqn
\tfrac{d-2}{2}\,\bar{\nabla}_\nu\bar{\nabla}_\mu\left(\bar{G}^{\mu\nu} \bar{G}^{\rho\sigma}-\bar{G}^{\mu\rho}\bar{G}^{\nu\sigma}\right)h_{\rho\sigma}+\left(\Lambda-\tfrac{d-1}{2}m^2_\mathrm{FP}\right)h=0\,.
\eeqn
If the mass is at the Higuchi bound, the terms without derivatives in this equation vanish identically, while the derivative terms are zero due to~(\ref{doublediv}).
Hence we find that for $m^2_\mathrm{FP}=\frac{2}{d-1}\Lambda$ the traced equations of motion are identical to their double divergence. Put differently, when multiplied by the appropriate factors, the difference of the trace and the double divergence is identically zero.
This identity signals the presence of a gauge symmetry. Since one particular combination of the equations of motion is identically satisfied, one component of $\hmn$ remains undetermined.  
In fact, a gauge identity of the above type even implies that the action is invariant under the corresponding gauge transformation. This follows from the fact that invariance of the action under~(\ref{linPMsym}) requires
\beqn
\Delta S=\frac{\delta S}{\delta \hmn}\Delta (\hmn)=0\,.
\eeqn
Since $\tfrac{\delta S}{\delta \hmn}$ is nothing else than the equation of motion for $\hmn$, after integrating by parts, we find that $\Delta S$ indeed vanishes due to the gauge identity. 

The conclusion is that the massive spin-2 field described by (\ref{lineqds}) with mass at the Higuchi bound has only $(d(d-1)/2-2)$ degrees of freedom, one less than is usually the case. Let us also remark that the existence of the gauge symmetry around de Sitter backgrounds is in agreement with the representation theory of the de Sitter group SO$(1,d)$, which allows for so-called \textit{partially massless} (PM) representations of higher-spin fields. For a discussion of this topic, consult e.g.~\cite{Garidi:2003ys}. The whole situation is summarized in Figure~6.1, where for definiteness we fix $d=4$.
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=200pt]{Pictures/dSPM.pdf}
    \caption{Unitary and nonunitary regions in the $\Lambda$-$m_\mathrm{FP}^2$-plane in $d=4$. The boundary of the shaded region corresponds to the Higuchi bound.}
    \end{center}
    \end{figure}

After the linear PM theory for spin-2 fields on de Sitter background had been established, it was attempted to construct higher order interactions for the perturbation $\hmn$ that would leave the gauge symmetry intact. At cubic order in $\hmn$ such a construction turned out to be possible in $d=4$~\cite{Zinoviev:2006im, Joung:2012rv}. In $d>4$, however, it was found that gauge invariant cubic vertices can only exist if one also includes higher derivative terms into the theory \cite{Zinoviev:2006im}. The construction of a fully nonlinear theory with a PM gauge symmetry remained an open task.



The remainder of this chapter summarizes the findings of {\protect{\hyperref[papVI]{Paper~VI}}} and {\protect{\hyperref[papVII]{Paper~VII}}} where we propose a nonlinear PM theory within the family of ghost-free bimetric theories. In particular, we show that in this framework it is possible to understand the outcome of the cubic-vertex analyses of~\cite{Zinoviev:2006im, Joung:2012rv}. We begin by explaining the properties of the candidate PM theory for the most relevant case of four space-time dimensions, before we generalize the arguments to $d>4$. Further remarkable features of the theory in $d=4$ will be presented in chapter~\ref{ch:HD} in the context of higher-curvature actions.


 
  
   
   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
\section{Towards a nonlinear PM theory}\label{secPmnonlin}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
It is natural to expect the nonlinear PM theory (if it exists) to be found within the family of ghost-free nonlinear theories for massive spin-2 fields. A first investigation of this possibility was carried out in \cite{deRham:2012kf} where the authors aimed to identify a PM theory in nonlinear Massive Gravity with the reference metric taken to be a fixed de Sitter background. Their construction used St\"uckelberg fields in a generalized decoupling limit and showed that, for a certain choice of the $\beta_n$-parameters, a scalar degree of freedom is not propagating. Although this seemed to be a solid argument for the presence of a gauge symmetry in the decoupling limit, it was later argued in \cite{Deser:2013uy, deRham:2013wv} that constructing a PM theory in the full theory of nonlinear Massive Gravity is impossible. Inspite of lacking a proof, another article also made similar negative statements about PM bimetric theory~\cite{Deser:2013gpa}.

Taking into account these objections, one could be worried about the possibility of constructing a PM bimetric theory. 
However, there are several reasons why the above no-go results need not concern us here:
First of all, the results of \cite{Deser:2013uy, deRham:2013wv} hold only for nonlinear Massive Gravity with fixed reference metric $\fmn$, and do not directly carry over to the ghost-free bimetric gravity where both metrics are dynamical. In fact, the analyses in these references merely show that in a nonlinear PM theory none of the metrics can be held fixed because both of them are expected to transform under the PM gauge symmetry. We will come back to this point in section~\ref{sec:PMMG}. Apart from this, the authors of \cite{Deser:2013uy, Deser:2013gpa} search for a nonlinear action with invariance under an infinitesimal PM gauge transformation and are unable to find it. The action will, however, not be invariant if the invariance is an on-shell symmetry of the equations of motion. In fact, it is possible to use the results we derive below to demonstrate that the nonlinear PM theory can only be invariant on-shell. This is part of an upcoming publication and beyond the scope of this thesis. However, we emphasize one more time that the no-go results of \cite{Deser:2013uy, deRham:2013wv, Deser:2013gpa} simply do not apply to the theory under consideration here.





In {\protect{\hyperref[papVI]{Paper~VI}}} we develop a method that allows us to identify a candidate PM theory within the family of ghost-free bimetric theories. To this end, we consider the proportional background solutions as well as the spectrum of linear perturbations around these that were discussed in section~\ref{sec:massspec}. This is a natural setup for extending the PM symmetry of perturbations around dS space because these backgrounds have constant curvature and, in particular, they are the only ones around which a massive fluctuation with Fierz-Pauli mass term exists. Our method is suitable for identifying or excluding PM candidates in bimetric theory in any space-time dimension. In this section, however, after outlining the general idea, we restrict to the case $d=4$. Dimensions greater than four will be the focus of section~\ref{PMdgf}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Identifying PM candidates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The equation of motion (\ref{dMeq}) for the massive fluctuation $\delta M_{\mu\nu}$ around proportional backgrounds is of the same form as (\ref{lineqds}) with $\Lambda=\bar{\Lambda}_g$.  
As a consequence, if the cosmological constant is assumed to be positive and if the Fierz-Pauli mass (\ref{FPmass}) is on the Higuchi bound, a gauge symmetry of the form (\ref{linPMsym}) is present in the linear theory around proportional backgrounds. In bimetric notation, the corresponding infinitesimal gauge transformation of the massive fluctuation reads
\beqn\label{linPMsym2}
\Delta (\delta M_{\mu\nu}) = \bar{\nabla}_\mu\partial_\nu\xi(x)+\tfrac{2\bar{\Lambda}_g}{(d-1)(d-2)} \bar{G}_{\mu\nu}\, \xi(x)\,.
\eeqn
On the other hand, the massless fluctuation does not transform under the PM symmetry, 
\beqn
\Delta (\delta G_{\mu\nu}) = 0\,.
\eeqn
This follows from the fact that its equation of motion (\ref{dGeq}) does not have any extra gauge symmetry besides the usual linearized diffeomorphism invariance. Therefore, $\delta G_{\mu\nu}$ itself must be invariant under the PM symmetry. 
The question is now under what conditions the above symmetry transformations for the fluctuations around dS background have a chance to be generalizable to the nonlinear level. 

Since the theory in terms of the nonlinear fields $M^G_{\mu\nu}$ and $G_{\mu\nu}$ has a very complicated form, we find it easier to work with the variables $\gmn$ and $\fmn$ instead. 
The above transformations of the mass eigenstates $\delta M_{\mu\nu}$ and $\delta G_{\mu\nu}$ allow us to uniquely determine the transformations of the fluctuations of $\gmn$ and $\fmn$ using the expressions for the massive and massless fluctuations given in (\ref{dGanddM}). The result is
\beqn\label{fgtrans}
\Delta (\delta\gmn)=-(\alpha c)^{\frac{d-2}{2}}\Delta (\delta\fmn)=\tfrac{-2(\alpha c)^{d-2}}{c(1+(\alpha c)^{d-2})}\Delta (\delta M_{\mu\nu})\,.
\eeqn
The crucial observation is now that in a theory with a gauge symmetry at the nonlinear level, it must be possible to shift these transformations of the fluctuations $\delta\gmn$ and $\delta\fmn$ to the backgrounds $\bgmn$ and $\bfmn$. This follows from the fact that the split into background and fluctuations is not unique and one can always take out part of the fluctuation to redefine the background. Therefore we demand that the symmetry transformations (\ref{fgtrans}) should also leave the background equations invariant. But since we are dealing with the proportional backgrounds, where the background equation is simply $\Lambda_g=\Lambda_f$ (c.f.~(\ref{propbackeq})), determining the proportionality constant $c^2$, we restrict ourselves to constant gauge transformations $\bar{\Delta}$ with $\xi(x)=$\,const. In this way we ensure that the transformation does not take us away from the proportional backgrounds and avoid unnecessary complication. 
The restriction to constant gauge transformations is a strong simplification, but as we will see now, demanding the background equation to be invariant under these is constraining enough to identify the PM candidate theory. Namely, it should be evident from (\ref{fgtrans}) that shifting the constant transformations to the backgrounds $\bgmn$ and $\bfmn=c^2\bgmn$ results in a shift in $c^2$,
\beqn
\bgmn\bar{\Delta}(c^2)= \bar{\Delta}(\bfmn)-c^2\bar{\Delta}(\bgmn)\,.
\eeqn
However, in general this cannot lead to an integrable\footnote{Integrability of the symmetry transformation means that it can be performed more than once and still leave the equations invariant. This is a natural requirement on any gauge symmetry. Without the integrability condition it is sufficient to set the mass to the Higuchi bound in order to have an invariant background.} symmetry of the background equations because $c$ is determined by $\Lambda_g=\Lambda_f$ and can therefore not be shifted. 
If this is the case, then a nonlinear PM symmetry cannot exist. The only possibility to avoid this immediate no-go statement is to demand that $c$ is not fixed by the background equation. 
Then, the equation $\Lambda_g=\Lambda_f$ that is automatically satisfied in this case (i.e.~without fixing $c$) is the gauge identity evaluated on the proportional backgrounds. Since making the proportional ansatz for the two metrics partly fixes the gauge, only constant scalings are left as residual transformations. The component of the metrics that remains undetermined by the equations therefore simply reduces to the constant $c$ on this solution. 

 
The whole idea will be made more explicit in the following, where we identify PM candidates in $d=4$, before we discuss the general case in the next section.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{PM candidate in $d=4$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In four space-time dimensions, the explicit expressions~(\ref{lambdas}) for the cosmological constants in terms of the $\beta_n$ parameters, the ratio of Planck masses $\alpha$ and the proportionality constant $c$ can be used to write the background condition $\Lambda_g=\Lambda_f$ as a polynomial equation for $c$,
\begin{align}
\beta_1+c(3\beta_2-\alpha^2\beta_0)&+3c^2(\beta_3-\alpha^2\beta_1)\nn\\
&+c^3(\beta_4-3\alpha^2\beta_2)-c^4\alpha^2\beta_3=0\,.
\end{align}
This equation clearly fixes $c$ unless all coefficients of different powers of $c$ vanish separately. A proportionality constant $c$ that is undetermined by the background equation therefore requires the following parameter choices in the bimetric interaction potential,
\beqn\label{PMpara}
\beta_1=\beta_3=0\,,\qquad \alpha^2\beta_0=3\beta_2=\alpha^{-2}\beta_4\,.
\eeqn
We will frequently refer to these values as the \textit{PM parameters}. Note that our requirement on the $\beta_n$-parameters fixes all but one of them uniquely in terms of the others and $\alpha$. The one remaining parameter is of course degenerate with the energy scale $m^4$ in the interaction potential and sets the scale for the Fierz-Pauli mass and the cosmological constant. Moreover, it is easy to check using the expressions (\ref{FPmass}) and (\ref{lambdas}) for $m_\mathrm{FP}^2$ and $\Lambda_g$, that the parameter choice (\ref{PMpara}) automatically puts the mass on the Higuchi bound. Therefore the theory of linear perturbations around the backgrounds at hand exhibits the usual PM gauge symmetry. It is worth emphasizing that we did not demand this in any way; it followed from an independent requirement on the background equations. 

On the other hand, we also make the following interesting observation: If we assume that there is a \textit{unique} PM theory, then satisfying the Higuchi bound is sufficient to determine its parameters. Namely, in this case, the symmetry (\ref{symbg}) of the interaction potential enforces $\alpha^{4-n}\beta_n=\alpha^{n}\beta_{4-n}$ because otherwise the theory obtained from replacing $\alpha^{4-n}\beta_n\rightarrow\alpha^{n}\beta_{4-n}$ would also be PM, contradicting the uniqueness requirement.
It is easy to see that this constraint on the $\beta_n$ parameters together with the Higuchi bound condition already implies (\ref{PMpara}).

We now turn to the requirement of integrability of the symmetry transformation. The constant parts of the PM symmetry transformations of the fluctuations can be written as 
\beqn\label{consttraf}
\Delta (\delta\gmn)=-\frac{2c\alpha^2}{1+(\alpha c)^2}\delta a\,\bgmn\,,\qquad \Delta (\delta\fmn)=\frac{2c}{1+(\alpha c)^2}\delta a\,\bgmn\,,
\eeqn
with  infinitesimal constant gauge parameter $\delta a$.
Furthermore, it is easy to check that with the PM parameters the background equations (\ref{bgeq}) are invariant under the nonlinear scaling transformations,
\beqn
\bgmn\rightarrow\frac{1+(\alpha c)^2}{1+\alpha^2(c+a)^2}\,\bgmn\,,\qquad \bfmn\rightarrow\frac{1+(\alpha c)^{-2}}{1+\alpha^{-2}(c+a)^{-2}}\,\bfmn
\eeqn
with finite constant gauge parameter $a$. Of course, these are simply the integrated versions of (\ref{consttraf}), verifying that the constant part of the gauge transformation is indeed integrable.
If the nonlinear PM symmetry exists, the above transformations constitute its form on the proportional backgrounds.

It is furthermore important to note that the Fierz-Pauli mass and cosmological constant, when taken with respect to the background metric~$\bar{G}_{\mu\nu}$, become independent of $c$,
\beqn
\bar{m}_\mathrm{FP}^2=\frac{2}{3}\bar{\Lambda}_g=2\beta_2\frac{m^4}{m_g^2}\,.
\eeqn
Hence, these can be regarded as physical quantities that do not depend on the gauge parameter $a$ that shifts the value of $c$.



By restricting to constant gauge transformations, clearly, we are not dealing with the full PM symmetry at the nonlinear level. Note, however, that since the set of constant transformations is a subset of the full gauge group, the theory we obtain by requiring invariance under this subset must contain the theory with the full gauge group (if it exists). Moreover, since in four dimensions the restriction to constant gauge transformations is sufficient to uniquely determine the $\beta_n$ parameters, we conclude that the resulting theory is already the unique candidate for having the full PM symmetry.

The scale invariance of the equations of motion for proportional backgrounds is not the only interesting property of the theory specified by the PM parameters. The PM candidate exhibits additional astonishing features that further support the existence of a gauge symmetry at the nonlinear level. For instance, consider again the homogeneous and isotropic solutions of {\protect{\hyperref[papII]{Paper~II}}} which we presented in chapter~\ref{ch:cosmo}. We saw that, after solving the Bianchi constraint, it was possible to arrive at (\ref{polynom}), an algebraic equation for the ratio of the two scale factors, $Y(t)/a(t)$. Inserting the PM parameters (\ref{PMpara}) into this equation, we find that it becomes an identity. Clearly, it is the analogue of the equation $\Lambda_g=\Lambda_f$ for proportional backgrounds. But instead of a constant, the equations evaluated on the cosmological ansatz now leave a time-dependent function undetermined. This shows that the cosmological evolution equations of PM bimetric theory are invariant under a symmetry that is local in time. Even if it eventually turns out that a PM symmetry does not exist in the nonlinear theory, a cosmological gauge symmetry could already be of interest on its own. 

Since, in four dimensions, the proportional backgrounds correspond to maximally symmetric space-times with ten independent Killing vectors and the homogeneous and isotropic solutions still possess six isometries, one might speculate that the presence of a symmetry on these solutions could somehow be related to the amount of symmetry of the underlying geometry. Then one could argue that a general solution with less symmetries than the above would not be invariant under any PM symmetry transformation. To invalidate this argument, it is therefore important to investigate the structure of our PM candidate theory away from the proportional and the cosmological backgrounds. This has been done in {\protect{\hyperref[papVIII]{Paper~VIII}}} which considers general perturbative solutions to the bimetric equations of motion. It turns out that the equations in the PM theory are conformally invariant to lowest order in a derivative expansion.
These remarkable results will be presented in section~\ref{secPMCG}.



To conclude this discussion, let us briefly mention that a PM candidate can also be obtained in $d=3$ where the background equation reads
\beqn
c(\beta_1-\alpha\beta_0)+2c^2(\beta_2-\alpha\beta_1)+c^3(\beta_3-\alpha\beta_2)=0\,.
\eeqn
Demanding this to leave $c$ undetermined results in the following PM parameters, 
\beqn
\beta_3=\alpha\beta_2=\alpha^2\beta_1=\alpha^3\beta_0\,.
\eeqn
Again, all but one of the $\beta_n$ parameters are fixed, and the Fierz-Pauli mass sits precisely on the Higuchi bound. 


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Massive gravity limit}\label{sec:PMMG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The PM parameters (\ref{PMpara}) in four space-time dimensions provide an example for a theory in which the coefficients in the interaction potential depend on the mass scale $m_f$ that is taken to infinity in the massive gravity limit that we discussed in section~\ref{sec:MGlim}. In this case, we have to be more careful when taking the limit because the $\beta_n$ parameters will scale as well. The conditions (\ref{PMpara}) fix the relative scale among them but their absolute scale may still be chosen freely. Suppose that $\beta_2$ does not scale when the limit $\alpha=m_f/m_g\rightarrow\infty$ is taken. Then $\beta_0\rightarrow 0$ and $\beta_4\rightarrow\infty$, whereas $\Lambda={\beta_4\,m^4}/{m_f^2}=\,$const.  In the Massive Gravity limit, the equations of motion for the PM theory thus reduce to
\beqn
\mathcal{G}_{\mu\nu}(g)
+\frac{\Lambda}{3}\,g_{\mu\lambda}{\big(Y^{(2)}\big)^\lambda}_{\nu}(S)&=&0\,, \label{gpm} \\
\mathcal{G}_{\mu\nu}(f)
+\Lambda\fmn&=&0 \,.\label{fpm}
\eeqn
Remarkably, these are exactly the equations singled out in \cite{deRham:2012kf, Deser:2013uy, deRham:2013wv} which investigated the possibility of realizing nonlinear partial masslessness in Massive Gravity with fixed reference metric. The methods invoked in those references are completely different from ours and hence provide independent support for the existence of a nonlinear PM symmetry. 

On the other hand, as we already mentioned previously, in \cite{Deser:2013uy, deRham:2013wv} it was also claimed that there is no nonlinear gauge symmetry present in (\ref{gpm}) and (\ref{fpm}). If correct, at first sight, this result might seem to rule out a nonlinear PM symmetry even in bimetric gravity because it should be possible to take the massive gravity limit to arrive at the above equations. There is, however, a caveat in this argument: If the symmetry transformation in PM bimetric gravity itself depends on $\alpha=m_f/m_g$, then it may become singular in the $\alpha\rightarrow\infty$ limit. In this case, it would not be consistent to only look for an invariance in (\ref{gpm}) and (\ref{fpm}) because terms in the original bimetric equations, that were neglected when taking the limit, could become relevant again due to the singular nature of the gauge transformation. In fact, our findings in chapter~\ref{ch:HD} suggest that the transformation of $\fmn$ indeed contains such singular terms and therefore the conclusions of \cite{Deser:2013uy, deRham:2013wv} are irrelevant for bimetric gravity. 


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
\section{Generalization to arbitrary dimensions}\label{PMdgf}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


In {\protect{\hyperref[papVII]{Paper~VII}}} we apply the procedure of identifying the candidate PM theories that we introduced in the previous section to bimetric theory in an arbitrary number of space-time dimensions. We find that in pure Hassan-Rosen bimetric theory there is no nonlinear PM theory for $d>4$. This outcome is in agreement with 3-vertex calculations~\cite{Zinoviev:2006im, Joung:2012rv}, which also suggest that it could be possible to find a nonlinear PM theory in higher dimensions if higher order derivative couplings are included into the theory. Inspired by these results we augment the bimetric action by the ghost-free Lanczos-Lovelock (LL) terms. In this LL-extended bimetric theory it is then possible to identify PM candidates even for $d>4$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background equation}\label{noPMdgeq5}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Let us first argue why in pure bimetric theory there is no PM candidate in dimensions greater than four. To this end, consider again the background equation $\Lambda_g=\Lambda_f$ which in $d$ dimensions assumes the following form,
\beqn\label{eqlad}
(\alpha c)^{d-2}\sum_{n=0}^{d-1}{d-1\choose n}c^n\beta_n
= \sum_{n=1}^{d}{d-1\choose n-1}c^n\beta_n\,.
\eeqn
As in the four-dimensional case, for $c$ to be undetermined by this polynomial equation, the coefficients of different powers of $c$ have to vanish separately. This requirement will again put constraints on the $\beta_n$-parameters and the ratio of Planck masses $\alpha$. It should be obvious that, for large $d$, the factor $c^{d-2}$ on the left-hand side produces a large number of terms with coefficients proportional to just one $\beta_n$-parameter. These $\beta_n$-parameters will then immediately forced to be zero. 
Explicitly, when multiplied by $c^{2-d}$, the above equation can be rewritten as
\beqn
\left( \alpha^{d-2}\sum_{n=0}^{d-1}{d-1\choose n}\beta_n-\sum_{n=3-d}^2{d-1\choose d+n-3}\beta_{n+d-2} \right)c^n=0\,.
\eeqn
In $d\geq 5$, demanding the coefficients of $c^n$ to vanish for $3-d\leq n\leq d-1$ then leads to the following constraints on the parameters,
\begin{align}
0&=\alpha^{d-2}{d-1\choose n}\beta_n-{d-1\choose d+n-3}\beta_{n+d-2} \qquad\text{for}\quad0\leq n\leq 2\,.,\nn\\
0&=\beta_m\qquad\text{for}\quad 1\leq m\leq d-1\,.
\end{align}
The second set of conditions inserted into the first also gives $\beta_0=\beta_d=0$ and hence for $d\geq 5$ all $\beta_n$ must vanish. This choice of parameters of course trivializes the interaction potential. Our conclusion therefore is that there exist no nontrivial parameter values for which the constant part of the gauge transformation leaves the background equations invariant. Hence there is no PM candidate in pure bimetric theory in dimensions greater than four. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bimetric theory with Lanczos-Lovelock terms}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

According to the constructive consistency proof in chapter~\ref{ch:MG}, the interaction potential of the Hassan-Rosen bimetric theory includes all  consistent non-derivative terms. Therefore, the only option to obtain an extended version of the theory is to add more derivative terms to the action. At this point, the only such terms that are expected to be ghost-free consist of the Lanczos-Lovelock invariants which are defined as totally antisymmetric contractions of Riemann tensors $R^{\alpha\beta}_{\phantom{\alpha\beta}\mu\nu}$,
\beqn\label{LLdef}
\mathcal{L}_{(n)}=\frac{1}{2^nn!}\delta^{\mu_1}_{[\alpha_1}\delta^{\nu_1}_{\beta_1}\hdots\delta^{\mu_n}_{\alpha_n}\delta^{\nu_n}_{\beta_n]}
\prod_{k=1}^nR^{\alpha_k\beta_k}_{\phantom{\alpha_k\beta_k}\mu_k\nu_k}\,.
\eeqn
In spite of being higher derivative operators, the LL invariants are believed to avoid inconsistencies that are usually introduced by such terms. This is due to the antisymmetric structure in (\ref{LLdef}) which ensures the absence of more than two time derivatives acting on one field in the action. It is interesting that the same structure appears in the interaction potential of ghost-free bimetric theory, but of course this is not really a coincidence: In the decoupling limit of nonlinear massive gravity it can be seen that the antisymmetric structure removes higher time derivatives from the longitudinal modes of the St\"uckelberg fields.  

Hoping to rediscover the possibility of finding PM candidates in $d>4$, we thus choose to extend the Hassan-Rosen bimetric action by the following terms,\footnote{In a different context, consistent bimetric theory extended by LL terms has already been considered in~\cite{Paulos:2012xe}.}
\begin{align}\label{LLaction}
S_\mathrm{LL}~&=~~m_g^{d-2}\int\dd^dx\sum_{n=2}^{[d/2]}\sqrt{-g}~l_n^g\,\mathcal{L}_{(n)}(g)\nn\\
&~+~m_f^{d-2}\int\dd^dx\sum_{n=2}^{[d/2]}\sqrt{-f}~l_n^f\,\mathcal{L}_{(n)}(f)\,,
\end{align}
where we have introduced two sets of couplings, $l_n^g$ and $l_n^f$, of mass dimension $2(1-n)$.
Furthermore, it is well known that the LL invariant $\mathcal{L}_{(n)}$ is topological in $d=2n$ and vanishes for $2n>d$ which is why the sums in (\ref{LLaction}) terminate at integer part of $d/2$. 



The equations of motion for $\gmn$ and $\fmn$ that follow from the LL extended bimetric action are
\beqn\label{LLeom}
\mathcal{G}_{\mu\nu}(g)+\sum_{n=2}^{[d/2]}l_n^g\mathcal{G}^{(n)}_{\mu\nu}(g)+\frac{m^d}{m_g^{d-2}}V^g_{\mu\nu}&=&0\,, \nn\\
\mathcal{G}_{\mu\nu}(f)+\sum_{n=2}^{[d/2]}l_n^f\mathcal{G}^{(n)}_{\mu\nu}(f)+\frac{m^d}{m_g^{d-2}}V^f_{\mu\nu}&=&0\,.
\eeqn
Here, $\mathcal{G}^{(n)}_{\mu\nu}$ are the Lovelock tensors that follow from variation of (\ref{LLaction}) and $V^g_{\mu\nu}$ and $V^f_{\mu\nu}$ are the contributions from the interaction potential which were defined in (\ref{poteom}). We will not need the explicit expressions for the Lovelock tensors, but let us note the important property,
\beqn\label{usefid}
g^{\mu\nu}\mathcal{G}^{(n)}_{\mu\nu}(g)=\frac{2n-d}{2}\mathcal{L}_{(n)}(g)\,,
\eeqn
which will be useful in what follows.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proportional backgrounds}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As in pure bimetric theory we are interested in the proportional background solutions to (\ref{LLeom}) and perturbations around those. Again, these backgrounds correspond to maximally symmetric spacetimes, for which the curvatures satisfy
\beqn\label{bgcurv}
R_{\mu\nu\rho\sigma}(\bar{g})&=&\frac{2\lambda}{(d-1)(d-2)}(\bar{g}_{\mu\rho}\bar{g}_{\nu\sigma}-\bar{g}_{\nu\rho}\bar{g}_{\mu\sigma})\,,\nn\\
R_{\mu\nu}(\bar{g})&=&\frac{2\lambda}{d-2}\bgmn\,,\qquad R(\bar{g})~=~\frac{2d\,\lambda}{d-2}\,,
\eeqn
with cosmological constant $\lambda$. On such backgrounds with constant curvature, the $n$-th order LL invariant is proportional to $\lambda^n$,
\beqn\label{LLbg}
\mathcal{L}_{(n)}=N_n(d)\,\lambda^n\,,\quad\text{with}~~N_n(d)\equiv\frac{2^n d!}{(d-1)^n(d-2)^n(d-2n)!}\,.
\eeqn
Next, we trace the equations of motion (\ref{LLeom}) in order to obtain two scalar equations and insert (\ref{bgcurv}) for the curvatures.
Furthermore, we make use of the identity (\ref{usefid}) and plug in the proportional ansatz, $\bfmn=c^2\bgmn$. 
Finally, in the equation for $\fmn$, we use $\mathcal{L}_{(n)}(c^2 \bar{g})=c^{-2n}\mathcal{L}_{(n)}( \bar{g})$. The resulting two equations read
\beqn\label{LLbgeq}
\lambda + \sum_{n=2}^{[d/2]}l^g_n\frac{d-2n}{2d}N_n(d)\lambda^n - \Lambda_g&=&0\,,\nn\\
\lambda + \sum_{n=2}^{[d/2]}c^{2-2n}l^f_n\frac{d-2n}{2d}N_n(d)\lambda^n - \Lambda_f&=&0\,.
\eeqn
Here, $\Lambda_g$ and $\Lambda_f$ are the contributions from the potential evaluated on the proportional backgrounds which defined earlier in (\ref{lambdas}). Note, however, that these no longer correspond to the physical cosmological constants and are not necessarily equal. 

For general parameters $\beta_n$, $l_n^g$, and $l_n^f$, the two algebraic equations in (\ref{LLbgeq}) serve to determine the background curvature $\lambda$ as well as the proportionality constant $c^2$. Note also that in the absence of the LL contributions, i.e.~for $l_n^g=l_n^f=0$, we rearrive at the bimetric background equations, $R(\bar{g})=\tfrac{2d}{d-2}\Lambda_g$ and $\Lambda_g=\Lambda_f$. Eventually, we will again be looking for the parameter values for which the equations (\ref{LLbgeq}) leave $c$ undetermined.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear Perturbations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Computing the linearized equations of motion from (\ref{LLeom}) is quite involved. Fortunately, it has been observed in \cite{Sisman:2012rc} that, around constant curvature backgrounds with cosmological constant $\lambda$, the fluctuation equations of General Relativity augmented by the LL terms with couplings $l_n^g$ assume the same form as the ones obtained from Einstein's equations. The only difference is that, in the linearized equations of the LL extended theory, the Planck mass $m_g$ needs to be replaced by an effective mass parameter $\tilde{m}_g$ defined through
\beqn\label{modmg}
\frac{\tilde{m}_g^{d-2}}{m_g^{d-2}}=1+(d-3)!\sum_{n=2}^{[d/2]}\frac{n(d-2n)l_n^g}{(d-2n)!}\left(\frac{2\lambda}{(d-1)(d-2)}\right)^{n-1}.
\eeqn
It is a remarkable feature of the Lovelock invariants that, in spite of being higher-derivative operators in the nonlinear theory, they give rise to linearized equations that are only second order in derivatives.

For the bimetric case the above result implies that the linear equations for the theory with LL terms are the same as in pure bimetric theory if one replaces $m_g$ by $\tilde{m}_g$ as above and $m_f$ by $\tilde{m}_f$ given by
\beqn\label{modmf}
\frac{\tilde{m}_f^{d-2}}{m_f^{d-2}}=1+(d-3)!\sum_{n=2}^{[d/2]}\frac{n(d-2n)c^{2-2n}l_n^f}{(d-2n)!}\left(\frac{2\lambda}{(d-1)(d-2)}\right)^{n-1}.
\eeqn
Hence, thanks to the results of~\cite{Sisman:2012rc}, without any computation we can conclude that the linear equations in a maximally symmetric background with cosmological constant $\lambda$ will again diagonalize into a massless and massive equation, where in the latter the Fierz-Pauli mass (\ref{FPmass}) is now given in terms of $\tilde{m}_g$ and $\tilde{m}_f$. Due to this similarity, the linear equations are again invariant under the usual PM symmetry (\ref{linPMsym}) if the mass is on the Higuchi bound, $m_{\mathrm{FP}}^2=\frac{2}{d-1}\lambda$. One can then hope that it is possible to find a nonlinear candidate PM theory within this generalized setup.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{PM candidates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We apply the same logic as in the four-dimensional case to LL extended bimetric theory:
For extending the linear PM symmetry to the nonlinear level, we need to be able to shift the proportionality constant $c^2$ and hence, in a PM candidate theory, the background equations (\ref{LLbgeq}) must not determine it. In order to see for which parameter values this is possible, we must first solve a combination of the two equations for $\lambda$, eliminate it from the remaining equation, and demand the result to be independent of $c$. 

Although this procedure sounds again straightforward, in practice, it cannot always be carried out immediately. Complications arise because the background equations (\ref{LLbgeq}) are polynomials of order $[d/2]$ in $\lambda$ and solving them does not result in a polynomial expression for $\lambda$ as a function of $c$. Therefore, generically, the equation that is supposed to leave $c$ undetermined is not a polynomial in $c$ and it becomes difficult to impose the requirement on the PM theory. 

Nevertheless, for small enough $d$ it is possible to arrive at a polynomial equation in $c$ and the analysis can be carried out. As an example, we present the analytical results in $d=5$ before summarizing the outcome of a computer-based analysis for dimensions up to $d=8$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Partial masslessness in $d=5$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In five space-time dimensions the equations are still simple enough to be solved by hand. The only nontrivial LL term is $\mathcal{L}_{(2)}$, also known as the Gauss-Bonnet combination,
\beqn\label{gaussbonnet}
\mathcal{L}_{(2)}=R^2-4R_{\mu\nu}R^{\mu\nu}+R_{\mu\nu\rho\sigma}R^{\mu\nu\rho\sigma}\,,
\eeqn
which is topological in $d=4$. 
When terms of this kind for both $\gmn$ and $\fmn$ are added to the bimetric action, the background equations (\ref{LLbgeq}) take the following form,
\beqn\label{bgeqLL5}
\lambda+\frac{l_2^g}{3}\lambda^2-\Lambda_g=0\,,\qquad
\lambda+\frac{l_2^f}{3c^2}\lambda^2-\Lambda_f=0\,.
\eeqn
Here the contributions from the interaction potential read
\beqn\label{contpotf}
\Lambda_g&=&\frac{m^5}{m_g^3}(\beta_0+4c\beta_1+6c^2\beta_2+4c^3\beta_3+c^4\beta_4)\,,\nn\\
\Lambda_f&=&\frac{m^5}{m_g^3(\alpha c)^3}(c\beta_1+4c^2\beta_2+6c^3\beta_3+4c^4\beta_4+c^5\beta_5)\,.
\eeqn
The system (\ref{bgeqLL5}) can easily be solved for $\lambda$ by building a linear combination of the equations in which the quadratic terms cancel out. This gives
\beqn
\lambda=\frac{c^2l_2^g\Lambda_f-l_2^f\Lambda_g}{c^2l_2^g-l_2^f}\,.
\eeqn
Plugging this result back into the difference of the two equations in (\ref{bgeqLL5}) results in a polynomial equation for $c$,
\beqn
l_2^g(l\Lambda_g-c^2\Lambda_f)^2+3(c^4-lc^2)(\Lambda_g-\Lambda_f)=0\,,
\eeqn
where, for notational simplicity, we have defined $l\equiv l_2^f/l_2^g$. After the expressions in (\ref{contpotf}) have been inserted, the left-hand side of this equation contains nine different powers of $c$. Demanding each coefficient to vanish, we obtain nine constraints on the parameters of the theory. As in the four-dimensional case, these constraints are not all independent, but they fix exactly seven out of the eight parameters $\{\beta_n, l_2^g, l_2^f\}$. The resulting values are
\begin{align}\label{PMvalf}
-\tfrac{1}{10}\beta_0&=\tfrac{1}{2\alpha}\beta_1=-\tfrac{1}{\alpha^2}\beta_2=-\tfrac{1}{\alpha^3}\beta_3=\tfrac{1}{2\alpha^4}\beta_4=-\tfrac{1}{10\alpha^5}\beta_5=\tfrac{m_g^3}{l_2^gm^5}\,,\nn\\
l_2^g&=\alpha^2l_f\,.
\end{align}
These parameters satisfy $\alpha^{5-n}\beta_n=\alpha^n\beta_{5-n}$ as well as $l_f=\alpha^{2-2n}l_n^g$, and hence the PM candidate theory is again symmetric under the interchange $\alpha^{-1}\gmn \leftrightarrow \alpha\fmn$. Using expression~(\ref{FPmass}) for the Fierz-Pauli mass with $m_g$ and $m_f$ replaced by the modified Planck masses given in (\ref{modmg}) and (\ref{modmf}), it is also straightforward to check that the Higuchi bound, $m_\mathrm{FP}^2=\frac{1}{2}\lambda$, is saturated. 

Note furthermore that one cannot set the Lovelock couplings $l_2^g$ and $l^f_2$ to zero because the $\beta_n$-parameters are inversely proportional to them. This is of course consistent with our findings in section \ref{noPMdgeq5}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Partial masslessness in $d>5$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The analysis in $d=6$ is very similar to the five-dimensional case since the only contributing LL term is still $\mathcal{L}_{(2)}$. Up to the sign of $\beta_3$, all but one of the parameters become fixed again. Their values are given in {\protect{\hyperref[papVII]{Paper VII}}}.

For dimensions greater than six, the cubic LL term $\mathcal{L}_{(3)}$ needs to be included into the action. According to (\ref{LLbg}), on the proportional backgrounds it reduces to $N_3(d)\lambda^3$. Hence the background equations (\ref{LLbgeq}) will now be cubic polynomials in $\lambda$. One can subtract the cubic term by building a linear combination of the two equations to arrive at a quadratic equation. But then the solution for $\lambda$ will invole a square root and, as a result, the equation determining $c$ will no longer be a polynomial. This complicates the determination of the PM parameters because we cannot apply our method, which proved successful in $d\leq 6$, to a non-polynomial equation. However, there is another possibility of solving the background equations (\ref{LLbgeq}): One can decompose them into a Gr\"obner basis of equivalent polynomial equations and thereby reduce the equation for $\lambda$ to a linear one. In addition, one obtains a consistency condition that is a polynomial in $c$ and can be used to impose the requirement for partial masslessness. Following this strategy, it is in principle possible to identify PM candidates in any dimension. The computational effort, however, becomes very large already when the quartic LL term $\mathcal{L}_{(4)}$ is included in the theory. Even with the help of a computer it was therefore only possible to determine the PM parameters in dimensions up to $d=8$ where $\mathcal{L}_{(4)}$ still does not contribute to the equations of motion. The results are summarized in Table~1 of {\protect{\hyperref[papVII]{Paper~VII}}}.  

As could have been anticipated, the PM parameters always satisfy the symmetry relations $\alpha^{d-n}\beta_n=\alpha^n\beta_{d-n}$ as well as $l_n^f=\alpha^{2-2n}l_n^g$.
The value for the Fierz-Pauli mass turns out to saturate the Higuchi bound in all cases. The fact that the scale invariance of the background and the PM gauge symmetry at the level of perturbations always coincide is entirely nontrivial and supports the validity of our approach.
Interestingly, there is no PM candidate in seven spacetime dimensions.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Relation to Higher-Curvature Gravity}
\label{ch:HD}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this chapter we discuss modified theories of gravity with higher powers of curvatures. A particular class of theories with at most four derivatives, including the famous examples of New Massive Gravity and Conformal Gravity, is known to be free of the Boulware-Deser ghost. However, one of the two spin-2 modes in these theories shows unavoidable ghost instabilities in all its helicity components. This has been an unresolved problem challenging the otherwise promising models of modified gravity. 

On the other hand, bimetric gravity with a large value for the Fierz-Pauli mass contains a heavy spin-2 excitation, and integrating out this field results in an effective theory for just one rank-2 tensor. In general, this effective action will be nonlocal, i.e.~it will not simply be an expansion in higher curvatures but involve inverted differential operators. However, in {\protect{\hyperref[papVIII]{Paper~VIII}}} we point out a definite relation among an effective action obtained from bimetric theory and the higher-curvature theories that avoid the Boulware-Deser ghost. We obtain a mapping between the two classes of theories and thereby also solve the ghost problem of the quadratic curvature theories by completing them into an infinite series of curvature terms. Furthermore, it is shown that, to lowest order in a derivative expansion, the effective theory obtained from the PM candidate introduced in chapter~\ref{ch:PM} is equivalent to Conformal Gravity.

Before explaining our method and presenting the results, we begin this chapter with a brief review of the relevant higher-curvature theories.  





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Higher-curvature gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
When viewed as a quantum theory, General Relativity is nonrenormalizable in the usual power-counting sense, which can be seen from the fact that, after canonical normalization of the fluctuations, the coupling constants of the nonlinear interactions have negative mass dimensions. Therefore the theory can be meaningful only as an effective theory which is valid at low energies and possesses a fully consistent (yet unknown) UV completion. One promising candidate for the theory at high energies is String Theory which is indeed a consistent quantum theory containing gravity as well as gauge theories that could reduce to the Standard Model of Particle Physics at low energies. In the framework of String Theory it is possible to derive the effective low-energy action for the metric $\gmn$ by integrating out heavy string states, which results in an expansion in curvatures suppressed by the mass scale of the heavy string excitations. String Theory theorefore constitutes one example of how higher-curvature terms enter the effective action. In general, the concept of effective field theory tells us that such corrections to the Einstein-Hilbert term are expected to arise from any UV completion. 


The most relevant correction to Einstein gravity is quadratic in curvatures for $\gmn$. The only possible (local) terms that can arise at this order are $R_{\mu\nu\rho\sigma}R^{\mu\nu\rho\sigma}$, $R_{\mu\nu}R^{\mu\nu}$ and $R^2$. In principle, we should also expect covariant derivatives acting on curvatures in the action, but due to the Bianchi identity the only possible term at quadratic order is $\Box R$ which is a total derivative. Also note that we can choose to complete the term $R_{\mu\nu\rho\sigma}R^{\mu\nu\rho\sigma}$ into the quadratic Lanczos-Lovelock combination~(\ref{gaussbonnet}) which we do not consider in this chapter but in principle can always be added to the action in $d>4$. One therefore only needs to take into account the terms $R_{\mu\nu}R^{\mu\nu}$ and $R^2$. It then turns out that the relative coefficient between these two contributions in the action is fixed by demanding the absence of the Boulware-Deser ghost, and the corresponding effective action truncated to a four-derivative theory is given by~\cite{Stelle:1976gc, Stelle:1977ry},
\begin{align}\label{HDact}
    S_\mathrm{HD}^{(2)}=m_g^{d-2}\int\dd^dx\sqrt{g}\,\Big[ &c_\Lambda+c_RR(g)\nn\\
    &-\frac{c_{RR}}{m^2}\left(R^{\mu\nu}R_{\mu\nu}-\frac{d}{4(d-1)}R^2\right) \Big]\,.
\end{align}
Here, $c_\Lambda$ is a cosmological constant term with mass dimension two, while $c_R$ and $c_{RR}$ are dimensionless coefficients. Furthermore, $m$ is the energy scale at which the effective field theory looses its validity. The relative coefficient between the two quadratic curvature terms is fixed to be equal to~$\frac{-d}{4(d-1)}$ which, as we shall now demonstrate, results in a mass term with the Fierz-Pauli combination at the linearized level. In order to see this, let us introduce an auxiliary tensor field $\varphi_{\mu\nu}$ into the theory, which we take to be symmetric in its indices. In terms of this new field we can write an equivalent action as follows,
\begin{align}\label{auxact}
    S_\mathrm{aux}=m_g^{d-2}\int\dd^dx\sqrt{g}\,\Big[ c_\Lambda+c_R&R(g) -\mathcal{G}_{\mu\nu}\varphi^{\mu\nu} \nn\\
    &+\frac{m^2}{4c_{RR}}(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,.
\end{align}
Here, $\mathcal{G}_{\mu\nu}$ is the Einstein tensor for $\gmn$ and the indices on the symmetric tensor $\varphi_{\mu\nu}$ are raised and lowered with~$\gmn$. As is easily verified, the solution to the equations of motion for $\varphi_{\mu\nu}$ reads
\beqn\label{phiauxeom}
\varphi_{\mu\nu}=\frac{2c_{RR}}{m^2}\left(\mathcal{G}_{\mu\nu}-\frac{1}{d-1}\mathcal{G}\gmn\right)\,,
\eeqn
which can be plugged back into (\ref{auxact}) to rearrive at (\ref{HDact}). Hence, we have defined a two-derivative theory involving an auxiliary field which can be integrated out to return to the higher-derivative action.

If now $c_\Lambda=0$ then $\bgmn=\emn$ and $\bar{\varphi}_{\mu\nu}=0$ solve both~(\ref{phiauxeom}) as well as the $\gmn$ equations. We then consider the quadratic action for fluctuations~$\varphi_{\mu\nu}$ and $\hmn=\gmn-\emn$ around this background, 
\begin{align}\label{quadactaux}
S_\mathrm{aux}^{\mathrm{lin}}=\tfrac{m_g^{d-2}}{4}\int\dd^dx\Big[h_{\mu\nu}\mathcal{E}^{\mu\nu\rho\sigma}\Big(c_{R}&h_{\rho\sigma}+\tfrac{d-2}{2}\varphi_{\rho\sigma}\Big)\nn\\
&+\tfrac{m^2}{c_{RR}}(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,,
\end{align}
where the linearized Einstein operator $\mathcal{E}^{\mu\nu\rho\sigma}$ in flat space was already given in (\ref{kinstruc1}). The kinetic terms are not diagonal, which motivates us to make the following linear redefinitions,
\beqn
\hmn'\equiv\tfrac{1}{2}m_g^{(d-2)/2} \hmn+\tfrac{d-2}{4}\tfrac{1}{c_R}\varphi_{\mu\nu}\,,\quad~~
 \varphi_{\mu\nu}'\equiv\tfrac{d-2}{4\sqrt{2}}\,m_g^{(d-2)/2}\varphi_{\mu\nu}\,,
\eeqn
where the normalizations in front have been chosen conveniently. These redefinitions diagonalize $S_\mathrm{aux}^{\mathrm{lin}}$ into an action for a massless spin-2 fluctuation $h'_{\mu\nu}$ and a massive spin-2 fluctuation $\varphi'_{\mu\nu}$,
\begin{align}\label{diagactaux}
S_\mathrm{aux}^{\mathrm{lin}}=\int\dd^dx\Big(c_Rh'_{\mu\nu}\mathcal{E}^{\mu\nu\rho\sigma}&h'_{\rho\sigma}-\tfrac{1}{c_R}\varphi'^{\mu\nu}\mathcal{E}^{\mu\nu\rho\sigma}\varphi'_{\rho\sigma}\nn\\
&+\tfrac{(d-2)^2}{16}\tfrac{m^2}{c_{RR}}(\varphi'^{\mu\nu}\varphi'_{\mu\nu}-\varphi'^2)\Big)\,.
\end{align}
As promised, the mass term has the Fierz-Pauli structure, which would not have been the case had we started with a different relative coefficient between the two quadratic-curvature terms in (\ref{HDact}). Furthermore, the sign of $c_{RR}$ determines the sign of the squared Fierz-Pauli mass and can be adjusted such that it is non-tachyonic.
On the other hand, the signs of the kinetic terms for the massless and massive spin-2 fluctuations are determined by the coefficient $c_R$ alone, and it is evident that they will always have opposite signs. As a consequence, it is unavoidable that either the massless or the massive fluctuation will be a ghost. Note that this ghost is not an extra degree of freedom and, in particular, it does not correspond to the Boulware-Deser instability. Instead, all helicity components of the massless or massive spin-2 fluctuation themselves suffer from a ghost-like kinetic term. This is a manifestation of Ostrogradski's theorem~\cite{Ostrogradski} which states that any theory with $N$ time derivatives, for $2<N<\infty$, is plagued by ghosts. Therefore the above higher-curvature action, despite being free of the Boulware-Deser ghost, is not consistent.
 
Before presenting the relation among higher-curvature gravity and Hassan-Rosen bimetric theory, let us briefly mention two popular examples for actions of the type (\ref{HDact}): New Massive Gravity in three and Conformal Gravity in four space-time dimensions.



    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsubsection{New Massive Gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As we already explained in section \ref{sec:FP}, the number degrees of freedom of a massless spin-2 particle in $d$ dimensions is $d(d-3)/2$. It follows that in $d=3$, there is no propagating massless spin-2 mode. This observation motivated the authors of \cite{Bergshoeff:2009hq, Bergshoeff:2009aq} to choose $c_R<0$ and $c_{RR}<0$ in the higher-curvature action~(\ref{HDact}) for the case $d=3$. As can be seen in the linearized auxiliary action~(\ref{diagactaux}), this choice renders the massive field healthy and turns the massless field into a ghost. However, since the massless field is not a propagating degree of freedom, the wrong sign in front of its kinetic term does not lead to an inconsistency in the theory. The higher-derivative action with these sign choices became very popular under the name \textit{New Massive Gravity}. Of course, the trick employed in \cite{Bergshoeff:2009hq, Bergshoeff:2009aq} fails to work in dimensions greater than three where the massless mode is propagating and ghost-like for $c_R<0$. In the past, the construction of a consistent higher-derivative theory in $d>3$ has therefore not been successful~\cite{Kleinschmidt:2012rs}. There have also been attempts to complete New Massive Gravity to a theory with infinitely many derivatives (see e.g.~\cite{Gullu:2010pc, Paulos:2010ke}) which could in principle avoid Ostrogradski's theorem and cure the ghost problem even in higher dimensions. We obtain such a completion in {\protect{\hyperref[papVIII]{Paper~VIII}}} where we show that the Hassan-Rosen bimetric theory when written as an effective theory for one of the metrics is closely related to New Massive Gravity in three and its generalized form in higher dimensions. Moreover, the spin-2 ghost that is unavoidably contained in (\ref{HDact}) is argued to arise from the truncation of an infinite derivative expansion to a four-derivative theory. This proposes the Hassan-Rosen bimetric action as a consistent nonlinear completion of the higher-derivative theory~(\ref{HDact}) in any number of space-time dimensions.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Conformal Gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In four spacetime dimensions, there is a particular choice of parameters for which the higher-derivative action (\ref{HDact}) develops a new gauge symmetry. 
Namely, if we set $c_\Lambda=c_R=0$ then the only terms left in the action are the four-derivative terms,~\cite{Bach} 
\beqn\label{CGact}
    S_\mathrm{CG}=-\frac{m_g^2c_{RR}}{m^2}\int\dd^4x\sqrt{g}\,\left(R^{\mu\nu}R_{\mu\nu}-\frac{1}{3}R^2\right)\,.
\eeqn
With help of the curvature relations (\ref{curvrel}) it is straightforward to show that this action is invariant under conformal transformations of the metric, 
\beqn\label{conftrafo}
\gmn\rightarrow \xi^2(x)\gmn\,,
\eeqn
where $\xi(x)$ is a local gauge parameter.
The theory therefore goes under the name of \textit{Conformal Gravity}. The cosmological constant and the Einstein-Hilbert term are not invariant under the transformation (\ref{conftrafo}) which is why their coefficients had to be set to zero.


The equations of motions that follow from variation of the conformal gravity action (\ref{CGact}) imply the vanishing of the Bach tensor for~$\gmn$,
\beqn\label{Bacheq}
   B_{\mu\nu}\equiv -\nabla^2 P_{\mu\nu}+\nabla^{\rho}\nabla_{(\mu}P_{\nu)\rho}+W_{\rho\mu\nu\sigma}P^{\rho\sigma}=0\,.
\eeqn 
Here, we have given the definition of $B_{\mu\nu}$ in terms of the Schouten tensor,
\beqn\label{schouten}
P_{\mu\nu}\equiv R_{\mu\nu}-\frac{1}{2(d-1)}\gmn R\,,
\eeqn
as well as the Weyl tensor,\footnote{In the literature, the Conformal Gravity action~(\ref{CGact}) is sometimes also expressed as the square of the Weyl tensor, $\mathcal{L}_\mathrm{CG}\propto\sqrt{g}\,W_{\rho\mu\nu\sigma}W^{\rho\mu\nu\sigma}$.}
\beqn
W_{\rho\mu\nu\sigma}\equiv R_{\rho\mu\nu\sigma}+g_{\mu[\nu}R_{\sigma]\rho}-g_{\rho[\nu}R_{\sigma]\mu}+\frac{1}{3}g_{\rho[\nu}g_{\sigma]\mu}R\,.
\eeqn 
The Bach tensor is invariant under conformal transformations in four space-time dimensions~\cite{Bach}.


The Conformal Gravity action is closely related to the linear theory for a partially massless spin-2 field discussed in section~\ref{seclinPM}. In order to see this, we again need to introduce an auxiliary field $\varphi_{\mu\nu}$. But since the equations of motion that follow from the above auxiliary action are consistent with vanishing background for $\varphi_{\mu\nu}$ only if $\gmn$ is flat, $S_\mathrm{aux}$ in (\ref{auxact}) needs to be slightly modified in order to give rise to more general de Sitter solutions for which the linear PM symmetry is known to exist. More precisely, one needs to add a linear term proportional to $\varphi=g^{\mu\nu} \varphi_{\mu\nu}$ such that $\mathcal{G}_{\mu\nu}(\bar{g})=\Lambda\bgmn$ with $\Lambda=$ const.~and $\bar{\varphi}_{\mu\nu}=0$ now solve the equations of motion. Instead of writing down the auxiliary action in the general case, here we only give the expression for Conformal Gravity which reads~\cite{Kaku:1977pa}
\begin{align}\label{CGauxact}
    S_\mathrm{CG}^{(2)}=\tfrac{4c_{RR}m_g^{2}\Lambda}{m^2}\int\dd^dx\sqrt{g}\,\Big[ \tfrac{1}{6}(R&-2\Lambda)+\varphi^{\mu\nu}\mathcal{G}_{\mu\nu} \nn\\
    &+ \Lambda\varphi+ \Lambda(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,.
\end{align}
Linearization around the constant curvature background and diagonalization into mass eigenstates shows that, for $c_{RR}>0$, the theory propagates a healthy massless and a ghost-like massive spin-2 particle. Moreover, the Fierz-Pauli mass of the massive fluctuation has the value corresponding to the Higuchi bound, $m_\mathrm{FP}^2=\frac{2}{3}\Lambda$, which implies the presence of the PM gauge symmetry (\ref{linPMsym}) for $\varphi_{\mu\nu}$. The massless fluctuation $\hmn'$ does not transform under this symmetry.
In fact, it is a simple exercise to check that, in addition to the obvious diffeomorphism invariance, the full nonlinear auxiliary action (\ref{CGauxact}) is invariant under the following linear gauge transformations~\cite{Deser:2012qg},
\beqn
\delta\gmn=2\xi(x)\gmn\,,\qquad \delta\varphi_{\mu\nu}=(\nabla_\mu\partial_\nu+\tfrac{\Lambda}{3})\xi(x)\,.
\eeqn
Note that the nonlinear field $\gmn$ transforms under the PM symmetry because its fluctuation does not correspond to the massless mode but is a linear superposition of mass eigenstates. Its transformation is of course nothing but the linear version of the conformal transformation (\ref{conftrafo}).

Conformal Gravity, or its equivalent form (\ref{CGauxact}), therefore describes only six propagating degrees of freedom instead of seven that would correspond to a massless and a massive spin-2 field. For more detailed discussions of its spectrum we refer the reader to \cite{Fradkin:1981iu, Lee:1982cp, Riegert:1984hf, Maldacena:2011mk}. 

Like any other conformal field theory, $S_\mathrm{CG}$ does not contain any dimensionful couplings and therefore avoids the nonrenormalizibility problem of General Relativity. Being a renormalizable field theory, conformal gravity has been suggested as a quantum theory for gravity. It has also been shown to allow for viable cosmological solutions and even fit galaxy rotation curves, providing a possible solution for at least part of the dark matter problem~\cite{Mannheim:2011ds}. 

Unfortunately, all of these promising features remain irrelevant unless a cure for the ghost problem is found. Suggestions for altering the theory in order to make it healthy include, for instance, a modification of quantum mechanics~\cite{Bender:2007wu} and the addition of specific boundary conditions~\cite{Maldacena:2011mk}, but none of these seemed sufficiently convincing for the theory to be accepted as a consistent alternative to General Relativity. 

In order to avoid the inconsistencies that plague theories with a finite number of higher derivatives, another possible solution is to complete the equations of motion~(\ref{Bacheq}) of Conformal Gravity with an infinite number of derivatives for which Ostrodgradski's theorem does not hold. Higher-derivative terms will, of course, break the conformal symmetry because they necessarily enter with a suppressing mass scale. On the other hand, one could imagine that the symmetry transformation needs to be completed with an infinite number of higher-derivative terms as well, in order to be a gauge symmetry of the full theory. In that case, both the equations of motion and the symmetry transformation could be thought of as a perturbative expansion in derivatives. Order by order, the equations would be invariant under the gauge symmetry, starting with the Bach tensor and its conformal invariance at lowest order. Although this idea sounds promising, without any further input it is difficult to guess the form of the higher-derivative corrections to the Bach equation that could give rise to such a gauge symmetry. It would therefore be helpful to have a guideline telling us how to construct these terms.

In section~\ref{secPMCG} we will see that the candidate for partially massless bimetric gravity introduced in section~\ref{secPmnonlin}, when written as an effective theory for $\gmn$, is equivalent to Conformal Gravity to lowest order in a derivative expansion. 
This observation motivates us to propose PM bimetric theory as a nonlinear ghost-free completion of Conformal Gravity. 
As in the case of general $\beta_n$ parameters that lead to the higher-curvature theory in (\ref{HDact}), the spin-2 ghost in Conformal Gravity is argued to be an artifact of truncating the full bimetric action to a four-derivative theory.
If our PM model possesses a nonlinear gauge symmetry then so does the corresponding effective theory for $\gmn$. Moreover, the derivative expansions of both the equations of motions for $\gmn$ and of the gauge symmetry can be constructed in a straightforward way.
This relation to the successful (but inconsistent) theory of Conformal Gravity turns ghost-free PM bimetric theory into a particularly interesting model.

   



%\begin{align}\label{auxactn}
    %S_\mathrm{aux}=m_g^{d-2}\int\dd^dx\sqrt{g}\,\Big[ \Big(&c_\Lambda+\tfrac{d}{d-1}c_{RR}m^2\Big)+\left(c_R-\tfrac{d-2}{d-1}c_{RR} \right)R(g) 
    %\nn\\
    %+\mathcal{G}_{\mu\nu}\varphi^{\mu\nu} &+m^2\varphi
    %-\frac{m^2}{4c_{RR}}(\varphi^{\mu\nu}\varphi_{\mu\nu}-\varphi^2)\Big]\,.
%\end{align}
%Here $\mathcal{G}_{\mu\nu}$ is the Einstein tensor for $\gmn$ and the indices on the symmetric tensor $\varphi_{\mu\nu}$ are raised and lowered with~$\gmn$. As is easily verified, the solution to the equations of motion for $\varphi_{\mu\nu}$ reads
%\beqn\label{phiauxeom}
%\varphi_{\mu\nu}=\frac{2c_{RR}}{m^2}\left(\mathcal{G}_{\mu\nu}-\frac{1}{d-1}\mathcal{G}\gmn-\frac{m^2}{d-1}\gmn\right)\,,
%\eeqn
%which can be plugged back into (\ref{auxact}) to reobtain (\ref{HDact}). 










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Relation to bimetric theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We now return to Hassan-Rosen bimetric gravity with the intention to demonstrate its close relation to the higher-curvature actions discussed above. First we outline two not entirely equivalent procedures of obtaining an effective action for one of the metrics by integrating out the other. Then we show that one of the procedures leads to the higher-derivative theory in~(\ref{HDact}) plus higher curvature corrections. Finally, we consider the PM bimetric theory as a particular example and demonstrate its equivalence to Conformal Gravity to lowest order in derivatives both at the level of the action and the equations of motion.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effective theories for $\gmn$}\label{sec:outl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Consider the two equations of motion obtained from varying the bimetric action (\ref{HR}) with respect to one of the two metrics while the other is held constant. Schematically, we write them as
\beqn
\mathcal{E}^g_{\mu\nu}(g,f)\equiv\left.\frac{\delta S_\mathrm{HR}}{\delta g^{\mu\nu}}\right|_{f}=0\,,\qquad \mathcal{E}^f_{\mu\nu}(g,f)\equiv\left.\frac{\delta S_\mathrm{HR}}{\delta f^{\mu\nu}}\right|_{g}=0\,.
\eeqn
Their explicit forms are given in (\ref{geq}) and (\ref{feq}), respectively, but are not important to us at this stage because our considerations here will be completely general. Suppose now that we intend to use one of the equations to express $\fmn$ in terms of $\gmn$ and then eliminate it in the second equation. For instance, we can think of obtaining a solution for $\fmn$ from its own equation of motion and plugging it into the $\gmn$ equation, such that we get an effective equation for $\gmn$,
\beqn\label{effeq1}
\mathcal{E}^g_{\mu\nu}(g, f(g))=0\,.
\eeqn
This equation will be nonlocal because solving the~$\fmn$ equation for $\fmn$ requires inverting derivative operators, leading to a nonlocal expression for $\fmn$ as a function of $\gmn$.

A more convenient way to arrive at an effective equation for $\gmn$ is to start instead by solving the $\gmn$ equation for $\fmn$, because this equation does not involve derivatives of $\fmn$.  This strategy therefore leads to an algebraic expression for $\fmn$ in terms of curvatures of $\gmn$. For general parameters in the potential, this solution can be obtained perturbatively as an infinite series in $R_{\mu\nu}(g)/m^2$. Plugging it into the other equation then results in a local effective equation for $\gmn$,
\beqn\label{effeq2}
\mathcal{E}^f_{\mu\nu}(g, f(g))=0\,,
\eeqn
which will acquire the form of a derivative expansion. Note that the two procedures of deriving an effective equation for $\gmn$ are completely equivalent: Both methods involved solving one subset of the system of equations and using these solutions in the remaining equations. Hence, the solutions to the two different effective equations for $\gmn$ will be identical in both cases.

Next let us address the question whether it is possible to derive equations (\ref{effeq1}) and (\ref{effeq2}) from an action principle. In both cases this clearly requires finding an effective action for $\gmn$. Let us first suppose that we have solved for $\fmn$ using its own equation of motion. Then we can plug this solution back into the action to obtain an effective action $S_\mathrm{eff}(g)=S_\mathrm{HR}(g, f(g))$ for $\gmn$. Variation of $S_\mathrm{eff}(g)$ then gives
\beqn\label{fpvar}
\frac{\delta S_\mathrm{eff}(g)}{\delta g^{\mu\nu}}&=&\left.\frac{\delta S_\mathrm{HR}(g, f(g))}{\delta g^{\mu\nu}}\right|_{f(g)}+\left.\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\frac{\delta S_\mathrm{HR}(g, f(g))}{\delta f^{\alpha\beta}}\right|_{g}\nn\\
&=& \mathcal{E}^g_{\mu\nu}(g, f(g))+\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\mathcal{E}^f_{\alpha\beta}(g, f(g))\,.
\eeqn
Here we have made use of the following short-hand notation for combining functional derivatives,
\beqn
\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\frac{\delta S}{\delta f^{\alpha\beta}}\equiv \int d^dy\, \frac{\delta f^{\alpha\beta}(y)}{\delta g^{\mu\nu}(x)}\frac{\delta S}{\delta f^{\alpha\beta}(y)}\,.
\eeqn
By definition, $f_{\mu\nu}(g)$ satisfies $\mathcal{E}^f_{\alpha\beta}(g, f(g))=0$. Using this in~(\ref{fpvar}) implies that, in fact, we have 
\beqn
\frac{\delta S_\mathrm{eff}(g)}{\delta g^{\mu\nu}}=\mathcal{E}^g_{\mu\nu}(g, f(g))\,.
\eeqn
This little exercise shows that the equation of motion obtained from $S_\mathrm{eff}(g)$ is precisely equation (\ref{effeq1}). We conclude that integrating out $\fmn$ in the action by using its own equation of motion is equivalent to plugging the solution directly into the $\gmn$ equation. 

Clearly, due to the nonlocality of the solution to the $\fmn$ equation, the action $S_\mathrm{eff}(g)$ will also be nonlocal and can thus not have the form of the higher-derivative theories discussed in the previous section. Let us therefore try to obtain a different effective action by integrating out $\fmn$ using the $\gmn$ equation. Since in this case the solution for $\fmn$ is an algebraic expression in terms of curvatures of $\gmn$, we can hope to arrive at a standard higher derivative theory. The variation of the effective action $S_\mathrm{HD}(g)=S_\mathrm{HR}(g, f(g))$ again reads
\beqn
\frac{\delta S_\mathrm{HD}(g)}{\delta g^{\mu\nu}}= \mathcal{E}^g_{\mu\nu}(g, f(g))+\frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\mathcal{E}^f_{\alpha\beta}(g, f(g))\,.
\eeqn
But since now $f_{\mu\nu}(g)$ is defined to satisfy $\mathcal{E}^g_{\alpha\beta}(g, f(g))=0$, we have
\beqn\label{HDactvar}
\frac{\delta S_\mathrm{HD}(g)}{\delta g^{\mu\nu}}= \frac{\delta f^{\alpha\beta}(g)}{\delta g^{\mu\nu}}\mathcal{E}^f_{\alpha\beta}(g, f(g))\,.
\eeqn
Obviously, this is not exactly equivalent to (\ref{feq}). The equations of motion obtained from the effective action $S_\mathrm{HD}(g)$ differ from the effective bimetric equations by an operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$. Therefore the solutions to these equations will differ by functions $\chi(x)$ that are annihilated by this operator, which means that instead of the bimetric equation $\mathcal{E}^f_{\alpha\beta}=0$ we now have
\beqn
\mathcal{E}^f_{\alpha\beta}(g, f(g))=\chi(x)\,,\quad \int d^dy\, \frac{\delta f^{\alpha\beta}(y)}{\delta g^{\mu\nu}(x)}\chi(y)=0\,.
\eeqn
Since $\fmn$ is a function of curvatures of $\gmn$, the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ will introduce derivative terms into the effective action that would not be present in the higher-derivative theory that is truly equivalent to bimetric gravity. Separating off these extra terms is a tedious task which we choose not to pursue. Instead we try to find out what features of the bimetric theory carry over to the local higher-derivative theory despite their inequivalence. In particular, we are interested in making statements about the consistency of the higher-derivative action $S_\mathrm{HD}(g)$. 

While it is clear that the nonlocal action $S_\mathrm{eff}(g)$ that is equivalent to the ghost-free bimetric theory must be consistent and propagate seven healthy degrees of freedom, it is an important to understand whether the local action $S_\mathrm{HD}(g)$ that differs from the Hassan-Rosen theory by an extra operator can contain ghosts. This question is difficult to answer for nonlinear spin-2 fields because the nonlinearities and the tensor structures complicate the analysis. In the appendix of {\protect{\hyperref[papVIII]{Paper VIII}}} we therefore address this issue only in two simplified models: an action for two scalar fields with linear mixing term and linearized bimetric gravity. The outcome of the analysis in both models shows that the analogue of the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ does not alter the vacuum persistence amplitude and therefore does not introduce ghosts into the theory. We therefore expect (but do not prove) that the nonlinear theory with action $S_\mathrm{HD}(g)$, obtained from integrating out $\fmn$ using the $\gmn$ equation, is also ghost-free. 

On the other hand, our examples in the appendix of {\protect{\hyperref[papVIII]{Paper VIII}}} also show that, besides shifting the mass pole in the massive field's propagator, a truncation of the derivative expansion can easily lead to ghost instabilities. This explains the presence of the spin-2 ghost in the New Massive Gravity and Conformal Gravity actions. In order to avoid Ostrogradski's theorem, the ghost-free theory certainly needs the infinite number of higher-derivative terms.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Perturbative solution to the $\gmn$ equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our focus in the following lies on the second of the two procedures outlined above, which will lead to a local effective action with higher derivatives for $\gmn$. We will apply it to bimetric gravity and explicitly work out the resulting higher-curvature terms. The first step in our declared strategy is to obtain an algebraic solution for $\fmn$ using the $\gmn$ equation, which is the purpose of this section. In order to present an instructive example, we start with a simple bimetric model in which the solution for $\fmn$ in terms of $\gmn$ curvatures has a closed and finite expression. Then we turn to the general case. In this whole chapter, as in {\protect{\hyperref[papVIII]{Paper VIII}}}, we replace the mass parameter $m^d$ in the bimetric action by $m^2m_g^{d-2}$ which slightly simplifies the expressions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{A simple example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

There is one choice of parameters for which the algebraic solution for $\fmn$ derived from the $\gmn$ equation is particularly simple and can be obtained in closed form straightforwardly. Namely, let us consider the $\gmn$ equation (\ref{geq}) in which we set all $\beta_n$ with $n=2,3\hdots d-1$ to zero. Only the contributions from $(Y^{(0)})^\mu_{~\nu}$ and $(Y^{(1)})^\mu_{~\nu}$ remain\footnote{Note that the $\gmn$ equation does not contain $\beta_d$ and hence the perturbative solution for $\fmn$ does not depend on it.} and the equation simply reads 
\beqn
\frac{1}{m^2}{\mathcal{G}^\mu}_\nu(g)+\beta_0\delta^\mu_\nu-\beta_1({S^\mu}_\nu-\Tr\,S~{\delta^\mu}_\nu)=0\,.
\eeqn
Here we have used the definition $S=\sqrt{g^{-1}f}$, as usual, and raised one index with $g^{\mu\nu}$. The trace of this equation may be used to eliminate $\Tr\,S$ and in this way the solution for ${S^\mu}_\nu$ is obtained as
\beqn\label{ssolbeta1}
{S^\mu}_\nu=\frac{1}{1-d}\frac{\beta_0}{\beta_1}\delta^\mu_\nu+\frac{1}{\beta_1m^2}{P^\mu}_\nu(g)\,,
\eeqn
which we we have expressed in terms of the Schouten tensor defined in~(\ref{schouten}).
Since $\fmn=g_{\mu\rho}{(S^2)^\rho}_\nu$ the corresponding solution for $\fmn$ immediately follows from (\ref{ssolbeta1}) and reads 
\beqn
\fmn=\left(\frac{1}{d-1}\frac{\beta_0}{\beta_1}\right)^2\gmn-\frac{2}{d-1}\frac{\beta_0}{\beta^2_1m^2}P_{\mu\nu}+\frac{1}{\beta^2_1m^4}{P_\mu}^\rho P_{\rho\nu}\,.
\eeqn
This expression already has the form of a perturbative expansion in curvatures. Remarkably, in this particular model the series terminates at quartic order in derivatives. As we will see below, for general $\beta_n$, it is not possible to solve the $\gmn$ equation for $\fmn$ exactly, but we can obtain a perturbative solution, i.e.~an expression for $\fmn$ as an infinite series in~$P/m^{2}$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{General case}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

After having explored the nature of the $\fmn$ solution in an instructive example, we now turn to the case of general $\beta_n$ parameters.
Our aim is to solve the $\gmn$ equation perturbatively for ${S^\mu}_\nu$. It will prove convenient to first rewrite the Einstein tensor in (\ref{geq}) in terms of the Schouten tensor and raise one index with $g^{\mu\nu}$. This gives
\beqn\label{eomrewr}
\Tr\,P\,\delta^\mu_\nu-{P^\mu}_\nu=m^2\sum_{n=0}^{d-1}(-1)^n\beta_n {(Y^{(n)})^\mu}_\nu(S)\,.
\eeqn
Note that for the sake of notational simplicity we have set the source for $\gmn$ to zero. This simplification constitutes no loss of generality because in the final results of our computation it can always be reinstated by making the following replacement,
\beqn\label{sourcerepl}
{P^\mu}_\nu~\longrightarrow~ {P^\mu}_\nu-m^{2-d}\left( {T^{g\mu}}_\nu -\tfrac{1}{d-1}\Tr\,T^g\,\delta^\mu_\nu\right)\,.
\eeqn
Equation (\ref{eomrewr}) is linear in curvatures for $\gmn$, but it is highly nonlinear in $\fmn$ which appears under a square-root within the tensor-valued functions~$(Y^{(n)})^\mu_{~\nu}$. It is not obvious how to obtain a closed-form solution for~$\fmn$ from it, but we can easily arrive at a perturbative solution:
As in our simple example, we first solve (\ref{eomrewr}) algebraically for ${S^\mu}_\nu$ and afterwards square the result to obtain the solution for $\fmn$. To this end, we make the following perturbative ansatz
\begin{align}\label{ansatzs}
{S^\mu}_\nu=a\delta^\mu_\nu&+\tfrac{1}{m^2}\Big(b_1{P^\mu}_\nu+b_2\Tr\,P\,\delta^\mu_\nu\Big)
+ \tfrac{1}{m^4}\Big( c_1{(P^2)^\mu}_\nu+c_2\Tr\,P\,{P^\mu}_\nu   \nn\\
&+c_3\Tr\,P^2\delta^\mu_\nu+c_4(\Tr\,P)^2\delta^\mu_\nu \Big) 
+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,,
\end{align}
with arbitrary complex coefficients $a, b_i, c_i,\hdots$ Allowing the parameters to assume complex values is reasonable as long as the coefficients that will finally appear in the effective action remain real. One can think of complex parameters in the solution for ${S^\mu}_\nu$ as being merely a tool to arrive at the most general solution. 
As we will see in section~\ref{secPMCG}, an example for a case with complex coefficients is the PM theory in which the perturbative solution for ${S^\mu}_\nu$ turns out to be purely imaginary. This leads to a real solution for $\fmn$ as well as a real effective action for $\gmn$. 

In what follows, the strategy will be to plug the above ansatz for ${S^\mu}_\nu$ into the $\gmn$ equation (\ref{eomrewr}) and fix its coefficients by satisfying the equation at each order in $P/m^2$ separately. 
In order to simplify the expressions in the following, we introduce two new sets of linear combinations of the $\beta_n$ parameters,
\beqn\label{snalphan}
s_n\equiv \sum_{k=n}^{d-1}{d-1-n\choose k-n}a^k\beta_k\,,\qquad \alpha_n=\sum_{k=n}^d {d-n \choose k-n} a^k\beta_k\,.
\eeqn
It is easy to show that these obey
\beqn\label{salphaid}
s_n=\alpha_n-\alpha_{n+1}\,.
\eeqn
On proportional backgrounds, $\fmn=c^2\gmn$ and $s_0$ is proportional to the cosmological constant $\Lambda_g$ defined in~(\ref{lambdas}) if in that expression one replaces $c$ by $a$. As we will see below, the equation of motion enforces $s_0=0$, and hence if $c=a$ the solutions for both of the metrics are flat. 
On these backgrounds then $s_1$ is proportional to the Fierz-Pauli mass~(\ref{FPmass}). In general, however, $c\neq a$ and the sums $s_n$ have no direct interpretation.

In the following it will be convenient to work with ${M^\mu}_\nu\equiv{S^\mu}_\nu/a- \delta^\mu_\nu$, for which the ansatz~(\ref{ansatzs}) starts at linear order in curvatures. In terms of this matrix we can rewrite powers and symmetric polynomials of ${S^\mu}_\nu$ as follows,
\begin{align}
 {(S^{n-k})^\mu}_\nu&=a^{n-k}\sum_{r=0}^{n-k}{n-k\choose r}{(M^r)^\mu}_\nu\,,\nn  \\
 e_k(S)&=a^k\sum_{m=0}^k{d-m\choose k-m}e_m(M)\,. \label{eitoM}
 \end{align}
These expressions enter the $\gmn$ equation of motion through the definition~(\ref{defY}) of ${(Y^{(n)})^\mu}_\nu$.
At this point let us also remark that from the latter equation in (\ref{eitoM}) it follows that the interaction potential in the bimetric action written in terms of ${M^\mu}_\nu$ becomes
 \beqn
\sum_{n=0}^{d}\beta_ne_n(S)=\sum_{n=0}^d\alpha_ne_n(M)\,,\label{senwM} 
\eeqn
which involves the $\alpha_n$ parameters defined above.
This identity will become useful in the next section when we derive the effective action for $\gmn$.

Next we use (\ref{eitoM}) in the definitions (\ref{defY}) of the matrices ${(Y^{(n)})^\mu}_\nu$ and plug the resulting expressions into the $\gmn$ equation of motion (\ref{eomrewr}). The outcome is  
\beqn
&~&m^2\sum_{n=0}^{d-1}a^n\beta_n \sum_{k=0}^n \sum_{m=0}^k \sum_{r=0}^{n-k}   (-1)^{n+k}{d-m\choose k-m}{n-k\choose r} e_m(M){(M^r)^\mu}_\nu\nn\\
&=&\Tr\,P~\delta^\mu_\nu-{P^\mu}_\nu\,.
\eeqn
The right-hand side of this equation is linear in curvatures for $\gmn$, whereas the left-hand side is a polynomial of degree $(d-1)$ in ${M^\mu}_\nu$.
In order to solve the equation perturbatively, we now insert our ansatz (\ref{ansatzs}) and compare the coefficients of $\delta^\mu_\nu$, ${P^\mu}_\nu$, $\Tr\,P\,\delta^\mu_\nu$, etc.~on both sides. For this, of course, one also needs to invoke the explicit expressions of the elementary symmetric polynomials $e_m$ that we list in (\ref{listesp}) for $m\leq4$.


For the lowest three orders it is simple to carry out this procedure by hand. The results are
\begin{align}\label{parsollo}
\mathcal{O}(1):&~~~~s_0\equiv\sum_{n=0}^{d-1} {d-1\choose n}\beta_na^n=0\,,\nn\\
\mathcal{O}\left(\tfrac{P}{m^2}\right):&~~~~  b_1=\frac{a}{s_1}\,,\quad  b_2=0\,,\nn\\
\mathcal{O}\left(\tfrac{P^2}{m^4}\right):&~~~~ 2(d-1)c_4=-2(d-1)c_3=-c_2=c_1=\frac{as_2}{s_1^3}\,.
\end{align}
The equation at lowest order, $s_0=0$, is a polynomial in $a$ that determines $a$ in terms of the $\beta_n$. Here we see explicitly that it is possible to have complex solutions for $a$ which, as stated before, do not cause any problems as long as all parameters appearing in the effective action and equations for $\gmn$ remain real. We will encounter an example for this situation in the next section. Order by order, the other equations determine the coefficients in the ansatz for ${S^\mu}_\nu$. 
Hence the perturbative solution that we have been looking for is of the following form,
\begin{align}\label{sols}
{S^\mu}_\nu=a\delta^\mu_\nu&+\tfrac{a}{s_1m^2}{P^\mu}_\nu +\tfrac{as_2}{s_1^3m^4}\Big[{(P^2)^\mu}_\nu-\Tr\,P\,{P^\mu}_\nu+\tfrac{1}{d-1}e_2( P)\delta^\mu_\nu\Big] \nn\\
&+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,.
\end{align}
For general $\beta_n$ the right-hand side is an infinite expansion in curvatures. The only case for which the series is known to terminate is the model with $\beta_n=0$ for $n=2,3\hdots d-1$ that we discussed previously.
Furthermore, the suppressing mass scale is $s_1m^2$ which, as we argued before, is proportional to the Fierz-Pauli mass of the massive fluctuation in flat space. Note also the absence of a term proportional to $\Tr\,P$ in~(\ref{sols}) as well as the fact that all relative coefficients between the quadratic curvature contributions are simply numbers independent of the parameters of the theory. For higher curvature corrections, which we have found with the help of a computer up to fifth order in curvatures, this is no longer true because some of the ratios between coefficients will become parameter dependent. 


Finally, we use $\fmn=g_{\mu\rho}{(S^2)^\rho}_\nu$ to arrive at
\begin{align}\label{fsolP}
\fmn=a^2\gmn&+\tfrac{2a^2}{s_1m^2}P_{\mu\nu}+\tfrac{a^2(s_1+2s_2)}{s_1^3m^4}{(P^2)^\mu}_\nu\nn\\
&+\tfrac{2a^2s_2}{s_1^3m^4}\Big[\tfrac{1}{d-1}e_2( P)\delta^\mu_\nu-\Tr\,P\,{P^\mu}_\nu\Big]
+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,.
\end{align}
This is the most general perturbative solution for $\fmn$ obtained from the $\gmn$ equation.

At this point let us make the remark that there are special corners in parameter space for which the perturbative solution does not exist. For instance, if $\beta_0=0$ then $a=0$ is a solution to $s_0=0$ and in this case it is not possible to find a perturbative solution for~$\fmn$. Another example of this type is a set of $\beta_n$ parameters such that $s_1=0$. In this case the perturbative solution at $\mathcal{O}(P/m^2)$ enforces $R_{\mu\nu}(g)=0$, i.e.~the solution for $\gmn$ has to be flat. It is certainly interesting to understand the nature of these special cases, but here our main focus lies on generic values for the parameters of the theory for which the perturbative solution exists.

An immediate consequence of the existence of the solution (\ref{fsolP}) is that if the solution for $\gmn$ has constant curvature, $P_{\mu\nu}\propto\gmn$, then it follows from (\ref{fsolP}) that $\fmn\propto\gmn$, i.e.~the two metrics are proportional to each other. But, as we saw in section~\ref{secpropbg}, this implies that also $\fmn$ has constant curvature. Of course, we can just as well solve the~$\fmn$ equation algebraically for $\gmn$ and interchange the roles of $\gmn$ and $\fmn$ in the argument, and hence a constant curvature solution for one of the metrics always implies proportional backgrounds and a constant curvature solution for the other metric.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Resulting theory for $\gmn$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Following the strategy described in section~\ref{sec:outl}, we now use the solution~(\ref{fsolP}) for $\fmn$ to eliminate it in the bimetric action~(\ref{HR}). 
In the interaction potential this is straightforward: One simply uses~(\ref{senwM}) to obtain an expansion in curvatures of~$\gmn$. Since the expansion of the matrix ${M^\mu}_\nu\equiv{S^\mu}_\nu/a- \delta^\mu_\nu$ starts with a term linear in~${P^\mu}_\nu$, only $e_n(M)$ with $n=0,1,2$ contribute to quadratic order in $P/m^2$. 

The kinetic term for $\fmn$ is a bit more tricky. First, we need to evaluate the inverse and the Jacobian determinant of $\fmn$. The result for the inverse reads
\beqn
(f^{-1})^{\mu\nu}=a^{-2}g^{\mu\nu}-\frac{2}{a^2s_1m^2}P^{\mu\nu}+\mathcal{O}\left(\tfrac{P^2}{m^4}\right)\,.
\eeqn
It is sufficient to expand this to first order in curvatures because in the kinetic term it is contracted with the Ricci tensor for $\fmn$ which involves no constant term. Furthermore, we have
\beqn 
\sqrt{f}=\sqrt{g}\,\det S=\sqrt{g}\,\det(a\mathbb{1}+aM)=a^d\sqrt{g}\sum_{n=0}^de_n(M)\,,
\eeqn
in which now only terms with $n=0,1$ contribute to quadratic order in curvatures.

In order to evaluate the Ricci tensor for $\fmn$, we invoke once more the curvature relations (\ref{curvrel}). With their help we can express $R_{\mu\nu}(f)$ as $R_{\mu\nu}(g)$ plus terms with covariant derivatives acting on $\gmn$ curvatures. It turns out that terms involving $\gmn$-covariant derivatives (which anyway would only give a total derivative contribution) drop out of the action upon use of the Bianchi identity. More details are provided in {\protect{\hyperref[papVIII]{Paper~VIII}}}, here we simply present the final result.
Putting everything together gives the following effective action for~$\gmn$,
\begin{align}\label{HDactobt}
    S_\mathrm{HD}=m_g^{d-2}&\int\dd^dx\sqrt{g}\,\Big[ c_\Lambda+c_RR(g)\nn\\
    &-\frac{c_{RR}}{m^2}\Big(R^{\mu\nu}R_{\mu\nu}-\frac{d}{4(d-1)}R^2\Big) \Big]~+~\mathcal{O}\left(\tfrac{P^3}{m^6}\right)\,.
\end{align}
The coefficients of different orders in curvatures are related to the original bimetric parameters through
\begin{align}
c_\Lambda&=-2m^2\alpha_0\,, \qquad c_R=1+(\alpha a)^{d-2}-\frac{\alpha_1(d-2)}{s_1(d-1)}\,,\nn\\
c_{RR}&=\frac{1}{s_1^2}\left( 2s_1(\alpha a)^{d-2}-\alpha_2+\frac{\alpha_1s_2(d-2)}{s_1(d-1)} \right)\,.
\end{align}
Remarkably, the effective action (\ref{HDactobt}) is exactly of the form (\ref{HDact}). In particular, the relative coefficient in between the two quadratic curvature coefficients is independent of the parameters of the theory and fixed to the value that removes the Boulware-Deser ghost from the spectrum. This is of course expected considering the fact that we started from the ghost-free bimetric theory. 

In the beginning of this chapter we showed that the quadratic curvature action (\ref{HDact}) always contains a spin-2 ghost. Clearly, this is not the case in bimetric gravity which gives rise to two healthy spin-2 modes at the linearized level. In {\protect{\hyperref[papVIII]{Paper~VIII}}} we  try to localize the origin of the inconsistency using a simplified model of two scalar fields. This example shows that the ghost is most likely not introduced by our procedure of obtaining the effective action for $\gmn$. That is to say,  we believe that the extra zero modes to the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ that appear in the solution are not responsible for the inconsistency. Rather, the scalar field model suggests that the ghost instability arises when the theory with infinitely many derivatives is truncated to the four-derivative level. This result is also in accordance with Ostrogradski's theorem.  We are thus lead to making the following conjecture: The local higher derivative theory with action $S_\mathrm{HD}$ obtained from bimetric gravity by integrating out $\fmn$ using the $\gmn$ equation provides a ghost-free extension of the incomplete quadratic curvature action~$S_\mathrm{HD}^{(2)}$.

Note also that the sources may be included into the theory by making the replacement~(\ref{sourcerepl}) in~(\ref{HDactobt}). As a result, in the effective action, the ghost-free coupling to matter sources is highly nontrivial. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Partially massless case}\label{secPMCG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now specialize to four space-time dimensions where, as we demonstrated in chapter~\ref{ch:PM}, the family of bimetric theories contains a candidate for the nonlinear theory of a partially massless field. But instead of fixing the parameters in the interaction potential immediately to their PM values, let us start from a different direction: Suppose our interest lies in finding the parameter values for which the higher-derivative action~(\ref{HDactobt}) obtained from bimetric gravity reduces to the Conformal Gravity action~(\ref{CGact}) at lowest order in derivatives. Clearly, this means that we must have
\beqn\label{condCG}
c_\Lambda=-2m^2\alpha_0=0\,,\qquad c_R=1+(\alpha a)^2-\frac{2\alpha_1}{3s_1}=0\,.
\eeqn
Recall that satisfying the $\gmn$ equation required $s_0=0$. Then, the identity (\ref{salphaid}) together with the first of the above conditions, $\alpha_0=0$, imply that also $\alpha_1=0$. Using this in the second condition we see that we must have $a=\pm i\alpha^{-1}$. Now we plug this value for $a$ into $s_0=0$ and $\alpha_0=0$ which we evaluate in terms of the $\beta_n$ parameters. This gives two complex equations,
\beqn
\beta_0+\frac{3i}{\alpha}\beta_1-\frac{3}{\alpha^2}\beta_2-\frac{i}{\alpha^3}\beta_3&=&0\,,\nn\\
\beta_0+\frac{4i}{\alpha}\beta_1-\frac{6}{\alpha^2}\beta_2-\frac{4i}{\alpha^3}\beta_3+\frac{1}{\alpha^4}\beta_4&=&0\,.
\eeqn
The real and imaginary parts must vanish separately and the unique solution is
\beqn\label{PMparz}
\beta_1=\beta_3=0\,,\qquad \alpha^2\beta_0=3\beta_2=\alpha^{-2}\beta_4\,.
\eeqn
Remarkably, these values precisely corresponds to the PM parameter choice in $d=4$ that we found in chapter~\ref{ch:PM}. We conclude that the PM candidate is the unique member of the family of bimetric theories with the feature that to lowest order in a derivative expansion the effective action for $\gmn$ is conformally invariant. To lowest order, the corresponding equations of motion obtained from the effective action for $\gmn$ are those of Conformal Gravity,
\beqn
B_{\mu\nu}+\mathcal{O}\left(\tfrac{P^3}{m^6}\right)=0\,.
\eeqn
Moreover, it is straightforward to show that the first method that we explained in section~\ref{sec:outl} yields a similar result:
The effective equation for $\gmn$, obtained from solving the $\gmn$ equation for $\fmn$ and plugging the solution into the $\fmn$ equation, also sets the Bach tensor to zero at lowest order in derivatives.
This is expected since the first term in the operator ${\delta f^{\alpha\beta}}/{\delta g^{\mu\nu}}$ in (\ref{HDactvar}) is proportional to the identity and hence the lowest-order terms are the same for both ways of integrating out $\fmn$.  

The nonlinear PM bimetric theory therefore proposes a ghost-free completion of Conformal Gravity. The presence of a gauge symmetry to lowest order in a derivative expansion further supports the existence of a PM gauge symmetry in the theory. In turn, if it exists, the PM symmetry constitutes the generalization of the gauge invariance of Conformal Gravity to higher orders in derivatives.

\subsubsection{Constructing the PM symmetry} 

The perturbative solution to the $\gmn$ equation and the analogous solution to the $\fmn$ equation can be used to construct the PM symmetry transformation order by order in derivatives. In fact, this method is powerful enough to prove the existence of a PM symmetry perturbatively. This is the subject of an upcoming publication and will not be discussed in detail in this thesis. However, since it strengthens the importance of {\protect{\hyperref[papVI]{Paper~VI}}}, {\protect{\hyperref[papVII]{Paper~VII}}} and {\protect{\hyperref[papVIII]{Paper~VIII}}}, let us briefly outline the idea of the proof.

An important tool in what follows is the discrete interchange symmetry of the PM candidate theory. Namely, recall that the action and the equations of motions are invariant under
\beqn\label{intsymPM}
\alpha^{-1}\gmn\longleftrightarrow \alpha \fmn\,.
\eeqn
With the PM parameters~(\ref{PMparz}), the perturbative solutions to the $\gmn$ and $\fmn$ equations of motion, respectively, assume the form,
\beqn\label{pertsolpm}
\fmn&=&-\alpha^{-2}\gmn+\frac{1}{\beta_2m^2}P_{\mu\nu}+\gamma_{\mu\nu}(\alpha^{-1}g,P)\,,\nn\\
\gmn&=&-\alpha^2\fmn+\frac{\alpha^2}{\beta_2m^2}\tilde{P}_{\mu\nu}+\alpha^2\gamma_{\mu\nu}(\alpha f,\tilde{P})\,,
\eeqn
where $\tilde{P}$ denote curvatures for $\fmn$. Furthermore, the function $\gamma_{\mu\nu}$ contains all higher-order contributions, starting at the four-derivative level. Due to the interchange symmetry (\ref{intsymPM}) the higher orders have the same functional form in both equations. 


It is easy to see that, to lowest order in derivatives, the perturbative solutions in (\ref{pertsolpm}) are invariant under two conformal transformations,
\begin{align}
\Delta\gmn&=\phi(x)\gmn + \mathcal{O}\left(\tfrac{P}{m^2}\right)\,,\nn\\
\Delta\fmn&=\phi(x)\fmn + \mathcal{O}\left(\tfrac{\tilde{P}}{m^2}\right)=-\alpha^{-2}\phi(x)\gmn+ \mathcal{O}\left(\tfrac{P}{m^2}\right)\,.
\end{align}
In the second line, we have used the solution for $\fmn$ to give two different expressions for its transformation: one that can be obtained from the $\gmn$ transformation via the interchange symmetry (\ref{intsymPM}) and one for which the invariance of the perturbative solutions is manifest. 
 
Although the conformal transformations are a symmetry of the lowest order terms in the above equations, it is clear that they will not leave the higher-order contributions invariant. In order to cancel the effects of the conformal transformations in higher orders, we need to include higher-derivative terms into the symmetry transformations of the metrics.

The next order of the transformations has two derivatives and consists of terms involving covariant derivatives acting on $\phi$ or curvatures multiplying $\phi$. They are constructed by plugging the lowest order of the transformation into the two-derivative terms of the equations. In order to cancel out these contributions one then adds corresponding terms in the transformations for $\gmn$ and $\fmn$. In fact, it is sufficient to consider only one of the above equations, say the solution for $\fmn$, and write down the necessary terms in the transformations to guarantee invariance of this equation. Then, for each type of term, there will still be an arbitrary relative coefficient between the $\gmn$ and $\fmn$ transformation. 
This coefficient is then fixed by imposing the interchange symmetry (\ref{intsymPM}). In this way, since it can be obtained from the solution for $\fmn$ through the interchange symmetry, the solution for $\gmn$ will also be invariant under the PM symmetry by construction. 

The results for the transformations to second order in derivatives derived in this manner have the following form,
\beqn\label{PMtrafso}
\Delta\gmn&=&\phi\gmn - \frac{\alpha^2}{2\beta_2m^2}\nabla_\mu\partial_\nu \phi-\frac{\alpha^2}{2\beta_2m^2}P_{\mu\nu}\phi+ \mathcal{O}\left(\tfrac{P^2}{m^4}\right)\,,\nn\\
\Delta\fmn&=&\phi\fmn - \frac{1}{2\beta_2m^2}\tilde{\nabla}_\mu\partial_\nu \phi-\frac{1}{2\beta_2m^2}\tilde{P}_{\mu\nu}\phi+\mathcal{O}\left(\tfrac{\tilde{P}^2}{m^4}\right)\nn\\
&=&-\alpha^{-2}\phi\gmn - \frac{1}{2\beta_2m^2}\nabla_\mu\partial_\nu \phi+\frac{1}{2\beta_2m^2}P_{\mu\nu}\phi+\mathcal{O}\left(\tfrac{\tilde{P}^2}{m^4}\right)\,.\nn\\
\eeqn
Again, we have expressed the $\fmn$ transformation in two different ways that are equivalent on-shell. The expression in the last line can be used to check the invariance of the perturbative solutions explicitly. When using the solution for $\fmn$ to rewrite its transformation in terms of only $\gmn$ and its curvatures, one introduces new higher-derivative terms that need to be taken care of at the next orders. This is how, for example, the term proportional to $P_{\mu\nu}\phi$ enters the transformations. 
A term $P\gmn\phi$ is absent because it is not introduced by using the perturbative solution for~$\fmn$.

The above construction of the transformations can be continued step by step at each order in derivatives, resulting in a perturbative expression for the PM gauge symmetry. Performing this construction explicitly is intricate already at the four-derivative level. Nevertheless, the mere fact that it is possible to construct the symmetry in a derivative expansion proves its existence on the perturbative solutions. Although these solutions are not the most general ones\footnote{For example, the perturbative solutions imply that if the curvatures are diagonal then so are the metrics, whereas bimetric theory is known to also contain solutions for which this is not the case, see e.g.~\cite{Volkov:2013roa}. However, in $d=4$, these are not continuously connected to the perturbative solutions above.}, they make up a large isolated class of all possible solutions. The existence of a gauge symmetry on this class of solutions is therefore highly nontrivial and furthermore supports its presence in the full theory.

Note that the precise form of the perturbative solutions in~(\ref{pertsolpm}) is unique to the PM parameters. It is quite simple to show that, for any other values of the $\beta_n$ parameters, the construction of a gauge symmetry fails latest at the two-derivative level. This could have been expected, since it was only the PM parameters that lead to the conformally invariant Bach equation when the $\gmn$ and $\fmn$ equations where combined. We conclude that our PM candidate theory is the unique theory with a scalar gauge symmetry in the perturbative solutions to its equations of motion.

To conclude this discussion, let us demonstrate that the above transformations reduce to the well-known PM gauge symmetry in the linear theory around a de Sitter background.
To this end, recall the transformation for the massive fluctuation $\delta M_{\mu\nu}$ around proportional backgrounds which, in $d=4$, can be written as
\beqn\label{linPMsym3}
\Delta (\delta M_{\mu\nu}) =  \phi(x)\bar{g}_{\mu\nu} +\frac{3}{\Lambda_g}\bar{\nabla}_\mu\partial_\nu\phi(x)\,.
\eeqn
According to its definition in (\ref{dGanddM}), the massive fluctuation satisfies $\delta M_{\mu\nu}\propto \delta\fmn-c^2\delta\gmn$. This implies that its transformation under the PM symmetry must be proportional to $\Delta\fmn-c^2\Delta\gmn$ evaluated on the proportional backgrounds. 
For $\bar{f}_{\mu\nu}=c^2\bar{g}_{\mu\nu}$ we have that
\beqn
P_{\mu\nu}(\bar{g})=\tilde{P}_{\mu\nu}(\bar{f})= \frac{\Lambda_g}{3}\bar{g}_{\mu\nu}\qquad \Lambda_g=3\beta_2m^2(1+\alpha^2c^2)\,.
\eeqn
Using these results in (\ref{PMtrafso}) it can easily be checked that on these backgrounds one obtains
\beqn
\left.\left(\Delta\fmn-c^2\Delta\gmn\right)\right|_{\bar{f}_{\mu\nu}=c^2\bar{g}_{\mu\nu}}=\frac{1}{2}(\alpha^4c^4-1)\left[\phi\bar{g}_{\mu\nu}+\frac{3}{\Lambda_g}\bar{\nabla}_\mu\partial_\nu\phi\right]\,,
\eeqn
which is indeed proportional to (\ref{linPMsym3}).
Hence, the above nonlinear transformations generate precisely the PM transformation of the massive fluctuation. As a side remark, let us point out that this also means that the higher-order terms of the PM transformation of $\delta M_{\mu\nu}$ must vanish on the proportional backgrounds.

The fact that we arrive at the correct form (\ref{linPMsym3}) starting from the nonlinear transformations shows that the gauge symmetry we constructed above corresponds precisely to the PM invariance of the linear theory. 
Our nonlinear PM candidate thus explains the origin of the PM symmetry around de Sitter backgrounds and, even at the nonlinear level, a gauge symmetry removes one degree of freedom. 


 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Summary $\&$ Outlook}
\label{ch:concl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this thesis, we discussed ghost-free nonlinear theories involving massive spin-2 fields. Our findings are summarized below.


\begin{itemize}

\item[$\diamond$] There are two classes of consistent nonlinear theories for massive spin-2 fields of rather distinct nature: Nonlinear Massive Gravity~\cite{deRham:2010kj, Hassan:2011vm} contains self-interactions of a massive spin-2 field in a background that is fixed by hand, whereas bimetric theory~\cite{Hassan:2011zd} describes two dynamical spin-2 fields, one with massive and one with massless fluctuation around maximally symmetric backgrounds. We demonstrated the absence of the Boulware-Deser ghost instability in nonlinear Massive Gravity both in the physical gauge and in a diffeomorphism invariant formulation. 

\item[$\diamond$] We computed the mass spectrum of bimetric theory around proportional background solutions and identified nonlinear fields with massive and massless fluctuations around these backgrounds. A Hamiltonian analysis revealed that the nonlinear massless field cannot have standard matter couplings, which suggested that, in the presence of a massive spin-2 field, the gravitational metric is a superposition of mass eigenstates.

\item[$\diamond$] In the vielbein formulation, bimetric theory can be generalized to describe interactions of multiple spin-2 fields~\cite{Hinterbichler:2012cn}. We introduced a set of St\"uckelberg fields to reinstore the broken local Lorentz symmetry in the theory, which enabled us to reformulate the multivielbein theory in terms of the respective metrics.


\item[$\diamond$] The most general homogeneous and isotropic solutions to the bimetric equations of motion were derived and in some special cases discussed in more detail. The parameters of the interaction potential could be fitted to observational data and thus, at the background level, bimetric theory could account for the observed cosmologial evolution. Certain parameter subspaces even gave rise to a viable self-accelerating cosmological expansion without the need to include vacuum energy~\cite{Akrami:2012vf}.

\item[$\diamond$] We developed a method to identify nonlinear candidate theories for a partially massless spin-2 field within the family of bimetric actions. The equations of motion in such a theory should be invariant under a generalization of the gauge symmetry for linear PM fields in de Sitter backgrounds.
In the four-dimensional candidate theory, several aspects pointed towards the presence of a gauge symmetry at the nonlinear level. 
In space-time dimensions greater than four, it was necessary to extend the bimetric action by the Lanczos-Lovelock terms in order to obtain nontrivial results.


\item[$\diamond$] Bimetric theory was shown to be closely related to a certain class of higher-curvature theories for gravity which are known to be free of the Boulware-Deser ghost. On the other hand, these theories contain a spin-2 field whose helicity components all show instabilities. We argued that this problem may be cured by completing the quadratic curvature terms in the action into an infinite expansion in derivatives whose form can be derived from bimetric gravity. 

\item[$\diamond$] A close connection between our candidate theory for nonlinear partial masslessness and Conformal Gravity was established. The equations of motion of PM bimetric theory were shown to be conformally invariant at the four-derivative level in a perturbative expansion. This observation further allowed us to explicitly construct the PM gauge symmetry perturbatively to second-order in derivatives, which resulted in an expression compatible with the well-known transformation of linear PM fields. Moreover, the perturbative solutions to the equations of motion in the PM bimetric theory opened up the possibility to prove the existence of a gauge symmetry at the nonlinear level.
\end{itemize}


Open issues in the field of nonlinear Massive Gravity and bimetric theory can be divided into phenomenological and more theoretical questions. On the phenomenology side, further investigation of classical solutions to the equations of motion is of great interest. On the theory side, it is most interesting to look for extensions of the consistent theories in order to fit them into a larger framework. In the following we mention some of the vividly ongoing research. 

\vspace*{5mm}

Having found viable cosmological background solutions to the bimetric equations, the next test the theory needs to pass is whether it can explain growth of structure in the universe. In order to address this question, one needs to study perturbations around the cosmological solutions. Unfortunately, this type of analysis is complicated by the square-root matrix in the interaction potential. First attempts to derive and solve the perturbation equations have been made in~\cite{Comelli:2012db, Berg:2012kn}, but the compatibility of bimetric theory with constraints from structure formation is still an open question.

Another important issue in theories with massive spin-2 fields coupled to matter is the existence of a Vainshtein mechanism in order to avoid the observationally discarded vDVZ discontinuity. Spherically symmetric solutions to the bimetric equations have been investigated in \cite{Comelli:2011wq, Volkov:2013roa, Volkov:2012wp}. The possibility for a Vainshtein mechanism and the reconcilability with astrophysical data were shown to be given both in Massive Gravity~\cite{Sjors:2011iv} and in bimetric theory~\cite{Enander:2013kza}.


The evidence for the existence of a gauge symmetry, which we discovered in several independent approaches, exposes the exceptional nature of the nonlinear PM bimetric theory. It would be of great interest to derive the explicit non-perturbative form of the gauge transformations that leave the bimetric equations invariant. But even without the knowledge of the exact transformations, physical aspects of the theory can be studied. An analysis of implications for cosmology has been started, for example, in~\cite{Akrami:2013ffa}. Moreover, in \cite{Brito:2013yxa} it was shown that the PM theory avoids the Gregory-Laflamme instability~\cite{Gregory:1993vy} which is a generic undesirable feature of black-hole solutions in nonlinear Massive Gravity and bimetric theory~\cite{Babichev:2013una, Brito:2013wya}.

Eventually, one would of course also like to return to the original motivation for constructing a nonlinear Massive Gravity theory and readdress the cosmological constant problem. So far, an obvious solution to the problem has been found neither in Massive Gravity nor in bimetric gravity. The self-accelerating cosmological backgrounds discussed in \cite{Akrami:2012vf, Akrami:2013ffa} demonstrate that bimetric theory can account for the observed rate of cosmic acceleration without any vacuum energy.
The acceleration is due to a spin-2 field with mass at the Hubble scale, which mildens the cosmological constant problem because a small spin-2 mass is technically natural. On the other hand, the origin of the small value for the graviton mass as well as the disappearance of vacuum energy from quantum field theory remain unexplained in this setup. 






\vspace*{5mm}


Turning to the prospects on the theory side, we emphasize that extensions of the bimetric action primarily need to maintain the consistency of the theory. In particular, they must not reintroduce the Boulware-Deser ghost instability. One possibility of extending the theory is then given by the Lanczos-Lovelock terms that we already considered in {\protect{\hyperref[papVII]{Paper~VII}}}. These are commonly believed to avoid the Boulware-Deser ghost and therefore provide a viable generalization of the Hassan-Rosen action. 
Another conceivable extension is the addition of further derivative interactions that respect the antisymmetric structure of the interaction potential and the LL terms. The consistency of such new interactions has recently been suggested in a pseudo-linear analysis~\cite{Hinterbichler:2013eza}, while their precise nonlinear form is still unknown.

Other extensions involving additional scalar fields have been introduced mainly in the context of nonlinear Massive Gravity. For example, it has been suggested to promote the $\beta_n$-parameters to functions of a scalar field~\cite{Huang:2012pe, Huang:2013mha}.
Furthermore, the proposals involve coupling the metric $\gmn$ to fields with Galileon symmetry~\cite{Gabadadze:2012tr} and to a quasi-dilaton~\cite{D'Amico:2012zv}. If the quasi-dilaton is self-interacting, the theory is classically equivalent to the Massive Gravity action extended by functions of the Ricci scalar~\cite{Cai:2013lqa}. A similar $f( R)$ generalization has also been considered for bimetric gravity~\cite{Nojiri:2013zza}.


Another important issue is the computation of quantum corrections to the consistent nonlinear actions for spin-2 fields. A first attempt to this effect has been made in~\cite{Buchbinder:2012wb} which, however, worked with the auxiliary model that we discussed in section~\ref{hamstuck}. Although, classically, this model is equivalent to the Massive Gravity action with a certain parameter choice, the two theories may differ at the quantum level. More recently, the one-loop effective action of the dRGT model was computed in~\cite{deRham:2013qqa}. There it was demonstrated that, at one-loop level, matter fields running in the loop do not change the structure of the interaction potential for the metric, whereas the ghost-free configuration does get modified by gravitons in the loop. Fortunately, the authors also argue that the mass of the ghost is never below the Planck scale and therefore does not propagate in the effective theory. These promising results suggest that consistent nonlinear Massive Gravity may be stable under quantum corrections. Besides the computation of higher-order loop diagrams in the dRGT model with fixed Minkowski background, it would be interesting to investigate whether this feature is shared by the fully dynamical bimetric theory.


Finally, one could explore the possibility of embedding the consistent bimetric models in String Theory. The most promising candidate for a unified description of particle physics and quantum gravity possesses a rich spectrum of massless and massive higher-spin fields. In particular, it contains a massless spin-2 field whose low-energy effective action is Einstein-Hilbert plus higher-curvature corrections. But the spectrum also includes a massive spin-2 field whose effective action has not been computed.
%\footnote{Derivations of effective actions in String Theory are very involved and usually the focus lies on massless fields that are most relevant in the low-energy limit.} 
It is therefore an interesting open question whether the ghost-free structure of the nonlinear massive spin-2 theories discussed in this thesis can be reproduced in String Theory. If this is the case, then, since phenomenologically viable String Theory requires Supersymmetry, it will contain a supersymmetrized version of bimetric theory. This motivates the search for a supersymmetric theory involving massive spin-2 fields which, even without String Theory, could be an interesting subject on its own. Interestingly, such a theory was already suggested several decades ago in~\cite{Chamseddine:1978yu} but without addressing the ghost issue.

Concluding remarks





 



\begin{thebibliography}{999}
\bibitem{Martin:2012bt}
  J.~Martin,
  %``Everything You Always Wanted To Know About The Cosmological Constant Problem (But Were Afraid To Ask),''
  Comptes Rendus Physique {\bf 13} (2012) 566
  [arXiv:1205.3365 [astro-ph.CO]].
  %%CITATION = ARXIV:1205.3365;%%
\bibitem{Wald:1984rg}
  R.~M.~Wald,
  %``General Relativity,''
  Chicago, Usa: Univ. Pr. ( 1984) 491p.
\bibitem{Weinberg:1988cp}
  S.~Weinberg,
  %``The Cosmological Constant Problem,''
  Rev.\ Mod.\ Phys.\  {\bf 61} (1989) 1.
  %%CITATION = RMPHA,61,1;%%
\bibitem{Jaffe:2005vp}
  R.~L.~Jaffe,
  %``The Casimir effect and the quantum vacuum,''
  Phys.\ Rev.\ D {\bf 72} (2005) 021301
  [hep-th/0503158].
  %%CITATION = HEP-TH/0503158;%%
\bibitem{Dvali:2002pe}
  G.~Dvali, G.~Gabadadze and M.~Shifman,
  %``Diluting cosmological constant in infinite volume extra dimensions,''
  Phys.\ Rev.\ D {\bf 67} (2003) 044020
  [hep-th/0202174].
  %%CITATION = HEP-TH/0202174;%%
\bibitem{Dvali:2002fz}
  G.~Dvali, G.~Gabadadze and M.~Shifman,
  %``Diluting cosmological constant via large distance modification of gravity,''
  hep-th/0208096.
  %%CITATION = HEP-TH/0208096;%%
\bibitem{Hinterbichler:2011tt}
  K.~Hinterbichler,
  %``Theoretical Aspects of Massive Gravity,''
  Rev.\ Mod.\ Phys.\  {\bf 84} (2012) 671
  [arXiv:1105.3735 [hep-th]].
  %%CITATION = ARXIV:1105.3735;%%
\bibitem{ArkaniHamed:2002sp}
  N.~Arkani-Hamed, H.~Georgi and M.~D.~Schwartz,
  %``Effective field theory for massive gravitons and gravity in
  %theory space,'' 
  Annals Phys.\  {\bf 305} (2003) 96
  [hep-th/0210184].
  %%CITATION = HEP-TH/0210184;%%
\bibitem{de Urries:1998bi}
  F.~J.~de Urries and J.~Julve,
  %``Ostrogradski formalism for higher derivative scalar field theories,''
  J.\ Phys.\ A {\bf 31} (1998) 6949
  [hep-th/9802115].
  %%CITATION = HEP-TH/9802115;%%
\bibitem{Fierz:1939ix}
  M.~Fierz and W.~Pauli,
  %``On relativistic wave equations for particles of arbitrary spin in 
  %an electromagnetic field,'' 
  Proc.\ Roy.\ Soc.\ Lond.\ A {\bf 173} (1939) 211.
  %%CITATION = PRSLA,A173,211;%%
\bibitem{Pauli:1939xp}
  W.~Pauli and M.~Fierz,
  %``On Relativistic Field Equations Of Particles With Arbitrary Spin
  %In An Electromagnetic Field,'' 
  Helv.\ Phys.\ Acta {\bf 12} (1939) 297.
  %%CITATION = HPACA,12,297;%%
\bibitem{vanDam:1970vg}
  H.~van Dam and M.~J.~G.~Veltman,
  %``Massive and massless Yang-Mills and gravitational fields,''
  Nucl.\ Phys.\ B {\bf 22} (1970) 397.
  %%CITATION = NUPHA,B22,397;%%
\bibitem{Zakharov:1970cc}
  V.~I.~Zakharov,
  %``Linearized gravitation theory and the graviton mass,''
  JETP Lett.\  {\bf 12} (1970) 312
   [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 12} (1970) 447].
  %%CITATION = JTPLA,12,312;%%
\bibitem{Iwasaki:1971uz}
  Y.~Iwasaki,
  %``Consistency condition for propagators,''
  Phys.\ Rev.\ D {\bf 2} (1970) 2255.
  %%CITATION = PHRVA,D2,2255;%%
\bibitem{Vainshtein:1972sx}
  A.~I.~Vainshtein,
  %``To the problem of nonvanishing gravitation mass,''
  Phys.\ Lett.\ B {\bf 39} (1972) 393.
  %%CITATION = PHLTA,B39,393;%%
\bibitem{Deser:1981wh}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Topologically Massive Gauge Theories,''
  Annals Phys.\  {\bf 140} (1982) 372
   [Erratum-ibid.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 281} (2000) 409].
  %%CITATION = APNYA,140,372;%%
\bibitem{Deser:1982vy}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Three-Dimensional Massive Gauge Theories,''
  Phys.\ Rev.\ Lett.\  {\bf 48} (1982) 975.
  %%CITATION = PRLTA,48,975;%%
\bibitem{Bergshoeff:2009hq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``Massive Gravity in Three Dimensions,''
  Phys.\ Rev.\ Lett.\  {\bf 102} (2009) 201301
  [arXiv:0901.1766 [hep-th]].
  %%CITATION = ARXIV:0901.1766;%%
\bibitem{Rosen:1940zz}
  N.~Rosen,
  %``General Relativity and Flat Space. II,''
  Phys.\ Rev.\  {\bf 57} (1940) 150.
  %%CITATION = PHRVA,57,150;%%
\bibitem{Rosen:1975kk}
  N.~Rosen,
  %``Bimetric Theory of Gravitation,''
  In *Erice 1975, Proceedings, Topics In Theoretical and Experimental
  Gravitation Physics*, New York 1977, 273-294 
 \bibitem{Aragone:1971kh}
  C.~Aragone and S.~Deser,
  %``Constraints on gravitationally coupled tensor fields,''
  Nuovo Cim.\ A {\bf 3} (1971) 709.
  %%CITATION = NUCIA,A3,709;%%
\bibitem{ISS}
  C.~J.~Isham, A.~Salam and J.~A.~Strathdee,
  %``F-dominance of gravity,''
  Phys.\ Rev.\ D {\bf 3} (1971) 867.
  %%CITATION = PHRVA,D3,867;%%
\bibitem{Boulware:1973my}
  D.~G.~Boulware and S.~Deser,
  %``Can gravitation have a finite range?,''
  Phys.\ Rev.\ D {\bf 6} (1972) 3368.
  %%CITATION = PHRVA,D6,3368;%%
\bibitem{Chamseddine:1978yu}
  A.~H.~Chamseddine, A.~Salam and J.~A.~Strathdee,
  %``Strong Gravity and Supersymmetry,''
  Nucl.\ Phys.\ B {\bf 136} (1978) 248.
  %%CITATION = NUPHA,B136,248;%%
\bibitem{Riess:1998cb}
  A.~G.~Riess {\it et al.}  [Supernova Search Team Collaboration],
  %``Observational evidence from supernovae for an accelerating universe and a cosmological constant,''
  Astron.\ J.\  {\bf 116} (1998) 1009
  [astro-ph/9805201].
  %%CITATION = ASTRO-PH/9805201;%%
\bibitem{Perlmutter:1998np}
  S.~Perlmutter {\it et al.}  [Supernova Cosmology Project Collaboration],
  %``Measurements of Omega and Lambda from 42 high redshift supernovae,''
  Astrophys.\ J.\  {\bf 517} (1999) 565
  [astro-ph/9812133].
  %%CITATION = ASTRO-PH/9812133;%%
\bibitem{Hubble:1926yw}
  E.~P.~Hubble,
  %``Extragalactic nebulae,''
  Astrophys.\ J.\  {\bf 64} (1926) 321.
  %%CITATION = ASJOA,64,321;%%
 \bibitem{Hubble:1929ig}
  E.~Hubble,
  %``A relation between distance and radial velocity among extra-galactic nebulae,''
  Proc.\ Nat.\ Acad.\ Sci.\  {\bf 15} (1929) 168.
  %%CITATION = PNASA,15,168;%%
\bibitem{ArkaniHamed:1998rs}
  N.~Arkani-Hamed, S.~Dimopoulos and G.~R.~Dvali,
  %``The Hierarchy problem and new dimensions at a millimeter,''
  Phys.\ Lett.\ B {\bf 429} (1998) 263
  [hep-ph/9803315].
  %%CITATION = HEP-PH/9803315;%%
\bibitem{Antoniadis:1998ig}
  I.~Antoniadis, N.~Arkani-Hamed, S.~Dimopoulos and G.~R.~Dvali,
  %``New dimensions at a millimeter to a Fermi and superstrings at a TeV,''
  Phys.\ Lett.\ B {\bf 436} (1998) 257
  [hep-ph/9804398].
  %%CITATION = HEP-PH/9804398;%%
\bibitem{Randall:1998uk}
  L.~Randall and R.~Sundrum,
  %``Out of this world supersymmetry breaking,''
  Nucl.\ Phys.\ B {\bf 557} (1999) 79
  [hep-th/9810155].
  %%CITATION = HEP-TH/9810155;%%
\bibitem{Dvali:2000hr}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``4-D gravity on a brane in 5-D Minkowski space,''
  Phys.\ Lett.\ B {\bf 485} (2000) 208
  [hep-th/0005016].
  %%CITATION = HEP-TH/0005016;%%
\bibitem{Dvali:2001gm}
  G.~R.~Dvali, G.~Gabadadze, M.~Kolanovic and F.~Nitti,
  %``The Power of brane induced gravity,''
  Phys.\ Rev.\ D {\bf 64} (2001) 084004
  [hep-ph/0102216].
  %%CITATION = HEP-PH/0102216;%%
\bibitem{Rubakov:2008nh}
  V.~A.~Rubakov and P.~G.~Tinyakov,
  %``Infrared-modified gravities and massive gravitons,''
  Phys.\ Usp.\  {\bf 51} (2008) 759
  [arXiv:0802.4379 [hep-th]].
  %%CITATION = ARXIV:0802.4379;%%
\bibitem{deRham:2007rw}
  C.~de Rham, S.~Hofmann, J.~Khoury and A.~J.~Tolley,
  %``Cascading Gravity and Degravitation,''
  JCAP {\bf 0802} (2008) 011
  [arXiv:0712.2821 [hep-th]].
  %%CITATION = ARXIV:0712.2821;%%
\bibitem{deRham:2007xp}
  C.~de Rham, G.~Dvali, S.~Hofmann, J.~Khoury, O.~Pujolas, M.~Redi and A.~J.~Tolley,
  %``Cascading gravity: Extending the Dvali-Gabadadze-Porrati model to higher dimension,''
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 251603
  [arXiv:0711.2072 [hep-th]].
  %%CITATION = ARXIV:0711.2072;%%
\bibitem{Dvali:2000rv}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``Metastable gravitons and infinite volume extra dimensions,''
  Phys.\ Lett.\ B {\bf 484} (2000) 112
  [hep-th/0002190].
  %%CITATION = HEP-TH/0002190;%%
\bibitem{Gregory:2000jc}
  R.~Gregory, V.~A.~Rubakov and S.~M.~Sibiryakov,
  %``Opening up extra dimensions at ultra large scales,''
  Phys.\ Rev.\ Lett.\  {\bf 84} (2000) 5928
  [hep-th/0002072].
  %%CITATION = HEP-TH/0002072;%%
\bibitem{Dvali:2001ae}
  G.~Dvali, G.~Gabadadze, X.~-r.~Hou and E.~Sefusatti,
  %``Seesaw modification of gravity,''
  Phys.\ Rev.\ D {\bf 67} (2003) 044019
  [hep-th/0111266].
  %%CITATION = HEP-TH/0111266;%%
\bibitem{Kiritsis:2001bc}
  E.~Kiritsis, N.~Tetradis and T.~N.~Tomaras,
  %``Induced brane gravity: Realizations and limitations,''
  JHEP {\bf 0108} (2001) 012
  [hep-th/0106050].
  %%CITATION = HEP-TH/0106050;%%
\bibitem{Corley:2001hg}
  S.~Corley, D.~A.~Lowe and S.~Ramgoolam,
  %``Einstein-Hilbert action on the brane for the bulk graviton,''
  JHEP {\bf 0107} (2001) 030
  [hep-th/0106067].
  %%CITATION = HEP-TH/0106067;%%
\bibitem{Ardalan:2002qt}
  F.~Ardalan, H.~Arfaei, M.~R.~Garousi and A.~Ghodsi,
  %``Gravity on noncommutative D-branes,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 18} (2003) 1051
  [hep-th/0204117].
  %%CITATION = HEP-TH/0204117;%%
\bibitem{Antoniadis:2002tr}
  I.~Antoniadis, R.~Minasian and P.~Vanhove,
  %``Noncompact Calabi-Yau manifolds and localized gravity,''
  Nucl.\ Phys.\ B {\bf 648} (2003) 69
  [hep-th/0209030].
  %%CITATION = HEP-TH/0209030;%%
\bibitem{Kohlprath:2004yw}
  E.~Kohlprath and P.~Vanhove,
  %``Localized gravity in non-compact superstring models,''
  hep-th/0409197.
  %%CITATION = HEP-TH/0409197;%%
\bibitem{Epple:2004ra}
  F.~T.~J.~Epple,
  %``Induced gravity on intersecting branes,''
  JHEP {\bf 0409} (2004) 021
  [hep-th/0408105].
  %%CITATION = HEP-TH/0408105;%%
\bibitem{Deffayet:2007zz}
  C.~Deffayet,
  %``The vDVZ discontinuity, DGP gravity, and cosmology,''
  Int.\ J.\ Theor.\ Phys.\  {\bf 46} (2007) 2242.
  %%CITATION = IJTPB,46,2242;%%
\bibitem{Fang:2008kc}
  W.~Fang, S.~Wang, W.~Hu, Z.~Haiman, L.~Hui and M.~May,
  %``Challenges to the DGP Model from Horizon-Scale Growth and Geometry,''
  Phys.\ Rev.\ D {\bf 78} (2008) 103509
  [arXiv:0808.2208 [astro-ph]].
  %%CITATION = ARXIV:0808.2208;%%
\bibitem{Lombriser:2009xg}
  L.~Lombriser, W.~Hu, W.~Fang and U.~Seljak,
  %``Cosmological Constraints on DGP Braneworld Gravity with Brane Tension,''
  Phys.\ Rev.\ D {\bf 80} (2009) 063536
  [arXiv:0905.1112 [astro-ph.CO]].
  %%CITATION = ARXIV:0905.1112;%%
\bibitem{Dubovsky:2002jm}
  S.~L.~Dubovsky and V.~A.~Rubakov,
  %``Brane induced gravity in more than one extra dimensions: Violation of equivalence principle and ghost,''
  Phys.\ Rev.\ D {\bf 67} (2003) 104014
  [hep-th/0212222].
  %%CITATION = HEP-TH/0212222;%%
\bibitem{Kolanovic:2003am}
  M.~Kolanovic, M.~Porrati and J.~-W.~Rombouts,
  %``Regularization of brane induced gravity,''
  Phys.\ Rev.\ D {\bf 68} (2003) 064018
  [hep-th/0304148].
  %%CITATION = HEP-TH/0304148;%%
\bibitem{Gabadadze:2003ck}
  G.~Gabadadze and M.~Shifman,
  %``Softly massive gravity,''
  Phys.\ Rev.\ D {\bf 69} (2004) 124032
  [hep-th/0312289].
  %%CITATION = HEP-TH/0312289;%%
\bibitem{Klebanov:1995ni}
  I.~R.~Klebanov and L.~Thorlacius,
  %``The Size of p-branes,''
  Phys.\ Lett.\ B {\bf 371} (1996) 51
  [hep-th/9510200].
  %%CITATION = HEP-TH/9510200;%%
\bibitem{'tHooft:2007bf}
  G.~'t Hooft,
  %``Unitarity in the Brout-Englert-Higgs Mechanism for Gravity,''
  arXiv:0708.3184 [hep-th].
  %%CITATION = ARXIV:0708.3184;%%
\bibitem{Kakushadze:2007hf}
  Z.~Kakushadze,
  %``Massive Gravity in Minkowski Space via Gravitational Higgs Mechanism,''
  Phys.\ Rev.\ D {\bf 77} (2008) 024001
  [arXiv:0710.1061 [hep-th]].
  %%CITATION = ARXIV:0710.1061;%%
\bibitem{Corradini:2001qv}
  O.~Corradini, A.~Iglesias, Z.~Kakushadze and P.~Langfelder,
  %``Gravity on a 3-brane in 6-D bulk,''
  Phys.\ Lett.\ B {\bf 521} (2001) 96
  [hep-th/0108055].
  %%CITATION = HEP-TH/0108055;%%
\bibitem{Kaloper:2007ap}
  N.~Kaloper and D.~Kiley,
  %``Charting the landscape of modified gravity,''
  JHEP {\bf 0705} (2007) 045
  [hep-th/0703190].
  %%CITATION = HEP-TH/0703190;%%
\bibitem{Kaloper:2007qh}
  N.~Kaloper,
  %``Brane Induced Gravity: Codimension-2,''
  Mod.\ Phys.\ Lett.\ A {\bf 23} (2008) 781
  [arXiv:0711.3210 [hep-th]].
  %%CITATION = ARXIV:0711.3210;%%
\bibitem{Deffayet:2001uk}
  C.~Deffayet, G.~R.~Dvali, G.~Gabadadze and A.~I.~Vainshtein,
  %``Nonperturbative continuity in graviton mass versus perturbative discontinuity,''
  Phys.\ Rev.\ D {\bf 65} (2002) 044026
  [hep-th/0106001].
  %%CITATION = HEP-TH/0106001;%%
\bibitem{Deffayet:2000uy}
  C.~Deffayet,
  %``Cosmology on a brane in Minkowski bulk,''
  Phys.\ Lett.\ B {\bf 502} (2001) 199
  [hep-th/0010186].
  %%CITATION = HEP-TH/0010186;%%
\bibitem{Peskin:1995ev}
  M.~E.~Peskin and D.~V.~Schroeder,
  %``An Introduction to quantum field theory,''
  Reading, USA: Addison-Wesley (1995) 842 p
%\cite{Srednicki:2007qs}
\bibitem{Srednicki:2007qs}
  M.~Srednicki,
  %``Quantum field theory,''
  Cambridge, UK: Univ. Pr. (2007) 641 p
\bibitem{Lee:1977eg}
  B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
  %``Weak Interactions at Very High-Energies: The Role of the Higgs Boson Mass,''
  Phys.\ Rev.\ D {\bf 16} (1977) 1519.
  %%CITATION = PHRVA,D16,1519;%%
\bibitem{Chanowitz:1985hj}
  M.~S.~Chanowitz and M.~K.~Gaillard,
  %``The TeV Physics of Strongly Interacting W's and Z's,''
  Nucl.\ Phys.\ B {\bf 261} (1985) 379.
  %%CITATION = NUPHA,B261,379;%%
\bibitem{ArkaniHamed:2003uy}
  N.~Arkani-Hamed, H.~-C.~Cheng, M.~A.~Luty and S.~Mukohyama,
  %``Ghost condensation and a consistent infrared modification of gravity,''
  JHEP {\bf 0405} (2004) 074
  [hep-th/0312099].
  %%CITATION = HEP-TH/0312099;%%
\bibitem{Rubakov:2004eb}
  V.~A.~Rubakov,
  %``Lorentz-violating graviton masses: Getting around ghosts, low strong coupling scale and VDVZ discontinuity,''
  hep-th/0407104.
  %%CITATION = HEP-TH/0407104;%%
\bibitem{Dubovsky:2004sg}
  S.~L.~Dubovsky,
  %``Phases of massive gravity,''
  JHEP {\bf 0410} (2004) 076
  [hep-th/0409124].
  %%CITATION = HEP-TH/0409124;%%
\bibitem{Creminelli:2005qk}
  P.~Creminelli, A.~Nicolis, M.~Papucci and E.~Trincherini,
  %``Ghosts in massive gravity,''
  JHEP {\bf 0509} (2005) 003
  [hep-th/0505147].
  %%CITATION = HEP-TH/0505147;%%
\bibitem{Nibbelink:2006sz}
  S.~Nibbelink Groot, M.~Peloso and M.~Sexton,
  %``Nonlinear Properties of Vielbein Massive Gravity,''
  Eur.\ Phys.\ J.\ C {\bf 51} (2007) 741
  [hep-th/0610169].
  %%CITATION = HEP-TH/0610169;%%
\bibitem{Gabadadze:2009ja}
  G.~Gabadadze,
  %``General Relativity With An Auxiliary Dimension,''
  Phys.\ Lett.\ B {\bf 681} (2009) 89
  [arXiv:0908.1112 [hep-th]].
  %%CITATION = ARXIV:0908.1112;%%
\bibitem{deRham:2009rm}
  C.~de Rham,
  %``Massive gravity from Dirichlet boundary conditions,''
  Phys.\ Lett.\ B {\bf 688} (2010) 137
  [arXiv:0910.5474 [hep-th]].
  %%CITATION = ARXIV:0910.5474;%%
\bibitem{deRham:2010gu}
  C.~de Rham and G.~Gabadadze,
  %``Selftuned Massive Spin-2,''
  Phys.\ Lett.\ B {\bf 693} (2010) 334
  [arXiv:1006.4367 [hep-th]].
  %%CITATION = ARXIV:1006.4367;%%
\bibitem{Hassan:2011zr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Exact Solution to the 'Auxiliary Extra Dimension' Model of Massive Gravity,''
  Phys.\ Lett.\ B {\bf 702} (2011) 90
  [arXiv:1104.1373 [hep-th]].
  %%CITATION = ARXIV:1104.1373;%%
\bibitem{deRham:2010ik}
  C.~de Rham and G.~Gabadadze,
  %``Generalization of the Fierz-Pauli Action,''
  Phys.\ Rev.\ D {\bf 82} (2010) 044020
  [arXiv:1007.0443 [hep-th]].
  %%CITATION = ARXIV:1007.0443;%%
\bibitem{deRham:2010kj}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Resummation of Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 106} (2011) 231101
  [arXiv:1011.1232 [hep-th]].
  %%CITATION = ARXIV:1011.1232;%%
\bibitem{Mirbabayi:2011aa}
  M.~Mirbabayi,
  %``A Proof Of Ghost Freedom In de Rham-Gabadadze-Tolley Massive Gravity,''
  arXiv:1112.1435 [hep-th].
  %%CITATION = ARXIV:1112.1435;%%
\bibitem{deRham:2011rn}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Ghost free Massive Gravity in the St\'uckelberg language,''
  Phys.\ Lett.\ B {\bf 711} (2012) 190
  [arXiv:1107.3820 [hep-th]].
  %%CITATION = ARXIV:1107.3820;%%
\bibitem{Alberte:2010qb}
  L.~Alberte, A.~H.~Chamseddine and V.~Mukhanov,
  %``Massive Gravity: Exorcising the Ghost,''
  JHEP {\bf 1104} (2011) 004
  [arXiv:1011.0183 [hep-th]].
  %%CITATION = ARXIV:1011.0183;%%
\bibitem{Higuchi:1986py}
  A.~Higuchi,
  %``Forbidden Mass Range For Spin-2 Field Theory In De Sitter Space-time,''
  Nucl.\ Phys.\ B {\bf 282} (1987) 397.
  %%CITATION = NUPHA,B282,397;%%
\bibitem{Higuchi:1989gz}
  A.~Higuchi,
  %``Massive Symmetric Tensor Field In Space-times With A Positive Cosmological Constant,''
  Nucl.\ Phys.\ B {\bf 325} (1989) 745.
  %%CITATION = NUPHA,B325,745;%%
\bibitem{Porrati:2000cp}
  M.~Porrati,
  %``No van Dam-Veltman-Zakharov discontinuity in AdS space,''
  Phys.\ Lett.\ B {\bf 498} (2001) 92
  [hep-th/0011152].
  %%CITATION = HEP-TH/0011152;%%
\bibitem{Kogan:2000uy}
  I.~I.~Kogan, S.~Mouslopoulos and A.~Papazoglou,
  %``The m ---> 0 limit for massive graviton in dS(4) and AdS(4): How to circumvent the van Dam-Veltman-Zakharov discontinuity,''
  Phys.\ Lett.\ B {\bf 503} (2001) 173
  [hep-th/0011138].
  %%CITATION = HEP-TH/0011138;%%
\bibitem{Deser:2001pe}
  S.~Deser and A.~Waldron,
  %``Gauge invariances and phases of massive higher spins in (A)dS,''
  Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 031601
  [hep-th/0102166].
  %%CITATION = HEP-TH/0102166;%%
\bibitem{Deser:2001us}
  S.~Deser and A.~Waldron,
  %``Partial masslessness of higher spins in (A)dS,''
  Nucl.\ Phys.\ B {\bf 607} (2001) 577
  [hep-th/0103198].
  %%CITATION = HEP-TH/0103198;%%
\bibitem{Deser:2001wx}
  S.~Deser and A.~Waldron,
  %``Stability of massive cosmological gravitons,''
  Phys.\ Lett.\ B {\bf 508} (2001) 347
  [hep-th/0103255].
  %%CITATION = HEP-TH/0103255;%%
\bibitem{Grisa:2009yy}
  L.~Grisa and L.~Sorbo,
  %``Pauli-Fierz Gravitons on Friedmann-Robertson-Walker Background,''
  Phys.\ Lett.\ B {\bf 686} (2010) 273
  [arXiv:0905.3391 [hep-th]].
  %%CITATION = ARXIV:0905.3391;%%
\bibitem{Berkhahn:2010hc}
  F.~Berkhahn, D.~D.~Dietrich and S.~Hofmann,
  %``Self-Protection of Massive Cosmological Gravitons,''
  JCAP {\bf 1011} (2010) 018
  [arXiv:1008.0644 [hep-th]].
  %%CITATION = ARXIV:1008.0644;%%
\bibitem{Berkhahn:2011hb}
  F.~Berkhahn, D.~D.~Dietrich and S.~Hofmann,
  %``Consistency of Relevant Cosmological Deformations on all Scales,''
  JCAP {\bf 1109} (2011) 024
  [arXiv:1104.2534 [hep-th]].
  %%CITATION = ARXIV:1104.2534;%%
\bibitem{Damour:2002ws}
  T.~Damour and I.~I.~Kogan,
  %``Effective Lagrangians and universality classes of nonlinear
  %bigravity,'' 
  Phys.\ Rev.\ D {\bf 66} (2002) 104024
  [hep-th/0206042].
  %%CITATION = HEP-TH/0206042;%%
\bibitem{Damour:2002wu}
  T.~Damour, I.~I.~Kogan and A.~Papazoglou,
  %``Nonlinear bigravity and cosmic acceleration,''
  Phys.\ Rev.\ D {\bf 66} (2002) 104025
  [hep-th/0206044].
  %%CITATION = HEP-TH/0206044;%%
\bibitem{Hassan:2011vm}
  S.~F.~Hassan and R.~A.~Rosen,
  %``On nonlinear Actions for Massive Gravity,''
  JHEP {\bf 1107} (2011) 009
  [arXiv:1103.6055 [hep-th]].
  %%CITATION = ARXIV:1103.6055;%%
\bibitem{Hassan:2011hr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Resolving the Ghost Problem in nonlinear Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 108} (2012) 041101
  [arXiv:1106.3344 [hep-th]].
  %%CITATION = ARXIV:1106.3344;%%
\bibitem{Hassan:2011tf}
  S.~F.~Hassan, R.~A.~Rosen and A.~Schmidt-May,
  %``Ghost-free Massive Gravity with a General Reference Metric,''
  JHEP {\bf 1202} (2012) 026
  [arXiv:1109.3230 [hep-th]].
  %%CITATION = ARXIV:1109.3230;%%
\bibitem{Hassan:2011zd}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Bimetric Gravity from Ghost-free Massive Gravity,''
  JHEP {\bf 1202} (2012) 126
  [arXiv:1109.3515 [hep-th]].
  %%CITATION = ARXIV:1109.3515;%%
\bibitem{Hassan:2011ea}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Confirmation of the Secondary Constraint and Absence of Ghost in Massive Gravity and Bimetric Gravity,''
  JHEP {\bf 1204} (2012) 123
  [arXiv:1111.2070 [hep-th]].
  %%CITATION = ARXIV:1111.2070;%%
\bibitem{Arnowitt:1962hi}
  R.~L.~Arnowitt, S.~Deser and C.~W.~Misner,
  %``The Dynamics of general relativity,''
  [gr-qc/0405109].
  %%CITATION = GR-QC/0405109;%%
\bibitem{Kluson:2012wf}
  J.~Kluson,
  %``Non-Linear Massive Gravity with Additional Primary Constraint and
  %Absence of Ghosts,'' 
  arXiv:1204.2957 [hep-th].
  %%CITATION = ARXIV:1204.2957;%%
\bibitem{Kluson:2012zz}
  J.~Kluson,
  %``Note About Hamiltonian Formalism for General Non-Linear Massive Gravity Action in Stuckelberg Formalism,''
  arXiv:1209.3612 [hep-th].
  %%CITATION = ARXIV:1209.3612;%%
\bibitem{Paulos:2012xe}
  M.~F.~Paulos and A.~J.~Tolley,
  %``Massive Gravity Theories and limits of Ghost-free Bigravity models,''
  arXiv:1203.4268 [hep-th].
  %%CITATION = ARXIV:1203.4268;%%
\bibitem{mvsLovelock} %{\bfseries MISSING REFERENCE!!!}
S.~F.~Hassan, A.~Schmidt-May and M.~von~Strauss,
{\it In preparation}
\bibitem{Volkov:2011an}
  M.~S.~Volkov,
  %``Cosmological solutions with massive gravitons in the bigravity
  %theory,'' 
  JHEP {\bf 1201} (2012) 035
  [arXiv:1110.6153 [hep-th]].
  %%CITATION = ARXIV:1110.6153;%%
\bibitem{Comelli:2011zm}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``FRW Cosmology in ghost-free Massive Gravity,''
  JHEP {\bf 1203} (2012) 067
   [Erratum-ibid.\  {\bf 1206} (2012) 020]
  [arXiv:1111.1983 [hep-th]].
  %%CITATION = ARXIV:1111.1983;%%
\bibitem{Baccetti:2012bk}
  V.~Baccetti, P.~Martin-Moruno and M.~Visser,
  %``Massive gravity from bimetric gravity,''
  arXiv:1205.2158 [gr-qc].
  %%CITATION = ARXIV:1205.2158;%%
\bibitem{Hinterbichler:2012cn}
  K.~Hinterbichler and R.~A.~Rosen,
  %``Interacting Spin-2 Fields,''
  JHEP {\bf 1207} (2012) 047
  [arXiv:1203.5783 [hep-th]].
  %%CITATION = ARXIV:1203.5783;%%
\bibitem{Chamseddine:2011mu}
  A.~H.~Chamseddine and V.~Mukhanov,
  %``Massive Gravity Simplified: A Quadratic Action,''
  JHEP {\bf 1108} (2011) 091
  [arXiv:1106.5868 [hep-th]].
  %%CITATION = ARXIV:1106.5868;%%
\bibitem{Chamseddine:2011bu}
  A.~H.~Chamseddine and M.~S.~Volkov,
  %``Cosmological solutions with massive gravitons,''
  Phys.\ Lett.\ B {\bf 704} (2011) 652
  [arXiv:1107.5504 [hep-th]].
  %%CITATION = ARXIV:1107.5504;%%
\bibitem{Gumrukcuoglu:2011ew}
  A.~E.~Gumrukcuoglu, C.~Lin and S.~Mukohyama,
  %``Open FRW universes and self-acceleration from nonlinear massive gravity,''
  JCAP {\bf 1111} (2011) 030
  [arXiv:1109.3845 [hep-th]].
  %%CITATION = ARXIV:1109.3845;%%
\bibitem{Volkov:2012cf} 
  M.~S.~Volkov,
  %``Exact self-accelerating cosmologies in the ghost-free bigravity and massive gravity,''
  Phys.\ Rev.\ D {\bf 86}, 061502 (2012)
  [arXiv:1205.5713 [hep-th]].
  %%CITATION = ARXIV:1205.5713;%%
\bibitem{Koyama:2011wx}
  K.~Koyama, G.~Niz and G.~Tasinato,
  %``The Self-Accelerating Universe with Vectors in Massive Gravity,''
  JHEP {\bf 1112} (2011) 065
  [arXiv:1110.2618 [hep-th]].
  %%CITATION = ARXIV:1110.2618;%%
\bibitem{DeFelice:2012mx}
  A.~De Felice, A.~E.~Gumrukcuoglu, S.~Mukohyama, A.~E.~Gumrukcuoglu and S.~Mukohyama,
  %``Massive gravity: nonlinear instability of the homogeneous and isotropic universe,''
  Phys.\ Rev.\ Lett.\  {\bf 109} (2012) 171101
  [arXiv:1206.2080 [hep-th]].
  %%CITATION = ARXIV:1206.2080;%%
\bibitem{Tasinato:2012ze}
  G.~Tasinato, K.~Koyama and G.~Niz,
  %``Vector instabilities and self-acceleration in the decoupling limit of massive gravity,''
  arXiv:1210.3627 [hep-th].
  %%CITATION = ARXIV:1210.3627;%%
\bibitem{Comelli:2012db}
  D.~Comelli, M.~Crisostomi and L.~Pilo,
  %``Perturbations in Massive Gravity Cosmology,''
  JHEP {\bf 1206} (2012) 085
  [arXiv:1202.1986 [hep-th]].
  %%CITATION = ARXIV:1202.1986;%%
\bibitem{Berg:2012kn}
  M.~Berg, I.~Buchberger, J.~Enander, E.~Mortsell and S.~Sjors,
  %``Growth Histories in Bimetric Massive Gravity,''
  arXiv:1206.3496 [gr-qc].
  %%CITATION = ARXIV:1206.3496;%%
\bibitem{Mukhanov:2005sc}
  V.~Mukhanov,
  %``Physical foundations of cosmology,''
  Cambridge, UK: Univ. Pr. (2005) 421 p
\bibitem{Weinberg:2008zzc}
  S.~Weinberg,
  %``Cosmology,''
  Oxford, UK: Oxford Univ. Pr. (2008) 593 p
\bibitem{Komatsu:2010fb}
  E.~Komatsu {\it et al.}  [WMAP Collaboration],
  %``Seven-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Interpretation,''
  Astrophys.\ J.\ Suppl.\  {\bf 192} (2011) 18
  [arXiv:1001.4538 [astro-ph.CO]].
  %%CITATION = ARXIV:1001.4538;%%
\bibitem{de Urries:1998bi}
  F.~J.~de Urries and J.~Julve,
  %``Ostrogradski formalism for higher derivative scalar field theories,''
  J.\ Phys.\ A {\bf 31} (1998) 6949
  [hep-th/9802115].
  %%CITATION = HEP-TH/9802115;%%
\bibitem{Zwicky:1933gu}
  F.~Zwicky,
  %``Spectral displacement of extra galactic nebulae,''
  Helv.\ Phys.\ Acta {\bf 6} (1933) 110.
  %%CITATION = HPACA,6,110;%%
\bibitem{Rubin:1970zza}
  V.~C.~Rubin and W.~K.~Ford, Jr.,
  %``Rotation of the Andromeda Nebula from a Spectroscopic Survey of Emission Regions,''
  Astrophys.\ J.\  {\bf 159} (1970) 379.
  %%CITATION = ASJOA,159,379;%%
\bibitem{Rubin:1980zd}
  V.~C.~Rubin, N.~Thonnard and W.~K.~Ford, Jr.,
  %``Rotational properties of 21 SC galaxies with a large range of luminosities and radii, from NGC 4605 /R = 4kpc/ to UGC 2885 /R = 122 kpc/,''
  Astrophys.\ J.\  {\bf 238} (1980) 471.
  %%CITATION = ASJOA,238,471;%%
\bibitem{Rubin:1985ze}
  V.~C.~Rubin, D.~Burstein, W.~K.~Ford, Jr. and N.~Thonnard,
  %``Rotation velocities of 16 SA galaxies and a comparison of Sa, Sb, and SC rotation properties,''
  Astrophys.\ J.\  {\bf 289} (1985) 81.
  %%CITATION = ASJOA,289,81;%%
\bibitem{Clowe:2006eq}
  D.~Clowe, M.~Bradac, A.~H.~Gonzalez, M.~Markevitch, S.~W.~Randall, C.~Jones and D.~Zaritsky,
  %``A direct empirical proof of the existence of dark matter,''
  Astrophys.\ J.\  {\bf 648} (2006) L109
  [astro-ph/0608407].
  %%CITATION = ASTRO-PH/0608407;%%
\bibitem{Amanullah:2010vv}
  R.~Amanullah, C.~Lidman, D.~Rubin, G.~Aldering, P.~Astier, K.~Barbary, M.~S.~Burns and A.~Conley {\it et al.},
  %``Spectra and Light Curves of Six Type Ia Supernovae at 0.511 < z < 1.12 and the Union2 Compilation,''
  Astrophys.\ J.\  {\bf 716} (2010) 712
  [arXiv:1004.1711 [astro-ph.CO]].
  %%CITATION = ARXIV:1004.1711;%%
\bibitem{Iocco:2008va}
  F.~Iocco, G.~Mangano, G.~Miele, O.~Pisanti and P.~D.~Serpico,
  %``Primordial Nucleosynthesis: from precision cosmology to fundamental physics,''
  Phys.\ Rept.\  {\bf 472} (2009) 1
  [arXiv:0809.0631 [astro-ph]].
  %%CITATION = ARXIV:0809.0631;%%
\bibitem{Massey:2007wb}
  R.~Massey, J.~Rhodes, R.~Ellis, N.~Scoville, A.~Leauthaud, A.~Finoguenov, P.~Capak and D.~Bacon {\it et al.},
  %``Dark matter maps reveal cosmic scaffolding,''
  Nature {\bf 445} (2007) 286
  [astro-ph/0701594].
  %%CITATION = ASTRO-PH/0701594;%%
\bibitem{Allen:2002eu}
  S.~W.~Allen, A.~C.~Fabian, R.~W.~Schmidt and H.~Ebeling,
  %``Cosmological constraints from the local x-ray luminosity function of the most x-ray luminous galaxy clusters,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 342} (2003) 287
  [astro-ph/0208394].
  %%CITATION = ASTRO-PH/0208394;%%
\bibitem{Baumann:2009ds}
  D.~Baumann,
  %``TASI Lectures on Inflation,''
  arXiv:0907.5424 [hep-th].
  %%CITATION = ARXIV:0907.5424;%%
\bibitem{Akrami:2012vf}
  Y.~Akrami, T.~S.~Koivisto and M.~Sandstad,
  %``Accelerated expansion from ghost-free bigravity: a statistical analysis with improved generality,''
  arXiv:1209.0457 [astro-ph.CO].
  %%CITATION = ARXIV:1209.0457;%%
\bibitem{Bengtsson:1994vn} 
  I.~Bengtsson,
  %``Note on massive spin-2 in curved space,''
  J.\ Math.\ Phys.\  {\bf 36}, 5805 (1995)
  [gr-qc/9411057].
  %%CITATION = GR-QC/9411057;%%
\bibitem{Zinoviev:2001dt}
  Y.~.M.~Zinoviev,
  %``On massive high spin particles in AdS,''
  hep-th/0108192.
  %%CITATION = HEP-TH/0108192;%%
\bibitem{Zinoviev:2011fv}
  Y.~.M.~Zinoviev,
  %``Gravitational cubic interactions for a massive mixed symmetry gauge field,''
  Class.\ Quant.\ Grav.\  {\bf 29} (2012) 015013
  [arXiv:1107.3222 [hep-th]].
  %%CITATION = ARXIV:1107.3222;%%
\bibitem{deRham:2012kf}
  C.~de Rham and S.~Renaux-Petel,
  %``Massive Gravity on de Sitter and Unique Candidate for Partially
  %Massless Gravity,'' 
  arXiv:1206.3482 [hep-th].
  %%CITATION = ARXIV:1206.3482;%%
\bibitem{Joung:2012rv}
  E.~Joung, L.~Lopez and M.~Taronna,
  %``On the cubic interactions of massive and partially-massless higher spins in (A)dS,''
  JHEP {\bf 1207} (2012) 041
  [arXiv:1203.6578 [hep-th]].
  %%CITATION = ARXIV:1203.6578;%%
\bibitem{Lovelock:1971yv}
  D.~Lovelock,
  %``The Einstein tensor and its generalizations,''
  J.\ Math.\ Phys.\  {\bf 12} (1971) 498.
  %%CITATION = JMAPA,12,498;%%
\bibitem{Sisman:2012rc}
  T.~C.~Sisman, I.~Gullu and B.~Tekin,
  %``Spectra, vacua and the unitarity of Lovelock gravity in D-dimensional AdS spacetimes,''
  Phys.\ Rev.\ D {\bf 86} (2012) 044041
  [arXiv:1204.3814 [hep-th]].
  %%CITATION = ARXIV:1204.3814;%%  
\bibitem{Bergshoeff:2009aq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``More on Massive 3D Gravity,''
  Phys.\ Rev.\ D {\bf 79} (2009) 124042
  [arXiv:0905.1259 [hep-th]].
  %%CITATION = ARXIV:0905.1259;%%
\bibitem{Kleinschmidt:2012rs}
  A.~Kleinschmidt, T.~Nutma and A.~Virmani,
  %``On unitary subsectors of polycritical gravities,''
  Gen.\  Rel.\  Grav.\  {\bf 45} (2013) 727
  [arXiv:1206.7095 [hep-th]].
  %%CITATION = ARXIV:1206.7095;%%
\bibitem{Gullu:2010pc}
  I.~Gullu, T.~C.~Sisman and B.~Tekin,
  %``Born-Infeld extension of new massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 27} (2010) 162001
  [arXiv:1003.3935 [hep-th]].
  %%CITATION = ARXIV:1003.3935;%%
\bibitem{Paulos:2010ke}
  M.~F.~Paulos,
  %``New massive gravity extended with an arbitrary number of curvature corrections,''
  Phys.\ Rev.\ D {\bf 82} (2010) 084042
  [arXiv:1005.1646 [hep-th]].
  %%CITATION = ARXIV:1005.1646;%%
\bibitem{Kaku:1977pa}
  M.~Kaku, P.~K.~Townsend and P.~van Nieuwenhuizen,
  %``Gauge Theory of the Conformal and Superconformal Group,''
  Phys.\ Lett.\ B {\bf 69} (1977) 304.
  %%CITATION = PHLTA,B69,304;%%
\bibitem{Deser:2012qg}
  S.~Deser, E.~Joung and A.~Waldron,
  %``Partial Masslessness and Conformal Gravity,''
  J.\ Phys.\ A (2012)
  [arXiv:1208.1307 [hep-th]].
  %%CITATION = ARXIV:1208.1307;%%
\bibitem{Stelle:1976gc}
  K.~S.~Stelle,
  %``Renormalization of Higher Derivative Quantum Gravity,''
  Phys.\ Rev.\ D {\bf 16} (1977) 953.
  %%CITATION = PHRVA,D16,953;%%
\bibitem{Stelle:1977ry}
  K.~S.~Stelle,
  %``Classical Gravity with Higher Derivatives,''
  Gen.\ Rel.\ Grav.\  {\bf 9} (1978) 353.
  %%CITATION = GRGVA,9,353;%%
\bibitem{Bach}
  R.~Bach,
  Math.\ Zeitschr.\ {\bf 9} (1921) 110.
  %%CITATION = GRGVA,9,353;%%  
\bibitem{Fradkin:1981iu}
  E.~S.~Fradkin and A.~A.~Tseytlin,
  %``Renormalizable asymptotically free quantum theory of gravity,''
  Nucl.\ Phys.\ B {\bf 201} (1982) 469.
  %%CITATION = NUPHA,B201,469;%%  
\bibitem{Lee:1982cp}
  S.~C.~Lee and P.~van Nieuwenhuizen,
  %``Counting Of States In Higher Derivative Field Theories,''
  Phys.\ Rev.\ D {\bf 26} (1982) 934.
  %%CITATION = PHRVA,D26,934;%%
\bibitem{Riegert:1984hf}
  R.~J.~Riegert,
  %``The Particle Content Of Linearized Conformal Gravity,''
  Phys.\ Lett.\ A {\bf 105} (1984) 110.
  %%CITATION = PHLTA,A105,110;%%
\bibitem{Maldacena:2011mk}
  J.~Maldacena,
  %``Einstein Gravity from Conformal Gravity,''
  arXiv:1105.5632 [hep-th].
  %%CITATION = ARXIV:1105.5632;%%
\bibitem{Ade:2013ktc}
  P.~A.~R.~Ade {\it et al.}  [Planck Collaboration],
  %``Planck 2013 results. I. Overview of products and scientific results,''
  arXiv:1303.5062 [astro-ph.CO].
  %%CITATION = ARXIV:1303.5062;%%  
\bibitem{Hinshaw:2012aka}
  G.~Hinshaw {\it et al.}  [WMAP Collaboration],
  %``Nine-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Parameter Results,''
  arXiv:1212.5226 [astro-ph.CO].
  %%CITATION = ARXIV:1212.5226;%% 
\bibitem{Deser:1983mm}
  S.~Deser and R.~I.~Nepomechie,
  %``Gauge Invariance Versus Masslessness In De Sitter Space,''
  Annals Phys.\  {\bf 154} (1984) 396.
  %%CITATION = APNYA,154,396;%%
\bibitem{Deser:2001pe}
  S.~Deser and A.~Waldron,
  %``Gauge invariances and phases of massive higher spins in (A)dS,''
  Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 031601
  [hep-th/0102166].
  %%CITATION = HEP-TH/0102166;%%
 \bibitem{Deser:2001us}
  S.~Deser and A.~Waldron,
  %``Partial masslessness of higher spins in (A)dS,''
  Nucl.\ Phys.\ B {\bf 607} (2001) 577
  [hep-th/0103198].
  %%CITATION = HEP-TH/0103198;%%
\bibitem{Deser:2001wx}
  S.~Deser and A.~Waldron,
  %``Stability of massive cosmological gravitons,''
  Phys.\ Lett.\ B {\bf 508} (2001) 347
  [hep-th/0103255].
  %%CITATION = HEP-TH/0103255;%%
\bibitem{Deser:2001xr}
  S.~Deser and A.~Waldron,
  %``Null propagation of partially massless higher spins in (A)dS and cosmological constant speculations,''
  Phys.\ Lett.\ B {\bf 513} (2001) 137
  [hep-th/0105181].
  %%CITATION = HEP-TH/0105181;%%
\bibitem{Deser:2004ji}
  S.~Deser and A.~Waldron,
  %``Conformal invariance of partially massless higher spins,''
  Phys.\ Lett.\ B {\bf 603} (2004) 30
  [hep-th/0408155].
  %%CITATION = HEP-TH/0408155;%%  
\bibitem{Deser:2006zx}
  S.~Deser and A.~Waldron,
  %``Partially Massless Spin 2 Electrodynamics,''
  Phys.\ Rev.\ D {\bf 74} (2006) 084036
  [hep-th/0609113].
  %%CITATION = HEP-TH/0609113;%%
\bibitem{Higuchi:1986py}
  A.~Higuchi,
  %``Forbidden Mass Range For Spin-2 Field Theory In De Sitter Space-time,''
  Nucl.\ Phys.\ B {\bf 282} (1987) 397.
  %%CITATION = NUPHA,B282,397;%%
\bibitem{Higuchi:1989gz}
  A.~Higuchi,
  %``Massive Symmetric Tensor Field In Space-times With A Positive Cosmological Constant,''
  Nucl.\ Phys.\ B {\bf 325} (1989) 745.
  %%CITATION = NUPHA,B325,745;%%
\bibitem{Joung:2012rv}
  E.~Joung, L.~Lopez and M.~Taronna,
  %``On the cubic interactions of massive and partially-massless higher spins in (A)dS,''
  JHEP {\bf 1207} (2012) 041
  [arXiv:1203.6578 [hep-th]].
  %%CITATION = ARXIV:1203.6578;%%
\bibitem{Zinoviev:2006im}
  Y.~.M.~Zinoviev,
  %``On massive spin 2 interactions,''
  Nucl.\ Phys.\ B {\bf 770} (2007) 83
  [hep-th/0609170].
  %%CITATION = HEP-TH/0609170;%%
\bibitem{Deser:2013uy}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``Nonlinear Partially Massless from Massive Gravity?,''
  Phys.\  Rev.\  D 87, {\bf 101501} (R) (2013)
  [arXiv:1301.5621 [hep-th]].
  %%CITATION = ARXIV:1301.5621;%%
\bibitem{Garidi:2003ys}
  T.~Garidi,
  %``What is mass in de Sitterian physics?,''
  hep-th/0309104.
  %%CITATION = HEP-TH/0309104;%%  
\bibitem{deRham:2013wv}
  C.~de Rham, K.~Hinterbichler, R.~A.~Rosen and A.~J.~Tolley,
  %``Evidence for and Obstructions to Non-Linear Partially Massless Gravity,''
  arXiv:1302.0025 [hep-th].
  %%CITATION = ARXIV:1302.0025;%%  
\bibitem{deRham:2012kf}
  C.~de Rham and S.~Renaux-Petel,
  %``Massive Gravity on de Sitter and Unique Candidate for Partially Massless Gravity,''
  JCAP {\bf 1301} (2013) 035
  [arXiv:1206.3482 [hep-th]].
  %%CITATION = ARXIV:1206.3482;%% 
\bibitem{Akrami:2013ffa}
  Y.~Akrami, T.~S.~Koivisto, D.~F.~Mota and M.~Sandstad,
  %``Bimetric gravity doubly coupled to matter: theory and cosmological implications,''
  arXiv:1306.0004 [hep-th].
  %%CITATION = ARXIV:1306.0004;%%
\bibitem{Ruegg:2003ps}
  H.~Ruegg and M.~Ruiz-Altaba,
  %``The Stueckelberg field,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 19} (2004) 3265
  [hep-th/0304245].
  %%CITATION = HEP-TH/0304245;%%
\bibitem{Henneaux:1997bm}
  M.~Henneaux,
  %``Consistent interactions between gauge fields: The Cohomological approach,''
  Contemp.\ Math.\  {\bf 219} (1998) 93
  [hep-th/9712226].
  %%CITATION = HEP-TH/9712226;%%
\bibitem{Wigner:1939cj}
  E.~P.~Wigner,
  %``On Unitary Representations of the Inhomogeneous Lorentz Group,''
  Annals Math.\  {\bf 40} (1939) 149
   [Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 6} (1989) 9].
  %%CITATION = ANMAA,40,149;%%
\bibitem{Boulware:1972zf}
  D.~G.~Boulware and S.~Deser,
  %``Inconsistency of finite range gravitation,''
  Phys.\ Lett.\ B {\bf 40} (1972) 227.
  %%CITATION = PHLTA,B40,227;%%
\bibitem{ArkaniHamed:2003uy}
  N.~Arkani-Hamed, H.~-C.~Cheng, M.~A.~Luty and S.~Mukohyama,
  %``Ghost condensation and a consistent infrared modification of gravity,''
  JHEP {\bf 0405} (2004) 074
  [hep-th/0312099].
  %%CITATION = HEP-TH/0312099;%%
\bibitem{Kaluza:1921tu}
  T.~Kaluza,
  %``On the Problem of Unity in Physics,''
  Sitzungsber.\ Preuss.\ Akad.\ Wiss.\ Berlin (Math.\ Phys.\ ) {\bf 1921} (1921) 966.
  %%CITATION = SPWPA,1921,966;%%  
\bibitem{Klein:1926tv}
  O.~Klein,
  %``Quantum Theory and Five-Dimensional Theory of Relativity. (In German and English),''
  Z.\ Phys.\  {\bf 37} (1926) 895
   [Surveys High Energ.\ Phys.\  {\bf 5} (1986) 241].
  %%CITATION = ZEPYA,37,895;%% 
\bibitem{Einstein:1916vd}
  A.~Einstein,
  %``The Foundation of the General Theory of Relativity,''
  Annalen Phys.\  {\bf 49} (1916) 769
   [Annalen Phys.\  {\bf 14} (2005) 517].
  %%CITATION = ANPYA,49,769;%%   
\bibitem{Date:2010xr}
  G.~Date,
  %``Lectures on Constrained Systems,''
  arXiv:1010.2062 [gr-qc].
  %%CITATION = ARXIV:1010.2062;%%
\bibitem{Khoury:2011ay}
  J.~Khoury, G.~E.~J.~Miller and A.~J.~Tolley,
  %``Spatially Covariant Theories of a Transverse, Traceless Graviton, Part I: Formalism,''
  Phys.\ Rev.\ D {\bf 85} (2012) 084002
  [arXiv:1108.1397 [hep-th]].
  %%CITATION = ARXIV:1108.1397;%%
\bibitem{Kluson:2011qe}
  J.~Kluson,
  %``Note About Hamiltonian Structure of Non-Linear Massive Gravity,''
  JHEP {\bf 1201} (2012) 013
  [arXiv:1109.3052 [hep-th]].
  %%CITATION = ARXIV:1109.3052;%%
\bibitem{Kluson:2011rt}
  J.~Kluson,
  %``Comments About Hamiltonian Formulation of Non-Linear Massive Gravity with Stuckelberg Fields,''
  JHEP {\bf 1206} (2012) 170
  [arXiv:1112.5267 [hep-th]].
  %%CITATION = ARXIV:1112.5267;%%
\bibitem{Kluson:2012gz}
  J.~Kluson,
  %``Remark About Hamiltonian Formulation of Non-Linear Massive Gravity in Stuckelberg Formalism,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124005
  [arXiv:1202.5899 [hep-th]].
  %%CITATION = ARXIV:1202.5899;%%  
\bibitem{Lee:1977yc}
  B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
  %``The Strength of Weak Interactions at Very High-Energies and the Higgs Boson Mass,''
  Phys.\ Rev.\ Lett.\  {\bf 38} (1977) 883.
  %%CITATION = PRLTA,38,883;%%  
\bibitem{Golovnev:2011aa}
  A.~Golovnev,
  %``On the Hamiltonian analysis of non-linear massive gravity,''
  Phys.\ Lett.\ B {\bf 707} (2012) 404
  [arXiv:1112.2134 [gr-qc]].
  %%CITATION = ARXIV:1112.2134;%%
\bibitem{Buchbinder:2012wb}
  I.~L.~Buchbinder, D.~D.~Pereira and I.~L.~Shapiro,
  %``One-loop divergences in massive gravity theory,''
  Phys.\ Lett.\ B {\bf 712} (2012) 104
  [arXiv:1201.3145 [hep-th]].
  %%CITATION = ARXIV:1201.3145;%%
\bibitem{Boulanger:2000rq}
  N.~Boulanger, T.~Damour, L.~Gualtieri and M.~Henneaux,
  %``Inconsistency of interacting, multigraviton theories,''
  Nucl.\ Phys.\ B {\bf 597} (2001) 127
  [hep-th/0007220].
  %%CITATION = HEP-TH/0007220;%%  
\bibitem{Isham:1971gm}
  C.~J.~Isham, A.~Salam and J.~A.~Strathdee,
  %``F-dominance of gravity,''
  Phys.\ Rev.\ D {\bf 3} (1971) 867.
  %%CITATION = PHRVA,D3,867;%%  
\bibitem{deRham:2010tw}
  C.~de Rham, G.~Gabadadze, L.~Heisenberg and D.~Pirtskhalava,
  %``Cosmic Acceleration and the Helicity-0 Graviton,''
  Phys.\ Rev.\ D {\bf 83} (2011) 103516
  [arXiv:1010.1780 [hep-th]].
  %%CITATION = ARXIV:1010.1780;%%  
\bibitem{D'Amico:2011jj}
  G.~D'Amico, C.~de Rham, S.~Dubovsky, G.~Gabadadze, D.~Pirtskhalava and A.~J.~Tolley,
  %``Massive Cosmologies,''
  Phys.\ Rev.\ D {\bf 84} (2011) 124046
  [arXiv:1108.5231 [hep-th]].
  %%CITATION = ARXIV:1108.5231;%%    
\bibitem{Comelli:2011wq}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``Spherically Symmetric Solutions in Ghost-Free Massive Gravity,''
  Phys.\ Rev.\ D {\bf 85} (2012) 024044
  [arXiv:1110.4967 [hep-th]].
  %%CITATION = ARXIV:1110.4967;%%
\bibitem{Volkov:2012wp}
  M.~S.~Volkov,
  %``Hairy black holes in the ghost-free bigravity theory,''
  Phys.\ Rev.\ D {\bf 85} (2012) 124043
  [arXiv:1202.6682 [hep-th]].
  %%CITATION = ARXIV:1202.6682;%%
\bibitem{Deser:2013gpa}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``No consistent bimetric gravity?,''
  arXiv:1306.0647 [hep-th].
  %%CITATION = ARXIV:1306.0647;%%
\bibitem{Ostrogradski}
  M.~Ostrogradski,
  Mem.\ Ac.\ St.~Petersbourg  {\bf VI} (1850) 385. 
\bibitem{Bach}
  R.~Bach,
  Mathematische\ Zeitschrift  {\bf 9} (1921) 110. 
\bibitem{Mannheim:2011ds}
  P.~D.~Mannheim,
  %``Making the Case for Conformal Gravity,''
  Found.\ Phys.\  {\bf 42} (2012) 388
  [arXiv:1101.2186 [hep-th]].
  %%CITATION = ARXIV:1101.2186;%%  
\bibitem{Bender:2007wu}
  C.~M.~Bender and P.~D.~Mannheim,
  %``No-ghost theorem for the fourth-order derivative Pais-Uhlenbeck oscillator model,''
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 110402
  [arXiv:0706.0207 [hep-th]].    
\bibitem{Volkov:2013roa}
  M.~S.~Volkov,
  %``Self-accelerating cosmologies and hairy black holes in ghost-free bigravity and massive gravity,''
  arXiv:1304.0238 [hep-th].
  %%CITATION = ARXIV:1304.0238;%% 
\bibitem{Ondo:2013wka}
  N.~A.~Ondo and A.~J.~Tolley,
  %``Complete Decoupling Limit of Ghost-free Massive Gravity,''
  arXiv:1307.4769 [hep-th]. 
\bibitem{Gabadadze:2013ria}
  G.~Gabadadze, K.~Hinterbichler, D.~Pirtskhalava and Y.~Shang,
  %``On the Potential for General Relativity and its Geometry,''
  arXiv:1307.2245 [hep-th].
  %%CITATION = ARXIV:1307.2245;%%    
\bibitem{Deffayet:2012nr}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``Covariant constraints in ghost free massive gravity,''
  JCAP {\bf 1301} (2013) 032
  [arXiv:1207.6338 [hep-th]].
  %%CITATION = ARXIV:1207.6338;%%
\bibitem{Deffayet:2012zc}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``A note on 'symmetric' vielbeins in bimetric, massive, perturbative and non perturbative gravities,''
  JHEP {\bf 1303} (2013) 086
  [arXiv:1208.4493 [gr-qc]].
  %%CITATION = ARXIV:1208.4493;%% 
\bibitem{Brito:2013wya}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Massive spin-2 fields on black hole spacetimes: Instability of the Schwarzschild and Kerr solutions and bounds on the graviton mass,''
  Phys.\  Rev.\ D {\bf 88} (2013) 023514
  [arXiv:1304.6725 [gr-qc]].
  %%CITATION = ARXIV:1304.6725;%% 
\bibitem{Brito:2013yxa}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Partially massless gravitons do not destroy general relativity black holes,''
  Phys.\  Rev.\ D {\bf 87} (2013) 124024
  [arXiv:1306.0908 [gr-qc]].
  %%CITATION = ARXIV:1306.0908;%%   
\bibitem{Gregory:1993vy}
  R.~Gregory and R.~Laflamme,
  %``Black strings and p-branes are unstable,''
  Phys.\ Rev.\ Lett.\  {\bf 70} (1993) 2837
  [hep-th/9301052].
  %%CITATION = HEP-TH/9301052;%% 
\bibitem{Enander:2013kza}
  J.~Enander and E.~Mortsell,
  %``Strong lensing constraints on bimetric massive gravity,''
  arXiv:1306.1086 [astro-ph.CO].
  %%CITATION = ARXIV:1306.1086;%%   
\bibitem{Babichev:2013una}
  E.~Babichev and A.~Fabbri,
  %``Instability of black holes in massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 30} (2013) 152001
  [arXiv:1304.5992 [gr-qc]].
  %%CITATION = ARXIV:1304.5992;%%
\bibitem{Sjors:2011iv}
  S.~Sjors and E.~Mortsell,
  %``Spherically Symmetric Solutions in Massive Gravity and Constraints from Galaxies,''
  JHEP {\bf 1302} (2013) 080
  [arXiv:1111.5961 [gr-qc]].
  %%CITATION = ARXIV:1111.5961;%%
\bibitem{Hinterbichler:2013eza}
  K.~Hinterbichler,
  %``Ghost-Free Derivative Interactions for a Massive Graviton,''
  arXiv:1305.7227 [hep-th].
  %%CITATION = ARXIV:1305.7227;%%      
\bibitem{deRham:2013qqa}
  C.~de Rham, L.~Heisenberg and R.~H.~Ribeiro,
  %``Quantum Corrections in Massive Gravity,''
  arXiv:1307.7169 [hep-th].
  %%CITATION = ARXIV:1307.7169;%%  
\bibitem{Cai:2013lqa}
  Y.~-F.~Cai, F.~Duplessis and E.~N.~Saridakis,
  %``$F(R)$ nonlinear massive gravity and cosmological implications,''
  arXiv:1307.7150 [hep-th].
  %%CITATION = ARXIV:1307.7150;%%  
\bibitem{Gabadadze:2012tr}
  G.~Gabadadze, K.~Hinterbichler, J.~Khoury, D.~Pirtskhalava and M.~Trodden,
  %``A Covariant Master Theory for Novel Galilean Invariant Models and Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124004
  [arXiv:1208.5773 [hep-th]].
  %%CITATION = ARXIV:1208.5773;%%
\bibitem{D'Amico:2012zv}
  G.~D'Amico, G.~Gabadadze, L.~Hui and D.~Pirtskhalava,
  %``Quasi-Dilaton: Theory and Cosmology,''
  arXiv:1206.4253 [hep-th].
  %%CITATION = ARXIV:1206.4253;%%   
%\cite{Ondo:2013wka}
\bibitem{Ondo:2013wka}
  N.~A.~Ondo and A.~J.~Tolley,
  %``Complete Decoupling Limit of Ghost-free Massive Gravity,''
  arXiv:1307.4769 [hep-th].
  %%CITATION = ARXIV:1307.4769;%%  
\bibitem{Huang:2013mha}
  Q.~-G.~Huang, K.~-C.~Zhang and S.~-Y.~Zhou,
  %``Generalized massive gravity in arbitrary dimensions and its Hamiltonian formulation,''
  arXiv:1306.4740 [hep-th].
  %%CITATION = ARXIV:1306.4740;%%   
\bibitem{Nojiri:2013zza}
  S.~'I.~Nojiri and S.~D.~Odintsov,
  %``Accelerating cosmology in modified gravity: from convenient $F(R)$ or string-inspired theory to bimetric $F(R)$ gravity,''
  arXiv:1306.4426 [gr-qc].
  %%CITATION = ARXIV:1306.4426;%% 
\bibitem{Huang:2012pe}
  Q.~-G.~Huang, Y.~-S.~Piao and S.~-Y.~Zhou,
  %``Mass-Varying Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124014
  [arXiv:1206.5678 [hep-th]].
  %%CITATION = ARXIV:1206.5678;%% 
\bibitem{Nomura:2012xr}
  K.~Nomura and J.~Soda,
  %``When is Multimetric Gravity Ghost-free?,''
  Phys.\ Rev.\ D {\bf 86} (2012) 084052
  [arXiv:1207.3637 [hep-th]].
  %%CITATION = ARXIV:1207.3637;%%    
  
  
    
  
\end{thebibliography}


    
    

    
    
    
    

        
        
        
    




==> Bibliography/mvs_bm_biblist.tex <==
\begin{thebibliography}{999}
\bibitem{Rosen:1940zz}
  N.~Rosen,
  %``General Relativity and Flat Space. II,''
  Phys.\ Rev.\  {\bf 57} (1940) 150.
  %%CITATION = PHRVA,57,150;%%
\bibitem{ISS}
  C.~J.~Isham, A.~Salam and J.~A.~Strathdee,
  %``F-dominance of gravity,''
  Phys.\ Rev.\ D {\bf 3} (1971) 867.
  %%CITATION = PHRVA,D3,867;%%
 \bibitem{Aragone:1971kh}
  C.~Aragone and S.~Deser,
  %``Constraints on gravitationally coupled tensor fields,''
  Nuovo Cim.\ A {\bf 3} (1971) 709.
  %%CITATION = NUCIA,A3,709;%%
\bibitem{Rosen:1975kk}
  N.~Rosen,
  %``Bimetric Theory of Gravitation,''
  In *Erice 1975, Proceedings, Topics In Theoretical and Experimental
  Gravitation Physics*, New York 1977, 273-294 
\bibitem{Chamseddine:1978yu}
  A.~H.~Chamseddine, A.~Salam and J.~A.~Strathdee,
  %``Strong Gravity and Supersymmetry,''
  Nucl.\ Phys.\ B {\bf 136} (1978) 248.
  %%CITATION = NUPHA,B136,248;%%
\bibitem{Print-79-0993}
  C.~Aragone and S.~Deser,
  %``Consistency Problems Of Spin-2 Gravity Coupling,''
  Nuovo Cim.\ B {\bf 57} (1980) 33.
  %%CITATION = NUCIA,B57,33;%%
\bibitem{hep-th/9908028}
  I.~L.~Buchbinder, V.~A.~Krykhtin and V.~D.~Pershin,
  %``On consistent equations for massive spin two field coupled to
  %gravity in string theory,'' 
  Phys.\ Lett.\ B {\bf 466} (1999) 216
  [hep-th/9908028].
  %%CITATION = HEP-TH/9908028;%%
\bibitem{hep-th/9910188}
  I.~L.~Buchbinder, D.~M.~Gitman, V.~A.~Krykhtin and V.~D.~Pershin, 
  %``Equations of motion for massive spin-2 field coupled to
  %gravity,'' 
  Nucl.\ Phys.\ B {\bf 584} (2000) 615
  [hep-th/9910188].
  %%CITATION = HEP-TH/9910188;%%
\bibitem{Boulanger:2000rq}
  N.~Boulanger, T.~Damour, L.~Gualtieri and M.~Henneaux,
  %``Inconsistency of interacting, multigraviton theories,''
  Nucl.\ Phys.\ B {\bf 597} (2001) 127
  [hep-th/0007220].
  %%CITATION = HEP-TH/0007220;%%
\bibitem{Damour:2002ws}
  T.~Damour and I.~I.~Kogan,
  %``Effective Lagrangians and universality classes of nonlinear
  %bigravity,'' 
  Phys.\ Rev.\ D {\bf 66} (2002) 104024
  [hep-th/0206042].
  %%CITATION = HEP-TH/0206042;%%
\bibitem{Damour:2002wu}
  T.~Damour, I.~I.~Kogan and A.~Papazoglou,
  %``Nonlinear bigravity and cosmic acceleration,''
  Phys.\ Rev.\ D {\bf 66} (2002) 104025
  [hep-th/0206044].
  %%CITATION = HEP-TH/0206044;%%
\bibitem{ArkaniHamed:2002sp}
  N.~Arkani-Hamed, H.~Georgi and M.~D.~Schwartz,
  %``Effective field theory for massive gravitons and gravity in
  %theory space,'' 
  Annals Phys.\  {\bf 305} (2003) 96
  [hep-th/0210184].
  %%CITATION = HEP-TH/0210184;%%
\bibitem{Blas:2007zz}
  D.~Blas, C.~Deffayet and J.~Garriga,
  %``Bigravity and Lorentz-violating Massive Gravity,''
  Phys.\ Rev.\ D {\bf 76} (2007) 104036
  [arXiv:0705.1982 [hep-th]].
  %%CITATION = ARXIV:0705.1982;%%
\bibitem{Banados:2008fi}
  M.~Banados, A.~Gomberoff, D.~C.~Rodrigues and C.~Skordis,
  %``A Note on bigravity and dark matter,''
  Phys.\ Rev.\ D {\bf 79} (2009) 063515
  [arXiv:0811.1270 [gr-qc]].
  %%CITATION = ARXIV:0811.1270;%%
\bibitem{Milgrom:2009gv}
  M.~Milgrom,
  %``Bimetric MOND gravity,''
  Phys.\ Rev.\ D {\bf 80} (2009) 123536
  [arXiv:0912.0790 [gr-qc]].
  %%CITATION = ARXIV:0912.0790;%%
\bibitem{Boulware:1973my}
  D.~G.~Boulware and S.~Deser,
  %``Can gravitation have a finite range?,''
  Phys.\ Rev.\ D {\bf 6} (1972) 3368.
  %%CITATION = PHRVA,D6,3368;%%
\bibitem{Hassan:2011zd}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Bimetric Gravity from Ghost-free Massive Gravity,''
  JHEP {\bf 1202} (2012) 126
  [arXiv:1109.3515 [hep-th]].
  %%CITATION = ARXIV:1109.3515;%%
\bibitem{arXiv:1111.2070}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Confirmation of the Secondary Constraint and Absence of Ghost in
  %Massive Gravity and Bimetric Gravity,'' 
  JHEP {\bf 1204} (2012) 123
  [arXiv:1111.2070 [hep-th]].
  %%CITATION = ARXIV:1111.2070;%%
\bibitem{Hassan:2011vm}
  S.~F.~Hassan and R.~A.~Rosen,
  %``On nonlinear Actions for Massive Gravity,''
  JHEP {\bf 1107} (2011) 009
  [arXiv:1103.6055 [hep-th]].
  %%CITATION = ARXIV:1103.6055;%%
\bibitem{Hassan:2011hr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Resolving the Ghost Problem in nonlinear Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 108} (2012) 041101
  [arXiv:1106.3344 [hep-th]].
  %%CITATION = ARXIV:1106.3344;%%
\bibitem{Hassan:2011tf}
  S.~F.~Hassan, R.~A.~Rosen and A.~Schmidt-May,
  %``Ghost-free Massive Gravity with a General Reference Metric,''
  JHEP {\bf 1202} (2012) 026
  [arXiv:1109.3230 [hep-th]].
  %%CITATION = ARXIV:1109.3230;%%
\bibitem{deRham:2010ik}
  C.~de Rham and G.~Gabadadze,
  %``Generalization of the Fierz-Pauli Action,''
  Phys.\ Rev.\ D {\bf 82} (2010) 044020
  [arXiv:1007.0443 [hep-th]].
  %%CITATION = ARXIV:1007.0443;%%
\bibitem{deRham:2010kj}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Resummation of Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 106} (2011) 231101
  [arXiv:1011.1232 [hep-th]].
  %%CITATION = ARXIV:1011.1232;%%
\bibitem{Hinterbichler:2012cn}
  K.~Hinterbichler and R.~A.~Rosen,
  %``Interacting Spin-2 Fields,''
  JHEP {\bf 1207} (2012) 047
  [arXiv:1203.5783 [hep-th]].
  %%CITATION = ARXIV:1203.5783;%%
\bibitem{Hassan:2012wt}
  S.~F.~Hassan, A.~Schmidt-May and M.~von Strauss,
  %``Metric Formulation of Ghost-Free Multivielbein Theory,''
  arXiv:1204.5202 [hep-th].
  %%CITATION = ARXIV:1204.5202;%%
\bibitem{Volkov:2011an}
  M.~S.~Volkov,
  %``Cosmological solutions with massive gravitons in the bigravity
  %theory,'' 
  JHEP {\bf 1201} (2012) 035
  [arXiv:1110.6153 [hep-th]].
  %%CITATION = ARXIV:1110.6153;%%
\bibitem{Volkov:2012wp}
  M.~S.~Volkov,
  %``Hairy black holes in the ghost-free bigravity theory,''
  arXiv:1202.6682 [hep-th].
  %%CITATION = ARXIV:1202.6682;%%
\bibitem{vonStrauss:2011mq}
  M.~von Strauss, A.~Schmidt-May, J.~Enander, E.~Mortsell and
  S.~F.~Hassan, 
  %``Cosmological Solutions in Bimetric Gravity and their
  %Observational Tests,'' 
  JCAP {\bf 1203} (2012) 042
  [arXiv:1111.1655 [gr-qc]].
  %%CITATION = ARXIV:1111.1655;%%
\bibitem{Comelli:2011wq}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``Spherically Symmetric Solutions in Ghost-Free Massive Gravity,''
  Phys.\ Rev.\ D {\bf 85} (2012) 024044
  [arXiv:1110.4967 [hep-th]].
  %%CITATION = ARXIV:1110.4967;%%
\bibitem{Comelli:2011zm}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``FRW Cosmology in ghost-free Massive Gravity,''
  JHEP {\bf 1203} (2012) 067
   [Erratum-ibid.\  {\bf 1206} (2012) 020]
  [arXiv:1111.1983 [hep-th]].
  %%CITATION = ARXIV:1111.1983;%%
\bibitem{Baccetti:2012ge}
  V.~Baccetti, P.~Martin-Moruno and M.~Visser,
  %``Gordon and Kerr-Schild ansatze in massive and bimetric gravity,''
  arXiv:1206.4720 [gr-qc].
  %%CITATION = ARXIV:1206.4720;%%
\bibitem{Deffayet:2011rh}
  C.~Deffayet and T.~Jacobson,
  %``On horizon structure of bimetric spacetimes,''
  Class.\ Quant.\ Grav.\  {\bf 29} (2012) 065009
  [arXiv:1107.4978 [gr-qc]].
  %%CITATION = ARXIV:1107.4978;%%
\bibitem{Fierz:1939ix}
  M.~Fierz and W.~Pauli,
  %``On relativistic wave equations for particles of arbitrary spin in 
  %an electromagnetic field,'' 
  Proc.\ Roy.\ Soc.\ Lond.\ A {\bf 173} (1939) 211.
  %%CITATION = PRSLA,A173,211;%%
\bibitem{Pauli:1939xp}
  W.~Pauli and M.~Fierz,
  %``On Relativistic Field Equations Of Particles With Arbitrary Spin
  %In An Electromagnetic Field,'' 
  Helv.\ Phys.\ Acta {\bf 12} (1939) 297.
  %%CITATION = HPACA,12,297;%%
\bibitem{Creminelli:2005qk}
  P.~Creminelli, A.~Nicolis, M.~Papucci and E.~Trincherini,
  %``Ghosts in massive gravity,''
  JHEP {\bf 0509} (2005) 003
  [hep-th/0505147].
  %%CITATION = HEP-TH/0505147;%%
\bibitem{Arnowitt:1962hi}
  R.~L.~Arnowitt, S.~Deser and C.~W.~Misner,
  %``The Dynamics of general relativity,''
  [gr-qc/0405109].
  %%CITATION = GR-QC/0405109;%%
\bibitem{Mirbabayi:2011aa}
  M.~Mirbabayi,
  %``A Proof Of Ghost Freedom In de Rham-Gabadadze-Tolley Massive Gravity,''
  arXiv:1112.1435 [hep-th].
  %%CITATION = ARXIV:1112.1435;%%
\bibitem{deRham:2012kf}
  C.~de Rham and S.~Renaux-Petel,
  %``Massive Gravity on de Sitter and Unique Candidate for Partially
  %Massless Gravity,'' 
  arXiv:1206.3482 [hep-th].
  %%CITATION = ARXIV:1206.3482;%%
\bibitem{Kluson:2011qe}
  J.~Kluson,
  %``Note About Hamiltonian Structure of Non-Linear Massive Gravity,''
  JHEP {\bf 1201} (2012) 013
  [arXiv:1109.3052 [hep-th]].
  %%CITATION = ARXIV:1109.3052;%%
\bibitem{Hassan:2012qv}
  S.~F.~Hassan, A.~Schmidt-May and M.~von Strauss,
  %``Proof of Consistency of Nonlinear Massive Gravity in the
  %St\'uckelberg Formulation,'' 
  arXiv:1203.5283 [hep-th].
  %%CITATION = ARXIV:1203.5283;%%
\bibitem{Kluson:2012wf}
  J.~Kluson,
  %``Non-Linear Massive Gravity with Additional Primary Constraint and
  %Absence of Ghosts,'' 
  arXiv:1204.2957 [hep-th].
  %%CITATION = ARXIV:1204.2957;%%
\bibitem{Baccetti:2012bk}
  V.~Baccetti, P.~Martin-Moruno and M.~Visser,
  %``Massive gravity from bimetric gravity,''
  arXiv:1205.2158 [gr-qc].
  %%CITATION = ARXIV:1205.2158;%%
\bibitem{Baccetti:2012re}
  V.~Baccetti, P.~Martin-Moruno and M.~Visser,
  %``Null Energy Condition violations in bimetric gravity,''
  arXiv:1206.3814 [gr-qc].
  %%CITATION = ARXIV:1206.3814;%%
\bibitem{Gumrukcuoglu:2011zh}
  A.~E.~Gumrukcuoglu, C.~Lin and S.~Mukohyama,
  %``Cosmological perturbations of self-accelerating universe in
  %nonlinear massive gravity,'' 
  JCAP {\bf 1203} (2012) 006
  [arXiv:1111.4107 [hep-th]].
  %%CITATION = ARXIV:1111.4107;%%
\bibitem{Crisostomi:2012db}
  M.~Crisostomi, D.~Comelli and L.~Pilo,
  %``Perturbations in Massive Gravity Cosmology,''
  JHEP {\bf 1206} (2012) 085
  [arXiv:1202.1986 [hep-th]].
  %%CITATION = ARXIV:1202.1986;%%
\bibitem{Berg:2012kn}
  M.~Berg, I.~Buchberger, J.~Enander, E.~Mortsell and S.~Sjors,
  %``Growth Histories in Bimetric Massive Gravity,''
  arXiv:1206.3496 [gr-qc].
  %%CITATION = ARXIV:1206.3496;%%
\bibitem{Paulos:2012xe}
  M.~F.~Paulos and A.~J.~Tolley,
  %``Massive Gravity Theories and limits of Ghost-free Bigravity models,''
  arXiv:1203.4268 [hep-th].
  %%CITATION = ARXIV:1203.4268;%%
\bibitem{Ortin:2004ms}
  T.~Ortin,
  %``Gravity and strings,''
  Cambridge Unversity, Cambridge University Press, 2004
\bibitem{Grinstein:2012pn}
  B.~Grinstein, C.~W.~Murphy, D.~Pirtskhalava and P.~Uttayarat,
  %``Massive Spin-2 States as the Origin of the Top Quark
  %Forward-Backward Asymmetry,'' 
  arXiv:1203.2183 [hep-ph].
  %%CITATION = ARXIV:1203.2183;%%
\bibitem{Wald:1984rg}
  R.~M.~Wald,
  %``General Relativity,''
  Chicago, Usa: Univ. Pr. ( 1984) 491p.
\bibitem{Hubble:1926yw}
  E.~P.~Hubble,
  %``Extragalactic nebulae,''
  Astrophys.\ J.\  {\bf 64} (1926) 321.
  %%CITATION = ASJOA,64,321;%%
 \bibitem{Hubble:1929ig}
  E.~Hubble,
  %``A relation between distance and radial velocity among extra-galactic nebulae,''
  Proc.\ Nat.\ Acad.\ Sci.\  {\bf 15} (1929) 168.
  %%CITATION = PNASA,15,168;%%
\bibitem{Randall:1998uk}
  L.~Randall and R.~Sundrum,
  %``Out of this world supersymmetry breaking,''
  Nucl.\ Phys.\ B {\bf 557} (1999) 79
  [hep-th/9810155].
  %%CITATION = HEP-TH/9810155;%%
\bibitem{ArkaniHamed:1998rs}
  N.~Arkani-Hamed, S.~Dimopoulos and G.~R.~Dvali,
  %``The Hierarchy problem and new dimensions at a millimeter,''
  Phys.\ Lett.\ B {\bf 429} (1998) 263
  [hep-ph/9803315].
  %%CITATION = HEP-PH/9803315;%%
\bibitem{Antoniadis:1998ig}
  I.~Antoniadis, N.~Arkani-Hamed, S.~Dimopoulos and G.~R.~Dvali,
  %``New dimensions at a millimeter to a Fermi and superstrings at a TeV,''
  Phys.\ Lett.\ B {\bf 436} (1998) 257
  [hep-ph/9804398].
  %%CITATION = HEP-PH/9804398;%%
\bibitem{Dvali:2000rv}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``Metastable gravitons and infinite volume extra dimensions,''
  Phys.\ Lett.\ B {\bf 484} (2000) 112
  [hep-th/0002190].
  %%CITATION = HEP-TH/0002190;%%
\bibitem{Dvali:2000hr}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``4-D gravity on a brane in 5-D Minkowski space,''
  Phys.\ Lett.\ B {\bf 485} (2000) 208
  [hep-th/0005016].
  %%CITATION = HEP-TH/0005016;%%
\bibitem{Dvali:2001gm}
  G.~R.~Dvali, G.~Gabadadze, M.~Kolanovic and F.~Nitti,
  %``The Power of brane induced gravity,''
  Phys.\ Rev.\ D {\bf 64} (2001) 084004
  [hep-ph/0102216].
  %%CITATION = HEP-PH/0102216;%%
\bibitem{Weinberg:1988cp}
  S.~Weinberg,
  %``The Cosmological Constant Problem,''
  Rev.\ Mod.\ Phys.\  {\bf 61} (1989) 1.
  %%CITATION = RMPHA,61,1;%%
\bibitem{Gregory:2000jc}
  R.~Gregory, V.~A.~Rubakov and S.~M.~Sibiryakov,
  %``Opening up extra dimensions at ultra large scales,''
  Phys.\ Rev.\ Lett.\  {\bf 84} (2000) 5928
  [hep-th/0002072].
  %%CITATION = HEP-TH/0002072;%%
\bibitem{Deffayet:2007zz}
  C.~Deffayet,
  %``The vDVZ discontinuity, DGP gravity, and cosmology,''
  Int.\ J.\ Theor.\ Phys.\  {\bf 46} (2007) 2242.
  %%CITATION = IJTPB,46,2242;%%
\bibitem{Dubovsky:2002jm}
  S.~L.~Dubovsky and V.~A.~Rubakov,
  %``Brane induced gravity in more than one extra dimensions: Violation of equivalence principle and ghost,''
  Phys.\ Rev.\ D {\bf 67} (2003) 104014
  [hep-th/0212222].
  %%CITATION = HEP-TH/0212222;%%
\bibitem{ArkaniHamed:2002sp}
  N.~Arkani-Hamed, H.~Georgi and M.~D.~Schwartz,
  %``Effective field theory for massive gravitons and gravity in theory space,''
  Annals Phys.\  {\bf 305} (2003) 96
  [hep-th/0210184].
  %%CITATION = HEP-TH/0210184;%%
\bibitem{Creminelli:2005qk}
  P.~Creminelli, A.~Nicolis, M.~Papucci and E.~Trincherini,
  %``Ghosts in massive gravity,''
  JHEP {\bf 0509} (2005) 003
  [hep-th/0505147].
  %%CITATION = HEP-TH/0505147;%%
\bibitem{Nibbelink:2006sz}
  S.~Nibbelink Groot, M.~Peloso and M.~Sexton,
  %``Nonlinear Properties of Vielbein Massive Gravity,''
  Eur.\ Phys.\ J.\ C {\bf 51} (2007) 741
  [hep-th/0610169].
  %%CITATION = HEP-TH/0610169;%%
\bibitem{Gabadadze:2009ja}
  G.~Gabadadze,
  %``General Relativity With An Auxiliary Dimension,''
  Phys.\ Lett.\ B {\bf 681} (2009) 89
  [arXiv:0908.1112 [hep-th]].
  %%CITATION = ARXIV:0908.1112;%%
\bibitem{deRham:2009rm}
  C.~de Rham,
  %``Massive gravity from Dirichlet boundary conditions,''
  Phys.\ Lett.\ B {\bf 688} (2010) 137
  [arXiv:0910.5474 [hep-th]].
  %%CITATION = ARXIV:0910.5474;%%
\bibitem{deRham:2010gu}
  C.~de Rham and G.~Gabadadze,
  %``Selftuned Massive Spin-2,''
  Phys.\ Lett.\ B {\bf 693} (2010) 334
  [arXiv:1006.4367 [hep-th]].
  %%CITATION = ARXIV:1006.4367;%%
\bibitem{Hassan:2011zr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Exact Solution to the 'Auxiliary Extra Dimension' Model of Massive Gravity,''
  Phys.\ Lett.\ B {\bf 702} (2011) 90
  [arXiv:1104.1373 [hep-th]].
  %%CITATION = ARXIV:1104.1373;%%
\bibitem{deRham:2010ik}
  C.~de Rham and G.~Gabadadze,
  %``Generalization of the Fierz-Pauli Action,''
  Phys.\ Rev.\ D {\bf 82} (2010) 044020
  [arXiv:1007.0443 [hep-th]].
  %%CITATION = ARXIV:1007.0443;%%
\bibitem{Mirbabayi:2011aa}
  M.~Mirbabayi,
  %``A Proof Of Ghost Freedom In de Rham-Gabadadze-Tolley Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 084006
  [arXiv:1112.1435 [hep-th]].
  %%CITATION = ARXIV:1112.1435;%%
\bibitem{deRham:2010kj}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Resummation of Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 106} (2011) 231101
  [arXiv:1011.1232 [hep-th]].
  %%CITATION = ARXIV:1011.1232;%%
\bibitem{deRham:2011rn}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Ghost free Massive Gravity in the St\'uckelberg language,''
  Phys.\ Lett.\ B {\bf 711} (2012) 190
  [arXiv:1107.3820 [hep-th]].
  %%CITATION = ARXIV:1107.3820;%%
\bibitem{Alberte:2010qb}
  L.~Alberte, A.~H.~Chamseddine and V.~Mukhanov,
  %``Massive Gravity: Exorcising the Ghost,''
  JHEP {\bf 1104} (2011) 004
  [arXiv:1011.0183 [hep-th]].
  %%CITATION = ARXIV:1011.0183;%%
\bibitem{Deser:2001pe}
  S.~Deser and A.~Waldron,
  %``Gauge invariances and phases of massive higher spins in (A)dS,''
  Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 031601
  [hep-th/0102166].
  %%CITATION = HEP-TH/0102166;%%
\bibitem{Deser:2001us}
  S.~Deser and A.~Waldron,
  %``Partial masslessness of higher spins in (A)dS,''
  Nucl.\ Phys.\ B {\bf 607} (2001) 577
  [hep-th/0103198].
  %%CITATION = HEP-TH/0103198;%%
\bibitem{Deser:2001wx}
  S.~Deser and A.~Waldron,
  %``Stability of massive cosmological gravitons,''
  Phys.\ Lett.\ B {\bf 508} (2001) 347
  [hep-th/0103255].
  %%CITATION = HEP-TH/0103255;%%
\bibitem{Higuchi:1986py}
  A.~Higuchi,
  %``Forbidden Mass Range For Spin-2 Field Theory In De Sitter Space-time,''
  Nucl.\ Phys.\ B {\bf 282} (1987) 397.
  %%CITATION = NUPHA,B282,397;%%
\bibitem{Higuchi:1989gz}
  A.~Higuchi,
  %``Massive Symmetric Tensor Field In Space-times With A Positive Cosmological Constant,''
  Nucl.\ Phys.\ B {\bf 325} (1989) 745.
  %%CITATION = NUPHA,B325,745;%%
\bibitem{ArkaniHamed:2003uy}
  N.~Arkani-Hamed, H.~-C.~Cheng, M.~A.~Luty and S.~Mukohyama,
  %``Ghost condensation and a consistent infrared modification of gravity,''
  JHEP {\bf 0405} (2004) 074
  [hep-th/0312099].
  %%CITATION = HEP-TH/0312099;%%
\bibitem{Rubakov:2004eb}
  V.~A.~Rubakov,
  %``Lorentz-violating graviton masses: Getting around ghosts, low strong coupling scale and VDVZ discontinuity,''
  hep-th/0407104.
  %%CITATION = HEP-TH/0407104;%%
\bibitem{Dubovsky:2004sg}
  S.~L.~Dubovsky,
  %``Phases of massive gravity,''
  JHEP {\bf 0410} (2004) 076
  [hep-th/0409124].
  %%CITATION = HEP-TH/0409124;%%
\bibitem{Hassan:2011vm}
  S.~F.~Hassan and R.~A.~Rosen,
  %``On Non-Linear Actions for Massive Gravity,''
  JHEP {\bf 1107} (2011) 009
  [arXiv:1103.6055 [hep-th]].
  %%CITATION = ARXIV:1103.6055;%%
\bibitem{Hassan:2011hr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Resolving the Ghost Problem in non-Linear Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 108} (2012) 041101
  [arXiv:1106.3344 [hep-th]].
  %%CITATION = ARXIV:1106.3344;%%
\bibitem{Hassan:2011tf}
  S.~F.~Hassan, R.~A.~Rosen and A.~Schmidt-May,
  %``Ghost-free Massive Gravity with a General Reference Metric,''
  JHEP {\bf 1202} (2012) 026
  [arXiv:1109.3230 [hep-th]].
  %%CITATION = ARXIV:1109.3230;%%
\bibitem{Hassan:2011zd}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Bimetric Gravity from Ghost-free Massive Gravity,''
  JHEP {\bf 1202} (2012) 126
  [arXiv:1109.3515 [hep-th]].
  %%CITATION = ARXIV:1109.3515;%%
\bibitem{Hassan:2011ea}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Confirmation of the Secondary Constraint and Absence of Ghost in Massive Gravity and Bimetric Gravity,''
  JHEP {\bf 1204} (2012) 123
  [arXiv:1111.2070 [hep-th]].
  %%CITATION = ARXIV:1111.2070;%%
\bibitem{Porrati:2000cp}
  M.~Porrati,
  %``No van Dam-Veltman-Zakharov discontinuity in AdS space,''
  Phys.\ Lett.\ B {\bf 498} (2001) 92
  [hep-th/0011152].
  %%CITATION = HEP-TH/0011152;%%
\bibitem{Kogan:2000uy}
  I.~I.~Kogan, S.~Mouslopoulos and A.~Papazoglou,
  %``The m ---> 0 limit for massive graviton in dS(4) and AdS(4): How to circumvent the van Dam-Veltman-Zakharov discontinuity,''
  Phys.\ Lett.\ B {\bf 503} (2001) 173
  [hep-th/0011138].
  %%CITATION = HEP-TH/0011138;%%
\bibitem{Grisa:2009yy}
  L.~Grisa and L.~Sorbo,
  %``Pauli-Fierz Gravitons on Friedmann-Robertson-Walker Background,''
  Phys.\ Lett.\ B {\bf 686} (2010) 273
  [arXiv:0905.3391 [hep-th]].
  %%CITATION = ARXIV:0905.3391;%%
\bibitem{Berkhahn:2010hc}
  F.~Berkhahn, D.~D.~Dietrich and S.~Hofmann,
  %``Self-Protection of Massive Cosmological Gravitons,''
  JCAP {\bf 1011} (2010) 018
  [arXiv:1008.0644 [hep-th]].
  %%CITATION = ARXIV:1008.0644;%%
\bibitem{Berkhahn:2011hb}
  F.~Berkhahn, D.~D.~Dietrich and S.~Hofmann,
  %``Consistency of Relevant Cosmological Deformations on all Scales,''
  JCAP {\bf 1109} (2011) 024
  [arXiv:1104.2534 [hep-th]].
  %%CITATION = ARXIV:1104.2534;%%
\bibitem{Paulos:2012xe}
  M.~F.~Paulos and A.~J.~Tolley,
  %``Massive Gravity Theories and limits of Ghost-free Bigravity models,''
  JHEP {\bf 1209} (2012) 002
  [arXiv:1203.4268 [hep-th]].
  %%CITATION = ARXIV:1203.4268;%%
\bibitem{Baccetti:2012bk}
  V.~Baccetti, P.~Martin-Moruno and M.~Visser,
  %``Massive gravity from bimetric gravity,''
  arXiv:1205.2158 [gr-qc].
  %%CITATION = ARXIV:1205.2158;%%
\bibitem{Visser:1997hd}
  M.~Visser,
  %``Mass for the graviton,''
  Gen.\ Rel.\ Grav.\  {\bf 30} (1998) 1717
  [gr-qc/9705051].
  %%CITATION = GR-QC/9705051;%%
\bibitem{Chamseddine:2011mu}
  A.~H.~Chamseddine and V.~Mukhanov,
  %``Massive Gravity Simplified: A Quadratic Action,''
  JHEP {\bf 1108} (2011) 091
  [arXiv:1106.5868 [hep-th]].
  %%CITATION = ARXIV:1106.5868;%%
\bibitem{Chamseddine:2011bu}
  A.~H.~Chamseddine and M.~S.~Volkov,
  %``Cosmological solutions with massive gravitons,''
  Phys.\ Lett.\ B {\bf 704} (2011) 652
  [arXiv:1107.5504 [hep-th]].
  %%CITATION = ARXIV:1107.5504;%%
\bibitem{Koyama:2011wx}
  K.~Koyama, G.~Niz and G.~Tasinato,
  %``The Self-Accelerating Universe with Vectors in Massive Gravity,''
  JHEP {\bf 1112} (2011) 065
  [arXiv:1110.2618 [hep-th]].
  %%CITATION = ARXIV:1110.2618;%%
\bibitem{DeFelice:2012mx}
  A.~De Felice, A.~E.~Gumrukcuoglu, S.~Mukohyama, A.~E.~Gumrukcuoglu and S.~Mukohyama,
  %``Massive gravity: nonlinear instability of the homogeneous and isotropic universe,''
  Phys.\ Rev.\ Lett.\  {\bf 109} (2012) 171101
  [arXiv:1206.2080 [hep-th]].
  %%CITATION = ARXIV:1206.2080;%%
\bibitem{Tasinato:2012ze}
  G.~Tasinato, K.~Koyama and G.~Niz,
  %``Vector instabilities and self-acceleration in the decoupling limit of massive gravity,''
  arXiv:1210.3627 [hep-th].
  %%CITATION = ARXIV:1210.3627;%%
\bibitem{Comelli:2012db}
  D.~Comelli, M.~Crisostomi and L.~Pilo,
  %``Perturbations in Massive Gravity Cosmology,''
  JHEP {\bf 1206} (2012) 085
  [arXiv:1202.1986 [hep-th]].
  %%CITATION = ARXIV:1202.1986;%%
\bibitem{Berg:2012kn}
  M.~Berg, I.~Buchberger, J.~Enander, E.~Mortsell and S.~Sjors,
  %``Growth Histories in Bimetric Massive Gravity,''
  arXiv:1206.3496 [gr-qc].
  %%CITATION = ARXIV:1206.3496;%%
\bibitem{Martin:2012bt}
  J.~Martin,
  %``Everything You Always Wanted To Know About The Cosmological Constant Problem (But Were Afraid To Ask),''
  Comptes Rendus Physique {\bf 13} (2012) 566
  [arXiv:1205.3365 [astro-ph.CO]].
  %%CITATION = ARXIV:1205.3365;%%
\bibitem{Jaffe:2005vp}
  R.~L.~Jaffe,
  %``The Casimir effect and the quantum vacuum,''
  Phys.\ Rev.\ D {\bf 72} (2005) 021301
  [hep-th/0503158].
  %%CITATION = HEP-TH/0503158;%%
\bibitem{Dvali:2002pe}
  G.~Dvali, G.~Gabadadze and M.~Shifman,
  %``Diluting cosmological constant in infinite volume extra dimensions,''
  Phys.\ Rev.\ D {\bf 67} (2003) 044020
  [hep-th/0202174].
  %%CITATION = HEP-TH/0202174;%%
\bibitem{Dvali:2002fz}
  G.~Dvali, G.~Gabadadze and M.~Shifman,
  %``Diluting cosmological constant via large distance modification of gravity,''
  hep-th/0208096.
  %%CITATION = HEP-TH/0208096;%%
\bibitem{vanDam:1970vg}
  H.~van Dam and M.~J.~G.~Veltman,
  %``Massive and massless Yang-Mills and gravitational fields,''
  Nucl.\ Phys.\ B {\bf 22} (1970) 397.
  %%CITATION = NUPHA,B22,397;%%
\bibitem{Zakharov:1970cc}
  V.~I.~Zakharov,
  %``Linearized gravitation theory and the graviton mass,''
  JETP Lett.\  {\bf 12} (1970) 312
   [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 12} (1970) 447].
  %%CITATION = JTPLA,12,312;%%
\bibitem{Iwasaki:1971uz}
  Y.~Iwasaki,
  %``Consistency condition for propagators,''
  Phys.\ Rev.\ D {\bf 2} (1970) 2255.
  %%CITATION = PHRVA,D2,2255;%%
\bibitem{Vainshtein:1972sx}
  A.~I.~Vainshtein,
  %``To the problem of nonvanishing gravitation mass,''
  Phys.\ Lett.\ B {\bf 39} (1972) 393.
  %%CITATION = PHLTA,B39,393;%%
\bibitem{Bergshoeff:2009hq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``Massive Gravity in Three Dimensions,''
  Phys.\ Rev.\ Lett.\  {\bf 102} (2009) 201301
  [arXiv:0901.1766 [hep-th]].
  %%CITATION = ARXIV:0901.1766;%%
\bibitem{Deser:1981wh}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Topologically Massive Gauge Theories,''
  Annals Phys.\  {\bf 140} (1982) 372
   [Erratum-ibid.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 281} (2000) 409].
  %%CITATION = APNYA,140,372;%%
\bibitem{Deser:1982vy}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Three-Dimensional Massive Gauge Theories,''
  Phys.\ Rev.\ Lett.\  {\bf 48} (1982) 975.
  %%CITATION = PRLTA,48,975;%%
\bibitem{Riess:1998cb}
  A.~G.~Riess {\it et al.}  [Supernova Search Team Collaboration],
  %``Observational evidence from supernovae for an accelerating universe and a cosmological constant,''
  Astron.\ J.\  {\bf 116} (1998) 1009
  [astro-ph/9805201].
  %%CITATION = ASTRO-PH/9805201;%%
\bibitem{Perlmutter:1998np}
  S.~Perlmutter {\it et al.}  [Supernova Cosmology Project Collaboration],
  %``Measurements of Omega and Lambda from 42 high redshift supernovae,''
  Astrophys.\ J.\  {\bf 517} (1999) 565
  [astro-ph/9812133].
  %%CITATION = ASTRO-PH/9812133;%%
\bibitem{deRham:2007rw}
  C.~de Rham, S.~Hofmann, J.~Khoury and A.~J.~Tolley,
  %``Cascading Gravity and Degravitation,''
  JCAP {\bf 0802} (2008) 011
  [arXiv:0712.2821 [hep-th]].
  %%CITATION = ARXIV:0712.2821;%%
\bibitem{deRham:2007xp}
  C.~de Rham, G.~Dvali, S.~Hofmann, J.~Khoury, O.~Pujolas, M.~Redi and A.~J.~Tolley,
  %``Cascading gravity: Extending the Dvali-Gabadadze-Porrati model to higher dimension,''
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 251603
  [arXiv:0711.2072 [hep-th]].
  %%CITATION = ARXIV:0711.2072;%%
\bibitem{Rubakov:2008nh}
  V.~A.~Rubakov and P.~G.~Tinyakov,
  %``Infrared-modified gravities and massive gravitons,''
  Phys.\ Usp.\  {\bf 51} (2008) 759
  [arXiv:0802.4379 [hep-th]].
  %%CITATION = ARXIV:0802.4379;%%
\bibitem{Klebanov:1995ni}
  I.~R.~Klebanov and L.~Thorlacius,
  %``The Size of p-branes,''
  Phys.\ Lett.\ B {\bf 371} (1996) 51
  [hep-th/9510200].
  %%CITATION = HEP-TH/9510200;%%
\bibitem{Gabadadze:2003ck}
  G.~Gabadadze and M.~Shifman,
  %``Softly massive gravity,''
  Phys.\ Rev.\ D {\bf 69} (2004) 124032
  [hep-th/0312289].
  %%CITATION = HEP-TH/0312289;%%
\bibitem{Kiritsis:2001bc}
  E.~Kiritsis, N.~Tetradis and T.~N.~Tomaras,
  %``Induced brane gravity: Realizations and limitations,''
  JHEP {\bf 0108} (2001) 012
  [hep-th/0106050].
  %%CITATION = HEP-TH/0106050;%%
\bibitem{Dvali:2001ae}
  G.~Dvali, G.~Gabadadze, X.~-r.~Hou and E.~Sefusatti,
  %``Seesaw modification of gravity,''
  Phys.\ Rev.\ D {\bf 67} (2003) 044019
  [hep-th/0111266].
  %%CITATION = HEP-TH/0111266;%%
\bibitem{Kolanovic:2003am}
  M.~Kolanovic, M.~Porrati and J.~-W.~Rombouts,
  %``Regularization of brane induced gravity,''
  Phys.\ Rev.\ D {\bf 68} (2003) 064018
  [hep-th/0304148].
  %%CITATION = HEP-TH/0304148;%%
\bibitem{'tHooft:2007bf}
  G.~'t Hooft,
  %``Unitarity in the Brout-Englert-Higgs Mechanism for Gravity,''
  arXiv:0708.3184 [hep-th].
  %%CITATION = ARXIV:0708.3184;%%
\bibitem{Kakushadze:2007hf}
  Z.~Kakushadze,
  %``Massive Gravity in Minkowski Space via Gravitational Higgs Mechanism,''
  Phys.\ Rev.\ D {\bf 77} (2008) 024001
  [arXiv:0710.1061 [hep-th]].
  %%CITATION = ARXIV:0710.1061;%%
\bibitem{Corradini:2001qv}
  O.~Corradini, A.~Iglesias, Z.~Kakushadze and P.~Langfelder,
  %``Gravity on a 3-brane in 6-D bulk,''
  Phys.\ Lett.\ B {\bf 521} (2001) 96
  [hep-th/0108055].
  %%CITATION = HEP-TH/0108055;%%
\bibitem{Kaloper:2007ap}
  N.~Kaloper and D.~Kiley,
  %``Charting the landscape of modified gravity,''
  JHEP {\bf 0705} (2007) 045
  [hep-th/0703190].
  %%CITATION = HEP-TH/0703190;%%
\bibitem{Kaloper:2007qh}
  N.~Kaloper,
  %``Brane Induced Gravity: Codimension-2,''
  Mod.\ Phys.\ Lett.\ A {\bf 23} (2008) 781
  [arXiv:0711.3210 [hep-th]].
  %%CITATION = ARXIV:0711.3210;%%
\bibitem{Deffayet:2001uk}
  C.~Deffayet, G.~R.~Dvali, G.~Gabadadze and A.~I.~Vainshtein,
  %``Nonperturbative continuity in graviton mass versus perturbative discontinuity,''
  Phys.\ Rev.\ D {\bf 65} (2002) 044026
  [hep-th/0106001].
  %%CITATION = HEP-TH/0106001;%%
\bibitem{Deffayet:2000uy}
  C.~Deffayet,
  %``Cosmology on a brane in Minkowski bulk,''
  Phys.\ Lett.\ B {\bf 502} (2001) 199
  [hep-th/0010186].
  %%CITATION = HEP-TH/0010186;%%
\bibitem{Peskin:1995ev}
  M.~E.~Peskin and D.~V.~Schroeder,
  %``An Introduction to quantum field theory,''
  Reading, USA: Addison-Wesley (1995) 842 p
%\cite{Srednicki:2007qs}
\bibitem{Srednicki:2007qs}
  M.~Srednicki,
  %``Quantum field theory,''
  Cambridge, UK: Univ. Pr. (2007) 641 p
\bibitem{Kluson:2012wf}
  J.~Kluson,
  %``Non-Linear Massive Gravity with Additional Primary Constraint and Absence of Ghosts,''
  Phys.\ Rev.\ D {\bf 86} (2012) 044024
  [arXiv:1204.2957 [hep-th]].
  %%CITATION = ARXIV:1204.2957;%%
\bibitem{Kluson:2012zz}
  J.~Kluson,
  %``Note About Hamiltonian Formalism for General Non-Linear Massive Gravity Action in Stuckelberg Formalism,''
  arXiv:1209.3612 [hep-th].
  %%CITATION = ARXIV:1209.3612;%%
\bibitem{Corley:2001hg}
  S.~Corley, D.~A.~Lowe and S.~Ramgoolam,
  %``Einstein-Hilbert action on the brane for the bulk graviton,''
  JHEP {\bf 0107} (2001) 030
  [hep-th/0106067].
  %%CITATION = HEP-TH/0106067;%%
\bibitem{Ardalan:2002qt}
  F.~Ardalan, H.~Arfaei, M.~R.~Garousi and A.~Ghodsi,
  %``Gravity on noncommutative D-branes,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 18} (2003) 1051
  [hep-th/0204117].
  %%CITATION = HEP-TH/0204117;%%
\bibitem{Antoniadis:2002tr}
  I.~Antoniadis, R.~Minasian and P.~Vanhove,
  %``Noncompact Calabi-Yau manifolds and localized gravity,''
  Nucl.\ Phys.\ B {\bf 648} (2003) 69
  [hep-th/0209030].
  %%CITATION = HEP-TH/0209030;%%
\bibitem{Kohlprath:2004yw}
  E.~Kohlprath and P.~Vanhove,
  %``Localized gravity in non-compact superstring models,''
  hep-th/0409197.
  %%CITATION = HEP-TH/0409197;%%
\bibitem{Epple:2004ra}
  F.~T.~J.~Epple,
  %``Induced gravity on intersecting branes,''
  JHEP {\bf 0409} (2004) 021
  [hep-th/0408105].
  %%CITATION = HEP-TH/0408105;%%
\bibitem{Lee:1977eg}
  B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
  %``Weak Interactions at Very High-Energies: The Role of the Higgs Boson Mass,''
  Phys.\ Rev.\ D {\bf 16} (1977) 1519.
  %%CITATION = PHRVA,D16,1519;%%
\bibitem{Chanowitz:1985hj}
  M.~S.~Chanowitz and M.~K.~Gaillard,
  %``The TeV Physics of Strongly Interacting W's and Z's,''
  Nucl.\ Phys.\ B {\bf 261} (1985) 379.
  %%CITATION = NUPHA,B261,379;%%
\bibitem{Akrami:2012vf}
  Y.~Akrami, T.~S.~Koivisto and M.~Sandstad,
  %``Accelerated expansion from ghost-free bigravity: a statistical analysis with improved generality,''
  arXiv:1209.0457 [astro-ph.CO].
  %%CITATION = ARXIV:1209.0457;%%
\bibitem{Weinberg:2008zzc}
  S.~Weinberg,
  %``Cosmology,''
  Oxford, UK: Oxford Univ. Pr. (2008) 593 p
\bibitem{Mukhanov:2005sc}
  V.~Mukhanov,
  %``Physical foundations of cosmology,''
  Cambridge, UK: Univ. Pr. (2005) 421 p
\bibitem{Baumann:2009ds}
  D.~Baumann,
  %``TASI Lectures on Inflation,''
  arXiv:0907.5424 [hep-th].
  %%CITATION = ARXIV:0907.5424;%%
\bibitem{Komatsu:2010fb}
  E.~Komatsu {\it et al.}  [WMAP Collaboration],
  %``Seven-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Interpretation,''
  Astrophys.\ J.\ Suppl.\  {\bf 192} (2011) 18
  [arXiv:1001.4538 [astro-ph.CO]].
  %%CITATION = ARXIV:1001.4538;%%
\bibitem{de Urries:1998bi}
  F.~J.~de Urries and J.~Julve,
  %``Ostrogradski formalism for higher derivative scalar field theories,''
  J.\ Phys.\ A {\bf 31} (1998) 6949
  [hep-th/9802115].
  %%CITATION = HEP-TH/9802115;%%
\bibitem{Bengtsson:1994vn} 
  I.~Bengtsson,
  %``Note on massive spin-2 in curved space,''
  J.\ Math.\ Phys.\  {\bf 36}, 5805 (1995)
  [gr-qc/9411057].
  %%CITATION = GR-QC/9411057;%%
\bibitem{Zinoviev:2001dt}
  Y.~.M.~Zinoviev,
  %``On massive high spin particles in AdS,''
  hep-th/0108192.
  %%CITATION = HEP-TH/0108192;%%
\bibitem{deRham:2012kf}
  C.~de Rham and S.~Renaux-Petel,
  %``Massive Gravity on de Sitter and Unique Candidate for Partially Massless Gravity,''
  arXiv:1206.3482 [hep-th].
  %%CITATION = ARXIV:1206.3482;%%
\bibitem{Zinoviev:2011fv}
  Y.~.M.~Zinoviev,
  %``Gravitational cubic interactions for a massive mixed symmetry gauge field,''
  Class.\ Quant.\ Grav.\  {\bf 29} (2012) 015013
  [arXiv:1107.3222 [hep-th]].
  %%CITATION = ARXIV:1107.3222;%%
\bibitem{Joung:2012rv}
  E.~Joung, L.~Lopez and M.~Taronna,
  %``On the cubic interactions of massive and partially-massless higher spins in (A)dS,''
  JHEP {\bf 1207} (2012) 041
  [arXiv:1203.6578 [hep-th]].
  %%CITATION = ARXIV:1203.6578;%%
\bibitem{Zwicky:1933gu}
  F.~Zwicky,
  %``Spectral displacement of extra galactic nebulae,''
  Helv.\ Phys.\ Acta {\bf 6} (1933) 110.
  %%CITATION = HPACA,6,110;%%
\bibitem{Rubin:1970zza}
  V.~C.~Rubin and W.~K.~Ford, Jr.,
  %``Rotation of the Andromeda Nebula from a Spectroscopic Survey of Emission Regions,''
  Astrophys.\ J.\  {\bf 159} (1970) 379.
  %%CITATION = ASJOA,159,379;%%
\bibitem{Rubin:1980zd}
  V.~C.~Rubin, N.~Thonnard and W.~K.~Ford, Jr.,
  %``Rotational properties of 21 SC galaxies with a large range of luminosities and radii, from NGC 4605 /R = 4kpc/ to UGC 2885 /R = 122 kpc/,''
  Astrophys.\ J.\  {\bf 238} (1980) 471.
  %%CITATION = ASJOA,238,471;%%
\bibitem{Rubin:1985ze}
  V.~C.~Rubin, D.~Burstein, W.~K.~Ford, Jr. and N.~Thonnard,
  %``Rotation velocities of 16 SA galaxies and a comparison of Sa, Sb, and SC rotation properties,''
  Astrophys.\ J.\  {\bf 289} (1985) 81.
  %%CITATION = ASJOA,289,81;%%
\bibitem{Clowe:2006eq}
  D.~Clowe, M.~Bradac, A.~H.~Gonzalez, M.~Markevitch, S.~W.~Randall, C.~Jones and D.~Zaritsky,
  %``A direct empirical proof of the existence of dark matter,''
  Astrophys.\ J.\  {\bf 648} (2006) L109
  [astro-ph/0608407].
  %%CITATION = ASTRO-PH/0608407;%%
\bibitem{Amanullah:2010vv}
  R.~Amanullah, C.~Lidman, D.~Rubin, G.~Aldering, P.~Astier, K.~Barbary, M.~S.~Burns and A.~Conley {\it et al.},
  %``Spectra and Light Curves of Six Type Ia Supernovae at 0.511 < z < 1.12 and the Union2 Compilation,''
  Astrophys.\ J.\  {\bf 716} (2010) 712
  [arXiv:1004.1711 [astro-ph.CO]].
  %%CITATION = ARXIV:1004.1711;%%
\bibitem{Iocco:2008va}
  F.~Iocco, G.~Mangano, G.~Miele, O.~Pisanti and P.~D.~Serpico,
  %``Primordial Nucleosynthesis: from precision cosmology to fundamental physics,''
  Phys.\ Rept.\  {\bf 472} (2009) 1
  [arXiv:0809.0631 [astro-ph]].
  %%CITATION = ARXIV:0809.0631;%%
\bibitem{Massey:2007wb}
  R.~Massey, J.~Rhodes, R.~Ellis, N.~Scoville, A.~Leauthaud, A.~Finoguenov, P.~Capak and D.~Bacon {\it et al.},
  %``Dark matter maps reveal cosmic scaffolding,''
  Nature {\bf 445} (2007) 286
  [astro-ph/0701594].
  %%CITATION = ASTRO-PH/0701594;%%
\bibitem{Allen:2002eu}
  S.~W.~Allen, A.~C.~Fabian, R.~W.~Schmidt and H.~Ebeling,
  %``Cosmological constraints from the local x-ray luminosity function of the most x-ray luminous galaxy clusters,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 342} (2003) 287
  [astro-ph/0208394].
  %%CITATION = ASTRO-PH/0208394;%%
\end{thebibliography}

==> Bibliography/references-original.tex <==
\begin{thebibliography}{999}
\bibitem{Martin:2012bt}
  J.~Martin,
  %``Everything You Always Wanted To Know About The Cosmological Constant Problem (But Were Afraid To Ask),''
  Comptes Rendus Physique {\bf 13} (2012) 566
  [arXiv:1205.3365 [astro-ph.CO]].
  %%CITATION = ARXIV:1205.3365;%%
\bibitem{Wald:1984rg}
  R.~M.~Wald,
  %``General Relativity,''
  Chicago, Usa: Univ. Pr. ( 1984) 491p.
\bibitem{Weinberg:1988cp}
  S.~Weinberg,
  %``The Cosmological Constant Problem,''
  Rev.\ Mod.\ Phys.\  {\bf 61} (1989) 1.
  %%CITATION = RMPHA,61,1;%%
\bibitem{Jaffe:2005vp}
  R.~L.~Jaffe,
  %``The Casimir effect and the quantum vacuum,''
  Phys.\ Rev.\ D {\bf 72} (2005) 021301
  [hep-th/0503158].
  %%CITATION = HEP-TH/0503158;%%
\bibitem{Dvali:2002pe}
  G.~Dvali, G.~Gabadadze and M.~Shifman,
  %``Diluting cosmological constant in infinite volume extra dimensions,''
  Phys.\ Rev.\ D {\bf 67} (2003) 044020
  [hep-th/0202174].
  %%CITATION = HEP-TH/0202174;%%
\bibitem{Dvali:2002fz}
  G.~Dvali, G.~Gabadadze and M.~Shifman,
  %``Diluting cosmological constant via large distance modification of gravity,''
  hep-th/0208096.
  %%CITATION = HEP-TH/0208096;%%
\bibitem{Hinterbichler:2011tt}
  K.~Hinterbichler,
  %``Theoretical Aspects of Massive Gravity,''
  Rev.\ Mod.\ Phys.\  {\bf 84} (2012) 671
  [arXiv:1105.3735 [hep-th]].
  %%CITATION = ARXIV:1105.3735;%%
\bibitem{ArkaniHamed:2002sp}
  N.~Arkani-Hamed, H.~Georgi and M.~D.~Schwartz,
  %``Effective field theory for massive gravitons and gravity in
  %theory space,'' 
  Annals Phys.\  {\bf 305} (2003) 96
  [hep-th/0210184].
  %%CITATION = HEP-TH/0210184;%%
\bibitem{de Urries:1998bi}
  F.~J.~de Urries and J.~Julve,
  %``Ostrogradski formalism for higher derivative scalar field theories,''
  J.\ Phys.\ A {\bf 31} (1998) 6949
  [hep-th/9802115].
  %%CITATION = HEP-TH/9802115;%%
\bibitem{Fierz:1939ix}
  M.~Fierz and W.~Pauli,
  %``On relativistic wave equations for particles of arbitrary spin in 
  %an electromagnetic field,'' 
  Proc.\ Roy.\ Soc.\ Lond.\ A {\bf 173} (1939) 211.
  %%CITATION = PRSLA,A173,211;%%
\bibitem{Pauli:1939xp}
  W.~Pauli and M.~Fierz,
  %``On Relativistic Field Equations Of Particles With Arbitrary Spin
  %In An Electromagnetic Field,'' 
  Helv.\ Phys.\ Acta {\bf 12} (1939) 297.
  %%CITATION = HPACA,12,297;%%
\bibitem{vanDam:1970vg}
  H.~van Dam and M.~J.~G.~Veltman,
  %``Massive and massless Yang-Mills and gravitational fields,''
  Nucl.\ Phys.\ B {\bf 22} (1970) 397.
  %%CITATION = NUPHA,B22,397;%%
\bibitem{Zakharov:1970cc}
  V.~I.~Zakharov,
  %``Linearized gravitation theory and the graviton mass,''
  JETP Lett.\  {\bf 12} (1970) 312
   [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 12} (1970) 447].
  %%CITATION = JTPLA,12,312;%%
\bibitem{Iwasaki:1971uz}
  Y.~Iwasaki,
  %``Consistency condition for propagators,''
  Phys.\ Rev.\ D {\bf 2} (1970) 2255.
  %%CITATION = PHRVA,D2,2255;%%
\bibitem{Vainshtein:1972sx}
  A.~I.~Vainshtein,
  %``To the problem of nonvanishing gravitation mass,''
  Phys.\ Lett.\ B {\bf 39} (1972) 393.
  %%CITATION = PHLTA,B39,393;%%
\bibitem{Deser:1981wh}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Topologically Massive Gauge Theories,''
  Annals Phys.\  {\bf 140} (1982) 372
   [Erratum-ibid.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 281} (2000) 409].
  %%CITATION = APNYA,140,372;%%
\bibitem{Deser:1982vy}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Three-Dimensional Massive Gauge Theories,''
  Phys.\ Rev.\ Lett.\  {\bf 48} (1982) 975.
  %%CITATION = PRLTA,48,975;%%
\bibitem{Bergshoeff:2009hq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``Massive Gravity in Three Dimensions,''
  Phys.\ Rev.\ Lett.\  {\bf 102} (2009) 201301
  [arXiv:0901.1766 [hep-th]].
  %%CITATION = ARXIV:0901.1766;%%
\bibitem{Rosen:1940zz}
  N.~Rosen,
  %``General Relativity and Flat Space. II,''
  Phys.\ Rev.\  {\bf 57} (1940) 150.
  %%CITATION = PHRVA,57,150;%%
\bibitem{Rosen:1975kk}
  N.~Rosen,
  %``Bimetric Theory of Gravitation,''
  In *Erice 1975, Proceedings, Topics In Theoretical and Experimental
  Gravitation Physics*, New York 1977, 273-294 
 \bibitem{Aragone:1971kh}
  C.~Aragone and S.~Deser,
  %``Constraints on gravitationally coupled tensor fields,''
  Nuovo Cim.\ A {\bf 3} (1971) 709.
  %%CITATION = NUCIA,A3,709;%%
\bibitem{ISS}
  C.~J.~Isham, A.~Salam and J.~A.~Strathdee,
  %``F-dominance of gravity,''
  Phys.\ Rev.\ D {\bf 3} (1971) 867.
  %%CITATION = PHRVA,D3,867;%%
\bibitem{Boulware:1973my}
  D.~G.~Boulware and S.~Deser,
  %``Can gravitation have a finite range?,''
  Phys.\ Rev.\ D {\bf 6} (1972) 3368.
  %%CITATION = PHRVA,D6,3368;%%
\bibitem{Chamseddine:1978yu}
  A.~H.~Chamseddine, A.~Salam and J.~A.~Strathdee,
  %``Strong Gravity and Supersymmetry,''
  Nucl.\ Phys.\ B {\bf 136} (1978) 248.
  %%CITATION = NUPHA,B136,248;%%
\bibitem{Riess:1998cb}
  A.~G.~Riess {\it et al.}  [Supernova Search Team Collaboration],
  %``Observational evidence from supernovae for an accelerating universe and a cosmological constant,''
  Astron.\ J.\  {\bf 116} (1998) 1009
  [astro-ph/9805201].
  %%CITATION = ASTRO-PH/9805201;%%
\bibitem{Perlmutter:1998np}
  S.~Perlmutter {\it et al.}  [Supernova Cosmology Project Collaboration],
  %``Measurements of Omega and Lambda from 42 high redshift supernovae,''
  Astrophys.\ J.\  {\bf 517} (1999) 565
  [astro-ph/9812133].
  %%CITATION = ASTRO-PH/9812133;%%
\bibitem{Hubble:1926yw}
  E.~P.~Hubble,
  %``Extragalactic nebulae,''
  Astrophys.\ J.\  {\bf 64} (1926) 321.
  %%CITATION = ASJOA,64,321;%%
 \bibitem{Hubble:1929ig}
  E.~Hubble,
  %``A relation between distance and radial velocity among extra-galactic nebulae,''
  Proc.\ Nat.\ Acad.\ Sci.\  {\bf 15} (1929) 168.
  %%CITATION = PNASA,15,168;%%
\bibitem{ArkaniHamed:1998rs}
  N.~Arkani-Hamed, S.~Dimopoulos and G.~R.~Dvali,
  %``The Hierarchy problem and new dimensions at a millimeter,''
  Phys.\ Lett.\ B {\bf 429} (1998) 263
  [hep-ph/9803315].
  %%CITATION = HEP-PH/9803315;%%
\bibitem{Antoniadis:1998ig}
  I.~Antoniadis, N.~Arkani-Hamed, S.~Dimopoulos and G.~R.~Dvali,
  %``New dimensions at a millimeter to a Fermi and superstrings at a TeV,''
  Phys.\ Lett.\ B {\bf 436} (1998) 257
  [hep-ph/9804398].
  %%CITATION = HEP-PH/9804398;%%
\bibitem{Randall:1998uk}
  L.~Randall and R.~Sundrum,
  %``Out of this world supersymmetry breaking,''
  Nucl.\ Phys.\ B {\bf 557} (1999) 79
  [hep-th/9810155].
  %%CITATION = HEP-TH/9810155;%%
\bibitem{Dvali:2000hr}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``4-D gravity on a brane in 5-D Minkowski space,''
  Phys.\ Lett.\ B {\bf 485} (2000) 208
  [hep-th/0005016].
  %%CITATION = HEP-TH/0005016;%%
\bibitem{Dvali:2001gm}
  G.~R.~Dvali, G.~Gabadadze, M.~Kolanovic and F.~Nitti,
  %``The Power of brane induced gravity,''
  Phys.\ Rev.\ D {\bf 64} (2001) 084004
  [hep-ph/0102216].
  %%CITATION = HEP-PH/0102216;%%
\bibitem{Rubakov:2008nh}
  V.~A.~Rubakov and P.~G.~Tinyakov,
  %``Infrared-modified gravities and massive gravitons,''
  Phys.\ Usp.\  {\bf 51} (2008) 759
  [arXiv:0802.4379 [hep-th]].
  %%CITATION = ARXIV:0802.4379;%%
\bibitem{deRham:2007rw}
  C.~de Rham, S.~Hofmann, J.~Khoury and A.~J.~Tolley,
  %``Cascading Gravity and Degravitation,''
  JCAP {\bf 0802} (2008) 011
  [arXiv:0712.2821 [hep-th]].
  %%CITATION = ARXIV:0712.2821;%%
\bibitem{deRham:2007xp}
  C.~de Rham, G.~Dvali, S.~Hofmann, J.~Khoury, O.~Pujolas, M.~Redi and A.~J.~Tolley,
  %``Cascading gravity: Extending the Dvali-Gabadadze-Porrati model to higher dimension,''
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 251603
  [arXiv:0711.2072 [hep-th]].
  %%CITATION = ARXIV:0711.2072;%%
\bibitem{Dvali:2000rv}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``Metastable gravitons and infinite volume extra dimensions,''
  Phys.\ Lett.\ B {\bf 484} (2000) 112
  [hep-th/0002190].
  %%CITATION = HEP-TH/0002190;%%
\bibitem{Gregory:2000jc}
  R.~Gregory, V.~A.~Rubakov and S.~M.~Sibiryakov,
  %``Opening up extra dimensions at ultra large scales,''
  Phys.\ Rev.\ Lett.\  {\bf 84} (2000) 5928
  [hep-th/0002072].
  %%CITATION = HEP-TH/0002072;%%
\bibitem{Dvali:2001ae}
  G.~Dvali, G.~Gabadadze, X.~-r.~Hou and E.~Sefusatti,
  %``Seesaw modification of gravity,''
  Phys.\ Rev.\ D {\bf 67} (2003) 044019
  [hep-th/0111266].
  %%CITATION = HEP-TH/0111266;%%
\bibitem{Kiritsis:2001bc}
  E.~Kiritsis, N.~Tetradis and T.~N.~Tomaras,
  %``Induced brane gravity: Realizations and limitations,''
  JHEP {\bf 0108} (2001) 012
  [hep-th/0106050].
  %%CITATION = HEP-TH/0106050;%%
\bibitem{Corley:2001hg}
  S.~Corley, D.~A.~Lowe and S.~Ramgoolam,
  %``Einstein-Hilbert action on the brane for the bulk graviton,''
  JHEP {\bf 0107} (2001) 030
  [hep-th/0106067].
  %%CITATION = HEP-TH/0106067;%%
\bibitem{Ardalan:2002qt}
  F.~Ardalan, H.~Arfaei, M.~R.~Garousi and A.~Ghodsi,
  %``Gravity on noncommutative D-branes,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 18} (2003) 1051
  [hep-th/0204117].
  %%CITATION = HEP-TH/0204117;%%
\bibitem{Antoniadis:2002tr}
  I.~Antoniadis, R.~Minasian and P.~Vanhove,
  %``Noncompact Calabi-Yau manifolds and localized gravity,''
  Nucl.\ Phys.\ B {\bf 648} (2003) 69
  [hep-th/0209030].
  %%CITATION = HEP-TH/0209030;%%
\bibitem{Kohlprath:2004yw}
  E.~Kohlprath and P.~Vanhove,
  %``Localized gravity in non-compact superstring models,''
  hep-th/0409197.
  %%CITATION = HEP-TH/0409197;%%
\bibitem{Epple:2004ra}
  F.~T.~J.~Epple,
  %``Induced gravity on intersecting branes,''
  JHEP {\bf 0409} (2004) 021
  [hep-th/0408105].
  %%CITATION = HEP-TH/0408105;%%
\bibitem{Deffayet:2007zz}
  C.~Deffayet,
  %``The vDVZ discontinuity, DGP gravity, and cosmology,''
  Int.\ J.\ Theor.\ Phys.\  {\bf 46} (2007) 2242.
  %%CITATION = IJTPB,46,2242;%%
\bibitem{Fang:2008kc}
  W.~Fang, S.~Wang, W.~Hu, Z.~Haiman, L.~Hui and M.~May,
  %``Challenges to the DGP Model from Horizon-Scale Growth and Geometry,''
  Phys.\ Rev.\ D {\bf 78} (2008) 103509
  [arXiv:0808.2208 [astro-ph]].
  %%CITATION = ARXIV:0808.2208;%%
\bibitem{Lombriser:2009xg}
  L.~Lombriser, W.~Hu, W.~Fang and U.~Seljak,
  %``Cosmological Constraints on DGP Braneworld Gravity with Brane Tension,''
  Phys.\ Rev.\ D {\bf 80} (2009) 063536
  [arXiv:0905.1112 [astro-ph.CO]].
  %%CITATION = ARXIV:0905.1112;%%
\bibitem{Dubovsky:2002jm}
  S.~L.~Dubovsky and V.~A.~Rubakov,
  %``Brane induced gravity in more than one extra dimensions: Violation of equivalence principle and ghost,''
  Phys.\ Rev.\ D {\bf 67} (2003) 104014
  [hep-th/0212222].
  %%CITATION = HEP-TH/0212222;%%
\bibitem{Kolanovic:2003am}
  M.~Kolanovic, M.~Porrati and J.~-W.~Rombouts,
  %``Regularization of brane induced gravity,''
  Phys.\ Rev.\ D {\bf 68} (2003) 064018
  [hep-th/0304148].
  %%CITATION = HEP-TH/0304148;%%
\bibitem{Gabadadze:2003ck}
  G.~Gabadadze and M.~Shifman,
  %``Softly massive gravity,''
  Phys.\ Rev.\ D {\bf 69} (2004) 124032
  [hep-th/0312289].
  %%CITATION = HEP-TH/0312289;%%
\bibitem{Klebanov:1995ni}
  I.~R.~Klebanov and L.~Thorlacius,
  %``The Size of p-branes,''
  Phys.\ Lett.\ B {\bf 371} (1996) 51
  [hep-th/9510200].
  %%CITATION = HEP-TH/9510200;%%
\bibitem{'tHooft:2007bf}
  G.~'t Hooft,
  %``Unitarity in the Brout-Englert-Higgs Mechanism for Gravity,''
  arXiv:0708.3184 [hep-th].
  %%CITATION = ARXIV:0708.3184;%%
\bibitem{Kakushadze:2007hf}
  Z.~Kakushadze,
  %``Massive Gravity in Minkowski Space via Gravitational Higgs Mechanism,''
  Phys.\ Rev.\ D {\bf 77} (2008) 024001
  [arXiv:0710.1061 [hep-th]].
  %%CITATION = ARXIV:0710.1061;%%
\bibitem{Corradini:2001qv}
  O.~Corradini, A.~Iglesias, Z.~Kakushadze and P.~Langfelder,
  %``Gravity on a 3-brane in 6-D bulk,''
  Phys.\ Lett.\ B {\bf 521} (2001) 96
  [hep-th/0108055].
  %%CITATION = HEP-TH/0108055;%%
\bibitem{Kaloper:2007ap}
  N.~Kaloper and D.~Kiley,
  %``Charting the landscape of modified gravity,''
  JHEP {\bf 0705} (2007) 045
  [hep-th/0703190].
  %%CITATION = HEP-TH/0703190;%%
\bibitem{Kaloper:2007qh}
  N.~Kaloper,
  %``Brane Induced Gravity: Codimension-2,''
  Mod.\ Phys.\ Lett.\ A {\bf 23} (2008) 781
  [arXiv:0711.3210 [hep-th]].
  %%CITATION = ARXIV:0711.3210;%%
\bibitem{Deffayet:2001uk}
  C.~Deffayet, G.~R.~Dvali, G.~Gabadadze and A.~I.~Vainshtein,
  %``Nonperturbative continuity in graviton mass versus perturbative discontinuity,''
  Phys.\ Rev.\ D {\bf 65} (2002) 044026
  [hep-th/0106001].
  %%CITATION = HEP-TH/0106001;%%
\bibitem{Deffayet:2000uy}
  C.~Deffayet,
  %``Cosmology on a brane in Minkowski bulk,''
  Phys.\ Lett.\ B {\bf 502} (2001) 199
  [hep-th/0010186].
  %%CITATION = HEP-TH/0010186;%%
\bibitem{Peskin:1995ev}
  M.~E.~Peskin and D.~V.~Schroeder,
  %``An Introduction to quantum field theory,''
  Reading, USA: Addison-Wesley (1995) 842 p
%\cite{Srednicki:2007qs}
\bibitem{Srednicki:2007qs}
  M.~Srednicki,
  %``Quantum field theory,''
  Cambridge, UK: Univ. Pr. (2007) 641 p
\bibitem{Lee:1977eg}
  B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
  %``Weak Interactions at Very High-Energies: The Role of the Higgs Boson Mass,''
  Phys.\ Rev.\ D {\bf 16} (1977) 1519.
  %%CITATION = PHRVA,D16,1519;%%
\bibitem{Chanowitz:1985hj}
  M.~S.~Chanowitz and M.~K.~Gaillard,
  %``The TeV Physics of Strongly Interacting W's and Z's,''
  Nucl.\ Phys.\ B {\bf 261} (1985) 379.
  %%CITATION = NUPHA,B261,379;%%
\bibitem{ArkaniHamed:2003uy}
  N.~Arkani-Hamed, H.~-C.~Cheng, M.~A.~Luty and S.~Mukohyama,
  %``Ghost condensation and a consistent infrared modification of gravity,''
  JHEP {\bf 0405} (2004) 074
  [hep-th/0312099].
  %%CITATION = HEP-TH/0312099;%%
\bibitem{Rubakov:2004eb}
  V.~A.~Rubakov,
  %``Lorentz-violating graviton masses: Getting around ghosts, low strong coupling scale and VDVZ discontinuity,''
  hep-th/0407104.
  %%CITATION = HEP-TH/0407104;%%
\bibitem{Dubovsky:2004sg}
  S.~L.~Dubovsky,
  %``Phases of massive gravity,''
  JHEP {\bf 0410} (2004) 076
  [hep-th/0409124].
  %%CITATION = HEP-TH/0409124;%%
\bibitem{Creminelli:2005qk}
  P.~Creminelli, A.~Nicolis, M.~Papucci and E.~Trincherini,
  %``Ghosts in massive gravity,''
  JHEP {\bf 0509} (2005) 003
  [hep-th/0505147].
  %%CITATION = HEP-TH/0505147;%%
\bibitem{Nibbelink:2006sz}
  S.~Nibbelink Groot, M.~Peloso and M.~Sexton,
  %``Nonlinear Properties of Vielbein Massive Gravity,''
  Eur.\ Phys.\ J.\ C {\bf 51} (2007) 741
  [hep-th/0610169].
  %%CITATION = HEP-TH/0610169;%%
\bibitem{Gabadadze:2009ja}
  G.~Gabadadze,
  %``General Relativity With An Auxiliary Dimension,''
  Phys.\ Lett.\ B {\bf 681} (2009) 89
  [arXiv:0908.1112 [hep-th]].
  %%CITATION = ARXIV:0908.1112;%%
\bibitem{deRham:2009rm}
  C.~de Rham,
  %``Massive gravity from Dirichlet boundary conditions,''
  Phys.\ Lett.\ B {\bf 688} (2010) 137
  [arXiv:0910.5474 [hep-th]].
  %%CITATION = ARXIV:0910.5474;%%
\bibitem{deRham:2010gu}
  C.~de Rham and G.~Gabadadze,
  %``Selftuned Massive Spin-2,''
  Phys.\ Lett.\ B {\bf 693} (2010) 334
  [arXiv:1006.4367 [hep-th]].
  %%CITATION = ARXIV:1006.4367;%%
\bibitem{Hassan:2011zr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Exact Solution to the 'Auxiliary Extra Dimension' Model of Massive Gravity,''
  Phys.\ Lett.\ B {\bf 702} (2011) 90
  [arXiv:1104.1373 [hep-th]].
  %%CITATION = ARXIV:1104.1373;%%
\bibitem{deRham:2010ik}
  C.~de Rham and G.~Gabadadze,
  %``Generalization of the Fierz-Pauli Action,''
  Phys.\ Rev.\ D {\bf 82} (2010) 044020
  [arXiv:1007.0443 [hep-th]].
  %%CITATION = ARXIV:1007.0443;%%
\bibitem{deRham:2010kj}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Resummation of Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 106} (2011) 231101
  [arXiv:1011.1232 [hep-th]].
  %%CITATION = ARXIV:1011.1232;%%
\bibitem{Mirbabayi:2011aa}
  M.~Mirbabayi,
  %``A Proof Of Ghost Freedom In de Rham-Gabadadze-Tolley Massive Gravity,''
  arXiv:1112.1435 [hep-th].
  %%CITATION = ARXIV:1112.1435;%%
\bibitem{deRham:2011rn}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Ghost free Massive Gravity in the St\'uckelberg language,''
  Phys.\ Lett.\ B {\bf 711} (2012) 190
  [arXiv:1107.3820 [hep-th]].
  %%CITATION = ARXIV:1107.3820;%%
\bibitem{Alberte:2010qb}
  L.~Alberte, A.~H.~Chamseddine and V.~Mukhanov,
  %``Massive Gravity: Exorcising the Ghost,''
  JHEP {\bf 1104} (2011) 004
  [arXiv:1011.0183 [hep-th]].
  %%CITATION = ARXIV:1011.0183;%%
\bibitem{Higuchi:1986py}
  A.~Higuchi,
  %``Forbidden Mass Range For Spin-2 Field Theory In De Sitter Space-time,''
  Nucl.\ Phys.\ B {\bf 282} (1987) 397.
  %%CITATION = NUPHA,B282,397;%%
\bibitem{Higuchi:1989gz}
  A.~Higuchi,
  %``Massive Symmetric Tensor Field In Space-times With A Positive Cosmological Constant,''
  Nucl.\ Phys.\ B {\bf 325} (1989) 745.
  %%CITATION = NUPHA,B325,745;%%
\bibitem{Porrati:2000cp}
  M.~Porrati,
  %``No van Dam-Veltman-Zakharov discontinuity in AdS space,''
  Phys.\ Lett.\ B {\bf 498} (2001) 92
  [hep-th/0011152].
  %%CITATION = HEP-TH/0011152;%%
\bibitem{Kogan:2000uy}
  I.~I.~Kogan, S.~Mouslopoulos and A.~Papazoglou,
  %``The m ---> 0 limit for massive graviton in dS(4) and AdS(4): How to circumvent the van Dam-Veltman-Zakharov discontinuity,''
  Phys.\ Lett.\ B {\bf 503} (2001) 173
  [hep-th/0011138].
  %%CITATION = HEP-TH/0011138;%%
\bibitem{Deser:2001pe}
  S.~Deser and A.~Waldron,
  %``Gauge invariances and phases of massive higher spins in (A)dS,''
  Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 031601
  [hep-th/0102166].
  %%CITATION = HEP-TH/0102166;%%
\bibitem{Deser:2001us}
  S.~Deser and A.~Waldron,
  %``Partial masslessness of higher spins in (A)dS,''
  Nucl.\ Phys.\ B {\bf 607} (2001) 577
  [hep-th/0103198].
  %%CITATION = HEP-TH/0103198;%%
\bibitem{Deser:2001wx}
  S.~Deser and A.~Waldron,
  %``Stability of massive cosmological gravitons,''
  Phys.\ Lett.\ B {\bf 508} (2001) 347
  [hep-th/0103255].
  %%CITATION = HEP-TH/0103255;%%
\bibitem{Grisa:2009yy}
  L.~Grisa and L.~Sorbo,
  %``Pauli-Fierz Gravitons on Friedmann-Robertson-Walker Background,''
  Phys.\ Lett.\ B {\bf 686} (2010) 273
  [arXiv:0905.3391 [hep-th]].
  %%CITATION = ARXIV:0905.3391;%%
\bibitem{Berkhahn:2010hc}
  F.~Berkhahn, D.~D.~Dietrich and S.~Hofmann,
  %``Self-Protection of Massive Cosmological Gravitons,''
  JCAP {\bf 1011} (2010) 018
  [arXiv:1008.0644 [hep-th]].
  %%CITATION = ARXIV:1008.0644;%%
\bibitem{Berkhahn:2011hb}
  F.~Berkhahn, D.~D.~Dietrich and S.~Hofmann,
  %``Consistency of Relevant Cosmological Deformations on all Scales,''
  JCAP {\bf 1109} (2011) 024
  [arXiv:1104.2534 [hep-th]].
  %%CITATION = ARXIV:1104.2534;%%
\bibitem{Damour:2002ws}
  T.~Damour and I.~I.~Kogan,
  %``Effective Lagrangians and universality classes of nonlinear
  %bigravity,'' 
  Phys.\ Rev.\ D {\bf 66} (2002) 104024
  [hep-th/0206042].
  %%CITATION = HEP-TH/0206042;%%
\bibitem{Damour:2002wu}
  T.~Damour, I.~I.~Kogan and A.~Papazoglou,
  %``Nonlinear bigravity and cosmic acceleration,''
  Phys.\ Rev.\ D {\bf 66} (2002) 104025
  [hep-th/0206044].
  %%CITATION = HEP-TH/0206044;%%
\bibitem{Hassan:2011vm}
  S.~F.~Hassan and R.~A.~Rosen,
  %``On nonlinear Actions for Massive Gravity,''
  JHEP {\bf 1107} (2011) 009
  [arXiv:1103.6055 [hep-th]].
  %%CITATION = ARXIV:1103.6055;%%
\bibitem{Hassan:2011hr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Resolving the Ghost Problem in nonlinear Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 108} (2012) 041101
  [arXiv:1106.3344 [hep-th]].
  %%CITATION = ARXIV:1106.3344;%%
\bibitem{Hassan:2011tf}
  S.~F.~Hassan, R.~A.~Rosen and A.~Schmidt-May,
  %``Ghost-free Massive Gravity with a General Reference Metric,''
  JHEP {\bf 1202} (2012) 026
  [arXiv:1109.3230 [hep-th]].
  %%CITATION = ARXIV:1109.3230;%%
\bibitem{Hassan:2011zd}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Bimetric Gravity from Ghost-free Massive Gravity,''
  JHEP {\bf 1202} (2012) 126
  [arXiv:1109.3515 [hep-th]].
  %%CITATION = ARXIV:1109.3515;%%
\bibitem{Hassan:2011ea}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Confirmation of the Secondary Constraint and Absence of Ghost in Massive Gravity and Bimetric Gravity,''
  JHEP {\bf 1204} (2012) 123
  [arXiv:1111.2070 [hep-th]].
  %%CITATION = ARXIV:1111.2070;%%
\bibitem{Arnowitt:1962hi}
  R.~L.~Arnowitt, S.~Deser and C.~W.~Misner,
  %``The Dynamics of general relativity,''
  [gr-qc/0405109].
  %%CITATION = GR-QC/0405109;%%
\bibitem{Kluson:2012wf}
  J.~Kluson,
  %``Non-Linear Massive Gravity with Additional Primary Constraint and
  %Absence of Ghosts,'' 
  arXiv:1204.2957 [hep-th].
  %%CITATION = ARXIV:1204.2957;%%
\bibitem{Kluson:2012zz}
  J.~Kluson,
  %``Note About Hamiltonian Formalism for General Non-Linear Massive Gravity Action in Stuckelberg Formalism,''
  arXiv:1209.3612 [hep-th].
  %%CITATION = ARXIV:1209.3612;%%
\bibitem{Paulos:2012xe}
  M.~F.~Paulos and A.~J.~Tolley,
  %``Massive Gravity Theories and limits of Ghost-free Bigravity models,''
  arXiv:1203.4268 [hep-th].
  %%CITATION = ARXIV:1203.4268;%%
\bibitem{mvsLovelock} %{\bfseries MISSING REFERENCE!!!}
S.~F.~Hassan, A.~Schmidt-May and M.~von~Strauss,
{\it In preparation}
\bibitem{Volkov:2011an}
  M.~S.~Volkov,
  %``Cosmological solutions with massive gravitons in the bigravity
  %theory,'' 
  JHEP {\bf 1201} (2012) 035
  [arXiv:1110.6153 [hep-th]].
  %%CITATION = ARXIV:1110.6153;%%
\bibitem{Comelli:2011zm}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``FRW Cosmology in ghost-free Massive Gravity,''
  JHEP {\bf 1203} (2012) 067
   [Erratum-ibid.\  {\bf 1206} (2012) 020]
  [arXiv:1111.1983 [hep-th]].
  %%CITATION = ARXIV:1111.1983;%%
\bibitem{Baccetti:2012bk}
  V.~Baccetti, P.~Martin-Moruno and M.~Visser,
  %``Massive gravity from bimetric gravity,''
  arXiv:1205.2158 [gr-qc].
  %%CITATION = ARXIV:1205.2158;%%
\bibitem{Hinterbichler:2012cn}
  K.~Hinterbichler and R.~A.~Rosen,
  %``Interacting Spin-2 Fields,''
  JHEP {\bf 1207} (2012) 047
  [arXiv:1203.5783 [hep-th]].
  %%CITATION = ARXIV:1203.5783;%%
\bibitem{Chamseddine:2011mu}
  A.~H.~Chamseddine and V.~Mukhanov,
  %``Massive Gravity Simplified: A Quadratic Action,''
  JHEP {\bf 1108} (2011) 091
  [arXiv:1106.5868 [hep-th]].
  %%CITATION = ARXIV:1106.5868;%%
\bibitem{Chamseddine:2011bu}
  A.~H.~Chamseddine and M.~S.~Volkov,
  %``Cosmological solutions with massive gravitons,''
  Phys.\ Lett.\ B {\bf 704} (2011) 652
  [arXiv:1107.5504 [hep-th]].
  %%CITATION = ARXIV:1107.5504;%%
\bibitem{Gumrukcuoglu:2011ew}
  A.~E.~Gumrukcuoglu, C.~Lin and S.~Mukohyama,
  %``Open FRW universes and self-acceleration from nonlinear massive gravity,''
  JCAP {\bf 1111} (2011) 030
  [arXiv:1109.3845 [hep-th]].
  %%CITATION = ARXIV:1109.3845;%%
\bibitem{Volkov:2012cf} 
  M.~S.~Volkov,
  %``Exact self-accelerating cosmologies in the ghost-free bigravity and massive gravity,''
  Phys.\ Rev.\ D {\bf 86}, 061502 (2012)
  [arXiv:1205.5713 [hep-th]].
  %%CITATION = ARXIV:1205.5713;%%
\bibitem{Koyama:2011wx}
  K.~Koyama, G.~Niz and G.~Tasinato,
  %``The Self-Accelerating Universe with Vectors in Massive Gravity,''
  JHEP {\bf 1112} (2011) 065
  [arXiv:1110.2618 [hep-th]].
  %%CITATION = ARXIV:1110.2618;%%
\bibitem{DeFelice:2012mx}
  A.~De Felice, A.~E.~Gumrukcuoglu, S.~Mukohyama, A.~E.~Gumrukcuoglu and S.~Mukohyama,
  %``Massive gravity: nonlinear instability of the homogeneous and isotropic universe,''
  Phys.\ Rev.\ Lett.\  {\bf 109} (2012) 171101
  [arXiv:1206.2080 [hep-th]].
  %%CITATION = ARXIV:1206.2080;%%
\bibitem{Tasinato:2012ze}
  G.~Tasinato, K.~Koyama and G.~Niz,
  %``Vector instabilities and self-acceleration in the decoupling limit of massive gravity,''
  arXiv:1210.3627 [hep-th].
  %%CITATION = ARXIV:1210.3627;%%
\bibitem{Comelli:2012db}
  D.~Comelli, M.~Crisostomi and L.~Pilo,
  %``Perturbations in Massive Gravity Cosmology,''
  JHEP {\bf 1206} (2012) 085
  [arXiv:1202.1986 [hep-th]].
  %%CITATION = ARXIV:1202.1986;%%
\bibitem{Berg:2012kn}
  M.~Berg, I.~Buchberger, J.~Enander, E.~Mortsell and S.~Sjors,
  %``Growth Histories in Bimetric Massive Gravity,''
  arXiv:1206.3496 [gr-qc].
  %%CITATION = ARXIV:1206.3496;%%
\bibitem{Mukhanov:2005sc}
  V.~Mukhanov,
  %``Physical foundations of cosmology,''
  Cambridge, UK: Univ. Pr. (2005) 421 p
\bibitem{Weinberg:2008zzc}
  S.~Weinberg,
  %``Cosmology,''
  Oxford, UK: Oxford Univ. Pr. (2008) 593 p
\bibitem{Komatsu:2010fb}
  E.~Komatsu {\it et al.}  [WMAP Collaboration],
  %``Seven-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Interpretation,''
  Astrophys.\ J.\ Suppl.\  {\bf 192} (2011) 18
  [arXiv:1001.4538 [astro-ph.CO]].
  %%CITATION = ARXIV:1001.4538;%%
\bibitem{de Urries:1998bi}
  F.~J.~de Urries and J.~Julve,
  %``Ostrogradski formalism for higher derivative scalar field theories,''
  J.\ Phys.\ A {\bf 31} (1998) 6949
  [hep-th/9802115].
  %%CITATION = HEP-TH/9802115;%%
\bibitem{Zwicky:1933gu}
  F.~Zwicky,
  %``Spectral displacement of extra galactic nebulae,''
  Helv.\ Phys.\ Acta {\bf 6} (1933) 110.
  %%CITATION = HPACA,6,110;%%
\bibitem{Rubin:1970zza}
  V.~C.~Rubin and W.~K.~Ford, Jr.,
  %``Rotation of the Andromeda Nebula from a Spectroscopic Survey of Emission Regions,''
  Astrophys.\ J.\  {\bf 159} (1970) 379.
  %%CITATION = ASJOA,159,379;%%
\bibitem{Rubin:1980zd}
  V.~C.~Rubin, N.~Thonnard and W.~K.~Ford, Jr.,
  %``Rotational properties of 21 SC galaxies with a large range of luminosities and radii, from NGC 4605 /R = 4kpc/ to UGC 2885 /R = 122 kpc/,''
  Astrophys.\ J.\  {\bf 238} (1980) 471.
  %%CITATION = ASJOA,238,471;%%
\bibitem{Rubin:1985ze}
  V.~C.~Rubin, D.~Burstein, W.~K.~Ford, Jr. and N.~Thonnard,
  %``Rotation velocities of 16 SA galaxies and a comparison of Sa, Sb, and SC rotation properties,''
  Astrophys.\ J.\  {\bf 289} (1985) 81.
  %%CITATION = ASJOA,289,81;%%
\bibitem{Clowe:2006eq}
  D.~Clowe, M.~Bradac, A.~H.~Gonzalez, M.~Markevitch, S.~W.~Randall, C.~Jones and D.~Zaritsky,
  %``A direct empirical proof of the existence of dark matter,''
  Astrophys.\ J.\  {\bf 648} (2006) L109
  [astro-ph/0608407].
  %%CITATION = ASTRO-PH/0608407;%%
\bibitem{Amanullah:2010vv}
  R.~Amanullah, C.~Lidman, D.~Rubin, G.~Aldering, P.~Astier, K.~Barbary, M.~S.~Burns and A.~Conley {\it et al.},
  %``Spectra and Light Curves of Six Type Ia Supernovae at 0.511 < z < 1.12 and the Union2 Compilation,''
  Astrophys.\ J.\  {\bf 716} (2010) 712
  [arXiv:1004.1711 [astro-ph.CO]].
  %%CITATION = ARXIV:1004.1711;%%
\bibitem{Iocco:2008va}
  F.~Iocco, G.~Mangano, G.~Miele, O.~Pisanti and P.~D.~Serpico,
  %``Primordial Nucleosynthesis: from precision cosmology to fundamental physics,''
  Phys.\ Rept.\  {\bf 472} (2009) 1
  [arXiv:0809.0631 [astro-ph]].
  %%CITATION = ARXIV:0809.0631;%%
\bibitem{Massey:2007wb}
  R.~Massey, J.~Rhodes, R.~Ellis, N.~Scoville, A.~Leauthaud, A.~Finoguenov, P.~Capak and D.~Bacon {\it et al.},
  %``Dark matter maps reveal cosmic scaffolding,''
  Nature {\bf 445} (2007) 286
  [astro-ph/0701594].
  %%CITATION = ASTRO-PH/0701594;%%
\bibitem{Allen:2002eu}
  S.~W.~Allen, A.~C.~Fabian, R.~W.~Schmidt and H.~Ebeling,
  %``Cosmological constraints from the local x-ray luminosity function of the most x-ray luminous galaxy clusters,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 342} (2003) 287
  [astro-ph/0208394].
  %%CITATION = ASTRO-PH/0208394;%%
\bibitem{Baumann:2009ds}
  D.~Baumann,
  %``TASI Lectures on Inflation,''
  arXiv:0907.5424 [hep-th].
  %%CITATION = ARXIV:0907.5424;%%
\bibitem{Akrami:2012vf}
  Y.~Akrami, T.~S.~Koivisto and M.~Sandstad,
  %``Accelerated expansion from ghost-free bigravity: a statistical analysis with improved generality,''
  arXiv:1209.0457 [astro-ph.CO].
  %%CITATION = ARXIV:1209.0457;%%
\bibitem{Bengtsson:1994vn} 
  I.~Bengtsson,
  %``Note on massive spin-2 in curved space,''
  J.\ Math.\ Phys.\  {\bf 36}, 5805 (1995)
  [gr-qc/9411057].
  %%CITATION = GR-QC/9411057;%%
\bibitem{Zinoviev:2001dt}
  Y.~.M.~Zinoviev,
  %``On massive high spin particles in AdS,''
  hep-th/0108192.
  %%CITATION = HEP-TH/0108192;%%
\bibitem{Zinoviev:2011fv}
  Y.~.M.~Zinoviev,
  %``Gravitational cubic interactions for a massive mixed symmetry gauge field,''
  Class.\ Quant.\ Grav.\  {\bf 29} (2012) 015013
  [arXiv:1107.3222 [hep-th]].
  %%CITATION = ARXIV:1107.3222;%%
\bibitem{deRham:2012kf}
  C.~de Rham and S.~Renaux-Petel,
  %``Massive Gravity on de Sitter and Unique Candidate for Partially
  %Massless Gravity,'' 
  arXiv:1206.3482 [hep-th].
  %%CITATION = ARXIV:1206.3482;%%
\bibitem{Joung:2012rv}
  E.~Joung, L.~Lopez and M.~Taronna,
  %``On the cubic interactions of massive and partially-massless higher spins in (A)dS,''
  JHEP {\bf 1207} (2012) 041
  [arXiv:1203.6578 [hep-th]].
  %%CITATION = ARXIV:1203.6578;%%
\bibitem{Lovelock:1971yv}
  D.~Lovelock,
  %``The Einstein tensor and its generalizations,''
  J.\ Math.\ Phys.\  {\bf 12} (1971) 498.
  %%CITATION = JMAPA,12,498;%%
\bibitem{Sisman:2012rc}
  T.~C.~Sisman, I.~Gullu and B.~Tekin,
  %``Spectra, vacua and the unitarity of Lovelock gravity in D-dimensional AdS spacetimes,''
  Phys.\ Rev.\ D {\bf 86} (2012) 044041
  [arXiv:1204.3814 [hep-th]].
  %%CITATION = ARXIV:1204.3814;%%
  
  
  
  
%%%%%%%%%%%%%%%%%%%%%%%%%%% ADDED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
\bibitem{Bergshoeff:2009aq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``More on Massive 3D Gravity,''
  Phys.\ Rev.\ D {\bf 79} (2009) 124042
  [arXiv:0905.1259 [hep-th]].
  %%CITATION = ARXIV:0905.1259;%%
\bibitem{Kleinschmidt:2012rs}
  A.~Kleinschmidt, T.~Nutma and A.~Virmani,
  %``On unitary subsectors of polycritical gravities,''
  Gen.\  Rel.\  Grav.\  {\bf 45} (2013) 727
  [arXiv:1206.7095 [hep-th]].
  %%CITATION = ARXIV:1206.7095;%%
\bibitem{Gullu:2010pc}
  I.~Gullu, T.~C.~Sisman and B.~Tekin,
  %``Born-Infeld extension of new massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 27} (2010) 162001
  [arXiv:1003.3935 [hep-th]].
  %%CITATION = ARXIV:1003.3935;%%
\bibitem{Paulos:2010ke}
  M.~F.~Paulos,
  %``New massive gravity extended with an arbitrary number of curvature corrections,''
  Phys.\ Rev.\ D {\bf 82} (2010) 084042
  [arXiv:1005.1646 [hep-th]].
  %%CITATION = ARXIV:1005.1646;%%
\bibitem{Kaku:1977pa}
  M.~Kaku, P.~K.~Townsend and P.~van Nieuwenhuizen,
  %``Gauge Theory of the Conformal and Superconformal Group,''
  Phys.\ Lett.\ B {\bf 69} (1977) 304.
  %%CITATION = PHLTA,B69,304;%%
\bibitem{Deser:2012qg}
  S.~Deser, E.~Joung and A.~Waldron,
  %``Partial Masslessness and Conformal Gravity,''
  J.\ Phys.\ A (2012)
  [arXiv:1208.1307 [hep-th]].
  %%CITATION = ARXIV:1208.1307;%%
\bibitem{Stelle:1976gc}
  K.~S.~Stelle,
  %``Renormalization of Higher Derivative Quantum Gravity,''
  Phys.\ Rev.\ D {\bf 16} (1977) 953.
  %%CITATION = PHRVA,D16,953;%%
\bibitem{Stelle:1977ry}
  K.~S.~Stelle,
  %``Classical Gravity with Higher Derivatives,''
  Gen.\ Rel.\ Grav.\  {\bf 9} (1978) 353.
  %%CITATION = GRGVA,9,353;%%
\bibitem{Bach}
  R.~Bach,
  Math.\ Zeitschr.\ {\bf 9} (1921) 110.
  %%CITATION = GRGVA,9,353;%%  
\bibitem{Fradkin:1981iu}
  E.~S.~Fradkin and A.~A.~Tseytlin,
  %``Renormalizable asymptotically free quantum theory of gravity,''
  Nucl.\ Phys.\ B {\bf 201} (1982) 469.
  %%CITATION = NUPHA,B201,469;%%  
\bibitem{Lee:1982cp}
  S.~C.~Lee and P.~van Nieuwenhuizen,
  %``Counting Of States In Higher Derivative Field Theories,''
  Phys.\ Rev.\ D {\bf 26} (1982) 934.
  %%CITATION = PHRVA,D26,934;%%
\bibitem{Riegert:1984hf}
  R.~J.~Riegert,
  %``The Particle Content Of Linearized Conformal Gravity,''
  Phys.\ Lett.\ A {\bf 105} (1984) 110.
  %%CITATION = PHLTA,A105,110;%%
\bibitem{Maldacena:2011mk}
  J.~Maldacena,
  %``Einstein Gravity from Conformal Gravity,''
  arXiv:1105.5632 [hep-th].
  %%CITATION = ARXIV:1105.5632;%%
\bibitem{Ade:2013ktc}
  P.~A.~R.~Ade {\it et al.}  [Planck Collaboration],
  %``Planck 2013 results. I. Overview of products and scientific results,''
  arXiv:1303.5062 [astro-ph.CO].
  %%CITATION = ARXIV:1303.5062;%%  
\bibitem{Hinshaw:2012aka}
  G.~Hinshaw {\it et al.}  [WMAP Collaboration],
  %``Nine-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Parameter Results,''
  arXiv:1212.5226 [astro-ph.CO].
  %%CITATION = ARXIV:1212.5226;%% 
\bibitem{Deser:1983mm}
  S.~Deser and R.~I.~Nepomechie,
  %``Gauge Invariance Versus Masslessness In De Sitter Space,''
  Annals Phys.\  {\bf 154} (1984) 396.
  %%CITATION = APNYA,154,396;%%
\bibitem{Deser:2001pe}
  S.~Deser and A.~Waldron,
  %``Gauge invariances and phases of massive higher spins in (A)dS,''
  Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 031601
  [hep-th/0102166].
  %%CITATION = HEP-TH/0102166;%%
 \bibitem{Deser:2001us}
  S.~Deser and A.~Waldron,
  %``Partial masslessness of higher spins in (A)dS,''
  Nucl.\ Phys.\ B {\bf 607} (2001) 577
  [hep-th/0103198].
  %%CITATION = HEP-TH/0103198;%%
\bibitem{Deser:2001wx}
  S.~Deser and A.~Waldron,
  %``Stability of massive cosmological gravitons,''
  Phys.\ Lett.\ B {\bf 508} (2001) 347
  [hep-th/0103255].
  %%CITATION = HEP-TH/0103255;%%
\bibitem{Deser:2001xr}
  S.~Deser and A.~Waldron,
  %``Null propagation of partially massless higher spins in (A)dS and cosmological constant speculations,''
  Phys.\ Lett.\ B {\bf 513} (2001) 137
  [hep-th/0105181].
  %%CITATION = HEP-TH/0105181;%%
\bibitem{Deser:2004ji}
  S.~Deser and A.~Waldron,
  %``Conformal invariance of partially massless higher spins,''
  Phys.\ Lett.\ B {\bf 603} (2004) 30
  [hep-th/0408155].
  %%CITATION = HEP-TH/0408155;%%  
\bibitem{Deser:2006zx}
  S.~Deser and A.~Waldron,
  %``Partially Massless Spin 2 Electrodynamics,''
  Phys.\ Rev.\ D {\bf 74} (2006) 084036
  [hep-th/0609113].
  %%CITATION = HEP-TH/0609113;%%
\bibitem{Higuchi:1986py}
  A.~Higuchi,
  %``Forbidden Mass Range For Spin-2 Field Theory In De Sitter Space-time,''
  Nucl.\ Phys.\ B {\bf 282} (1987) 397.
  %%CITATION = NUPHA,B282,397;%%
\bibitem{Higuchi:1989gz}
  A.~Higuchi,
  %``Massive Symmetric Tensor Field In Space-times With A Positive Cosmological Constant,''
  Nucl.\ Phys.\ B {\bf 325} (1989) 745.
  %%CITATION = NUPHA,B325,745;%%
\bibitem{Joung:2012rv}
  E.~Joung, L.~Lopez and M.~Taronna,
  %``On the cubic interactions of massive and partially-massless higher spins in (A)dS,''
  JHEP {\bf 1207} (2012) 041
  [arXiv:1203.6578 [hep-th]].
  %%CITATION = ARXIV:1203.6578;%%
\bibitem{Zinoviev:2006im}
  Y.~.M.~Zinoviev,
  %``On massive spin 2 interactions,''
  Nucl.\ Phys.\ B {\bf 770} (2007) 83
  [hep-th/0609170].
  %%CITATION = HEP-TH/0609170;%%
\bibitem{Deser:2013uy}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``Nonlinear Partially Massless from Massive Gravity?,''
  Phys.\  Rev.\  D 87, {\bf 101501} (R) (2013)
  [arXiv:1301.5621 [hep-th]].
  %%CITATION = ARXIV:1301.5621;%%
\bibitem{Garidi:2003ys}
  T.~Garidi,
  %``What is mass in de Sitterian physics?,''
  hep-th/0309104.
  %%CITATION = HEP-TH/0309104;%%  
\bibitem{deRham:2013wv}
  C.~de Rham, K.~Hinterbichler, R.~A.~Rosen and A.~J.~Tolley,
  %``Evidence for and Obstructions to Non-Linear Partially Massless Gravity,''
  arXiv:1302.0025 [hep-th].
  %%CITATION = ARXIV:1302.0025;%%  
\bibitem{deRham:2012kf}
  C.~de Rham and S.~Renaux-Petel,
  %``Massive Gravity on de Sitter and Unique Candidate for Partially Massless Gravity,''
  JCAP {\bf 1301} (2013) 035
  [arXiv:1206.3482 [hep-th]].
  %%CITATION = ARXIV:1206.3482;%% 
\bibitem{Akrami:2013ffa}
  Y.~Akrami, T.~S.~Koivisto, D.~F.~Mota and M.~Sandstad,
  %``Bimetric gravity doubly coupled to matter: theory and cosmological implications,''
  arXiv:1306.0004 [hep-th].
  %%CITATION = ARXIV:1306.0004;%%
\bibitem{Ruegg:2003ps}
  H.~Ruegg and M.~Ruiz-Altaba,
  %``The Stueckelberg field,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 19} (2004) 3265
  [hep-th/0304245].
  %%CITATION = HEP-TH/0304245;%%
\bibitem{Henneaux:1997bm}
  M.~Henneaux,
  %``Consistent interactions between gauge fields: The Cohomological approach,''
  Contemp.\ Math.\  {\bf 219} (1998) 93
  [hep-th/9712226].
  %%CITATION = HEP-TH/9712226;%%
\bibitem{Wigner:1939cj}
  E.~P.~Wigner,
  %``On Unitary Representations of the Inhomogeneous Lorentz Group,''
  Annals Math.\  {\bf 40} (1939) 149
   [Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 6} (1989) 9].
  %%CITATION = ANMAA,40,149;%%
\bibitem{Boulware:1972zf}
  D.~G.~Boulware and S.~Deser,
  %``Inconsistency of finite range gravitation,''
  Phys.\ Lett.\ B {\bf 40} (1972) 227.
  %%CITATION = PHLTA,B40,227;%%
\bibitem{ArkaniHamed:2003uy}
  N.~Arkani-Hamed, H.~-C.~Cheng, M.~A.~Luty and S.~Mukohyama,
  %``Ghost condensation and a consistent infrared modification of gravity,''
  JHEP {\bf 0405} (2004) 074
  [hep-th/0312099].
  %%CITATION = HEP-TH/0312099;%%
\bibitem{Kaluza:1921tu}
  T.~Kaluza,
  %``On the Problem of Unity in Physics,''
  Sitzungsber.\ Preuss.\ Akad.\ Wiss.\ Berlin (Math.\ Phys.\ ) {\bf 1921} (1921) 966.
  %%CITATION = SPWPA,1921,966;%%  
\bibitem{Klein:1926tv}
  O.~Klein,
  %``Quantum Theory and Five-Dimensional Theory of Relativity. (In German and English),''
  Z.\ Phys.\  {\bf 37} (1926) 895
   [Surveys High Energ.\ Phys.\  {\bf 5} (1986) 241].
  %%CITATION = ZEPYA,37,895;%% 
\bibitem{Einstein:1916vd}
  A.~Einstein,
  %``The Foundation of the General Theory of Relativity,''
  Annalen Phys.\  {\bf 49} (1916) 769
   [Annalen Phys.\  {\bf 14} (2005) 517].
  %%CITATION = ANPYA,49,769;%%   
\bibitem{Date:2010xr}
  G.~Date,
  %``Lectures on Constrained Systems,''
  arXiv:1010.2062 [gr-qc].
  %%CITATION = ARXIV:1010.2062;%%
\bibitem{Khoury:2011ay}
  J.~Khoury, G.~E.~J.~Miller and A.~J.~Tolley,
  %``Spatially Covariant Theories of a Transverse, Traceless Graviton, Part I: Formalism,''
  Phys.\ Rev.\ D {\bf 85} (2012) 084002
  [arXiv:1108.1397 [hep-th]].
  %%CITATION = ARXIV:1108.1397;%%
\bibitem{Kluson:2011qe}
  J.~Kluson,
  %``Note About Hamiltonian Structure of Non-Linear Massive Gravity,''
  JHEP {\bf 1201} (2012) 013
  [arXiv:1109.3052 [hep-th]].
  %%CITATION = ARXIV:1109.3052;%%
\bibitem{Kluson:2011rt}
  J.~Kluson,
  %``Comments About Hamiltonian Formulation of Non-Linear Massive Gravity with Stuckelberg Fields,''
  JHEP {\bf 1206} (2012) 170
  [arXiv:1112.5267 [hep-th]].
  %%CITATION = ARXIV:1112.5267;%%
\bibitem{Kluson:2012gz}
  J.~Kluson,
  %``Remark About Hamiltonian Formulation of Non-Linear Massive Gravity in Stuckelberg Formalism,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124005
  [arXiv:1202.5899 [hep-th]].
  %%CITATION = ARXIV:1202.5899;%%  
\bibitem{Lee:1977yc}
  B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
  %``The Strength of Weak Interactions at Very High-Energies and the Higgs Boson Mass,''
  Phys.\ Rev.\ Lett.\  {\bf 38} (1977) 883.
  %%CITATION = PRLTA,38,883;%%  
\bibitem{Golovnev:2011aa}
  A.~Golovnev,
  %``On the Hamiltonian analysis of non-linear massive gravity,''
  Phys.\ Lett.\ B {\bf 707} (2012) 404
  [arXiv:1112.2134 [gr-qc]].
  %%CITATION = ARXIV:1112.2134;%%
\bibitem{Buchbinder:2012wb}
  I.~L.~Buchbinder, D.~D.~Pereira and I.~L.~Shapiro,
  %``One-loop divergences in massive gravity theory,''
  Phys.\ Lett.\ B {\bf 712} (2012) 104
  [arXiv:1201.3145 [hep-th]].
  %%CITATION = ARXIV:1201.3145;%%
\bibitem{Boulanger:2000rq}
  N.~Boulanger, T.~Damour, L.~Gualtieri and M.~Henneaux,
  %``Inconsistency of interacting, multigraviton theories,''
  Nucl.\ Phys.\ B {\bf 597} (2001) 127
  [hep-th/0007220].
  %%CITATION = HEP-TH/0007220;%%  
\bibitem{Isham:1971gm}
  C.~J.~Isham, A.~Salam and J.~A.~Strathdee,
  %``F-dominance of gravity,''
  Phys.\ Rev.\ D {\bf 3} (1971) 867.
  %%CITATION = PHRVA,D3,867;%%  
\bibitem{deRham:2010tw}
  C.~de Rham, G.~Gabadadze, L.~Heisenberg and D.~Pirtskhalava,
  %``Cosmic Acceleration and the Helicity-0 Graviton,''
  Phys.\ Rev.\ D {\bf 83} (2011) 103516
  [arXiv:1010.1780 [hep-th]].
  %%CITATION = ARXIV:1010.1780;%%  
\bibitem{D'Amico:2011jj}
  G.~D'Amico, C.~de Rham, S.~Dubovsky, G.~Gabadadze, D.~Pirtskhalava and A.~J.~Tolley,
  %``Massive Cosmologies,''
  Phys.\ Rev.\ D {\bf 84} (2011) 124046
  [arXiv:1108.5231 [hep-th]].
  %%CITATION = ARXIV:1108.5231;%%    
\bibitem{Comelli:2011wq}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``Spherically Symmetric Solutions in Ghost-Free Massive Gravity,''
  Phys.\ Rev.\ D {\bf 85} (2012) 024044
  [arXiv:1110.4967 [hep-th]].
  %%CITATION = ARXIV:1110.4967;%%
\bibitem{Volkov:2012wp}
  M.~S.~Volkov,
  %``Hairy black holes in the ghost-free bigravity theory,''
  Phys.\ Rev.\ D {\bf 85} (2012) 124043
  [arXiv:1202.6682 [hep-th]].
  %%CITATION = ARXIV:1202.6682;%%
\bibitem{Deser:2013gpa}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``No consistent bimetric gravity?,''
  arXiv:1306.0647 [hep-th].
  %%CITATION = ARXIV:1306.0647;%%
\bibitem{Ostrogradski}
  M.~Ostrogradski,
  Mem.\ Ac.\ St.~Petersbourg  {\bf VI} (1850) 385. 
\bibitem{Bach}
  R.~Bach,
  Mathematische\ Zeitschrift  {\bf 9} (1921) 110. 
\bibitem{Mannheim:2011ds}
  P.~D.~Mannheim,
  %``Making the Case for Conformal Gravity,''
  Found.\ Phys.\  {\bf 42} (2012) 388
  [arXiv:1101.2186 [hep-th]].
  %%CITATION = ARXIV:1101.2186;%%  
\bibitem{Bender:2007wu}
  C.~M.~Bender and P.~D.~Mannheim,
  %``No-ghost theorem for the fourth-order derivative Pais-Uhlenbeck oscillator model,''
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 110402
  [arXiv:0706.0207 [hep-th]].    
\bibitem{Volkov:2013roa}
  M.~S.~Volkov,
  %``Self-accelerating cosmologies and hairy black holes in ghost-free bigravity and massive gravity,''
  arXiv:1304.0238 [hep-th].
  %%CITATION = ARXIV:1304.0238;%% 
\bibitem{Ondo:2013wka}
  N.~A.~Ondo and A.~J.~Tolley,
  %``Complete Decoupling Limit of Ghost-free Massive Gravity,''
  arXiv:1307.4769 [hep-th]. 
\bibitem{Gabadadze:2013ria}
  G.~Gabadadze, K.~Hinterbichler, D.~Pirtskhalava and Y.~Shang,
  %``On the Potential for General Relativity and its Geometry,''
  arXiv:1307.2245 [hep-th].
  %%CITATION = ARXIV:1307.2245;%%    
\bibitem{Deffayet:2012nr}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``Covariant constraints in ghost free massive gravity,''
  JCAP {\bf 1301} (2013) 032
  [arXiv:1207.6338 [hep-th]].
  %%CITATION = ARXIV:1207.6338;%%
\bibitem{Deffayet:2012zc}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``A note on 'symmetric' vielbeins in bimetric, massive, perturbative and non perturbative gravities,''
  JHEP {\bf 1303} (2013) 086
  [arXiv:1208.4493 [gr-qc]].
  %%CITATION = ARXIV:1208.4493;%% 
\bibitem{Brito:2013wya}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Massive spin-2 fields on black hole spacetimes: Instability of the Schwarzschild and Kerr solutions and bounds on the graviton mass,''
  Phys.\  Rev.\ D {\bf 88} (2013) 023514
  [arXiv:1304.6725 [gr-qc]].
  %%CITATION = ARXIV:1304.6725;%% 
\bibitem{Brito:2013yxa}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Partially massless gravitons do not destroy general relativity black holes,''
  Phys.\  Rev.\ D {\bf 87} (2013) 124024
  [arXiv:1306.0908 [gr-qc]].
  %%CITATION = ARXIV:1306.0908;%%   
\bibitem{Gregory:1993vy}
  R.~Gregory and R.~Laflamme,
  %``Black strings and p-branes are unstable,''
  Phys.\ Rev.\ Lett.\  {\bf 70} (1993) 2837
  [hep-th/9301052].
  %%CITATION = HEP-TH/9301052;%% 
\bibitem{Enander:2013kza}
  J.~Enander and E.~Mortsell,
  %``Strong lensing constraints on bimetric massive gravity,''
  arXiv:1306.1086 [astro-ph.CO].
  %%CITATION = ARXIV:1306.1086;%%   
\bibitem{Babichev:2013una}
  E.~Babichev and A.~Fabbri,
  %``Instability of black holes in massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 30} (2013) 152001
  [arXiv:1304.5992 [gr-qc]].
  %%CITATION = ARXIV:1304.5992;%%
\bibitem{Sjors:2011iv}
  S.~Sjors and E.~Mortsell,
  %``Spherically Symmetric Solutions in Massive Gravity and Constraints from Galaxies,''
  JHEP {\bf 1302} (2013) 080
  [arXiv:1111.5961 [gr-qc]].
  %%CITATION = ARXIV:1111.5961;%%
\bibitem{Hinterbichler:2013eza}
  K.~Hinterbichler,
  %``Ghost-Free Derivative Interactions for a Massive Graviton,''
  arXiv:1305.7227 [hep-th].
  %%CITATION = ARXIV:1305.7227;%%      
\bibitem{deRham:2013qqa}
  C.~de Rham, L.~Heisenberg and R.~H.~Ribeiro,
  %``Quantum Corrections in Massive Gravity,''
  arXiv:1307.7169 [hep-th].
  %%CITATION = ARXIV:1307.7169;%%  
\bibitem{Cai:2013lqa}
  Y.~-F.~Cai, F.~Duplessis and E.~N.~Saridakis,
  %``$F(R)$ nonlinear massive gravity and cosmological implications,''
  arXiv:1307.7150 [hep-th].
  %%CITATION = ARXIV:1307.7150;%%  
\bibitem{Gabadadze:2012tr}
  G.~Gabadadze, K.~Hinterbichler, J.~Khoury, D.~Pirtskhalava and M.~Trodden,
  %``A Covariant Master Theory for Novel Galilean Invariant Models and Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124004
  [arXiv:1208.5773 [hep-th]].
  %%CITATION = ARXIV:1208.5773;%%
\bibitem{D'Amico:2012zv}
  G.~D'Amico, G.~Gabadadze, L.~Hui and D.~Pirtskhalava,
  %``Quasi-Dilaton: Theory and Cosmology,''
  arXiv:1206.4253 [hep-th].
  %%CITATION = ARXIV:1206.4253;%%   
%\cite{Ondo:2013wka}
\bibitem{Ondo:2013wka}
  N.~A.~Ondo and A.~J.~Tolley,
  %``Complete Decoupling Limit of Ghost-free Massive Gravity,''
  arXiv:1307.4769 [hep-th].
  %%CITATION = ARXIV:1307.4769;%%  
\bibitem{Huang:2013mha}
  Q.~-G.~Huang, K.~-C.~Zhang and S.~-Y.~Zhou,
  %``Generalized massive gravity in arbitrary dimensions and its Hamiltonian formulation,''
  arXiv:1306.4740 [hep-th].
  %%CITATION = ARXIV:1306.4740;%%   
\bibitem{Nojiri:2013zza}
  S.~'I.~Nojiri and S.~D.~Odintsov,
  %``Accelerating cosmology in modified gravity: from convenient $F(R)$ or string-inspired theory to bimetric $F(R)$ gravity,''
  arXiv:1306.4426 [gr-qc].
  %%CITATION = ARXIV:1306.4426;%% 
\bibitem{Huang:2012pe}
  Q.~-G.~Huang, Y.~-S.~Piao and S.~-Y.~Zhou,
  %``Mass-Varying Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124014
  [arXiv:1206.5678 [hep-th]].
  %%CITATION = ARXIV:1206.5678;%% 
\bibitem{Nomura:2012xr}
  K.~Nomura and J.~Soda,
  %``When is Multimetric Gravity Ghost-free?,''
  Phys.\ Rev.\ D {\bf 86} (2012) 084052
  [arXiv:1207.3637 [hep-th]].
  %%CITATION = ARXIV:1207.3637;%%    
  
  
    
  
\end{thebibliography}

==> Bibliography/references.tex <==
\begin{thebibliography}{999}
\bibitem{Einstein:1916vd}
  A.~Einstein,
  %``The Foundation of the General Theory of Relativity,''
  Annalen Phys.\  {\bf 49} (1916) 769
   [Annalen Phys.\  {\bf 14} (2005) 517].
  %%CITATION = ANPYA,49,769;%% 
\bibitem{Weinberg:1988cp}
  S.~Weinberg,
  %``The Cosmological Constant Problem,''
  Rev.\ Mod.\ Phys.\  {\bf 61} (1989) 1.
  %%CITATION = RMPHA,61,1;%%    
\bibitem{Zwicky:1933gu}
  F.~Zwicky,
  %``Spectral displacement of extra galactic nebulae,''
  Helv.\ Phys.\ Acta {\bf 6} (1933) 110.
  %%CITATION = HPACA,6,110;%%  
\bibitem{Fierz:1939ix}
  M.~Fierz and W.~Pauli,
  %``On relativistic wave equations for particles of arbitrary spin in 
  %an electromagnetic field,'' 
  Proc.\ Roy.\ Soc.\ Lond.\ A {\bf 173} (1939) 211.
  %%CITATION = PRSLA,A173,211;%%
\bibitem{vanDam:1970vg}
  H.~van Dam and M.~J.~G.~Veltman,
  %``Massive and massless Yang-Mills and gravitational fields,''
  Nucl.\ Phys.\ B {\bf 22} (1970) 397.
  %%CITATION = NUPHA,B22,397;%%
\bibitem{Zakharov:1970cc}
  V.~I.~Zakharov,
  %``Linearized gravitation theory and the graviton mass,''
  JETP Lett.\  {\bf 12} (1970) 312
   [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 12} (1970) 447].
  %%CITATION = JTPLA,12,312;%%
\bibitem{Vainshtein:1972sx}
  A.~I.~Vainshtein,
  %``To the problem of nonvanishing gravitation mass,''
  Phys.\ Lett.\ B {\bf 39} (1972) 393.
  %%CITATION = PHLTA,B39,393;%%
\bibitem{Boulware:1972zf}
  D.~G.~Boulware and S.~Deser,
  %``Inconsistency of finite range gravitation,''
  Phys.\ Lett.\ B {\bf 40} (1972) 227.
  %%CITATION = PHLTA,B40,227;%%
\bibitem{Boulware:1973my}
  D.~G.~Boulware and S.~Deser,
  %``Can gravitation have a finite range?,''
  Phys.\ Rev.\ D {\bf 6} (1972) 3368.
  %%CITATION = PHRVA,D6,3368;%%
\bibitem{Creminelli:2005qk}
  P.~Creminelli, A.~Nicolis, M.~Papucci and E.~Trincherini,
  %``Ghosts in massive gravity,''
  JHEP {\bf 0509} (2005) 003
  [hep-th/0505147].
  %%CITATION = HEP-TH/0505147;%%  
\bibitem{ArkaniHamed:2002sp}
  N.~Arkani-Hamed, H.~Georgi and M.~D.~Schwartz,
  %``Effective field theory for massive gravitons and gravity in
  %theory space,'' 
  Annals Phys.\  {\bf 305} (2003) 96
  [hep-th/0210184].
  %%CITATION = HEP-TH/0210184;%%
\bibitem{deRham:2010ik}
  C.~de Rham and G.~Gabadadze,
  %``Generalization of the Fierz-Pauli Action,''
  Phys.\ Rev.\ D {\bf 82} (2010) 044020
  [arXiv:1007.0443 [hep-th]].
  %%CITATION = ARXIV:1007.0443;%%
\bibitem{deRham:2010kj}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Resummation of Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 106} (2011) 231101
  [arXiv:1011.1232 [hep-th]].
  %%CITATION = ARXIV:1011.1232;%%
\bibitem{Hassan:2011vm}
  S.~F.~Hassan and R.~A.~Rosen,
  %``On nonlinear Actions for Massive Gravity,''
  JHEP {\bf 1107} (2011) 009
  [arXiv:1103.6055 [hep-th]].
  %%CITATION = ARXIV:1103.6055;%%
\bibitem{Hassan:2011hr}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Resolving the Ghost Problem in nonlinear Massive Gravity,''
  Phys.\ Rev.\ Lett.\  {\bf 108} (2012) 041101
  [arXiv:1106.3344 [hep-th]].
  %%CITATION = ARXIV:1106.3344;%%
\bibitem{Hassan:2011ea}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Confirmation of the Secondary Constraint and Absence of Ghost in Massive Gravity and Bimetric Gravity,''
  JHEP {\bf 1204} (2012) 123
  [arXiv:1111.2070 [hep-th]].
  %%CITATION = ARXIV:1111.2070;%%
\bibitem{Hassan:2011zd}
  S.~F.~Hassan and R.~A.~Rosen,
  %``Bimetric Gravity from Ghost-free Massive Gravity,''
  JHEP {\bf 1202} (2012) 126
  [arXiv:1109.3515 [hep-th]].
  %%CITATION = ARXIV:1109.3515;%%
\bibitem{Rosen:1940zz}
  N.~Rosen,
  %``General Relativity and Flat Space. II,''
  Phys.\ Rev.\  {\bf 57} (1940) 150.
  %%CITATION = PHRVA,57,150;%%
\bibitem{Rosen:1975kk}
  N.~Rosen,
  %``Bimetric Theory of Gravitation,''
  In *Erice 1975, Proceedings, Topics In Theoretical and Experimental
  Gravitation Physics*, New York 1977, 273-294 
 \bibitem{Aragone:1971kh}
  C.~Aragone and S.~Deser,
  %``Constraints on gravitationally coupled tensor fields,''
  Nuovo Cim.\ A {\bf 3} (1971) 709.
  %%CITATION = NUCIA,A3,709;%%
\bibitem{Isham:1971gm}
  C.~J.~Isham, A.~Salam and J.~A.~Strathdee,
  %``F-dominance of gravity,''
  Phys.\ Rev.\ D {\bf 3} (1971) 867.
  %%CITATION = PHRVA,D3,867;%%  
\bibitem{Chamseddine:1978yu}
  A.~H.~Chamseddine, A.~Salam and J.~A.~Strathdee,
  %``Strong Gravity and Supersymmetry,''
  Nucl.\ Phys.\ B {\bf 136} (1978) 248.
  %%CITATION = NUPHA,B136,248;%%
\bibitem{Dvali:2000rv}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``Metastable gravitons and infinite volume extra dimensions,''
  Phys.\ Lett.\ B {\bf 484} (2000) 112
  [hep-th/0002190].
  %%CITATION = HEP-TH/0002190;%%
\bibitem{Dvali:2000hr}
  G.~R.~Dvali, G.~Gabadadze and M.~Porrati,
  %``4-D gravity on a brane in 5-D Minkowski space,''
  Phys.\ Lett.\ B {\bf 485} (2000) 208
  [hep-th/0005016].
  %%CITATION = HEP-TH/0005016;%%
\bibitem{Kaluza:1921tu}
  T.~Kaluza,
  %``On the Problem of Unity in Physics,''
  Sitzungsber.\ Preuss.\ Akad.\ Wiss.\ Berlin (Math.\ Phys.\ ) {\bf 1921} (1921) 966.
  %%CITATION = SPWPA,1921,966;%%  
\bibitem{Klein:1926tv}
  O.~Klein,
  %``Quantum Theory and Five-Dimensional Theory of Relativity. (In German and English),''
  Z.\ Phys.\  {\bf 37} (1926) 895
   [Surveys High Energ.\ Phys.\  {\bf 5} (1986) 241].
  %%CITATION = ZEPYA,37,895;%% 
\bibitem{Bergshoeff:2009hq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``Massive Gravity in Three Dimensions,''
  Phys.\ Rev.\ Lett.\  {\bf 102} (2009) 201301
  [arXiv:0901.1766 [hep-th]].
  %%CITATION = ARXIV:0901.1766;%%
\bibitem{Deser:1981wh}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Topologically Massive Gauge Theories,''
  Annals Phys.\  {\bf 140} (1982) 372
   [Erratum-ibid.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 185} (1988) 406]
   [Annals Phys.\  {\bf 281} (2000) 409].
  %%CITATION = APNYA,140,372;%%
\bibitem{Deser:1982vy}
  S.~Deser, R.~Jackiw and S.~Templeton,
  %``Three-Dimensional Massive Gauge Theories,''
  Phys.\ Rev.\ Lett.\  {\bf 48} (1982) 975.
  %%CITATION = PRLTA,48,975;%%
\bibitem{ArkaniHamed:2003uy}
  N.~Arkani-Hamed, H.~-C.~Cheng, M.~A.~Luty and S.~Mukohyama,
  %``Ghost condensation and a consistent infrared modification of gravity,''
  JHEP {\bf 0405} (2004) 074
  [hep-th/0312099].
  %%CITATION = HEP-TH/0312099;%%
\bibitem{Riess:1998cb}
  A.~G.~Riess {\it et al.}  [Supernova Search Team Collaboration],
  %``Observational evidence from supernovae for an accelerating universe and a cosmological constant,''
  Astron.\ J.\  {\bf 116} (1998) 1009
  [astro-ph/9805201].
  %%CITATION = ASTRO-PH/9805201;%%
\bibitem{Perlmutter:1998np}
  S.~Perlmutter {\it et al.}  [Supernova Cosmology Project Collaboration],
  %``Measurements of Omega and Lambda from 42 high redshift supernovae,''
  Astrophys.\ J.\  {\bf 517} (1999) 565
  [astro-ph/9812133].
  %%CITATION = ASTRO-PH/9812133;%%
\bibitem{Martin:2012bt}
  J.~Martin,
  %``Everything You Always Wanted To Know About The Cosmological Constant Problem (But Were Afraid To Ask),''
  Comptes Rendus Physique {\bf 13} (2012) 566
  [arXiv:1205.3365 [astro-ph.CO]].
  %%CITATION = ARXIV:1205.3365;%%
\bibitem{Wigner:1939cj}
  E.~P.~Wigner,
  %``On Unitary Representations of the Inhomogeneous Lorentz Group,''
  Annals Math.\  {\bf 40} (1939) 149
   [Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 6} (1989) 9].
  %%CITATION = ANMAA,40,149;%%
\bibitem{Hinterbichler:2011tt}
  K.~Hinterbichler,
  %``Theoretical Aspects of Massive Gravity,''
  Rev.\ Mod.\ Phys.\  {\bf 84} (2012) 671
  [arXiv:1105.3735 [hep-th]].
  %%CITATION = ARXIV:1105.3735;%%
\bibitem{Henneaux:1997bm}
  M.~Henneaux,
  %``Consistent interactions between gauge fields: The Cohomological approach,''
  Contemp.\ Math.\  {\bf 219} (1998) 93
  [hep-th/9712226].
  %%CITATION = HEP-TH/9712226;%%
\bibitem{Ruegg:2003ps}
  H.~Ruegg and M.~Ruiz-Altaba,
  %``The Stueckelberg field,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 19} (2004) 3265
  [hep-th/0304245].
  %%CITATION = HEP-TH/0304245;%%
\bibitem{Arnowitt:1962hi}
  R.~L.~Arnowitt, S.~Deser and C.~W.~Misner,
  %``The Dynamics of general relativity,''
  [gr-qc/0405109].
  %%CITATION = GR-QC/0405109;%%
\bibitem{Date:2010xr}
  G.~Date,
  %``Lectures on Constrained Systems,''
  arXiv:1010.2062 [gr-qc].
  %%CITATION = ARXIV:1010.2062;%%
\bibitem{Khoury:2011ay}
  J.~Khoury, G.~E.~J.~Miller and A.~J.~Tolley,
  %``Spatially Covariant Theories of a Transverse, Traceless Graviton, Part I: Formalism,''
  Phys.\ Rev.\ D {\bf 85} (2012) 084002
  [arXiv:1108.1397 [hep-th]].
  %%CITATION = ARXIV:1108.1397;%%
\bibitem{Deffayet:2012nr}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``Covariant constraints in ghost free massive gravity,''
  JCAP {\bf 1301} (2013) 032
  [arXiv:1207.6338 [hep-th]].
  %%CITATION = ARXIV:1207.6338;%%
\bibitem{Kluson:2011qe}
  J.~Kluson,
  %``Note About Hamiltonian Structure of Non-Linear Massive Gravity,''
  JHEP {\bf 1201} (2012) 013
  [arXiv:1109.3052 [hep-th]].
  %%CITATION = ARXIV:1109.3052;%%
\bibitem{Chamseddine:2011mu}
  A.~H.~Chamseddine and V.~Mukhanov,
  %``Massive Gravity Simplified: A Quadratic Action,''
  JHEP {\bf 1108} (2011) 091
  [arXiv:1106.5868 [hep-th]].
  %%CITATION = ARXIV:1106.5868;%%
\bibitem{Kluson:2011rt}
  J.~Kluson,
  %``Comments About Hamiltonian Formulation of Non-Linear Massive Gravity with Stuckelberg Fields,''
  JHEP {\bf 1206} (2012) 170
  [arXiv:1112.5267 [hep-th]].
  %%CITATION = ARXIV:1112.5267;%%
\bibitem{Kluson:2012gz}
  J.~Kluson,
  %``Remark About Hamiltonian Formulation of Non-Linear Massive Gravity in Stuckelberg Formalism,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124005
  [arXiv:1202.5899 [hep-th]].
  %%CITATION = ARXIV:1202.5899;%%  
\bibitem{Lee:1977yc}
  B.~W.~Lee, C.~Quigg and H.~B.~Thacker,
  %``The Strength of Weak Interactions at Very High-Energies and the Higgs Boson Mass,''
  Phys.\ Rev.\ Lett.\  {\bf 38} (1977) 883.
  %%CITATION = PRLTA,38,883;%%  
\bibitem{Chanowitz:1985hj}
  M.~S.~Chanowitz and M.~K.~Gaillard,
  %``The TeV Physics of Strongly Interacting W's and Z's,''
  Nucl.\ Phys.\ B {\bf 261} (1985) 379.
  %%CITATION = NUPHA,B261,379;%%
\bibitem{Ondo:2013wka}
  N.~A.~Ondo and A.~J.~Tolley,
  %``Complete Decoupling Limit of Ghost-free Massive Gravity,''
  arXiv:1307.4769 [hep-th]. 
\bibitem{deRham:2011rn}
  C.~de Rham, G.~Gabadadze and A.~J.~Tolley,
  %``Ghost free Massive Gravity in the St\'uckelberg language,''
  Phys.\ Lett.\ B {\bf 711} (2012) 190
  [arXiv:1107.3820 [hep-th]].
  %%CITATION = ARXIV:1107.3820;%%
\bibitem{Golovnev:2011aa}
  A.~Golovnev,
  %``On the Hamiltonian analysis of non-linear massive gravity,''
  Phys.\ Lett.\ B {\bf 707} (2012) 404
  [arXiv:1112.2134 [gr-qc]].
  %%CITATION = ARXIV:1112.2134;%%
\bibitem{Buchbinder:2012wb}
  I.~L.~Buchbinder, D.~D.~Pereira and I.~L.~Shapiro,
  %``One-loop divergences in massive gravity theory,''
  Phys.\ Lett.\ B {\bf 712} (2012) 104
  [arXiv:1201.3145 [hep-th]].
  %%CITATION = ARXIV:1201.3145;%%
\bibitem{Boulanger:2000rq}
  N.~Boulanger, T.~Damour, L.~Gualtieri and M.~Henneaux,
  %``Inconsistency of interacting, multigraviton theories,''
  Nucl.\ Phys.\ B {\bf 597} (2001) 127
  [hep-th/0007220].
  %%CITATION = HEP-TH/0007220;%%  
\bibitem{Damour:2002wu}
  T.~Damour, I.~I.~Kogan and A.~Papazoglou,
  %``Nonlinear bigravity and cosmic acceleration,''
  Phys.\ Rev.\ D {\bf 66} (2002) 104025
  [hep-th/0206044].
  %%CITATION = HEP-TH/0206044;%%
\bibitem{Nibbelink:2006sz}
  S.~Nibbelink Groot, M.~Peloso and M.~Sexton,
  %``Nonlinear Properties of Vielbein Massive Gravity,''
  Eur.\ Phys.\ J.\ C {\bf 51} (2007) 741
  [hep-th/0610169].
  %%CITATION = HEP-TH/0610169;%%
\bibitem{Damour:2002ws}
  T.~Damour and I.~I.~Kogan,
  %``Effective Lagrangians and universality classes of nonlinear
  %bigravity,'' 
  Phys.\ Rev.\ D {\bf 66} (2002) 104024
  [hep-th/0206042].
  %%CITATION = HEP-TH/0206042;%%
\bibitem{Akrami:2013ffa}
  Y.~Akrami, T.~S.~Koivisto, D.~F.~Mota and M.~Sandstad,
  %``Bimetric gravity doubly coupled to matter: theory and cosmological implications,''
  arXiv:1306.0004 [hep-th].
  %%CITATION = ARXIV:1306.0004;%%
\bibitem{Baccetti:2012bk}
  V.~Baccetti, P.~Martin-Moruno and M.~Visser,
  %``Massive gravity from bimetric gravity,''
  arXiv:1205.2158 [gr-qc].
  %%CITATION = ARXIV:1205.2158;%%
\bibitem{Hinterbichler:2012cn}
  K.~Hinterbichler and R.~A.~Rosen,
  %``Interacting Spin-2 Fields,''
  JHEP {\bf 1207} (2012) 047
  [arXiv:1203.5783 [hep-th]].
  %%CITATION = ARXIV:1203.5783;%%
\bibitem{Nomura:2012xr}
  K.~Nomura and J.~Soda,
  %``When is Multimetric Gravity Ghost-free?,''
  Phys.\ Rev.\ D {\bf 86} (2012) 084052
  [arXiv:1207.3637 [hep-th]].
  %%CITATION = ARXIV:1207.3637;%%    
\bibitem{Gabadadze:2013ria}
  G.~Gabadadze, K.~Hinterbichler, D.~Pirtskhalava and Y.~Shang,
  %``On the Potential for General Relativity and its Geometry,''
  arXiv:1307.2245 [hep-th].
  %%CITATION = ARXIV:1307.2245;%%    
\bibitem{Deffayet:2012zc}
  C.~Deffayet, J.~Mourad and G.~Zahariade,
  %``A note on 'symmetric' vielbeins in bimetric, massive, perturbative and non perturbative gravities,''
  JHEP {\bf 1303} (2013) 086
  [arXiv:1208.4493 [gr-qc]].
  %%CITATION = ARXIV:1208.4493;%% 
\bibitem{deRham:2010tw}
  C.~de Rham, G.~Gabadadze, L.~Heisenberg and D.~Pirtskhalava,
  %``Cosmic Acceleration and the Helicity-0 Graviton,''
  Phys.\ Rev.\ D {\bf 83} (2011) 103516
  [arXiv:1010.1780 [hep-th]].
  %%CITATION = ARXIV:1010.1780;%%  
\bibitem{Gumrukcuoglu:2011ew}
  A.~E.~Gumrukcuoglu, C.~Lin and S.~Mukohyama,
  %``Open FRW universes and self-acceleration from nonlinear massive gravity,''
  JCAP {\bf 1111} (2011) 030
  [arXiv:1109.3845 [hep-th]].
  %%CITATION = ARXIV:1109.3845;%%
\bibitem{D'Amico:2011jj}
  G.~D'Amico, C.~de Rham, S.~Dubovsky, G.~Gabadadze, D.~Pirtskhalava and A.~J.~Tolley,
  %``Massive Cosmologies,''
  Phys.\ Rev.\ D {\bf 84} (2011) 124046
  [arXiv:1108.5231 [hep-th]].
  %%CITATION = ARXIV:1108.5231;%%    
\bibitem{Volkov:2011an}
  M.~S.~Volkov,
  %``Cosmological solutions with massive gravitons in the bigravity
  %theory,'' 
  JHEP {\bf 1201} (2012) 035
  [arXiv:1110.6153 [hep-th]].
  %%CITATION = ARXIV:1110.6153;%%
\bibitem{Comelli:2011zm}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``FRW Cosmology in ghost-free Massive Gravity,''
  JHEP {\bf 1203} (2012) 067
   [Erratum-ibid.\  {\bf 1206} (2012) 020]
  [arXiv:1111.1983 [hep-th]].
  %%CITATION = ARXIV:1111.1983;%%
\bibitem{Hinshaw:2012aka}
  G.~Hinshaw {\it et al.}  [WMAP Collaboration],
  %``Nine-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Parameter Results,''
  arXiv:1212.5226 [astro-ph.CO].
  %%CITATION = ARXIV:1212.5226;%% 
\bibitem{Ade:2013ktc}
  P.~A.~R.~Ade {\it et al.}  [Planck Collaboration],
  %``Planck 2013 results. I. Overview of products and scientific results,''
  arXiv:1303.5062 [astro-ph.CO].
  %%CITATION = ARXIV:1303.5062;%%  
\bibitem{Comelli:2012db}
  D.~Comelli, M.~Crisostomi and L.~Pilo,
  %``Perturbations in Massive Gravity Cosmology,''
  JHEP {\bf 1206} (2012) 085
  [arXiv:1202.1986 [hep-th]].
  %%CITATION = ARXIV:1202.1986;%%
\bibitem{Berg:2012kn}
  M.~Berg, I.~Buchberger, J.~Enander, E.~Mortsell and S.~Sjors,
  %``Growth Histories in Bimetric Massive Gravity,''
  arXiv:1206.3496 [gr-qc].
  %%CITATION = ARXIV:1206.3496;%%
\bibitem{Comelli:2011wq}
  D.~Comelli, M.~Crisostomi, F.~Nesti and L.~Pilo,
  %``Spherically Symmetric Solutions in Ghost-Free Massive Gravity,''
  Phys.\ Rev.\ D {\bf 85} (2012) 024044
  [arXiv:1110.4967 [hep-th]].
  %%CITATION = ARXIV:1110.4967;%%
\bibitem{Volkov:2012wp}
  M.~S.~Volkov,
  %``Hairy black holes in the ghost-free bigravity theory,''
  Phys.\ Rev.\ D {\bf 85} (2012) 124043
  [arXiv:1202.6682 [hep-th]].
  %%CITATION = ARXIV:1202.6682;%%
\bibitem{Akrami:2012vf}
  Y.~Akrami, T.~S.~Koivisto and M.~Sandstad,
  %``Accelerated expansion from ghost-free bigravity: a statistical analysis with improved generality,''
  arXiv:1209.0457 [astro-ph.CO].
  %%CITATION = ARXIV:1209.0457;%%
\bibitem{Higuchi:1986py}
  A.~Higuchi,
  %``Forbidden Mass Range For Spin-2 Field Theory In De Sitter Space-time,''
  Nucl.\ Phys.\ B {\bf 282} (1987) 397.
  %%CITATION = NUPHA,B282,397;%%
\bibitem{Deser:1983mm}
  S.~Deser and R.~I.~Nepomechie,
  %``Gauge Invariance Versus Masslessness In De Sitter Space,''
  Annals Phys.\  {\bf 154} (1984) 396.
  %%CITATION = APNYA,154,396;%%
\bibitem{Deser:2001pe}
  S.~Deser and A.~Waldron,
  %``Gauge invariances and phases of massive higher spins in (A)dS,''
  Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 031601
  [hep-th/0102166].
  %%CITATION = HEP-TH/0102166;%%
\bibitem{Deser:2001us}
  S.~Deser and A.~Waldron,
  %``Partial masslessness of higher spins in (A)dS,''
  Nucl.\ Phys.\ B {\bf 607} (2001) 577
  [hep-th/0103198].
  %%CITATION = HEP-TH/0103198;%%
\bibitem{Deser:2001wx}
  S.~Deser and A.~Waldron,
  %``Stability of massive cosmological gravitons,''
  Phys.\ Lett.\ B {\bf 508} (2001) 347
  [hep-th/0103255].
  %%CITATION = HEP-TH/0103255;%%
\bibitem{Deser:2001xr}
  S.~Deser and A.~Waldron,
  %``Null propagation of partially massless higher spins in (A)dS and cosmological constant speculations,''
  Phys.\ Lett.\ B {\bf 513} (2001) 137
  [hep-th/0105181].
  %%CITATION = HEP-TH/0105181;%%
\bibitem{Deser:2004ji}
  S.~Deser and A.~Waldron,
  %``Conformal invariance of partially massless higher spins,''
  Phys.\ Lett.\ B {\bf 603} (2004) 30
  [hep-th/0408155].
  %%CITATION = HEP-TH/0408155;%%  
\bibitem{Deser:2006zx}
  S.~Deser and A.~Waldron,
  %``Partially Massless Spin 2 Electrodynamics,''
  Phys.\ Rev.\ D {\bf 74} (2006) 084036
  [hep-th/0609113].
  %%CITATION = HEP-TH/0609113;%%
\bibitem{Higuchi:1989gz}
  A.~Higuchi,
  %``Massive Symmetric Tensor Field In Space-times With A Positive Cosmological Constant,''
  Nucl.\ Phys.\ B {\bf 325} (1989) 745.
  %%CITATION = NUPHA,B325,745;%%
\bibitem{Garidi:2003ys}
  T.~Garidi,
  %``What is mass in de Sitterian physics?,''
  hep-th/0309104.
  %%CITATION = HEP-TH/0309104;%%  
\bibitem{Zinoviev:2006im}
  Y.~.M.~Zinoviev,
  %``On massive spin 2 interactions,''
  Nucl.\ Phys.\ B {\bf 770} (2007) 83
  [hep-th/0609170].
  %%CITATION = HEP-TH/0609170;%%
\bibitem{Joung:2012rv}
  E.~Joung, L.~Lopez and M.~Taronna,
  %``On the cubic interactions of massive and partially-massless higher spins in (A)dS,''
  JHEP {\bf 1207} (2012) 041
  [arXiv:1203.6578 [hep-th]].
  %%CITATION = ARXIV:1203.6578;%%
\bibitem{deRham:2012kf}
  C.~de Rham and S.~Renaux-Petel,
  %``Massive Gravity on de Sitter and Unique Candidate for Partially
  %Massless Gravity,'' 
  arXiv:1206.3482 [hep-th].
  %%CITATION = ARXIV:1206.3482;%%
\bibitem{Deser:2013uy}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``Nonlinear Partially Massless from Massive Gravity?,''
  Phys.\  Rev.\  D 87, {\bf 101501} (R) (2013)
  [arXiv:1301.5621 [hep-th]].
  %%CITATION = ARXIV:1301.5621;%%
\bibitem{deRham:2013wv}
  C.~de Rham, K.~Hinterbichler, R.~A.~Rosen and A.~J.~Tolley,
  %``Evidence for and Obstructions to Non-Linear Partially Massless Gravity,''
  arXiv:1302.0025 [hep-th].
  %%CITATION = ARXIV:1302.0025;%%  
\bibitem{Deser:2013gpa}
  S.~Deser, M.~Sandora and A.~Waldron,
  %``No consistent bimetric gravity?,''
  arXiv:1306.0647 [hep-th].
  %%CITATION = ARXIV:1306.0647;%%
\bibitem{Paulos:2012xe}
  M.~F.~Paulos and A.~J.~Tolley,
  %``Massive Gravity Theories and limits of Ghost-free Bigravity models,''
  arXiv:1203.4268 [hep-th].
  %%CITATION = ARXIV:1203.4268;%%
\bibitem{Sisman:2012rc}
  T.~C.~Sisman, I.~Gullu and B.~Tekin,
  %``Spectra, vacua and the unitarity of Lovelock gravity in D-dimensional AdS spacetimes,''
  Phys.\ Rev.\ D {\bf 86} (2012) 044041
  [arXiv:1204.3814 [hep-th]].
  %%CITATION = ARXIV:1204.3814;%%  
\bibitem{Stelle:1976gc}
  K.~S.~Stelle,
  %``Renormalization of Higher Derivative Quantum Gravity,''
  Phys.\ Rev.\ D {\bf 16} (1977) 953.
  %%CITATION = PHRVA,D16,953;%%
\bibitem{Stelle:1977ry}
  K.~S.~Stelle,
  %``Classical Gravity with Higher Derivatives,''
  Gen.\ Rel.\ Grav.\  {\bf 9} (1978) 353.
  %%CITATION = GRGVA,9,353;%%
\bibitem{Ostrogradski}
  M.~Ostrogradski,
  Mem.\ Ac.\ St.~Petersbourg  {\bf VI} (1850) 385. 
\bibitem{Bergshoeff:2009aq}
  E.~A.~Bergshoeff, O.~Hohm and P.~K.~Townsend,
  %``More on Massive 3D Gravity,''
  Phys.\ Rev.\ D {\bf 79} (2009) 124042
  [arXiv:0905.1259 [hep-th]].
  %%CITATION = ARXIV:0905.1259;%%
\bibitem{Kleinschmidt:2012rs}
  A.~Kleinschmidt, T.~Nutma and A.~Virmani,
  %``On unitary subsectors of polycritical gravities,''
  Gen.\  Rel.\  Grav.\  {\bf 45} (2013) 727
  [arXiv:1206.7095 [hep-th]].
  %%CITATION = ARXIV:1206.7095;%%
\bibitem{Gullu:2010pc}
  I.~Gullu, T.~C.~Sisman and B.~Tekin,
  %``Born-Infeld extension of new massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 27} (2010) 162001
  [arXiv:1003.3935 [hep-th]].
  %%CITATION = ARXIV:1003.3935;%%
\bibitem{Paulos:2010ke}
  M.~F.~Paulos,
  %``New massive gravity extended with an arbitrary number of curvature corrections,''
  Phys.\ Rev.\ D {\bf 82} (2010) 084042
  [arXiv:1005.1646 [hep-th]].
  %%CITATION = ARXIV:1005.1646;%%
\bibitem{Bach}
  R.~Bach,
  Math.\ Zeitschr.\ {\bf 9} (1921) 110.
  %%CITATION = GRGVA,9,353;%%  
\bibitem{Kaku:1977pa}
  M.~Kaku, P.~K.~Townsend and P.~van Nieuwenhuizen,
  %``Gauge Theory of the Conformal and Superconformal Group,''
  Phys.\ Lett.\ B {\bf 69} (1977) 304.
  %%CITATION = PHLTA,B69,304;%%
\bibitem{Deser:2012qg}
  S.~Deser, E.~Joung and A.~Waldron,
  %``Partial Masslessness and Conformal Gravity,''
  J.\ Phys.\ A (2012)
  [arXiv:1208.1307 [hep-th]].
  %%CITATION = ARXIV:1208.1307;%%
\bibitem{Fradkin:1981iu}
  E.~S.~Fradkin and A.~A.~Tseytlin,
  %``Renormalizable asymptotically free quantum theory of gravity,''
  Nucl.\ Phys.\ B {\bf 201} (1982) 469.
  %%CITATION = NUPHA,B201,469;%%  
\bibitem{Lee:1982cp}
  S.~C.~Lee and P.~van Nieuwenhuizen,
  %``Counting Of States In Higher Derivative Field Theories,''
  Phys.\ Rev.\ D {\bf 26} (1982) 934.
  %%CITATION = PHRVA,D26,934;%%
\bibitem{Riegert:1984hf}
  R.~J.~Riegert,
  %``The Particle Content Of Linearized Conformal Gravity,''
  Phys.\ Lett.\ A {\bf 105} (1984) 110.
  %%CITATION = PHLTA,A105,110;%%
\bibitem{Maldacena:2011mk}
  J.~Maldacena,
  %``Einstein Gravity from Conformal Gravity,''
  arXiv:1105.5632 [hep-th].
  %%CITATION = ARXIV:1105.5632;%%
\bibitem{Mannheim:2011ds}
  P.~D.~Mannheim,
  %``Making the Case for Conformal Gravity,''
  Found.\ Phys.\  {\bf 42} (2012) 388
  [arXiv:1101.2186 [hep-th]].
  %%CITATION = ARXIV:1101.2186;%%  
\bibitem{Bender:2007wu}
  C.~M.~Bender and P.~D.~Mannheim,
  %``No-ghost theorem for the fourth-order derivative Pais-Uhlenbeck oscillator model,''
  Phys.\ Rev.\ Lett.\  {\bf 100} (2008) 110402
  [arXiv:0706.0207 [hep-th]].    
\bibitem{Volkov:2013roa}
  M.~S.~Volkov,
  %``Self-accelerating cosmologies and hairy black holes in ghost-free bigravity and massive gravity,''
  arXiv:1304.0238 [hep-th].
  %%CITATION = ARXIV:1304.0238;%% 
\bibitem{Sjors:2011iv}
  S.~Sjors and E.~Mortsell,
  %``Spherically Symmetric Solutions in Massive Gravity and Constraints from Galaxies,''
  JHEP {\bf 1302} (2013) 080
  [arXiv:1111.5961 [gr-qc]].
  %%CITATION = ARXIV:1111.5961;%%
\bibitem{Enander:2013kza}
  J.~Enander and E.~Mortsell,
  %``Strong lensing constraints on bimetric massive gravity,''
  arXiv:1306.1086 [astro-ph.CO].
  %%CITATION = ARXIV:1306.1086;%%   
\bibitem{Brito:2013yxa}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Partially massless gravitons do not destroy general relativity black holes,''
  Phys.\  Rev.\ D {\bf 87} (2013) 124024
  [arXiv:1306.0908 [gr-qc]].
  %%CITATION = ARXIV:1306.0908;%%   
\bibitem{Gregory:1993vy}
  R.~Gregory and R.~Laflamme,
  %``Black strings and p-branes are unstable,''
  Phys.\ Rev.\ Lett.\  {\bf 70} (1993) 2837
  [hep-th/9301052].
  %%CITATION = HEP-TH/9301052;%% 
\bibitem{Babichev:2013una}
  E.~Babichev and A.~Fabbri,
  %``Instability of black holes in massive gravity,''
  Class.\ Quant.\ Grav.\  {\bf 30} (2013) 152001
  [arXiv:1304.5992 [gr-qc]].
  %%CITATION = ARXIV:1304.5992;%%
\bibitem{Brito:2013wya}
  R.~Brito, V.~Cardoso and P.~Pani,
  %``Massive spin-2 fields on black hole spacetimes: Instability of the Schwarzschild and Kerr solutions and bounds on the graviton mass,''
  Phys.\  Rev.\ D {\bf 88} (2013) 023514
  [arXiv:1304.6725 [gr-qc]].
  %%CITATION = ARXIV:1304.6725;%% 
\bibitem{Hinterbichler:2013eza}
  K.~Hinterbichler,
  %``Ghost-Free Derivative Interactions for a Massive Graviton,''
  arXiv:1305.7227 [hep-th].
  %%CITATION = ARXIV:1305.7227;%% 
\bibitem{Kimura:2013ika}
  R.~Kimura and D.~Yamauchi,
  %``Derivative interactions in de Rham-Gabadadze-Tolley massive gravity,''
  arXiv:1308.0523 [gr-qc].
  %%CITATION = ARXIV:1308.0523;%%  
\bibitem{Huang:2012pe}
  Q.~-G.~Huang, Y.~-S.~Piao and S.~-Y.~Zhou,
  %``Mass-Varying Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124014
  [arXiv:1206.5678 [hep-th]].
  %%CITATION = ARXIV:1206.5678;%% 
\bibitem{Huang:2013mha}
  Q.~-G.~Huang, K.~-C.~Zhang and S.~-Y.~Zhou,
  %``Generalized massive gravity in arbitrary dimensions and its Hamiltonian formulation,''
  arXiv:1306.4740 [hep-th].
  %%CITATION = ARXIV:1306.4740;%%   
\bibitem{Gabadadze:2012tr}
  G.~Gabadadze, K.~Hinterbichler, J.~Khoury, D.~Pirtskhalava and M.~Trodden,
  %``A Covariant Master Theory for Novel Galilean Invariant Models and Massive Gravity,''
  Phys.\ Rev.\ D {\bf 86} (2012) 124004
  [arXiv:1208.5773 [hep-th]].
  %%CITATION = ARXIV:1208.5773;%%
\bibitem{D'Amico:2012zv}
  G.~D'Amico, G.~Gabadadze, L.~Hui and D.~Pirtskhalava,
  %``Quasi-Dilaton: Theory and Cosmology,''
  arXiv:1206.4253 [hep-th].
  %%CITATION = ARXIV:1206.4253;%%   
%\cite{Ondo:2013wka}
\bibitem{Cai:2013lqa}
  Y.~-F.~Cai, F.~Duplessis and E.~N.~Saridakis,
  %``$F(R)$ nonlinear massive gravity and cosmological implications,''
  arXiv:1307.7150 [hep-th].
  %%CITATION = ARXIV:1307.7150;%%  
\bibitem{Nojiri:2013zza}
  S.~'I.~Nojiri and S.~D.~Odintsov,
  %``Accelerating cosmology in modified gravity: from convenient $F(R)$ or string-inspired theory to bimetric $F(R)$ gravity,''
  arXiv:1306.4426 [gr-qc].
  %%CITATION = ARXIV:1306.4426;%% 
\bibitem{deRham:2013qqa}
  C.~de Rham, L.~Heisenberg and R.~H.~Ribeiro,
  %``Quantum Corrections in Massive Gravity,''
  arXiv:1307.7169 [hep-th].
  %%CITATION = ARXIV:1307.7169;%% 
\bibitem{Wald:1984rg}
  R.~M.~Wald,
  %``General Relativity,''
  Chicago, Usa: Univ. Pr. ( 1984) 491p.  
  
  

\end{thebibliography}


